Earn While You Reveal: Private Set Intersection that Rewards Participants

In Private Set Intersection protocols (PSIs), a non-empty result always reveals something about the private input sets of the parties. Moreover, in various variants of PSI, not all parties necessarily receive or are interested in the result. Nevertheless, to date, the literature has assumed that those parties who do not receive or are not interested in the result still contribute their private input sets to the PSI for free, although doing so would cost them their privacy. In this work, for the first time, we propose a multi-party PSI, called "Anesidora", that rewards parties who contribute their private input sets to the protocol. Anesidora is efficient; it mainly relies on symmetric key primitives and its computation and communication complexities are linear with the number of parties and set cardinality. It remains secure even if the majority of parties are corrupted by active colluding adversaries.

==> CCS-24/Acknowledgments-final.tex <==
% !TEX root =main.tex


\section*{Acknowledgements}

Aydin Abadi was supported in part by REPHRAIN: The National Research Centre on Privacy, Harm Reduction and Adversarial Influence Online, under UKRI grant: EP/V011189/1. Steven J. Murdoch was supported by REPHRAIN and The Royal Society under grant UF160505. We would like to thank Yvo Desmedt for his suggestion of having a flexible reward mechanism. 


==> CCS-24/Anesidora-challenges.tex <==
% !TEX root =main.tex


%%%%%%%%%%%%%%%%%
 %%%%%%%%%%%%%



\section{Main Challenges that \withRew Overcomes}\label{sec::Annesidora-challenges}


\subsection{Rewarding Clients Proportionate to the Intersection Size.}
In PSIs, the main private information about the clients that is revealed to a result recipient is the private set elements that the clients have in common. Thus, honest clients must receive a reward proportionate to the intersection cardinality, from a buyer. To receive the reward, the clients need to reach a consensus on the intersection cardinality. The naive way to do that is to let every client find the intersection and declare it to the smart contract. Under the assumption that the majority of clients are honest, then the smart contract can reward the honest result recipient (from the buyer's deposit). But, the honest majority assumption is strong in the context of multi-party PSI. 

Moreover, this approach requires all clients to extract the intersection, which would increase the overall costs.  Some clients may not even be interested in or available to do so. This task could also be conducted by a single entity, such as the dealer; but this approach would introduce a single point of failure and all clients have to depend on this entity.  
%
To address these challenges, we allow any two clients to become extractors.  Each of them finds and sends to the contract the (encrypted) elements in the intersection. The contract compensates them if it determines their honesty. This approach allows us to avoid (i) relying on the assumption of an honest majority, (ii) requiring all clients to find the intersection, and (iii) depending on a single trusted or semi-honest party to perform the task. 






\subsection{Dealing with Extractors' Collusion.}
%


Introducing two extractors brings about another challenge: the possibility of collusion between them (as well as with the buyer) to present a consistent but erroneous result. This kind of behavior cannot be discerned by a verifier unless the verifier consistently undertakes the delegated task themselves, which would defeat the purpose of delegation. To efficiently confront this challenge, we implement counter-collusion smart contracts (as detailed in Section \ref{Counter-Collusion-Smart-Contracts}) that create distrust among the extractors and provide incentives for them to behave honestly. 













 


==> CCS-24/Arbiter-algorithm.tex <==
% !TEX root =main.tex




\begin{figure}[ht]%[!htbp]
\setlength{\fboxsep}{1pt}
\begin{center}
    \begin{tcolorbox}[enhanced,width=3.3in, height=98.2mm,right=.5mm,
    drop fuzzy shadow southwest,
    colframe=black,colback=white]


{\small{
\vspace{-2mm}
%\underline{$\mathtt{Audit}( \vv{{k}},  q, \bm\zeta, \bar d, g, \vv v)\rightarrow (L, \vv{{\mu}})$}
\begin{enumerate}[leftmargin=-.2mm]
%\item[$\bullet$] Parties: clients: $\{  {   A}_{    {    1}},...,   {   A}_{    {    m}}\}$, the dealer and  an Arbiter.


\item[$\bullet$]    {Parties.} A set of clients $\{ A_{\st 1},...,  A_{\st m}\}$ and an external auditor, \aud. 

\item[$\bullet$]    {Input.}  $m$: the total number of participants (excluding the auditor), $\bm\zeta$: a random polynomial of degree $1$, $b$: the total number of vectors, and $adr$: a deployed smart contract's address. Let $b'=b-1$.





%\item[$\bullet$]   {Input.} $\vv{{k}}=[k_{\st 1},..., k_{\st m}]$,    $q$: a  hash value, $\bm\zeta$: a random polynoimal of degree $1$, $\bar d$: a polynoimal's degree,   $g$: a root of Merkle tree, and $\vv v$: binary vector of size $m$. 


\item[$\bullet$]  {Output of  each} $  A_{\st j}$.   $k$: a secret key that generates $b$ vectors $[z_{\scriptscriptstyle 0,1},...,z_{\scriptscriptstyle 0,m}],...,[z_{\scriptscriptstyle b',1},...,z_{\scriptscriptstyle b', m}]$ of pseudorandom values, $h$: hash of the key,  $g$: a Merkle tree's root, and a vector of (signed) messages. 



\item[$\bullet$]    {Output of \aud.} $L$: a list of misbehaving parties' indices, and  $\vv{{\mu}}$: a vector of random polynomials.
%
\item\label{ZSPA::ZSPA-invocation} {\textbf{\zspa invocation.}  $\zspa(\bot,..., \bot)\rightarrow \Big((k, g, q),..., (k, g,q )\Big)$}. 

All parties in $\{A_{\st 1},...,  A_{\st m}\}$ call the same instance of \zspa, which results in  $(k, g, q), ..., (k, g, q)$. 
%

\item\label{ZSPA-A::Auditor-computation}  {\textbf{Auditor computation.} $\mathtt{Audit}(m, \vv{{k}},  q, \bm\zeta, b, g)\rightarrow (L, \vv{{\mu}})$}. 

\aud\ takes the below steps. Note,  each $k_{\st j}\in \vv{{k}}$ is given by  $  A_{\st j}$. An honest party's input, $k_{\st j}$,  equals $k$, where $1\leq j \leq m$. 


\begin{enumerate}[leftmargin=1.3mm]
%
\item runs the checks in the verification phase (i.e., Phase \ref{ZSPA:verify}) of \zspa for every $j$, i.e., $\mathtt{Verify}(k_{\st j}, g, q, m, auditor)\rightarrow (a_{\st j}, s)$.
\item appends $j$ to $L$, if any checks fails, i.e., if $a_{\st j}=0$. In this case, it skips the next two steps for the current $j$. 



%
%
%\item  Checks whether equation $\mathtt{H}(k_{\st j})=q$ holds  for every $j$, $1\leq j \leq m$.   
%%
%\begin{itemize}
%%
%\item[$\bullet$] if any $j$-th check fails,  it adds $j$ to $L$.
%%
%\item[$\bullet$]  if $L$ contains all $j\in[1,m]$, it returns $L$ and aborts. 
%%
%\end{itemize}
%%
%\item\label{zero-sum-arbiter-verification} Verifies the Merkle tree's root, $g$, by checking if the tree (corresponding to  $g$) has been correctly constructed on the correct leaf nodes. In particular, it takes the following steps. 
%
%\begin{enumerate}
%
%\item regenerates the tree's leaf nodes (similar to step \ref{ZSPA:val-gen} in Fig. \ref{fig:ZSPA}) as follows. Let $k$ be a key that passed the above check.  For every $i$ (where $0\leq i \leq \bar d$), it recomputes $m$ pseudorandom values: 
%%
%$$\forall j, 1\leq j \leq m-1: z_{\st i,j}=\mathtt{PRF}(k,i||j), \hspace{4mm} z_{\st i,m}=-\sum\limits^{\st m-1}_{\st j=1}z_{\st i,j}$$
%%
%\item   constructs a Merkel tree on top of all pseudorandom values generated in the previous step, i.e., $\mathtt{MT.genTree}(z_{\st 0,1},...,z_{\st \bar d,m})\rightarrow g'$. 
%%
%\item checks if $g=g'$. If the equation does not hold, then it adds to $L$ every index $j$ whose value in $\vv v$ is $1$, i.e., $\vv v[j]=1$; in this case, it returns $L$ and aborts.
%%
%\end{enumerate}
%

\item\label{ZSPA-A::gen-z} For every $i$ (where $0\leq i \leq b'$), it recomputes $m$ pseudorandom values: 
%
$\forall j, 1\leq j \leq m-1: z_{\st i,j}=\mathtt{PRF}(k,i||j), \hspace{2mm} z_{\st i,m}=-\sum\limits^{\st m-1}_{\st j=1}z_{\st i,j}$.
%
 \item generates polynomial $\bm\mu^{\st (j)}$ as: 
  %
   $\bm\mu^{\st (j)} = \bm\zeta\cdot \bm\xi^{\st (j)}-\bm\tau^{\st (j)}$, 
   %
    where $\bm\xi^{\st (j)}$ is a random polynomial of degree $b'-1$ and $\bm\tau^{\st (j)}=\sum\limits^{\st b'}_{\st i=0}z_{\st i,j}\cdot x^{\st i}$. By this step, a vector $\vv{{\mu}}$ containing at most $m$ polynomials is generated. 
%
 \item returns   list $L$ and $\vv{{\mu}}$.
 
\end{enumerate}
 \end{enumerate}
}}
 \end{tcolorbox}
\end{center}
\vspace{-4mm}
\caption{\zspa with an external auditor (\zspaa).} 
\label{fig:arbiter}
\vspace{-3.5mm}
\end{figure}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}[ht]%[!htbp]
%\setlength{\fboxsep}{1pt}
%\begin{center}
%    \begin{tcolorbox}[enhanced,width=5.5in, 
%    drop fuzzy shadow southwest,
%    colframe=black,colback=white]
%
%
%{\small{
%
%\underline{$\mathtt{Audit}( \vv{{k}},  q, \bm\zeta, \bar d, g, \vv v)\rightarrow (L, \vv{{\mu}})$}
%\begin{enumerate}
%%\item[$\bullet$] Parties: clients: $\{  {   A}_{    {    1}},...,   {   A}_{    {    m}}\}$, the dealer and  an Arbiter.
%\item[$\bullet$]   {Input.} $\vv{{k}}=[k_{\st 1},...,k_{\st m}]$,    $q$: a  hash value, $\bm\zeta$: a random polynoimal of degree $1$, $\bar d$: a polynoimal's degree,   $g$: a root of Merkle tree, and $\vv v$: binary vector of size $m$. 
%
%
%\item[$\bullet$]    {Output.} A list of rejected values' indices: $L$, a vector of random polynomials: $\vv{{\mu}}$.
%%
%\item  Checks whether equation $\mathtt{H}(k_{\st j})=q$ holds  for every $j$, $1\leq j \leq m$.   
%%
%\begin{itemize}
%%
%\item[$\bullet$] if any $j$-th check fails,  it adds $j$ to $L$.
%%
%\item[$\bullet$]  if $L$ contains all $j\in[1,m]$, it returns $L$ and aborts. 
%%
%\end{itemize}
%%
%\item\label{zero-sum-arbiter-verification} Verifies the Merkle tree's root, $g$, by checking if the tree (corresponding to  $g$) has been correctly constructed on the correct leaf nodes. In particular, it takes the following steps. 
%
%\begin{enumerate}
%
%\item regenerates the tree's leaf nodes (similar to step \ref{ZSPA:val-gen} in Fig. \ref{fig:ZSPA}) as follows. Let $k$ be a key that passed the above check.  For every $i$ (where $0\leq i \leq \bar d$), it recomputes $m$ pseudorandom values: 
%%
%$$\forall j, 1\leq j \leq m-1: z_{\st i,j}=\mathtt{PRF}(k,i||j), \hspace{4mm} z_{\st i,m}=-\sum\limits^{\st m-1}_{\st j=1}z_{\st i,j}$$
%%
%\item   constructs a Merkel tree on top of all pseudorandom values generated in the previous step, i.e., $\mathtt{MT.genTree}(z_{\st 0,1},...,z_{\st \bar d,m})\rightarrow g'$. 
%%
%\item checks if $g=g'$. If the equation does not hold, then it adds to $L$ every index $j$ whose value in $\vv v$ is $1$, i.e., $\vv v[j]=1$; in this case, it returns $L$ and aborts.
%%
%\end{enumerate}
%%
% \item Generates polynomial $\bm\mu^{\st (j)}$, for every $j$ such that $j\in[1,m]$ and $j \notin L$,  as follows:
%  %
%   $$\bm\mu^{\st (j)} = \bm\zeta\cdot \bm\xi^{\st (j)}-\bm\tau^{\st (j)}$$
%   %
%    where $\bm\xi^{\st (j)}$ is a random polynomial of degree $\bar d-1$ and $\bm\tau^{\st (j)}=\sum\limits^{\st \bar d}_{\st i=0}z_{\st i,j}\cdot x^{\st i}$. By the end of this step, a vector $\vv{{\mu}}$ containing at most $m$ polynomials is generated. 
%%
% \item Returns   list $L$ and $\vv{{\mu}}$.
% 
%
% \end{enumerate}
%}}
% \end{tcolorbox}
%\end{center}
%\caption{$\text{Audit}$ Algorithm} 
%\label{fig:arbiter}
%\end{figure}


==> CCS-24/Arbiter-protocol.tex <==
% !TEX root =main.tex





\vspace{-2mm}

\subsection{\zspa's Extension: \zspa with an External Auditor (\zspaa)}
\vspace{-1mm}

Now, we present an extension of \zspa, called \zspaa, which lets a (trusted) third-party auditor, \aud, help identify misbehaving clients in the \zspa and generate a vector of random polynomials with a specific structure. Specifically, the functionality that \zspaa computes is defined as 
%
$f^{\st \zspaa}(\underbrace{\bot,..., \bot}_{\st m}, b, \bm\zeta)\rightarrow (\underbrace{(k, g, q),..., (k, g,q)}_{\st m},$ $\bm\mu^{\st (1)},..., \bm\mu^{\st (m)})$, where $g$ is the root of the Markle tree built on the pseudorandom values $z_{\st i, j}$, $q$ is the hash value of the key used to generate the pseudorandom values, $m\geq 2$, $b$ is constant value, $\bm\zeta$ is a random polynomial of degree $1$, each $\bm\mu^{\st (j)} $ has the form $\bm\mu^{\st (j)} = \bm\zeta\cdot \bm\xi^{\st (j)}-\bm\tau^{\st (j)}$,  $\bm\xi^{\st (j)}$ is a random polynomial of degree $b-2$, and $\bm\tau^{\st (j)}=\sum\limits^{\st b-1}_{\st i=0}z_{\st i,j}\cdot x^{\st i}$. 



Informally, \zspaa ensures that misbehaving parties are always detected, except with a negligible probability. \aud of this protocol will be invoked by \withFai when \withFai's smart contract detects that a combination of the messages sent by the clients is not well-formed. Later, in \withFai's proof, we will show that even a \emph{semi-honest} \aud who observes all messages that clients send to \withFai's smart contracts, cannot learn anything about their set elements. We present \zspaa in Figure \ref{fig:arbiter}. 

\vspace{-4.5mm}
\input{Arbiter-algorithm}


\vspace{-2mm}
\begin{theorem}\label{theorem::ZSPA-A}
If\ $\zspa$ is secure, $\mathtt{H}$ is second-preimage resistant, and the correctness of $\mathtt{PRF}$, $\mathtt{H}$, and Merkle tree hold,  then \zspaa securely computes $f^{\st \zspaa}$ in the presence of $m-1 $ malicious adversaries.% or (ii) a semi-honest auditor. 
\end{theorem}

%As we stated previously, the ZSPA-A protocol will be invoked as a subroutine in the fair PSI protocol. As part of proving Theorem \ref{theorem::ZSPA-A}, we would like to show that the semi-honest auditor's view can be simulated (so it cannot learn the parties' set elements), even if it has access to those transcripts of the fair PSI protocol sent to the smart contract; because such an approach offers a stronger security guarantee than proving the ZSPA-A protocol in isolation.  Therefore, we will present the proof of Theorem \ref{theorem::ZSPA-A} after we present the fair PSI protocol. 

\vspace{-1mm}

We refer readers to Appendix \ref{sec::proof-of-zspa-a} for the proof of Theorem \ref{theorem::ZSPA-A}. 




%\begin{theorem}\label{theorem::ZSPA-comp-correctness}
%If the coin-tossing protocol is secure against a malicious adversary, then the ZSPA protocol,  in Figure \ref{fig:ZSPA}, securely computes $f^{\st \text {ZSPA}}$ in the presence of a malicious adversary. 
%\end{theorem}


%\begin{figure}%[ht]
%\setlength{\fboxsep}{0.7pt}
%\begin{center}
%\begin{boxedminipage}{12.3cm}
%
%\small{
%
%\begin{enumerate}
%\item[$\bullet$] Parties: clients: $\{\resizeT {\textit A}_{\resizeS {\textit  1}},..., \resizeT {\textit A}_{\resizeS {\textit  m}}\}$, the dealer and  an Arbiter.
%\item[$\bullet$] Input: Empty malicious clients list: $L$ and a deployed smart contract's address. 
%\item[$\bullet$] Output: Misbehaving clients list: $L$
%\item Every client sends to the Arbiter  two keys: $k_{\scriptscriptstyle 1}, k_{\scriptscriptstyle 2}$, used to generate the zero-sum values and their commitments. 
%%
%\item  The Arbiter checks if the clients  provided correct keys, by ensuring that the keys' hashes matches the ones stored in the contract. It appends the IDs of those  provided inconsistent keys to $L$. If all clients provided inconsistent keys it aborts. Otherwise, it proceed to the next step where it uses correct keys: $k_{\scriptscriptstyle 1}, k_{\scriptscriptstyle 2}$. 
%%
%\item\label{zero-sum-arbiter-verification} The Arbiter (given correct keys) regenerate the  zero-sum values $z_{\scriptscriptstyle i, j}$ and verify the correctness of their commitments and the Merkel tree root contracted on top of the commitments, i.e. takes the same step as step \ref{ZSPA:verify} in Fig \ref{fig:ZSPA}.   It aborts if any of the   checks is rejected, and appends to $L$ the IDs of the clients which sent the ``approved'' message to the contract. 
%%
% \item The Arbiter for each client $\resizeT {\textit C}$, who provided correct keys,  generates polynomial $\bm\mu^{\resizeS {\textit {(C)}}}$, for each bin, as follows:
%  %
%   $$\bm\mu^{\resizeS {\textit {(C)}}} = \bm\zeta\cdot \bm\xi^{\resizeS {\textit {(C)}}}-\bm\tau^{\resizeS {\textit {(C)}}}$$
%   %
%    where $\bm\xi^{\resizeS {\textit {(C)}}}$ is a random polynomial of degree $3d+1$ and $\bm\tau^{\resizeS {\textit {(C)}}}=\sum\limits^{\st 3d+2}_{\st i=0}z_{\st i,c}\cdot x^{\st i}$. By the end of this step, a vector $\vv{\bm{\mu}}$ containing polynomial $\bm\mu^{\resizeS {\textit {(C)}}}$ for every bin of client $\resizeT {\textit C}$ that is not in list $L$. 
%    %
%     \item returns   list $L$ and $\vv{\bm{\mu}}$.
 
%
%
% \item The dealer, for each client $\resizeT {\textit C}\in \{\resizeT {\textit A}_{\resizeS {\textit  1}},..., \resizeT {\textit A}_{\resizeS {\textit  m}}\}$,  sends to the Arbiter a blind polynomial of the form: $\bm\zeta\cdot \bm\eta^{\resizeS {\textit {(D,C)}}}-(\bm\gamma^{\resizeS {\textit {(D,C)}}}+\bm\delta^{\resizeS {\textit {(D,C)}}})$, where $\bm\eta^{\resizeS {\textit {(D,C)}}}$ is a fresh random degree $3d+1$ polynomial. The blind polynomial will allow the arbiter to obliviously verify the correctness of the message each client sent to the  contract. 
% 
% \item The Arbiter for each client $\resizeT {\textit C}$ who provided correct keys: 
% 
% \begin{enumerate}
% \item adds together the blind polynomial above and the blind polynomial $\bm\nu^{\resizeS {\textit {(C)}}}$ the client sent to the contract (in step \ref{blindPoly-C-sends-to-contract} in the PSI protocol). Then, it removes the client's zero-sum pseudorandom values from the result. In particular, it computes:    
%\begin{equation*}
%\begin{split}
% \bm\iota^{\resizeS {\textit {(C)}}}&=\bm\zeta\cdot \bm\eta^{\resizeS {\textit {(D,C)}}}-(\bm\gamma^{\resizeS {\textit {(D,C)}}}+\bm\delta^{\resizeS {\textit {(D,C)}}})+\bm\nu^{\resizeS {\textit {(C)}}}-\sum\limits^{\scriptscriptstyle 3d+1}_{\scriptscriptstyle i=0}z_{\scriptscriptstyle i,c}\cdot x^{\scriptscriptstyle i} \\ &=\bm\zeta\cdot(\bm\eta^{\resizeS {\textit {(D,C)}}} + \bm\omega^{\resizeS {\textit {(D,C)}}}\cdot \bm\omega^{\resizeS {\textit {(C,D)}}}\cdot \bm\pi^{\resizeS {\textit {(C)}}}+\bm\rho^{\resizeS {\textit {(D,C)}}}\cdot \bm\rho^{\resizeS {\textit {(C,D)}}}\cdot \bm\pi^{\resizeS {\textit {(D)}}})
% \end{split}
%\end{equation*}
%  \item checks if $\bm\zeta$ can divide $\bm\iota^{\resizeS {\textit {(C)}}}$. If can not, it appends the client's ID to $L$.
%  \end{enumerate}
  %$deg(\eta^{\resizeS {\textit {D,C}}})=3d+1$
% \end{enumerate}
%}
%\end{boxedminipage}
%\end{center}
%\caption{$\mathtt{Arbiter}$ Protocol} 
%\label{fig:arbiter}
%\end{figure}










==> CCS-24/Colluder-contract.tex <==
% !TEX root =main.tex





\subsection{Colluder's Contract (\SCcc)}

Recall that \SCpc aimed at creating a dilemma between the two servers. However, this dilemma can be addressed if they can make an enforceable promise.  This enforceable promise can be another smart contract, called Colluder's Contract (\SCcc).  This contract imposes additional rules that ultimately would affect the parties’ payoffs and would make collusion the most profitable strategy for the colluding parties. In \SCcc, the party who initiates the collusion would pay its counterpart a certain amount (or bribe) if both follow the collusion and provide an incorrect result of the computation to \SCpc.  Note, \SCcc requires both servers to send a fixed amount of deposit when signing the contract.  The party who deviates from collusion will be punished by losing the deposit. Below, we reiterate the description of \SCcc. 


\begin{enumerate}[leftmargin=5.2mm]
%
\item The contract is signed between the server who initiates the collusion, called ringleader (LDR), and the other server called follower (FLR). 
%
\item The two agree on providing to \SCpc a different result $res'$ than a correct computation of $f$ on $x$ would yield, i.e., $res'\neq f(x)$. Parameter $res'$ is recorded in this contract. 
%
\item LDR and FLR deposit $\tc+\bc$ and $\tc$ amounts in this contract respectively. 
%
\item The above deposit must be paid before the result delivery deadline in \SCpc, i.e., before deadline $T_{\st 2}$. If this condition is not met, the parties' deposit in this contract is refunded and this contract is terminated. 
%
\item When \SCpc is finalized (i.e., all the results have been provided), the following steps are taken.
%
\begin{enumerate}
%
\item \underline{both follow the collusion}: if both LDR and FLR provided $res'$ to \SCpc, then $\tc$ and $\tc+\bc$ amounts are delivered to LDR and FLR respectively. Therefore, FLR receives its deposit plus the bribe, which is $\bc$ amount. 
%
\item \underline{only FLR deviates from the collusion}:  if LDR and FLR provide $res'$ and $res''\neq res'$ to \SCpc respectively, then $2\cdot \tc+\bc$ amount is transferred to LDR while nothing is sent to FLR. 
%
\item \underline{only LDR deviates from the collusion}: if LDR and FLR provide $res''\neq res'$ and $res'$ to \SCpc respectively, then $2\cdot \tc+\bc$ amount is sent to FLR while nothing is transferred to LDR.  
%
\item \underline{both deviate from the collusion}: if LDR and FLR deviate and provide any result other than $res'$ to \SCpc, then  $2\cdot \tc+\bc$ amount is sent to LDR and $\tc$ amount is sent to FLR. 
%
\end{enumerate}
%
\end{enumerate}

The amount of bribe a rational LDR is willing to pay is less than its computation cost (i.e., $\bc<\cc$). Otherwise, this collusion would not offer a higher payoff. We refer readers to \cite{dong2017betrayal} for further discussion. 
























==> CCS-24/Communication-cost.tex <==
% !TEX root =test.tex


\begin{table*}[!htbp]
\begin{footnotesize}
\begin{center}
\caption{\small Total communication costs in bits for different protocols} \label{tbl::update}


\renewcommand{\arraystretch}{1.3}

\begin{tabular}{|c|c|c} 

\hline 
%{\rowcolors{2}{blue!80!gray!18}{blue!10!gray!18}
\cellcolor{gray!20} \scriptsize \textbf{Protocols} &\cellcolor{gray!20}\scriptsize  Communication cost: total number of bits exchanged \\
    \hline
    
    \hline



\cellcolor{white!20}  \scriptsize Our U-PSI:&\cellcolor{white!20}\scriptsize $ u((\textsl{m}-1)(4hd+4h+3)+h(2d+1)+1)+5771h$& \\

   \cellcolor{cyan!20}\scriptsize Using External Trusted Server in \cite{DBLP:conf/scn/InbarOP18}:    &\cellcolor{cyan!20}\scriptsize  $\textsl{m}^{\scriptscriptstyle 2}  |BF| |s_{\scriptscriptstyle i}|$  &\\ 

\cellcolor{white!20}  \scriptsize Semi-honest PSI in \cite{DBLP:conf/scn/InbarOP18}: &\cellcolor{white!20}\scriptsize   $(\textsl{m}^{\scriptscriptstyle 2}-1)  |BF| (k+2|s_{\scriptscriptstyle i}|)$&\\ 


 
    \cellcolor{cyan!20}\scriptsize Basic Semi-honest PSI in \cite{DBLP:conf/pkc/HazayV17}:      &\cellcolor{cyan!20}\scriptsize$(2  \textsl{m} - 1)  |S|  \Upsilon$&\\ 
    
        \cellcolor{white!20}\scriptsize Table-hashing based PSI in \cite{DBLP:conf/ccs/KolesnikovMPRT17}:      &\cellcolor{white!20}\scriptsize$(\textsl{m} +1)(\textsl{m} -1)( k'  (m_{\scriptscriptstyle 1}  \beta_{\scriptscriptstyle 1} + m_{\scriptscriptstyle 2}  \beta_{\scriptscriptstyle 2}) + 500(m_{\scriptscriptstyle 1}+m_{\scriptscriptstyle 2}) )$&\\ 
        
        \cellcolor{cyan!20}\scriptsize  \cite{DBLP:conf/ccs/ChenLR17}:      &\cellcolor{cyan!20}\scriptsize$1.5 \textsl {C}$ $(\textsl{m}-1) |s_{\scriptscriptstyle i}| |S| \log_{\scriptscriptstyle 2}(|S|)$&\\ 


      \cellcolor{white!20}\scriptsize  \cite{DBLP:conf/uss/Pinkas0SZ15}:      &\cellcolor{white!20}\scriptsize $|S|\theta v+k''(1.2|S|+\theta)$&\\ 
      
      
            \cellcolor{cyan!20}\scriptsize  \cite{kamarascaling}:      &\cellcolor{cyan!20}\scriptsize $3.5 u' (\textsl{m}-1)  |S|$&\\ 


       \hline



 %$ |BF|(\textsl{m}-1)((k+2l)+\textsl{m} (k+2l))$

\end{tabular}
\end{center}
\end{footnotesize}
\end{table*}

 %$ |BF|(\textsl{m}-1)((k+2l)+\textsl{m} (k+2l))$



In the above table, $\textsl{m}$: total number of clients, $u$: finite field size or the output size of pseudorandom function (e.g. $32, 64$ or $128$ bits), $d$: a bin capacity, i.e. $d=100$, also $5771$ is bit-length of a bloom filter that encodes $d$ elements with false positive probability of $2^{\scriptscriptstyle -40}$, and $h$: total number of bins. Also $|s_i|$ refers to bit length of the set element, $k$ is security parameter for OT (for simplicity we set $k=|s_i|$). Moreover, $|BF|$ denotes the bit length of bloom filter, e.g. for $2^{\scriptscriptstyle 20}$ elements and $2^{\scriptscriptstyle -40}$ false positive probability $|BF|=57,707,802$ bits. Also, for \cite{DBLP:conf/scn/InbarOP18}, the communication cost of $|BF|$ times invocation of 1-out-of-2 OT, is calculated according to 2\textsuperscript{nd} row in Table 2 in \cite{DBLP:conf/ccs/AsharovL0Z13}. Moreover, $\Upsilon$ denote the minimla bit-size of ciphertext in additive homomorphic encryption, i.e. $\Upsilon\geq 2048$ and $|S|$ is set cardinality. Furthermore,   $k'$ is the bit-length of oblivious programmable pseudorandom function's (OPRF) output, and $m_{\scriptscriptstyle i}, \beta_{\scriptscriptstyle i}$ are parameters of Cuckoo hashing, defined in Table 2 in \cite{DBLP:conf/ccs/KolesnikovMPRT17}, and $500$ refers to the amortized communication cost of each OPRF instance in bits, and $\textsl{C}$ refers to ciphertext expansion, e.g.  when the sets size are $2^{\scriptscriptstyle 20}$, then $\textsl{C}\geq8.67$, according to Table 5 in \cite{DBLP:conf/ccs/ChenLR17}. Furthermore, $\theta$ denotes the stash size in cuckoo hashing and equals $6$, $v$ is the bit-length of the oblivious pseudorandom function's output, $k''$ is the with of the pseudorandom code, $1.2$ is related to cuckoo hashing utilisation and $u'$ is the output size of pseudorandom permutation.


==> CCS-24/Concrete-parameters.tex <==
% !TEX root =main.tex



\subsection{Concrete Parameters}\label{sec::conc-parameters}

\subsubsection{Hash Table Parameters.}


As detailed in Appendix \ref{Preliminary-Hash-Table}, a hash table is characterized by several key parameters:

\begin{itemize}

\item[$\bullet$] $h$: the number of bins.

\item[$\bullet$] $d$: the maximum size (or capacity) of each bin.

\item[$\bullet$] $c$: the maximum number of elements that are mapped to the hash table.

\item[$\bullet$] $pr$: the probability that the number of elements mapped to a bin does not exceed a predefined capacity.
 
 \end{itemize}
 
 It is important to note that in the context of PSI, the parameter $c$ represents the maximum of the sizes of all sets involved. 
 
 The literature, as evidenced in sources such as \cite{Feather2020-full,DBLP:conf/ccs/KolesnikovMPRT17,DBLP:conf/uss/Pinkas0SZ15}) has extensively examined the specific parameters of a hash table, even within the context of PSI. For instance, as illustrated in Section 6 and Appendix J.1 of \cite{Feather2020-full}, when $c$ falls within the range of  $[2^{\st 10},\ 2^{\st 20}]$ and $pr$ is set to $2^{\st -40}$, then $d$ is $100$. Furthermore, we have $h\approx\frac{4c}{d}$. To provide a concrete value, when $c=2^{\st 20}$ and $d=100$, we would have $h=41943$. 




\subsubsection{Field Size.} 
%
In this paper, all arithmetic operations are defined over a finite field $\mathbb{F}_{\st p}$, where $\log_{\st 2}(p)=\lambda$ represents the security parameter. The outputs of $\mathtt {PRF}(.)$ and  $\mathtt {PRP}(.) $ are also of size $\lambda$. Concrete value of $\lambda$ can be set based on the maximum bit size of set elements. For instance, one can choose $\lambda = 60$, when the maximum bit size of set elements is slightly less than $60$ or  $\lambda = 128$ if it is slightly less than $128$. 






==> CCS-24/E-PSI-proof.tex <==
% !TEX root =main.tex


\section{Proof of \epsi}\label{sec::E-PSI-proof}



In this section, we prove Theorem \ref{theorem::E-PSI-security}, i.e., the security of \epsi. 


\begin{proof}
%
We prove the theorem by considering the case where each party is corrupt, at a time.



%\noindent\textbf{Case 1: Corrupt $m-3$ clients in $\{  {  A}_{ \st {   1}}, ...,   {  A}_{ \st {   m}}\}\setminus\{E_{\st 1},E_{\st 2}\}$}.  Let $G$ be a set of at most $m-3$ corrupt clients, where $G\subset \{  {  A}_{ \st {   1}}, ...,   {  A}_{ \st {   m}}\}\setminus\{E_{\st 1},E_{\st 2}\}$. Let set $\hat G$ be a set of honest clients excluding the (dealer and) extractors, i.e., $\hat G=\{  {  A}_{ \st {   1}}, ...,   {  A}_{ \st {   m}}\}\setminus\{G,E_{\st 1},E_{\st 2}\}$. Also, let $\mathsf{Sim}^{\st\text{E-PSI}}_{\st A_{\st j}}$ be the simulator, which uses a subroutine adversary, $\mathcal{A}_{\st A_{\st j}}$.  Next, we explain how $\mathsf{Sim}^{\st \text{E-PSI}}_{\st _{\st A_{\st j}}}$, which receives the input sets of honest dealer client $D$ and honest client(s) in $\hat G$,  works. 

\

\noindent\textbf{Case 1: Corrupt extractors $\{A_{\st 1}, A_{\st 2}\}$ and $m-3$ clients in $\{  {  A}_{ \st {   3}}, ...,$ $   {  A}_{ \st {   m}}\}$}.  Let set $G$ include extractors $\{A_{\st 1}, A_{\st 2}\}$ and a set of at most $m-3$ corrupt clients in $\{  {  A}_{ \st {   3}}, ...,   {  A}_{ \st {   m}}\}$. Let set $\hat G$ be a set of honest clients in  $\{  {  A}_{ \st {   3}}, ...,   {  A}_{ \st {   m}}\}$. Also, let $\mathsf{Sim}^{\st\epsi}_{\st A}$ be the simulator. We allow the simulator to interact with (i) active adversary  $\mathcal{A}'$ that may corrupt $m-3$ clients in $\{  {  A}_{ \st {   3}}, ...,   {  A}_{ \st {   m}}\}$, and (ii) two rational adversaries  $\mathcal{A}'':=(\mathcal{A}_{\st 1}, \mathcal{A}_{\st 2})$ that corrupt extractors $(A_{\st 1},A_{\st 2})$ component-wise.  
%
%We let $\mathcal{A}:=(\mathcal{A}', \mathcal{A}'')$. 
%
In the simulation, before the point where the extractors are invoked to provide proofs and results, the simulator directly deals with active adversary  $\mathcal{A}'$. However, when the extractors are involved (to generate proofs and extract the result) we require the simulator to interact with each rational adversary $\mathcal{A}_{\st 1}$ and $\mathcal{A}_{\st 2}$.  We allow these two subroutine adversaries $(\mathcal{A}', \mathcal{A}'')$  to internally interact with each other.  Now, we explain how $\mathsf{Sim}^{\st \epsi}_{\st A}$, which receives the input sets of honest dealer $D$ and honest client(s) in $\hat G$,  works. 



\begin{enumerate}
%
\item constructs and deploys two smart contracts (for \fpsi and \epsi). It sends the contracts' addresses to $\mathcal{A}'$.  It also simulates \ct and receives the output value, $ {mk}$, from its functionality, $f_{\st \ct}$.
%
\item\label{sim::case1-buyer-deposit} deposits $S_{\st min}\cdot \vc$ amount to $\mathcal{SC}_{\st\epsi}$  if buyer $A_{\st m}$ is honest, i.e.,  $A_{\st m}\in \hat G$. Otherwise, $\mathsf{Sim}^{\st \epsi}_{\st _{\st A}}$ checks if  $\mathcal{A}'$ has deposited $\Smin\cdot \vc$ amount in $\mathcal{SC}_{\st\epsi}$. If the check fails, it instructs the ledger to refund the coins that every party deposited and sends message $abort_{\st 1}$ to TTP (and accordingly to all parties); it outputs whatever $\mathcal{A}'$ outputs and then halts.


%it aborts if $\mathcal{A}'$ has not deposited enough coins. 
%
\item\label{e-psi::deploy-prisoners} constructs and deploys a (Prisoner's) contract and transfers $\wc=\Smin\cdot \rc$  amount for each extractor. $\mathsf{Sim}^{\st \epsi}_{\st A}$ ensures that each extractor deposited $\dc'=\dc+\Smin\cdot \fc$ coins in this contract; otherwise, it instructs the ledger to refund the coins that every party deposited and sends message $abort_{\st 1}$ to TTP; it outputs whatever $\mathcal{A}'$ outputs and then halts.

 
%
\item encrypts $ mk$ under the public key of the dispute resolver;  let $ct_{\st {mk}}$ be the resulting ciphertext.   It also generates a commitment of ${mk}$ as follows: $ com_{\st {mk}}=\comcom({mk}, \mathtt{PRF}({mk}, 0))$. It stores $ct_{\st {mk}}$  and ${com}_{\st {mk}}$ in $\mathcal{SC}_{\st\epsi}$. 
%
\item  simulates \ct again and receives the output value $ {mk}'$ from  $f_{\st \ct}$.

\item\label{sim::case1-merkle-tree-root} receives from $\mathcal{A}'$ a Merkle tree's root $g'$ for each extractor. 


\item\label{sim::case1-F-PSI} simulates the steps of \ref{ZSPA}--\ref{compute-res-poly} in \fpsi. For completeness, we include the steps that the simulator takes in this proof. Specifically, $\mathsf{Sim}^{\st \epsi}_{\st _{\st A}}$:

\begin{enumerate}
\item\label{sim::E-PSI-ZSPA-A-invocation-} simulates \zspaa for each bin and receives the output value $( k,  g,  q)$ from $f^{\st \zspaa}$.
%
\item deposits in the contract the  amount of $\yc'=\Smin\cdot \vc+\chc$ for client $D$ and each honest client in $\hat G$. It sends to $\mathcal{A}'$ the amount deposited in the contract. 
%
\item\label{sim::case1-check-Adv-deposited-y.|G|}  checks if $\mathcal{A}'$ has deposited $\yc'\cdot |G|$ amount (in addition to $\dc'$ amount deposited in step \ref{e-psi::deploy-prisoners} above). If the check fails, it instructs the ledger to refund the coins that every party deposited and sends message $abort_{\st 1}$ to TTP (and accordingly to all parties); it outputs whatever $\mathcal{A}'$ outputs and then halts.
%
\item picks a random polynomial ${\bm\zeta}$ of degree $1$, for each bin. $\mathsf{Sim}^{\st \epsi}_{\st A}$, for each client $  {  C}\in \{  {  A}_{ \st {   1}}, ...,   {  A}_{ \st {   m}}\}$ allocates to each bin two degree $d$ random polynomials: (${\bm\omega}^{ \st {  {(D,C)}}}, {\bm\rho}^{ \st {  {(D,C)}}}$), and   two  degree $3d+1$ random polynomials: (${\bm\gamma}^{ \st {  {(D,C)}}}$, ${\bm\delta}^{ \st {  {(D,C)}}}$). Also, $\mathsf{Sim}^{\st \epsi}_{\st A}$ for each honest client $C'\in \hat G$, for each bin, picks two  degree $d$ random polynomials: (${\bm\omega}^{ \st {  {(C',D)}}}$, ${\bm\rho}^{ \st {  {(C',D)}}}$). 

\item\label{E-PSI::sim-A-first-VOPR-invocation} simulates \vopr using inputs ${\bm\zeta} \cdot {\bm\omega}^{ \st {  {(D,C)}}}$ and ${\bm\gamma}^{ \st {  {(D,C)}}}$ for each bin. It receives the inputs of clients $C''\in G$, i.e., ${\bm\omega}^{ \st {  {(C'',D)}}}\cdot {\bm\pi}^{ \st {  {(C'')}}}$, from its functionality $f^{\st \vopr}$, for each bin.  
%
\item extracts the roots of polynomial ${\bm\omega}^{ \st {  {(C'',D)}}}\cdot {\bm\pi}^{ \st {  {(C'')}}}$ for each bin and appends those roots that are in the sets universe to a new set $S^{\st(C'')}$. 
%
\item simulates again \vopr using inputs ${\bm\zeta}\cdot {\bm \rho}^{ \st {  {(D,C)}}}\cdot {\bm\pi}^{ \st {  {(D)}}}$ and ${\bm\delta}^{ \st {  {(D,C)}}}$, for each bin.
%
\item sends to TTP the input sets of all parties; specifically, (i) client $D$'s input set: $S^{\st (D)}$, (ii) honest clients' input sets: $S^{\st (C')}$ for all $C'$ in $\hat G$, and (iii) $\mathcal{A}'$'s input sets: $S^{\st(C'')}$, for all $C''$ in $G$.  For each bin, it receives the intersection set, $S_{\st\cap}$, from TTP. 
%
\item represents the intersection set for each bin as a polynomial, ${\bm \pi}$, as follows. First, it encrypts each element $s_{\st i}$ of $S_{\st\cap}$ as $e_{\st i}=\mathtt{PRP}({mk}', s_{\st i})$. Second, it encodes each encrypted element as $\bar{e}_{\st i} =e_{\st i} || \mathtt{H}(e_{\st i})$. Third, it constructs ${\bm \pi}$ as ${\bm \pi}=\prod\limits^{\st |S_{\st\cap}|}_{\st i=1 }(x-s_{\st i})\cdot \prod\limits^{\st d-|S_{\st\cap}|}_{\st j=1 }(x-u_{\st j})$, where $u_{\st j}$ is a dummy value. 
%
\item constructs polynomials ${\bm\theta}^{ \st {  {(C')}}}_{\st 1}={\bm\zeta} \cdot {\bm\omega}^{ \st {  {(D,C')}}}\cdot {\bm\omega}^{ \st {  {(C',D)}}}\cdot {\bm\pi}+ {\bm\gamma}^{ \st {  {(D,C')}}}, {\bm\theta}^{ \st {  {(C')}}}_{\st 2}= {\bm\zeta} \cdot {\bm\rho}^{ \st {  {(D,C')}}}\cdot {\bm\rho}^{ \st {  {(C',D)}}}\cdot {\bm\pi}+ {\bm\delta}^{ \st {  {(D,C')}}}$, and $ {\bm\nu}^{ \st {  {(C')}} }=  {\bm\theta}^{ \st {  {(C')}}}_{\st 1}+ {\bm\theta}^{ \st {  {(C')}}}_{\st 2}+ {\bm \tau}^{ \st {  {(C')}} }$, for each bin and each honest client $C'\in\hat G$, such that $ {\bm\tau}^{ \st {  {(C)}}}=\sum\limits^{\st 3d+2}_{\st i=0}z_{\st i,c}\cdot x^{\st i}$ and each value $z_{\st i,c}$ is derived from key $ k$ generated in step \ref{sim::E-PSI-ZSPA-A-invocation-}.  It sends to $\mathcal{A}'$ polynomial  $ {\bm\nu}^{ \st {  {(C')}} }$ for each bin and each honest client $C'\in\hat G$. 
%
\item\label{E-PSI::sim-A-receive-nu-from-adv} receives ${\bm\nu}^{ \st {  {(C'')}} }$  from $\mathcal{A}'$, for each bin and each corrupt client $C''\in G$. It checks whether the output for every $C''$ has been provided. Otherwise, it halts. 
%
\item if there is any abort within steps \ref{E-PSI::sim-A-first-VOPR-invocation}--\ref{E-PSI::sim-A-receive-nu-from-adv}, then it sends $abort_{\st 2}$ to TTP and instructs the ledger to refund the coins that every party deposited.  It outputs whatever $\mathcal{A}'$ outputs and then halts. 
%
\item constructs polynomial  ${\bm\nu}^{ \st {  {(D)}}}={\bm\zeta} \cdot  {\bm\omega'}^{ \st {  {(D)}}}\cdot {\bm\pi} - \sum\limits^{ \st {   A}_{ \st {   m}}}_{  \st {  {C }= }  \st {   A}_{ \st {  1}}}({\bm\gamma}^{ \st {  {(D,C)}}} + {\bm\delta}^{ \st {  {(D,C)}}}) + {\bm\zeta} \cdot {\bm\gamma'}$ for each bin on behalf of client $D$, where ${\bm\omega'}^{ \st {  {(D)}}}$ is a fresh random polynomial of degree $d$ and ${\bm\gamma'}$ is a pseudorandom polynomial derived from $ {mk}$.
%
\item sends to $\mathcal{A}'$ polynomials ${\bm\nu}^{ \st {  {(D)}}}$ and ${\bm\zeta}$ for each bin. 
%
\item\label{sim::case1-sim-check-res} computes polynomial $ {\bm\phi'}$ as $ {\bm\phi'} = \sum\limits_{\st \forall C''\in G}{\bm\nu}^{ \st {  {(C'')}} }- \sum\limits_{\st \forall C''\in G}({\bm\gamma}^{ \st {  {(D,C'')}}} + {\bm\delta}^{ \st {  {(D,C'')}}})$, for every bin. Next, it checks if  ${\bm\zeta}$  divides ${\bm\phi'}$, for every bin. If the check passes, it sets $Flag=True$. Otherwise, it sets $Flag=False$. 
%
\item if $Flag=True$, then instructs the ledger to send back each party's deposit, i.e., $\yc'$ amount. It sends a message $deliver$ to TTP.  It proceeds to step \ref{sim::case1-what-adv-extract-sends} below. 

 %
\item if $Flag=False$: 
\begin{enumerate}
%
 \item receives $|G|$ keys of the $\mathtt{PRF}$ from $\mathcal{A}'$, i.e., $\vv k'=[  k'_{\st 1}, ...,$ $  k'_{\st |G|}]$, for every bin. %, which should be the output of $f^{\st \text{ZSPA-A}}$ in step \ref{sim::ZSPA-A-invocation} above. 
 %
\item checks if $ k'_{\st j}= k$, for every $ k'_{\st j}\in\vv k'$. Recall,  $ k$ was generated in step \ref{sim::ZSPA-A-invocation}. It constructs an empty list $ L'$ and appends to it the indices (e.g., $j$) of the keys that do not pass the above check. 
 %
 \item receives from $f^{\st \zspaa}$ the output containing a vector of random polynomials, $\vv{\mu}'$, for each valid key. 
 %
 \item sends to  $\mathcal{A}'$, $ L'$ and $\vv{\mu}'$, for every bin. 
 %
 \item  for each bin of client $  {  C}$ whose index is not in $ L'$ computes polynomial ${\bm\chi}^{ \st {  {(D, C)}}}$ as
 %
 ${\bm\chi}^{ \st {  {(D, C)}}}={\bm\zeta}\cdot {\bm\eta}^{ \st {  {(D,C)}}}-({\bm\gamma}^{ \st {  {(D,C)}}}+{\bm\delta}^{ \st {  {(D,C)}}})$,   where ${\bm\eta}^{ \st {  {(D,C)}}}$ is a fresh random polynomial of degree $3d+1$. Note that  $C$ includes both honest and corrupt clients, except those clients whose index is in  $ L'$. $\mathsf{Sim}^{\st \epsi}_{\st A}$ sends every polynomial ${\bm\chi}^{ \st {  {(D, C)}}}$ to  $\mathcal{A}'$. 
 %
 \item\label{sim::case1-check-final-res-for-each-client} given each ${\bm\nu}^{ \st {  {(C'')}} }$ (by $\mathcal{A}'$ in step \ref{E-PSI::sim-A-receive-nu-from-adv}), computes polynomial $ {\bm\phi'}^{ \st {  {(C'')}} }$ as follows: ${\bm\phi'}^{ \st {  {(C'')}} } = {\bm\nu}^{ \st {  {(C'')}} }- {\bm\gamma}^{ \st {  {(D,C'')}}} - {\bm\delta}^{ \st {  {(D,C'')}}}$, for every bin.  $\mathsf{Sim}^{\st \epsi}_{\st A}$ checks if  ${\bm\zeta}$  divides $ {\bm\phi'}^{ \st {  {(C'')}} }$, for every bin. It appends the index of those clients that did not pass the above check to a new list, $ L''$. 
 %
 \item if  $ L'$ or $ L''$ is not empty, then instructs the ledger: (a) to refund $\yc'$ amount to each  client whose index is not in $ L'$ and $ L''$, (b) to retrieve $\chc$ amount from the adversary (i.e., one of the parties whose index is in one of the lists) and send the $\chc$ amount to \aud, and (c) to reward and compensate each honest party (whose index is not in the two lists)  $\frac{m'\cdot \yc'-\chc}{m-m'}$ amount, where $m'=| L'|+| L''|$.  Then, it sends message $abort_{\st 3}$ to TTP. 
%
\item outputs whatever $\mathcal{A}'$ outputs and halts.
 %
 \end{enumerate}
 \end{enumerate}
%
\item\label{sim::case1-what-adv-extract-sends}  for each $I\in \{1,2\}$, receives from $\mathcal{A}_{\st I}$ (1) a set $E^{\st (I)}$ of encoded encrypted elements, e.g., $\bar e_{\st i}$, in the intersection, (2) each $\bar e_{\st i}$'s commitment $com_{\st i,j}$, (3) each $com_{\st i,j}$'s opening $\hat{x}'$, (4) a proof $h_{\st i}$ that each $com_{\st i,j}$ is a leaf node of a Merkle tree with root $g'$ (given to simulator in step \ref{sim::case1-merkle-tree-root} above), and (5) the opening $\hat x$ of commitment  $com_{\st {mk}}$.
%
\item encrypts each element $s_{\st i}$ of $S_{\st\cap}$ as $e_{\st i}=\mathtt{PRP}({mk}', s_{\st i})$. Then, it encodes each encrypted element as $\bar{e}_{\st i} =e_{\st i} || \mathtt{H}(e_{\st i})$. Let set $S'$ include all encoded encrypted elements in the intersection.
%
\item\label{sim::case1-traitor-cont} sings a \SCtc with $\mathcal{A}_{\st I}$, if $\mathcal{A}_{\st I}$ decides to be a traitor extractor. In this case, $\mathcal{A}_{\st I}$, provides the intersection to \SCtc.  $\mathsf{Sim}^{\st \epsi}_{\st A}$ checks this intersection's validity. Shortly (in step \ref{sim::case1-both-cheated-traitor-correct-res}), we will explain how $\mathsf{Sim}^{\st \epsi}_{\st A}$ acts based on the outcome of this check. 
%
\item\label{sim::case1-check-result-correctness} checks if each set $E^{\st (I)}$ equals set $S'$. 
%
\item checks if $com_{\st i,j}$ matches the opening $\hat{x}'$ and the opening corresponds to a unique element in $S'$. 
%
\item\label{sim::case1-ver-Merkle-tree-proof} verifies each commitment's proof, $h_{\st i}$. Specifically, given the proof and root $g$, it ensures the commitment $com_{\st i,j}$  is a leaf node of a Merkle tree with a root node $g'$. It also checks whether the opening $\hat x$ matches $com_{\st {mk}}$. 
%
%\item if any of the checks in steps \ref{sim::case1-check-result-correctness}-\ref{sim::case1-ver-Merkle-tree-proof} fail, it aborts.
%
\item \label{sim::case1-all-check-pass} if all the checks in steps \ref{sim::case1-check-result-correctness}--\ref{sim::case1-ver-Merkle-tree-proof} pass, then instructs the ledger (i) to take $|S_{\st\cap}|\cdot m\cdot \lc$ amount from the buyer's deposit and distributes it among all clients, except the buyer, (ii) to return the extractors deposit (i.e., $\dc'$ amount each) and pay each extractor $|S_{\st\cap}|\cdot \rc$ amount, and (iii) to return $(\Smin-|S_{\scriptscriptstyle\cap}|)\cdot \vc$ amount to the buyer.
%
\item \label{sim::case1-no-result} if neither extractor sends the extractor's set intersection $(E^{\st (A_{\st 1})}, E^{\st (A_{\st 2})})$  in step \ref{sim::case1-what-adv-extract-sends}, then instructs the ledger  (i) to refund the buyer, by sending $\Smin\cdot \vc$ amount back to the buyer and (ii) to
 retrieve each extractor's deposit (i.e., $\dc'$ amount) from \SCpc and distribute it among the rest of the clients (except the buyer and extractors).  
%
\item if the checks in step \ref{sim::case1-all-check-pass} fail or in step  \ref{sim::case1-no-result} both $\mathcal{A}_{\st 1}$  and $\mathcal{A}_{\st 2}$ send the extractors' set intersection but they are inconsistent with each other, then it tags the extractor whose proof or set intersection was invalid as a misbehaving extractor. $\mathsf{Sim}^{\st \epsi}_{\st A}$ instructs the ledger to pay the auditor (of \SCpc) the total amount of $\chc$ coins taken from the misbehaving extractor(s) deposit. Furthermore, $\mathsf{Sim}^{\st \epsi}_{\st A}$ takes the following steps. 
%
\begin{enumerate}
\item\label{sim::case1-both-cheated-no-traitor} if both extractors cheated and there is no traitor, then instructs the ledger (i) to refund the buyer $\Smin\cdot \vc$ amount, and (ii) to take $2 \dc'-\chc$ amount from the misbehaving extractors'  deposit and distribute it to the rest of the clients except the buyer and extractors. 
%
\item\label{sim::case1-both-cheated-traitor-correct-res} if both extractors cheated, there is a traitor, and the traitor delivered a correct result (in step \ref{sim::case1-traitor-cont}), then instructs the ledger (i) to take $\dc'-\dc$ amount from the other misbehaving extractor's deposit and distribute it among the rest of the clients (except the buyer and dishonest extractor), (ii) to distribute $|S_{\st\cap}|\cdot \rc+\dc'+\dc-\chc$ amount to the traitor, (iii) to refund the traitor  $\chc$ amount, and (iv) to refund the buyer $\Smin\cdot \vc-|S_{\st\cap}|\cdot \rc$ amount. 
%
\item if both extractors cheated, there is a traitor, and the traitor delivered an incorrect result (in step \ref{sim::case1-traitor-cont}), then instructs the ledger to distribute coins the same way it does in step \ref{sim::case1-both-cheated-no-traitor}. 
%
\item if one of the extractors cheated and there is no traitor, then instructs the ledger (i) to return the honest extractor’s deposit (i.e., $\dc'$ amount), (ii) to pay the honest extractor $|S_{\st\cap}|\cdot \rc$ amount,  (iii)  to pay this extractor $ \dc-\chc$ amount taken from the dishonest extractor's deposit, and (iv) to pay the buyer and the rest of the clients the same way it does in step \ref{sim::case1-both-cheated-traitor-correct-res}. 
%
\item if one of the extractors cheated, there is a traitor, and the traitor delivered a correct result (in step \ref{sim::case1-traitor-cont}), then instructs the ledger (i) to return the other honest extractor's deposit (i.e., $\dc'$ amount), (ii) to pay the honest extractor $|S_{\st\cap}|\cdot \rc$ amount, taken from the buyer's deposit,  (iii) to pay the honest extractor $\dc- \chc$ amount, taken from the traitor's deposit,   (iv) to pay to the traitor $|S_{\st\cap}|\cdot \rc$ amount, taken from the buyer’s deposit,  (v) to refund the traitor $\dc'-\dc$ amount, (vi) to refund the traitor $\chc$ amount,  (vii) to take $|S_{\st\cap}|\cdot m\cdot \lc$ amount from the buyer's deposit and distribute it among all clients, except the buyer, and (viii) to return $(\Smin-|S_{\scriptscriptstyle\cap}|)\cdot \vc$ amount back  to the buyer. 
%
\item if one of the extractors cheated, there is a traitor, and the traitor delivered an incorrect result (in step \ref{sim::case1-traitor-cont}), then instructs the ledger (i) to pay the honest extractor the same way it does in step \ref{one-cheated-exists-traitor-honest-traitor}, (ii) to refund the traitor  $\chc$ amount, and (iii)  to pay the buyer and the rest of the clients in the same way it does in step \ref{sim::case1-both-cheated-traitor-correct-res}.
%
\item outputs whatever $\mathcal{A}$ outputs and then halts.
%
\end{enumerate}
%
\end{enumerate}



Next, we demonstrate that the real and ideal models are computationally indistinguishable. Initially, we focus on the adversary’s output. The addresses of the smart contracts have identical distribution in both models. In the real and ideal models, the adversary sees the transcripts of ideal calls to $f_{\st \ct}$ as well as the functionality outputs ($mk,  mk'$). Due to the security of \ct (as we are in the $f_{\st \ct}$-hybrid world), the transcripts of $f_{\st \ct}$ in both models have identical distribution, so have the random outputs of $f_{\st \ct}$, i.e., ($mk,  mk'$). Furthermore, the deposit amounts $\Smin\cdot \vc$ and $\wc$ have identical distributions in both models. 

Due to the semantical security of the public key encryption, the ciphertext $ct_{\st mk}$ in the real model is computationally indistinguishable from the ciphertext $ct_{\st {mk}}$ in the ideal model. Due to the hiding property of the commitment scheme, commitment $com_{\st mk}$ in the real model is computationally indistinguishable from commitment $com_{\st {mk}}$ in the ideal model.  

Furthermore, due to the security of \fpsi, all transcripts and outputs produced in the ideal model, in step \ref{sim::case1-F-PSI} on page \pageref{sim::case1-F-PSI}, have identical distribution to the corresponding transcripts and outputs produced in \fpsi in the real model.  
%
The address of \SCtc has the same distribution in both models. The amounts each party receives in the real and ideal models are the same, except when both extractors produce an identical and incorrect result (i.e., intersection) in the real model, as we will shortly discuss, this would not occur under the assumption that the extractors are rational and due to the security of the counter collusion smart contracts.

Now, we demonstrate that an honest party aborts with the same probability in the real and ideal models. As before, for the sake of completeness, we include the \fpsi in the following discussion as well.  Due to the security of \ct, an honest party, during \ct invocation, aborts with the same probability in both models; in this case, the adversary learns nothing about the parties' input set and the sets' intersection as the parties have not sent out any encoded input set yet. In both models, an honest party can read the smart contract and check if sufficient amounts of coins have been deposited. 

Thus, it would halt with the same probability in both models.  If the parties halt because of insufficient amounts of deposit, no one could learn about (i) the parties' input set and (ii) the sets' intersection because the inputs (representation) have not been dispatched at this point.  Due to the security of \zspaa, an honest party during \zspaa execution aborts with the same probability in both models.  In this case, an aborting adversary also learns nothing about the parties' input set and the sets' intersection. %Since all parties' deposit is public, an honest party can read from the smart contract and detect if not all parties have deposited a sufficient amount with the same probability in both models. 




Due to the security of \vopr, honest parties abort with the same probability in both models. In the case where a party aborts during the execution of \vopr, the adversary would learn nothing (i) about its counter party's input set, and (ii) about the rest of the honest parties' input sets and the intersection as the other parties' input sets remain blinded by random blinding factors known only to client $D$.

In the real model, client $D$ can check if all parties provided their encoded inputs via reading the state of the smart contract.  The simulator can perform the same check to ensure  $\mathcal{A}'$ has provided the encoded inputs of all corrupt parties. Hence, in both models, an honest party with the same probability detects if not all encoded inputs have been provided. In this case, if an adversary aborts and does not provide its encoded inputs (i.e., polynomials ${\bm\nu}^{ \st {  {(C'')}} }$), then it learns nothing about the honest parties' input sets and the intersection, for the same reason explained above. 



In the real model,  the contract sums every client $C$'s polynomial $\bm\nu^{ \st {  {(C)}} }$ with each other and with client $D$'s polynomial $\bm\nu^{ \st {  {(D)}} }$, that ultimately removes the blinding factors that  $D$ initially inserted (during the \vopr execution), and then checks if the result is divisible by  $\bm \zeta$. Due to the following reasons the contract can detect if a set of outputs of \vopr were tampered with, with a probability at least $1-\negl(\lambda)$: (a) Theorem \ref{Unforgeable-Polynomials-Linear-Combination}, (b) the fact that the smart contract is given the random polynomial $\bm \zeta$ in plaintext, (c) no party (except honest $D$) knew polynomial $\bm \zeta$ before they send their input to the contract, and (d) the security of the contract, i.e., the adversary cannot influence the correctness of the smart contract's verifications.



In the ideal model, in step \ref{sim::case1-sim-check-res} on page \pageref{sim::case1-sim-check-res}, $\mathsf{Sim}^{\st \epsi}_{\st A}$  can remove the blinding factors and it knows the random polynomial ${\bm \zeta}$. Therefore, $\mathsf{Sim}^{\st \epsi}_{\st A}$ can detect when $\mathcal{A}'$ tampers with a set of the outputs of \vopr (sent to  $\mathsf{Sim}^{\st \epsi}_{\st A}$) with a probability at least $1-\negl(\lambda)$,  due to Theorem \ref{Unforgeable-Polynomials-Linear-Combination}. This means that the smart contract in the real model and the simulator in the ideal model would abort with a similar probability. 




Due to the security of \zspaa, the probability that in the real model an invalid $k_{\st i}\in \vv{k}$ is appended to $ L$ is similar to the probability that  $\mathsf{Sim}^{\st \epsi}_{\st A}$ detects an invalid $ k'_{\st i}\in \vv{k'}$ in the ideal model. In the real model, when $Flag=False$, the smart contract can identify each ill-structured output of \vopr (i.e.,  $\bm\nu^{ \st {  {(C)}} }$) with a probability of at least $1-\negl(\lambda)$ by checking whether $\bm\zeta$  divides $\bm\iota^{ \st {  {(C)}}}$, due to  (a) Theorem \ref{proof::unforgeable-poly} (i.e., unforgeable polynomial), (b) the fact that the smart contract is given $\bm \zeta$ in plaintext, (c) no party (except honest client $D$) knew anything about $\bm \zeta$ before they send their input to the contract, and (d) the security of the contract.  

In the ideal model, when $Flag=False$, given each ${\bm\nu}^{ \st {  {(C'')}} }$, $\mathsf{Sim}^{\st \epsi}_{\st A}$ can remove its blinding factors from  ${\bm\nu}^{ \st {  {(C'')}} }$ which results in $ {\bm\phi'}^{ \st {  {(C'')}} }$ and then can check if ${\bm\zeta}$  divides $ {\bm\phi'}^{ \st {  {(C'')}} }$, in step \ref{sim::case1-check-final-res-for-each-client} on page \pageref{sim::case1-check-final-res-for-each-client}. $\mathsf{Sim}^{\st \epsi}_{\st A}$ can detect an ill-structured  ${\bm\nu}^{ \st {  {(C'')}} }$ with a probability of at least $1-\negl(\lambda)$, due to Theorem \ref{proof::unforgeable-poly}, the fact that the simulator is given ${\bm \zeta}$ in plaintext,  and the adversary is not given any knowledge about ${\bm \zeta}$ before it sends to the simulator the outputs of \vopr.  Therefore, the smart contract in the real model and $\mathsf{Sim}^{\st \epsi}_{\st A}$ in the ideal model can detect an ill-structured input of an adversary with the same probability.  

The smart contract in the real model and $\mathsf{Sim}^{\st \epsi}_{\st A}$ in the ideal model can detect and abort with the same probability if the adversary provides an invalid opening to each commitment $com_{\st i,j}$ and $com_{\st {mk}}$, due to the binding property of the commitment scheme. Also, the smart contract in the real model and $\mathsf{Sim}^{\st \epsi}_{\st A}$ in the ideal model, can abort with the same probability if a Merkle tree proof is invalid, due to the security of the Merkle tree, i.e., due to the collision resistance of Merkle tree's hash function. 



Note that in the ideal model, $\mathsf{Sim}^{\st \epsi}_{\st A}$ can detect and abort with a probability of $1$, if $\mathcal{A}_{\st I}$ does not send to the simulator all encoded encrypted elements of the intersection,  i.e., when $E^{\st (I)}\neq S'$. Because the simulator already knows all elements in the intersection (and the encryption key). Thus, it can detect with a probability of $1$ if both the intersection sets that the extractors provide are identical but incorrect.   

 In the real world, if the extractors collude with each other and provide identical but incorrect intersections,   then an honest client (or the smart contract) cannot detect it. Thus, the adversary can distinguish the two models, based on the probability of aborting.  However, under the assumption that the smart contracts of Dong \textit{et al.} \cite{dong2017betrayal} are secure (i.e., are counter-collusion), and the extractors are rational, such an event (i.e., providing identical but incorrect result without one extractor betraying the other) would not occur in either model, as the real model and $(\mathcal{A}_{\st 1}, \mathcal{A}_{\st 2})$ rational adversaries follow the strategy that leads to a higher payoff. Specifically, as shown in \cite{dong2017betrayal}, providing incorrect but identical results is not the preferred strategy of the extractors; instead, the betrayal of one extractor by the other is the most profitable strategy in the case of (enforceable) collusion between the two extractors. This also implies that the amounts that the extractors would receive in both models are identical. 


%$\ddot Q:=(\qinit,  \qdelwr, \qUnFAbtwr, \qFAbt)$

Now, we analyze the output of the predicates $\bar Q:=(\qinit,  \qdelwr, $ $\qUnFAbtwr, \qFAbt)$ in the real and ideal models. In the real model, all clients proceed to prepare their input set only if the predefined amount of coins has been deposited by the parties; otherwise (if in steps \ref{sim::case1-buyer-deposit},\ref{e-PSI::buyer-deposit},\ref{e-PSI::extractor-deposit} of \epsi and step \ref{F-PSI::each-client-deposit} of \fpsi there is not enough deposit), they will be refunded and the protocol halts. In the ideal model, the simulator proceeds to prepare its inputs only if enough deposit has been placed in the contract. Otherwise, it would send message $abort_{\st 1}$ to TTP, during steps \ref{sim::case1-buyer-deposit}--\ref{sim::case1-check-Adv-deposited-y.|G|}. Thus, in both models, the parties proceed to prepare their inputs only if $\qinit(.) \rightarrow1$.  

In the real model, if there is an abort after the parties ensure there is enough deposit and before client $D$ provides its encoded input to the contract, then all parties can retrieve their deposit in full. In this case, the aborting adversary cannot learn anything about honest parties' input sets, as the parties' input sets have been blinded by random blinding polynomials known only to client $D$. In the ideal model, if there is any abort during steps \ref{E-PSI::sim-A-first-VOPR-invocation}--\ref{E-PSI::sim-A-receive-nu-from-adv}, then the simulator sends $abort_{\st 2}$ to TTP and instructs the ledger to refund every party's deposit. In the case of an abort, within the above two steps, the auditor is not involved and paid. Therefore, in both models,  in the case of an abort within the above steps, we would have $\qFAbt(.)\rightarrow1$. 




In the real model, if $Flag=True$, then all parties can locally extract the intersection, regardless of the extractors' behavior. In this case, each honest party receives $\yc'$ amount that it initially deposited in $\mathcal{SC}_{\st\fpsi}$. Moreover, each honest party receives \emph{at least} $|S_{\st\cap}|\cdot \lc$ amount as a reward, for contributing to the result. In this case, the honest buyer always collects the leftover of its deposit. Specifically, if both extractors act honestly, and the intersection cardinality is smaller than $|\Smin|$, then the buyer collects its deposit leftover, after paying all honest parties. If any extractor misbehaves, then the honest buyer fully recovers its deposit (and the misbehaving extractor pays the rest). 




Even if an extractor misbehaves and subsequently acts as a traitor to rectify its prior misconduct,  the buyer recovers the remaining deposit if the intersection's cardinality is less than $|\Smin|$.  In the ideal model, when $Flag=True$, then $\mathsf{Sim}^{\st \epsi}_{\st A}$ can extract the intersection by summing the output of \vopr provided by all parties and removing the blinding polynomials. In this case, it sends back each party's deposit placed in $\mathcal{SC}_{\st\fpsi}$, i.e., $\yc'$ amount. Also, in this case, each honest party receives at least $|S_{\st\cap}|\cdot \lc$ amount as a reward and the honest buyer always collects the leftover of its deposit. Thus, in both models in the case of $Flag=True$, we would have $\qdelwr(.)\rightarrow 1$. 




In the real model, when $Flag=False$, only the adversary can learn the result. In this case, the contract sends (i) $\chc$ amount to \aud, and (ii) $\frac{m'\cdot \yc'-\chc}{m-m'}$ amount, as compensation and reward, to each honest party, in addition to each party's initial deposit. In the ideal model,  when $Flag=False$, $\mathsf{Sim}^{\st \epsi}_{\st A}$ sends $abort_{\st 3}$ to TTP and instructs the ledger to distribute the same amount the contract distributes among the auditor (e.g., with address $adr_{\st j}$) and every honest party (e.g., with address $adr_{\st i}$) in the real model.  Thus, in both models when $Flag=False$, we would have $\qUnFAbtwr(., ., ., ., adr_{\st i})\rightarrow (a=1, .)$ and  $\qUnFAbtwr(., ., ., ., adr_{\st j})\rightarrow (., b=1)$. 

We conclude that the distribution of the joint outputs of the honest client $C\in \hat G$, client $D$, \aud, and the adversary in the real and ideal models are computationally indistinguishable.



\



\noindent\textbf{Case 2: Corrupt dealer $D$}.  In the real execution, the dealer's view is defined as follows: 


$$ \mathsf{View}_{\st D}^{\st \epsi} \Big(S^{\st (D)}, (S^{\st (1)},..., S^{\st (m)})\Big)=$$ $$ \{S^{\st (D)}, adr_{\st sc}, S_{\minn}\cdot \vc, 2\cdot \dc', 
%
%
 r_{\st D},  \mathsf{View}^{\st \fpsi}_{\st D}, \mathsf{View}^{\st \ct}_{\st D}, (com_{\st 1,j}, \bar{e}_{\st 1}, q_{\st 1}, h_{\st 1})...,$$ $$ (com_{\st sz, j'}, \bar{e}_{\st sz}, q_{\st {sz}}, h_{\st sz}), g, \hat{x}:=({mk}, z'), 
 %
  S_{\st \cap}\}$$

where  $\mathsf{View}^{\st \ct}_{\st D}$ and $\mathsf{View}^{\st \vopr}_{\st D}$ refer to $D$'s real-model view during the execution of \ct and \vopr respectively. Furthermore, $r_{\st D}$ is the outcome of internal random coins of $D$, $adr_{\st sc}$ is the address of contract, $\mathcal{SC}_{\st\epsi}$, $(j, ...,j')\in \{1,..., h\}$, $z'=\mathtt{PRF}(\bar{mk}, 0)$, $sz=|S_{\st \cap}|$, and $h_{\st i}$ is a Merkle tree proof asserting that $com_{\st i,j}$ is a leaf node of a Merkle tree with root node $g$. The simulator $\mathsf{Sim}^{\st \epsi}_{\st D}$, which receives all parties' input sets, operates as follows. 

\begin{enumerate}

%\item receives from the subroutine adversary polynomials $\bar{\bm\zeta}, (\bar{\bm\gamma}^{\st(A_1)}, \bar{\bm\delta}^{\st (A_1)}),..., (\bar{\bm\gamma}^{\st(A_m)}, \bar{\bm\delta}^{\st (A_m)})$,  $(\bar{\bm\omega}'^{\st (A_1)}, \bar{\bm\rho}'^{\st (A_1)}),..., $ $(\bar{\bm\omega}'^{\st (A_m)}, \bar{\bm\rho}'^{\st (A_m)})$, where $deg(\bar{\bm\gamma}^{\st(C)})=deg(\bar{\bm\delta}^{\st(C)})=3d+1, deg(\bar{\bm\omega}'^{\st (C)}) =deg(\bar{\bm\rho}'^{\st (C)})= d$, and $deg(\bar{\bm\zeta})=1$, where $C\in  \{  {  A}_{ \st {   1}}, ...,   {  A}_{ \st {   m}}\} $.
%
\item generates an empty view. It appends to the view, the input set $S^{\st (D)}$. It constructs and deploys a smart contract. It appends the contract's address, $ {adr}_{\st sc}$, to the view. 


\item appends to the view integer $\Smin\cdot \vc$, and $2\cdot \dc'$. Also, it appends uniformly random coins $r'_{\st D}$ to the view. 

%
\item extracts the simulation of \fpsi from \fpsi's simulator for client $D$. Let $\mathsf{Sim}^{\st \fpsi}_{\st D}$ be the simulation, that also includes a random key $mk$. It appends $\mathsf{Sim}^{\st \fpsi}_{\st D}$ to the view. 


%
 \item extracts the simulation of \ct from \ct's simulator, yielding  the simulation $\mathsf{Sim}^{\st \ct}_{\st D}$ that includes its output $mk'$. It appends $\mathsf{Sim}^{\st \ct}_{\st D}$ to the view. 
 
%
 
 \item\label{sim::case2-encode-intersection} encrypts each element $s_{\st i,j}$ in the intersection set $S_{\st \cap}$  as $e_{\st i,j}=\mathtt{PRP}(mk', s_{\st i,j})$ and then encodes the result as $\bar{e}_{\st i,j} = e_{\st i,j}||\mathtt{H}(e_{\st i, j})$. It commits to each encoded value as $com_{\st i,j}=\comcom(\bar{e}_{\st i,j}, q_{\st i,j})$, where $j$ is the index of the bin to which $\bar{e}_{\st i,j}$ belongs and  $q_{\st i, j}$ is a random value. 
 
 %
 
 
  \item\label{sim::case2-gen-commitments} constructs $(com'_{\st 1,1}, ..., com'_{\st d, h})$ where each $com'_{\st i, j}$ is a value picked uniformly at random from the commitment scheme output range. For every $j$-th bin, it sets each  $com'_{\st i', j}$ to unique $com_{\st i,j}$ if value $com_{\st i,j}$ for $j$-th bin has been generated in step \ref{sim::case2-encode-intersection}. Otherwise, the original values of $com'_{\st i', j}$ remain unchanged. 
 
 
 
 
% \item\label{sim::case2-gen-commitments} picks random values $(r_{\st 1,1}, ..., r_{\st d, h})$, from the $\mathtt{PRP}$'s range. It commits to them that yields $(com'_{\st 1,1}, ..., com'_{\st d, h})$ using fresh uniformly random values $q'=\{q'_{\st 1,1}, ..., q'_{\st d, h}\}$. For every $j$-th bin, it sets each  $com'_{\st i', j}$ to unique $com_{\st i,j}$ if value $com_{\st i,j}$ for $j$-th bin has been generated in step \ref{sim::case2-encode-intersection}. Otherwise, the original values of $com'_{\st i', j}$ remains unchanged. 
 
% \begin{itemize}
% 
%\item[$\bullet$] $r_{\st i, j}$ to a unique $\bar{e}_{\st ., j}$
%%
%\item[$\bullet$] $com'_{\st i, j}$ to unique $com_{\st .,j}$
%%
%\item[$\bullet$] $q'_{\st i, j}$ to unique $q_{\st ., j}$ 
%
% \end{itemize}
 
% Note the above allocation takes place only if values $\bar{e}_{\st ., j}$, $com_{\st .,j}$, and $q_{\st ., j}$ for $j$-th have been generated in step \ref{sim::case2-encode-intersection}. Otherwise, the original values of $r_{\st i, j}$, $com'_{\st i, j}$, and $q'_{\st i, j}$ remain unchanged. 
 
 
 \item constructs a  Merkle tree on top of the values $(com'_{\st 1,1}, ..., $ $com'_{\st d, h})$ generated in step \ref{sim::case2-gen-commitments}. Let $g$ be the resulting tree's root.  
 %
 \item for each element $s_{\st i,j}$ in the intersection, it constructs $(com'_{\st i',j}, $ $ \bar{e}_{\st i,j}, q_{\st i,j}, h_{\st i,j})$, where $com'_{\st i',j}$ is the commitment of $ \bar{e}_{\st i,j}$, $com'_{\st i',j}\in com$,  $(\bar{e}_{\st i,j}$ $q_{\st i,j})$ is the commitment's opening generated in step \ref{sim::case2-encode-intersection}, and $h_{\st i,j}$ is a Merkle tree proof asserting that $com'_{\st i',j}$ is a leaf of a Merkle tree with root $g$. It appends all  $(com'_{\st i',j}, \bar{e}_{\st i,j}, q_{\st i,j}, h_{\st i,j})$ along with $g$ to the view. 
 
 %
\item generates a commitment to $mk$ as $com_{\st mk}=\comcom(mk, z')$ where $z'=\mathtt{PRF}(mk, 0)$. It appends $(mk, z')$  and  $S_{\st \cap}$ to the view. 

%
\end{enumerate}
 

Now, let us delve into the reasons why the two views are computationally indistinguishable. $D$'s input $S^{\st (D)}$ is
 identical in both models, so they have identical distributions.  The contract's address has the same distribution in both models. The same holds for the integers $\Smin\cdot \vc$ and $ 2\cdot \dc'$. Moreover, because the real-model semi-honest adversary samples its randomness according to the protocol’s description, the random coins in both models (i.e., $r_{\st D}$  and $r'_{\st D}$) have identical distribution. Due to the security of \fpsi, $\mathsf{View}^{\st \fpsi}_{\st D}$ and $\mathsf{Sim}^{\st \fpsi}_{\st D}$ have identical distribution, so do  $\mathsf{View}^{\st \ct}_{\st D}$ and $\mathsf{Sim}^{\st \ct}_{\st D}$ due to the security of \ct. The intersection elements in both models have identical distributions and the encryption scheme is schematically secure. Therefore, each intersection element's representation (i.e., $\bar{e}_{\st i}$ in the real model and $\bar{e}_{\st i, j}$ in the deal model) are computationally indistinguishable. Each $q_{\st i}$ in the real model and $q_{\st i, j}$ in the ideal model have identical distributions as they have been picked uniformly at random. Each commitment $com_{\st i,j}$ in the real model is computationally indistinguishable from commitment $com'_{\st i',j}$ in the ideal model. 
 
 
 
 
 In the real model, each Merkle tree proof $h_{\st i}$ contains two leaf nodes (along with intermediary nodes that are the hash values of a subset of leaf nodes) that are themselves the commitment values. Furthermore, for each $h_{\st i}$, only one of the leaf node's openings (that contains an element in the intersection) is seen by $D$. The same holds in the ideal model, with the difference that for each Merkle tree proof $h_{\st i, j}$ the leaf node whose opening is not provided is a random value, instead of an actual commitment. 
 
 However, due to the hiding property of the commitment scheme, in the real and ideal models,  these two leaf nodes (whose openings are not provided) and accordingly the two proofs are computationally indistinguishable. In both models, values $mk$ and $z'$ are random values, so they have identical distributions. Furthermore, the intersection $S_{\st \cap}$ is identical in both models. 
 
 Thus, we conclude that the two views are computationally indistinguishable.
 
 
 \

\noindent\textbf{Case 3: Corrupt auditor}.  In this case, the real-model view of the auditor is defined as  follows: 

$$ \mathsf{View}_{\st Aud}^{\st \epsi} \Big(\bot, S^{\st (D)}, (S^{\st (1)},..., S^{\st (m)})\Big)=$$

$$ \{\mathsf{View}^{\st \fpsi}_{\st Aud}, adr_{\st sc}, \Smin\cdot \vc, 2\cdot \dc', (com_{\st 1,j}, \bar{e}_{\st 1}, q_{\st 1}, h_{\st 1})..., (com_{\st sz, j'}, \bar{e}_{\st sz}, q_{\st {sz}},$$ $$ h_{\st sz}), g, \hat{x}:=({mk}, z')\}$$


  Due to the security of \fpsi, \aud's view $\mathsf{View}^{\st \fpsi}_{\st Aud}$ during the execution of \fpsi can be easily simulated. As we have shown in Case 2, for the remaining transcript, its real-model view can be simulated too. There is a difference between Case 3 and Case 2; namely, in the former case, \aud does not have the $\mathtt{PRP}$'s key $mk'$ used to encrypt each set element. However, due to the security of  $\mathtt{PRP}$, it cannot distinguish each encrypted encoded element from a uniformly random element and cannot distinguish $\mathtt{PRP}(mk',.)$ from a uniform permutation. Therefore, each value $\bar{e}_{\st j}$ in the real model has identical distribution to each value $\bar{e}_{\st i,j}$ (as defined in Case 2) in the ideal model, as both are the outputs of $\mathtt{PRP}$. 

We conclude that the two views are computationally indistinguishable.


%by using the proof that we have already provided for Case 1 (i.e.,  $m-1$ client $A_{\st j}$s are corrupt), we can easily construct a simulator that generates a view computationally distinguishable from the real world semi-honest auditor. 
% The reason is that, in the worst-case scenario where $m-1$ malicious client $A_{\st j}$s reveal their input sets and randomness to the auditor, the auditor's view would be similar to the view of these corrupt clients, which we have shown to be indistinguishable. The only extra messages the auditor generates, that a corrupt client $A_{\st j}$ would not see in plaintext, are random blinding polynomials $(\bm\xi^{\st (A_1)},..., \bm\xi^{\st (A_m)})$ generated during the execution of $\mathtt{Audit}(.)$ of the ZSPA-A; however, these polynomials are picked uniformly at random and independent of the parties' input sets. Thus, if the smart contract detects misbehaviour and invokes the auditor, even if $m-1$ corrupt client $A_{\st j}$ reveals their input sets, then the auditor cannot learn anything about honest parties' input sets.    
 
 \

\noindent\textbf{Case 4: Corrupt public}. In the real model, the view of the public (i.e., non-participants of the protocol) is defined as below: 
 

 $$ \mathsf{View}_{\st Pub}^{\st \epsi} \Big(\bot, S^{\st (D)},(S^{\st (A_1)},..., S^{\st (A_m)})\Big)=$$ $$ 
 %
 %
 %
\{\mathsf{View}^{\st \fpsi}_{\st Pub}, adr_{\st sc}, \Smin\cdot \vc, 2\cdot \dc', (com_{\st 1,j}, \bar{e}_{\st 1}, q_{\st 1}, h_{\st 1})..., (com_{\st sz, j'}, \bar{e}_{\st sz}, q_{\st {sz}}, $$ $$h_{\st sz}), g, \hat{x}:=({mk}, z')\}$$
 
 
 
  Due to the security of \fpsi, the public's view $\mathsf{View}^{\st \fpsi}_{\st Pub}$ during \fpsi's execution can be simulated in the same manner as described in Case 4 on page \pageref{sec::F-PSI-proof}. The rest of the public's view overlaps with \aud's view in Case 3, excluding $\mathsf{View}^{\st \fpsi}_{\st Aud}$. Therefore, we can use the argument provided in Case 3 to show that the rest of the public's view can be simulated.     
   We conclude that the public's real and ideal views are computationally indistinguishable. 
 %
\end{proof}

















==> CCS-24/F-PSI-proof.tex <==
% !TEX root =main.tex


\section{Proof of \fpsi}\label{sec::F-PSI-proof}

In this section, we provide the proof for Theorem \ref{theorem::F-PSI-security}, which establishes the security of \fpsi. 


\begin{proof}
%
We prove Theorem  \ref{theorem::F-PSI-security} by considering the case where each party is corrupt, at a time.

\

\noindent\textbf{Case 1: Corrupt $m-1$ clients in $\{  {  A}_{ \st {   1}}, ...,   {  A}_{ \st {   m}}\}$}.  Let $P'$ be a set of at most $m-1$ corrupt clients, where $P'\subset \{  {  A}_{ \st {   1}}, ...,   {  A}_{ \st {   m}}\}$. Let set $\hat P$ be defined as follows: $\hat P=\{  {  A}_{ \st {   1}}, ...,   {  A}_{ \st {   m}}\}\setminus P'$. Moreover, let $\mathsf{Sim}^{\st\fpsi}_{\st A}$ be the simulator, which uses a subroutine adversary, $\mathcal{A}$.  Below, we explain how $\mathsf{Sim}^{\st \fpsi}_{\st A}$ (which receives the input sets of honest dealer $D$ and honest client(s) in $\hat P$) works. 


\begin{enumerate}[leftmargin=5.5mm]
%
\item constructs and deploys a smart contract. It sends the contract's address to $\mathcal{A}$. 
%
\item simulates \ct and receives the output value, $ {mk}$, from its functionality, $f_{\st \ct}$.
%
\item\label{sim::ZSPA-A-invocation} simulates \zspaa for each bin and receives the output value, $( k,  g,  q)$, from its functionality, $f^{\st \zspaa}$.
%
\item deposits in the contract the total amount of $(\yc+\chc)\cdot (m-|P'|+1)$ coins on behalf of $D$ and honest client(s) in $\hat P$. It sends to $\mathcal{A}$ the amount deposited in the contract. 
%
\item checks if $\mathcal{A}$ has deposited $(\yc+\chc)\cdot |P'|$ amount. If the check fails, it instructs the ledger to refund the coins that every party deposited and sends message $abort_{\st 1}$ to TTP (and accordingly to all parties); it outputs whatever $\mathcal{A}$ outputs and then halts. 

%
\item selects a random polynomial ${\bm\zeta}$ of degree $1$, for each bin. Also, $\mathsf{Sim}^{\st \fpsi}_{\st A}$, for each client $  {  C}\in \{  {  A}_{ \st {   1}}, ...,   {  A}_{ \st {   m}}\}$ allocates to each bin two random polynomials: (${\bm\omega}^{ \st {  {(D,C)}}}, {\bm\rho}^{ \st {  {(D,C)}}}$) of degree $d$ and   two random polynomials: (${\bm\gamma}^{ \st {  {(D,C)}}}$, ${\bm\delta}^{ \st {  {(D,C)}}}$) of degree $3d+1$. Moreover, $\mathsf{Sim}^{\st \fpsi}_{\st A}$ for every honest client $C'\in \hat P$, for each bin, picks two random polynomials: (${\bm\omega}^{ \st {  {(C',D)}}}$, ${\bm\rho}^{ \st {  {(C',D)}}}$) of degree $d$. %Note, all polynomials are picked from $\mathbb{F}_{\st p}[X]$. 
%
\item\label{F-PSI::sim-A-first-VOPR-invocation} simulates \vopr using inputs ${\bm\zeta} \cdot {\bm\omega}^{ \st {  {(D,C)}}}$ and ${\bm\gamma}^{ \st {  {(D,C)}}}$ for each bin. Accordingly, it receives the inputs of clients $C''\in P'$, i.e., ${\bm\omega}^{ \st {  {(C'',D)}}}\cdot {\bm\pi}^{ \st {  {(C'')}}}$, from its functionality $f^{\st \vopr}$, for each bin.  
%
%\item receives from $\mathcal{A}$ the outputs of VOPR for every client $C'' \in P'$. It ensures the output for every $C''$ has been provided. Otherwise, it halts.  
%
\item extracts the roots of polynomial ${\bm\omega}^{ \st {  {(C'',D)}}}\cdot {\bm\pi}^{ \st {  {(C'')}}}$ for each bin and appends those roots that are in the sets universe to a new set $S^{\st(C'')}$. 
%
\item simulates  \vopr again using inputs ${\bm\zeta}\cdot {\bm \rho}^{ \st {  {(D,C)}}}\cdot {\bm\pi}^{ \st {  {(D)}}}$ and ${\bm\delta}^{ \st {  {(D,C)}}}$, for each bin. %It receives the inputs of clients $C''\in P'$, i.e., $ {\bm\rho}^{ \st {  {(C'',D)}}}$, from $f^{\st \text{VOPR}}$, for each bin. 
%
\item sends to TTP the input sets of all parties; namely, (i) client $D$'s input set: $S^{\st (D)}$, (ii) honest clients' input sets: $S^{\st (C')}$ for all $C'$ in $\hat P$, and (iii) $\mathcal{A}$'s input sets: $S^{\st(C'')}$, for all $C''$ in $P'$.  For each bin, it receives the intersection set, $S_{\st\cap}$, from TTP. 
%
\item represents the intersection set for each bin as a polynomial, ${\bm \pi}$, as follows: ${\bm \pi}=\prod\limits^{\st |S_{\st\cap}|}_{\st i=1 }(x-s_{\st i})$, where $s_{\st i}\in S_{\st\cap}$. 

%
\item constructs polynomials ${\bm\theta}^{ \st {  {(C')}}}_{\st 1}={\bm\zeta} \cdot {\bm\omega}^{ \st {  {(D,C')}}}\cdot {\bm\omega}^{ \st {  {(C',D)}}}\cdot {\bm\pi}+{\bm\gamma}^{ \st {  {(D,C')}}}, {\bm\theta}^{ \st {  {(C')}}}_{\st 2}=  {\bm\zeta} \cdot  {\bm\rho}^{ \st {  {(D,C')}}}\cdot  {\bm\rho}^{ \st {  {(C',D)}}}\cdot  {\bm\pi}+  {\bm\delta}^{ \st {  {(D,C')}}}$, and $ {\bm\nu}^{ \st {  {(C')}} }=  {\bm\theta}^{ \st {  {(C')}}}_{\st 1}+ {\bm\theta}^{ \st {  {(C')}}}_{\st 2}+ {\bm \tau}^{ \st {  {(C')}} }$, for each bin and each honest client $C'\in\hat P$, where $ {\bm\tau}^{ \st {  {(C)}}}=\sum\limits^{\st 3d+2}_{\st i=0}z_{\st i,c}\cdot x^{\st i}$ and each $z_{\st i,c}$ is derived from $  k$. 
%
\item sends to $\mathcal{A}$ polynomial  $ {\bm\nu}^{ \st {  {(C')}} }$ for each bin and each client $C'$. 
%
\item\label{F-PSI::sim-A-receive-nu-from-adv} receives $ {\bm\nu}^{ \st {  {(C'')}} }$  from $\mathcal{A}$, for each bin and each client $C''\in P'$. It ensures that the output for every $C''$ has been provided. Otherwise, it halts. 
%
\item if there is any abort within steps \ref{F-PSI::sim-A-first-VOPR-invocation}--\ref{F-PSI::sim-A-receive-nu-from-adv}, then it sends $abort_{\st 2}$ to TTP and instructs the ledger to refund the coins that every party deposited.  It outputs whatever $\mathcal{A}$ outputs and then halts. 
%
\item constructs polynomial  $ {\bm\nu}^{ \st {  {(D)}}}= {\bm\zeta} \cdot   {\bm\omega'}^{ \st {  {(D)}}}\cdot  {\bm\pi} - \sum\limits^{ \st {   A}_{ \st {   m}}}_{  \st {  {C }= }  \st {   A}_{ \st {  1}}}( {\bm\gamma}^{ \st {  {(D,C)}}} +  {\bm\delta}^{ \st {  {(D,C)}}}) +  {\bm\zeta} \cdot  {\bm\gamma'}$ for each bin, where $ {\bm\omega'}^{ \st {  {(D)}}}$ is a fresh random polynomial of degree $d$ and $ {\bm\gamma'}$ is a pseudorandom polynomial derived from $  {mk}$.
%
\item sends to $\mathcal{A}$ polynomials $ {\bm\nu}^{ \st {  {(D)}}}$ and $ {\bm\zeta}$ for each bin. 
%
\item given each $ {\bm\nu}^{ \st {  {(C'')}} }$, computes polynomial $ {\bm\phi'}$ as follows $ {\bm\phi'} = \sum\limits_{\st \forall C''\in P'} {\bm\nu}^{ \st {  {(C'')}} }- \sum\limits_{\st \forall C''\in P'}( {\bm\gamma}^{ \st {  {(D,C'')}}} +  {\bm\delta}^{ \st {  {(D,C'')}}})$, for every bin. Then, $\mathsf{Sim}^{\st \fpsi}_{\st A}$ checks whether  $ {\bm\zeta}$  divides ${\bm\phi'}$, for every bin. If the check passes, it sets $Flag=True$. Otherwise, it sets $Flag=False$. 
%
\item if $Flag=True$:

\begin{enumerate}
%
 \item instructs the ledger to send back each party's deposit, i.e., $\yc+\chc$ amount. It sends a message $deliver$ to TTP.  
 %
 \item outputs whatever $\mathcal{A}$ outputs and then halts. 
 %
 \end{enumerate}
%
\item if $Flag=False$: 
%
\begin{enumerate}
%
 \item receives $|P'|$ keys of the $\mathtt{PRF}$ from $\mathcal{A}$, i.e., $\vv k'=[   k'_{\st 1}, ...,   k'_{\st |P'|}]$, for every bin. %, which should be the output of $f^{\st \text{ZSPA-A}}$ in step \ref{sim::ZSPA-A-invocation} above. 
%
\item checks whether the following equation holds: $  k'_{\st j}=  k$, for every $  k'_{\st j}\in\vv k'$. Note that $  k$ is the output of $f^{\st \zspaa}$ generated in step \ref{sim::ZSPA-A-invocation}. It constructs an empty list $  L'$ and appends to it the indices (e.g., $j$) of the keys that do not pass the above check. 
%
\item simulates \zspaa and receives from $f^{\st \zspaa}$ the output that contains a vector of random polynomials, $\vv{\mu}'$, for each valid key. 
%
\item sends to  $\mathcal{A}$, the list $  L'$ and vector  $\vv{\mu}'$, for every bin. 
%
\item  for each bin of client $  {  C}$ whose index (or ID) is not in $  L'$ computes polynomial $ {\bm\chi}^{ \st {  {(D, C)}}}$ as follows: 
 %
 $ {\bm\chi}^{ \st {  {(D, C)}}}= {\bm\zeta}\cdot  {\bm\eta}^{ \st {  {(D,C)}}}-( {\bm\gamma}^{ \st {  {(D,C)}}}+ {\bm\delta}^{ \st {  {(D,C)}}})$,   where $ {\bm\eta}^{ \st {  {(D,C)}}}$ is a fresh random polynomial of degree $3d+1$. Note, $C$ includes both honest and corrupt clients, except those clients whose index is in  $  L'$. $\mathsf{Sim}^{\st \fpsi}_{\st A}$ sends every polynomial $ {\bm\chi}^{ \st {  {(D, C)}}}$ to  $\mathcal{A}$. 
 %
 \item given each $ {\bm\nu}^{ \st {  {(C'')}} }$ (by $\mathcal{A}$ in step \ref{F-PSI::sim-A-receive-nu-from-adv}), computes polynomial $ {\bm\phi'}^{ \st {  {(C'')}} }$ as follows: ${\bm\phi'}^{ \st {  {(C'')}} } =  {\bm\nu}^{ \st {  {(C'')}} }-  {\bm\gamma}^{ \st {  {(D,C'')}}} -  {\bm\delta}^{ \st {  {(D,C'')}}}$, for every bin. Then, $\mathsf{Sim}^{\st \fpsi}_{\st A}$ checks whether  $ {\bm\zeta}$  divides $ {\bm\phi'}^{ \st {  {(C'')}} }$, for every bin. It appends the index of those clients that did not pass the above check to a new list, $  L''$. Note that $  L'\cap   L''=\bot$.
%
\item if  $  L'$ or $  L''$ is not empty, then it instructs the ledger: (i) to refund the coins of those parties whose index is not in $  L'$ and $  L''$, (ii) to retrieve $\chc$ amount from the adversary (i.e., one of the parties whose index is in one of the lists) and send the $\chc$ amount to the auditor, and (iii) to compensate each honest party (whose index is not in the two lists)  $\frac{m'\cdot (\yc+\chc)-\chc}{m-m'}$ amount, where $m'=|  L'|+|  L''|$.  Then, it sends  message $abort_{\st 3}$ to TTP. 
%
\item outputs whatever $\mathcal{A}$ outputs and halts. 
 %
 \end{enumerate}
%
\end{enumerate}

Next, we demonstrate that the real and ideal models are computationally indistinguishable, with our initial focus on the adversary's output. In the real and ideal models, the adversary sees the transcripts of ideal calls to $f_{\st \ct}$ as well as this functionality outputs, i.e., $mk$. 

Due to the security of \ct (as we are in the $f_{\st \ct}$-hybrid world), the transcripts of $f_{\st \ct}$ in both models have identical distribution, which also applies to the random output of $f_{\st \ct}$, namely $mk$. The same principle holds for the transcripts and outputs $(  k,   g,   q)$ of $f^{\st \zspaa}$ that the adversary observes in the two models. Also, the deposit amount is identical in both models. Thus, in the case where $abort_{\st 1}$ is disseminated at this point; the adversary's output distribution in both models is identical. 



The adversary also observes (the transcripts and) outputs of ideal calls to $f^{\st \vopr}$ in both models, i.e., output ($\bm\theta^{ \st {  {(C'')}}}_{\st 1}=\bm\zeta \cdot \bm\omega^{ \st {  {(D, C'')}}}\cdot \bm\omega^{ \st {  {(C'', D)}}}\cdot \bm\pi^{ \st {  {(C'')}}}+\bm\gamma^{ \st {  {(D,C'')}}}, \bm\theta^{ \st {  {(C'')}}}_{\st 2}=\bm\zeta \cdot \bm\rho^{ \st {  {(D, C'')}}}\cdot \bm\rho^{ \st {  {(C'',D)}}}\cdot \bm\pi^{ \st {  {(D)}}}+\bm\delta^{ \st {  {(D, C'')}}}$) for each corrupted client $C''$. However, due to the security of \vopr, the $\mathcal{A}$'s view, regarding \vopr, in both models have identical distribution.  
%
In the real model, the adversary observes the polynomial ${\bm\nu}^{ \st {  {(C)}}}$ that each honest client $C$ stores in the smart contract. Nevertheless, this is a blinded polynomial comprising of two uniformly random blinding polynomials (i.e., $\bm\gamma^{ \st {  {(D,C)}}}$ and $\bm\delta^{ \st {  {(D,C)}}}$) unknown to the adversary. In the ideal model, $\mathcal{A}$ is given polynomial  $ {\bm\nu}^{ \st {  {(C')}}}$ for each honest client $C'$. This polynomial has also been blinded via two uniformly random polynomials (i.e., $ {\bm\gamma}^{ \st {  {(D, C')}}}$ and $ {\bm\delta}^{ \st {  {(D, C')}}}$) unknown to $\mathcal{A}$. Thus, ${\bm\nu}^{ \st {  {(C)}}}$ in the real model and $ {\bm\nu}^{ \st {  {(C)}}}$ in the ideal model have identical distributions. As a result, in the case where $abort_{\st 2}$ is disseminated at this point; the adversary's output distribution in both models is identical. 



Furthermore, in the real world, the adversary observes polynomials ${\bm\zeta}$ and  $\bm\nu^{ \st {  {(D)}}}$  that  $D$ stores in the smart contract. Nevertheless, ${\bm\zeta}$ is a uniformly random polynomial, also polynomial $\bm\nu^{ \st {  {(D)}}}$ has been blinded; its blinding factors are the additive inverse of  the sum of the random polynomials $\bm\gamma^{ \st {  {(D,C)}}}$ and $\bm\delta^{ \st {  {(D,C)}}}$ unknown to the adversary, for every client $C\in \{  {  A}_{ \st {   1}}, ...,   {  A}_{ \st {   m}}\}$ and  $D$. In the ideal model, $\mathcal{A}$ is given $ {\bm\zeta}$ and $ {\bm\nu}^{ \st {  {(D)}}}$, where the former is a random polynomial and the latter is a blinded polynomial that has been blinded with the additive inverse of the sum of random polynomials $ {\bm\gamma}^{ \st {  {(D,C)}}}$ and $ {\bm\delta}^{ \st {  {(D,C)}}}$ unknown to it,  for all client $C$. Therefore,  (${\bm\zeta}, \bm\nu^{ \st {  {(D)}}}$)  in the real model and  ($ {\bm\zeta},  {\bm\nu}^{ \st {  {(D)}}}$) in the ideal model component-wise have identical distribution. 



Additionally, the sum of less than $m+1$ blinded polynomials ${\bm\nu}^{\st (A_{\st 1})},...,$ ${\bm\nu}^{\st (A_{\st m})}, \bm\nu^{ \st {  {(D)}}}$   in the real model has identical distribution to the sum of less than $m+1$ blinded polynomials $ {\bm\nu}^{\st (A_{\st 1})},...,  {\bm\nu}^{\st (A_{\st m})},  {\bm\nu}^{ \st {  {(D)}}}$ in the ideal model, as this combination would still be blinded by a set of random blinding polynomials unknown to the adversary. Now we discuss why the two polynomials $\frac{\bm\phi}{\bm\zeta}- \bm\gamma'$ in the real model and $\frac{ {\bm\phi}} { {\bm\zeta}}-  {\bm\gamma'}$ in the ideal model are indistinguishable. Note that, in this proof, we divide and then subtract polynomials ${\bm\phi}$ because the adversary already knows (and must know) polynomials $(\bm\zeta, \bm\gamma')$. In the real model, polynomial $\frac{\bm\phi}{\bm\zeta}- \bm\gamma'$ takes the following form: 
%
\begin{equation}\label{equ::-corrupt-A-real-world-phi}
%
\begin{split}
 \frac{\bm\phi}{\bm\zeta}- \bm\gamma'=\ &  \bm\omega'^{ \st {  {(D)}}}\cdot \bm\pi^{ \st {  {(D)}} } +\sum\limits^{ \st {   A}_{ \st {   m}}}_{ \st {  {C }= }  \st {   A}_{ \st {  1}}}(\bm\omega^{ \st {  {(D,C)}}} \cdot \bm\omega^{ \st {  {(C,D)}}}\cdot \bm\pi^{ \st {  (C)}})+ \\+ & \bm\pi^{ \st {  {(D)}}}\cdot\sum\limits^{ \st {   A}_{ \st {   m}}}_{ \st {  {C }= }  \st {   A}_{ \st {  1}}}(\bm\rho^{ \st {  {(D,C)}}} \cdot \bm\rho^{ \st {  {(C,D)}}})\\=\ &\bm\mu\cdot gcd( \bm\pi^{ \st {  {(D)}} },\bm\pi^{\st (A_1)}, ..., \bm\pi^{\st (A_m)})
 %
 \end{split}
\end{equation}

\

In Equation \ref{equ::-corrupt-A-real-world-phi}, every element of   $[\bm\omega'^{ \st {  {(D)}}},..., \bm\omega^{ \st {  {(D,C)}}}, \bm\rho^{ \st {  {(D,C)}}}]$ is a uniformly random polynomial for every  client $C\in \{  {  A}_{ \st {   1}}, ...,   {  A}_{ \st {   m}}\}$  (including corrupt ones) and client $D$. This is because it has been chosen by (in this case honest) client $D$. Thus,  as shown in Section \ref{sec::poly-rep}, $\frac{\bm\phi}{\bm\zeta}- \bm\gamma'$ takes the form $\bm\mu\cdot gcd( \bm\pi^{ \st {  {(D)}} },\bm\pi^{\st (A_1)}, ..., \bm\pi^{\st (A_m)})$, where $\bm\mu$ is a uniformly random polynomial and $gcd( \bm\pi^{ \st {  {(D)}} },\bm\pi^{\st (A_1)}, ..., \bm\pi^{\st (A_m)})$ represents the intersection of the input sets. 

In the ideal model, $\mathcal{A}$ can construct polynomial $ {\bm\phi}$ using its (well-formed) inputs $ {\bm\nu}^{ \st {  {(C'')}} }$ and polynomials $ {\bm\nu}^{ \st {  {(C')}} }$ that the simulator has transmitted to it, for all $C'\in\hat P$ and all $C''\in P'$. Thus, in the ideal model, polynomial $\frac{ {\bm\phi}}{\bm\zeta}-  {\bm\gamma'}$ has the following form:

\begin{equation}\label{equ::-corrupt-A-ideal-world-phi}
\begin{split}
%
\frac{ {\bm\phi}}{\bm\zeta}-  {\bm\gamma'}  = &\  { \bm\pi}\cdot\Big(\sum\limits_{\st \forall C'\in \hat P}(\bm\omega^{ \st {  {(D, C')}}} \cdot \bm\omega^{ \st {  {(C', D)}}}) + \sum\limits_{\st \forall C'\in \hat P}(\bm\rho^{ \st {  {(D, C')}}} \cdot \bm\rho^{ \st {  {(C', D)}}})\Big)+\\+ & \Big(\sum\limits_{\st \forall C''\in P'}(\bm\omega^{ \st {  {(D,C'')}}} \cdot \bm\omega^{ \st {  {(C'',D)}}}\cdot \bm\pi^{ \st {  (C'')}}) +\bm\pi^{ \st {  {(D)}}}\cdot\sum\limits_{\st \forall C''\in P'} (\bm\rho^{ \st {  {(D, C'')}}}\cdot \\ \cdot \ & \bm\rho^{ \st {  {(C'',D)}}})\Big) \\  =  &\ {\bm\mu}\cdot gcd(  {\bm\pi}, \bm\pi^{ \st {  {(D)}}}, \bm\pi^{ \st {  {(C'')}}})
 %
 \end{split}
\end{equation}

In Equation \ref{equ::-corrupt-A-ideal-world-phi}, every element of the vector $[\bm\omega^{ \st {  {(D,C')}}}, \bm\omega^{ \st {  {(D,C'')}}}, \bm\rho^{ \st {  {(D,C')}}}, $ $\bm\rho^{ \st {  {(D,C'')}}}]$ is a uniformly random polynomial for all $C'\in\hat P$ and all $C''\in P'$, because they have been selected by $\mathsf{Sim}^{\st \fpsi}_{\st A}$. Therefore, $\frac{ {\bm\phi}}{\bm\zeta}-  {\bm\gamma'}$ takes the form $ {\bm\mu}\cdot gcd(  {\bm\pi}, \bm\pi^{ \st {  {(D)}}}, \bm\pi^{ \st {  {(C'')}}})$, such that $ {\bm\mu}$ is a uniformly random polynomial and $gcd(  {\bm\pi}, \bm\pi^{ \st {  {(D)}}}, \bm\pi^{ \st {  {(C'')}}})$ represents the intersection of the input sets. We know that $gcd( \bm\pi^{ \st {  {(D)}} },\bm\pi^{\st (A_1)}, ..., \bm\pi^{\st (A_m)})=gcd(  {\bm\pi}, \bm\pi^{ \st {  {(D)}}}, \bm\pi^{ \st {  {(C'')}}})$, because $ {\bm\pi}$ includes the intersection of all clients' sets. Moreover, $ {\bm\mu}$ has identical distribution in the two models because they are uniformly random polynomials. Thus,  $\frac{\bm\phi}{\bm\zeta}- \bm\gamma'$ in the real model and $\frac{ {\bm\phi}} { {\bm\zeta}}-  {\bm\gamma'}$ in the ideal model are indistinguishable.


Now we focus on the case where $Flag=False$.  In the real model, the adversary observes the output of $\mathtt{Audit}(.)$ which is a list of indices $  L$ and a vector of random polynomials $\vv\mu$ picked by an honest auditor.  In the ideal model, $\mathcal{A}$ is given a  list $  L'$ of indices and a vector of random polynomials $\vv{\mu}'$ picked by the simulator. Thus, the pair ($  L, \vv\mu$) in the real model has identical distribution to the pair ($  L', \vv\mu'$) in the ideal model. 

Moreover, in the real model, the adversary observes each polynomial $\bm\chi^{ \st {  {(D, C)}}}=\bm\zeta\cdot \bm\eta^{ \st {  {(D,C)}}}-(\bm\gamma^{ \st {  {(D,C)}}}+\bm\delta^{ \st {  {(D,C)}}})$ that $D$ stores in the contract, for each bin and each client $C$ whose index is not in $  L$. This is a blinded polynomial with blinding factor $\bm\eta^{ \st {  {(D,C)}}}$ which itself is a uniformly random polynomial picked by $D$. In the ideal model, $\mathcal{A}$ is given a polynomial of the form $ {\bm\chi}^{ \st {  {(D, C)}}}= {\bm\zeta}\cdot  {\bm\eta}^{ \st {  {(D,C)}}}-( {\bm\gamma}^{ \st {  {(D,C)}}}+ {\bm\delta}^{ \st {  {(D,C)}}})$, for each bin and each client $C$ whose index is not in $  L'$. This is also a blinded polynomial whose blinding factor is  $ {\bm\eta}^{ \st {  {(D,C)}}}$ which itself is a random polynomial picked by the simulator.  Therefore, $\bm\chi^{ \st {  {(D, C)}}}$ in the real model has  identical distribution to $\bm\chi^{ \st {  {(D, C)}}}$ in the ideal model.  

In the real model, the adversary observes polynomial $ \bm\iota^{ \st {  {(C)}}}= \bm\zeta\cdot(\bm\eta^{ \st {  {(D,C)}}} + \bm\omega^{ \st {  {(D,C)}}}\cdot \bm\omega^{ \st {  {(C,D)}}}\cdot \bm\pi^{ \st {  {(C)}}}+\bm\rho^{ \st {  {(D,C)}}}\cdot \bm\rho^{ \st {  {(C,D)}}}\cdot \bm\pi^{ \st {  {(D)}}}+\bm\xi^{ \st {  {(C)}}})$ which is a blinded polynomial whose blinding factor is the sum of the above random polynomials, i.e., $\bm\eta^{ \st {  {(D,C)}}}+\bm\xi^{ \st {  {(C)}}}$. In the ideal model, $\mathcal{A}$ already has  polynomials $ {\bm\chi}^{ \st {  {(D, C)}}},  {\bm\nu}^{ \st {  {(C)}}}$, and $ {\bm\mu}^{ \st {  {(C)}}}$, where $ {\bm\mu}^{ \st {  {(C)}}}\in {\vv \mu'}$. This enables $\mathcal{A}$ to compute
 %
 $  {\bm\iota}^{ \st {  {(C)}}} =  {\bm\chi}^{ \st {  {(D, C)}}} +   {\bm\nu}^{ \st {  {(C)}}} +  {\bm\mu}^{ \st {  {(C)}}}= {\bm\zeta}\cdot ( {\bm\eta}^{ \st {  {(D,C)}}}+  {\bm\omega}^{ \st {  {(D,C')}}}\cdot  {\bm\omega}^{ \st {  {(C',D)}}}\cdot  {\bm\pi}+  {\bm\rho}^{ \st {  {(D,C')}}}\cdot  {\bm\rho}^{ \st {  {(C',D)}}}\cdot  {\bm\pi}+ {\bm\xi}^{ \st {  {(C)}}})$,
 %
  where $ {\bm\xi}^{ \st {  {(C)}}}$ is a random blinding polynomial used in $ {\bm\mu}^{ \st {  {(C)}}}$. Nevertheless, $ {\bm\iota}^{ \st {  {(C)}}}$ itself is a blinded polynomial whose blinding factor is the sum of random polynomials, i.e., $ {\bm\eta}^{ \st {  {(D,C)}}}+ {\bm\xi}^{ \st {  {(C)}}}$. Hence, the distribution of polynomial $ \bm\iota^{ \st {  {(C)}}}$ in the real model and $ {\bm\iota}^{ \st {  {(C)}}}$ in the ideal model are identical. Moreover, the integer $\yc+\chc+\frac{m'\cdot (\yc+\chc)-\chc}{m-m'}$ has identical distribution  in both  models. 

Next, we demonstrate that the honest party aborts with the same probability in the real and ideal models. Due to the security of \ct, an honest party (during the execution of \ct) aborts with the same probability in both models. 
%
In this scenario, the adversary gains no information about the parties' input sets and the intersection of these sets because the parties have not yet transmitted any encoded input sets. The same principle applies to the probability of honest parties aborting during the execution of \zspaa.  In this case, an aborting adversary also learns nothing about the parties' input set and the sets' intersection. 

Since the deposit of all parties is made public, an honest party can check and identify whether all parties have deposited a sufficient amount with the same probability in both models. If parties halt due to insufficient deposits, no one gains knowledge about the parties' input sets or the intersection of the sets because the inputs (representation) have not been transmitted at this stage.


Due to the security of \vopr, honest parties abort with the same probability in both models. In the case of an abort during \vopr execution, the adversary would learn nothing (i) about its counter party' input set due to the security of \vopr, and (ii) about the rest of the honest parties' input sets and the intersection as the other parties' input sets are still blinded by random blinding factors known only to $D$. In the real model, $D$ can check if all parties provided their encoded inputs, by reading from the smart contract.  

The simulator can also perform the same verification to ensure that  $\mathcal{A}$ has supplied the encoded inputs of all corrupt parties. Hence, in both models, an honest party would detect the violation of this requirement, which is providing all encoded inputs, with the same probability. Even in this scenario, if an adversary aborts by not providing proof of its encoded inputs, it gains no knowledge about the input sets of honest parties or the intersection, for the previously explained reasons.

%Now we determine the probability that $Flag=True$ in each model. 

In the real model, the smart contract sums every client $C$'s polynomial $\bm\nu^{ \st {  {(C)}} }$ with each other and with $D$'s polynomial $\bm\nu^{ \st {  {(D)}} }$, which removes the blinding factors that $D$ initially inserted (during the execution of \vopr). After that, it checks whether the result is divisible by  $\bm \zeta$. 
%
Due to the following reasons the smart contract can detect if a set of outputs of \vopr has been tampered with, with a probability at least $1-\negl(\lambda)$:

\begin{itemize}
\item Theorem \ref{Unforgeable-Polynomials-Linear-Combination}, i.e., unforgeable polynomials’ linear combination.

\item  The fact that the smart contract is given the random polynomial $\bm \zeta$ in plaintext. 

\item No party (excluding honest client $D$) knew anything about $\bm \zeta$ before they send their input to the contract. 
\item The security of the smart contract, i.e., the adversary cannot influence the correctness of the above verification performed by the contract. 
\end{itemize}




%Due to (a) Theorem \ref{Unforgeable-Polynomials-Linear-Combination} (i.e., unforgeable polynomials’ linear combination), (b) the fact that the smart contract is given the random polynomial $\bm \zeta$ in plaintext, (c) no party (except honest client $D$) knew anything about $\bm \zeta$ before they send their input to the contract, and (d) the security of the contract (i.e., the adversary cannot influence the correctness of the above verification performed by the contract), the contract can detect if a set of outputs of \vopr has been tampered with, with a probability at least $1-\negl(\lambda)$. 





In the ideal model, $\mathsf{Sim}^{\st \fpsi}_{\st A}$ also can remove the blinding factors and it knows the random polynomial $ {\bm \zeta}$, unlike the adversary who does not know $ {\bm \zeta}$ when it sends the outputs of \vopr to $\mathsf{Sim}^{\st \fpsi}_{\st A}$. So, $\mathsf{Sim}^{\st \fpsi}_{\st A}$ can detect when $\mathcal{A}$ modifies a set of the outputs of \vopr that were sent to  $\mathsf{Sim}^{\st \fpsi}_{\st A}$ with a probability at least $1-\negl(\lambda)$,  due to Theorem \ref{Unforgeable-Polynomials-Linear-Combination}. Hence, the smart contract in the real model and the simulator in the ideal model would abort with a similar probability. 

Moreover, due to the security of \zspaa, the probability that an invalid key $k_{\st i}\in \vv{k}$ is added to the list $  L$ in the real world is similar to the probability that  $\mathsf{Sim}^{\st \fpsi}_{\st A}$ detects an invalid key $  k'_{\st i}\in \vv{k'}$ in the ideal world. 


In the real model, when $Flag=False$, the smart contract can identify each ill-structured output of \vopr (i.e.,  $\bm\nu^{ \st {  {(C)}} }$) with a probability of at least $1-\negl(\lambda)$ by checking whether $\bm\zeta$  divides $\bm\iota^{ \st {  {(C)}}}$, for the following reasons:  (a) Theorem \ref{proof::unforgeable-poly} (i.e., unforgeable polynomial), (b) the fact that the smart contract is given $\bm \zeta$ in plaintext, (c) no party (excluding honest client $D$) knew anything about $\bm \zeta$ before they send their input to the contract, and (d) the security of the contract. 

In the ideal model, when $Flag=False$, given each $ {\bm\nu}^{ \st {  {(C'')}} }$, $\mathsf{Sim}^{\st \fpsi}_{\st A}$ can remove its blinding factors from  $ {\bm\nu}^{ \st {  {(C'')}} }$ which results in $ {\bm\phi'}^{ \st {  {(C'')}} }$ and then check if $ {\bm\zeta}$  divides $ {\bm\phi'}^{ \st {  {(C'')}} }$. The simulator can also detect an ill-structured  $ {\bm\nu}^{ \st {  {(C'')}} }$ with a probability of at least $1-\negl(\lambda)$, due to Theorem \ref{proof::unforgeable-poly}, the fact that the simulator is given $ {\bm \zeta}$ in plaintext,  and the adversary is not given any knowledge about $ {\bm \zeta}$ before it sends to the simulator the outputs of \vopr.  Hence, the smart contract in the real model and $\mathsf{Sim}^{\st \fpsi}_{\st A}$ in the ideal model would detect an ill-structured input of an adversary with the same probability. 

%$Q:=(\qinit, \qdel, \qUnFAbt, \qFAbt)$


Now, we analyze the output of the predicates $(\qinit, \qdel, \qUnFAbt, $ $\qFAbt)$ in the real and ideal models. In the real model, all clients proceed to prepare their input set only if the predefined amount of coins has been deposited by the parties. Otherwise, they will be refunded and the protocol halts. In the ideal model also the simulator proceeds to prepare its inputs only if a sufficient amount of deposit has been put in the contract.  Otherwise, it would send message $abort_{\st 1}$ to TTP. Thus, in both models, the parties proceed to prepare their inputs only if $\qinit(.) \rightarrow1$. 

In the real model, if there is an abort after the parties ensure that there is enough deposit and before client $D$ provides its encoded input to the contract, then all parties would be able to retrieve their deposit in full. In this case, the aborting adversary would not be able to learn anything about honest parties' input sets, because the parties' input sets are still blinded by random blinding polynomials known only to client $D$. 

In the ideal model, if there is any abort during steps \ref{F-PSI::sim-A-first-VOPR-invocation}--\ref{F-PSI::sim-A-receive-nu-from-adv}, then the simulator sends $abort_{\st 2}$ to TTP and instructs the ledger to refund the coins that every party deposited. Also, in the case of an abort (within the above two points of time), the auditor is not involved. Thus, in both models, if an abort occurs within the specified time frames, we would have $\qFAbt(.)\rightarrow1$. In the real model, if $Flag=True$, then all parties would be able to learn the intersection, and the smart contract refunds all parties, i.e., sends each party $\yc+\chc$ amount which is the amount each party initially deposited. 

In the ideal model, when $Flag=True$, then $\mathsf{Sim}^{\st \fpsi}_{\st A}$ can extract the intersection (by summing the output of \vopr provided by all parties and removing the blinding polynomials) and sends back each party's deposit, i.e., $\yc+\chc$ amount. Hence, in both models in the case of $Flag=True$, when all of the parties receive the result, we would have $\qdel(.)\rightarrow 1$. In the real model, when $Flag=False$, only the adversary which might corrupt $m'$ clients would be able to learn the result; in this case, the contract sends (i) $\chc$ amount to the auditor, and (ii) $\frac{m'\cdot (\yc+\chc)-\chc}{m-m'}$ amount as a compensation, to each honest party, in addition to each party's deposit $\yc+\chc$. 

In the ideal model,  when $Flag=False$, $\mathsf{Sim}^{\st \fpsi}_{\st A}$  sends $abort_{\st 3}$ to TTP and instructs the ledger to distribute the same amount among the auditor (e.g., with address $adr_{\st j}$) and every honest party (e.g., with address $adr_{\st i}$) as the contract does in the real model. Thus, in both models when $Flag=False$, we would have $\qUnFAbt(., ., ., ., adr_{\st i})\rightarrow (a=1, .)$ and  $\qUnFAbt(., ., ., ., adr_{\st j})\rightarrow (., b=1)$. 

We conclude that the distributions of the joint outputs of the honest client $C\in \hat P$, client $D$, \aud, and the adversary in the real and ideal models are computationally indistinguishable.


\

\noindent\textbf{Case 2: Corrupt dealer $D$}.  In the real execution, the dealer's view is defined as follows: 


$$ \mathsf{View}_{\st D}^{\st \fpsi} \Big(S^{\st (D)},(S^{\st (1)},..., S^{\st (m)})\Big)=$$ $$ \{S^{\st (D)}, adr_{\st sc}, m\cdot(\yc+\chc), r_{\st D}, \mathsf{View}^{\st \ct}_{\st D}, k, g, q, \mathsf{View}^{\st \vopr}_{\st D}, \bm\nu^{\st (A_1)},..., \bm\nu^{\st (A_m)}, S_{\st \cap}\}$$
%
where  $\mathsf{View}^{\st \ct}_{\st D}$ and $\mathsf{View}^{\st \vopr}_{\st D}$ refer to the dealer's real-model view during the execution of \ct and \vopr respectively. Moreover, $r_{\st D}$ is the outcome of internal random coins of client $D$, and $adr_{\st sc}$ is the address of contract $\mathcal{SC}_{\fpsi}$. The simulator $\mathsf{Sim}^{\st \fpsi}_{\st D}$, which receives all parties' input sets, works as follows. 

\begin{enumerate}[leftmargin=4.6mm]

\item receives from the subroutine adversary polynomials: 
%
$ {\bm\zeta}, ( {\bm\gamma}^{\st(A_1)},$ $  {\bm\delta}^{\st (A_1)}),...,$ $ ( {\bm\gamma}^{\st(A_m)}, $ $ {\bm\delta}^{\st (A_m)})$,  $( {\bm\omega}'^{\st (A_1)},  {\bm\rho}'^{\st (A_1)}),..., $ $( {\bm\omega}'^{\st (A_m)},  {\bm\rho}'^{\st (A_m)})$,
 
  where $deg( {\bm\gamma}^{\st(C)})=deg( {\bm\delta}^{\st(C)})=3d+1,  deg( {\bm\omega}'^{\st (C)}) =   deg( {\bm\rho}'^{\st (C)})= d$, and $deg( {\bm\zeta})=1$, and $C\in  \{  {  A}_{ \st {   1}}, ...,   {  A}_{ \st {   m}}\} $.
%
\item generates an empty view. It appends to the view, the input set $S^{\st (D)}$. It constructs a smart contract  and deploys it. Let $  {adr}_{\st sc}$ be the contract's address. It appends $ {adr}_{\st sc}$ to the view. 


\item appends to the view integer $m\cdot(\yc+\chc)$   and coins $r'_{\st D}$ chosen uniformly at random. 
%
\item extracts the simulation of \ct from \ct's simulator for client $D$. Let $\mathsf{Sim}^{\st \ct}_{\st D}$ be the simulation. It appends $\mathsf{Sim}^{\st \ct}_{\st D}$ to the view. 
%
\item picks a random key, $  k'$, and derives pseudorandom values $z'_{\st i,j}$ from the key (the same way is done in Figure \ref{fig:ZSPA}). It constructs a Merkle tree on top of all values $z'_{\st i, j}$. Let $g'$ be the root of the resulting tree. It appends $  k', g'$, and $q'=\mathtt{H}(  k')$ to the view. 
%
\item invokes \vopr's functionality twice and extracts the simulation of \vopr from \vopr's simulator for client $D$. Let $\mathsf{Sim}^{\st \vopr}_{\st D}$ be the simulation. It appends $\mathsf{Sim}^{\st \vopr}_{\st D}$ to the view.  
%
\item given the parties' input sets, computes a polynomial $ {\bm\pi}$ that represents the intersection of the sets. 

\item picks $m$ random polynomials $ {\bm\tau}^{\st (A_1)}, ...,  {\bm\tau}^{\st (A_m)}$ of degree $3d+1$ such that their sum is $0$.  

%\item picks $m$ pair of random polynomials $(\bm\gamma^{\st(1)}, \bm\delta^{\st (1)}),..., (\bm\gamma^{\st(m)}, \bm\delta^{\st (m)})$ where each polynomial is of degree $3d+1$.

\item picks $m$ pairs of random polynomials $( {\bm\omega}^{\st (A_1)},  {\bm\rho}^{\st (A_1)}),..., ( {\bm\omega}^{\st (A_m)},$ $  {\bm\rho}^{\st (A_m)})$, where each polynomial is of degree $d$. Then, $\mathsf{Sim}^{\st \fpsi}_{\st D}$ for each client $C\in  \{  {  A}_{ \st {   1}}, ...,   {  A}_{ \st {   m}}\} $ computes polynomial $ {\bm\nu}^{\st (C)}= {\bm\zeta}\cdot {\bm\pi}\cdot(  {\bm\omega}^{\st (C)}\cdot  {\bm\omega}'^{\st (C)}+  {\bm\rho}^{\st (C)}\cdot  {\bm\rho}'^{\st (C)})+ {\bm\delta}^{\st (C)}+ {\bm\gamma}^{\st(C)}+  {\bm\tau}^{ \st {  {(C)}}}$. 
%
\item appends $ {\bm\nu}^{\st (A_1)},...,  {\bm\nu}^{\st (A_m)}$ and the intersection of the sets $S'_{\st \cap}$ to the view. 
%
\end{enumerate}



 Next, we will demonstrate that the two views are computationally indistinguishable. $D$'s input $S^{\st (D)}$ is
 identical in both models. Therefore, they have identical distributions. Furthermore, the contract's address has the same distribution in both views, the same applies to the integer $ m\cdot(\yc+\chc)$. Since the real-model semi-honest adversary samples its randomness according to the protocol’s description, the random coins in both models (i.e., $r_{\st D}$  and $r'_{\st D}$) have identical distributions. 
 
 Moreover, due to the security of  \ct, $\mathsf{View}^{\st \ct}_{\st D}$ and $\mathsf{Sim}^{\st \ct}_{\st D}$ have identical distributions. Keys $k$ and $  k'$ have identical distributions as well because both have been chosen uniformly at random from the same domain.  In the real model, each element of the pair $(g, p)$ is the output of a deterministic function on a random value $k$. We know that $k$ in the real model has identical distribution to $  k'$ in the ideal model, so do the evaluations of deterministic functions (i.e., Merkle tree, $\mathtt{H}$, and $\mathtt {PRF}$) on them. Therefore, each pair $(g, q)$ in the real model component-wise has an identical distribution to each pair $(g', q')$ in the ideal model.  
 %
 Furthermore, due to the security of the \vopr, $\mathsf{View}^{\st \vopr}_{\st D}$ and $\mathsf{Sim}^{\st \vopr}_{\st D}$ have identical distributions.
 
 
 In the real model, each $\bm\nu^{\st (C)}$ has been blinded by a pseudorandom polynomial (i.e., derived from $\mathtt{PRF}$'s output) unknown to client $D$. In the ideal model, however, each $ {\bm\nu}^{\st (C)}$ has been blinded by a random polynomial unknown to client $D$. Due to the security of $\mathtt{PRF}$,  its outputs are computationally indistinguishable from truly random values.  Therefore, ${\bm\nu}^{\st (C)}$ in the real model and $ {\bm\nu}^{\st (C)}$ in the ideal model are computationally indistinguishable. 
 
 Now we focus on the sum of all ${\bm\nu}^{\st (C)}$ in the real model and the sum of all $ {\bm\nu}^{\st (C)}$ in the ideal model, as adding them together would remove the above blinding polynomials that are unknown to client $D$.  Specifically, in the real model, after client $D$ sums all  ${\bm\nu}^{\st (C)}$ and removes the blinding factors and $\bm\zeta$ that it initially imposed, it would get a polynomial of the  form 
 %
  $\bm{\hat\phi}= \frac{ \sum\limits^{ \st {   A}_{ \st {   m}}}_{  \st {  {C }= }  \st {   A}_{ \st {  1}}}\bm\nu^{ \st {  {(C)}} }-\sum\limits^{ \st {   A}_{ \st {   m}}}_{  \st {  {C }= }  \st {   A}_{ \st {  1}}}(\bm\gamma^{ \st {  {(D,C)}}} + \bm\delta^{ \st {  {(D,C)}}})}{\bm\zeta}= \sum\limits^{ \st {   A}_{ \st {   m}}}_{ \st {  {C }= }  \st {   A}_{ \st {  1}}}(\bm\omega^{ \st {  {(D,C)}}} \cdot \bm\omega^{ \st {  {(C,D)}}}\cdot \bm\pi^{ \st {  (C)}}) +\bm\pi^{ \st {  {(D)}}}\cdot\sum\limits^{ \st {   A}_{ \st {   m}}}_{ \st {  {C }= }  \st {   A}_{ \st {  1}}}(\bm\rho^{ \st {  {(D,C)}}} \cdot \bm\rho^{ \st {  {(C,D)}}}) $, 
%
  where $\bm\omega^{ \st {  {(C,D)}}}$ and $\bm\rho^{ \st {  {(C,D)}}}$ are random polynomials unknown to client $D$. 
 
 In the ideal model, after summing all $ {\bm\nu}^{\st (C)}$ and removing the random polynomials that it already knows, it would get a polynomial of the following form: 
 %
 $\bm{\hat\phi}'= \frac{\sum\limits^{ \st {   A}_{ \st {   m}}}_{  \st {  {C }= }  \st {   A}_{ \st {  1}}} {\bm\nu}^{\st(C)}-\sum\limits^{ \st {   A}_{ \st {   m}}}_{  \st {  {C }= }  \st {   A}_{ \st {  1}}}( {\bm\gamma}^{\st(C)} +  {\bm\delta}^{\st(C)})}{ {\bm\zeta}}=  {\bm\pi}\cdot\sum\limits^{ \st {   A}_{ \st {   m}}}_{ \st {  {C }= }  \st {   A}_{ \st {  1}}}( {\bm\omega}'^{\st(C)} \cdot  {\bm\omega}^{\st(C)})+( {\bm\rho}'^{\st(C)} \cdot  {\bm\rho}^{\st(C)})  $.
 
 
 As shown in Section \ref{sec::poly-rep},  polynomial $\bm{\hat\phi}$ has the form $\bm\mu\cdot gcd( \bm\pi^{ \st {  {(D)}} },$ $\bm\pi^{\st (A_1)}, ..., $ $\bm\pi^{\st (A_m)})$, where $\bm\mu$ is a uniformly random polynomial and $gcd( \bm\pi^{ \st {  {(D)}} },\bm\pi^{\st (A_1)}, ..., \bm\pi^{\st (A_m)})$ represents the intersection of the input sets. Moreover, it is evident that $\bm{\hat\phi}'$ has the form $ {\bm\mu} \cdot  {\bm\pi}$, where $ {\bm\mu} $ is a random polynomial and $ {\bm\pi}$ represents the intersection. We know that both $gcd( \bm\pi^{ \st {  {(D)}} },\bm\pi^{\st (A_1)}, ..., \bm\pi^{\st (A_m)})$ and $ {\bm\pi}$  represent the same intersection. Furthermore,  ${\bm\mu} $ in the real model and $ {\bm\mu} $ in the ideal model have identical distributions as they are uniformly random polynomials. Thus, two polynomials $\bm{\hat\phi}$ and $\bm{\hat\phi}'$ are indistinguishable. Also, the output $S_{\st \cap}$ is identical in both views. We conclude that the two views are computationally indistinguishable.
 
 
 \

\noindent\textbf{Case 3: Corrupt auditor}. 

In this scenario, we can leverage the proof we have already presented for Case 1 (i.e.,  $m-1$ client $A_{\st j}$s are corrupt), to construct a simulator that produces a view computationally distinguishable from that of the semi-honest auditor in the real model. 

 The reason is that, in the worst-case scenario where $m-1$ malicious client $A_{\st j}$s reveal their input sets and randomness to the auditor, the auditor's view would be similar to the view of these corrupt clients, which we have shown to be indistinguishable. The only extra messages the auditor generates, that a corrupt client $A_{\st j}$ would not see in plaintext, are random blinding polynomials $(\bm\xi^{\st (A_1)},..., \bm\xi^{\st (A_m)})$ generated during the execution of $\mathtt{Audit}(.)$ of \zspaa. However, these polynomials have been chosen uniformly at random and independent of the parties' input sets. Thus, if the smart contract detects misbehavior and invokes the auditor, even if $m-1$ corrupt client $A_{\st j}$ reveals their input sets, then the auditor cannot learn anything about honest parties' input sets.    
 
 \

\noindent\textbf{Case 4: Corrupt public}. In the real model, the view of the public (i.e., non-participants of the protocol) is defined as below: 
 

 $$ \mathsf{View}_{\st Pub}^{\st \fpsi} \Big(\bot, S^{\st (D)},(S^{\st (A_1)},..., S^{\st (A_m)})\Big)=$$ $$ \{\bot, adr_{\st sc}, (m+1)\cdot(\yc+\chc), k, g, q, \bm\nu^{\st (A_1)},..., \bm\nu^{\st (A_m)}, \bm\nu^{\st (D)}\}$$
 
 
 Now, we describe how the simulator $\mathsf{Sim}^{\st \fpsi}_{\st Pub}$  operates. 
 
 \begin{enumerate}
 %
 \item generates an empty view and appends to it an empty symbol, $\bot$. It constructs and deploys a smart contract. It appends the contract's address, $  {adr}_{\st sc}$ and integer $(m+1)\cdot(\yc+\chc)$ to the view.
 %
\item picks a random key, $  k'$, and derives pseudorandom values $z'_{\st i,j}$ from the key,  in the same way, done in Figure \ref{fig:ZSPA}. It constructs a Merkle tree on top of the $z'_{\st i, j}$ values. Let $g'$ be the root of the resulting tree. It appends $  k', g'$, and $q' = \mathtt{H}(  k')$ to the view. 
%
\item for each client $C\in \{  {  A}_{ \st {   1}}, ...,   {  A}_{ \st {   m}}\}$ and client $D$ generates a random polynomial of degree $3d+1$ (for each bin), i.e.,  $ {\bm\nu}^{\st (A_1)}, ...,  {\bm\nu}^{\st (A_m)},  {\bm\nu}^{\st (D)}$. 
 %
 \end{enumerate}
 
 Next, we will illustrate that the two views are computationally indistinguishable. In both views, $\bot$ is identical. Also, the contract’s addresses (i.e., ${adr}_{\st sc}$) have the same
distribution in both views and so has the integer $(m+1)\cdot(\yc+\chc)$. Keys $k$ and $  k'$ have identical distributions as well because both of them have been picked uniformly at random from the same domain.  In the real model, each element of pair $(g, p)$ is the output of a deterministic function on the random key $k$. We know that $k$ in the real model has an identical distribution to $  k'$ in the ideal model, and so do the evaluations of deterministic functions on them. Hence, each pair $(g, q)$ in the real model component-wise has an identical distribution to each pair $(g', q')$ in the ideal model. 

In the real model, each polynomial  $\bm\nu^{\st (C)}$ is a blinded polynomial comprising of two uniformly random blinding polynomials (i.e., $\bm\gamma^{ \st {  {(D,C)}}}$ and $\bm\delta^{ \st {  {(D,C)}}}$) unknown to the adversary. In the ideal model, each polynomial  $ {\bm\nu}^{\st (C)}$ is a random polynomial; thus, polynomials $\bm\nu^{\st (A_1)},..., \bm\nu^{\st (A_m)}$ in the real model have identical distribution to  polynomials $ {\bm\nu}^{\st (A_1)}, ...,  {\bm\nu}^{\st (A_m)}$ in the ideal model.  Similarly,  polynomial $\bm\nu^{\st (D)}$ has been blinded in the real model; its blinding factors are the additive inverse of the sum of the random polynomials $\bm\gamma^{ \st {  {(D,C)}}}$ and $\bm\delta^{ \st {  {(D,C)}}}$ unknown to the adversary. In the ideal model, polynomial $ {\bm\nu}^{\st (D)}$ is a uniformly random polynomial; thus, ${\bm\nu}^{\st (D)}$ in the real model and $ {\bm\nu}^{\st (D)}$ in the ideal model have identical distributions.

Moreover, in the real model even though the sum $\bm\phi$ of polynomials  $\bm\nu^{\st (A_1)},..., $ $\bm\nu^{\st (A_m)}, \bm\nu^{\st (D)}$ would remove some of the blinding random polynomials, it is still a blinded polynomial with a pseudorandom blinding factor $\bm\gamma'$ (derived from the output of $\mathtt{PRF}$), unknown to the adversary. In the ideal model, the sum of polynomials $ {\bm\nu}^{\st (A_1)}, ...,  {\bm\nu}^{\st (A_m)}, $ $ {\bm\nu}^{\st (D)}$ is also a random polynomial. Thus, the sum of the above polynomials in the real model is computationally indistinguishable from the sum of those polynomials in the ideal model. 

We conclude that the two views are computationally indistinguishable. 
 %
\end{proof}

















==> CCS-24/Fair-PSI.tex <==
% !TEX root =main.tex

\vspace{-2.5mm}

\section{Definition of Multi-party PSI with Fair Compensation}\label{sec::F-PSI-model}%\label{Fair-PSI-Protocol}


\vspace{-.5mm}



Now, we present the concept of multi-party PSI with Fair Compensation  (\p) which ensures that either all clients receive the result or honest parties are financially compensated in the event of an unfair protocol abortion, wherein only dishonest parties gain access to the result.  
%
In a  $\mathcal{PSI}^{\st \mathcal{FC}}$, three types of parties are involved:  (1) a set of clients $\{A_{\st 1},...,A_{\st m}\}$ potentially \emph{malicious} (i.e., active adversaries), where all but one may collude with each other, (2) a non-colluding dealer, $D$, potentially semi-honest, and (3) an auditor, \aud, potentially semi-honest, where all parties except \aud have input set. For simplicity, we assume that one can determine whether a given address belongs to \aud. The fundamental functionality computed by any multi-party PSI can be defined as  $f^{\st\text{PSI}} (S_{\st 1},..., S_{\st m})\rightarrow(\underbrace{S_{\st\cap},..., S_{\st\cap}}_{\st m})$, where $S_{\st\cap}= S_{\st 1} \cap S_{\st 2}, ...,\cap\  S_{\st m}$.  

At a high level, the standard simulation-based paradigm ensures only privacy and output correctness \cite{DBLP:books/cu/Goldreich2004}. To enhance the simulation-based model and accommodate additional security requirements (such as fairness, compensation, or transactions' correctness) researchers often follow these steps: (i) define a set of predicates and (ii) use a wrapper that encapsulates and parameterizes the original paradigm with the defined predicates. This approach can be observed in \cite{KiayiasZZ16,BadertscherMTZ17,BadertscherGKRZ19}. Hence, to formally define a \p, we parameterize $f^{\st\text{PSI}}$ with four predicates,  $Q:=(\qinit, \qdel, \qUnFAbt, \qFAbt)$, which ensure that certain financial conditions are met. We borrow three of these predicates (i.e., $\qinit, \qdel, \qUnFAbt$) from \cite{KiayiasZZ16}. But, we will (i) introduce an additional predicate  \qFAbt and (ii) provide more formal accurate definitions of these predicates. %Below, we provide a brief description of these predicates.% (in Appendix \ref{sec::Formal-Definitions-of-F-PSI-Predicates}). 






   %  that are invoked after the functionality $f^{\st \text{PSI}}$ is executed. 
%   We borrow  $\qinit, \qdel$ and $\qUnFAbt$ from \cite{KiayiasZZ16}; nevertheless, we will (i) introduce an additional predicate  \qFAbt and (ii) provide more formal accurate definitions of these predicates. 

\vspace{-1mm}
\begin{itemize}[leftmargin=4mm]
    \item[$\bullet$] \underline{\qinit:  Initiation predicate}. It defines the conditions under which a protocol realizing \p should begin execution, i.e., when all set owners have sufficient deposit. 
 
  \item[$\bullet$] \underline{\qdel: Delivery predicate}. It defines the circumstances in which parties receive their output, specifically when honest parties receive their deposit back.
 
  \item[$\bullet$] \underline{\qUnFAbt: UnFair-Abort predicate}. It specifies the conditions under which the simulator can force parties to abort if the adversary learns the output, i.e., when an honest party receives its deposit back along with a predefined amount of compensation.
 
 
 
 \item[$\bullet$] \underline{\qFAbt: Fair-Abort predicate}. It specifies the conditions under which the simulator can compel parties to abort if the adversary receives no output, i.e., when honest parties receive their deposits. 
 
   \end{itemize}
   \vspace{-1mm}
%
%We observed that the latter predicate should have been defined in the generic framework in \cite{KiayiasZZ16} too; as the framework should have also captured the cases where an adversary may abort without learning any output after the onset of the protocol.  

By requiring any protocol that realizes \p, to implement a wrapped version of $f^{\st\text{PSI}}$ that includes $Q$, we will ensure that an honest set owner only aborts unfairly if \qUnFAbt returns  $1$, it only aborts in a fair manner if \qFAbt returns  $1$, and outputs a valid value if \qdel returns $1$. Appendix \ref{sec::Formal-Definitions-of-F-PSI-Predicates} presents formal definitions of these predicates.   Next, we present a formal definition of \p. 
 

% 
% 
% \begin{definition}
% %
%  [\qinit: Initiation predicate] Let $\mathcal{G}$ be a stable ledger, $adr_{\st sc}$ be smart contract $sc$'s address, $Adr$ be a set of $m+1$ distinct addresses, and $\xc$ be a fixed amount of coins. Then, predicate $\qinit(\mathcal{G}, adr_{\st sc}, m+1, Adr, \xc)$ returns $1$ if every address in $Adr$ has at least $\xc$ coins in $sc$; otherwise, it returns $0$. 
% %
% \end{definition}
%
% 
% 
%    \begin{definition}  [\qdel:
%    %
%    Delivery predicate] Let $pram:=(\mathcal{G}, adr_{\st sc}, \xc)$ be the parameters defined above, and   $adr_{\st i}\in Adr$ be the address of an honest party. 
%    %
%%    Let also $G$ be a compensation function that takes as input  two parameters $(deps, m')$, where $deps$ is the amount of coins  that all $m+1$ parties  deposit; it returns the amount of compensation each honest party must receive, i.e., $G(deps, m')\rightarrow c'$. 
%    %
%    Then, predicate $\qdel(pram, adr_{\st i})$ returns $1$ if $adr_{\st i}$ has sent $\xc$ amount to $sc$ and received  $\xc$ amount from it; thus,  its balance in $sc$ is $0$. Otherwise, it returns $0$. 
% %
%  \end{definition}
% 
% 
% 
%   \begin{definition}  [\qUnFAbt: UnFair-Abort predicate]
%   %
% Let $pram:=(\mathcal{G}, adr_{\st sc}, \xc)$ be the parameters defined above, and $Adr'\subset Adr$ be a set containing honest parties' addresses, $m' = |Adr'|$,  and   $adr_{\st i}\in Adr'$. Let also $G$ be a compensation function that takes as input  three parameters $(\depsc, adr_{\st i}, m')$, where $\depsc$ is the amount of coins  that all $m+1$ parties  deposit. It returns the amount of compensation each honest party must receive, i.e., $G(\depsc, ard_{\st i}, m')\rightarrow \xci$. Then, predicate $\qUnFAbt$ is defined as $\qUnFAbt(pram, G, \depsc, m', adr_{\st i})\rightarrow (a,b)$, where $a=1$ if $adr_{\st i}$ is an honest party's address and $adr_{\st i}$ has sent $\xc$ amount to $sc$ and received  $\xc+\xci$  from it, and $b=1$ if $adr_{\st i}$ is \aud's address and $adr_{\st i}$ received $\xci$  from $sc$. Otherwise, $a=b=0$. 
%  %
%  \end{definition}
%  
%  
%\begin{definition}  [\qFAbt: Fair-Abort predicate]
%   %
% Let $pram:=(\mathcal{G}, adr_{\st sc}, \xc)$ be the parameters defined above, and $Adr'\subset Adr$ be a set containing honest parties' addresses, $m' = |Adr'|$,     $adr_{\st i}\in Adr'$, and  $adr_{\st j}$ be \aud's address. Let $G$ be the compensation function, defined above and let $G(deps, ard_{\st j}, m')\rightarrow \xc_{\st j}$ be the compensation that the auditor must receive.  Then, predicate $\qFAbt(pram, G, \depsc, m', adr_{\st i}, adr_{\st j})$ returns $1$, if $adr_{\st i}$ (s.t. $adr_{\st i}\neq adr_{\st j}$) has sent $\xc$ amount to $sc$ and received  $\xc$  from it, and $adr_{\st j}$ received $\xc_{\st j}$  from $sc$. Otherwise, it returns $0$. 
%  %
% \end{definition}
  
  
  
 
%Note that we have upgraded the simulation-based definition of secure computation (i.e., Definition \ref{def::MPC-active-adv}) to define the security requirements of \p, by incorporating the above predicates into the definition. 
 
 \vspace{-1mm}
 
\begin{definition}[\p]\label{def::PSI-Q-fair}
Let $f^{\st \text{PSI}}$ be the functionality defined above. Protocol $\Gamma$ realizes  $f^{\st \text{PSI}}$ with $Q$-fairness in the presence of $m-1$ active-adversary clients or a passive dealer $D$ or auditor $Aud$, if for every PPT adversary $\mathcal{A}$ for the real model, there is a PPT  simulator $\mathsf{Sim}$ for the ideal model, such that for every $I\in \{A_{\st 1},...,A_{\st m}, D, Aud\}$, it holds that: 
%\begin{equation*}
$\{\mathsf {Ideal}^{\st \mathcal{W}(f^{\st \text{PSI}},Q)}_{\st \mathsf{Sim}(z), I}(S_{\st 1},..., S_{\st m+1})\}_{\st S_{\st 1},..., S_{\st m+1},z}\stackrel{c}{\equiv} \{\mathsf{Real}_{\st \mathcal{A}(z), I}^{\st \Gamma}(S_{\st 1},$ $..., S_{\st m+1}) \}_{\st S_{\st 1},..., S_{\st m+1}, z}$,  
%\end{equation*}
where  $z$ is an auxiliary input given to $\mathcal{A}$ and  $\mathcal{W}(f^{\st \text{PSI}},Q)$ is a functionality that wraps $f^{\st \text{PSI}}$ with predicates $Q:=(\qinit, \qdel,$ $\qUnFAbt, \qFAbt)$. 
  \end{definition}
 

 

  
\input{Sub-protocols.tex}
  
\input{Unforgeable-polynomials}


 \vspace{-2mm}
\section{Concrete Construction of \p}

\vspace{-1mm}
 
% %%%%%%%%%%%%%
%\subsection{Main Challenges to Overcome}
%
% We need to address several key challenges, to design an efficient scheme that realises \p. Below, we outline these challenges.
% 
%  \vspace{-1mm}
% \subsubsection{Keeping Overall Complexities Low.}
% 
% In general, in multi-party PSIs, each client needs to send messages to the rest of the clients and/or engage in secure computation with them, e.g., in \cite{DBLP:conf/scn/InbarOP18,DBLP:conf/ccs/KolesnikovMPRT17}, which would result in communication and/or computation quadratic with the number of clients. To address this challenge, we  (a) allow one of the clients as a dealer to interact with the rest of the clients,\footnote{This approach has similarity with the non-secure PSIs in \cite{GhoshN19}.} and   (b) we use a smart contract, which acts as a bulletin board to which most messages are sent and also performs lightweight computation on the clients' messages. The combination of these approaches will keep the overall communication and computation linear with the number of clients (and sets' cardinality). 
% 
% 
% \vspace{-2mm}
% 
% \subsubsection{Randomising Input Polynomials.}  In multi-party PSIs that use the polynomial representation, it is essential that a client's input polynomial be randomised by another client \cite{AbadiMZ21}. To do that securely and efficiently, we require the dealer and each client together to engage in an instance of \vopr, which we developed in Section \ref{sec::subroutines}. 
% 
%  \vspace{-2mm}
% 
% \subsubsection{Preserving the Privacy of Outgoing Messages.} Although the use of public smart contracts (e.g., Ethereum) will help keep overall complexity low, it introduces another challenge; namely, if clients do not protect the privacy of the messages they send to the smart contracts, then other clients (e.g., dealer) and non-participants of PSI (i.e., the public) can learn the clients' set elements and/or the intersection. To efficiently protect the privacy of each client's messages (sent to the contracts) from the dealer, we require the clients (except the dealer) to engage in \zspaa which lets each of them generate a pseudorandom polynomial with which it can blind its message. To protect the privacy of the intersection from the public, we require all clients to run a coin-tossing protocol to agree on a blinding polynomial, with which the final result that encodes the intersection on the smart contract will be blinded.  
% 
% 
%  \vspace{-2mm}
% \subsubsection{Ensuring the Correctness of Subroutine Protocols' Outputs.} 
% 
% In general, any MPC that must remain secure against an active adversary is equipped with a verification mechanism that ensures an adversary is detected if it affects messages' integrity, during the protocol's execution. This is the case for the subroutine protocols that we use, i.e., \vopr and \zspaa. However, this type of check itself is not always sufficient. Because in certain cases, the output of an MPC may be fed as input to another MPC and we need to ensure that the \emph{intact} output of the first MPC is fed to the second one. This is the case in our PSI's subroutines too. To address this challenge, we use unforgeable polynomials; specifically, the output of \vopr is an unforgeable polynomial (that encodes the actual output). If the adversary tampers with the \vopr's output and uses it later, then a verifier can detect it. We will have the same integrity guarantee for the output of \zspaa for free. Because (i) \vopr is called before \zspaa, and (ii) if clients use intact outputs of \zspaa, then the final result (i.e., the sum of all clients' messages) will not contain any output of \zspaa, as they will cancel out each other. Thus, by checking the correctness of the final result, one can ensure the correctness of the outputs of \vopr and \zspaa, in one go. 
% %%%%%%%%%%%%%%
 
 


  
\subsection{An Overview of \withFai (\fpsi)}\label{Fair-PSI-Protocol}
%This section presents \fpsi, a protocol that realises \p. 
 \vspace{-.5mm}

At a very high level, \withFai (\fpsi) operates as follows. Initially, each client encodes its set elements into a polynomial. All clients collectively sign a smart contract \scf and make a predefined coin deposit into it. One of the clients, designated as the dealer, $D$, takes on the responsibility of randomizing the polynomials of the remaining clients and applying a specific structure to their respective polynomials. The clients also randomize $D$'s polynomials. Next, all clients transmit their randomized polynomials to \scf.  

 \scf consolidates all the polynomials and verifies whether the resultant polynomial adheres to the structure imposed by $D$. If it determines that the resultant polynomial lacks the prescribed structure, it triggers an auditor, \aud, to identify clients who may have acted improperly and impose penalties on them. However, if the resultant polynomial indeed maintains the required structure,  \scf produces an encoded polynomial and reimburses the deposits made by the clients. In this case, all clients can utilize the encoded polynomial (provided by \scf) to find the intersection. Figure \ref{fig:parties-interactions-in-Jus} in Appendix \ref{sec::Justitia-workflow} outlines the interaction among the parties. 





%%%%%%%%%%%%


One of the novelties of \fpsi is its lightweight verification mechanism, which enables a smart contract  \scf to efficiently validate the accuracy of clients' messages while preserving the confidentiality of the clients' set elements. To achieve this, $D$ randomizes each client's polynomials and constructs unforgeable polynomials on the randomized polynomials.  If any client alters an unforgeable polynomial it receives and subsequently sends the modified polynomial to \scf,  then  \scf can detect this manipulation by verifying if the sum of all clients' (unforgeable) polynomials is divisible by a specific polynomial of degree $1$.  This verification process is considered lightweight for several reasons: (i) it does not use any public key cryptography, which can often be computationally expensive, (ii) it only requires polynomial division, and (iii) it can perform batch verification by aggregating all clients' randomized polynomials and then verifying the correctness of the result. 


%%%%%%%%%%%%





Now, we will delve into a more detailed description of \fpsi. Initially, all clients sign and deploy \scf, each contributing a predetermined deposit amount to it. Then, they collectively execute a coin-tossing protocol \ct to reach a consensus on a key, $mk$. This key will be used to generate a series of blinding polynomials, concealing the final result from the public. 
%
Following this, each client maps its set elements to a hash table and represents the contents of each bin (in the hash table) as a polynomial, $\bm\pi$. 

Afterward, for each bin, the following steps are undertaken.  All clients, excluding $D$, participate in \zspaa to reach an agreement on a set of pseudorandom blinding factors, ensuring that their sum equals zero. 
%
Next, $D$ takes on the task of randomizing each client's polynomial $\bm\pi$ and constructing an unforgeable polynomial on it. To achieve this, $D$ and every other client, $C$, participate in \vopr. This process results in
$C$ receiving a polynomial. Following this, $D$ and each $C$ invoke \vopr once more, this time to randomize $D$'s polynomial, resulting in $C$ obtaining another unforgeable polynomial. 
%
Note that the output of \vopr does not reveal any information about any client's original polynomial $\bm\pi$. This is because $D$  has previously concealed this polynomial with another secret random polynomial during the execution of
  \vopr. 
  
  Each $C$ adds the two polynomials together, applies blinding factors (using the output of  \zspaa), and then forwards the result to \scf. 
%
 Once all clients have transmitted their input polynomials to \scf, $D$ sends a \textbf{switching polynomial}  to \scf.  This switching polynomial allows \scf to obliviously alter the secret blinding polynomials previously employed by $D$ during the execution of \vopr. This alteration ensures that each client's original polynomial $\bm \pi$ is blinded with a different blinding polynomial, which can be independently removed by the clients using  $mk$.  

Following this, $D$ transmits a secret polynomial $\bm\zeta$ to \scf. This polynomial enables \scf to validate the correctness of unforgeable polynomials. Subsequently, \scf sums all clients' polynomials together and checks if $\bm\zeta$ can divide the sum. \scf approves the clients' inputs if the polynomial can divide the sum; otherwise, it invokes \aud to identify misbehaving parties.  


In case of misbehavior, all honest parties receive a refund of their deposits, while the deposits of the misbehaving parties are redistributed among the honest ones. If all clients behave honestly,  then each client can independently ascertain the intersection. To achieve this, they use $mk$ to remove the blinding polynomial from the sum (that the contract generated), evaluate the unblinded polynomial at each of their set elements, and consider an element to be part of the intersection if the evaluation yields zero. 


 

\vspace{-2.5mm}
\subsection{Detailed Description of \fpsi.} Now, we will elaborate on how \fpsi operates (for a description of the main notations used, see Table \ref{table:notation-table} in Appendix \ref{sec::notation-table}). 




\vspace{-1mm}
\begin{enumerate}[leftmargin=.55cm]


\item\label{gen-FPSI-cont} All clients in $\cl=\{ A_{\st 1},...,   A_{\st m},  D\}$ sign a smart contract: \scf and deploy it to a blockchain. Each client obtains the address of the deployed contract. Also, all clients participate in \ct to agree on a secret master key, $mk$.

\item \label{encode-encrypt} Each client in $\cl$  builds a  hash table,  $\mathtt{HT}$, and inserts the set elements into  it, i.e.,  $\forall i: \mathtt{H}( s_{\st i})={indx}$, then $ s_{\st i}\rightarrow \mathtt{HT}_{\st indx}$. It pads every bin with random dummy elements to $d$ elements (if needed). Then,  for every bin, it constructs a polynomial whose roots are the bin's content: $\bm\pi=\prod\limits^{\st d}_{\st i=1} (x-s'_{\st i})$, where $s'_{\st i}$ is either $s_{\st i}$ or a random value. 
%
\item \label{ZSPA} Every client $ C$ in $\cl\setminus D$, for every bin, agree on $b=3d+3$ vectors of pseudorandom blinding factors: $z_{\st i,j}$, such that the sum of each vector elements is zero, i.e., $\sum\limits^{\st m}_{\st j=1}z_{\st i,j}=0$, where $0\leq i\leq b-1$. To do that, they participate in step \ref{ZSPA::ZSPA-invocation} of \zspaa. By the end of this step, for each bin, they agree on a secret key $k$ (that will be used to generate the zero-sum values) as well as two values stored in $\mathcal{SC}_{\st\fpsi}$, i.e., $q$: the key's hash value and $g$: a Merkle tree's root. After time $t_{\st 1}$,  $D$ ensures that all other clients have agreed on the vectors (i.e., all provided ``approved''  to the contract). If the check fails, it halts. 
%
\item\label{F-PSI::each-client-deposit} Each client in $\cl$ deposits $\yc+\chc$ amount to $\mathcal{SC}_{\st\fpsi}$. After time $t_{\st 2}$, $\mathcal{SC}_{\st\fpsi}$ checks if $(\yc+\chc)\cdot (m+1)$ amount has been deposited. If the check fails, it refunds the clients' deposit and halts. 







\item\label{JUS::check-non-zero-coeff}  $D$ picks a  random polynomial $\bm\zeta \stackrel{\st\$}\leftarrow \mathbb{F}_{\st p}[X]$ of degree $1$, for each bin.  
It, for each  $C$, allocates to each bin two random polynomials: $\bm\omega^{\st(D,C)}, \bm\rho^{\st (D,C)}\stackrel{\st\$}\leftarrow \mathbb{F}_{\st p}[X]$ of degree $d$, and  two  random polynomials: $\bm\gamma^{\st (D,C)}, \bm\delta^{\st (D,C)} \leftarrow \mathbb{F}_{\st p}[X]$ of degree $3d+1$. Also, each $C$, for each bin, picks two  random polynomials: $\bm\omega^{\st (C,D)}, \bm\rho^{\st (C,D)}\stackrel{\st\$}\leftarrow \mathbb{F}_{\st p}[X]$ of degree $d$, and checks polynomials $\bm\omega^{\st (C,D)}\cdot \bm\pi^{\st  {  {(C)}}}$ and  $\bm\rho^{\st (C,D)}$ do not contain zero coefficients. Appendix \ref{sec::error-prob}, provides further discussion about this check. %It also evaluates each polynomial at every element of $\vv{\bm{x}}$ that results in  $\omega^{  {  {D,C}}}_{\st i}$ and $\rho^{  {  {D,C}}}_{\st i}$.


\item\label{e-psi::D-randomises}  $D$ randomizes other clients' polynomials. To do so, for every bin, it invokes an instance of {\vopr} (presented in Fig. \ref{fig:VOPR}) with each client $  C$; where  $D$ sends $\bm\zeta \cdot \bm\omega^{\st  {  {(D,C)}}}$ and $\bm\gamma^{\st  {  {(D,C)}}}$, while client $ C$ sends $\bm\omega^{\st  {  {(C,D)}}}\cdot \bm\pi^{\st  {  {(C)}}}$ to {\vopr}. Each client $C$, for every bin, receives a blinded polynomial of the following form: 
%
 \vspace{-1.3mm}
$$\bm\theta^{  {  {(C)}}}_{\st 1}=\bm\zeta \cdot \bm\omega^{\st  {  {(D,C)}}}\cdot \bm\omega^{\st  {  {(C,D)}}}\cdot \bm\pi^{\st  {  {(C)}}}+\bm\gamma^{\st  {  {(D,C)}}}$$

 \vspace{-1.6mm}

 from {\vopr}. If any party aborts, all parties receive their deposit. %the deposit would be refunded to all parties.

\item\label{e-psi::C-randomises} Each client $    {  C}$ randomizes  $ {D}$'s polynomial. To do that, each client $    {  C}$, for each bin,  invokes an instance of {\vopr} with   $ {D}$,    where each client $    {  C}$  sends $\bm\rho^{\st  {  {(C,D)}}}$, while  ${D}$  sends $\bm\zeta\cdot\bm \rho^{\st  {  {(D,C)}}}\cdot \bm\pi^{  {  {(D)}}}$ and $\bm\delta^{\st  {  {(D,C)}}}$ to {\vopr}. Every client   $    {  C}$, for each bin,  receives a blinded polynomial of the following form: 
%

 \vspace{-2.5mm}

$$\bm\theta^{  {  {(C)}}}_{\st 2}=\bm\zeta \cdot \bm\rho^{\st  {  {(D,C)}}}\cdot \bm\rho^{\st  {  {(C,D)}}}\cdot \bm\pi^{\st  {  {(D)}}}+\bm\delta^{\st  {  {(D,C)}}}$$

 \vspace{-1mm}
 
 from {\vopr}. If a party aborts, all parties get their deposit back. 


\item\label{blindPoly-C-sends-to-contract} Each client $ C$, for every bin, blinds the sum of polynomials $\bm\theta^{\st  {  {(C)}}}_{\st 1}$ and $\bm\theta^{\st  {  {(C)}}}_{\st 2}$  using the blinding factors: $z_{\st i,c}$, generated in step \ref{ZSPA}. Specifically, it computes the following blinded polynomial (for every bin):  
%
$\bm\nu^{ \st {  {(C)}} }= \bm\theta^{ \st {  {(C)}}}_{\st 1}+\bm\theta^{\st  {  {(C)}}}_{\st 2}+\bm \tau^{\st  {  {(C)}} }$, 
%
where $\bm\tau^{\st  {  {(C)}}}=\sum\limits^{\st 3d+2}_{\st i=0}z_{\st i,c}\cdot x^{\st i}$. Next, it sends  all $\bm\nu^{\st  {  {(C)}} }$ to $\mathcal{SC}_{\st\fpsi}$. If any party aborts, the deposit will be refunded to all parties.


%\item Client $    {  D}$ ensures all clients have sent their inputs to $\mathcal{SC}_{  {   {F-PSI}}}$. In the case where $m'$ parties do not provide their inputs, client $    {  D}$ aborts. In this case, the rest (including the dealer) get their deposit back. Also,  the deposit of the parties who did not send  inputs would be evenly distributed among the rest. The total amount each party above receives is: $y+\frac{m'\cdot y}{m-m'}$




%%
%\item Client $    {  D}$ and each client $    {  C}$ collaboratively, for each bin, generate a polynomial that will be used to (obliviously) check if  $    {  C}$ misbehaved during the computation of each $\bm\nu^{  {  {(C)}} }$. To do so, for every bin, client $    {  D}$ invokes an instance of $\mathtt{VOPR}$ with  each client $    {  C}$, where  client $    {  D}$ sends: $\bm\zeta$, while client $    {  C}$ sends $\bm\xi^{  {  {(C)}}}$ and $-\bm\tau^{  {  {(C)}}}$   to $\mathtt{VOPR}$, where $\bm\xi^{  {  {(C)}}}$ is a random polynomial of degree $3d+1$. Client $    {  D}$ for each  $    {  C}$'s bin recives the following polynomial: 
%%
%$$\bm\mu^{  {  {(D,C)}}} = \bm\zeta\cdot \bm\xi^{  {  {(C)}}}-\bm\tau^{  {  {(C)}}}$$
%%




\item\label{f-psi::D-gen-random-poly} ${D}$ ensures all clients sent their inputs to $\mathcal{SC}_{\st\fpsi}$. If the check fails, it halts and the deposit is refunded to all parties. Otherwise, it allocates a pseudorandom polynomial $\bm\gamma'$ of degree $3d$, to each bin. To do so, it uses $mk$ to derive a key for each bin: $k_{\st  { {indx}}}=\mathtt{PRF}(mk, {    {   {indx}}})$ and  uses $k_{\st  { {indx}}}$ to generate $3d+1$ pseudorandom coefficients $g_{\st  { {j,indx}}}=\mathtt{PRF}(k_{\st  { {indx}}}, j)$ where $ 0\leq j \leq 3d$. Also, for each bin, it allocates a  random polynomial  $\bm\omega'^{\st  {  {(D)}}}$ of degree $d$. 

\item\label{f-psi::D-gen-switching-poly}  $ {D}$,  for every bin, computes a switching polynomial of the form:  
 \vspace{-3.8mm}
$$\bm\nu^{\st  {  {(D)}}}=\bm\zeta \cdot  \bm\omega'^{\st  {  {(D)}}}\cdot \bm\pi^{\st  {  {(D)}} }-\sum\limits^{\st  {   A}_{\st  {   m}}}_{\st   {  {C }= }   {   A}_{\st  {  1}}}(\bm\gamma^{\st  {  {(D,C)}}} + \bm\delta^{\st  {  {(D,C)}}}) + \bm\zeta \cdot \bm\gamma'$$ 
%
 \vspace{-3mm}
 
It sends to $\mathcal{SC}_{\st\fpsi}$  polynomials $\bm\nu^{\st  {  {(D)}}}$ and $\bm\zeta$, for each bin.

 \item\label{compute-res-poly}  $\mathcal{SC}_{\st\fpsi}$ takes the following steps:
 \begin{enumerate}[leftmargin=.7mm]
 \item for every bin, sums all related polynomials  provided by all clients in $\bar{P}$:
 %
  \vspace{-1mm}
 \begin{equation*}
 \begin{split}
 \bm\phi&= \bm\nu^{\st  {  {(D)}} }+\sum\limits^{\st  {   A}_{\st  {   m}}}_{\st   {  {C }= }   {   A}_{\st  {  1}}}\bm\nu^{\st  {  {(C)}} }= \bm\zeta\cdot \Big(\bm\omega'^{\st  {  {(D)}}}\cdot \bm\pi^{\st  {  {(D)}} } +\sum\limits^{\st  {   A}_{  {   m}}}_{\st  {  {C }= }   {   A}_{\st  {  1}}}(\bm\omega^{\st  {  {(D,C)}}} \cdot \bm\omega^{\st  {  {(C,D)}}}\cdot\\&\cdot \bm\pi^{\st  {  (C)}}) +\bm\pi^{\st  {  {(D)}}}\cdot\sum\limits^{\st  {   A}_{ \st {   m}}}_{\st  {C= }   {   A}_{\st  {  1}}}(\bm\rho^{\st  {  {(D,C)}}} \cdot \bm\rho^{\st  {  {(C,D)}}}) + \bm\gamma'\Big)
 \end{split}
\end{equation*}
  \vspace{-3mm}
 
 
 
 
 
 
 %
% \vspace{-1mm}
% \begin{equation*}
% \begin{split}
% \bm\phi&= \bm\nu^{\st  {  {(D)}} }+\sum\limits^{\st  {   A}_{\st  {   m}}}_{\st   {  {C }= }   {   A}_{\st  {  1}}}\bm\nu^{\st  {  {(C)}} }= \bm\zeta\cdot (\bm\omega'^{\st  {  {(D)}}}\cdot \bm\pi^{\st  {  {(D)}} } +\\&+\sum\limits^{\st  {   A}_{  {   m}}}_{\st  {  {C }= }   {   A}_{\st  {  1}}}(\bm\omega^{\st  {  {(D,C)}}} \cdot \bm\omega^{\st  {  {(C,D)}}}\cdot \bm\pi^{\st  {  (C)}}) +\bm\pi^{\st  {  {(D)}}}\cdot\sum\limits^{\st  {   A}_{ \st {   m}}}_{\st  {C= }   {   A}_{\st  {  1}}}(\bm\rho^{\st  {  {(D,C)}}} \cdot \bm\rho^{\st  {  {(C,D)}}}) + \bm\gamma')
% \end{split}
%\end{equation*}
%  \vspace{-3mm}
 
 
 
 
 
 
 
 
% \begin{equation*}
%\begin{split}
% \bm\phi&= \bm\nu^{\st  {  {(D)}} }+\sum\limits^{\st  {   A}_{\st  {   m}}}_{\st   {  {C }= }   {   A}_{\st  {  1}}}\bm\nu^{\st  {  {(C)}} }\\
% &= \bm\zeta\cdot \bigg(\bm\omega'^{\st  {  {(D)}}}\cdot \bm\pi^{\st  {  {(D)}} } +\sum\limits^{\st  {   A}_{  {   m}}}_{\st  {  {C }= }   {   A}_{\st  {  1}}}(\bm\omega^{\st  {  {(D,C)}}} \cdot \bm\omega^{\st  {  {(C,D)}}}\cdot \bm\pi^{\st  {  (C)}}) +\bm\pi^{\st  {  {(D)}}}\cdot\sum\limits^{\st  {   A}_{ \st {   m}}}_{\st  {C= }   {   A}_{\st  {  1}}}(\bm\rho^{\st  {  {(D,C)}}} \cdot \bm\rho^{\st  {  {(C,D)}}}) + \bm\gamma'\bigg)
%  \end{split}
%\end{equation*}
% \item\label{F-PSI:detect-misbehaving-party} ensures that, for every bin, $\bm\zeta$ divides $\bm\phi$. Otherwise, it aborts and Arbiter protocol (presented in Fig. \ref{fig:arbiter}) is invoked to find misbehaving parties.
 
  \item\label{F-PSI:detect-misbehaving-party} checks whether, for every bin, $\bm\zeta$ divides $\bm\phi$. If the check passes, it sets $Flag=True$. Otherwise, it sets $Flag=False$. 
  
   %aborts and Arbiter protocol (presented in Fig. \ref{fig:arbiter}) is invoked to find misbehaving parties.
 
 
% \item if the check passes (i.e., $Flag=True$), each party gets back its deposit (i.e., $y$ amount).
 \end{enumerate}
 
\item\label{F-PSI::flag-is-true} If $Flag=True$, then the following steps are taken:

\begin{enumerate}[leftmargin=.7mm]
 \item $\mathcal{SC}_{\st\fpsi}$ sends back each party's deposit, i.e., $\yc+\chc$ amount.
 
  \item each client (given $\bm\zeta$ and $mk$) finds the elements in the intersection as follows. 
  \begin{enumerate}
  \item derives a bin's pseudorandom polynomial, $\bm\gamma'$, from $mk$. 
  
  \item removes the blinding polynomial from each bin's polynomial:  
 %
  $\bm\phi'=\bm\phi-\bm\zeta\cdot \bm\gamma'$.
  
  \item\label{F-PSI::find-intersection} evaluates each bin's unblinded polynomial at every element $s_{\st i}$ belonging to that bin and considers the element in the intersection if the evaluation is zero: i.e., $\bm\phi'(s_{\st i})=0$.
 
 \end{enumerate}
 
 
 \end{enumerate}
 
 \item\label{F-PSI::flag-is-false} If $Flag=False$, then the following steps are taken.
 
 

 
 \begin{enumerate}[leftmargin=.7mm]
 

 \item\label{auditor}  \aud asks every client $    {  C}$ to send to it the  $\mathtt{PRF}$'s key (generated in step \ref{ZSPA}), for every bin. It inserts the keys to $\vv k$.  It generates an empty list $\bar L$. Then, for every bin,  \aud takes step \ref{ZSPA-A::Auditor-computation} of \zspaa, i.e., invokes  $\mathtt{Audit}(m, \vv{{k}},  q, \bm\zeta, 3d+3, g)\rightarrow (L, \vv{{\mu}})$.  Every time it invokes $\mathtt{Audit}$, it appends the elements of returned $L$ to $\bar L$.  \aud for each bin sends  $ \vv{{\mu}}$ to $\mathcal{SC}_{\st\fpsi}$. It also sends to $\mathcal{SC}_{\st\fpsi}$ the list $\bar L$ of all misbehaving clients detected so far. The above check allows \aud to identify clients who misbehaved in \zspaa. 
 

 
 \item to  help identify further  misbehaving clients, $D$ takes the following steps,  for each bin of client $    {  C}$ whose ID is not in $\bar L$.   
 \begin{enumerate}
 \item\label{gen-unmaking-poly} computes polynomial $\bm\chi^{  {  {(D, C)}}}$ as follows. 
 %
 \vspace{-.3mm}
 %
 $$\bm\chi^{ \st {  {(D, C)}}}=\bm\zeta\cdot \bm\eta^{ \st {  {(D,C)}}}-(\bm\gamma^{ \st {  {(D,C)}}}+\bm\delta^{ \st {  {(D,C)}}})$$
 
 \vspace{-1mm}
 
  where $\bm\eta^{ \st {  {(D,C)}}}$ is a fresh random polynomial of degree $3d+1$. 
  
  \item\label{send-unmaking-poly} sends  polynomial $\bm\chi^{ \st {  {(D, C)}}}$ to  $\mathcal{SC}_{\st\fpsi}$. 
  

 \end{enumerate}
  Note, if $\bar L$ contains all clients' IDs, then $D$ does not need to take the above steps \ref{gen-unmaking-poly} and \ref{send-unmaking-poly}. 
 %%%%%%%%%%%%%%%%%%%%%%
 
 \item  $\mathcal{SC}_{\st\fpsi}$,   takes the following steps to check if the client misbehaved,  for each bin of client $    {  C}$ whose ID is not in $\bar L$.
 
 %for each client $    {  C}$'s bin, takes the following steps to check if the client misbehaved.
 
  \begin{enumerate}
  
 \item computes  polynomial $\bm\iota^{\st  {  {(C)}}}$ as follows: 
 
 $\bm\iota^{ \st {  {(C)}}}=\bm\chi^{\st  {  {(D, C)}}}+\bm\nu^{\st  {  {(C)}}} +\bm\mu^{ \st {  {(C)}}}  
 =\\ = \bm\zeta\cdot(\bm\eta^{ \st {  {(D,C)}}} + \bm\omega^{ \st {  {(D,C)}}}\cdot \bm\omega^{ \st {  {(C,D)}}}\cdot \bm\pi^{ \st {  {(C)}}}+\bm\rho^{ \st {  {(D,C)}}}\cdot \bm\rho^{ \st {  {(C,D)}}}\cdot \bm\pi^{ \st {  {(D)}}}+\bm\xi^{ \st {  {(C)}}})$\\ 
%
%  \begin{equation*}
%\begin{split}
% \bm\iota^{ \st {  {(C)}}}&=\bm\chi^{\st  {  {(D, C)}}}+\bm\nu^{\st  {  {(C)}}} +\bm\mu^{ \st {  {(C)}}} \\ 
% &=\bm\zeta\cdot(\bm\eta^{ \st {  {(D,C)}}} + \bm\omega^{ \st {  {(D,C)}}}\cdot \bm\omega^{ \st {  {(C,D)}}}\cdot \bm\pi^{ \st {  {(C)}}}+\bm\rho^{ \st {  {(D,C)}}}\cdot \bm\rho^{ \st {  {(C,D)}}}\cdot \bm\pi^{ \st {  {(D)}}}+\bm\xi^{ \st {  {(C)}}})
% \end{split}
%\end{equation*}
%
 where $\bm\mu^{ \st {  {(C)}}} \in \vv{\mu}$ was sent to $\mathcal{SC}_{\st\fpsi}$  by \aud in step \ref{auditor}.   
  \item checks if $\bm\zeta$  divides $\bm\iota^{ \st {  {(C)}}}$. If the check fails, it appends the client's ID to  a list $ L'$.
  %
  \end{enumerate}
   If $\bar L$ contains all IDs, $\mathcal{SC}_{\st\fpsi}$ does not take the above two steps. 

 %
   \item  $\mathcal{SC}_{\st\fpsi}$  refunds the honest parties' deposit. Also, it retrieves the total amount of  $\chc$ from the deposit of dishonest clients (i.e., those clients whose IDs are in $\bar L$ or $L'$) and sends it to \aud.  It also splits the remaining deposit of the misbehaving parties among the honest ones. Thus, each honest client  receives $\yc+\chc+\frac{m'\cdot (\yc+\chc)-\chc}{m-m'}$ amount in total, where $m'$ is the total number of misbehaving parties.
 
 
%  \item  $\mathcal{SC}_{  {   {F-PSI}}}$  refunds the honest parties' deposit and splits the deposit of the misbehaving parties (i.e., those clients whose IDs are in $\bar L$ or $L'$)  among the honest ones. Thus, each honest party would receive $y+\frac{m'\cdot y}{m-m'}$ amount in total, where $m'$ is the total number of misbehaving parties.
 %%%%%%%%%%%%%%%%%%%%%
  \end{enumerate}
  
% \item If  $Flag=False$,  then $\mathcal{SC}_{  {   {F-PSI}}}$,  for each client $    {  C}$'s bin, takes the following steps:
% 
%  \begin{enumerate}
%  
% \item computes the following polynomial: 
% 
%  \begin{equation*}
%\begin{split}
% \bm\iota^{  {  {(C)}}}&=\bm\chi^{  {  {(D, C)}}}+\bm\nu^{  {  {(C)}}} \\ 
% &=\bm\zeta\cdot(\bm\eta^{  {  {(D,C)}}} + \bm\omega^{  {  {(D,C)}}}\cdot \bm\omega^{  {  {(C,D)}}}\cdot \bm\pi^{  {  {(C)}}}+\bm\rho^{  {  {(D,C)}}}\cdot \bm\rho^{  {  {(C,D)}}}\cdot \bm\pi^{  {  {(D)}}}+\bm\xi^{  {  {(C)}}})
% \end{split}
%\end{equation*}
% 
%  \item checks if $\bm\zeta$  divides $\bm\iota^{  {  {(C)}}}$. If does not, it appends the client's ID to a  list, $L$.
%  
%  \end{enumerate}
 
% \begin{equation*}
%\begin{split}
% \bm\iota^{  {  {(C)}}}&=\bm\zeta\cdot \bm\eta^{  {  {(D,C)}}}-(\bm\gamma^{  {  {(D,C)}}}+\bm\delta^{  {  {(D,C)}}})+\bm\nu^{  {  {(C)}}}-\sum\limits^{\st 3d+1}_{\st i=0}z_{\st i,c}\cdot x^{\st i} \\ &=\bm\zeta\cdot(\bm\eta^{  {  {(D,C)}}} + \bm\omega^{  {  {(D,C)}}}\cdot \bm\omega^{  {  {(C,D)}}}\cdot \bm\pi^{  {  {(C)}}}+\bm\rho^{  {  {(D,C)}}}\cdot \bm\rho^{  {  {(C,D)}}}\cdot \bm\pi^{  {  {(D)}}})
% \end{split}
%\end{equation*}
%  \item checks if $\bm\zeta$ can divide $\bm\iota^{  {  {(C)}}}$. If can not, it appends the client's ID to $L$.
% 
 

 
 
 
% \item Each client (given $\bm\zeta$ and $k_{\st 1}$), finds the elements in the intersection as follows. First, it derives a bin's pseudorandom polynomial: $\bm\gamma'$ from $k_{\st 1}$.  Next, it removes the blinding polynomial from each bin's polynomial: $\bm\phi'=\bm\phi-\bm\zeta\cdot \bm\gamma'$. Then, it evaluates each bin's unblinded polynomial at every  element belonging to that bin and considers the element in the intersection if the evaluation is zero: i.e. $\bm\phi'(s^{  {  {(I)}}}_{\st i})=0$
 
  \end{enumerate}
 
% the result: $cccc$ by locally evaluating the result polynomial: $\phi(x)$, at every  encrypted element, $e^{  {  {(I)}}}_{\st i}$, it has and considering the elements in the intersection if the following equation holds.  $\forall i, 1\leq i\leq d: \phi(e^{  {  {(I)}} }_{\st i})-\zeta(e^{  {  {(I)}}}_{\st i})\cdot \gamma'(e^{  {  {(I)}}}_{\st i})=0$.
 
 
 
%\begin{remark} After the Arbiter detects  misbehaving parties,  in step \ref{F-PSI:detect-misbehaving-party},  it sends their ID's to $\mathcal{SC}_{  {   {F-PSI}}}$ which refunds the honest parties' deposit and splits the misbehaving parties' deposit among the honest ones. Thus, each honest party would receive: $y+\frac{m'\cdot y}{m-m'}$ amount in total, where $m'$ is the total number of misbehaving parties.
% \end{remark}
 
  \vspace{-1mm}

%\begin{remark}

We refer readers to Appendix \ref{sec::Discussion-justitia} for a more in-depth discussion of $\withFai$ which encompasses (i) the inadequacy of strawman approaches such as using a server-aided PSI or charging the buyer a flat fee, (ii) instructions on how to eliminate the check in step \ref{JUS::check-non-zero-coeff}, (iii) an outline of the primary challenges we addressed during $\withFai$ design, and (iv) choice of concrete (security) parameters.  

Next, we present a theorem formally stating the security of \fpsi. 
 
 \vspace{-1mm}
 
 \begin{theorem}\label{theorem::F-PSI-security}
Let polynomials $\bm\zeta$, $\bm\omega$, and $\bm\gamma$ be three secret uniformly random polynomials. If  $\bm\theta=\bm\zeta\cdot \bm\omega\cdot\bm \pi+\bm \gamma \bmod p$ is an unforgeable polynomial (w.r.t. Theorem \ref{proof::unforgeable-poly}), \zspaa, \vopr,  $\mathtt{PRF}$, and smart contracts are secure, then \fpsi securely realizes  $f^{\st \text{PSI}}$ with $Q$-fairness (w.r.t. Definition \ref{def::PSI-Q-fair}) in the presence of $m-1$  active-adversary clients (i.e., $A_{\st j}$s) or a passive dealer, auditor, or public. 
 \end{theorem}
 

 \vspace{-1mm}

We refer readers to Appendix \ref{sec::F-PSI-proof} for the proof of Theorem \ref{theorem::F-PSI-security}. 













 

==> CCS-24/Justitia-challenges.tex <==
% !TEX root =main.tex


%%%%%%%%%%%%%%%%%
 %%%%%%%%%%%%%
\subsection{Main Challenges that \withFai Overcomes}\label{sec::Justitia-challenges}

To design an efficient scheme that realizes \p,  we had to address several key challenges. Below, we outline these challenges.



 \subsubsection{Keeping Overall Complexities Low.}
 
 In general, in multi-party PSIs, each client must exchange messages with the other clients and potentially engage in secure computations with them, as seen in \cite{DBLP:conf/scn/InbarOP18,DBLP:conf/ccs/KolesnikovMPRT17}. This can lead to communication and computational costs that grow quadratically with the number of clients.
 
 To tackle this challenge, we employed two strategies: (a) allowing one of the clients to act as a dealer, interacting with the remaining clients\footnote{This approach has similarity with the non-secure PSIs in \cite{GhoshN19}.}, and (b) implementing a smart contract that serves as a bulletin board for receiving most messages and conducting lightweight computations on the clients' messages. The combination of these approaches ensures that the overall communication and computation remain linear in relation to the number of clients (and the cardinality of sets).



 
 
 \subsubsection{Randomising Input Polynomials.}  In multi-party PSIs that utilize the polynomial representation, it is crucial for a client's input polynomial to undergo randomization by another client \cite{AbadiMZ21}. To achieve this securely and efficiently, we required the dealer and each client to jointly participate in an instance of  \vopr, a protocol we developed in Section \ref{sec::subroutines}. 
 

 
 \subsubsection{Preserving the Privacy of Outgoing Messages.} 
 
 
 While the utilization of public smart contracts, such as Ethereum, helps maintain overall complexity low, it introduces another challenge. Specifically, if clients fail to safeguard the privacy of the messages they transmit to the smart contracts, then both other clients (e.g., the dealer) and individuals who are not participants in PSI (i.e., the public) can gain access to the clients' set elements and/or the intersection.
 
 To ensure the efficient protection of each client's messages sent to the contracts from the dealer, we necessitate that the clients, excluding the dealer, participate in \zspaa. This protocol allows each client to create a pseudorandom polynomial, which they can employ to obscure their messages. To safeguard the privacy of the intersection from the public, we require that  all clients to run a coin-tossing protocol to reach a consensus on a blinding polynomial.  This blinding polynomial will be used to obscure the final result that encodes the intersection on the smart contract.  
 
 

 \subsubsection{Ensuring the Correctness of Subroutine Protocols' Outputs.} 
 
 
 Typically, any MPC protocol designed to withstand active adversaries incorporates a verification mechanism to detect any tampering with message integrity during the protocol's execution. This applies to the subroutine protocols we utilize, namely \vopr and \zspaa. 
 
 
  However, relying solely on this type of check is not always adequate. There are situations where the output of one MPC serves as input to another MPC, and it becomes essential to guarantee that the unaltered output of the first MPC is securely passed to the second one. This holds for our PSI's subroutines as well. 
  
  To address this challenge, we employ unforgeable polynomials. Specifically, the output of \vopr is an unforgeable polynomial that encodes the actual output. If the adversary tampers with the \vopr's output and later uses it, then a verifier can detect this tampering. 
 
 We obtain the same integrity guarantee for the output of \zspaa without any additional effort. This is because (i) \vopr is called before \zspaa, and (ii) if clients use the unaltered outputs of \zspaa, then the final result (i.e., the sum of all clients' messages) will not contain any output of \zspaa, as they will cancel each other out. Thus, by verifying the correctness of the final result, one can ensure the correctness of the outputs of \vopr and \zspaa, in a single step. 
 %%%%%%%%%%%%%%





 


==> CCS-24/Merkle-tree-short.tex <==
% !TEX root =main.tex


\vspace{-1mm}

\subsection{Merkle Tree}\label{sec::merkle-tree-short}
\vspace{-.5mm}

A Merkle tree is a data structure that facilitates a concise commitment to a set of values or blocks, involving two parties: a prover and a verifier. 
%
The Merkle tree scheme includes three algorithms; namely, $\mathtt{MT.genTree}$, $ \mathtt{MT.prove}$, and  $\mathtt{MT.verify}$. Briefly, the first algorithm constructs a Merkle tree on a set of blocks, the second generates a proof of a block's (or set of blocks') membership, and the third verifies the proof. Appendix \ref{sec::merkle-tree} provides more details. 

%
%
%
% The  Merkle tree scheme includes three algorithms $(\mkgen, \mkprove,$ $\mkver)$, defined as follows: 
%
%\begin{itemize}
%%
%\item[$\bullet$] The algorithm that constructs a Merkle tree, $\mkgen$, is run by $\mathcal{V}$. It takes  blocks, $u:=u_{\st 1},...,u_{\st n}$, as input. Then, it groups the blocks  in pairs. Next,   a collision-resistant hash function, $\mathtt{H}(.)$, is used to hash each pair. After that, the hash values are grouped in pairs and each pair is further hashed, and this process is repeated until only a single hash value, called ``root'', remains. This yields a  tree with the leaves corresponding to the input blocks and the root corresponding to the last remaining hash value. $\mathcal{V}$ sends the root to $\mathcal{P}$.
%%
%\item[$\bullet$] The proving algorithm, $\mkprove$, is run by $\mathcal{P}$. It takes a block index, $i$, and a tree as inputs. It outputs a vector proof, of  $\log_{\st 2}(n)$ elements. The proof asserts the membership of $i$-th block in the tree, and consists of all the sibling nodes on a path from the $i$-th block to the root of the Merkle tree (including $i$-th block). The proof is given to $\mathcal{V}$.
%%
%\item[$\bullet$] The verification algorithm, $\mkver$, is run by $\mathcal{V}$. It takes as an input $i$-th block, a proof, and the tree's root. It checks if the $i$-th block corresponds to the root. If the verification passes, it outputs $1$; otherwise, it outputs $0$.
%
%\end{itemize}
%
%The Merkle tree-based scheme has two properties: \emph{correctness} and \emph{security}. Informally, the correctness requires that if both parties run the algorithms correctly, then a proof is always accepted by  $\mathcal{V}$. The security requires that a computationally bounded malicious $\mathcal{P}$ cannot convince  $\mathcal{V}$ into accepting an incorrect proof, e.g., proof for a non-member block. The security relies on the assumption that it is computationally infeasible to find the hash function's collision. Usually, for the sake of simplicity, it is assumed that the number of blocks, $n$, is a power of $2$. The height of the tree, constructed on $m$ blocks, is $\log_{\st 2}(n)$. 

==> CCS-24/Merkle-tree.tex <==
% !TEX root =main.tex


\section{Merkle Tree}\label{sec::merkle-tree}






A Merkle tree is a data structure that supports a compact commitment of a set of values/blocks.  As a result, it includes two parties, prover $\mathcal{P}$ and verifier $\mathcal{V}$. The  Merkle tree scheme includes three algorithms $(\mkgen, \mkprove,$ $\mkver)$, defined as follows: 

\begin{itemize}
%
\item[$\bullet$] The algorithm that constructs a Merkle tree, $\mkgen$, is run by $\mathcal{V}$. It takes  blocks, $u:=u_{\st 1},...,u_{\st n}$, as input. Then, it groups the blocks  in pairs. Next,   a collision-resistant hash function, $\mathtt{H}(.)$, is used to hash each pair. After that, the hash values are grouped in pairs and each pair is further hashed, and this process is repeated until only a single hash value, called ``root'', remains. This yields a  tree with the leaves corresponding to the input blocks and the root corresponding to the last remaining hash value. $\mathcal{V}$ sends the root to $\mathcal{P}$.
%
\item[$\bullet$] The proving algorithm, $\mkprove$, is run by $\mathcal{P}$. It takes a block index, $i$, and a tree as inputs. It outputs a vector proof, of  $\log_{\st 2}(n)$ elements. The proof asserts the membership of $i$-th block in the tree and consists of all the sibling nodes on a path from the $i$-th block to the root of the Merkle tree (including $i$-th block). The proof is given to $\mathcal{V}$.
%
\item[$\bullet$] The verification algorithm, $\mkver$, is run by $\mathcal{V}$. It takes as an input $i$-th block, a proof, and the tree's root. It checks if the $i$-th block corresponds to the root. If the verification passes, it outputs $1$; otherwise, it outputs $0$.

\end{itemize}

The Merkle tree-based scheme has two properties: \emph{correctness} and \emph{security}. Informally, the correctness requires that if both parties run the algorithms correctly, then a proof is always accepted by  $\mathcal{V}$. The security requires that a computationally bounded malicious $\mathcal{P}$ cannot convince  $\mathcal{V}$ into accepting an incorrect proof, e.g., proof for a non-member block. 
%
The security relies on the assumption that it is computationally infeasible to find the hash function's collision. Usually, for the sake of simplicity, it is assumed that the number of blocks, $n$, is a power of $2$. The height of the tree, constructed on $m$ blocks, is $\log_{\st 2}(n)$. 

==> CCS-24/Notations-Preliminaries.tex <==
% !TEX root =main.tex

\vspace{-2mm}

\section{Preliminaries}

\vspace{-.8mm}


Table \ref{table:notation-table} in Appendix \ref{sec::notation-table} summarizes the notations used in this paper. All arithmetic operations are defined over a field $\mathbb{F}_{p}$ of prime order. 

%\input{notation-Table}


\input{short-security-model}
%\input{Security-model}


\vspace{-3.1mm}

\subsection{Smart Contracts}
\vspace{-1mm}

Cryptocurrencies, such as Bitcoin \cite{bitcoin} and Ethereum \cite{ethereum},  go beyond merely providing a decentralized currency; they also facilitate computations on transactions. These cryptocurrencies allow for a specific computational logic to be encoded in a computer program known as a \emph{``smart contract''}.  As of now, Ethereum stands as the foremost cryptocurrency framework that empowers users to define arbitrary smart contracts. Within this framework, contract code resides on the blockchain and is executed by all parties involved in maintaining the cryptocurrency. The correctness of program execution is ensured by the security of the underlying blockchain components. In this work, \textbf{standard} public (Ethereum) smart contracts align with the requirements of our protocols.


%Cryptocurrencies, such as Bitcoin \cite{bitcoin} and Ethereum \cite{ethereum}, beyond offering a decentralised currency,  support computations on transactions. In this setting, often a certain computation logic is encoded in a computer program, called a \emph{``smart contract''}. To date, Ethereum is the most predominant cryptocurrency framework that enables users to define arbitrary smart contracts. In this framework,  contract code is stored on the blockchain and executed by all parties (i.e., miners) maintaining the cryptocurrency,  when the program inputs are provided by transactions. The program execution's correctness is guaranteed by the security of the underlying blockchain components. To prevent a denial-of-service attack, the framework requires a transaction creator to pay a  fee, called \emph{``gas''}, depending on the complexity of the contract running on it. 

\vspace{-3mm}

\subsection{Counter Collusion Smart Contracts}\label{Counter-Collusion-Smart-Contracts}
\vspace{-1mm}




To enable a party, such as a client, to efficiently delegate computation to multiple potentially colluding third parties, like servers, Dong   \et \cite{dong2017betrayal}  
introduced two primary smart contracts: the ``Prisoner's Contract'' ($\SCpc$) and the ``Traitor's Contract'' (\SCtc).  
%
$\SCpc$ is jointly signed by both the client and the servers and is designed to incentivize accurate computation. This contract mandates that each server must submit a deposit before the computation is delegated. Furthermore, it is equipped with an external auditor that can be invoked to identify any misbehaving server when it provides dissimilar results. 
%
If a server behaves honestly, it is eligible to withdraw its deposit. However, if the auditor detects a cheating server, a portion of its deposit is transferred to the client. If one server is honest while the other one cheats, the honest server receives a reward sourced from the deposit of the cheating server.

However, the dilemma, created by \SCpc between the two servers, can be resolved if they can establish an enforceable promise, such as through a ``Colluder's Contract'' (\SCcc). In this contract,  one party, referred to as the ``ringleader'', commits to paying a bribe to its counterpart if both parties engage in collusion and deliver an incorrect result to \SCpc. 
%
To counter \SCcc, Dong   \et proposed \SCtc, which provides incentives for a colluding server to expose the other server and report the collusion without facing penalties from \SCpc. In this work, we have made slight adjustments and employed these contracts. The relevant parameters for these contracts are outlined in Table \ref{table:notation-table}. For a comprehensive description of the contracts, we refer readers to Appendix \ref{appendix::Counter-Collusion-Contracts}. 


%
\vspace{-3mm}
\subsection{Pseudorandom Function and Permutation}
\vspace{-1mm}

A pseudorandom function is a deterministic function that takes a key of length $\lambda$ and an input; and outputs a value indistinguishable from that of  a truly random function.  In this paper, we use pseudorandom functions:   $\mathtt {PRF}: \{0,1\}^{\st \lambda}\times \{0,1\}^{\st *} \rightarrow  \mathbb{F}_{\st p}$, where $\log_{\st 2}(p)=\lambda$ is the security parameter. In practice, a pseudorandom function can be obtained from an efficient block cipher \cite{DBLP:books/crc/KatzLindell2007}. 
%
The definition of a pseudorandom permutation, $\mathtt {PRP}: \{0,1\}^{\st \lambda}\times \{0,1\}^{\st *} \rightarrow  \mathbb{F}_{\st p}$, is similar to that of a pseudorandom function, with a difference, it is required  $\PRP(k,.)$ to be indistinguishable from a uniform permutation, instead of a uniform function.  %In cryptographic schemes that involve $\PRP$, sometimes honest parties may require to compute the inverse of pseudorandom permutation, i.e., $\mathtt {PRP}^{\st -1}(k, .)$, as well. In this case, it would require that $\PRP(k,.)$ be indistinguishable from a uniform permutation even if the distinguisher is additionally given oracle access to the inverse of the permutation. 




%\subsection{Random Extraction Beacon}
%\subsection{Commitment Scheme}

\vspace{-2mm}

\input{short-commitment}

\vspace{-2.5mm}

\subsection{Hash Tables}
\vspace{-.5mm}

A hash table is an array of bins, each containing a set of elements, and is paired with a hash function. To insert an element, we compute the element's hash and place the element into the bin corresponding to the computed hash value. In this paper, we ensure that the number of elements in each bin does not surpass a predefined capacity. By considering the maximum number of elements as $c$ and the maximum size of a bin as $d$, we can calculate the number of bins, denoted as $h$, through an analysis of hash tables using the ``balls into the bins'' model  \cite{DBLP:conf/stoc/BerenbrinkCSV00}. Appendix \ref{Preliminary-Hash-Table} explains how the hash table parameters are configured. In this paper, we use hash tables to partition parties' sets into smaller sets to achieve efficiency.




%\subsection{Merkel Tree}

\vspace{-2mm}

\input{Merkle-tree-short}

\vspace{-2.2mm}

\subsection{Polynomial Representation of Sets}\label{sec::poly-rep}
\vspace{-.5mm}


%The idea of representing a set's elements using a polynomial was originally proposed by Freedman  \et in \cite{DBLP:conf/eurocrypt/FreedmanNP04}. Since its introduction, this idea has gained widespread adoption  e.g., in \cite{GhoshS19,DBLP:conf/crypto/KissnerS05}. 

In this representation, set elements $S=\{s_{\st 1},...,s_{\st d}\}$ are defined over a field $\mathbb{F}_{\st p}$ and  set $S$ is represented as a polynomial: $\mathbf{p}(x)=\prod\limits ^{\st {d}}_{\st i=1}(x-s_{\st i})$, where $\mathbf{p}(x) \in \mathbb{F}_{\st p}[X]$ and $\mathbb{F}_{\st p}[X]$ is a polynomial ring \cite{DBLP:conf/eurocrypt/FreedmanNP04}.  
%
%Often a   polynomial,  $\mathbf{p}(x)$, of degree $d$ is  represented in the ``coefficient form'' as follows:  $\mathbf{p}(x)=a_{\st 0}+a_{\st 1}\cdot x+...+ a_{\st d}\cdot x^{\st d}$.   
As shown in \cite{BonehGHWW13,DBLP:conf/crypto/KissnerS05}, for sets $S^{\st (A)}$ and $S^{\st (B)}$ represented by polynomials $\mathbf{p}_{\st A}$ and $\mathbf{p}_{\st B}$, their product, $\mathbf{p}_{\st A}\cdot \mathbf{p}_{\st  B}$,  represents the set union, while their greatest common divisor, $gcd($$\mathbf{p}_{\st A}$$,\mathbf{p}_{\st B})$, represents the intersection. 

For polynomials $\mathbf{p}_{\st A}$ and $\mathbf{p}_{\st B}$ of degree $d$, and random polynomials $\bm\gamma_{\st A}$ and  $\bm\gamma_{\st B}$ of degree $d$, it is proven in~\cite{BonehGHWW13,DBLP:conf/crypto/KissnerS05} that: $\bm\theta=\bm\gamma_{\st A}\cdot \mathbf{p}_{\st A}+\bm\gamma_{\st B}\cdot\mathbf{p}_{\st B}=\bm\mu\cdot gcd(\mathbf{p}_{\st A},\mathbf{p}_{\st B})$, where $\bm\mu$ is a uniformly random polynomial, and $\bm\theta$ contains only information about the elements in  $S^{\st (A)}\cap S^{\st (B)}$.  {In this paper, the parties employ this technique to compute polynomial $\bm\theta$ that encodes the intersection}.  
%
Given a polynomial $\bm\theta$ that encodes sets intersection, one can find the set elements in the intersection through one of the following two approaches: 

\vspace{-1mm}
\begin{enumerate}[leftmargin=5mm]
\item\label{Polynomial-evaluation}  \textit{polynomial evaluation}: the party in possession of one of the original input sets, for example $\mathbf{p}_{\st A}$,  evaluates $\bm\theta$ at every element $s_{\st i}$ of $\mathbf{p}_{\st A}$ and considers $s_{\st i}$ in the intersection if $\mathbf{p}_{\st A}(s_{\st i})=0$. 

\item\label{Root-extraction}  \textit{root extraction}:   the party who does not have one of the original input sets, extracts the roots of $\bm\theta$,  which contain the roots of (i) random polynomial  $\bm\mu$ and (ii) the polynomial that represents the intersection, i.e., $gcd(\mathbf{p}_{\st A},\mathbf{p}_{\st B})$. 
\end{enumerate}
\vspace{-1mm}
Within Approach \ref{Root-extraction}, to distinguish errors (i.e., roots of $\bm\mu$) from the intersection, PSIs in \cite{eopsi,DBLP:conf/crypto/KissnerS05} use the \emph{``hash-based padding technique''}. In this technique, every element $u_{\st i}$ in the set universe $\mathcal{U}$, becomes $s_{\st i}=u_{\st i}||\mathtt{H}(u_{\st i})$, where $\mathtt{H}$ is a cryptographic hash function with a sufficiently large output size. Given a field's arbitrary element, $s \in \mathbb{F}_p$ and $\mathtt{H}$'s output size $|\mathtt{H}(.)|$, we can parse $s$ into $x_{\st 1}$ and $x_{\st 2}$, such that $s=x_{\st 1}||x_{\st 2}$ and  $|x_{\st 2}|=|\mathtt{H}(.)|$. In a  PSI that uses polynomial representation and this padding technique, after we extract each root of  $\bm\theta$, say $s$, we parse it into $(x_{\st 1}, x_{\st 2})$ and check $x_{\st 2}\stackrel{?}=\mathtt{H}(x_{\st 1})$.  If the equation holds, then we consider $s$ as an element of the intersection. In \withFai and \withRew, the clients will use Approach \ref{Polynomial-evaluation}: polynomial evaluation, while in \withRew the auditor of the counter collusion contracts will use approach \ref{Root-extraction}: root extraction. 


\vspace{-3mm}

\subsection{Horner's Method}
\vspace{-.5mm}

Horner's method \cite{DBLP:journals/ibmrd/Dorn62} enables an efficient evaluation of polynomials at a specified point, e.g., $x_{\st 0}$. In particular, when dealing with a polynomial in the following form: $\bm\tau(x)= a_{\st 0}+a_{\st 1}\cdot x+a_{\st 2}\cdot x^{\st 2}+...+a_{\st d}\cdot x^{\st d}$ and a given point: $x_{\st 0}$, one can efficiently evaluate the polynomial at $x_{\st 0}$ iteratively using the following method: $\bm\tau(x_{\st 0})=a_{\st 0}+x_{\st 0}(a_{\st 1} + x_{\st 0}(a_{\st 2}+...+x_{\st 0}(a_{\st d-1}+x_{\st 0}\cdot a_{\st d})...)))$. Evaluating  a polynomial of degree $d$ naively requires  $d$ additions and $\frac{(d^{\st 2}+d)}{2}$ multiplications. However, using Horner's method the evaluation requires only $d$ additions and $2d$ multiplications. We use this method in this paper. 

\vspace{-2.5mm}

\subsection{Oblivious Linear Function Evaluation}\label{sec::OLE-plus}
\vspace{-.5mm}

Oblivious Linear function Evaluation (\ole) is a two-party protocol that involves a sender and receiver. In \ole,  the sender has two inputs  $a, b\in \mathbb{F}_{\st p}$ and the receiver has a single input, $c \in \mathbb{F}_{p}$.  The protocol allows the receiver to learn only $s = a\cdot c + b \in \mathbb{F}_{\st p}$, while the sender learns nothing. Ghosh \textit{et al.} \cite{GhoshNN17} proposed an efficient \ole that has $O(1)$ overhead and involves mainly symmetric key operations. Later, in \cite{GhoshN19} an enhanced \ole, called $\ole^{\st +}$ was proposed. The latter ensures that the receiver cannot learn anything about the sender's inputs,  even if it sets its input to $0$. In this paper, we use $\ole^{\st +}$. We refer readers to Appendix \ref{apndx:F-OLE-plus}, for its construction. 

\vspace{-1mm}
\input{short-coin-tossing}


%,  as an aborting party can be excluded from the next run of the protocol and the aborting party cannot learn partsets' intersection 









==> CCS-24/OLE-plus.tex <==
% !TEX root =main.tex


\section{Enhanced OLE's Protocol}\label{apndx:F-OLE-plus}



The PSIs proposed in \cite{GhoshN19} use an enhanced version of the  \ole.  The enhanced \ole ensures that the receiver cannot learn anything about the sender's inputs,  in the case where it sets its input to $0$, i.e., $c=0$. The enhanced \ole's protocol (denoted by $\ole^{\st +}$) is presented in Figure \ref{fig:OLE-plus-protocol}. In this paper, $\ole^{\st +}$ is used as a subroutine in \vopr, in Section \ref{sec::vopr}. 



%
%The PSIs in \cite{GhoshN19} also use an enhanced version of the  OLE. In short, the enhanced OLE  ensures that the receiver cannot learn anything (other than a random value) about the sender's inputs,  in the case where it  sets its input to $0$, i.e., $c=0$. The enhanced OLE's ideal functionality (denoted by $\mathcal{F}_{\st \text{OLE}^{+}}$) and protocol  (denoted by $\text{OLE}^{\st +}$)  are presented in  Figures \ref{fig:OLE-plus-func} and \ref{fig:OLE-plus-protocol} respectively.






%\begin{figure}[!htb]
%\setlength{\fboxsep}{1pt}
%\begin{center}
%\begin{boxedminipage}{12.3cm}
%
%\begin{small}
%
%
%\begin{enumerate}
%
%%\small{
%\item Upon receiving a message $(\mathtt{inputS},(a, b))$ from the sender, where $a, b \in \mathbb{F} $, verify that there is no 
%tuple stored; otherwise, ignore that message. Store $a$ and $b$ and send a message $(\mathtt{input})$ to the adversary, $\mathcal{A}$.
%
%
%
%\item Upon receiving a message $(\mathtt{inputR}, c)$ from the receiver, where $c \in \mathbb{F} $, verify that there is no 
%value stored; otherwise, ignore the message. Store $c$ and send a message $(\mathtt{input})$ to $\mathcal{A}$.
%
%
%\item Upon receiving a message $(\mathtt{deliver})$ from $\mathcal{A}$, check if both $(a, b)$ and $c$ have been stored; otherwise, ignore that message.  If $x \neq 0$, set $s = a\cdot c + b$. Otherwise, pick a uniformly random value, $s\stackrel{\st\$}\leftarrow  \mathbb{F} $,  and send $(\mathtt{output}, s)$  to the receiver. Ignore all further messages.
%
%
%%}
%\end{enumerate}
%
%\end{small}
%\end{boxedminipage}
%\end{center}
%\caption{
%\small {Enhanced oblivious linear function evaluation ($\text{OLE}^{\st +}$) ideal functionality, $\mathcal{F}_{\st\text{OLE}^{+}}$  \cite{GhoshN19}}.} 
%\label{fig:OLE-plus-func}
%\end{figure}




\begin{figure}[ht]
\setlength{\fboxsep}{1pt}
\begin{center}
\begin{boxedminipage}{8.5cm}
\begin{small}
\begin{enumerate}[leftmargin=5.5mm]
%
\item  Receiver (input $c \in \mathbb{F}_{\st p} $): Pick a random value, $r\stackrel{\st\$}\leftarrow  \mathbb{F}_{\st p} $, and send  $(\mathtt{inputS}, (c^{\st -1}, r))$ to the first $\mathcal{F}_{\st\ole}$.
%
%Upon receiving a message $(\mathtt{inputS},(a, b))$ from the sender, where $a, b \in \mathbb{F} $, verify that there is no  tuple stored; otherwise, ignore that message. Store $a$ and $b$ and send a message $(\mathtt{input})$ to the adversary, $\mathcal{A}$.
%
\item Sender (input $a, b \in \mathbb{F}_{\st p} $): Pick a random value, $u \stackrel{\st\$}\leftarrow  \mathbb{F}_{\st p} $, and send $(\mathtt{inputR}, u)$ to the first $\mathcal{F}_{\st\ole}$, to learn $t =  c^{\st -1}\cdot u
 + r$. Send $(\mathtt{inputS},(t + a, b - u))$ to the second $\mathcal{F}_{\st\ole}$.
%
\item Receiver: Send $(\mathtt{inputR}, c)$ to the second $\mathcal{F}_{\st\ole}$ and obtain $k = (t+a)\cdot c+(b-u)=a\cdot c + b + r\cdot c$. Output $s=k - r\cdot c=a\cdot c + b$.

%}
\end{enumerate}
\end{small}
\end{boxedminipage}
\end{center}
 \vspace{-2mm}
\caption{
\small {Enhanced Oblivious Linear function Evaluation  ($\ole^{\st +}$)  \cite{GhoshN19}}.} 
\label{fig:OLE-plus-protocol}
 \vspace{-2mm}
\end{figure}


==> CCS-24/PSI-FC-predicates.tex <==
% !TEX root =main.tex


\section{Formal Definitions of Predicates of \p}\label{sec::Formal-Definitions-of-F-PSI-Predicates}

 In this section, we present the formal definitions of predicates $\qinit, \qdel, \qUnFAbt$ and \qFAbt. We borrowed  the first three predicates from the ``fair and robust multi-party computation'' initially proposed in \cite{KiayiasZZ16}. Nevertheless, we  (i) have introduced an additional predicate  \qFAbt and (ii) will offer more precise and formal definitions of all these predicates. 
 
 
 
 \begin{definition}
 %
  [\qinit: Initiation predicate] Let $\mathcal{G}$ be a stable ledger, $adr_{\st sc}$ be smart contract $sc$'s address, $Adr$ be a set of $m+1$ distinct addresses, and $\xc$ be a fixed amount of coins. Then, predicate $\qinit(\mathcal{G}, adr_{\st sc}, m+1, Adr, \xc)$ returns $1$ if every address in $Adr$ has at least $\xc$ coins in $sc$. Otherwise, it returns $0$. 
 %
 \end{definition}

 
 
    \begin{definition}  [\qdel:
    %
    Delivery predicate] Let $pram:=(\mathcal{G}, adr_{\st sc}, \xc)$ be the parameters defined above, and   $adr_{\st i}\in Adr$ be the address of an honest party. 
    %
%    Let also $G$ be a compensation function that takes as input  two parameters $(deps, m')$, where $deps$ is the amount of coins  that all $m+1$ parties  deposit; it returns the amount of compensation each honest party must receive, i.e., $G(deps, m')\rightarrow c'$. 
    %
    Then, predicate $\qdel(pram, adr_{\st i})$ returns $1$ if $adr_{\st i}$ has sent $\xc$ amount to $sc$ and received  $\xc$ amount from it; thus,  its balance in $sc$ is $0$. Otherwise, it returns $0$. 
 %
  \end{definition}
 
 
 
   \begin{definition}  [\qUnFAbt: UnFair-Abort predicate]
   %
 Let $pram:=(\mathcal{G}, $ $adr_{\st sc}, \xc)$ be the parameters defined above, and $Adr'\subset Adr$ be a set containing honest parties' addresses, $m' = |Adr'|$,  and   $adr_{\st i}\in Adr'$. Let also $G$ be a compensation function that takes as input  three parameters $(\depsc, adr_{\st i}, m')$, where $\depsc$ is the number of coins  that all $m+1$ parties  deposit. It returns the amount of compensation each honest party must receive, i.e., $G(\depsc, ard_{\st i}, m')\rightarrow \xci$. Then, predicate $\qUnFAbt$ is defined as $\qUnFAbt(pram, G, \depsc, m', adr_{\st i})\rightarrow (a,b)$, where $a=1$ if $adr_{\st i}$ is an honest party's address and $adr_{\st i}$ has sent $\xc$ amount to $sc$ and received  $\xc+\xci$  from it, and $b=1$ if $adr_{\st i}$ is \aud's address and $adr_{\st i}$ received $\xci$  from $sc$. Otherwise, $a=b=0$. 
  %
  \end{definition}
  
  
\begin{definition}  [\qFAbt: Fair-Abort predicate]
   %
 Let $pram:=(\mathcal{G},$ $ adr_{\st sc},$ $ \xc)$ be the parameters defined above, and $Adr'\subset Adr$ be a set containing honest parties' addresses, $m' = |Adr'|$,     $adr_{\st i}\in Adr'$, and  $adr_{\st j}$ be \aud's address. Let $G$ be the compensation function, defined above, and let $G(deps, ard_{\st j}, m')\rightarrow \xc_{\st j}$ be the compensation that the auditor must receive.  Then, predicate $\qFAbt(pram, G,$ $ \depsc, m', adr_{\st i}, adr_{\st j})$ returns $1$, if $adr_{\st i}$ (s.t. $adr_{\st i}\neq adr_{\st j}$) has sent $\xc$ amount to $sc$ and received  $\xc$  from it, and $adr_{\st j}$ received $\xc_{\st j}$  from $sc$. Otherwise, it returns $0$. 
  %
 \end{definition}
 
 

 
 

    
    We observed that predicate \qFAbt should have been defined in the generic framework in \cite{KiayiasZZ16} too. Because the framework should have also captured the cases where an adversary may abort without learning any output after the onset of the protocol.  
 
 

==> CCS-24/PSI-FCR-predicates.tex <==
% !TEX root =main.tex

 \vspace{-3mm}
\section{Formal Definitions of Predicates of \ep}\label{sec::Formal-Definitions-of-E-PSI-Predicates}

 
 Below, we present the formal definition of predicates \qdelwr and \qUnFAbtwr. 

    \begin{definition}  [\qdelwr:
    %
    Delivery-with-Reward predicate] Let $\mathcal{G}$ be a stable ledger, $adr_{\st sc}$ be smart contract $sc$'s address, $adr_{\st i}\in Adr$ be the address of an honest party, $\xc$ be a fixed amount of coins, and $pram:=(\mathcal{G}, adr_{\st sc}, \xc)$. Let $R$ be a reward function that takes as input the computation result: $res$, a party's address: $adr_{\st i}$, a reward a party should receive for each unit of revealed information:  $\lc$, and input size: $inSize$.  Then $R$ is defined as follows. If $adr_{\st i}$ belongs to a non-buyer, then it returns the total amount that $adr_{\st i}$ should be rewarded and if $adr_{\st i}$ belongs to a buyer client, then it returns the reward's leftover that the buyer can collect, i.e., $R(res, adr_{\st i}, \lc, inSize)\rightarrow \rewci$.    Then, the delivery with reward predicate $\qdelwr(pram,  adr_{\st i}, res, \lc, inSize)$ returns $1$ if $adr_{\st i}$ has sent $\xc$ amount to $sc$ and received at least $\xc+\rewci$ amount from it. Else, it returns $0$. 
    
    
    
    %
%    Let also $G$ be a compensation function that takes as input  two parameters $(deps, m')$, where $deps$ is the amount of coins  that all $m+1$ parties  deposit; it returns the amount of compensation each honest party must receive, i.e., $G(deps, m')\rightarrow c'$. 
    %

 %
  \end{definition}


 \vspace{-2mm}


   \begin{definition}  [\qUnFAbtwr: UnFair-Abort-with-Reward predicate]
   %
 Let\\ $pram:=(\mathcal{G}, adr_{\st sc}, \xc)$ be the parameters defined above, and $Adr'\subset Adr$ be a set containing honest parties' addresses, $m' = |Adr'|$,  and   $adr_{\st i}\in Adr'$. Let also $G$ be a compensation function that takes as input  three parameters $(\depsc, adr_{\st i}, m')$, where $\depsc$ is the amount of coins that all $m+1$ parties deposit, $adr_{\st i}$ is an honest party's address, and $m' = |Adr'|$; it returns the amount of compensation each honest party must receive, i.e., $G(\depsc, adr_{\st i}, m')\rightarrow \xci$. Let $R$ be the reward function defined above, i.e., $R(res, adr_{\st i}, \lc, inSize)\rightarrow \rewci$, and let $\hat {pram}:=(res, \lc, inSize)$.  Then, predicate \qUnFAbtwr is defined as $\qUnFAbtwr(pram, \hat {pram}, G, R, $ $\depsc, m', adr_{\st i})\rightarrow (a,b)$, where $a=1$ if $adr_{\st i}$ is an honest party's address which has sent $\xc$ amount to $sc$ and received  $\xc+\xci+\rewci$  from it, and $b=1$ if $adr_{\st i}$ is an auditor's address which received $\xci$  from $sc$. Otherwise, $a=b=0$. 
  %
  \end{definition}


==> CCS-24/Peisoner-contract.tex <==
% !TEX root =main.tex


\subsection{Prisoner's Contract (\SCpc)}

\SCpc has been designed for outsourcing a certain computation. It is signed by a client who delegates the computation and two other parties  (or servers)  who perform the computation.  

This contract aims to encourage accurate computation by implementing the following concept. It mandates that each server submit a deposit before the delegation of computation. If a server adheres to honest behavior, it retains the ability to withdraw its deposit. However, if a server engages in dishonest practices (and is subsequently detected), its deposit is transferred to the client. When one of the servers behaves honestly while the other cheats, the honest server receives a reward. This reward is deducted from the deposit of the cheating server.

Hence, the goal of \SCpc is to create a Prisoner’s dilemma between the two servers in the following sense. Although the servers may collude with each other (to cut costs and provide identical but incorrect computation results) which leads to a higher payoff than both behaving honestly,  there is an even higher payoff if one of the servers manages to persuade the other server to collude and provide an incorrect result while itself provides a correct result. In this setting, each server knows that collusion is not stable as its counterpart will always try to deviate from the collusion to increase its payoff.  If a server tries to convince its counterpart (without a credible and enforceable promise), then the latter party will consider it as a trap; consequently, collusion will not occur. Below, we restate the contract. %We have slightly adjusted the contract such that misbehaving servers deposit is transferred to another contract (denoted with $\mathcal{SC}_{\st\epsi}$) instead of transferring directly to the client. 

\begin{enumerate}[leftmargin=5mm]
%
\item The contract is signed by three parties; namely, client $ {D}$ and two other parties $E_{\st 1}$ and $E_{\st 2}$. A third-party auditor will resolve any dispute between $ { D}$ and the servers.  \textcolor{blue}{The address of another contract, called $\mathcal{SC}_{\st\epsi}$, is hardcoded in this contract.} 
%
\item The servers agree to run computation $f$ on input $x$, both of which have been provided by $ { D}$. 
%
\item The parties agree on three deadlines $(T_{\st 1}, T_{\st 2}, T_{\st 3})$, where $T_{\st i+1} > T_{\st i}$.
%
\item $ { D}$ agrees to pay $\wc$ amount to each server for the correct and on-time computation. Therefore, $ { D}$ deposits $2\cdot \wc$ amount in the contract. \textcolor{blue}{This deposit is transferred from $\mathcal{SC}_{\st\epsi}$ to this contract}.
%
\item Each server deposits \textcolor{blue}{$\dc'=$ }$\dc$\textcolor{blue}{$\ +\ \Xc$} amount in the contract. 
%
\item The servers must pay the deposit before $T_{\st 1}$. If a server fails to meet the deadline, then the contract would refund the parties' deposit (if any) and terminate.  
%
\item The servers must deliver the computation's result before $T_{\st 2}$. 
%
\item  The following steps are taken when (i) both servers provided the computation's result or (ii) deadline $T_{\st 2}$ elapsed. 
%
\begin{enumerate}
%
\item if both servers failed to deliver the computation's result, then the contract transfers their deposits to \textcolor{blue}{$\mathcal{SC}_{\st\epsi}$}.
%
\item if both servers delivered the result, and the results are equal, then (after verifying the results) \textcolor{blue}{this contract} must pay the agreed
amount $\wc$ and refund the deposit of $\dc'$ amount to each server. 
%
\item\label{prisoner-cont-raise-disp} otherwise, $ { D}$ raises a dispute with the auditor.  
%
\end{enumerate}
%
\item When a dispute is raised, the auditor (which is independent of \aud in \fpsi) re-generates the computation's result, \textcolor{blue}{by using algorithm $\mathtt{resComp}(.)$ described shortly in Appendix \ref{sec::auditor-res-Comp}.} Let $y_{\st t}, y_{\st 1},$ and $y_{\st 2}$ be the result computed by the auditor, $E_{\st 1}$, and $E_{\st 2}$ respectively. The auditor uses the following role to identify the cheating party.  
%
\begin{itemize}
%
\item[$\bullet$] if $E_{\st i}$ failed to deliver the result (i.e., $y_{\st i}$ is null), then it has cheated. 
%
\item[$\bullet$] if a result $y_{\st i}$ has been delivered before the deadline and $y_{\st i}\neq y_{\st t}$, then $E_{\st i}$ has cheated. 
%
\end{itemize}
%
\textcolor{blue}{The auditor sends its verdict to \SCpc.} 
%
\item Given the auditor's decision, the dispute is settled according to the following rules.
%
\begin{itemize}
%
\item[$\bullet$] if none of the servers cheated, then \textcolor{blue}{this contract} transfers to each server (i) $\wc$ amount for performing the computation and (ii) its deposit, i.e., $\dc'$ amount. The client also pays the auditor $\chc$ amount.  
%
\item[$\bullet$] if both servers cheated, then \textcolor{blue}{this contract (i) pays the auditor the total amount of $\chc$, taken from the servers' deposit, and (ii) transfers to  $\mathcal{SC}_{\st\epsi}$ the rest of the deposit, i.e., $2\cdot \dc'-\chc$ amount.} 
%
\item[$\bullet$] if one of the servers cheated, then \textcolor{blue}{this contract (i) pays the auditor the total amount of $\chc$, taken from the misbehaving server's deposit, (ii) transfers the honest server's deposit (i.e., $\dc'$ amount) back to this server,  (iii) transfers to the honest server $\wc+\dc-\chc$ amount (which covers its computation cost and the reward), and  (iv) transfers to $\mathcal{SC}_{\st\epsi}$ the rest of the misbehaving server's deposit, i.e., $\Xc$ amount.} The cheating server receives nothing.  
%
\end{itemize} 
%
\item After deadline $T_{\st 3}$, if $ { D}$ has neither paid nor raised a dispute, then \textcolor{blue}{this contract} pays $\wc$ to each server which delivered a result before deadline $T_{\st 2}$ and refunds each server its deposit, i.e., $\dc'$ amount. Any deposit left after that will be transferred to \textcolor{blue}{$\mathcal{SC}_{\st\epsi}$}. 
%
\end{enumerate}


Now, let us elaborate on why we have implemented the aforementioned modifications to the original \SCpc introduced by Dong \et \cite{dong2017betrayal}. In the original \SCpc (a) the client does not deposit any amount in this contract; instead, it directly sends its coins to a server (and auditor) according to the auditor's decision,  (b) the computation correctness is determined only within this contract (with the involvement of the auditor if required), and (c)  the auditor simply re-generates the computation's result given the computation's plaintext inputs.  

Nevertheless, in \epsi, (1) \emph{all clients} need to deposit a certain amount in $\mathcal{SC}_{\st\epsi}$ and only the contracts must transfer the parties' deposit,  (2) $\mathcal{SC}_{\st\epsi}$ also needs to verify a part of the computation's correctness without the involvement of the auditor and accordingly distribute the parties deposit based on the verification's outcome,  and (3) the auditor must be able to re-generate the computation's result without being able to learn the computation's plaintext input, i.e., elements of the set. 

Therefore, we have included the address of $\mathcal{SC}_{\st\epsi}$ in \SCpc to enable the parties' deposit to be moved between the two contracts (if necessary). Moreover, we have allowed \SCpc to distribute the parties' deposit; thus, the requirements in points (1) and (2) are met. To satisfy the requirement in point (3) above, we have included a new algorithm, called $\mathtt{resComp}(.)$, in \SCpc.  Shortly, we will provide more details about this algorithm. Moreover, to make this contract compatible with \epsi, we increased the amount of each server's deposit by  $\Xc$. Nevertheless, this adjustment does not change the logic behind \SCpc's design and its analysis.  







\subsubsection{Auditor's Result-Computation Algorithm.}\label{sec::auditor-res-Comp}


In this work,  we use \SCpc to delegate the computation of intersection cardinality to two extractor clients, a.k.a. servers in the original \SCpc. In this setting, the contract's auditor is invoked when an inconsistency is detected in step \ref{smart-PSI-inconsistency} of \epsi. For the auditor to recompute the intersection cardinality, we have designed $\mathtt{resComp}(.)$ algorithm. The auditor uses this algorithm for every bin's index $indx$,  where $1\leq indx\leq h$ and $h$ is the hash table's length. We present this algorithm in Figure \ref{fig::resComp}.  The auditor collects the inputs of this algorithm as follows: (a)  reads random polynomial $\bm\zeta$, and blinded polynomial $\bm\phi$ from contract $\mathcal{SC}_{\fpsi}$, (b) reads the ciphertext of secret key $mk$ from $\mathcal{SC}_{\st\epsi}$, and (c) retrieves public parameters $(des_{\mathtt{H}}, h)$ from the hash table's public description. 



Note that in the original  \SCpc, the auditor is assumed to be fully trusted. However, in this work, we have relaxed this assumption. We have designed \epsi and $\mathtt{resComp}(.)$ in such a way that even a semi-honest auditor cannot learn anything about the actual elements of the sets, as they have been encrypted under a key unknown to the auditor. 



\input{auditor-res-Comp}





















==> CCS-24/Priliminary.tex <==
% !TEX root =U-PSI.tex

\section{Priliminaries}

\subsection{Notations}
In the following, we  provide a basic and enhanced multiple clients PSI protocols. In the basic protocol, there are three types of parties involved in the protocols: $m>1$ authoriser clients: $\resizeT {\textit A}_{\resizeS {\textit  j}}$ who are not interested in the result, the result recipient client: $B$, and a non-colluding dealer: $D$. All parties are potentially semi-honest. In the first variant of the protocol the dealer does not have any set elements. Then we provide an enhanced protocol   that supports a distributed dealers such that the protocol remains secure even if  all but one dealers collude with client $B$ or  a subset of authoriser clients collude with each other and client $B$. Moreover, in the enhanced protocol, the dealers are actually clients who have  set elements as the computation's inputs.  Note that, in the following protocols, all  values and operations are defined over a finite field of prime order. Let each client $I\in \{\resizeT {\textit A}_{\resizeS {\textit  1}},...,\resizeT {\textit A}_{\resizeS {\textit  m}},B\}$, have a set $S^{\resizeS {\textit I} }=\{s^{\resizeS {\textit I} }_{\scriptscriptstyle 1},..., s^{\resizeS {\textit I} }_{\scriptscriptstyle d}\}$ and   $\vv{\bm{x}}=[x_{\scriptscriptstyle 1},..., x_{\scriptscriptstyle n}]$ be a  public vector of non-zero unique elements, where $n=2d+1$, and $d$ be the set cardinality's upper bound. Let $e$ be a flat price of learning one element of the set.   

\subsection{Shamir Secret Sharing}

\subsection{Oblivious Polynomial Evaluation and Oblivious Linear Function Evaluation} Oblivious polynomial evaluation: OPE, introduced by \cite{Naor:1999:OTP}, is a two-party protocol where a sender  inputs a polynomial, defined over a finite field, and a receiver inputs a single
point of the same finite field. At the end of the protocol, the sender receives nothing while the receiver  receives the polynomial evaluated on the point chosen by the receiver. Informally, the protocol is secure if the sender learns nothing on which point was chosen by the receiver and the receiver evaluates the polynomial on at most one point. OPE protocols can be broadly categorised in two groups: (a) computationally (or conditionally) secure, and (b) information theoretically (or unconditionally) secure. In this paper, we use OPE to evaluate a polynomial of \emph{degree one} and our focus is on the latter category as it best fits our purpose, e.g. due to its computational efficiency, (similar to our protocols) using a finite field over which are arithmetic operations are defined, etc. Information  theoretically OPE protocols can be further divided into three  classes: those that  (a) use an initializer that has an \emph{active role}, e.g. \cite{DBLP:conf/asiacrypt/ChangL01} (b) use an initializer that has a \emph{one-off role} and distributes  random parameters among receiver and sender in the setup phase and does not play any further role, e.g. \cite{DBLP:conf/acisp/HanaokaIMNOW04} and (c) are based on a distributed setting in which a set of servers implement the function of the sender, e.g. in \cite{DBLP:conf/icisc/CianciulloG18}. Our PSI protocol, can use either of these highly efficient OPE protocols, i.e.  \cite{DBLP:conf/acisp/HanaokaIMNOW04} or \cite{DBLP:conf/icisc/CianciulloG18}.  The scheme in \cite{DBLP:conf/acisp/HanaokaIMNOW04} is secure under the assumption that the initializer does not collude with the sender and receiver. Moreover, the scheme in \cite{DBLP:conf/icisc/CianciulloG18} remains secure as long as the sender does not collude with the servers, however if a threshold of the servers  collude with each other they cannot learn anything about the sender's or receiver's input and if a threshold of the servers collude with the receiver they cannot learn the sender's input. We note that the  use of the  OPE proposed in \cite{DBLP:conf/icisc/CianciulloG18}  in our protocol does not introduce any  additional servers, as  their roles are played by a subset of  clients in our protocol, i.e. assistant authorizer clients. For the sake of completeness, we provide both protocols \cite{DBLP:conf/acisp/HanaokaIMNOW04} in this section. 

%\begin{enumerate}
%\item There are three parties involved in this protocol: Sender: $S$, receiver $R$ and initializer $T$, where $S$'s input is $\beta(x)$ and $R$'s input is $b$.
%\item Setup: $T$ picks a random polynomial $\tau(x)$ of degree $d$ and a random value $v$. It sends $\tau(x)$ to $S$. Also, it sends  $v$ and $g=\tau(v)$ to $R$. 
%\item Computation: $R$ sends the value $l=b-v$ to $S$. $S$ then computes and sends to $R$ the polynomial $\delta (x)= \beta(l+x)+\tau(x)$. Then, $R$ computes $\delta(d)-g=\beta(b)=$
%\end{enumerate}





\begin{figure}[ht]
\setlength{\fboxsep}{2pt}
\begin{center}
\begin{boxedminipage}{11cm}
\small{

\

\noindent\textbf {Parties:} Sender: $\mathcal{S}$, receiver: $\mathcal{R}$ and initialiser: $\mathcal{T}$.

\noindent\textbf {Input:} $\mathcal{S}$ has a polynomial: $\beta(x)$  of degree at most $\mathsf{d}$. Also, $\mathcal{R}$ has a value:  $\mathsf{a}$.

\noindent\textbf {Output:} $\mathcal{R}$ obtains $\mathsf{b}=\beta(\mathsf{a})$ and $\mathcal{S}$ gets nothing.

\noindent\textbf {Setup:} 
\begin{enumerate}
\item Initializer $\mathcal{T}$ picks a random polynomial $\tau(x)$ of degree $\mathsf{d}$ and sends it to $\mathcal{S}$. 
\item Also, $\mathcal{T}$ picks a random value $\mathsf{v}$ and sends $\mathsf{v}$ and $\tau(\mathsf{v})$ to $\mathcal{R}$.
\end{enumerate}

\noindent\textbf {Computation:} 
\begin{enumerate}
\item $\mathcal{R}$ sends the value $\mathsf{f}=\mathsf{a}-\mathsf{v}$ to $\mathcal{S}$. 
\item Next, $\mathcal{S}$  computes polynomial $\delta(x)=\beta(\mathsf{f}+x)+\tau(x)$ and sends $\delta(x)$ to $\mathcal{R}$.
\item $\mathcal{R}$ computes $\delta(\mathsf{v})-\tau(\mathsf{v})=\mathsf{b}$
 \end{enumerate}
 \
}


\end{boxedminipage}
\end{center}
\caption{Efficient Information Theoretic OPE \cite{DBLP:conf/acisp/HanaokaIMNOW04}.} 
\label{fig:subroutines}
\end{figure}







\begin{figure}[ht]
\setlength{\fboxsep}{2pt}
\begin{center}
\begin{boxedminipage}{11cm}
\small{

\

\noindent\textbf {Parties:} Sender: $\mathcal{S}$, receiver: $\mathcal{R}$ and $\mathsf{k}$ servers: $\{\mathcal{S}_{\scriptscriptstyle {1}},...,\mathcal{S}_{\scriptscriptstyle \mathsf{k}}\}$.

\noindent\textbf {Input:} $\mathcal{S}$ has a polynomial: $\beta(x)=\mathsf{c}_{\scriptscriptstyle 0}+\mathsf{c}_{\scriptscriptstyle 1}x+...+\mathsf{c}_{\scriptscriptstyle \mathsf{d}}x^{\scriptscriptstyle \mathsf{d}}$  of degree at most $\mathsf{d}$. Also, $\mathcal{R}$ has a value:  $\mathsf{a}$.

\noindent\textbf {Output:} $\mathcal{R}$ obtains $\mathsf{b}=\beta(\mathsf{a})$ and $\mathcal{S}$ gets nothing.

\noindent\textbf {Setup:} 
\begin{enumerate}
\item $\mathcal{S}$ picks $\mathsf{d}$ random values: $\{\mathsf{r}_{\scriptscriptstyle 1},...,\mathsf{r}_{\scriptscriptstyle \mathsf{d}}\}$. Then, it computes the following values. $\forall i,1\leq i \leq \mathsf{d}: \mathsf{z}_{\scriptscriptstyle i}=\mathsf{r}_{\scriptscriptstyle i}\cdot \mathsf{c}_{\scriptscriptstyle i}$


\item $\mathcal{S}$  uses ($\mathsf{k},\mathsf{k}$) Shamir secret sharing scheme to split each coefficient $\mathsf{c}_{\scriptscriptstyle j}$,  into $\mathsf{k}$ shares.  In particular, for each $\mathsf{c}_{\scriptscriptstyle j} \in \{\mathsf{c}_{\scriptscriptstyle 0},...,\mathsf{c}_{\scriptscriptstyle \mathsf{d}}\}$, it:

\begin{enumerate}
\item picks a random polynomial $\tau_{\scriptscriptstyle j}(x)$ of degree at most $\mathsf{k}-1$, such that $\tau_{\scriptscriptstyle j}(0)=\mathsf{c}_{\scriptscriptstyle j}$. 
\item evaluates $\tau_{\scriptscriptstyle j}(x)$ at every elements of  vector $\{1,...,\mathsf{k}\}$.  At the end of this process, each $\mathsf{c}_{\scriptscriptstyle j}$ is split into $\{ \tau_{\scriptscriptstyle j}(1),..., \tau_{\scriptscriptstyle j}(\mathsf{k})\}$ shares. 



%$\forall w,\mathbf{1}\leq w \leq \mathbf{k}: \tau_{\scriptscriptstyle j}(w)= {\tau}_{\scriptscriptstyle j,w}$

\end{enumerate}

\item $\mathcal{S}$  splits each value $\mathsf{z}_{\scriptscriptstyle j}$ into $\mathsf{k}$ shares using ($\mathsf{k},\mathsf{k}$) Shamir secret sharing. At the end of this process, each $\mathsf{z}_{\scriptscriptstyle j}$ is split into $\{ \lambda_{\scriptscriptstyle j}(1),..., \lambda_{\scriptscriptstyle j}(\mathsf{k})\}$ shares, where $\lambda_{\scriptscriptstyle j}(x)$ is a random polynomial of degree at most $\mathsf{k}-1$, such that $\lambda_{\scriptscriptstyle j}(0)=\mathsf{z}_{\scriptscriptstyle j}$.

\item $\mathcal{S}$ privately sends to  $\mathcal{R}$ values: $\{\mathsf{r}_{\scriptscriptstyle 1},..., \mathsf{r}_{\scriptscriptstyle \mathsf{d}}\}$. Moreover, $\mathcal{S}$ sends  to each server: $\mathcal{S}_{\scriptscriptstyle  \mathsf{p}}$, two sets of shares (computed above): $\{\tau_{\scriptscriptstyle 0}( \mathsf{p}),..., \tau_{\scriptscriptstyle \mathsf{d}}( \mathsf{p})\}$ and $\{\lambda_{\scriptscriptstyle 1}( \mathsf{p}),..., \lambda_{\scriptscriptstyle \mathsf{d}}( \mathsf{p})\}$, where $1\leq \mathsf{p}\leq \mathsf{k}$. 



\end{enumerate}

\noindent\textbf {Computation:} 
\begin{enumerate}
\item  $\mathcal{R}$ broadcasts to all servers the following set: $\{\mathsf{e}_{\scriptscriptstyle 1 },...,\mathsf{e}_{\scriptscriptstyle \mathsf{d}}\}$ where $\mathsf{e}_{\scriptscriptstyle i}=\mathsf{a}^{\scriptscriptstyle i}-\mathsf{r}_{\scriptscriptstyle i}$


\item Each server: $\mathcal{S}_{\scriptscriptstyle  \mathsf{p}}$, computes the following value: $  \mathsf{u}_{\scriptscriptstyle \mathsf{p}}=\tau_{\scriptscriptstyle 0}( \mathsf{p})+ \sum\limits^{\scriptscriptstyle \mathsf{d}}_{\scriptscriptstyle i=1}(\tau_{\scriptscriptstyle i}( \mathsf{p})\cdot \mathsf{e}_{\scriptscriptstyle i}+\lambda_{\scriptscriptstyle i}( \mathsf{p}))$

\item $\mathcal{R}$, given pairs ($\mathsf{u}_{\scriptscriptstyle \mathsf{p}}, \mathsf{p}$), interpolates a polynomial $\phi(x)$, e.g.  using Lagrange interpolation, and considers the constant coefficient as the result, i.e. $\phi(0)=\mathsf{b}$.


 \end{enumerate}
 \
}


\end{boxedminipage}
\end{center}
\caption{Efficient Information Theoretic distributed OPE \cite{DBLP:conf/icisc/CianciulloG18}.} 
\label{fig:subroutines}
\end{figure}




\subsection{Pseudorandom Permutation} 


A pseudorandom permutation, $\mathtt{PRP}(,)$,






==> CCS-24/Security-model-long.tex <==
% !TEX root =main.tex


\section{Full Description of the Security Model}\label{sec::sec-model-long}

In this paper, we employ the simulation-based paradigm of secure computation \cite{DBLP:books/cu/Goldreich2004} to establish and demonstrate the security of the proposed protocols. As our protocols encompass both static active and passive adversaries, we will provide formal definitions for each type.%
 

 
 \subsubsection{Two-party Computation.} A two-party protocol, denoted as $\Gamma$, is characterized by describing a random process that maps pairs of inputs to pairs of outputs, with one output for each party involved. This process is commonly referred to as functionality, denoted as  $f:\{0,1\}^{\st *}\times\{0,1\}^{\st *}\rightarrow\{0,1\}^{\st *}\times\{0,1\}^{\st *}$, where $f:=(f_{\st 1},f_{\st 2})$. 
 
 For every input pair $(x,y)$, the output pair is a random variable $(f_{\st 1} (x,y), $ $f_{\st 2} (x,y))$, such that the party with input $x$ wishes to obtain $f_{\st 1} (x,y)$ while the party with input $y$ wishes to receive $f_{\st 2} (x,y)$. When $f$ is deterministic, then $f_{\st 1} =f_{\st 2}$. In the setting where $f$ is asymmetric and only one party (say the first one) receives the result, $f$ is defined as $f:=(f_{\st 1}(x,y), \bot)$. 
 

 
 \subsubsection{Security in the Presence of Passive Adversaries.}  In the passive adversarial model, the party corrupted by such an adversary correctly follows the protocol specification. Nonetheless, the adversary obtains the internal state of the corrupted party, including the transcript of all the messages received, and tries to use this to learn information that should remain private. 
 %
 In loose terms, a protocol is considered secure when anything that a party can compute within the protocol can also be computed using only its input and output. In the simulation-based model, the essential condition is that a party's view during a protocol's execution can be recreated or simulated solely based on its input and output. This condition ensures that the parties gain no additional knowledge from the protocol's execution.
 
In a more formal sense, party $i$’s view (during the execution of $\Gamma$) on input pair  $(x, y)$ is denoted by $\mathsf{View}_{\st i}^{\st \Gamma}(x,y)$ and equals $(w, r^{\st i}, m_{\st 1}^{\st i}, ..., m_{\st t}^{\st i})$, where $w\in\{x,y\}$ is the input of $i^{\st th}$ party, $r_{\st i}$ is the outcome of this party's internal random coin tosses, and $m_{\st j}^{\st i}$ represents the $j^{\st th}$ message this party receives.  The output of the $i^{\st th}$ party during the execution of $\Gamma$ on $(x, y)$ is denoted by $\mathsf{Output}_{\st 1}^{\st \Gamma}(x,y)$ and can be generated from its view of the execution.  The joint output of both parties is denoted by $\mathsf{Output}^{\st \Gamma}(x,y):=(\mathsf{Output}_{\st 1}^{\st \Gamma}(x,y), \mathsf{Output}_{\st 2}^{\st \Gamma}(x,y))$.

\begin{definition}
Let $f$ be the deterministic functionality defined above. Protocol $\Gamma$ security computes $f$ in the presence of a  passive adversary if there exist polynomial-time algorithms $(\mathsf {Sim}_{\st 1}, \mathsf {Sim}_{\st 2})$ such that:
\end{definition}
%
  \begin{equation*}
  \{\mathsf {Sim}_{\st 1}(x,f_{\st 1}(x,y))\}_{\st x,y}\stackrel{c}{\equiv} \{\mathsf{View}_{\st 1}^{\st \Gamma}(x,y) \}_{\st x,y}\\
  \end{equation*}
  %
  \begin{equation*}
    \{\mathsf{Sim}_{\st 2}(x,f_{\st 2}(x,y))\}_{\st x,y}\stackrel{c}{\equiv} \{\mathsf{View}_{\st 2}^{\st \Gamma}(x,y) \}_{\st x,y}
  \end{equation*}
  %
  

%\vs

 \subsubsection{Security in the Presence of Active Adversaries.}  
 
 
the corrupted party has the freedom to deviate from the protocol specification in arbitrary ways, either to gain knowledge about the private inputs of the other parties or to manipulate the computation's result. In such cases, the adversary may choose not to utilize the provided input. Therefore, in addition to the concern that a corrupted party might gain unauthorized information, correctness is also a crucial requirement. This entails that a corrupted party must not have the ability to cause incorrect distribution of the output. Furthermore, we demand input independence, which means that a corrupted party cannot make its input contingent on the input of the other party.


To comprehend the potential threats, the security of a protocol is assessed by contrasting the actions an adversary can take in the actual protocol with those in an ideal scenario that is inherently secure. This comparison is formalized by examining an ideal computation that involves an incorruptible TTP to whom the parties submit their inputs and receive the output corresponding to the ideal functionality. Below, we provide descriptions of the executions in both the ideal and real models.
 
Initially, we describe the execution in the ideal model. Let $P_{\st 1}$ and $P_{\st 2}$ be the parties participating in the
protocol, $i\in \{0, 1\}$ be the index of the corrupted party, and $\mathcal A$ be a non-uniform
probabilistic polynomial-time adversary. Moreover, let $z$ be an auxiliary input given to $\mathcal A$ while  $x$ and $y$ be the input of party $P_{\st 1}$ and $P_{\st 2}$  respectively.  The honest party, $P_{\st j}$, sends its received input to TTP.  The corrupted party $P_{\st i}$ may either abort (by replacing the input with a special abort message $\Lambda_{\st i}$),  send its received input, or send some other input of the same length to TTP. This decision is made by the adversary and may depend on the input value of $P_{\st i}$ and $z$. If TTP receives $\Lambda_{\st i}$, then it sends $\Lambda_{\st i}$ to the honest party, and the ideal execution terminates.  Upon obtaining an input pair $(x, y)$, TTP computes $f_{\st 1}(x, y)$ and $f_{\st 2}(x, y)$. It first sends $f_{\st i}(x, y)$ to  $P_{\st i}$ which replies with ``continue'' or $\Lambda_{\st i}$. In the former case, TTP sends  $f_{\st j}(x, y)$ to  $P_{\st j}$ and in the latter it sends $\Lambda_{\st i}$ to  $P_{\st j}$. The honest party always outputs the message that it obtained from TTP. 

A malicious party may output an arbitrary function of its initial inputs and the message it has obtained from TTP.  The ideal execution of $f$ on inputs $(x, y)$ and $z$ is denoted by $\mathsf{Ideal}^{\st f}_{\st\mathcal{A}(z), i}(x,y)$ and is defined as the output pair of the honest party and $\mathcal{A}$ from the above ideal execution.  In the real model, the real two-party protocol $\Gamma$ is executed
without the involvement of TTP. In this setting, $\mathcal{A}$ sends all messages on
behalf of the corrupted party and may follow an arbitrary strategy.
The honest party follows the instructions of $\Gamma$. The real execution of $\Gamma$ is denoted by $\mathsf{Real}^{\st \Gamma}_{\st\mathcal{A}(z), i}(x,y)$, it is defined as the joint output of the parties engaging in the real execution of $\Gamma$ (on the inputs), in the presence of $\mathcal{A}$.
 
 
Next, we proceed to define security. At a high level, the definition asserts that a secure protocol in the real model replicates the behavior of the ideal model. This is expressed by stating that adversaries in the ideal model can simulate the executions of the protocol in the real model. 
 
\begin{definition}\label{def::MPC-active-adv}
Let $f$ be the two-party functionality defined above and $\Gamma$ be a two-party protocol that computes $f$.   Protocol $\Gamma$ securely computes $f$ with abort in the presence of static active adversaries if for every non-uniform probabilistic polynomial time adversary $\mathcal{A}$ for the real model, there exists a non-uniform probabilistic polynomial-time adversary (or simulator) $\mathsf{Sim}$ for the ideal model, such that for every $i\in \{0,1\}$, it holds that: 
%
\begin{equation*}
\{\mathsf {Ideal}^{\st f}_{\st \mathsf{Sim}(z), i}(x,y)\}_{\st x,y,z}\stackrel{c}{\equiv} \{\mathsf{Real}_{\st \mathcal{A}(z), i}^{\st \Gamma}(x,y) \}_{\st x,y,z}
\end{equation*}
%
\end{definition}
 
 
  
  

==> CCS-24/Security-model.tex <==
% !TEX root =main.tex


\section{Security Model}\label{sec::sec-model}

In this paper, we use the simulation-based paradigm of secure computation \cite{DBLP:books/cu/Goldreich2004} to define and prove the proposed protocols. Since both types of (static) active and passive adversaries are involved in our protocols, we will provide formal definitions for both types. In this work, we consider a static adversary, we assume there is an authenticated private (off-chain) channel between the clients and we consider a standard public blockchain, e.g., Ethereum.
%
 
 \subsubsection{Two-party Computation.} A two-party protocol $\Gamma$ problem is captured by specifying a random process that maps pairs of inputs to pairs of outputs, one for each party. Such process is referred to as a functionality denoted by  $f:\{0,1\}^{\st *}\times\{0,1\}^{\st *}\rightarrow\{0,1\}^{\st *}\times\{0,1\}^{\st *}$, where $f:=(f_{\st 1},f_{\st 2})$. For every input pair $(x,y)$, the output pair is a random variable $(f_{\st 1} (x,y), f_{\st 2} (x,y))$, such that the party with input $x$ wishes to obtain $f_{\st 1} (x,y)$ while the party with input $y$ wishes to receive $f_{\st 2} (x,y)$. When $f$ is deterministic, then $f_{\st 1} =f_{\st 2}$. In the setting where $f$ is asymmetric and only one party (say the first one) receives the result, $f$ is defined as $f:=(f_{\st 1}(x,y), \bot)$. 
 
 
 \subsubsection{Security in the Presence of Passive Adversaries.}  In the passive adversarial model, the party corrupted by such an adversary correctly follows the protocol specification. Nonetheless, the adversary obtains the internal state of the corrupted party, including the transcript of all the messages received, and tries to use this to learn information that should remain private. Loosely speaking, a protocol is secure if whatever can be computed by a party in the protocol can be computed using its input and output only. In the simulation-based model, it is required that a party’s view in a protocol's 
 execution can be simulated given only its input and output. This implies that the parties learn nothing from the protocol's execution. More formally, party $i$’s view (during the execution of $\Gamma$) on input pair  $(x, y)$ is denoted by $\mathsf{View}_{\st i}^{\st \Gamma}(x,y)$ and equals $(w, r^{\st i}, m_{\st 1}^{\st i}, ..., m_{\st t}^{\st i})$, where $w\in\{x,y\}$ is the input of $i^{\st th}$ party, $r_{\st i}$ is the outcome of this party's internal random coin tosses, and $m_{\st j}^{\st i}$ represents the $j^{\st th}$ message this party receives.  The output of the $i^{\st th}$ party during the execution of $\Gamma$ on $(x, y)$ is denoted by $\mathsf{Output}_{\st i}^{\st \Gamma}(x,y)$ and can be generated from its own view of the execution.  The joint output of both parties is denoted by $\mathsf{Output}^{\st \Gamma}(x,y):=(\mathsf{Output}_{\st 1}^{\st \Gamma}(x,y), \mathsf{Output}_{\st 2}^{\st \Gamma}(x,y))$.

\begin{definition}
Let $f$ be the deterministic functionality defined above. Protocol $\Gamma$ security computes $f$ in the presence of a static  passive adversary if there exist polynomial-time algorithms $(\mathsf {Sim}_{\st 1}, \mathsf {Sim}_{\st 2})$ such that:
\end{definition}

  \begin{equation*}
  \{\mathsf {Sim}_{\st 1}(x,f_{\st 1}(x,y))\}_{\st x,y}\stackrel{c}{\equiv} \{\mathsf{View}_{\st 1}^{\st \Gamma}(x,y) \}_{\st x,y}\\
  \end{equation*}
  %
  \begin{equation*}
    \{\mathsf{Sim}_{\st 2}(y, f_{\st 2}(x,y))\}_{\st x,y}\stackrel{c}{\equiv} \{\mathsf{View}_{\st 2}^{\st \Gamma}(x,y) \}_{\st x,y}
  \end{equation*}
  
  
  
 \subsubsection{Security in the Presence of Active Adversaries.}  In this adversarial model, the corrupted party may
arbitrarily deviate from the protocol specification, to learn the private inputs of the other parties or to influence the outcome of the computation. In this case,  the adversary may not use the input provided. Therefore, beyond the possibility that a corrupted party may learn more than it should, correctness is also required. This means that a corrupted party must not be able to cause the output to be incorrectly distributed. Moreover, we require independence of inputs meaning that a corrupted party cannot make its input depend on the other party’s input. To capture the threats,
the security of a protocol is analyzed by comparing what an adversary can do in the real protocol to what it can do in an ideal scenario that is secure by definition. This is formalized by considering an ideal computation involving an incorruptible Trusted Third Party (TTP) to whom the parties send their inputs and receive the output of the ideal functionality. Below, we describe the executions in the ideal and real models. 
 
First, we describe the execution in the ideal model. Let $P_{\st 1}$ and $P_{\st 2}$ be the parties participating in the
protocol, $i\in \{0, 1\}$ be the index of the corrupted party, and $\mathcal A$ be a non-uniform
PPT adversary. Also, let $z$ be an auxiliary input given to $\mathcal A$ while  $x$ and $y$ be the input of party $P_{\st 1}$ and $P_{\st 2}$  respectively.  The honest party, $P_{\st j}$, sends its received input to TTP.  The corrupted party $P_{\st i}$ may either abort (by replacing the input with a special abort message $\Lambda_{\st i}$),  send its received input or send some other input of the same length to TTP. This decision is made by the adversary and may depend on the input value of $P_{\st i}$ and $z$. If TTP receives $\Lambda_{\st i}$, then it sends $\Lambda_{\st i}$ to the honest party and the ideal execution terminates.  Upon obtaining an input pair $(x, y)$, TTP computes $f_{\st 1}(x, y)$ and $f_{\st 2}(x, y)$. It first sends $f_{\st i}(x, y)$ to  $P_{\st i}$ which replies with ``continue'' or $\Lambda_{\st i}$. In the former case, TTP sends  $f_{\st j}(x, y)$ to  $P_{\st j}$ and in the latter it sends $\Lambda_{\st i}$ to  $P_{\st j}$. The honest party always outputs the message that it obtained from TTP. A malicious party may output an arbitrary function of its initial inputs and the message it has obtained from TTP.  The ideal execution of $f$ on inputs $(x, y)$ and $z$ is denoted by $\mathsf{Ideal}^{\st f}_{\st\mathcal{A}(z), i}(x,y)$ and is defined as the output pair of the honest party and $\mathcal{A}$ from the above ideal execution.  In the real model, the real two-party protocol $\Gamma$ is executed
without the involvement of TTP. In this setting, $\mathcal{A}$ sends all messages on
behalf of the corrupted party and may follow an arbitrary strategy.
The honest party follows the instructions of $\Gamma$. The real execution of $\Gamma$ is denoted by $\mathsf{Real}^{\st \Gamma}_{\st\mathcal{A}(z), i}(x,y)$, it is defined as the joint output of the parties engaging in the real execution of $\Gamma$ (on the inputs), in the presence of $\mathcal{A}$.
 
 
 Next, we define security. At a high level, the definition states that a secure protocol in the real model emulates the ideal model. This is formulated by stating that adversaries in the ideal model can simulate executions of the protocol in the real model. 
 
\begin{definition}\label{def::MPC-active-adv}
Let $f$ be the two-party functionality defined above and $\Gamma$ be a two-party protocol that computes $f$.   Protocol $\Gamma$ securely computes $f$ with abort in the presence of static active adversaries if for every non-uniform probabilistic polynomial time adversary $\mathcal{A}$ for the real model, there exists a non-uniform probabilistic polynomial-time adversary (or simulator) $\mathsf{Sim}$ for the ideal model, such that for every $i\in \{0,1\}$, it holds that: 

\begin{equation*}
\{\mathsf {Ideal}^{\st f}_{\st \mathsf{Sim}(z), i}(x,y)\}_{\st x,y,z}\stackrel{c}{\equiv} \{\mathsf{Real}_{\st \mathcal{A}(z), i}^{\st \Gamma}(x,y) \}_{\st x,y,z}
\end{equation*}
%
\end{definition}
 
 
  
  

==> CCS-24/Sub-protocols.tex <==
% !TEX root =main.tex


\vspace{-4mm}



\section{Other Subroutines Used in \withFai}\label{sec::subroutines}
\vspace{-1mm}

In this section, we introduce three subroutines and a primitive that we will use in the instantiation of \p.%, known as \withFai. 


\vspace{-2.5mm}
\subsection{Verifiable Oblivious Polynomial Randomization (\vopr)}\label{sec::vopr}
\vspace{-.5mm}

%In this section, we present ``Verifiable Oblivious Polynomial Randomisation'' (VOPR) protocol. 

In the \vopr, two types of party are involved, (i) a sender, potentially a passive adversary, and (ii) a receiver, potentially an active adversary. The protocol enables the receiver, with input polynomial $\bm\beta$ (of degree $e'$), and the sender, with input random polynomials $\bm\psi$ (of degree $e$) and  $\bm{\alpha}$ (of degree $e+e'$),   to compute: $\bm\theta=\bm\psi\cdot \bm\beta+\bm\alpha$, satisfying the following conditions: (a) the receiver learns only $\bm\theta$ and gains no knowledge of the sender's input even when setting $\bm \beta=0$, (b) the sender gains no knowledge, and (c) protocol detects the receiver's misbehavior.  Thus, the functionality that  \vopr computes is defined as $f^{\st {\vopr}}( (\bm\psi, \bm{\alpha}), \bm\beta)\rightarrow(\bot, \bm\psi\cdot \bm\beta+\bm\alpha)$.  
%
We will use {\vopr} in \withFai for two main purposes:  (a) to enable a party to re-randomize its counterpart's polynomial (representing its set) and (b) to impose a MAC-like structure on the randomized polynomial.  This structure will allow a verifier to detect any modifications to \vopr's output. 

Now, we will outline how we design \vopr without using any zero-knowledge proofs.\footnote{Previously, Ghosh \textit{et al.}  \cite{GhoshN19} designed a protocol to meet similar security requirements that we laid out above. But, as shown in \cite{AbadiMZ21}, it  is susceptible to several serious attacks. } In the setup phase, both parties represent their input polynomials in the regular coefficient form; therefore, the sender's polynomials are defined as $\bm\psi=\sum\limits^{\st e}_{\st i=0}g_{\st i}\cdot x^{\st i}$ and  $\bm\alpha=\sum\limits^{\st e+e'}_{\st j=0}a_{\st j}\cdot x^{\st j}$ and the receiver's polynomial is defined as $\bm\beta=\sum\limits^{\st e'}_{\st i=0}b_{\st i}\cdot x^{\st i}$, where $b_{\st i}\neq 0$. But, the sender computes each coefficient $a_{\st j}$ (of polynomial $\bm \alpha$) as follows,  $a_{\st j}=\sum\limits^{\substack{\st k=e'\\ \st t=e}}_{\st t,k=0} a_{\st t,k}$,  where  $t+k=j$ and each $a_{\st t,k}$ is a random value. For instance, if $e=4$ and $e'=3$, then $a_{\st 3}=a_{\st \st 0,3}+a_{\st 3,0}+a_{\st 1,2}+a_{\st 2,1}$. Shortly, we explain why polynomial $\bm\alpha$ is constructed this way. 



In the computation phase,  to compute polynomial $\bm\theta$, the two parties interactively multiply and add the related coefficients using $\ole^{\st +}$. Specifically,
%
%For simplicity, let $i=0$. 
%
for every $j$  (where $0\leq j\leq e'$) the sender sends $g_{\st i}$ and $a_{\st i,j}$ to an instance of  $\ole^{\st +}$, while the receiver sends $b_{\st j}$ to the same instance,  which returns $c_{\st i,j}=g_{\st i}\cdot b_{\st j}+ a_{\st i,j}$ to the receiver. This process is repeated for every $i$, where $0 \leq i \leq e$. Then, the receiver uses $c_{\st i,j}$ values to construct the resulting polynomial, $\bm\theta=\bm\psi\cdot \bm\beta+\bm\alpha$.  

The sender imposes the above structure on (the coefficients of)  $\bm\alpha$ during the setup to enable the parties to securely compute $\bm\theta$ via  $\ole^{\st +}$.  This structure serves two key purposes: (1) allowing the sender  to blind each product $g_{\st i}\cdot b_{\st j}$  with random value $a_{\st i,j}$ which is a component of $\bm\alpha$'s coefficient and (2) enabling the receiver to construct a result polynomial in the form $\bm\theta=\bm\psi\cdot \bm\beta+\bm\alpha$. 


To verify the result's correctness, the sender selects a random value, $z$, and transmits it to the receiver.   Subsequently, the receiver computes  $\bm\theta(z)$ and $\bm\beta(z)$ and sends these two values to the sender. The sender computes  $\bm\psi(z)$ and $\bm\alpha(z)$ and proceeds to validate the equation $\bm\theta({ z})=\bm\psi({ z})\cdot \bm\beta({ z})+\bm\alpha({ z})$. If the check is successful, the sender accepts the result. Figure \ref{fig:VOPR} describes \vopr in detail. 


%\vspace{-1mm}
\input{VOPR}

Note that \vopr requires the sender to insert non-zero coefficients, i.e., $b_{\st i}\neq 0$ for all $i,0 \leq i \leq e'$. If the sender includes a zero-coefficient, then it will only obtain a random value (due to  $\ole^{\st +}$), making it fail to pass \vopr's verification phase. However, this requirement does not affect the correctness of \withFai, as we will explain in Section \ref{Fair-PSI-Protocol} and Appendix \ref{sec::error-prob}.  

\vspace{-2mm}



%\vspace{-1mm}
\begin{theorem}\label{theorem::VOPR}
%
Let $f^{\st \vopr}$ be the functionality defined above. If the enhanced \ole (i.e., $\ole^{\st +}$) is secure against malicious adversaries, then the  \vopr, presented in Figure \ref{fig:VOPR}, securely computes $f^{\st \vopr}$ in the presence of (i) semi-honest sender and honest receiver or (ii) malicious receiver and honest sender. 
%
\end{theorem}

\vspace{-2mm}
We refer readers to Appendix \ref{sec::proof-of-vopr} for the proof of Theorem \ref{theorem::VOPR}. 


\input{ZSPA.tex}

%\input{Arbiter-algorithm}

\input{Arbiter-protocol.tex}

==> CCS-24/Traitor-contract.tex <==
% !TEX root =main.tex


\subsection{Traitor's Contract (\SCtc)}

\SCtc incentivises a colluding server (who has signed \SCcc) to betray its counterpart and report the collusion without being penalised by \SCpc.  The Traitor’s contract promises that the reporting server will not be
punished by \SCpc which makes it safe for the reporting server to follow the collusion strategy (of \SCcc), and get away from the punishment imposed by \SCpc. Below, we restate the description of \SCtc. 


\begin{enumerate}
%
\item This contract is signed among $ { D}$ and the traitor server (TRA) who reports the collusion. This contract is signed only if the parties have already signed \SCpc. 
%
\item  $ { D}$ signs this contract only with the first server who reports the collusion. 
%
\item The traitor TRA must also provide to this contract the result of the computation, i.e., $f(x)$. The result provided in this contract could be different than the one provided in \SCpc, e.g., when TRA has to follow \SCcc and provide an incorrect result to \SCpc. 
%
\item  $  D$ needs to pay  $\wc \ +\ $\textcolor{blue}{ $\dc' \ + $} $\dc-\chc$ amount to this contract. This amount equals the maximum amount TRA could lose in \SCpc plus the reward. \textcolor{blue}{This deposit will be transferred via $\mathcal{SC}_{\st\epsi}$ to this contract.}  TRA must deposit in this contract $\chc$ amount to cover the cost of resolving a potential dispute.  
%
\item  This contract should be signed before the deadline  $T_{\st 2}$  for the delivery of the computation result in \SCpc. If it is not signed on time, then this contract will be terminated and any deposit paid will be refunded.
%
\item It is required that the TRA provide the computation result to this contract before the above deadline $T_{\st 2}$.
%
\item If this contract is fully signed, then during the execution of \SCpc, $ { D}$ always raises a dispute, i.e., takes step \ref{prisoner-cont-raise-disp} in \SCpc.
%
\item After \SCpc is finalized (with the involvement of the auditor), the following steps are taken to pay the parties involved.   
%
\begin{enumerate}
%
\item  if none of the servers cheated in \SCpc (according to the auditor), then $\wc \ +\ $\textcolor{blue}{ $\dc' \ + $} $\dc-\chc$ amount is refunded to \textcolor{blue}{$\mathcal{SC}_{\st\epsi}$} and TRA's deposit (i.e., $\chc$ amount) is transferred to $ { D}$. Nothing is paid to TRA. 
%
\item if in \SCpc, the other server did not cheat and TRA  cheated; however, TRA provided a correct result in this contract, then \textcolor{blue}{ $\dc' \ + $} $\dc-\chc$ amount is transferred to  \textcolor{blue}{$\mathcal{SC}_{\st\epsi}$}. Also,    TRA gets its deposit back (i.e., $\chc$ amount) plus $\wc$ amount for providing a correct result to this contract. 
%
\item if in \SCpc, both servers cheated; however, TRA delivered a correct computation result to this contract, then TRA gets its deposit back (i.e., $\chc$ amount), it also receives $\wc \ +\ $\textcolor{blue}{ $\dc' \ + $} $\dc-\chc$ amount.   
%
\item otherwise,  $\wc \ +\ $\textcolor{blue}{ $\dc' \ + $} $\dc-\chc$ and $\chc$ amounts are transferred to  \textcolor{blue}{$\mathcal{SC}_{\st\epsi}$} and TRA respectively. 
%
\end{enumerate}
%
\item If TRA provided a result to this contract, and deadline $T_{\st 3}$ (in \SCpc) has passed, then all deposits, if any left, will be transferred to TRA. %this ensures that the deposit will not be locked in the contract forever. 
%
\end{enumerate}

TRA must take the following three steps to report collusion: (i) it waits until \SCcc is signed by the other server, (ii) it reports the collusion to $ { D}$ before signing \SCcc, and (iii) it signs \SCcc only after it signed \SCtc with $ { D}$. 

Note that the original analysis of \SCtc does not require \SCtc to remain secret. Therefore, in our  \epsi, parties TRA and $ { D}$ can sign this contract and  then store its address in $\mathcal{SC}_{\st\epsi}$. Alternatively, to keep this contract confidential, $ { D}$ can deploy a template \SCtc to the blockchain and store the commitment of the contract's address (instead of the plaintext address) in $\mathcal{SC}_{\st\epsi}$. When a traitor (TRA) wants to report collusion, it signs the deployed \SCtc with  $ { D}$ which provides the commitment opening to TRA. In this case, at the time when the deposit is distributed,   either $ { D}$ or TRA   provides the opening of the commitment to  $\mathcal{SC}_{\st\epsi}$ which checks whether it matches the commitment. If the check passes, then it distributes the deposit as before. 



































==> CCS-24/U-PSI-Parties-Communication-cost.tex <==
% !TEX root =test.tex








\begin{table*}[!htbp]
\begin{footnotesize}
\begin{center}
\caption{ \small U-PSI communication: breakdown by step (in MB).}\label{tbl::PSI} 
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|} 
\hline 
%{\rowcolors{2}{blue!80!gray!18}{blue!10!gray!18}
\cellcolor{gray!20}\scriptsize \textbf{Party} &\cellcolor{gray!20} \scriptsize \textbf{Setting}&\cellcolor{gray!20} \scriptsize \textbf{Field-size} &\scriptsize\cellcolor{gray!20} $2^{\scriptscriptstyle 10}$\scriptsize &\scriptsize\cellcolor{gray!20}  $2^{\scriptscriptstyle 11}$&\scriptsize  \cellcolor{gray!20}$2^{\scriptscriptstyle 12}$&\scriptsize\cellcolor{gray!20}  $2^{\scriptscriptstyle 13}$&\scriptsize\cellcolor{gray!20} $2^{\scriptscriptstyle 14}$&\scriptsize\cellcolor{gray!20}   $2^{\scriptscriptstyle 15}$&\scriptsize\cellcolor{gray!20}  $2^{\scriptscriptstyle 16}$&\scriptsize\cellcolor{gray!20}   $2^{\scriptscriptstyle 17}$&\scriptsize \cellcolor{gray!20}  $2^{\scriptscriptstyle 18}$&\scriptsize \cellcolor{gray!20} $2^{\scriptscriptstyle 19}$&\scriptsize\cellcolor{gray!20}  $2^{\scriptscriptstyle 20}$ \\
    \hline
    
     \hline
%\NameEntry{\rotatebox{90}{standards}}
\multirow{20}{*}{\rotatebox[origin=c]{90}{Result Recipient}}
 \multirow{4}{*}&\multirow{5}{*}{\rotatebox[origin=c]{90}{2-Client}}&\cellcolor{cyan!20}\scriptsize 32-bit: &\cellcolor{cyan!20}\scriptsize  0.04&\cellcolor{cyan!20}\scriptsize  0.09&\cellcolor{cyan!20}\scriptsize 0.18   &\cellcolor{cyan!20}\scriptsize   0.37  &\cellcolor{cyan!20}\scriptsize    0.74 &\cellcolor{cyan!20}\scriptsize  1.49   &\cellcolor{cyan!20}\scriptsize 3.99  &\cellcolor{cyan!20} \scriptsize 7.99  &\cellcolor{cyan!20} \scriptsize 15.99  &\cellcolor{cyan!20}\scriptsize 31.98  & \cellcolor{cyan!20} \scriptsize 63.97 \\ 
   \cline{3-13}
  \multirow{4}{*}&&\cellcolor{white!20}\scriptsize  40-bit: &\cellcolor{white!20}\scriptsize 0.05 &\cellcolor{white!20}\scriptsize 0.1  &\cellcolor{white!20}\scriptsize  0.21 &\cellcolor{white!20}\scriptsize   0.42  &\cellcolor{white!20}\scriptsize   0.84  &\cellcolor{white!20}\scriptsize  1.69 &\cellcolor{white!20}\scriptsize 4.52 &\cellcolor{white!20} \scriptsize   9.04&\cellcolor{white!20} \scriptsize 18.1 &\cellcolor{white!20}\scriptsize 36.2  & \cellcolor{white!20} \scriptsize 72.4 \\ 
    \cline{3-13}
      \multirow{4}{*}&&\cellcolor{cyan!20}\scriptsize 60-bit: &\cellcolor{cyan!20}\scriptsize 0.06 &\cellcolor{cyan!20}\scriptsize 0.13&\cellcolor{cyan!20}\scriptsize   0.27&\cellcolor{cyan!20}\scriptsize    0.54 &\cellcolor{cyan!20}\scriptsize 1.09  &\cellcolor{cyan!20}\scriptsize  2.19   &\cellcolor{cyan!20}\scriptsize 5.84 &\cellcolor{cyan!20} \scriptsize   11.68&\cellcolor{cyan!20} \scriptsize  23.36 &\cellcolor{cyan!20}\scriptsize 46.74  & \cellcolor{cyan!20} \scriptsize 93.48 \\ 
    \cline{3-13}
          \multirow{4}{*}&&\cellcolor{white!20}\scriptsize  64-bit: &\cellcolor{white!20}\scriptsize 0.06 &\cellcolor{white!20}\scriptsize 0.14&\cellcolor{white!20}\scriptsize  0.28&\cellcolor{white!20}\scriptsize 0.57   &\cellcolor{white!20}\scriptsize  1.14  &\cellcolor{white!20}\scriptsize 2.28 &\cellcolor{white!20}\scriptsize 6.1 &\cellcolor{white!20} \scriptsize   12.21&\cellcolor{white!20} \scriptsize  24.42 &\cellcolor{white!20}\scriptsize  48.849 & \cellcolor{white!20} \scriptsize 97.7\\ 
    \cline{3-13}
              \multirow{4}{*}&&\cellcolor{cyan!20}\scriptsize  128-bit: &\cellcolor{cyan!20}\scriptsize  0.11&\cellcolor{cyan!20}\scriptsize  0.24&\cellcolor{cyan!20}\scriptsize  0.48  &\cellcolor{cyan!20}\scriptsize    0.96 &\cellcolor{cyan!20}\scriptsize 1.93  &\cellcolor{cyan!20}\scriptsize  3.87   &\cellcolor{cyan!20}\scriptsize   10.31&\cellcolor{cyan!20} \scriptsize  20.63 &\cellcolor{cyan!20} \scriptsize  41.28 &\cellcolor{cyan!20}\scriptsize  82.57 & \cellcolor{cyan!20} \scriptsize 165.14\\ 
    \cline{2-13}

&\multirow{5}{*}{\rotatebox[origin=c]{90}{3-Client}}&\cellcolor{white!20}\scriptsize  32-bit:&\cellcolor{white!20}\scriptsize    0.06&\cellcolor{white!20}  \scriptsize 0.14 &\cellcolor{white!20} \scriptsize 0.28&\cellcolor{white!20}\scriptsize 0.57   &\cellcolor{white!20}  \scriptsize 1.14 &\cellcolor{white!20}  \scriptsize 2.28  &\cellcolor{white!20} \scriptsize  6.1  &\cellcolor{white!20} \scriptsize 12.21 &\cellcolor{white!20} \scriptsize 41.28 &\cellcolor{white!20}\scriptsize 48.84  &\cellcolor{white!20}\scriptsize 97.7  \\ 
    \cline{3-13}
     &&\cellcolor{cyan!20}\scriptsize  40-bit:&\cellcolor{cyan!20}\scriptsize 0.08   &\cellcolor{cyan!20}  \scriptsize 0.16&\cellcolor{cyan!20} \scriptsize 0.33&\cellcolor{cyan!20}\scriptsize  0.66  &\cellcolor{cyan!20}  \scriptsize  1.34&\cellcolor{cyan!20}  \scriptsize 2.68&\cellcolor{cyan!20} \scriptsize 7.15  &\cellcolor{cyan!20} \scriptsize 14.31&\cellcolor{cyan!20} \scriptsize  28.63&\cellcolor{cyan!20}\scriptsize 57.27&\cellcolor{cyan!20}\scriptsize 114.56 \\ 
    \cline{3-13}

     &&\cellcolor{white!20}\scriptsize 60-bit:&\cellcolor{white!20}\scriptsize   0.11&\cellcolor{white!20}  \scriptsize  0.22&\cellcolor{white!20} \scriptsize 0.45&\cellcolor{white!20}\scriptsize  0.91 &\cellcolor{white!20}  \scriptsize  1.83&\cellcolor{white!20}  \scriptsize  3.67 &\cellcolor{white!20} \scriptsize   9.79&\cellcolor{white!20} \scriptsize  19.58&\cellcolor{white!20} \scriptsize 39.17&\cellcolor{white!20}\scriptsize 78.35&\cellcolor{white!20}\scriptsize 156.71 \\ 
    \cline{3-13}
     &&\cellcolor{cyan!20}\scriptsize 64-bit:&\cellcolor{cyan!20}\scriptsize  0.11  &\cellcolor{cyan!20}  \scriptsize 0.24&\cellcolor{cyan!20} \scriptsize 0.48&\cellcolor{cyan!20}\scriptsize 0.96 &\cellcolor{cyan!20}  \scriptsize 1.93&\cellcolor{cyan!20}  \scriptsize 3.87  &\cellcolor{cyan!20} \scriptsize 10.31&\cellcolor{cyan!20} \scriptsize 20.63&\cellcolor{cyan!20} \scriptsize 41.28&\cellcolor{cyan!20}\scriptsize  82.57&\cellcolor{cyan!20}\scriptsize  165.14 \\ 
    \cline{3-13}
         &&\cellcolor{white!20}\scriptsize   128-bit:&\cellcolor{white!20}\scriptsize   0.21&\cellcolor{white!20}  \scriptsize 0.43 &\cellcolor{white!20} \scriptsize  0.87&\cellcolor{white!20}\scriptsize    1.75&\cellcolor{white!20}  \scriptsize  3.51&\cellcolor{white!20}  \scriptsize    7.03&\cellcolor{white!20} \scriptsize 18.74  &\cellcolor{white!20} \scriptsize 37.49 &\cellcolor{white!20} \scriptsize 75&\cellcolor{white!20}\scriptsize  150.01  &\cellcolor{white!20}\scriptsize 300.03  \\ 
    \cline{2-13}

    &\multirow{5}{*}{\rotatebox[origin=c]{90}{5-Client}}&\cellcolor{cyan!20}\scriptsize 32-bit:&\cellcolor{cyan!20}\scriptsize  0.11&\cellcolor{cyan!20}  \scriptsize 0.24 &\cellcolor{cyan!20}\scriptsize   0.48&\cellcolor{cyan!20}\scriptsize   0.96&\cellcolor{cyan!20}\scriptsize 1.93&\cellcolor{cyan!20}  \scriptsize 3.87&\cellcolor{cyan!20}\scriptsize  10.31&\cellcolor{cyan!20}\scriptsize 20.63&\cellcolor{cyan!20}\scriptsize 83.43&\cellcolor{cyan!20}\scriptsize  82.57&\cellcolor{cyan!20}\scriptsize  165.14 \\ 
        \cline{3-13}
          & &\cellcolor{white!20}\scriptsize  40-bit:&\cellcolor{white!20}\scriptsize  0.14&\cellcolor{white!20}  \scriptsize  0.28&\cellcolor{white!20}\scriptsize   0.57 &\cellcolor{white!20}\scriptsize 1.16 &\cellcolor{white!20}\scriptsize 2.32&\cellcolor{white!20}  \scriptsize 4.66&\cellcolor{white!20}\scriptsize 12.42 &\cellcolor{white!20}\scriptsize  24.85&\cellcolor{white!20}\scriptsize  49.71&\cellcolor{white!20}\scriptsize 99.43&\cellcolor{white!20}\scriptsize  198.86\\ 
        \cline{3-13}
           &&\cellcolor{cyan!20}\scriptsize 60-bit:&\cellcolor{cyan!20}\scriptsize  0.2 &\cellcolor{cyan!20}  \scriptsize 0.41 &\cellcolor{cyan!20}\scriptsize 0.82 &\cellcolor{cyan!20}\scriptsize   1.65 &\cellcolor{cyan!20}\scriptsize 3.31&\cellcolor{cyan!20}  \scriptsize 6.63 &\cellcolor{cyan!20}\scriptsize  17.69&\cellcolor{cyan!20}\scriptsize 35.39&\cellcolor{cyan!20}\scriptsize  70.78&\cellcolor{cyan!20}\scriptsize  141.58&\cellcolor{cyan!20}\scriptsize  283.17  \\ 
        \cline{3-13}
          & &\cellcolor{white!20}\scriptsize  64-bit:&\cellcolor{white!20}\scriptsize  0.21&\cellcolor{white!20}  \scriptsize 0.43 &\cellcolor{white!20}\scriptsize   0.87&\cellcolor{white!20}\scriptsize  1.75&\cellcolor{white!20}\scriptsize 3.51&\cellcolor{white!20}  \scriptsize 7.03 &\cellcolor{white!20}\scriptsize  18.74&\cellcolor{white!20}\scriptsize  37.49&\cellcolor{white!20}\scriptsize  75&\cellcolor{white!20}\scriptsize 150&\cellcolor{white!20}\scriptsize  300 \\ 
        \cline{3-13}
          & &\cellcolor{cyan!20}\scriptsize 128-bit:&\cellcolor{cyan!20}\scriptsize  0.4&\cellcolor{cyan!20}  \scriptsize   0.82&\cellcolor{cyan!20}\scriptsize  1.65   &\cellcolor{cyan!20}\scriptsize  3.32&\cellcolor{cyan!20}\scriptsize  6.67&\cellcolor{cyan!20}  \scriptsize 13.35  &\cellcolor{cyan!20}\scriptsize  35.6 &\cellcolor{cyan!20}\scriptsize  71.21&\cellcolor{cyan!20}\scriptsize   142.44&\cellcolor{cyan!20}\scriptsize  284.89&\cellcolor{cyan!20}\scriptsize  569.81  \\ 
        \cline{2-13}
     &\multirow{5}{*}{\rotatebox[origin=c]{90}{10-Client}}&\cellcolor{white!20}\scriptsize  32-bit:&\cellcolor{white!20} \scriptsize  0.23&\cellcolor{white!20}\scriptsize 0.48  &\cellcolor{white!20}\scriptsize  0.97&\cellcolor{white!20}\scriptsize  1.94&\cellcolor{white!20} \scriptsize  3.9&\cellcolor{white!20}\scriptsize 7.82  &\cellcolor{white!20}\scriptsize 20.85  &\cellcolor{white!20}\scriptsize  41.71&\cellcolor{white!20}  \scriptsize 125.58&\cellcolor{white!20}\scriptsize 166.87 &\cellcolor{white!20} \scriptsize 333.75  \\ 
        \cline{3-13}
           &&\cellcolor{cyan!20}\scriptsize  40-bit:&\cellcolor{cyan!20}\scriptsize  0.29  &\cellcolor{cyan!20}  \scriptsize  0.59 &\cellcolor{cyan!20}\scriptsize 1.19    &\cellcolor{cyan!20}\scriptsize  2.39  &\cellcolor{cyan!20}\scriptsize 4.79 &\cellcolor{cyan!20}  \scriptsize 9.6 &\cellcolor{cyan!20}\scriptsize 25.59  &\cellcolor{cyan!20}\scriptsize  51.19 &\cellcolor{cyan!20}\scriptsize  102.4 &\cellcolor{cyan!20}\scriptsize 204.81 &\cellcolor{cyan!20}\scriptsize  409.63 \\ 
        \cline{3-13}
           &&\cellcolor{white!20}\scriptsize  60-bit:&\cellcolor{white!20}\scriptsize    0.42&\cellcolor{white!20}  \scriptsize   0.87&\cellcolor{white!20}\scriptsize   1.74 &\cellcolor{white!20}\scriptsize    3.5 &\cellcolor{white!20}\scriptsize  7.01&\cellcolor{white!20}  \scriptsize  14&\cellcolor{white!20}\scriptsize   37.45&\cellcolor{white!20}\scriptsize  74.9&\cellcolor{white!20}\scriptsize   149.81&\cellcolor{white!20}\scriptsize   299.65&\cellcolor{white!20}\scriptsize   599.31 \\ 
        \cline{3-13}
           &&\cellcolor{cyan!20}\scriptsize  64-bit:&\cellcolor{cyan!20}\scriptsize  0.45 &\cellcolor{cyan!20}  \scriptsize  0.92&\cellcolor{cyan!20}\scriptsize  1.85 &\cellcolor{cyan!20}\scriptsize   3.72 &\cellcolor{cyan!20}\scriptsize  7.46&\cellcolor{cyan!20}  \scriptsize  14.93 &\cellcolor{cyan!20}\scriptsize  39.82 &\cellcolor{cyan!20}\scriptsize  79.64 &\cellcolor{cyan!20}\scriptsize  159.3&\cellcolor{cyan!20}\scriptsize  318.62&\cellcolor{cyan!20}\scriptsize    637.25\\ 
        \cline{3-13}
          & &\cellcolor{white!20}\scriptsize  128-bit:&\cellcolor{white!20}\scriptsize  0.89&\cellcolor{white!20}  \scriptsize   1.8&\cellcolor{white!20}\scriptsize   3.61  &\cellcolor{white!20}\scriptsize 7.26   &\cellcolor{white!20}\scriptsize  14.56&\cellcolor{white!20}  \scriptsize 29.16 &\cellcolor{white!20}\scriptsize   77.75&\cellcolor{white!20}\scriptsize   155.5&\cellcolor{white!20}\scriptsize  311.04&\cellcolor{white!20}\scriptsize   622.11&\cellcolor{white!20}\scriptsize    1244.26 \\ 
        \cline{3-13}
       \hline

%\scriptsize Each  Authoriser 
\multirow{5}{*}{\rotatebox[origin=c]{90}{Each  Authoriser }}

     &\cellcolor{gray!40}&\cellcolor{cyan!20}\scriptsize 32-bit&\cellcolor{cyan!20} \scriptsize  0.02  &\cellcolor{cyan!20}\scriptsize  0.04 &\cellcolor{cyan!20}\scriptsize   0.09 &\cellcolor{cyan!20}\scriptsize   0.19 &\cellcolor{cyan!20}\scriptsize   0.39&\cellcolor{cyan!20} \scriptsize 0.79 &\cellcolor{cyan!20}\scriptsize 2.12   &\cellcolor{cyan!20} \scriptsize  4.25  &\cellcolor{cyan!20} \scriptsize 8.51  &\cellcolor{cyan!20}\scriptsize 17.02   &\cellcolor{cyan!20}\scriptsize  34.05   \\
        \cline{3-13}
           &\cellcolor{gray!40}&\cellcolor{white!20}\scriptsize 40-bit:&\cellcolor{white!20}\scriptsize  0.03  &\cellcolor{white!20}  \scriptsize 0.06  &\cellcolor{white!20}\scriptsize  0.12   &\cellcolor{white!20}\scriptsize 0.24   &\cellcolor{white!20}\scriptsize 0.49 &\cellcolor{white!20}  \scriptsize 0.99 &\cellcolor{white!20}\scriptsize 2.66  &\cellcolor{white!20}\scriptsize  5.32 &\cellcolor{white!20}\scriptsize 10.64  &\cellcolor{white!20}\scriptsize 21.28 &\cellcolor{white!20}\scriptsize 42.57  \\ 
        \cline{3-13}
           &\cellcolor{gray!40}&\cellcolor{cyan!20}\scriptsize 60-bit:&\cellcolor{cyan!20}\scriptsize  0.04  &\cellcolor{cyan!20}  \scriptsize 0.09  &\cellcolor{cyan!20}\scriptsize 0.18    &\cellcolor{cyan!20}\scriptsize   0.37  &\cellcolor{cyan!20}\scriptsize  0.74&\cellcolor{cyan!20}  \scriptsize  1.49&\cellcolor{cyan!20}\scriptsize 3.99  &\cellcolor{cyan!20}\scriptsize  7.98&\cellcolor{cyan!20}\scriptsize 15.96  &\cellcolor{cyan!20}\scriptsize  31.92 &\cellcolor{cyan!20}\scriptsize 63.85   \\ 
        \cline{3-13}
           &\cellcolor{gray!40}&\cellcolor{white!20}\scriptsize 64-bit:&\cellcolor{white!20}\scriptsize  0.04 &\cellcolor{white!20}  \scriptsize  0.09&\cellcolor{white!20}\scriptsize   0.19&\cellcolor{white!20}\scriptsize    0.39&\cellcolor{white!20}\scriptsize  0.79&\cellcolor{white!20}  \scriptsize   1.59&\cellcolor{white!20}\scriptsize  4.25 &\cellcolor{white!20}\scriptsize  8.51 &\cellcolor{white!20}\scriptsize 17.02 &\cellcolor{white!20}\scriptsize  34.05&\cellcolor{white!20}\scriptsize   68.11 \\ 
        \cline{3-13}
           &\cellcolor{gray!40}&\cellcolor{cyan!20}\scriptsize 128-bit:&\cellcolor{cyan!20}\scriptsize  0.09&\cellcolor{cyan!20}  \scriptsize   0.19&\cellcolor{cyan!20}\scriptsize 0.39     &\cellcolor{cyan!20}\scriptsize  0.79  &\cellcolor{cyan!20}\scriptsize  1.59&\cellcolor{cyan!20}  \scriptsize  3.19&\cellcolor{cyan!20}\scriptsize   8.51&\cellcolor{cyan!20}\scriptsize 17.02  &\cellcolor{cyan!20}\scriptsize  34.05&\cellcolor{cyan!20}\scriptsize  68.11 &\cellcolor{cyan!20}\scriptsize   136.23  \\ 
        \cline{3-13}
   
    \hline
%\scriptsize Cloud
\multirow{5}{*}{\rotatebox[origin=c]{90}{Cloud}}
    &\cellcolor{gray!40}&\cellcolor{white!20}\scriptsize  32-bit &\cellcolor{white!20} \scriptsize  0.02&\cellcolor{white!20} \scriptsize 0.04 &\cellcolor{white!20}\scriptsize 0.09   &\cellcolor{white!20} \scriptsize  0.19&\cellcolor{white!20}\scriptsize  0.39&\cellcolor{white!20}\scriptsize 0.79&\cellcolor{white!20}\scriptsize  2.1  &\cellcolor{white!20}\scriptsize  4.21  & \cellcolor{white!20}\scriptsize 8.42  &\cellcolor{white!20}\scriptsize 16.86  &\cellcolor{white!20}\scriptsize 33.72 \\
        \cline{3-13}
           &\cellcolor{gray!40}&\cellcolor{cyan!20}\scriptsize 40-bit:&\cellcolor{cyan!20}\scriptsize   0.03 &\cellcolor{cyan!20}  \scriptsize  0.06 &\cellcolor{cyan!20}\scriptsize   0.12  &\cellcolor{cyan!20}\scriptsize  0.24  &\cellcolor{cyan!20}\scriptsize 0.49 &\cellcolor{cyan!20}  \scriptsize  0.98&\cellcolor{cyan!20}\scriptsize  2.63 &\cellcolor{cyan!20}\scriptsize 5.26  &\cellcolor{cyan!20}\scriptsize 10.53  &\cellcolor{cyan!20}\scriptsize 21.07 &\cellcolor{cyan!20}\scriptsize 42.15   \\ 
        \cline{3-13}
           &\cellcolor{gray!40}&\cellcolor{white!20}\scriptsize 60-bit:&\cellcolor{white!20}\scriptsize  0.04  &\cellcolor{white!20}  \scriptsize   0.09&\cellcolor{white!20}\scriptsize 0.18   &\cellcolor{white!20}\scriptsize  0.36   &\cellcolor{white!20}\scriptsize  0.74&\cellcolor{white!20}  \scriptsize  1.48&\cellcolor{white!20}\scriptsize   3.95&\cellcolor{white!20}\scriptsize  7.9&\cellcolor{white!20}\scriptsize   15.8&\cellcolor{white!20}\scriptsize  31.61 &\cellcolor{white!20}\scriptsize  63.22  \\ 
        \cline{3-13}
           &\cellcolor{gray!40}&\cellcolor{cyan!20}\scriptsize 64-bit:&\cellcolor{cyan!20}\scriptsize  0.04 &\cellcolor{cyan!20}  \scriptsize  0.09&\cellcolor{cyan!20}\scriptsize 0.19   &\cellcolor{cyan!20}\scriptsize   0.39 &\cellcolor{cyan!20}\scriptsize 0.78 &\cellcolor{cyan!20}  \scriptsize  1.58 &\cellcolor{cyan!20}\scriptsize 4.21  &\cellcolor{cyan!20}\scriptsize  8.42 &\cellcolor{cyan!20}\scriptsize 16.85 &\cellcolor{cyan!20}\scriptsize  33.72&\cellcolor{cyan!20}\scriptsize 67.44   \\ 
        \cline{3-13}
           &\cellcolor{gray!40}&\cellcolor{white!20}\scriptsize 128-bit:&\cellcolor{white!20}\scriptsize  0.09&\cellcolor{white!20}  \scriptsize 0.19  &\cellcolor{white!20}\scriptsize 0.39     &\cellcolor{white!20}\scriptsize   0.78 &\cellcolor{white!20}\scriptsize  1.57&\cellcolor{white!20}  \scriptsize  3.16&\cellcolor{white!20}\scriptsize 8.42  &\cellcolor{white!20}\scriptsize   16.85&\cellcolor{white!20}\scriptsize  33.71&\cellcolor{white!20}\scriptsize   67.44&\cellcolor{white!20}\scriptsize 134.88    \\ 
        \cline{3-13}
       \hline
 
\end{tabular}
\end{center}
\end{footnotesize}
\end{table*}





%
%\begin{table*}[!htbp]
%\begin{footnotesize}
%\begin{center}
%\caption{ \small U-PSI communication cost when element and field bit-size is $32$: breakdown by step (in MB).}\label{tbl::PSI} 
%\renewcommand{\arraystretch}{1.3}
%\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|} 
%\hline 
%%{\rowcolors{2}{blue!80!gray!18}{blue!10!gray!18}
%\cellcolor{gray!20}\scriptsize \textbf{Party} &\cellcolor{gray!20} \scriptsize \textbf{Setting} &\scriptsize\cellcolor{gray!20} $2^{\scriptscriptstyle 10}$\scriptsize &\scriptsize\cellcolor{gray!20}  $2^{\scriptscriptstyle 11}$&\scriptsize  \cellcolor{gray!20}$2^{\scriptscriptstyle 12}$&\scriptsize\cellcolor{gray!20}  $2^{\scriptscriptstyle 13}$&\scriptsize\cellcolor{gray!20} $2^{\scriptscriptstyle 14}$&\scriptsize\cellcolor{gray!20}   $2^{\scriptscriptstyle 15}$&\scriptsize\cellcolor{gray!20}  $2^{\scriptscriptstyle 16}$&\scriptsize\cellcolor{gray!20}   $2^{\scriptscriptstyle 17}$&\scriptsize \cellcolor{gray!20}  $2^{\scriptscriptstyle 18}$&\scriptsize \cellcolor{gray!20} $2^{\scriptscriptstyle 19}$&\scriptsize\cellcolor{gray!20}  $2^{\scriptscriptstyle 20}$ \\
%    \hline
%    
%     \hline
%\NameEntry{\center \scriptsize Result \\ \scriptsize Recipient}
% \multirow{4}{*}&\cellcolor{cyan!20}  \scriptsize 2-Client: &\cellcolor{cyan!20}\scriptsize  0.04&\cellcolor{cyan!20}\scriptsize  0.09&\cellcolor{cyan!20}\scriptsize 0.18   &\cellcolor{cyan!20}\scriptsize   0.37  &\cellcolor{cyan!20}\scriptsize    0.74 &\cellcolor{cyan!20}\scriptsize  1.49   &\cellcolor{cyan!20}\scriptsize 3.99  &\cellcolor{cyan!20} \scriptsize 7.99  &\cellcolor{cyan!20} \scriptsize 15.99  &\cellcolor{cyan!20}\scriptsize 31.98  & \cellcolor{cyan!20} \scriptsize 63.97 \\ 
%    \cline{2-13}
% &\cellcolor{white!20}\scriptsize 3-Client:&\cellcolor{white!20}\scriptsize    0.06&\cellcolor{white!20}  \scriptsize 0.14 &\cellcolor{white!20} \scriptsize 0.28&\cellcolor{white!20}\scriptsize 0.57   &\cellcolor{white!20}  \scriptsize 1.14 &\cellcolor{white!20}  \scriptsize 2.28  &\cellcolor{white!20} \scriptsize  6.1  &\cellcolor{white!20} \scriptsize 12.21 &\cellcolor{white!20} \scriptsize 41.28 &\cellcolor{white!20}\scriptsize 48.84  &\cellcolor{white!20}\scriptsize 97.7  \\ 
%    \cline{2-13}
%    &\cellcolor{cyan!20}\scriptsize 5-Client:&\cellcolor{cyan!20}\scriptsize 0.11  &\cellcolor{cyan!20}  \scriptsize  0.24&\cellcolor{cyan!20}\scriptsize 0.48   &\cellcolor{cyan!20}\scriptsize 0.96   &\cellcolor{cyan!20}\scriptsize 1.93&\cellcolor{cyan!20}  \scriptsize 3.87 &\cellcolor{cyan!20}\scriptsize  10.31&\cellcolor{cyan!20}\scriptsize 20.63 &\cellcolor{cyan!20}\scriptsize 83.43 &\cellcolor{cyan!20}\scriptsize 82.57 &\cellcolor{cyan!20}\scriptsize 165.14   \\ 
%        \cline{2-13}
%    &\cellcolor{white!20}\scriptsize 10-Client:&\cellcolor{white!20} \scriptsize  0.23&\cellcolor{white!20}\scriptsize 0.48  &\cellcolor{white!20}\scriptsize  0.97&\cellcolor{white!20}\scriptsize  1.94&\cellcolor{white!20} \scriptsize  3.9&\cellcolor{white!20}\scriptsize 7.82  &\cellcolor{white!20}\scriptsize 20.85  &\cellcolor{white!20}\scriptsize  41.71&\cellcolor{white!20}  \scriptsize 125.58&\cellcolor{white!20}\scriptsize 166.87 &\cellcolor{white!20} \scriptsize 333.75  \\ 
%       \hline
%
%\scriptsize Each  Authoriser 
%
%    \cellcolor{cyan!20} \scriptsize &\cellcolor{cyan!20} &\cellcolor{cyan!20} \scriptsize  0.02  &\cellcolor{cyan!20}\scriptsize  0.04 &\cellcolor{cyan!20}\scriptsize   0.09 &\cellcolor{cyan!20}\scriptsize   0.19 &\cellcolor{cyan!20}\scriptsize   0.39&\cellcolor{cyan!20} \scriptsize 0.79 &\cellcolor{cyan!20}\scriptsize 2.12   &\cellcolor{cyan!20} \scriptsize  4.25  &\cellcolor{cyan!20} \scriptsize 8.51  &\cellcolor{cyan!20}\scriptsize 17.02   &\cellcolor{cyan!20}\scriptsize  34.05   \\
%   
%    \hline
%\scriptsize Cloud
%
%    \multirow{3}{*}%{\scriptsize Cloud-side computation}
%    &\cellcolor{white!20}\scriptsize   &\cellcolor{white!20} \scriptsize  0.02&\cellcolor{white!20} \scriptsize 0.04 &\cellcolor{white!20}\scriptsize 0.09   &\cellcolor{white!20} \scriptsize  0.19&\cellcolor{white!20}\scriptsize  0.39&\cellcolor{white!20}\scriptsize 0.79&\cellcolor{white!20}\scriptsize  2.1  &\cellcolor{white!20}\scriptsize  4.21  & \cellcolor{white!20}\scriptsize 8.42  &\cellcolor{white!20}\scriptsize 16.86  &\cellcolor{white!20}\scriptsize 33.72 \\
%       \hline
% 
%\end{tabular}
%\end{center}
%\end{footnotesize}
%\end{table*}



==> CCS-24/Unforgeable-poly-proof.tex <==
% !TEX root =main.tex



\section{Proof of Unforgeable Polynomials}\label{sec::proof-of-unforgeable-polys}




Our initial step is to prove Theorem \ref{proof::unforgeable-poly}, which concerns unforgeable polynomials.  


\begin{proof}

Let $\bm\tau=\bm\delta-\bm\gamma$ and $\bm\zeta=a\cdot x+b$. Since $\bm\gamma$ is a random polynomial of degree $d+1$ and unknown to the adversary when given $(\bm\theta, \bm\pi)$,  the adversary cannot gain any information about the factor $\bm\zeta$.  From its perspective, every polynomial of degree $1$ in $\mathbb{F}_{\st p}[X]$ is equally likely to be $\bm\zeta$. 

Furthermore,  the polynomial $\bm\tau$ has at most $Max\big(deg(\bm\delta), d+1\big)$ irreducible non-constant factors.  For $\bm\zeta $ to divide $\bm\tau$,  one of the factors of $\bm\tau$ must be equal to $\bm\zeta$. We  also know that $\bm\zeta$ has been picked uniformly at random (i.e., $a,b
\stackrel{\st \$}\leftarrow \mathbb F_{\st p}$). Thus, the probability that $\bm\zeta $ divides $\bm\tau$ is negligible with respect to the security parameter, $\lambda$. Specifically,

$$Pr[ \bm\zeta \ | \ (\bm\delta-\bm\gamma)]\leq \frac{Max\big(deg(\bm\delta), d+1\big)} {2^{\st \lambda}}=\negl(\lambda)$$
\end{proof} 

%$Max\big(deg(\theta'), d+1\big)$


% An interesting feature of an unforgeable polynomial is that the verifier can perform the check without needing to know the original polynomial $\bm\pi$. Another appealing feature of the unforgeable polynomial is that it supports \emph{linear combination} and accordingly \emph{batch verification}. Specifically, to turn $n$ arbitrary polynomials $[\bm\pi_{\st 1},..., \bm\pi_{\st n}]$ into unforgeable polynomials, one can construct  $\bm\theta_{\st i}=\bm\zeta\cdot \bm\omega_{\st i}\cdot \bm\pi_{\st i}+ \bm\gamma_{\st i} \bmod p$, where $\forall i, 1\leq i\leq n$.  
 
 

 
Next, we prove Theorem \ref{Unforgeable-Polynomials-Linear-Combination}, concerning unforgeable polynomials' linear combination.  
 
 

%%%%
\begin{proof}  
This proof serves as a generalization of that for Theorem \ref{proof::unforgeable-poly}.  
Let $\bm\tau_{\st j}=\bm\delta_{\st j}-\bm\gamma_{\st j}$ and $\bm\zeta=a\cdot x+b$. Since  every $\bm\gamma_{\st j}$ is a random polynomial of degree $d+1$ and unknown to the adversary, given $(\vv{\bm\theta}, \vv{\bm\pi})$,  the adversary cannot learn anything about the factor $\bm\zeta$. Each polynomial $\bm\tau_{\st j}$ has at most $Max\big(deg(\bm\delta_{\st j}), d+1\big)$ irreducible non-constant factors. 
%
%In order for $\bm\zeta$ to divide polynomial $\sum\limits_{\st j=1}^{\st t}\bm\delta_{\st j} + \sum\limits_{\st j=t+1}^{\st n}\bm\theta_{\st j} - \sum\limits_{\st j=1}^{\st n}\bm\gamma_{\st j}$  one of the factors of every $\bm\tau_{\st j}$ needs to equal $\bm\zeta$, where $1 \leq j \leq t$. 
%
We  know that $\bm\zeta$ has been picked uniformly at random (i.e., $a,b
\stackrel{\st \$}\leftarrow \mathbb F_{\st p}$). Therefore, the probability that $\bm\zeta$ divides $\sum\limits_{\st j=1}^{\st t}\bm\delta_{\st j} + \sum\limits_{\st j=t+1}^{\st n}\bm\theta_{\st j} - \sum\limits_{\st j=1}^{\st n}\bm\gamma_{\st j}$ equals the probability that $\bm\zeta$ equals to one of the factors of  every $\bm\tau_{\st j}$, that is negligible in the security parameter. Concretely,


$$Pr[ \bm\zeta \ | \ (\sum\limits_{\st j=1}^{\st t}\bm\delta_{\st j} + \sum\limits_{\st j=t+1}^{\st n}\bm\theta_{\st j} - \sum\limits_{\st j=1}^{\st n}\bm\gamma_{\st j} ) ]\leq  \frac{\prod \limits^{\st t}_{\st j=1}Max\big(deg(\bm\delta_{\st j}), d+1\big)} {2^{\st \lambda t}}=\negl(\lambda)$$
%
\end{proof} 


%It is not hard to see that, Theorem \ref{Unforgeable-Polynomials-Linear-Combination} is a generalisation of Theorem \ref{proof::unforgeable-poly}. Briefly, in \withFai, we will use unforgeable polynomials (and their linear combinations) to allow a smart contract to efficiently check whether the polynomials that the clients send to it are intact, i.e., they are \vopr's outputs.









==> CCS-24/Unforgeable-polynomials.tex <==
% !TEX root =main.tex






\vspace{-2.45mm}

\subsection{Unforgeable Polynomials}

\vspace{-1mm}

In this section, we introduce the new concept of unforgeable polynomials. Informally, an unforgeable polynomial is accompanied by a secret factor. To verify that an unforgeable polynomial has not been tampered with, a verifier can check whether the polynomial is divisible by the secret factor. 

To transform an arbitrary polynomial $\bm\pi$ of degree $d$ into an unforgeable polynomial $\bm\theta$, we can follow these steps: (i) select two secret random polynomials $(\bm\zeta, \bm \gamma)$ and (ii) calculate $\bm\theta=\bm\zeta\cdot\bm \pi + \bm \gamma \bmod p$, where  $deg(\bm\zeta)= 1, $ and   $deg(\bm\gamma)= d+1$. 


To determine whether $\bm\theta$ has been tampered with, a verifier (given $\bm\theta, \bm \gamma$, and $\bm\zeta$) can check if $\bm\theta-\bm \gamma$ is divisible by $\bm\zeta$. Informally, the security of an unforgeable polynomial asserts that an adversary (who is unaware of the two secret random polynomials) cannot tamper with an unforgeable polynomial without being detected, except with a negligible probability. Below, we formally state it. 

\vspace{-1mm}
\begin{theorem}[Unforgeable Polynomial]\label{proof::unforgeable-poly}
%Let polynomials $\zeta$ and $\gamma$ be two secret uniformly random polynomials (i.e., $\zeta, \gamma\stackrel{\st\$}\leftarrow \mathbb F_{\st p}[x]$),   $GCD(\zeta, \gamma)=1$, polynomial $\pi$ be an arbitrary polynomial,   $deg(\zeta)= 1, deg(\gamma)= d+1$,  $deg(\pi)=d$, and $p$ be a $\lambda$-bit prime number. Also, let polynomial $\theta$ be defined as  $\theta=\zeta\cdot \pi+ \gamma \bmod p$. Given $(\theta,\pi)$, the probability that a PPT adversary (which does not know $\zeta$ and $\gamma$) can forge $\theta$ to an arbitrary polynomial $\theta'$ such that  $\theta'\neq \theta$, $deg(\theta')\leq poly(\lambda)$, and $\zeta$ divides $\theta'-\gamma$ is negligible in the security parameter, i.e.,
%
Let polynomials $\bm\zeta$ and $\bm\gamma$ be secret uniformly random polynomials (i.e., $\bm\zeta, \bm\gamma\stackrel{\st\$}\leftarrow \mathbb F_{\st p}[x]$), polynomial $\bm\pi$ be an arbitrary polynomial,   $deg(\bm\zeta)= 1,$ $ deg(\bm\gamma)= d+1$,  $deg(\bm\pi)=d$, and $p$ be a $\lambda$-bit prime number. Also, let polynomial $\bm\theta$ be defined as  $\bm\theta=\bm\zeta\cdot\bm \pi+\bm \gamma \bmod p$. Given $(\bm\theta,\bm\pi)$, the probability that an adversary (which does not know $\bm\zeta$ and $\bm\gamma$) can forge $\bm\theta$ to an arbitrary polynomial $\bm\delta$ such that  $\bm\delta\neq \bm\theta$, $deg(\bm\delta)= const(\lambda)$, and $\bm\zeta$ divides $\bm\delta-\bm\gamma$ is negligible in the security parameter $\lambda$, i.e., 
%
$Pr[ \bm\zeta \ | \ (\bm\delta-\bm\gamma) ]\leq \negl(\lambda)$.

\end{theorem}


%\begin{proof}
%
%Let $\bm\tau=\bm\delta-\bm\gamma$ and $\bm\zeta=a\cdot x+b$. Since $\bm\gamma$ is a random polynomial of degree $2d+1$ and unknown to the adversary, given $(\bm\theta, \bm\pi)$,  the adversary cannot learn anything about the factor $\bm\zeta$; as from its point of view every polynomial of degree $1$ in $\mathbb{F}_{\st p}[X]$ is equally likely to be $\bm\zeta$. Moreover,  polynomial $\bm\tau$ has at most $Max\big(deg(\bm\delta), 2d+1\big)$ irreducible non-constant factors.  For $\bm\zeta $ to divide $\bm\tau$,  one of the factors of $\bm\tau$ must be equal to $\bm\zeta$. We  also know that $\bm\zeta$ has been picked uniformly at random (i.e., $a,b
%\stackrel{\st \$}\leftarrow \mathbb F_{\st p}$). Thus, the probability that $\bm\zeta $ divides $\bm\tau$ is negligible in the security parameter, $\lambda$. Specifically,
%
%$$Pr[ \bm\zeta \ | \ (\bm\delta-\bm\gamma)]\leq \frac{Max\big(deg(\bm\delta), 2d+1\big)} {2^{\st \lambda}}=\negl(\lambda)$$
%\end{proof} 

%$Max\big(deg(\theta'), d+1\big)$

\vspace{-2mm}
 An interesting feature of an unforgeable polynomial is that the verifier can perform the check without needing knowledge of the original polynomial $\bm\pi$. Another appealing aspect of the unforgeable polynomial is its  support for \emph{linear combination} and, consequently, \emph{batch verification}. Specifically, to transform $n$ arbitrary polynomials $[\bm\pi_{\st 1},..., \bm\pi_{\st n}]$ into unforgeable polynomials, one can construct  $\bm\theta_{\st i}=\bm\zeta\cdot \bm\pi_{\st i}+ \bm\gamma_{\st i} \bmod p$, where $\forall i, 1\leq i\leq n$.  
 
 
To verify the integrity of all polynomials $[\bm\theta_{\st 1},..., \bm\theta_{\st n}]$, a verifier can (i) compute their sum $\bm \chi=\sum\limits_{\st i=1}^{\st n}\bm\theta_{\st i}$ and (ii) check whether $\bm \chi- \sum\limits_{\st i=1}^{\st n}\bm\gamma_{\st i} $ is divisible by $\bm \zeta$.  Informally, the security of an unforgeable polynomial states that an adversary (who is unaware of the two secret random polynomials for each $\bm\theta_{\st i}$) cannot tamper with any subset of the unforgeable polynomials without being detected, except with a negligible probability. We formally state it, below. 
 
 
\vspace{-1.2mm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{theorem}[Unforgeable Polynomials' Linear Combination]\label{Unforgeable-Polynomials-Linear-Combination}
%
 Let polynomial $\bm\zeta$ be a secret polynomial picked uniformly at random; also, let   $\vv{\bm\gamma}=[\bm\gamma_{\st 1},..., \bm\gamma_{\st n}]$ be a vector of secret uniformly random polynomials (i.e., ${\bm\zeta}, \bm\gamma_{\st i} \stackrel{\st\$}\leftarrow \mathbb F_{\st p}[x]$),  $\vv{\bm\pi}=[\bm\pi_{\st 1},..., \bm\pi_{\st n}]$ be a vector of arbitrary polynomials,   $deg(\bm\zeta)= 1,  deg(\bm\gamma_{\st i})= d+1$,  $deg(\bm\pi_{\st i})=d$,  $p$ be a $\lambda$-bit prime number, and $1\leq i \leq n$. Moreover, let polynomial $\bm\theta_{\st i}$ be defined as  $\bm\theta_{\st i}=\bm\zeta\cdot  \bm\pi_{\st i}+ \bm\gamma_{\st i} \bmod p$, and $\vv{\bm\theta} = [\bm\theta_{\st 1},..., \bm\theta_{\st n}]$.  Given $(\vv{\bm\theta}, \vv{\bm\pi})$, the probability that an adversary (which does not know $\bm\zeta$ and $\vv{\bm\gamma}$) can forge $t$ polynomials, without loss of generality, let us say $\bm\theta_{\st 1},..., \bm\theta_{\st t} \in \vv{\bm\theta}$, to arbitrary polynomials $\bm\delta_{\st 1},..., \bm\delta_{\st t}$ such that   $\sum\limits_{\st j=1}^{\st t}\bm\delta_{\st j}\neq \sum\limits_{\st j=1}^{\st t}\bm\theta_{\st j}$, $deg(\bm\delta_{\st j})= const(\lambda)$, and $\bm\zeta$ divides $(\sum\limits_{\st j=1}^{\st t}\bm\delta_{\st j} + \sum\limits_{\st j=t+1}^{\st n}\bm\theta_{\st j} - \sum\limits_{\st j=1}^{\st n}\bm\gamma_{\st j} )$ is negligible in the security parameter $\lambda$, i.e.,  
\vspace{-2mm}
$$Pr[ \bm\zeta \ | \ (\sum\limits_{\st j=1}^{\st t}\bm\delta_{\st j} + \sum\limits_{\st j=t+1}^{\st n}\bm\theta_{\st j} - \sum\limits_{\st j=1}^{\st n}\bm\gamma_{\st j} ) ]\leq \negl(\lambda)$$ 

\end{theorem}



%%%%
%\begin{proof}  
%This proof is a generalisation of that of Theorem \ref{proof::unforgeable-poly}.  
%Let $\bm\tau_{\st j}=\bm\delta_{\st j}-\bm\gamma_{\st j}$ and $\bm\zeta=a\cdot x+b$. Since  every $\bm\gamma_{\st j}$ is a random polynomial of degree $2d+1$ and unknown to the adversary, given $(\vv{\bm\theta}, \vv{\bm\pi})$,  the adversary cannot learn anything about the factor $\bm\zeta$. Each polynomial $\bm\tau_{\st j}$ has at most $Max\big(deg(\bm\delta_{\st j}), 2d+1\big)$ irreducible non-constant factors. 
%%
%%In order for $\bm\zeta$ to divide polynomial $\sum\limits_{\st j=1}^{\st t}\bm\delta_{\st j} + \sum\limits_{\st j=t+1}^{\st n}\bm\theta_{\st j} - \sum\limits_{\st j=1}^{\st n}\bm\gamma_{\st j}$  one of the factors of every $\bm\tau_{\st j}$ needs to equal $\bm\zeta$, where $1 \leq j \leq t$. 
%%
%We  know that $\bm\zeta$ has been picked uniformly at random (i.e., $a,b
%\stackrel{\st \$}\leftarrow \mathbb F_{\st p}$). Therefore, the probability that $\bm\zeta$ divides $\sum\limits_{\st j=1}^{\st t}\bm\delta_{\st j} + \sum\limits_{\st j=t+1}^{\st n}\bm\theta_{\st j} - \sum\limits_{\st j=1}^{\st n}\bm\gamma_{\st j}$ equals the probability that $\bm\zeta$ equals to one of the factors of  every $\bm\tau_{\st j}$, that is negligible in the security parameter. Concretely,
%
%
%$$Pr[ \bm\zeta \ | \ (\sum\limits_{\st j=1}^{\st t}\bm\delta_{\st j} + \sum\limits_{\st j=t+1}^{\st n}\bm\theta_{\st j} - \sum\limits_{\st j=1}^{\st n}\bm\gamma_{\st j} ) ]\leq  \frac{\prod \limits^{\st t}_{\st j=1}Max\big(deg(\bm\delta_{\st j}), 2d+1\big)} {2^{\st \lambda t}}=\negl(\lambda)$$
%%
%\end{proof} 


%It is not hard to see that, Theorem \ref{Unforgeable-Polynomials-Linear-Combination} is a generalisation of Theorem \ref{proof::unforgeable-poly}. 

\vspace{-1.2mm}

Appendix \ref{sec::proof-of-unforgeable-polys} presents the proofs of Theorems \ref{proof::unforgeable-poly} and \ref{Unforgeable-Polynomials-Linear-Combination}. In \withFai, we will employ unforgeable polynomials to enable a smart contract to efficiently verify the integrity of the polynomials sent by clients, ensuring that they are indeed the outputs of \vopr.









==> CCS-24/VOPR-proof.tex <==
% !TEX root =main.tex





\section{Proof of \vopr}\label{sec::proof-of-vopr}
\begin{proof}

Before proving Theorem \ref{theorem::VOPR}, we present Lemma \ref{theorem::evaluation-of-random-poly} and Theorem \ref{theorem:coef-poly-prod} that will be used in the proof of Theorem \ref{theorem::VOPR}. 
\input{vopr-two-theorems}





We refer readers to Appendix \ref{sec::proof-of-poly-union} for the proof of Theorem \ref{theorem:coef-poly-prod}. Next, we  prove the main theorem, i.e., Theorem \ref{theorem::VOPR}, by considering the case where each party is corrupt, in turn. 


% In each case, we invoke the simulator with the corresponding party’s input and output. 

\

\noindent\textbf{Case 1: Corrupt sender.} In the real execution, the sender's view is defined as follows: 


$$ \mathsf{View}_{\st S}^{\st \vopr} \Big((\bm\psi, \bm{\alpha}), \bm\beta\Big)=\{\bm\psi, \bm{\alpha}, r_{\st S},  \bm\beta(z), \bm\theta(z), \mathsf{View}^{\st \ole^{\st +}}_{\st S}, \bot \}$$
%
where $r_{\st S}$ is the outcome of internal random coins of the sender and $\mathsf{View}^{\st \ole^{\st +}}_{\st S}$ refers to the sender's real-model view during the execution of  $\ole^{\st +}$. The simulator $\mathsf{Sim}^{\st \vopr}_{\st S}$, which receives $\bm\psi$ and $\bm \alpha$, works as follows. 
%
\begin{enumerate}
\item generates an empty view. It appends to the view polynomials $(\bm\psi$, $\bm{\alpha})$ and coins $r'_{\st S}$ chosen uniformly at random. 
%
\item computes polynomial $\bm\beta=\bm\beta_{\st 1} \cdot \bm\beta_{\st 2}$, where $\bm\beta_{\st 1}$ is a random polynomial of degree $1$ and $\bm\beta_{\st 2}$ is an arbitrary polynomial of degree $e'-1$. Next,  it constructs polynomial $\bm\theta$ as follows: $\bm\theta=\bm\psi\cdot \bm\beta+\bm \alpha$.

\item chooses value $z\stackrel{\st\$}\leftarrow \mathbb{F}_{p}$. Then, it evaluates polynomials $\bm\beta$ and $\bm\theta$  at point $z$. This results in values $\beta_{\st z}$ and $\theta_{\st z}$ respectively. It appends these two values to the view. 
\item extracts the sender-side simulation of $\ole^{\st +}$ from  $\ole^{\st +}$'s simulator. Let $\mathsf{Sim}^{\st \ole^{\st +}}_{\st S}$ be this simulation. Note, the latter simulation is guaranteed to exist, as $\ole^{\st +}$ has been proven secure (in \cite{GhoshN19}). It appends $\mathsf{Sim}^{\st \ole^{\st +}}_{\st S}$ and $\bot$ to its view. 
\end{enumerate}

Now, we are prepared to demonstrate that the two views are computationally indistinguishable. The sender's inputs are identical in both models, so they have identical distributions. Since the real-model semi-honest adversary samples its randomness according to the protocol's description, the random coins in both models have identical distributions.  Next, we explain why values $\bm\beta(z)$ in the real model and $\beta_{\st z}$ in the ideal model are (computationally) indistinguishable. In the real model, $\bm\beta(z)$ is the evaluation of polynomial $\bm\beta=\bm\beta_{\st 1}\cdot \bm\beta_{\st 2}$ at random point $z$, where $\bm\beta_{\st 1}$ is a random polynomial. We know that $\bm\beta(z)=\bm\beta_{\st 1}(z)\cdot \bm\beta_{\st 2}(z)$, for any (non-zero) $z$.  

Moreover, by Lemma \ref{theorem::evaluation-of-random-poly}, we know that $\bm\beta_{\st 1}(z)$ is a uniformly random value. Therefore, $\bm\beta(z)=\bm\beta_{\st 1}(z)\cdot \bm\beta_{\st 2}(z)$ is a uniformly random value as well. In the ideal world, polynomial $\bm\beta$ has the same structure as $\bm\beta$ has (i.e., $\bm\beta=\bm\beta_{\st 1}\cdot \bm\beta_{\st 2}$, where $\bm\beta_{\st 1}$ is a random polynomial). That means $\beta_{\st z}$ is a uniformly random value too. Thus,  $\bm\beta(z)$ and $\beta_{\st z}$ are computationally indistinguishable. Next, we turn our attention to values $\bm\theta(z)$ in the real model and $\theta_{\st z}$ in the ideal model. We know that $\bm\theta(z)$ is a function of $\bm\beta_{\st 1}(z)$, as polynomial $\bm\theta$ has been defined as $\bm\theta=\bm\psi\cdot \bm(\bm\beta_{\st 1}\cdot \bm\beta_{\st 2})+\bm\alpha$. Similarly, $\theta_{\st z}$ is a function of  $\beta_{\st z}$. As we have already discussed,  $\bm\beta(z)$ and $\beta_{\st z}$ are computationally indistinguishable, so are their functions $\bm\theta(z)$ and $\theta_{\st z}$. Moreover, as  $\ole^{\st +}$ has been proven secure,  $\mathsf{View}^{\st \ole^{\st +}}_{\st S}$ and  $\mathsf{Sim}^{\st \ole^{\st +}}_{\st S}$ are computationally indistinguishable. It is also clear that $\bot$ is identical in both models. We deduce that the two views are computationally indistinguishable.


\


\noindent\textbf{Case 2: Corrupt receiver.}  Let $\mathsf{Sim}^{\st\vopr}_{\st R}$ be the simulator, in this case, which uses a subroutine adversary, $\mathcal{A}_{\st R}$. $\mathsf{Sim}^{\st \vopr}_{\st R}$ works as follows. 
%
\begin{enumerate}
%
\item simulates ${\ole^{\st +}}$ and receives $\mathcal{A}_{\st R}$'s input coefficients $b_{\st j}$ for all $j$, $0\leq j \leq e'$, as we are in $f_{\st \ole^{\st +}}$-hybrid model.
%
\item reconstructs polynomial $\bm \beta$, given the above coefficients. 
%
\item simulates the honest sender's inputs as follows. 
%%%%%%%%%
It picks two random polynomials: ${\bm\psi}=\sum\limits^{\st e}_{\st i=0}{g}_{\st i}\cdot x^{\st i}$ and  ${\bm\alpha}=\sum\limits^{\st e+e'}_{\st j=0}{a}_{\st j}\cdot x^{\st j}$, such that ${g}_{\st i}\stackrel{\st \$}\leftarrow \mathbb{F}_{\st p}$ and  every $a_{\st j}$ has the  form: $a_{\st j}=\sum\limits^{\substack{\st k=e'\\ \st t=e}}_{\st t,k=0} a_{\st t,k}$,  where $t+k=j$ and $a_{\st t,k}\stackrel{\st \$}\leftarrow \mathbb{F}_{\st p}$. 
%%%%%%%
\item sends to ${\ole^{\st +}}$'s functionality values $g_{\st i}$ and $a_{\st i,j}$ and receives   $c_{\st i,j}$ from this functionality (for all $i,j$).
%
\item sends all ${c}_{\st i,j}$ to TTP and receives polynomial ${\bm\theta}$. 
%
\item picks a random value $ z$ from $\mathbb{F}_{\st p}$. Then, it computes $ \psi_{\st  z} = {\bm\psi}(  z)$ and $\alpha_{\st  z}= {\bm\alpha}(z)$. 
%
\item sends $ z$ and all ${c}_{\st i,j}$ to $\mathcal{A}_{\st R}$ which sends back $\theta_{ z}$ and $\beta_{\st z}$ to the simulator. 
%
\item sends  $ \psi_{\st  z}$ and $\alpha_{\st z}$ to $\mathcal{A}_{\st R}$. 
%
\item checks if the following relation holds:

\vspace{-1mm}
\begin{equation}\label{equ::beta}
 \beta_{\st \bar z}={\bm\beta}( z) \hspace{3mm} \wedge \hspace{6mm} \theta_{\st  z}={\bm\theta}( z) \hspace{3mm}\wedge\hspace{3mm} {\bm\theta}( z)=  \psi_{\st  z}\cdot \beta_{\st  z}+\alpha_{\st  z}
 \end{equation}
 %
% \begin{equation}\label{equ::theta}
% \bar\theta_{\st \bar z}=\bar{\bm\theta}(\bar z) 
% \end{equation}
% %
%\begin{equation}\label{equ::theta-equals=psi}
%\bar{\bm\theta}(\bar z)= \bar \psi_{\st \bar z}\cdot \bar\beta_{\st \bar z}+\bar\alpha_{\st  \bar z}
%  \end{equation}
%%
% \begin{equation}\label{equ::theta-evl-equals=psi}
% \bar\theta_{\st \bar z}= \bar \psi_{\st \bar z}\cdot \bar\beta_{\st \bar z}+\bar\alpha_{\st  \bar z}
 %\end{equation}
%





%%%%%%%%%%%%%%%


%
% $\bar{\bm\theta}(\bar z) =\bar\theta_{\st \bar z} = \bar \psi_{\st \bar z}\cdot \bar\beta_{\st \bar z}+\bar\alpha_{\st  \bar z}$. 
 %
 If Relation \ref{equ::beta} does not hold, it aborts (i.e., sends abort signal $\Lambda$ to the sender) and still proceeds to the next step. 
 
 \item outputs whatever $\mathcal{A}_{\st R}$ outputs. 
%
\end{enumerate}

We initially direct our attention to the adversary's output. Both values of $z$ in the real and ideal models have been selected uniformly at random from $\mathbb{F}_{\st p}$. Therefore, they have identical distributions. In the real model, values  $\psi_{\st z}$ and $\alpha_{\st z}$ are the result of the evaluation of two random polynomials at (random) point $z$. In the ideal model, values $\psi_{\st  z}$ and $\alpha_{\st z}$ are also the result of the evaluation of two random polynomials (i.e., ${\bm\psi}$ and ${\bm\alpha}$) at point $ z$.  By Lemma \ref{theorem::evaluation-of-random-poly}, we know that the evaluation of a random polynomial at an arbitrary value  
 yields a uniformly random value in $\mathbb{F}_{\st p}$. Therefore, the distribution of pair $(\psi_{\st z}, \alpha_{\st z})$ in the real model is identical to that of pair $( \psi_{\st  z}, \alpha_{\st  z})$ in the ideal model. 
 
 Moreover, the final result (i.e., values ${c}_{\st i,j}$) in the real model shares the same distribution as the final result (i.e., values ${c}_{\st i,j}$)  in the ideal model, since they are the outputs of the ideal calls to $f_{\st \ole^{\st +}}$, within the context of the $f_{\st \ole^{\st +}}$-hybrid model. 

Next, we turn our attention to the sender's output. We will demonstrate that the output distributions of the honest sender in both the ideal and real models exhibit statistical closeness. 
%
%Note that the messages distributions the sender receive from the ideal call to $f_{\st \text{OLE}^{\st +}}$ are identical in both models. 
%
Our focus will be on the probability that it aborts in each model, as it does not receive any other output. In the ideal model, $\mathsf{Sim}^{\st \vopr}_{\st R}$ is given the honestly generated result polynomial ${\bm \theta}$ (computed by TTP) and the adversary's input polynomial ${\bm \beta}$. $\mathsf{Sim}^{\st \vopr}_{\st R}$ aborts with a probability of 1 if Relation \ref{equ::beta} (on page \pageref{equ::beta}) does not hold. However, in the real model, the honest sender (in addition to its inputs) is given only $\beta_{\st  z}$ and $\theta_{\st  z}$ and is not given polynomials ${\bm\beta}$ and  ${\bm\theta}$; it wants to check if the following equation holds, $\theta_{\st z} =  \psi_{\st z}\cdot  \beta_{\st z}+ \alpha_{\st z}$. 

Note that polynomial $\bm\theta=\bm\psi\cdot \bm\beta+\bm\alpha$ (resulted from ${c}_{\st i,j}$) is well-structured, as it satisfies the following three conditions (regardless of the adversary's input $\bm\beta$ to $\ole^{\st +}$): 
\begin{enumerate}%[i.]

\item $deg(\bm\theta)=Max \Big(deg(\bm\beta)+deg(\bm\psi), deg(\bm\alpha) \Big)$, as $\mathbb{F}_{\st p}[X]$ is an integral domain and ($\bm\psi,\bm\alpha$) are random polynomials.

\item  the roots of the product polynomial $\bm\nu=\bm\psi\cdot \bm\beta$ contains exactly both polynomials' roots, by Theorem \ref{theorem:coef-poly-prod}, on page \pageref{theorem:coef-poly-prod}.

\item  the roots of $\bm\nu+\bm\alpha$ is the intersection of the roots of $\bm\nu$ and $\bm\alpha$, as demonstrated in \cite{DBLP:conf/crypto/KissnerS05}. 
 
 \end{enumerate}
 
 Furthermore, polynomial $\bm \theta$ reveals no information (about  $\bm \psi$ and $\bm\alpha$ except their degrees) to the adversary and the pair $(\psi_{\st z}, \alpha_{\st z})$ is given to the adversary after it sends the pair $(\theta_{\st z}, \beta_{\st z})$ to the sender. 
%
There are exactly four cases where pair $(\theta_{\st z}, \beta_{\st z})$ can be constructed by the real-model adversary. Below, we state each case and the probability that the adversary is detected in that case during the verification, i.e., $\theta_{\st z}\stackrel{\st ?}=\psi{\st z}\cdot \beta_{\st z}+\alpha_{\st z}$. 
%
\begin{enumerate}
%
\item $\theta_{\st z}= \bm\theta(z) \wedge  \beta_{\st  z}={\bm\beta}( z)$. This is a trivial non-interesting case, as the adversary has behaved honestly, so it can always pass the verification. %, i.e., $\theta_{\st z}\stackrel{\st ?}=\psi{\st z}\cdot \beta_{\st z}+\alpha_{\st z}$.
%
\item $\theta_{\st z}\neq \bm\theta(z) \wedge  \beta_{\st  z}={\bm\beta}( z)$. In this case, the adversary is detected with a probability of 1. 
%
\item $\theta_{\st z}= \bm\theta(z) \wedge  \beta_{\st  z}\neq {\bm\beta}( z)$.  In this case, the adversary is also detected with a probability of 1.
%
\item $\theta_{\st z}\neq \bm\theta(z) \wedge  \beta_{\st  z} \neq {\bm\beta}( z)$. In this case, the adversary is detected with an overwhelming probability, i.e., $1-\frac{1}{2^{\st 2\lambda}}$. 
%
\end{enumerate}



As demonstrated above, in the real model, the minimum probability of the honest sender aborting in the event of adversarial behavior is $1-\frac{1}{2^{\st 2\lambda}}$. Hence, the output distributions of the honest sender in both the ideal and real models are statistically close, i.e., $1$ \text{vs} $1-\frac{1}{2^{\st 2\lambda}}$. 

In conclusion, we establish that the distribution of the joint outputs from the honest sender and the adversary in both the real and ideal models is computationally indistinguishable.
%
  \end{proof}
  
  
  
  
  
  
  
  
  
  
  
  

==> CCS-24/VOPR.tex <==
% !TEX root =main.tex



%%%%%%%%
\begin{figure}[ht]%[!htbp]
\setlength{\fboxsep}{1pt}
\begin{center}
    \begin{tcolorbox}[enhanced,width=3.3in,height=99.2mm,right=.5mm,
    drop fuzzy shadow southwest,
    colframe=black,colback=white]
%%%%%%%%
\vspace{-2.2mm}
\begin{enumerate}[leftmargin=-.2mm]
\small{
\item[$\bullet$] \textit{Input.}
\begin{enumerate}
\item[$\bullet$]  \textit{Public Parameters}: upper bound on input polynomials' degree: $e$ and $e'$. %, where $e\geq e'$.
%\item[$\bullet$]  \textit{Sender}: picks an upper bound on input polynomials's degree:  $d$ and $d'$. It sends them to the receiver.

\vspace{-1mm}
\item[$\bullet$]  \textit{Sender Input}:  random polynomials: $\bm\psi=\sum\limits^{\st e}_{\st i=0}g_{\st i}\cdot x^{\st i}$ and  $\bm\alpha=\sum\limits^{\st e+e'}_{\st j=0}a_{\st j}\cdot x^{\st j}$, where $g_{\st i}\stackrel{\st \$}\leftarrow \mathbb{F}_p$.  Each $a_{\st j}$ has the  form: $a_{\st j}=\sum\limits^{\substack{\st k=e'\\ \st t=e}}_{\st t,k=0} a_{\st t,k}$,  such that $t+k=j$ and $a_{\st t,k}\stackrel{\st \$}\leftarrow \mathbb{F}_p$.

\vspace{-1mm}
\item[$\bullet$] \textit{Receiver Input}:  polynomial $\bm\beta=\bm\beta_{\st 1}\cdot \bm\beta_{\st 2}=\sum\limits^{\st e'}_{\st i=0}b_{\st i}\cdot x^{\st i}$, where $\bm\beta_{\st 1}$ is a random polynomial of degree $1$, $\bm\beta_{\st 2}$ is an arbitrary polynomial of degree $e'-1$, and $b_{\st i}\neq 0$.


\end{enumerate}
\item[$\bullet$] \textit{Output.} The receiver obtains $\bm\theta=\bm\psi\cdot \bm\beta+\bm\alpha$.
\item \textbf{Computation:}

\begin{enumerate} [leftmargin=1.7mm]

\item Sender and receiver together for every $j$, $0\leq j\leq e'$,  invoke $e+1$ instances of $\ole^{\st +}$. In particular, $\forall j, 0\leq j\leq e'$: sender sends $g_{\st i}$ and $a_{\st i,j}$ while the receiver sends $b_{\st j}$ to $\ole^{\st +}$ that returns: $c_{\st i,j}=g_{\st i}\cdot b_{\st j}+ a_{\st i,j}$ to the receiver ($\forall i, 0\leq i\leq e$). 


 \item The receiver sums component-wise values $c_{\st i,j}$  that results:
 %
 \vspace{-1.7mm}
 %
  $$\bm\theta=\bm\psi\cdot \bm\beta+\bm\alpha=\sum\limits^{\substack{\st i=e\\ \st j=e'}}_{\st i,j=0}c_{\st i, j}\cdot x^{\st i+j}$$ 
 %
  \vspace{-3mm}
  %
 




% \item The receiver sums component-wise values $c_{\st i,j}$  that results polynomial $\bm\theta=\bm\psi\cdot \bm\beta+\bm\alpha=\sum\limits^{\st e+e'}_{\st j=0}c_{\st j}\cdot x^{\st j}$, where  each $c_{\st j}$ has   form: $c_{\st j}=\sum\limits^{\substack{\st k=e'\\ \st t=e}}_{\st  t,k=0} c_{\st t,k}$, such that $ t+k=j$.
%\item Sender: $\forall j, 1\leq j\leq 2d+1$, computes $a_{\st j}=a(x_{\st j})$ and $r_{\st j}=r(x_{\st j})$. Then, it  inserts $(a_{\st j}, r_{\st j})$ into  $\mathcal{F}_{\st OLE^{\st +}}$
%\item\label{computing-receiver} Receiver:  $\forall j, 1 \leq j\leq 2d+1$, computes $b_{\st j}=b(x_{\st j})$. Then, it  inserts $b_{\st j}$ into  $\mathcal{F}_{\st OLE^{\st +}}$ and receives $s_{\st j}=a_{\st j}+b_{\st j}\cdot r_{\st j}$. It interpolates a polynomial $s(x)$ using pairs $s_{\st j},x_{\st j}$. 
\end{enumerate}
\vspace{-1mm}
\item \label{Verification} \textbf{Verification:}
\begin{enumerate}[leftmargin=1.7mm]

\item \label{picking-random-x}Sender: picks a random non-zero value  $z$ and sends it to the receiver. 

\item\label{receiver-OLE-invocation} Receiver: sends $\theta_{\st z}=\bm\theta(z)$ and $\beta_{\st z}=\bm\beta(z)$ to the sender.

\item\label{receiver-OLE-invocation} Sender:  computes $\psi_{\st z}=\bm\psi(z)$ and $\alpha_{\st z}=\bm\alpha(z)$ and checks   if equation  $\theta_{\st z}=\psi{\st z}\cdot \beta_{\st z}+\alpha_{\st z}$ holds. If the equation holds, it concludes that the computation was performed correctly. Otherwise, it aborts. 
%
\end{enumerate}
}
 \end{enumerate}
 \end{tcolorbox}
\end{center}
\vspace{-4.5mm}
\caption{Verifiable Oblivious Polynomial Randomization.} 
\label{fig:VOPR}
\vspace{-6mm}
\end{figure}
 %%%%%%%


==> CCS-24/ZSPA-A-proof.tex <==
% !TEX root =main.tex




%\subsection{Proof of the ZSPA-A Protocol}\label{subsec::ZSPA-A-proof}

%Below, we prove Theorem \ref{theorem::ZSPA-A}, i.e., the security of the ZSPA-A.  Note, to allow this proof to be self-contained, we repeat some content from the proof of Theorem \ref{theorem::ZSPA-comp-correctness}. 

 \vspace{-2mm}
\section{Proof of \zspaa}\label{sec::proof-of-zspa-a}
\begin{proof}
First, we consider the case where a sender, who (may collude with $m-2$ senders and) generates pairs $(g,q)$, is corrupt. 

\

\noindent\textbf{Case 1: Corrupt sender.}  Let $\mathsf{Sim}^{\st \zspaa}_{\st S}$ be the simulator using a subroutine adversary, $\mathcal{A}_{\st S}$. Below, we explain how $\mathsf{Sim}^{\st \zspaa}_{\st S}$ works.  


%%%%%%%%%%%%%%%%%%%
\begin{enumerate}
%
\item simulates  \ct  and receives the output value $ k$ from $f_{\st \ct}$.
%
\item sends $ k$ to TTP and receives back from it $m$ pairs, where each pair is of the form $( g,  q)$. 
%
\item sends $ k$ to $\mathcal{A}_{\st S}$ and receives back from it $m$ pairs  where each pair is of the form $( g',  q')$. 
%

\item constructs an empty vector $ L$. $\mathsf{Sim}^{\st \zspaa}_{\st S}$ checks whether the following equations hold for each $j$-th pair: $ g= g' \hspace{2mm} \wedge  \hspace{2mm}  q= q'$. If these two equations do not hold, it sends an abort message $\Lambda$ to other receiver clients, appends the index of the pair (i.e., $j$) to $ L$, and proceeds to the next step for the valid pairs. In the case where there are no valid pairs, it moves on to step \ref{adversary-outputs}. 
%
\item picks a random polynomial ${\bm \zeta}$ of degree $1$. Moreover, for every $j\notin  L$, $\mathsf{Sim}^{\st \zspaa}_{\st S}$ picks a random polynomial ${\bm\xi}^{\st (j)}$ of degree $b'-1$, where $1\leq j \leq m$.
%

\item computes $m$ pseudorandom values  for every $i,j'$, where $0\leq i \leq b'$ and $j'\notin  L$ as follows.   
%
$$\forall j', 1\leq j' \leq m-1: z_{\st i,j}=\mathtt{PRF}( k,i||j')\hspace{5mm}  \text{and }\hspace{5mm} z_{\st i,m}=-\sum\limits^{\st m-1}_{\st j'=1}z_{\st i,j}$$ 
%
 \item generates polynomial ${\bm\mu}^{\st (j)}$, for every $j \notin L$, as follows:
  %
   ${\bm\mu}^{\st (j)} = {\bm\zeta}\cdot {\bm\xi}^{\st (j)}-\bm\tau^{\st (j)}$, where ${\bm\tau}^{\st (j)}=\sum\limits^{\st b'}_{\st i=0}z_{\st i,j}\cdot x^{\st i}$.
%
\item sends the above ${\bm \zeta}$,  ${\bm\xi}^{\st (j)}$, and ${\bm\mu}^{\st (j)}$ to all parties (i.e., $\mathcal{A}_{\st S}$ and the receivers), for every $j\notin L$. 
%
\item\label{adversary-outputs} outputs whatever $\mathcal{A}_{\st S}$ outputs.
%
 \end{enumerate}
%%%%%%%%%%%%%%%%%

 Now, we focus on the adversary’s output. In the real model, the messages that the adversary receives include those messages it receives as the result of the ideal call to $f_{\st \ct}$ and (${\bm \zeta}, {\bm\xi}^{\st (j)}, \bm\mu^{\st (j)}$), where $j \notin L$ and $1\leq j\leq m$. Those messages yielded from the ideal calls have an identical distribution to the distribution of the messages in the ideal model, as \ct is secure. The distribution of each $\bm\mu^{\st (j)}$ depends on the distribution of its components; namely, ${\bm \zeta}, {\bm\xi}^{\st (j)}$, and $\bm \tau^{\st j}$. As we are in the $f_{\st \ct}$-hybrid model, the distributions of $\bm \tau^{\st (j)}$ in the real model and ${\bm \tau}^{\st (j)}$ in the ideal model are identical, as they were derived from the output of $f_{\st \ct}$. Furthermore, in the real model, each polynomial  ${\bm \zeta}$ and ${\bm\xi}^{\st (j)}$ has been picked uniformly at random and they are independent of the clients' and the adversary's inputs. The same arguments hold for  ($ {\bm \zeta}, {\bm\xi}^{\st (j)}, {\bm\mu}^{\st (j)}$) in the ideal model. Therefore, (${\bm \zeta}, {\bm\xi}^{\st (j)}, {\bm\mu}^{\st (j)}$) in the real model and ($ {\bm \zeta}, {\bm\xi}^{\st (j)}, {\bm\mu}^{\st (j)}$) in the ideal model have identical distributions. 
 
 
 
 
 Next, we turn our attention to the receiver’s output. We will show that the output distributions of an honest receiver and the auditor in the ideal and real models are computationally indistinguishable. In the real model,  each element of the pair $(g, p)$ is the output of a deterministic function on the output of $f_{\st \ct}$. We know the outputs of $f_{\st \ct}$ in the real and ideal models have an identical distribution, and so do the evaluations of deterministic functions (namely Merkle tree, $\mathtt{H}$, and $\mathtt{PRF}$) on them. Therefore, each pair $(g,q)$ in the real model has an identical distribution to the pair $( g, q)$ in the ideal model.  For the same reasons, the honest receiver in the real model aborts with the same probability as  $\mathsf{Sim}^{\st \zspaa}_{\st S}$ does in the ideal model.  
 
 The same argument holds for the arbiter's output, as it performs the same checks that an honest receiver does.  Thus, the distribution of the joint outputs of the adversary, honest receiver, and honest in the real and ideal models is computationally indistinguishable. 

\

\noindent\textbf{Case 2: Corrupt receiver.}   Let $\mathsf{Sim}^{\st \zspaa}_{\st R}$ be the simulator that uses subroutine adversary $\mathcal{A}_{\st R}$. Below, we explain how $\mathsf{Sim}^{\st \zspaa}_{\st R}$ works. 




\begin{enumerate}
%
\item simulates  \zspa and receives the $m$ output pairs of the form $( k,  g,  q) $ from $f^{\st \zspa}$.
%
\item sends $( k,  g,  q) $ to $\mathcal{A}_{\st R}$ and receives $m$ keys, $ k'_{\st j}$, where $1\leq j \leq m$. 
%
\item\label{ZSPA-A-Case-2-generate-z} generates an empty vector $ L$. Next, for every $j$, $\mathsf{Sim}^{\st \zspaa}_{\st R}$ computes $q'_{\st j}$ as $\mathtt {H}( k'_{\st j})=q_{\st j}$.  It generates $g_{\st j}$ as follows. 


\begin{enumerate}

\item\label{gen-pr-vals} for every $i$ (where $0\leq i \leq b'$), generates $m$ pseudorandom values as below. 
%
 $$\forall j, 1\leq j' \leq m-1: z_{\scriptscriptstyle i,j}=\mathtt{PRF}( k'_{\st j},i||j'), \hspace{5mm} z_{\scriptscriptstyle i,m}=-\sum\limits^{\scriptscriptstyle m-1}_{\scriptscriptstyle j=1}z_{\scriptscriptstyle i,j}$$
%
\item   constructs a Merkle tree on top of all pseudorandom values,  

$\mathtt{MT.genTree}(z_{\scriptscriptstyle 0,1},...,z_{\scriptscriptstyle b', m})\rightarrow  g'_{\st j}$. 
%
\end{enumerate}
%
\item checks if the following equations hold for each $j$-th pair: 
%
$( k=    k'_{\st j}) \ \wedge\  ( g=   g'_{\st j})  \ \wedge\ ( q=  q'_{\st j})$.
%
%\item generates an empty vector $\bar L$ and then checks if the following equations hold for each $j$-th pair: 
%%
%$\bar k=   \bar k' \ \wedge\  \bar g=  \bar g'  \ \wedge\ \bar q= \bar q'$.
%
\item If these equations do not hold for $j$-th value, it appends $j$ to $ L$ and proceeds to the next step for the valid value. In the case where there is no valid value, it moves on to step \ref{adversary-outputs--}. 


\item picks a random polynomial ${\bm \zeta}$ of degree $1$. Also, for every $j\notin  L$, it picks a random polynomial ${\bm\xi}^{\st (j)}$ of degree $b'-1$, where $1\leq j \leq m$. 
%

%\item computes $m$ pseudorandom values  for every $i,j'$, where $0\leq i \leq \bar d$ and $j'\notin \bar L$ as follows.   
%%
%$\forall j', 1\leq j' \leq m-1: z_{\st i,j}=\mathtt{PRF}(\bar k,i||j')\hspace{3mm}  \text{and }\hspace{3mm} z_{\st i,m}=-\sum\limits^{\st m-1}_{\st j'=1}z_{\st i,j}$.
%
 \item generates polynomial ${\bm\mu}^{\st (j)}$, for every $j \notin L$, as follows:
  %
   ${\bm\mu}^{\st (j)} = {\bm\zeta}\cdot {\bm\xi}^{\st (j)}-\bm\tau^{\st (j)}$, where ${\bm\tau}^{\st (j)}=\sum\limits^{\st b'}_{\st i=0}z_{\st i,j}\cdot x^{\st i}$, and values $z_{\st i,j}$ were generated in step \ref{gen-pr-vals}.
%
\item sends the above ${\bm \zeta}$,  ${\bm\xi}^{\st (j)}$, and ${\bm\mu}^{\st (j)}$ to $\mathcal{A}_{\st R}$, for every $j\notin L$ and $1\leq j \leq m$. 
%
\item\label{adversary-outputs--} outputs whatever  $\mathcal{A}_{\st R}$ outputs. 
%
 \end{enumerate}
%
% \vspace{-2mm}
 
In the real model, the adversary receives two sets of messages, the first set includes the transcripts (including $ k,  g,  q$) it receives when it makes an ideal call to $f^{\st \zspa}$ and the second set includes pairs $({\bm \zeta},  {\bm\xi}^{\st (j)}, {\bm\mu}^{\st (j)})$, for every $j\notin  L$ and $1\leq j \leq m$. Since we are in the  $f^{\st \zspa}$-hybrid model and (based on our assumption) there is at least one honest party participated in  $\zspa$ (i.e., there are at most $m-1$ malicious participants of \zspa), the distribution of the messages it receives from $f^{\st \zspa}$ in the real and ideal models is identical. Furthermore, as we discussed in Case 1, (${\bm \zeta}, {\bm\xi}^{\st (j)}, {\bm\mu}^{\st (j)}$) in the real model and ($ {\bm \zeta}, {\bm\xi}^{\st (j)}, {\bm\mu}^{\st (j)}$) in the ideal model have identical distribution. The honest sender's output distribution in both models is identical, as the distribution of $f_{\st \ct}$'s output (i.e., $ k$) in both models is identical.



Now we show that the probability that the auditor aborts in the ideal and real models is statistically close. In the ideal model, $\mathsf{Sim}^{\st \zspaa}_{\st R}$ is given the ideal functionality's output that includes key $ k$. Therefore, it can check whether the key that $\mathcal{A}_{\st R}$ sends to it equals $ k$, i.e., $ k\stackrel{\st ?}=    k'_{\st j}$. Thus, it aborts with the probability $1$. However, in the real model, an honest auditor is not given the output of \ct (say key $k$) and it can only check whether the key is consistent with the hash value $q$ and the Merkle tree's root $g$ stored on the blockchain. This implied that the adversary can distinguish between the two models if, in the real model, it sends a key $\ddot k$, such that $\ddot k\neq k$, and still passes the checks. More precisely, it sends the invalid key $\ddot k$ that can generate  valid pair $(g, q)$, as follows: $\mathtt{H}(\ddot k)=q$ and $\mkgen(z'_{\scriptscriptstyle 0,1}, ..., z'_{\scriptscriptstyle b', m})\rightarrow  g$, where each $z'_{\scriptscriptstyle i,j}$ is derived from $\ddot k$ using the same technique described in step \ref{ZSPA-A-Case-2-generate-z} above. 

This means that the adversary breaks the second pre-image resistance property of  $\mathtt{H}$.  However, $\mathtt{H}$ is indeed the second-pre-image resistance and the probability that the adversary succeeds in finding the second pre-image is negligible in the security parameter, i.e., $\negl(\lambda)$ where $\lambda$ is the hash function's security parameter. Therefore, in the real model, the auditor aborts if an invalid key is provided with a probability $1-\negl(\lambda)$ which is statically close to the probability that $\mathsf{Sim}^{\st \zspaa}_{\st R}$ aborts in the same situation in the ideal model, i.e., $1-\negl(\lambda)$ vs $1$. 
 % 
Hence, the distribution of the joint outputs of the adversary, honest sender, and honest auditor in the real and ideal models is indistinguishable.
%%%%%%%%%%%
%\noindent\textbf{Case 3: Corrupt auditor.} In the real execution, the auditor's view is defined as follows: 
%%
%$$ \mathsf{View}_{\st \text{Aud}}^{\st \text{ZSPA-A}} \Big((\bm\zeta, \bm\xi^{\st (1)},...,\bm\xi^{\st (m)}), (\vv k,g,q)\Big)=\{r_{\st \text{Aud}}, \bm\zeta, \bm\xi^{\st (1)},...,\bm\xi^{\st (m)},  \vv k, g, q, \bot \}$$
%%
%where $\vv{k}=[k_{\st 1},..., k_{\st m}]$ and $r_{\st \text{Aud}}$ is the outcome of internal random coins of the sender. The simulator $\mathsf{Sim}^{\st \text{ZSPA}}_{\st \text{Aud}}$, which receives $({\bm\zeta}, {\bm\xi}^{\st (1)}, ..., {\bm\xi}^{\st (m)} )$, works as follows. 
%
%\begin{enumerate}
%%
%\item generates an empty view and appends to it coins $r'_{\st \text{Aud}}$ chosen uniformly at random and polynomials $({\bm\zeta}, {\bm\xi}^{\st (1)}, ..., {\bm\xi}^{\st (m)} )$. 
%%
%\item picks a random key, $ k\stackrel{\st\$}\leftarrow \{0,1\}^{\st \Lambda}$, and then constructs vector $\vv k'$ as follows: $\vv k'=[ k,...,  k]$, where $|\vv k'|=m$. It appends $\vv k'$ to the view. 
%%
%\item computes $ q$ as $\mathtt{H}( k)= q$. It computes $ g$ as $\mathtt{MT.genTree}(z_{\scriptscriptstyle 0,1}, ..., z_{\scriptscriptstyle b', m})\rightarrow  g$, where each $z_{\scriptscriptstyle i,j}$ is derived from $ k$ using the same technique described in step \ref{ZSPA-A::gen-z} of Figure \ref{fig:arbiter}. It appends $ g$, $ q$, and $\bot$ to the view. 
%%
%\end{enumerate}
%
%Now, we show that the two views are (computationally) indistinguishable. Both set of polynomials $\{\bm\zeta, \bm\xi^{\st (1)},..., $ $\bm\xi^{\st (m)} \}$ in the real model and $\{\bm\zeta, {\bm\xi}^{\st (1)}, ..., {\bm\xi}^{\st (m)}\}$ in the ideal model have identical distribution as the polynomials in the sets have been picked uniformly at random from $\mathbb{F}_{\st p}[x]$, by a semi-honest adversary. Moreover, since the real world semi-honest adversary samples its randomness according to the protocol's description, the random coins in both worlds (i.e., $r_{\st \text{Aud}}$ and $r'_{\st \text{Aud}}$) have identical distribution. Also, vector $\vv k$ in the real model has identical values, so does  $\vv k'$ in the ideal model. Moreover, the elements of $\vv k$ and $\vv k'$ have identical distribution as their elements have been picked uniformly at random from $\{0,1\}^{\st \Lambda}$. As we already discussed,   the evaluations of deterministic functions (namely Merkle tree, $\mathtt{H}$, and $\mathtt{PRF}$) on the uniformly random values $k$ and $k'$ have identical distributions as well; thus, $(g, q)$ in the real model and $( g,  q)$ in the ideal model have identical distribution component-wise. We conclude that the two views are indistinguishable.
%%%%%%%%%%%%%%%%
%
 \end{proof}










==> CCS-24/ZSPA-proof.tex <==
% !TEX root =main.tex



\section{Proof of \zspa}\label{sec::proof-of-zspa}


%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}
For the sake of simplicity, we will assume the sender, which generates the result, directly transmits the result to the remaining parties (i.e., receivers) rather than sending it to a smart contract. We first consider the case in which the sender is corrupt. 



\noindent\textbf{Case 1: Corrupt sender.}  Let $\mathsf{Sim}^{\st \zspa}_{\st S}$ be the simulator using a subroutine adversary, $\mathcal{A}_{\st S}$. $\mathsf{Sim}^{\st \zspa}_{\st S}$ operates as follows. 
%
\begin{enumerate}
%
\item simulates  \ct  and receives the output value $k$ from $f_{\st \ct}$, as we are in $f_{\st \ct}$-hybrid model.
%
\item sends $k$ to TTP and receives back from it $m$ pairs, where each pair is of the form $( g,  q)$. 
%
\item sends $ k$ to $\mathcal{A}_{\st S}$ and receives back from it $m$ pairs  where each pair is of the form $( g',  q')$. 
%
\item checks whether the following equations hold (for each pair): $ g= g' \hspace{2mm} \wedge  \hspace{2mm}  q= q'$. If the two equations do not hold, then it aborts (i.e., sends abort signal $\Lambda$ to the receiver) and proceeds to the next step.
%
\item outputs whatever $\mathcal{A}_{\st S}$ outputs.
%
 \end{enumerate}
 
 Initially, we focus on the adversary’s output. In the real model, the only messages that the adversary receives are those messages it receives as the result of the ideal call to $f_{\st \ct}$. These messages have an identical distribution to the distribution of the messages in the ideal model, as the \ct is secure. 
 
 Now, we move on to the receiver’s output. We will demonstrate that the output distributions of the honest receiver in the ideal and real models are computationally indistinguishable. In the real model,  each element of pair $(g, p)$ is the output of a deterministic function on the output of $f_{\st \ct}$. We know the output of $f_{\st \ct}$ in the real and ideal models have an identical distribution, and so do the evaluations of deterministic functions (i.e., Merkle tree, $\mathtt{H}$, and $\mathtt{PRF}$) on them, as long as these three functions' correctness hold. Therefore, each pair $(g,q)$ in the real model has an identical distribution to pair $(g,  q)$ in the ideal model.  For the same reasons, the honest receiver in the real model aborts with the same probability as  $\mathsf{Sim}^{\st \zspa}_{\st S}$ does in the ideal model.  
 
 We conclude that the distributions of the joint outputs of the adversary and honest receiver in the real and ideal models are computationally indistinguishable. 


\

\noindent\textbf{Case 2: Corrupt receiver.}   Let $\mathsf{Sim}^{\st \zspa}_{\st R}$ be the simulator that uses subroutine adversary $\mathcal{A}_{\st R}$. $\mathsf{Sim}^{\st \zspa}_{\st R}$ operates as follows. 

\begin{enumerate}
%
\item simulates   \ct  and receives the output value $ k$ from $f_{\st \ct}$.
%
\item sends $ k$ to TTP and receives back $m$ pairs of the form $( g,  q)$ from TTP. 
%
\item sends $( k,  g,  q)$ to $\mathcal{A}_{\st R}$ and outputs whatever  $\mathcal{A}_{\st R}$ outputs. 
%
 \end{enumerate}
 
 
In the real model, the adversary receives two sets of messages, the first set includes the transcripts (including $ k$) it receives when it makes an ideal call to $f_{\st \ct}$ and the second set includes pair $(g, q)$. As we already discussed above (because we are in the  $f_{\st \ct}$-hybrid model) the distributions of the messages it receives from $f_{\st \ct}$ in the real and ideal models are identical. Moreover, the distribution of $f_{\st \ct}$'s output (i.e., $\bar k$ and $k$) in both models is identical; therefore, the honest sender's output distribution in both models is identical. As we already discussed,  the evaluations of deterministic functions (i.e., Merkle tree, $\mathtt{H}$, and $\mathtt{PRF}$) on $f_{\st \ct}$'s outputs have an identical distribution. Therefore, each pair $(g, q)$ in the real model has an identical distribution to the pair $(g, q)$ in the ideal model.  

Hence, the distribution of the joint outputs of the adversary and honest receiver in the real and ideal models is indistinguishable.
%
\end{proof}

In addition to the security guarantee stated by Theorem \ref{theorem::ZSPA-comp-correctness} (which ensures computation correctness against malicious sender or receiver)  \zspa also provides  (a) privacy against the public, and (b)  non-refutability. In informal terms, privacy in this context implies that, with the contract's state (i.e., $g$ and  $q$), an external party cannot glean any information about any of the pseudorandom values,  $z_{\scriptscriptstyle j}$.  On the other hand, non-refutability signifies that if a party sends ``approved'', they cannot later deny knowledge of the values whose representations are stored in the contract. %Furthermore, indistinguishability means that every $z_{\scriptscriptstyle j}$ ($1\leq j \leq m$) should be indistinguishable from a truly random value. 


 \vspace{-2mm}
\begin{theorem}
If  $\mathtt{H}$ is preimage resistance, $\mathtt{PRF}$ is secure, the signature scheme used in the smart contract is secure (i.e., existentially unforgeable under chosen message attacks), and the blockchain is secure (i.e., offers persistence and liveness properties \cite{GarayKL15}) then \zspa offers (i) privacy against the public and (ii) non-refutability. 
\end{theorem}
 
 

\begin{proof}
We will initially focus on privacy. Since key $k$ for $\mathtt{PRF}$ has been uniformly and randomly selected, and $\mathtt{H}$ exhibits pre-image resistance, the probability that the adversary can find $k$ (given $g$ ), is negligible with respect to the security parameter, i.e., $\negl(\lambda)$. Furthermore, because $\mathtt{PRF}$ is secure (i.e., its outputs are indistinguishable from random values) and  $\mathtt{H}$ is pre-image resistance, given the Merkle tree's root $g$, the probability that the adversary can find a leaf node, which is the output of $\mathtt{PRF}$, is $\negl(\lambda)$ too. 



Now we move on the non-refutability. Due to the persistency property of the blockchain, when a transaction or message reaches a depth of more than $v$ in the blockchain of one honest player (where $v$ is a security parameter),  it will be included in the blockchain of every honest player with overwhelming probability, and it will be given a permanent position in the blockchain, making it highly unlikely to be modified.


Furthermore, thanks to the liveness property, all transactions originating from honest parties will eventually reach a depth of more than $v$ blocks in an honest player's blockchain. Consequently, the adversary cannot carry out a selective denial-of-service attack against honest account holders. Moreover, due to the security of the digital signature (i.e., existentially unforgeable under chosen message attacks), one cannot deny having sent the messages to the blockchain and smart contract.
\end{proof}
%%%%%%%%%%%

==> CCS-24/ZSPA-protocol.tex <==
% !TEX root =main.tex




\begin{figure}[ht]%[!htbp]
\setlength{\fboxsep}{1pt}
\begin{center}
    \begin{tcolorbox}[enhanced,width=3.3in, height=94mm,right=.5mm,
    drop fuzzy shadow southwest,
    colframe=black,colback=white]


\small{
\vspace{-2mm}
\begin{enumerate}[leftmargin=-.2mm]
\item[$\bullet$]    {Parties.} A set of clients $\{    A_{\st 1},...,  A_{\st m}\}$.
%
\item[$\bullet$]    {Input.}  $m$: the total number of participants, $adr$: an address of a deployed smart contract which maintains the clients' addresses and accepts messages only from them, and $b$: the total number of vectors. Let $b'=b-1$. 
%
\item[$\bullet$]   {Output.}  $k$: a secret key that generates $b$ vectors $[z_{\scriptscriptstyle 0,1},...,z_{\scriptscriptstyle 0,m}],...,[z_{\scriptscriptstyle b',1},...,z_{\scriptscriptstyle b',m}]$, $q$: hash of the key,  $g$: a Merkle tree's root, and a vector of (signed) messages. 


%, such that the sum of each vector's elements equals zero: $\sum\limits^{\scriptscriptstyle m}_{\scriptscriptstyle j=1}z_{\scriptscriptstyle i,j}=0$. 


\item {\textbf{Coin-tossing.} $\ct (in_{\st 1},..., in_{\st m})\rightarrow k$}. 

All participants run a coin-tossing protocol to agree on $\mathtt{PRF}$'s key, $k$.
\item\label{ZSPA:val-gen}  {\textbf{Encoding.} $\mathtt{Encode}(k, m)\rightarrow (g,q)$}.

 One of the parties takes the following steps:  
\begin{enumerate}%[leftmargin=1mm]

\item for every $i$ ($0\leq i \leq b'$), generates $m$ pseudorandom values: 
%
\vspace{-2mm}
%
 $$\forall j, 1\leq j \leq m-1: z_{\scriptscriptstyle i,j}=\mathtt{PRF}(k,i||j), \hspace{2mm} z_{\scriptscriptstyle i,m}=-\sum\limits^{\scriptscriptstyle m-1}_{\scriptscriptstyle j=1}z_{\scriptscriptstyle i,j}$$
 %
\vspace{-3mm}
\item   constructs a Merkel tree on top of all pseudorandom values,  $\mkgen(z_{\scriptscriptstyle 0,1},...,z_{\scriptscriptstyle b',m})\rightarrow g$. 

\item sends the tree's root: $g$,   and the key's hash: $q=\mathtt {H}(k)$ to $adr$. 

\end{enumerate}

\item\label{ZSPA:verify}{\textbf{Verification.} $\mathtt{Verify}(k, g, q, m, flag)\rightarrow (a, s)$}. 
%
Each party $A_{\st t}$ checks if, all $z_{\scriptscriptstyle i,j}$ values, the root $g$, and key's hash $q$ have been correctly generated, by retaking  step \ref{ZSPA:val-gen}. 
%
\begin{itemize}
\item If the checks pass, then it sets $a=1$ and
\begin{itemize}
\item if $flag=A$, where $A\in \{    A_{\st 1},...,  A_{\st m}\}$, then  it sets $s$ to a (signed) ``approved'' message, and sends $s$ to $adr$.
\item  if $flag= A$, where $A\notin \{    A_{\st 1},...,  A_{\st m}\}$, then it sets $s = \bot$. 
\end{itemize}
%it sets $a=1$,  sets $s$ to a signed ``approved'' message, and sends $s$ to $adr$. 
\item If the checks do not pass, it aborts by returning $a=0$ and $s = \bot$. 
\end{itemize}
%\item\label{ZSPA:verify}\textbf{Sending-approval.} $\mathtt{Approve}(a)\rightarrow s$.
%Each party  sets $s$ to a signed ``approved'' message if $a=1$, and sends $s$ to $adr$. Otherwise, it sets $s = \bot$ and aborts if $a=0$. 
%
 \end{enumerate}
}
 \end{tcolorbox}
\end{center}
\vspace{-3mm}
\caption{Zero-sum Pseudorandom Values Agreement (\zspa). Note, $flag$ lets an external auditor locally run the verification without having to send a message to the smart contract.} 
\label{fig:ZSPA}
\vspace{-4mm}
\end{figure}



==> CCS-24/ZSPA.tex <==
% !TEX root =main.tex


\vspace{-5mm}
\subsection{Zero-sum Pseudorandom Values Agreement Protocol (\zspa)}

\vspace{-.5mm}

 \zspa allows $m$ parties (the majority of which is potentially malicious) to efficiently agree on (a set of vectors, where each $i$-th vector has) $m$ pseudorandom values such that their sum equals zero. At a high level, the parties first sign a smart contract, register their addresses in it, and run a  coin-tossing protocol \ct to agree on a key: $k$.  Next, one of the parties generates $m-1$ pseudorandom values $z_{\scriptscriptstyle i, j}$ (where $1\leq j\leq m-1$) using key $k$ and $\mathtt{PRF}$. It sets the last value as the additive inverse of the sum of the values generated, i.e., $z_{\scriptscriptstyle i, m}=-\sum\limits^{\scriptscriptstyle m-1}_{\scriptscriptstyle j=1}z_{\scriptscriptstyle i, j}$ (similar to the XOR-based secret sharing \cite{Schneier0078909}). 
%
%Next, it commits to each value, where it uses $k_{\scriptscriptstyle 2}$ to generate the randomness of each commitment. 

Then, it constructs a Merkel tree on top of the pseudorandom values and stores only the tree's root $g$ and the key's hash value $q$ in the smart contract.  Then, each party (using the key)  checks if the values (on the contract) have been computed correctly; if so, it sends a (signed) ``approved'' message to the contract which only accepts messages from registered parties. Hence, the functionality that \zspa computes is: $f^{\st \zspa}\underbrace{(\bot,..., \bot)}_{\st m}\rightarrow \underbrace{((k, g, q),..., (k, g,q))}_{\st m}$, where $g$ is the root of the Markle tree built on the pseudorandom values $z_{\st i, j}$, $q$ is the hash value of the key used to generate the pseudorandom values, and $m\geq 2$. Figure \ref{fig:ZSPA} presents \zspa in detail.  



\zspa will be used in \withFai to let clients $\{A_{\st 1},...,A_{\st m}\}$ provably agree on sets of pseudorandom values. Every client uses the elements of these sets (as coefficients) to generate a distinct pseudorandom polynomial such that when all clients' pseudorandom polynomials are added it will result in $0$, due to \zspa's property.  Each of these polynomials will be used by a client to blind the messages it sends to the smart contract, to protect the privacy of the plaintext message (from \aud, D, and the public). To compute the sum of the plaintext messages, one can easily sum the blinded messages, which removes the blinding polynomials. 



%\zspa will be used in \withFai to let clients $\{A_{\st 1},...,A_{\st m}\}$ provably agree on sets of pseudorandom values, where each set represents a pseudorandom polynomial (as the set's elements are considered the polynomial's coefficients). Due to \zspa's property, the sum of these polynomials is zero.  Each of these polynomials will be used by a client to blind the messages it sends to the smart contract, to protect the privacy of the plaintext message (from \aud, D, and the public). To compute the sum of the plaintext messages, one can easily sum the blinded messages, which removes the blinding polynomials. 

\vspace{-3.5mm}
\input{ZSPA-protocol}

\vspace{-2mm}
\begin{theorem}\label{theorem::ZSPA-comp-correctness}
Let $f^{\st \zspa}$ be the functionality defined above. If \ct is secure against a malicious adversary and the correctness of $\mathtt{PRF}$, $\mathtt{H}$, and Merkle tree hold, then \zspa,  in Figure \ref{fig:ZSPA}, securely computes $f^{\st \zspa}$ in the presence of $m-1 $ malicious adversaries. 
\end{theorem}


We refer readers to Appendix \ref{sec::proof-of-zspa} for the proof of Theorem \ref{theorem::ZSPA-comp-correctness}. 


%Informally, there are four main security requirements that ZSPA must meet: (a) privacy, (b)  non-refutability, (c) indistinguishability, and (d) result correctness. Privacy here means given the state of the contract, an external party cannot learn any information about any of the (pseudorandom) values:  $z_{\scriptscriptstyle j}$; while non-refutability means that if a party sends ``approved" then in future cannot deny the knowledge of the values whose representation is stored in the contract. Furthermore, indistinguishability means that every $z_{\scriptscriptstyle j}$ ($1\leq j \leq m$) should be indistinguishable from a truly random value and result correctness means that a malicious result generator cannot convince other parties to accept an invalid final result, i.e., the root constructed on the invalid leaf node(s). In Figure \ref{fig:ZSPA}, we provide ZSPA that efficiently generates $b$ vectors where each vector elements is sum to zero. 






%\begin{figure}[ht]
%\setlength{\fboxsep}{0.7pt}
%\begin{center}
%\begin{boxedminipage}{12.3cm}

%
%\begin{figure}[ht]%[!htbp]
%\setlength{\fboxsep}{1pt}
%\begin{center}
%    \begin{tcolorbox}[enhanced,width=5.5in, 
%    drop fuzzy shadow southwest,
%    colframe=black,colback=white]
%
%
%\small{
%
%\begin{enumerate}
%\item[$\bullet$]  \textit{Parties.} $\{\resizeT {\textit A}_{\resizeS {\textit  1}},..., \resizeT {\textit A}_{\resizeS {\textit  m}}\}$
%\item[$\bullet$]  \textit{Input.}  $m$: the total number of participants and a deployed smart contract's address. 
%\item[$\bullet$] \textit{Output.}  $k$: a secret key that generates $b+1$ vectors $[z_{\scriptscriptstyle 0,1},...,z_{\scriptscriptstyle 1,m}],...,[z_{\scriptscriptstyle b,1},...,z_{\scriptscriptstyle b,m}]$ of pseudorandom values, $h$: hash of the key,  $g$: a Merkle tree's root, and a vector of signed messages. 
%
%
%%, such that the sum of each vector's elements equals zero: $\sum\limits^{\scriptscriptstyle m}_{\scriptscriptstyle j=1}z_{\scriptscriptstyle i,j}=0$. 
%
%
%\item All participants run a coin tossing protocol to agree on a key $k$  of $\mathtt{PRF}$.
%\item\label{ZSPA:val-gen} One of the parties:  
%\begin{enumerate}
%
%\item for every $i$ (where $0\leq i \leq b$), generates $m$ pseudorandom values as follows. 
%%
% $$\forall j, 1\leq j \leq m-1: z_{\scriptscriptstyle i,j}=\mathtt{PRF}(k,i||j), \hspace{5mm} z_{\scriptscriptstyle i,m}=-\sum\limits^{\scriptscriptstyle m-1}_{\scriptscriptstyle j=1}z_{\scriptscriptstyle i,j}$$
%%
%\item   constructs a Merkel tree on top of all pseudorandom values,  $\mathtt{MT.genTree}(z_{\scriptscriptstyle 0,1},...,z_{\scriptscriptstyle b,m})\rightarrow g$. 
%
%\item  sends the Merkel tree's root: $g$,   and the key's hash: $q=\mathtt {H}(k)$ to the smart contract. 
%
%\end{enumerate}
%
%\item\label{ZSPA:verify} The rest of parties (given $k_{\scriptscriptstyle 1}, k_{\scriptscriptstyle 2}$) check if, all $z_{\scriptscriptstyle i,j}$ values, the root $g$ and key's hash have been correctly generated (by redoing  step \ref{ZSPA:val-gen}). If the checks pass, each party sends a singed ``approved'' message to the  contract. Otherwise, it aborts. 
%
%
% \end{enumerate}
%}
% \end{tcolorbox}
%\end{center}
%\caption{Zero-sum Pseudorandom Values Agreement (ZSPA) Protocol} 
%\label{fig:ZSPA}
%\end{figure}
%




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}[ht]
%\setlength{\fboxsep}{0.7pt}
%\begin{center}
%\begin{boxedminipage}{12.3cm}
%
%\small{
%
%\begin{enumerate}
%\item[$\bullet$]  \textit{Parties:} $\{\resizeT {\textit A}_{\resizeS {\textit  1}},..., \resizeT {\textit A}_{\resizeS {\textit  m}}\}$
%\item[$\bullet$]  \textit{Public Parameters and Functions:} A pseudorandom function: $\mathtt{PRF}$, a deployed smart contract, and total number of participants: $m$. 
%\item[$\bullet$] \textit{Output}:  All parties agree on $b+1$ vectors $[z_{\scriptscriptstyle 0,1},...,z_{\scriptscriptstyle 1,m}],...,[z_{\scriptscriptstyle b,1},...,z_{\scriptscriptstyle b,m}]$, of pseudorandom values, such that the sum of each vector's elements equals zero: $\sum\limits^{\scriptscriptstyle m}_{\scriptscriptstyle j=1}z_{\scriptscriptstyle i,j}=0$
%
%
%\item All participants run a coin tossing protocol to agree on two keys $k_{\scriptscriptstyle 1}$ and $k_{\scriptscriptstyle 2}$ of $\mathtt{PRF}$.
%\item\label{ZSPA:val-gen} One of the parties:  
%\begin{enumerate}
%
%\item For every $i$, computes $m$ pseudorandom values: $\forall j, 1\leq j \leq m-1: z_{\scriptscriptstyle i,j}=\mathtt{PRF}(k_{\scriptscriptstyle 1},i||j)$ and sets $z_{\scriptscriptstyle i,m}=-\sum\limits^{\scriptscriptstyle m-1}_{\scriptscriptstyle j=1}z_{\scriptscriptstyle i,j}$, where $0\leq i \leq b$
%
%\item   commits to every $z_{\scriptscriptstyle i,j}$  as follows: $\mathtt{a}_{\scriptscriptstyle i,j}=\mathtt{Com}(z_{\scriptscriptstyle i,j}, q_{\scriptscriptstyle i,j})$, where the randomness of the commitment is computed as: $ q_{\scriptscriptstyle i,j}=\mathtt{PRF}(k_{\scriptscriptstyle 2},i||j)$ and  $1\leq j \leq m$.
%
%\item   constructs a Merkel tree on top of the committed values: $\mathtt{MT}(\mathtt{a}_{\scriptscriptstyle 0,1},...,\mathtt{a}_{\scriptscriptstyle b,m})\rightarrow g$ 
%
%\item  sends the Merkel tree's root: $g$,   and the keys' hashes: $\mathtt {H}(k_{\scriptscriptstyle 1})$ and $ \mathtt {H}(k_{\scriptscriptstyle 2})$, to the contract. 
%
%\end{enumerate}
%
%\item\label{ZSPA:verify} The rest of parties (given $k_{\scriptscriptstyle 1}, k_{\scriptscriptstyle 2}$) check if, all $z_{\scriptscriptstyle i,j}$ values, the root $g$ and keys' hashes have been correctly generated (by redoing  step \ref{ZSPA:val-gen}). If passed, each party sends a singed ``approved'' message to the  contract. Otherwise, it aborts. 
%
%
% \end{enumerate}
%}
%\end{boxedminipage}
%\end{center}
%\caption{Zero-sum Pseudorandom Values Agreement ($\mathtt{ZSPA}$) Protocol} 
%\label{fig:ZSPA}
%\end{figure}




==> CCS-24/anesidora-further-discussion.tex <==
% !TEX root =main.tex


%%%%%%%%%%%%%%%%%

\section{Further Discussion on \withRew}\label{sec::Discussion-Anesidora}


\subsection{Application to Vertical Federated Learning}\label{sec:Application-to-VFL}

Federated Learning (FL) is a machine learning framework where multiple parties collaboratively build machine learning models without revealing their sensitive input data to their counterparts \cite{YangLCT19,McMahanMRA16}. FL can be categorized into three classes, based on how data is partitioned. 

Vertical Federated Learning (VFL) is one of the primary classes that has found applications in dealing with crime \cite{abs-2310-04546}, developing financial risk models \cite{ChengLCY20}, or healthcare \cite{NguyenPPDSLDH23}. VFL refers to the FL setting
where datasets distributed among different parties share the same samples while holding different features. 

For different parties to identify the common samples (or rows), often VFL schemes use PSIs, before they start developing a global model \cite{YangLCT19}.  
Nevertheless, similar to the MPC schemes, VFL schemes assume that parties contribute their private inputs free of charge.  The development of an incentivization mechanism for (V)FL has been identified as an open research question  \cite{KairouzMABBBBCC21}. 

This mechanism gains particular relevance in scenarios where participants may simultaneously function as business rivals. In such cases, each participant may harbor concerns that sharing their private data for training FL models could inadvertently benefit their competitors, particularly the party interested in and receiving the final result.

Moreover, parties engaging in the FL procedure must contend with a substantial overhead that may act as a deterrent to their participation.

\withRew emerges as a potential solution to the aforementioned research question, offering the capacity to supplant the current PSIs employed in VFL schemes. In this framework, \withRew assumes a pivotal role in motivating diverse parties to share their private inputs, thereby nurturing collaboration in the creation of global models. This ensures that participants receive fair compensation for their contributions. The fundamental concept is to establish a system where collaborative machine learning efforts are not only secure through privacy-preserving measures but are also actively incentivized, fostering increased involvement and participation.


\subsection{Strawman Approach}


There is a simpler but more expensive approach to finding the intersection without the participation of the extractors. In this approach, the smart contract identifies the (encoded) elements of the intersection and distributes the parties' deposits based on the number of elements it discovers. While this method is simpler, as it eliminates the need for both (i) the involvement of the extractors and (ii) the three counter-collusion contracts, it comes at a higher cost.

This increased cost arises because the contract itself must factorize the unblinded resulting polynomial and locate the roots, incurring an $O(d^{\st 2})$ computational cost for each bin, where $d$ is the size of each bin. In contrast, our proposed approach offloads such computations off-chain, resulting in a lower monetary computation cost.

%\end{remark}


 
\subsection{Encrypting Set Elements}
In \epsi, each party initially encrypts its set elements (using deterministic encryption) to preserve the privacy of the elements from non-participants of the protocol, e.g., the public. This allows extractors to prove to the (public) smart contract $\SCe$ that they have already committed to the encryption of the elements in the intersection without revealing the actual plaintext elements. 


 
\subsection{The Use of the Hash-based Padding}
The reason each client uses the hash-based padding to encode each encrypted element $e_{\st i}$  as $\bar{e}_{\st i} =e_{\st i} || \mathtt{H}(e_{\st i})$ is to allow the auditor in the counter collusion contracts to find the error-free intersection, without having to access to one of the original (encrypted) sets. 



 
\subsection{Extracting the Elements in the Intersection}\label{sec::Extracting-Elements-in-Intersection}
Compared to \fpsi, there is a minor difference in finding the result in \epsi. Specifically, because in \epsi each set element  $s_{\st i}$ is encoded as  (i) $e_{\st i}=\mathtt{PRP}(mk', s_{\st i})$ and then (ii) $\bar{e}_{\st i} =e_{\st i} || \mathtt{H}(e_{\st i})$ by a client, then when the client wants to find the intersection it needs to first regenerate $\bar{e}_{\st i}$ as above and then treat it as a set element to check if  $\bm\phi'(\bar e_{\st i})=0$, in step \ref{F-PSI::find-intersection} of \fpsi. 

%
%\end{remark}


%\begin{remark}
%The protocol requires  extractor clients  to commit to their encrypted set elements \emph{before} \epsi starts, to prevent the clients to find some random roots introduced in the result and sell them to the buyer. Furthermore, instead of the extractor's commitment scheme we proposed, one could  use polynomial commitment scheme \cite{Kate-poly-commit}. However, our scheme (tailored for our Smart PSI) is more efficient, as it is based on efficient symmetric key primitives; whereas, \cite{Kate-poly-commit} requires expensive public key and bilinear pairing operations. 
%\end{remark}

%\begin{remark}
%The Traitor's contract must be signed between the dealer and the extractor client who betrays the other colluding extractor or buyer  before step \ref{extractor-proves}. Also, the dealer pays the refundable deposits in the Traitor's contract. 
%
%\end{remark}




%\begin{remark}
%For ease of exposition, $\mathtt{ZSPA}$ protocol (in Fig \ref{fig:ZSPA}) was presented for single bin. However, it can easily be extended to multiple bins (using only two keys: $k_{\st 1}, k_{\st 2}$). To do so, for each bin $l$ (in step \ref{ZSPA:val-gen}) each blinding factor is computed as  $z_{\st i,j,l}=\mathtt{PRF}(k_{\st 1},i||j||l)$ and  the randomness of the commitment  is generated as: $ q_{\st i,j,l}=\mathtt{PRF}(k_{\st 2},i||j||l)$. Also, a Merkel tree is built on top of all bins' committed values that yields single root. 
%\end{remark}

%\begin{remark}
%Recall, when $Flag=False$, each honest party receives the total amount of $\frac{m'\cdot \yc'-\chc}{m-m'}$ amount from $\mathcal{SC}_{\fpsi}$ as compensation and reward.  
%\end{remark}


%\begin{remark} 

\subsection{The Use of Double-layered Commitments}
In \epsi, each extractor employs double-layered commitments, which involve initially committing to the encryption of each element and subsequently constructing a Merkle tree on top of all these commitments. This approach is adopted for efficiency and privacy reasons.


Constructing a Merkle tree on top of the commitments enables the extractor to store just a single value in $\SCe$  resulting in significantly lower storage costs compared to the alternative scenario where all commitments would need to be stored in $\SCe$. Additionally, committing to the encryption of the elements allows the extractor to conceal from other clients the encryption of those elements that do not belong to the intersection. It is important to note that simply encrypting each element would not suffice to protect one client's elements from the other clients, as they all possess knowledge of the decryption key.





\subsection{Inserting Garbage Inputs}

To potentially increase their reward, malicious clients might be tempted to insert ``garbage'' elements into their sets,  hoping that these spurious elements will appear in the result, thus yielding a greater reward. However, their efforts would be in vain as long as a semi-honest client (such as dealer $D$) includes genuine set elements. In this scenario, according to the set intersection definition, those garbage elements will not be part of the intersection.




\subsection{Using Generic Reward Function}
In \epsi, for the sake of simplicity, we allowed each party to receive a fixed reward, i.e., $\lc$, for every element it contributes to the intersection. It is possible to make the process more flexible/generic. For instance, we could define a Reward Function $RF$ that takes $\lc$, an (encoded) set element $e_{\st i}$ in the intersection, its distribution/value $val_{\st e_{\st i}}$, and output a reward $rew_{\st e_{\st i}}$ that each party should receive for contributing that element to the intersection, i.e., $RF(\lc, e_{\st i}, val_{\st e_{\st i}})\rightarrow rew_{\st e_{\st i}}$.





 

==> CCS-24/auditor-res-Comp.tex <==
% !TEX root =main.tex


%\vspace{-2mm}
\begin{figure}[ht]
\setlength{\fboxsep}{1pt}
\begin{center}
    \begin{tcolorbox}[enhanced, 
    drop fuzzy shadow southwest,
    colframe=black,colback=white]
   % {\small{
    %\vspace{-2.5mm}
 \underline{$\mathtt{resComp}(\bm\zeta, \bm\phi, sk, ct_{\st mk}, indx, {des}_{\st \mathtt{H}})\rightarrow R$}\\
%
%\vspace{-2.2mm}
\begin{itemize}[leftmargin=.6mm]
%
\item \noindent\textit{Input}. $\bm\zeta$: a random polynomial of degree $1$, $\bm\phi$: a blinded polynomial of the form $\bm\zeta\cdot(\bm\epsilon + \bm\gamma')$ where $\bm\epsilon$ and $\bm\gamma'$ are arbitrary and  pseudorandom polynomials respectively, $deg(\bm\phi)-1=deg(\bm\gamma')$, $sk$: the auditor's secret key, $ct_{\st mk}$: ciphertext of $mk$ which is a  key of $\mathtt{PRF}$, $indx$: an input of $\mathtt{PRF}$, and   ${des}_{\st \mathtt{H}}$: a description of hash function $\mathtt{H}$.
%
\item\noindent\textit{Output}. $R$: a set containing valid roots of unblinded $\bm\phi$. 
%
\end{itemize}
%
\begin{enumerate}[leftmargin=.5mm]
%
\item decrypts the ciphertext $ct_{\st mk}$ under key $sk$. Let $mk$ be the result. 
%
\item unblinds polynomial $\bm\phi$, as follows:
%
\begin{enumerate}
%
\item re-generates pseudorandom polynomial $\bm\gamma'$ using key $mk$. Specifically, it uses $mk$ to derive a key: $k=\mathtt{PRF}(mk,  indx)$. Then, it uses the derived key to generate $3d+1$ pseudorandom coefficients, i.e.,  $ \forall j, 0\leq j \leq deg(\bm\phi)-1: g_{\st j}=\mathtt{PRF}(k, j)$. Next, it uses these coefficients to construct polynomial $\bm\gamma'$, i.e., $\bm\gamma'=\sum\limits_{\st j=0}^{\st deg(\bm\phi)-1} g_{\st j}\cdot x^{\st j}$.
%
\item removes the blinding factor from $\bm\phi$. Specifically, it computes polynomial $\bm\phi'$ of the following form $\bm\phi'= \bm\phi - \bm\zeta\cdot\bm\gamma'$. 
%
\end{enumerate}
%
\item extracts roots of polynomial $\bm\phi'$. 
\item finds valid roots, by (i) parsing each root $\bar{e}$ as $(e_{\st 1}, e_{\st 2})$ with the assistance of $des_{\st \mathtt{H}}$  and (ii) checking if $e_{\st 2}=\mathtt{H}(e_{\st 1})$. It considers a root valid if this equation holds. 
%
\item returns set $R$ containing all valid roots.
%

%\vspace{-1mm}
\end{enumerate}
%}   }
\end{tcolorbox}
\end{center}
\vspace{-4mm}
\caption{Auditor's result computation, $\mathtt{resComp}(.)$, algorithm} 
\label{fig::resComp}
 \vspace{-4mm}
\end{figure}

==> CCS-24/blank.tex <==
% !TEX root =main.tex



==> CCS-24/coin-tossing.tex <==
% !TEX root =main.tex





\section{Coin-Tossing Protocol}\label{sec::coin-tossing}

A Coin-Tossing protocol, \ct, allows two mutually distrustful parties, say $A$ and $B$, to jointly generate a single random bit. Formally, \ct computes the functionality $\fct(in_{\st A}, in_{\st B})\rightarrow (out_{\st A}, out_{\st B})$, which takes $in_{\st A}$ and  $in_{\st B}$ as inputs of $A$ and $B$ respectively and outputs $out_{\st A}$ to $A$ and $out_{\st B}$ to $B$, where $out_{\st A}=out_{\st B}$. A basic security requirement of a \ct is that the resulting bit is (computationally) indistinguishable from a truly random bit. 

Blum proposed a simple \ct in \cite{Blum82} that works as follows. Party $A$ picks a random bit $in_{\st A}\stackrel{\st \$}\leftarrow\{0,1\}$, commits to it and sends the commitment to $B$ which sends its choice of random input, $in_{\st B}\stackrel{\st \$}\leftarrow\{0,1\}$, to $A$. Then, $A$ sends the opening of the commitment (including $in_{\st A}$) to $B$, which checks whether the commitment matches its opening. If so, each party computes the final random bit as $in_{\st A}\oplus in_{\st B}$.  

There have also been \emph{fair} coin-tossing protocols, e.g., in \cite{MoranNS09}, that ensure either both parties learn the result or nobody does. These protocols can be generalized to \emph{multi-party} coin-tossing protocols to generate a \emph{random string} (rather than a single bit), e.g., see \cite{BeimelOO10,KiayiasRDO17}.
%
The overall computation and communication complexities of (fair) multi-party coin-tossing protocols are often linear with the number of participants. In this paper, any secure multi-party \ct that generates a random string can be used. For the sake of simplicity, we let a multi-party \fct take $m$ inputs and output a single value, i.e., $\fct(in_{\st 1}, ..., in_{\st m})\rightarrow out$. 





==> CCS-24/commitment.tex <==
% !TEX root =main.tex




\section{Commitment Scheme}\label{subsec:commit}


 A commitment scheme involves a  \emph{sender} and a \emph{receiver}. It also  involves  two phases; namely, \emph{commit} and  \emph{open}. In the commit phase, the sender  commits to a message: $x$ as $\comcom(x,r)=com$, that involves a secret value: $r\stackrel{\st\$}\leftarrow \{0,1\}^{\st\lambda}$. At the end of the commit phase,  the commitment ${com}$ is sent to the receiver. In the open phase, the sender sends the opening $\hat{x}:=(x, r)$ to the receiver who verifies its correctness: $\comver({com},\hat{x})\stackrel{\st ?}=1$ and accepts if the output is $1$.  
 
 A commitment scheme must satisfy two properties: (a) \textit{hiding}: it is infeasible for an adversary (i.e., the receiver) to learn any information about the committed message $x$, until the commitment ${com}$ is opened, and (b) \textit{binding}: it is infeasible for an adversary (i.e., the sender) to open a commitment ${com}$ to different values $\hat{x}':=(x',r')$ than that was used in the commit phase, i.e., infeasible to find  $\hat{x}'$, \textit{s.t.} $\comver({com},\hat{x})=\comver({com},\hat{x}')=1$, where $\hat{x}\neq \hat{x}'$.  
 
 There exist efficient commitment schemes both in (a) the standard model, e.g., Pedersen scheme \cite{Pedersen91}, and (b)  the random oracle model using the well-known hash-based scheme such that committing  is : $\mathtt{H}(x||r)={com}$ and $\comver({com},\hat{x})$ requires checking: $\mathtt{H}(x||r)\stackrel{\st ?}={com}$, where $\mathtt{H}:\{0,1\}^{\st *}\rightarrow \{0,1\}^{\st\lambda}$ is a collision-resistant hash function, i.e., the probability to find $x$ and $x'$ such that $\mathtt{H}(x)=\mathtt{H}(x')$ is negligible in the security parameter $\lambda$.

==> CCS-24/complexity.tex <==
% !TEX root =U-PSI.tex
\section{Complexity Analysis}
\vspace{-2mm}
\subsection{Computation Complexity} \label{compcomp}

We first analyse the computation cost of U-PSI when the clients delegate PSI to the cloud. In our analysis, we do not count the pseudorandom function invocation cost, as it is a fast operation, and dominated by the other operations (e.g. modular arithmetic, shuffling and factorization). In step d.\ref{shuffleB}, client $B$ executes $h$ modular additions, and  shuffles a vector of $h$ elements with a cost of $O(c)$. Also, it performs  $nh$ modular additions in each of steps d.\ref{blindshuffleB} and f.\ref{unblind} to  blind and unblind  the hash table elements,  respectively. In step f.\ref{interpolate} it interpolates $h$ polynomials with each interpolation costing $O(d)$, where $d$ is a constant value. In step f.\ref{factorize}, it factorizes $h$ polynomials with each factorization costing $O(d^{\scriptscriptstyle 2})$. So in total client $B$'s computation cost is $(4+5d+d^{\scriptscriptstyle 2})h$ which is $O(c)$. Client $A$ in step  d.\ref{RegenKeys}  shuffles a vector of $h$ elements that costs $O(h)$ and in  step d.\ref{cleintAshuffles} it does $h$ modular additions, and shuffles a vector of $h$ elements. In step d.\ref{shuffleA}, it performs $2hnd$ modular multiplications and $2hnd$ modular additions to evaluate the pseudorandom polynomials. In the same step, to generate vectors $\vv{\bm{v}}^{\scriptscriptstyle (A)}$ and $\vv{\bm{v}}^{\scriptscriptstyle (B)}$, it performs $2nh$ modular multiplications. In step d.\ref{vectorq}, it permutes two vectors of  $h$ elements and carries out $2nh$ modular additions to generate  vectors $\vv{\bm{q}_{\scriptscriptstyle e}}$. Thus, in total it performs $(9+12d+8d^{\scriptscriptstyle 2})h$ or $O(c)$ modular operations. The cloud in step e.\ref{cloudcomp} performs  $2hnd$ modular multiplications and $2hnd$ modular additions to evaluate the pseudorandom polynomials. In the same step, it performs $2nh$ modular multiplications and $3nh$ modular additions to generate the vectors $\vv{\bm{t}_{\scriptscriptstyle e}}$. Thus, in total the cloud's computation involves $(5+14d+8d^{\scriptscriptstyle 2})h$ or  $O(c)$ modular operations. 
%In our multi-client protocol, the  computation complexity for those clients who authorise the computation,  is similar  to the  two-client protocol's, also the complexity for the cloud and result recipient would be $O(c\textsl{m-2c} )$, where $\textsl{m}$ is the total number of clients. 

In the update phase, each client  carries out $2d+2$ modular additions in step c.\ref{unblindupdate}. It interpolates a polynomial in step c.\ref{interpolateupdate} which costs $O(d)$.  In step c.\ref{InsertionDeletion}, it executes $d$ modular additions and $d$ modular multiplications to evaluate the polynomial at the single value $s$. In the same step, when the update is element insertion, the client extracts a bin's set elements that costs $O(d^{\scriptscriptstyle 2})$, and carries out $nd$ modular multiplications and $nd$ modular additions to evaluate the polynomial. So, the total computation cost for insertion is $5d(1+d)$, or $O(1)$ as $d$ is constant. If the update is element deletion, the client performs $2n$ modular additions to evaluate the two polynomials and $2n$ modular multiplications to generate  pseudorandom values. Finally, in step c.\ref{freshfactors}, the client performs $n+1$ modular additions. Therefore, the client's total computation cost for deletion is $6d+4$ or $O(1)$. 

In \cite{opsi15,DBLP:conf/fc/AbadiTD16,yang2018improved} set elements are represented as a single polynomial whose degree is linear to the set cardinality, $c$. In these protocols, the cost  of computing PSI is dominated by public key encryption operations, with complexity $O(c)$, and  polynomial factorization, with complexity $O(c^{\scriptscriptstyle 2})$. To insert/delete an element in  \cite{opsi15,yang2018improved}, a client needs to encode the element to be inserted/deleted as a polynomial, evaluate the polynomial on $2c+1$ elements and perform $2c+1$ modular multiplications, to blind the evaluated values. Also, the cloud needs to perform the same number of multiplications to apply the update. Therefore, the protocols' update complexity is $O(c)$. However, in \cite{DBLP:conf/fc/AbadiTD16} due to the way each outsourced value is blinded, the client has to download the entire date, remove the blinding factors and apply the change locally that also costs it $O(c)$. The protocol in \cite{eopsi} uses a hash table and encodes  set elements into a set of polynomials of constant degree, and this leads to $O(c)$ for computing PSI. In this protocol, if a client naively updates only one bin, then the cloud would be able to learn which elements have been updated with a non-negligible probability. The reason is that the bins are in their original order, and each bin's address is the hash value of an element in the bin, so if the client retrieves one bin, then the cloud would be able to figure out  what element is being updated  with a non-negligible probability when the set universe is not big. So, for the client to securely update its data, it has to re-encode the entire outsourced data that costs $O(c)$ too. 

Thus, the PSI computation cost in \cite{opsi15,DBLP:conf/fc/AbadiTD16,yang2018improved} is $O(c^{\scriptscriptstyle 2})$ while in our protocol and in \cite{eopsi} it is  $O(c)$. Moreover, update phase has $O(c)$ complexity in  \cite{opsi15,DBLP:conf/fc/AbadiTD16,yang2018improved,eopsi} while it has  much less cost, i.e. $O(1)$, in our protocol. 

\vspace{-3mm}

\subsection{Communication Complexity} \label{commcomp}

In U-PSI for PSI delegation client $B$, in step d.\ref{whatBSends}, sends a single value $tk^{\scriptscriptstyle (B)}$ to the cloud. In this step, it sends two  values, $pk^{\scriptscriptstyle (B)}$ and $lk^{\scriptscriptstyle (B)}$, and vector $\vv{\bm{r}}^{\scriptscriptstyle (B)}$ of $h$ bins to client $A$. Therefore, client $B$'s communication cost is $h(2d+1)+3$ or $O(c)$. In step d.\ref{WhatclientAsends}, client $A$ sends $tk^{\scriptscriptstyle (A)}$ and vector $\pi(pk^{\scriptscriptstyle (A)},\vv{\bm{m}}_{\scriptscriptstyle A \rightarrow B})$ containing $2h$ elements to the cloud. In the same step, it sends vector $\vv{\bm{q}}$ containing $h$ bins to client $B$. So, client $A$'s total communication cost  is $h(3+2d)+1$ or $O(c)$. The cloud's communication cost is $h(2d+1)$ or $O(c)$, as in step e.\ref{EO-cloudRes}, it sends vector $\vv{\bm{t}}$ of $h$ bins to client $B$. 
%Moreover, in our multi-client protocol, the communication cost of the cloud and the clients who authorize the computation remains the same as that of in two-client case, i.e. $O(c)$, but the result recipient' communication cost is $O(c\textsl{m}-c )$. 
To update its outsourced set a client sends to the cloud two labels, one in each of steps c.\ref{firstupdatestep} and c.\ref{lastupdatestep}. Moreover, it sends a vector of $2d+1$ elements in step c.\ref{lastupdatestep}. So, in total its communication cost is $3+2d$ or $O(1)$. Also, the cloud in step c.\ref{firstupdatestep} sends a vector of $2d+1$ elements to the client. Therefore,  the cloud's communication cost is $2d+1$ or $O(1)$. Note that  every message in our protocol is a random element of a finite field.

% Note that in our scheme for a fixed probability of overflow and fixed bin maximum load, the hash table length $h$ is linear to the set cardinality $c=\frac{c'}{m}$ (see section \ref{balls-bins}). 

%The reason is that if we rewrite $d=(1+\sigma)\cdot \frac{c}{h}$ (presented in subsection \ref{balls-bins}) we would have $h=(1+\sigma)\cdot \frac{c}{d}$.  

Both the PSI computation and update phases in the protocols in \cite{opsi15,yang2018improved,DBLP:conf/fc/AbadiTD16} have  $O(c)$ communication complexity.  Note that each message in these protocols for PSI computation is a ciphertext of a public key encryption and its size is  much larger  than the size of a field element, but the messages sent for an update is a field element. The protocol in \cite{eopsi} has $O(c)$ communication complexity for PSI computation, and as a client needs to re-encode the entire dataset to securely update it, it requires sending $h(2d+1)$, or $O(c)$ elements of a finite field.  

%As we stated earlier in section \ref{U-PSIdiscussion}, in O-PSI protocol, in order for a client to  update the data it needs to download them,  update locally, and upload them to the cloud, so its update cost is $O(c)$. Also, in EO-PSI, if  client  simply updates one bin it would leak non-negligible information about  set elements to the cloud (see section \ref{U-PSIdiscussion} for discussion). So,  in EO-PSI, the  secure way for the client to update the outsourced dataset is to retrieve the entire dataset and update it locally and send it back to the cloud.  However, such approach imposes $O(hd)$ communication cost. On the other hand, the protocol in \cite{Lopez-Alt12} that utilizes FHE can support data update  by using the FHE's capabilities. But, the protocol is designed for generic computation and the complexity of update in delegated PSI has not been defined. Note that each message in EO-PSI and U-PSI protocols is a random element of a   field (e.g. $p$ is about $112$ bits), whereas the messages in the other two protocols are ciphertexts of public key encryption that operate in a much larger group/ring. 

Hence,  our protocol and those in \cite{opsi15,DBLP:conf/fc/AbadiTD16,yang2018improved} have $O(c)$ communication complexity for PSI computation, but for updates only in U-PSI the client can securely update its dataset with $O(1)$ communication cost, while this cost is $O(c)$  for the other three protocols.

==> CCS-24/conclusion.tex <==
% !TEX root =main.tex

\vspace{-2mm}
\section{Conclusion and Future Direction}\label{sec::concl}
\vspace{-.5mm}

PSI is a crucial protocol with numerous applications. In this work, we proposed, \withFai, the first multi-party fair PSI that ensures that either all parties get the result or if the protocol aborts in an unfair manner, then honest parties will receive financial compensation. We then upgraded it to \withRew, the first PSI ensuring that honest parties who contribute their private sets receive a reward proportionate to the number of elements they reveal. 
%
Since an MPC that rewards participants for contributing their private inputs will help increase its real-world adoption, an interesting open question is: \emph{How can we generalize the idea of rewarding participants to MPC?}


==> CCS-24/content.tex <==
% !TEX root =main.tex




\vspace{-2mm}


\section{Introduction}

Secure Multi-Party Computation (MPC) is a general-purpose cryptographic protocol that enables multiple mutually distrustful parties to collectively compute a certain functionality on their private inputs, safeguarding their inputs' privacy, beyond the result. Private Set Intersection (PSI) is a cub-class of MPC, that allows parties to compute the intersection of their private sets. It aims to efficiently attain the same security as MPC.


Two facts about PSIs exist: (i) a non-empty result always reveals something about the parties' private input sets (i.e., the set elements that are in the intersection), and (ii) various variants of PSIs do not output the result to all parties, even in those PSIs that do,  not all of the parties are necessarily interested in it.  Given these facts, a natural question arises:   
%
\emph{How can we incentivize parties that do not receive the result or do not express interest in it to participate in a PSI?}



To date, the literature has not addressed the aforementioned question. It has assumed that all parties would engage in a PSI free of charge, resulting in them bearing the privacy burden (in addition to the costs associated with the PSI).\footnote{Combining a multi-party PSI with a payment mechanism that charges a fixed amount to the initiating buyer presents serious issues. Firstly, this approach compels the buyer to pay, even if malicious clients tamper with result accuracy, enabling them to gain knowledge without the buyer learning the correct result, as there exists no fair multi-party PSI in the literature. Secondly, it enforces a fixed fee irrespective of the intersection size. Overcharging dissuades buyers from participation while undercharging discourages other clients from engaging in the protocol. This highlights the need for a more equitable and flexible payment model in such scenarios.}




In this work, we provide the first-ever answer to the above question. We present a multi-party PSI, called ``\withRew'', which enables the buyer who initiates the PSI computation (and has an interest in the result) to pay other parties proportionally based on the number of elements it learns about other parties' private inputs.  
%
\withRew is efficient and predominantly \emph{relies on symmetric key primitives}.  Its computation and communication complexities scale linearly with the number of parties and set cardinality. \withRew maintains security even in scenarios where the majority of parties are compromised by malicious adversaries who may collude.




We construct \withRew in a modular manner. Specifically, we introduce the formal concept of ``PSI with Fair Compensation'' (\p) and devise  ``\withFai'' which realizes this concept. 
%
 \p guarantees that either all parties obtain the result, or in the event of an unfair protocol abortion (where only dishonest parties gain access to the result), honest parties will receive financial compensation. \withFai stands as \textit{the inaugural} fair multi-party PSI.
 
 

Subsequently, we advance from the \p to the ``PSI with Fair Compensation and Reward'' (\ep) notion and develop \withRew to actualize \ep. The latter notion guarantees that honest parties (a) receive rewards irrespective of the honesty of all parties or if a subset aborts unfairly, and (b) are compensated in the case of an unfair termination. We prove the two PSIs using the simulation-based model. In pursuit of efficient PSIs, we introduce a novel primitive, called unforgeable polynomials, which may independently pique interest. 

During the development of  \withFai and \withRew we had to tackle several challenges, including (i) minimizing overhead, (ii) safeguarding against collusion among malicious parties to prevent unfair payment, (iii) ensuring the transfer of the \textit{intact} output from one subroutine as input to another, (iv) providing clients with rewards commensurate with the intersection size, and (v) maintaining the confidentiality of outgoing messages.





\withRew, supporting multiple parties and rewarding them, can offer opportunities for richer analytics, and incentivize participation.  It can be used in various scenarios: (1) by Vertical Federate Learning schemes \cite{YangLCT19} that use PSIs (e.g., for identity alignment), (2) by banks, like ``WeBank'' \cite{ChengLCY20},  that rely on  Federated Learning and PSI to gather customer data from partners to enhance loan risk management,  (3) by advertisers targeting specific customers by identifying shared shopping patterns across different e-commerce databases \cite{IonKNPSS0SY20}, or (4) by a malware detection service querying multiple antivirus databases to identify applications as malware \cite{TamrakarLPEPA17}. In these cases, set contributors will receive rewards via \withRew (to explore incentivization mechanisms' benefits for VFL, see Appendix \ref{sec:Application-to-VFL} and  \cite[p. 15]{KairouzMABBBBCC21}). 
%
We also hope that our work serves as a catalyst for future research in (a) developing reward mechanisms for participants in \textit{generic} MPC, enhancing MPC's real-world adoption, and (b) bridging between ``data market'' \cite{golob2023decentralized,KochKMMR22,abs-2210-08723} and MPC  domains. %Furthermore, PSI has been widely used in Federated Learning \cite{}. 





%
{\noindent\textbf{Summary of Our Contributions.}} In this work, we: (1) introduce \withRew, a \textit{novel} multi-party PSI that incentivizes participants to contribute their set elements to the intersection, (2) introduce \withFai, which is the first fair multi-party PSI, (3) provide formal definitions and proofs for the above constructions within the simulation-based model, and (4) introduce unforgeable polynomials' concept. 
%









\input{Notations-Preliminaries.tex}





%\input{Priliminary}




\input{security-definition}
\input{Fair-PSI}


\input{smart-PSI-protocol}
\input{related-work}
\input{evaluation}

%\input{Related-work}















==> CCS-24/counter-collusion-contracts.tex <==
% !TEX root =main.tex


\section{Counter Collusion Contracts}\label{appendix::Counter-Collusion-Contracts}

In this section, we  present descriptions of the Prisoner’s Contract (\SCpc), Colluder’s Contract (\SCcc), and Traitor’s Contract (\SCtc) originally introduced by Dong \textit{et al.} \cite{dong2017betrayal}. As mentioned earlier, we have made slight adjustments to these contracts. We will mark these modifications in blue. To ensure a comprehensive understanding, below we reiterate the parameters utilized in these contracts.




\begin{itemize}
\item[$\bullet$] $\bc$: the bribe paid by the ringleader of the collusion to the other
server in the collusion agreement, in \SCcc.
%
\item[$\bullet$] $\cc$: a server’s cost for computing the task.
%
\item[$\bullet$] $\chc$: the fee paid to invoke an auditor for recomputing a task and resolving
disputes.
%
\item[$\bullet$] $\dc$: the deposit a server needs to pay to be eligible for getting the job.
%
\item[$\bullet$] $\tc$: the deposit the colluding parties need to pay in the collusion agreement, in \SCcc.
%
\item[$\bullet$] $\wc$: the amount that a server receives for completing the task.
%
\item[$\bullet$] $\wc \geq \cc$: the server would not accept underpaid jobs.
%
\item[$\bullet$] $\chc > 2\wc$: if it does not hold, then there would be no need to use the servers and the auditor would do the computation.
%
\item [$\bullet$] $(pk,sk)$: an asymmetric-key encryption's public-private key pair belonging to the auditor. 
\end{itemize}

The following relations must be satisfied when establishing the contracts to ensure that the desirable equilibria are maintained:

\vspace{-1.5mm}
 $$(\dc>\cc+\chc) \wedge (\bc<\cc) \wedge (\tc<\wc-\cc + 2\dc - \chc -\bc)$$





\input{Peisoner-contract.tex}

\input{Colluder-contract.tex}

\input{Traitor-contract.tex}



==> CCS-24/error-prob.tex <==
% !TEX root =main.tex


\subsection{Error Probability}\label{sec::error-prob}


Recall that in \fpsi, during step \ref{JUS::check-non-zero-coeff},  each client $C$ needs to ensure that polynomials $\bm\omega^{\st (C,D)}\cdot \bm\pi^{\st  {  {(C)}}}$ and  $\bm\rho^{\st (C,D)}$ do not contain any zero coefficient. This check ensures that client $C$ (the receiver in \vopr) does not insert any zero values to  \vopr, especially within $\ole^{\st +}$, which is a subroutine of \vopr. If a zero value is inserted in \vopr, an honest receiver will only learn a random value, and more importantly they cannot successfully pass \vopr's verification phase. 
%
However, this check can be omitted from \ref{JUS::check-non-zero-coeff}, if we permit \fpsi to produce an error with a very low probability.\footnote{By error we mean even if all parties are honest,  \vopr halts when an honest party inserts $0$ to it.} In the remainder of this section, we demonstrate that this probability is negligible with regard to the security parameter. 


Initially, we focus on the product $\bm\omega^{\st (C,D)}\cdot \bm\pi^{\st  {  {(C)}}}$. We know that $\bm\pi^{\st  {  {(C)}}}$ takes the form of  $\prod\limits^{\st d}_{\st i=1} (x-s'_{\st i})$, where $s'_{\st i}$ is either a set element $s_{\st i}$ or a random value.  Thus, all of its coefficients are non-zero. Additionally, the probability that at least one of the coefficients of $d$-degree random polynomial $\bm\omega^{\st (C,D)}$ equals $0$ is at most $\frac{d+1}{p}$.  Below, we formally state this.


\begin{theorem}\label{theorem::zero-coeff-in-ran-poly}
Let $\bm\delta=\sum\limits_{\st t=0}^{\st d}u_{\st  t} \cdot x^{\st t}$, where  $u_{\st  t}\stackrel{\st\$}\leftarrow\mathbb{F}_{\st p}$, for all $t, 0\leq t\leq d$. Then, the probability that at least one of the coefficients equals $0$ is at most $\frac{d+1}{p}$, i.e., 

$$Pr[\exists u_{\st t}, u_{\st t}=0]\leq \frac{d+1}{p}$$
\end{theorem}


\begin{proof}
The proof is straightforward. Since $\bm\delta$'s coefficients are picked uniformly at random from  $\mathbb{F}_{\st p}$, the probability that $u_{\st t}$ equals $0$ is $\frac{1}{p}$. Since $\bm\delta$ is of degree $d$, due to the union bound, the probability that at least one of $u_{\st t}$s equals $0$ is at most $\frac{d+1}{p}$. 
%
 \end{proof}



Next, we demonstrate that the probability of the polynomial  $\bm\omega^{\st (C,D)}\cdot \bm\pi^{\st  {  {(C)}}}$ having at least one zero coefficient is negligible with respect to the security parameter. We assume polynomial $\bm\omega^{\st (C,D)}$  has no zero coefficient. 


%For the sake of simplicity,  we set $\bm{p}_1=\bm\omega^{\st (C,D)}=a_{\st 0}\cdot a_{\st 1}\cdot x+...+a_{\st d}\cdot x^{\st d}$ and $\bm{p}_2= \bm\pi^{\st  {  {(C)}}}$. 

\begin{theorem}\label{theorem::zero-coeff-in-product}
Let  $\bm\alpha=\sum\limits_{\st j=0}^{\st m}a_{\st  i} \cdot x^{\st i}$ and  $\bm\beta=\sum\limits_{\st j=0}^{\st n}b_{\st  j} \cdot x^{\st j}$,  where $a_{\st i}\stackrel{\st\$}\leftarrow \mathbb{F}_{\st p}$ and $a_{\st i}, b_{\st j}\neq0$, for all $i,j, 0\leq i \leq m$ and $0\leq j \leq n$. Also, let $\bm\gamma=\bm\alpha\cdot\bm\beta=\sum\limits_{\st j=0}^{\st m+n}c_{\st  j} \cdot x^{\st j}$. Then, the probability that at lest one of the coefficients of polynomial $\bm\gamma$ equals $0$ is at most $\frac{m+n+1}{p}$, i.e., 
%
$$Pr[\exists c_{\st j}, c_{\st j}=0]\leq \frac{m+n+1}{p}$$
%
\end{theorem}



\begin{proof}
Each coefficient $c_{\st  k}$ of $\bm\gamma$ can be defined as $c_{\st  k}=\sum\limits_{\substack{\st j=0\\ \st i=0}}^{\substack{\st i=m\\ \st j=n}}a_{\st i}\cdot b_{\st j}$, where $i+j=k$. We can rewrite $c_{\st  k}$ as  $c_{\st  k}=a_{\st w}\cdot b_{\st z}+ \sum\limits_{\substack{\st j=0, j\neq z\\ \st i=0, i\neq w}}^{\substack{\st i=m\\ \st j=n}}a_{\st i}\cdot b_{\st j}$, where $w+z=i+j=k$. 
%
We consider two cases for each $c_{\st  k}$:

\begin{itemize}

\item[$\bullet$]  {Case 1}: $\sum\limits_{\substack{\st j=0, j\neq z\\ \st i=0, i\neq w}}^{\substack{\st i=m\\ \st j=n}}a_{\st i}\cdot b_{\st j}=0$.  This is a trivial case because with the  probability of $1$ it holds that $c_{\st  k}=a_{\st w}\cdot b_{\st z}\neq 0$. Because by  definition $a_{\st w}, b_{\st z}\neq0$ and $\mathbb{F}_{\st p}$ is an integral domain. 

%In this case, since $a_{\st w}$ has been picked uniformly at random, the probability that $c_{\st  k}=a_{\st w}\cdot b_{\st z}=0$ is $\frac{1}{p}$.

%
% This is a trivial case, because with the  probability of $1$ it holds that $c_{\st  k}=a_{\st w}\cdot b_{\st z}\neq 0$. 


%In this case, because $a_{\st w}$ has been picked uniformly at random, with the  probability of $\frac{1}{p}$ it holds that $c_{\st  k}=a_{\st w}\cdot b_{\st z}=0$. 


\item[$\bullet$]  {Case 2}: $q=\sum\limits_{\substack{\st j=0, j\neq z\\ \st i=0, i\neq w}}^{\substack{\st i=m\\ \st j=n}}a_{\st i}\cdot b_{\st j}\neq 0$. In this case, for  event $c_{\st  k}=a_{\st w}\cdot b_{\st z}+q=0$ to occur, $a_{\st w}\cdot b_{\st z}$ must equal the additive inverse of $q$. Since $a_{\st w}$ has been uniformly selected at random, the probability of such an event occurring is $\frac{1}{p}$.
\end{itemize}

The above analysis is for a single $c_{\st  k}$. Thus, as a result of applying the union bound, the probability that at least one of the coefficients $c_{\st  k}$ equals $0$ is at most $\sum\limits^{\st m+n}_{\st j=0}\frac{1}{p}= \frac{m+n+1}{p}$.
%
 \end{proof}




Next we turn out attention to $\bm\rho^{\st (C,D)}$. Due to Theorem \ref{theorem::zero-coeff-in-ran-poly}, the probability that at least one of the coefficients of $\bm\rho^{\st (C,D)}$ equals $0$ is at most $\frac{d+1}{p}$. 
%
Hence, due to Theorems \ref{theorem::zero-coeff-in-ran-poly}, \ref{theorem::zero-coeff-in-product}, and union bound, the probability that at least one of the coefficients in $\bm\omega^{\st (C,D)}\cdot \bm\pi^{\st  {  {(C)}}}$ and  $\bm\rho^{\st (C,D)}$ equals $0$ is at most $\frac{3d+2}{p}$, which is negligible in  $p$. 

















==> CCS-24/evaluation-table.tex <==
%!TEX root = main.tex

\begin{table*} 

\begin{center}

\caption{ \small{Comparison of the asymptotic complexities and features of state-of-the-art PSIs. In the table, $t$ is a parameter that determines the maximum number of colluding parties and $\kappa$ is a security parameter.}}  \label{table::comparisonTable} 
\vspace{-3mm}
%\renewcommand{\arraystretch}{1}
\scalebox{.85}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|} 
\hline

%\multicolumn{3}{c|}

%\multirow{2}{*} {\scriptsize {Schemes}} &{\scriptsize {Computation}}& \scriptsize{Communication}&{\scriptsize{Fairness}}&{ \scriptsize Rewarding}& {\scriptsize{ Sym-key based}}& {\scriptsize{Multi-party}}&\scriptsize Active Adversary \\
%\hline

\multirow{2}{*} {\scriptsize {Schemes}} &\multicolumn{2}{c|}{\scriptsize Asymptotic Cost}&\multicolumn{5}{c|}{\scriptsize{Features}} \\

\cline{2-8}

& \scriptsize{Computation}&\scriptsize{Communication}&{\scriptsize{Fairness}}&{ \scriptsize Rewarding}& {\scriptsize{ Sym-key based}}& {\scriptsize{Multi-party}}&\scriptsize Active Adversary\\




\hline 

%&\scriptsize {Modular expo.}&\cellcolor{gray!20}\scriptsize {$0$}&\cellcolor{gray!20}\scriptsize$5$&\cellcolor{gray!20}\scriptsize$12$\\


\scriptsize  \scriptsize{ \cite{AbadiDMT22}}&\cellcolor{gray!20}\scriptsize{$O( h\cdot d^{\st 2}\cdot m)$}&\cellcolor{gray!20}\scriptsize$O(h\cdot d\cdot m)$&\cellcolor{gray!20}\scriptsize\textcolor{red}{$\times$}&\cellcolor{gray!20}\scriptsize\textcolor{red}{$\times$}&\cellcolor{gray!20}\scriptsize\textcolor{blue}\checkmark  &\cellcolor{gray!20}\scriptsize\textcolor{blue}\checkmark&\cellcolor{gray!20}\scriptsize\textcolor{red}{$\times$} \\


\hline 


\scriptsize \cite{DebnathD16}&\cellcolor{gray!50}\scriptsize{$O(|S|)$}&\cellcolor{gray!50}\scriptsize{$O(|S|)$}&\cellcolor{gray!50}\scriptsize\textcolor{blue}\checkmark&\cellcolor{gray!50}\scriptsize\textcolor{red}{$\times$}&\cellcolor{gray!50}\scriptsize\textcolor{red}{$\times$} &\cellcolor{gray!50}\scriptsize\textcolor{red}{$\times$}&\cellcolor{gray!50}\scriptsize\textcolor{blue}\checkmark \\ 




\hline

\scriptsize {\cite{DBLP:conf/dbsec/DongCCR13}}&\cellcolor{gray!20}\scriptsize{$O(|S|^{\st 2}$)}&\cellcolor{gray!20}\scriptsize$O(|S|)$&\cellcolor{gray!20}\scriptsize\textcolor{blue}\checkmark&\cellcolor{gray!20}\scriptsize\textcolor{red}{$\times$}  &\cellcolor{gray!20}\scriptsize\textcolor{red}{$\times$} &\cellcolor{gray!20}\scriptsize\textcolor{red}{$\times$}&\cellcolor{gray!20} \scriptsize\textcolor{blue}\checkmark\\ 

\hline
\scriptsize \cite{DBLP:conf/ccs/KolesnikovMPRT17}   &\cellcolor{gray!50}\scriptsize{$O(|S|\cdot m^{\st 2}+|S|\cdot m )$}&\cellcolor{gray!50}\scriptsize$O(|S|\cdot m^{\st 2})$&\cellcolor{gray!50}\scriptsize\textcolor{red}{$\times$}&\cellcolor{gray!50}\scriptsize\textcolor{red}{$\times$}  &\cellcolor{gray!50}\scriptsize\textcolor{blue}\checkmark &\cellcolor{gray!50}\scriptsize\textcolor{blue}\checkmark&\cellcolor{gray!50}\scriptsize\textcolor{red}{$\times$}\\ 

\hline


\scriptsize \cite{NevoTY21}&\cellcolor{gray!20}\scriptsize{$O(|S|\cdot \kappa(m+t^{\st 2}-t(m+1)))$}&\cellcolor{gray!20}\scriptsize{$O(|S|\cdot m\cdot \kappa)$}&\cellcolor{gray!20}\scriptsize{\textcolor{red}{$\times$}}&\cellcolor{gray!20}\scriptsize\textcolor{red}{$\times$}&\cellcolor{gray!20}\scriptsize\textcolor{blue}\checkmark  &\cellcolor{gray!20}\scriptsize\textcolor{blue}\checkmark&\cellcolor{gray!20}\scriptsize\textcolor{blue}\checkmark\\ 

\hline


\scriptsize \cite{RaghuramanR22}&\cellcolor{gray!50}\scriptsize{$O(|S|)$}&\cellcolor{gray!50}\scriptsize{$O(|S|\cdot \kappa)$}&\cellcolor{gray!50}\scriptsize{\textcolor{red}{$\times$}}&\cellcolor{gray!50}\scriptsize\textcolor{red}{$\times$} &\cellcolor{gray!50}\scriptsize\textcolor{blue}\checkmark &\cellcolor{gray!50}\scriptsize{\textcolor{red}{$\times$}} &\cellcolor{gray!50}\scriptsize\textcolor{blue}\checkmark\\ 

\hline



{\scriptsize \textbf{Ours:} \epsi}&\cellcolor{gray!20}\scriptsize{$O (h\cdot d^{2}\cdot m)$}&\cellcolor{gray!20}\scriptsize$O (h\cdot d^{\st 2}\cdot \bar\xi\cdot m )$&\cellcolor{gray!20}\scriptsize\textcolor{blue}\checkmark&\cellcolor{gray!20}\scriptsize \textcolor{blue}\checkmark&\cellcolor{gray!20}\scriptsize\textcolor{blue}\checkmark &\cellcolor{gray!20}\scriptsize\textcolor{blue}\checkmark&\cellcolor{gray!20}\scriptsize\textcolor{blue}\checkmark \\

\hline 

\end{tabular}
}
%\renewcommand{\arraystretch}{1}
%\end{footnotesize}
\end{center}
%}
\vspace{-3.5mm}
\end{table*}






==> CCS-24/evaluation.tex <==
% !TEX root =main.tex


\vspace{-2mm}

\section{Evaluation}\label{sec::valuation}

\vspace{-1mm}

In this section, we analyze the overhead of \epsi and compare its costs and features with the fastest two and multiple parties PSIs in \cite{AbadiDMT22,DBLP:conf/ccs/KolesnikovMPRT17,NevoTY21,RaghuramanR22}), as well as with the fair PSIs in \cite{DebnathD16,DBLP:conf/dbsec/DongCCR13}. Tables \ref{table::Asymptotic-Cost} and \ref{table::comparisonTable} respectively summarize the result of the analysis. 

\vspace{-1mm}

\input{table-cost}
\vspace{-1mm}
\input{evaluation-table}

\vspace{-2mm}
\subsection{Computation Cost}

\vspace{-.6mm}
\subsubsection{Client's and Dealer's Costs.}

In step \ref{e-psi::call-F-PSI-stepOne}, the cost of each client (including $D$) is $O(m)$ and mainly involves an invocation of \ct. 
% 
In steps \ref{e-psi::deploy-SC-E-PSI}--\ref{e-PSI::extractor-deposit}, the clients' cost is negligible. 
%
In step \ref{e-psi::gen-mk-prime}, the clients' cost is  $O(m)$, as they need to invoke an instance of \ct. 
%
In step \ref{Smart-PSI:encode-elem}, each client invokes \prp and $\mathtt{H}$ linear with its set's cardinality. In the same step, it also constructs $h$ polynomials, where the construction of each polynomial involves $d$   multiplications and additions. Thus, its complexity in this step is $O(h\cdot d)$. As shown in \cite{AbadiDMT22},  $O(h\cdot d)=O(|S|)$ and  $d=100$ for all set sizes. 
%


In step \ref{e-psi::invoke-remainer-F-PSI}, each client   $A_{\st  1},...,    A_{\st   m}$ (excluding $D$): (i) invokes an instance of \zspaa which involves $O(h\cdot m)$ invocations of \ct, $3h\cdot m (d+1)$ invocations of \prf, $3h\cdot m (d+1)$ addition, and $O(h\cdot m\cdot d)$ invocations of $\mathtt{H}$ (in step \ref{ZSPA} of subroutine \fpsi), (ii) invokes $2h$ instances of \vopr, where each \vopr invocation involves $2d(1+d)$ invocations of $\ole^{\st +}$, multiplications, and additions  (in steps \ref{e-psi::D-randomises} and \ref{e-psi::C-randomises} of \fpsi), and (iii) performs $h(3d+2)$ addition (in step \ref{blindPoly-C-sends-to-contract} of  \fpsi).  
 
If $Flag=True$, each client invokes $h (3d+1)$ instances of $\prf$,  performs $h (3d+1)$ additions, and performs polynomial evaluations linear with $|S|$, where each evaluation involves  $O(d)$  additions and multiplications. % (in step \ref{F-PSI::flag-is-true} of \fpsi). 
 %
 Step \ref{e-psi::commit-to-mk} involves only $D$ whose cost in this step is constant, as it involves invoking public key encryption, \prf,  and commitment once. Also, $D$:  (a) invokes $2h\cdot m$ instances of \vopr  (in steps \ref{e-psi::D-randomises} and \ref{e-psi::C-randomises} of \fpsi), (b) invokes  $h(3d+1)$ instances of $\prf$ (in step \ref{f-psi::D-gen-random-poly} of \fpsi), and (c) does $h(d^{\st 2}+1)$ multiplications and $3h\cdot m\cdot d$ additions (in step \ref{f-psi::D-gen-switching-poly} of \fpsi). If $Flag=False$, then $D$ performs $O(h\cdot m\cdot d)$ multiplications and additions (in step \ref{F-PSI::flag-is-false} of \fpsi).  

\vspace{-2.4mm}
 \subsubsection{Auditor's Cost.}
 
When $Flag=False$, \aud invokes $3h\cdot m(d+1)$ instances of $\prf$, and $O(h\cdot m\cdot d)$ instances of $\mathtt{H}$ (in step \ref{F-PSI::flag-is-false} of \fpsi). 


\vspace{-2.4mm}
 \subsubsection{Extractor's Cost.}
 
 
 In step \ref{merkel-tree-cons}, each extractor invokes the commitment scheme linearly with the number of its set cardinality $|S|$ and constructs a Merkle tree on top of the commitments. %Therefore, its complexity is $O(|S|)$.  
%
In step \ref{smart-PSI::extractors}, each extractor invokes $\mathtt{H}$ linear with its set cardinality $|S|$. It also performs polynomial evaluations linear with $|S|$. 

\vspace{-1.5mm}
 \subsubsection{Smart Contracts' Cost.}

In step \ref{e-psi::invoke-remainer-F-PSI}, the subroutine smart contract $\mathcal{SC}_{\st\fpsi}$ performs $h\cdot m(3d+1)$ additions and $h$ polynomial divisions,  where each division includes dividing a polynomial of degree $3d+1$ by a polynomial of degree $1$ (in step \ref{compute-res-poly} of \fpsi). In step \ref{e-psi::SC-verification--derive-mk}, $\mathcal{SC}_{\st\epsi}$ invokes the commitment's verification algorithm $\comver$ only once,  calls at most $|S_{\st \cap}|$ instances of  $\mathtt{H}$, and invokes $|S_{\st \cap}| (3d+1)$ instances of $\prf$. In step \ref{e-psi::SC-verification--check-three-vals}, $\mathcal{SC}_{\st\epsi}$ invokes  at most $|S_{\st \cap}|$ instances of $\comver$, and calls $O(|S_{\st \cap}|\cdot \log_{\st 2} |S|)$ instances of $\mathtt{H}$. In the same step, it performs polynomial evaluation linear with  $|S_{\st \cap}|$. Thus, its overall complexity is $O( |S_{\st \cap}|(d+ \log_{\st 2} |S|))$.
%



%In the same step, the subroutine smart contract $\mathcal{SC}_{\st\fpsi}$ performs $h\cdot m(3d+1)$ additions and $h$ polynomial divisions,  where each division includes dividing a polynomial of degree $3d+1$ by a polynomial of degree $1$ (in step \ref{compute-res-poly} of \fpsi). 





%Moreover, if $Flag=True$, then each client invokes $\prf$ $h (3d+1)$ times, and performs $h (3d+1)$ additions, and performs polynomial evaluations linear with its set cardinality, where each evaluation involves  $O(d)$  additions and $O(\frac{d^{\st 2}+d}{2})$ multiplications (in step \ref{F-PSI::flag-is-true} of \fpsi). If $Flag=False$, then (a) \aud invokes $\prf$ $3h\cdot m(d+1)$ times  and  invokes $\mathtt{H}$ $O(h\cdot m\cdot d)$ times, and (b) $D$ performs $O(h\cdot m\cdot d)$ multiplications and additions (in step \ref{F-PSI::flag-is-false} of \fpsi). 




%

  
  % (where each evaluation involves  $O(d)$  additions and $O(\frac{d^{\st 2}+d}{2})$ multiplications). 



%In step \ref{e-psi::SC-verification}, $\mathcal{SC}_{\st\epsi}$ invokes the commitment's verification algorithm, the hash function, at most linear with the intersection cardinality $|S_{\st \cap}|$, invokes $\prf$ $3d+1$ times, invokes the hash function $O(\log_{\st 2} (d\cdot m))$ times, and performs polynomial evaluations linear with the smallest set cardinality.% (where each evaluation involves  $O(d)$  additions and $O(\frac{d^{\st 2}+d}{2})$ multiplications). 

 %\scf  performs $h\cdot m(3d+1)$ modular additions and $h$ polynomial divisions (in step \ref{compute-res-poly} of F-PSI). 


\vspace{-2.9mm}
\subsection{Communication Cost}

\vspace{-.7mm}

In steps  \ref{e-psi::call-F-PSI-stepOne} and \ref{e-psi::gen-mk-prime}, the clients' communication cost is dominated by the cost of \ct which is $O(m)$. In steps \ref{e-psi::deploy-SC-E-PSI}--\ref{e-psi::commit-to-mk}, the clients' cost is negligible, as it involves sending a few transactions to the smart contracts. Step \ref{merkel-tree-cons} involves only extractors whose cost is $O(h)$ as each of them only sends to $\mathcal{SC}_{\st\epsi}$  a  value for each bin. In step \ref{e-psi::invoke-remainer-F-PSI}, the clients' cost is dominated by \vopr's cost; specifically, each pair of client and $D$ invokes $O(d^{\st 2})$ instances of \vopr for each bin. Therefore, the cost of each client (excluding $D$) is $O(h\cdot d^{\st 2}\cdot \bar\xi)$ while the cost of $D$ is $O(h\cdot d^{\st 2}\cdot \bar\xi\cdot m)$, where $\bar\xi$ is \ole's security parameter. 
%
Step \ref{smart-PSI::extractors}  involves only the extractors, where each extractor's cost is dominated by the size of the Merkle tree's proof sent to $\mathcal{SC}_{\st\epsi}$, i.e., $O(|S_{\scriptscriptstyle\cap}|\cdot \log_{\st 2}|S|)$, where $|S|$ is the extractor's set cardinality. 
%
In step \ref{F-PSI::flag-is-false}, \aud sends $h$ polynomials of degree $3d+1$ to $\mathcal{SC}_{\st\fpsi}$. Thus, its complexity is $O(h\cdot d)$. 
%
The other steps have negligible communication costs. 

\vspace{-2.7mm}
\subsection{Comparison}
\vspace{-.6mm}


We show that \epsi provides multiple features, not found in other PSIs while maintaining a comparable overhead to efficient PSIs.

\vspace{-2mm}
\subsubsection{Computation Complexity.} \epsi's computation complexity is similar to that of PSI in \cite{AbadiDMT22}, but is better than the multi-party PSI's complexity in \cite{DBLP:conf/ccs/KolesnikovMPRT17} as  the latter's complexity is quadratic with the number of parties, i.e., $O(|S|\cdot d\cdot m)$ versus $O(|S|\cdot m^{\st 2}+|S|\cdot m )$. \epsi's complexity  is better than the PSI's complexity in   \cite{NevoTY21}  that is quadratic with parameter $t$. Similar to the two-party PSIs in \cite{DebnathD16,RaghuramanR22}, \epsi's complexity is linear with $|S|$.  The two-party PSI in \cite{DBLP:conf/dbsec/DongCCR13} has a higher computation cost than \epsi does, as its complexity is quadratic with sets' cardinality. Hence, the complexity of \epsi is: (i) linear with the set size, similar to the above schemes except for the one in \cite{DBLP:conf/dbsec/DongCCR13} and (ii) linear with the total number of parties, similar to  the above multi-party schemes, excluding the one in \cite{DBLP:conf/ccs/KolesnikovMPRT17}. 
%
%Hence, the computation complexity of \epsi is linear with the set cardinality and the number of parties, similar to the above schemes except for the ones in \cite{DBLP:conf/ccs/KolesnikovMPRT17,DBLP:conf/dbsec/DongCCR13} whose complexities are quadratic with the set cardinality or the number of parties. 

\vspace{-2mm}
\subsubsection{Communication Complexity.}  \epsi's communication complexity is slightly higher than the complexity of the PSI in \cite{AbadiDMT22}, by a factor of $d\cdot \bar\xi$. However, it is better than the  PSI's complexity in \cite{DBLP:conf/ccs/KolesnikovMPRT17} as the latter has a complexity quadratic with the number of parties. \epsi's complexity is slightly higher than the one in \cite{NevoTY21}, by a factor of $d$. Similar to the two-party PSIs in  \cite{DebnathD16,RaghuramanR22,DBLP:conf/dbsec/DongCCR13}, \epsi's complexity is linear with $c$. 
%
Hence, \epsi's communication complexity is linear with the set cardinality and number of parties, similar to the above schemes except for the one in \cite{DBLP:conf/ccs/KolesnikovMPRT17} whose complexity is quadratic.% with the number of parties. 

\vspace{-2mm}
\subsubsection{Features.} \epsi stands out as the sole scheme offering five vital features: fairness support, participant rewards, reliance on symmetric key primitives, multi-party capability, and security against active adversaries.  In contrast, the next most comprehensive scheme, introduced in \cite{NevoTY21}, offers only three of these features. The remaining protocols provide support for just two of the mentioned features. We highlight that our \epsi and  \fpsi are the only PSIs that use smart contracts (that require additional but standard blockchain-related assumptions). The other protocols do not utilize smart contracts. 










==> CCS-24/hash-table.tex <==
% !TEX root =main.tex

\section{Hash Tables}\label{Preliminary-Hash-Table}

We set the table's parameters appropriately to ensure the number of elements in each bin does not exceed a predefined capacity. Given the maximum number of elements $c$ and the bin's maximum size $d$, we can determine the number of bins by analyzing hash tables under the balls into bins model  \cite{DBLP:conf/stoc/BerenbrinkCSV00}.
\vspace{-1mm}
\begin{theorem}\label{chernoff}\textbf{(Upper Tail in Chernoff Bounds)} Let $X_{\scriptscriptstyle i}$ be a random variable defined as $X_{\scriptscriptstyle i}=\sum\limits^{\scriptscriptstyle c}_{\scriptscriptstyle  i=1} Y_{\scriptscriptstyle i}$, where $Pr[Y_{\scriptscriptstyle i}=1]=p_{\scriptscriptstyle i}$, $Pr[Y_{\scriptscriptstyle i}=0]=1-p_{\scriptscriptstyle i}$, and all $Y_{\scriptscriptstyle i}$ are independent. Let the expectation be $\mu=\mathrm{E}[X_{\scriptscriptstyle i}]=\sum\limits ^{\scriptscriptstyle h}_{\scriptscriptstyle  i=1} p_{\scriptscriptstyle i}$, then 
$Pr[X_{\scriptscriptstyle i}>d=(1+\sigma)\cdot \mu]<\Big(\frac{e^{\scriptscriptstyle \sigma}}{(1+\sigma)^{\scriptscriptstyle (1+\sigma)}}\Big)^{\scriptscriptstyle \mu}, \forall \sigma>0$
\end{theorem}

In this model, the expectation is  $\mu=\frac{c}{h}$, where $c$ is the number of  balls and $h$ is the number of bins. The above inequality provides the probability that bin $i$ gets more than $(1+\sigma)\cdot \mu$ balls. Since there are $h$ bins, the probability that at least one of them is overloaded is bounded by the union bound:
\begin{equation}\label{equation:the-bound}
Pr[\exists i, X_{\scriptscriptstyle i}>d]\leq \sum\limits^{\scriptscriptstyle h}_{\scriptscriptstyle i=1}Pr[X_{\scriptscriptstyle i}>d] = h\cdot  \Big(\frac{e^{\scriptscriptstyle \sigma}}{(1+\sigma)^{\scriptscriptstyle (1+\sigma)}}\Big)^{\scriptscriptstyle \frac{c}{h}}
\end{equation}

Thus, for a hash table of length $h=O(c)$, there is always an  \emph{almost constant} expected number of elements, $d$,  mapped to the same bin with a high probability \cite{DBLP:conf/ccs/PapamanthouTT08}, e.g., $1-2^{\scriptscriptstyle -40}$. 

Appendix \ref{sec::conc-parameters} explains how to establish concrete parameters for a hash table.

==> CCS-24/justitia-further-discussion.tex <==
% !TEX root =main.tex


%%%%%%%%%%%%%%%%%
\section{Further Discussion on  \withFai}\label{sec::Discussion-justitia}


\subsection{Input and Output Privacy}

Intuitively, all parties locally blind/encrypt all (set element related) messages before they send them the smart contract \scf. Moreover, the resultant polynomial that \scf computes is in a blinded form and it reveals only the intersection of the sets after it is unblinded (as discussed in Section \ref{sec::poly-rep}, on page \pageref{sec::poly-rep}).


Hence, (i) no party (including the protocol's participants) can learn other parties input set elements and (ii) the non-participants of the protocol cannot learn anything about the protocol's output, not even the intersection cardinality. 


\subsection{Strawman Approaches}


\subsubsection{Relying on a Server-aide PSI.} One may be tempted to replace $\withFai$ with a scheme in which all clients send their encrypted sets to a server (potentially semi-honest and plays \aud's role) which computes the result in a privacy-preserving manner.  We highlight that the main difference is that in this (hypothetical) scheme the server is \emph{always involved};  whereas, in our protocol, \aud remains offline as long as the clients behave honestly and it is invoked only when the contract detects misbehaviors.  


\subsubsection{Charging the Buyer a Flat Fee.}

One might wish to incorporate a straightforward payment mechanism into an existing multi-party PSI such that a buyer is always required to pay a fixed amount, which could depend on factors such as the total number of clients and the minimum size of the sets. However, this approach presents challenges, because:

\begin{enumerate}
\item it compels the buyer to make payments even if certain malicious clients misbehave during the protocol execution and compromise the accuracy of the results. This situation could enable malicious clients to gain access to the result at the buyer's expense without allowing the buyer to obtain the correct result. Unfortunately, there is no fair multi-party PSI in the existing literature that guarantees either all parties learn the correct result or none of them do. 

\item it compels the buyer to make payments regardless of the precise size of the intersection. If the buyer ends up paying more than the amount it would have paid for the exact cardinality of the intersection, it might become discouraged from participating in the protocol altogether. Conversely, if the buyer has to pay less than what it would have paid for the size of the intersection, it may discourage other clients from participating in the protocol.

\end{enumerate}



\input{error-prob}


 
\input{Justitia-challenges}

\input{zeta}

\input{Concrete-parameters}


==> CCS-24/notation-Table.tex <==
% !TEX root =main.tex


\section{Notation Table}\label{sec::notation-table}
%\vspace{-1.2mm}
Table \ref{commu-breakdown-party} summarizes the main notations used in the paper. 

\vspace{-3mm}

\begin{table}[!h]
\begin{scriptsize}
\begin{center}
\footnotesize{
%\vspace{-6mm}
\caption{ \small{Notation Table}.}\label{commu-breakdown-party} 
\renewcommand{\arraystretch}{.94}
\scalebox{0.94}{
% 1st table
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|} 

%\hline 
%\multicolumn{1}{|c|}{\cellcolor{yellow!10}\scriptsize{Setting}}&\cellcolor{yellow!10} \scriptsize{Symbol}&\cellcolor{yellow!10} \scriptsize{Description}\\
%\hline 

\hline 
\multicolumn{1}{|c|}{\rotatebox[origin=c]{45}{\cellcolor{yellow!10}\scriptsize{ {Setting}}}}&\cellcolor{yellow!10} \scriptsize{Symbol}&\cellcolor{yellow!10} \scriptsize{Description}\\
\hline 

%{\rotatebox[origin=c]{90}{\scriptsize{ {Contracts}}}}

%%%%%%%%%. Generic %%%%%

\cellcolor{yellow!10}&\cellcolor{gray!20}\scriptsize$p$&\cellcolor{gray!20}\scriptsize \text{Large prime number}\\   
%
\cellcolor{yellow!10}&\cellcolor{white!20}\scriptsize{$\mathbb{F}_{\st p}$}&\cellcolor{white!20}\scriptsize \text{A finite field of prime order $p$}\\   
%
\cellcolor{yellow!10}&\cellcolor{gray!20}\scriptsize$\cl$&\cellcolor{gray!20}\scriptsize \text{Set of all clients, $\{ A_{\st 1},...,   A_{\st m},  D\}$ }\\   
%
\cellcolor{yellow!10}&\cellcolor{white!20}\scriptsize$D$&\cellcolor{white!20}\scriptsize \text{Dealer client}\\   
%
\cellcolor{yellow!10}&\cellcolor{gray!20}\scriptsize$A_{\st m}$&\cellcolor{gray!20}\scriptsize{Buyer client}\\ 
%
\cellcolor{yellow!10}&\cellcolor{white!20}\scriptsize$m$&\cellcolor{white!20}\scriptsize \text{Total number of clients (excluding $D$)}\\   
%
\cellcolor{yellow!10}&\cellcolor{gray!20}\scriptsize$\mathtt{H}$&\cellcolor{gray!20}\scriptsize \text{Hash function}\\ 
%
\cellcolor{yellow!10}&\cellcolor{white!20}\scriptsize$|S_{\st\cap}|$&\cellcolor{white!20}\scriptsize{Intersection size}\\ 
%
\cellcolor{yellow!10}&\cellcolor{gray!20}\scriptsize$\Smin$&\cellcolor{gray!20}\scriptsize{Smallest set's size}\\
%
\cellcolor{yellow!10}&\cellcolor{white!20}\scriptsize$\Smax$&\cellcolor{white!20}\scriptsize{Largest set's size}\\
%
\cellcolor{yellow!10}&\cellcolor{gray!20}\scriptsize$|$&\cellcolor{gray!20}\scriptsize{Divisible}\\
%
\cellcolor{yellow!10}&\cellcolor{white!20}\scriptsize$\setminus$&\cellcolor{white!20}\scriptsize{Set subtraction}\\
%
\cellcolor{yellow!10}&\cellcolor{gray!20}\scriptsize$c$&\cellcolor{gray!20}\scriptsize{Set's cardinality}\\ 
 %
 \cellcolor{yellow!10}&\cellcolor{white!20}\scriptsize$h$&\cellcolor{white!20}\scriptsize{Total number of bins in a hash table}\\ 
 %
 \cellcolor{yellow!10}&\cellcolor{gray!20}\scriptsize$d$&\cellcolor{gray!20}\scriptsize{A bin's capacity}\\ 
 %
\cellcolor{yellow!10}&\cellcolor{white!20}\scriptsize$\lambda$ &\cellcolor{white!20}\scriptsize Security parameter  \\  

%
\cellcolor{yellow!10}&\cellcolor{gray!20}\scriptsize \ole&\cellcolor{gray!20}\scriptsize{Oblivious Linear Evaluation}\\ 
%
\cellcolor{yellow!10}&\cellcolor{white!20}\scriptsize$\ole^{\st +}$&\cellcolor{white!20}\scriptsize{Advanced \ole}\\ 

\cellcolor{yellow!10}&\cellcolor{gray!20}\scriptsize$\comcom$&\cellcolor{gray!20}\scriptsize \text{Commitment algorithm of commitment}\\ 

\cellcolor{yellow!10}&\cellcolor{white!20}\scriptsize$\comver$&\cellcolor{white!20}\scriptsize \text{Verification algorithm of commitment}\\ 

\cellcolor{yellow!10}&\cellcolor{gray!20}\scriptsize$\mkgen$&\cellcolor{gray!20}\scriptsize \text{Tree construction algorithm of Merkle tree}\\ 

\cellcolor{yellow!10}&\cellcolor{white!20}\scriptsize$\mkprove$&\cellcolor{white!20}\scriptsize \text{Proof generation algorithm of Merkle tree}\\ 

\cellcolor{yellow!10}&\cellcolor{gray!20}\scriptsize$\mkver$&\cellcolor{gray!20}\scriptsize \text{Verification algorithm of Merkle tree}\\ 

\cellcolor{yellow!10}&\cellcolor{white!20}\scriptsize{\ct}&\cellcolor{white!20}\scriptsize \text{Coin tossing protocol}\\  

 \cellcolor{yellow!10}&\cellcolor{gray!20}\scriptsize{\vopr}&\cellcolor{gray!20}\scriptsize \text{Verifiable Oblivious Poly. Randomization}\\
 
 \cellcolor{yellow!10} &\cellcolor{white!20}\scriptsize{\zspa}&\cellcolor{white!20}\scriptsize \text{ Zero-sum Pseudorandom Values Agreement}\\
  
  \cellcolor{yellow!10}   &\cellcolor{gray!20}\scriptsize{\zspaa}&\cellcolor{gray!20}\scriptsize \text{\zspa with an External Auditor}\\

   \cellcolor{yellow!10}  &\cellcolor{white!20}\scriptsize{\p}&\cellcolor{white!20}\scriptsize \text{Multi-party PSI with Fair Compensation}\\
     
    \cellcolor{yellow!10}      &\cellcolor{gray!20}\scriptsize{\ep}&\cellcolor{gray!20}\scriptsize \text{Multi-party PSI with Fair Compensation and Reward}\\

  \cellcolor{yellow!10}   &\cellcolor{white!20}\scriptsize{\fpsi}&\cellcolor{white!20}\scriptsize \text{Protocol that realizes \p}\\
     
     
  \cellcolor{yellow!10}   &\cellcolor{gray!20}\scriptsize{\epsi}&\cellcolor{gray!20}\scriptsize \text{
          Protocol that realizes \ep}\\

\cellcolor{yellow!10}&\cellcolor{white!20}\scriptsize$\prf$ &\cellcolor{white!20}\scriptsize  Pseudorandom function \\ 


  \cellcolor{yellow!10}&\cellcolor{gray!20}\scriptsize$\prp$ &\cellcolor{gray!20}\scriptsize  Pseudorandom permutation \\ 

%
  \cellcolor{yellow!10}   &\cellcolor{white!20}\scriptsize{$gcd$}&\cellcolor{white!20}\scriptsize \text{Greatest common divisor}\\
%

\cellcolor{yellow!10}\multirow{-34}{*}{\rotatebox[origin=c]{90}{\cellcolor{yellow!10}\scriptsize{ {Generic}}}}
  \cellcolor{yellow!10}   &\cellcolor{gray!20}\scriptsize{$\negl$}&\cellcolor{gray!20}\scriptsize \text{Negligible function}\\
%
     \hline
%%%%%%%%%%%%


%\end{tabular}
%}
%\scalebox{.668}{
%\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|} 
%%%%%%%%%%%
%\hline 
%\multicolumn{1}{|c|}{\rotatebox[origin=c]{45}{\cellcolor{yellow!10}\scriptsize{ {Setting}}}}&\cellcolor{yellow!10} \scriptsize{Symbol}&\cellcolor{yellow!10} \scriptsize{Description}\\

     
\cellcolor{yellow!10}&\cellcolor{white!20}\scriptsize$\SCpc$&\cellcolor{white!20}\scriptsize \text{Prisoner's Contract}\\   

\cellcolor{yellow!10}&\cellcolor{gray!20}\scriptsize$\SCcc$&\cellcolor{gray!20}\scriptsize \text{Colluder’s Contract}\\   

\cellcolor{yellow!10}&\cellcolor{white!20}\scriptsize$\SCtc$&\cellcolor{white!20}\scriptsize \text{Traitor's Contract}\\   
%
\cellcolor{yellow!10}&\scriptsize  \cellcolor{gray!20}\scriptsize$\cc$&\cellcolor{gray!20}\scriptsize \text{Server’s cost for computing a task}\\   
%
\cellcolor{yellow!10}&\cellcolor{white!20}\scriptsize$\chc$&\cellcolor{white!20}\scriptsize \text{Auditor's cost for resolving disputes
}\\   
%
\cellcolor{yellow!10}&\scriptsize  \cellcolor{gray!20}\scriptsize$\dc$&\cellcolor{gray!20}\scriptsize \text{Deposit a server pays to get the job}\\  
%
\cellcolor{yellow!10}&\cellcolor{white!20}\scriptsize$\wc$&\cellcolor{white!20}\scriptsize \text{Amount a server receives for completing the task}\\  
%
\multirow{-8}{*}{\rotatebox[origin=c]{90}{\cellcolor{yellow!10}\scriptsize{ {Counter}}}}
%
\multirow{-8}{*}{\rotatebox[origin=c]{90}{\scriptsize{ {Collusion}}}}
%
\multirow{-8}{*}{\rotatebox[origin=c]{90}{\scriptsize{ {Contracts}}}}
&\cellcolor{gray!20}\scriptsize$(pk, sk)$&\cellcolor{gray!20}\scriptsize \text{\scf's auditor's public-private key pair}\\  
 %
\hline 
%%%% End of Counter Collusion Contacts %%%%%

%%%%%%%.      F-PSI      %%%%%%

%\qinit: Initiation predicate


\cellcolor{yellow!10}&\cellcolor{white!20}\scriptsize$\scf$&\cellcolor{white!20}\scriptsize {\fpsi's smart contract}\\   
%
\cellcolor{yellow!10}&\cellcolor{gray!20}\scriptsize$\bm\omega, \bm\omega',\bm\rho  $&\cellcolor{gray!20}\scriptsize {Random poly. of degree} $d$\\   
 %
\cellcolor{yellow!10}&\cellcolor{white!20}\scriptsize$\bm\gamma, \bm\delta$&\cellcolor{white!20}\scriptsize {Random poly. of degree} $d+1$\\
%
\cellcolor{yellow!10}&\cellcolor{gray!20}\scriptsize$\bm\nu^{\st{{(C)}}}$&\cellcolor{gray!20}\scriptsize {Blinded poly. sent by each $C$ to \scf}\\ 
%  
\cellcolor{yellow!10}&\cellcolor{white!20}\scriptsize$\bm\phi$&\cellcolor{white!20}\scriptsize {Blinded poly. encoding the intersection}\\   
%
\cellcolor{yellow!10}&\cellcolor{gray!20}\scriptsize$\bm\chi$&\cellcolor{gray!20}\scriptsize {Poly. sent to \scf to identify misbehaving parties}\\ 
%
\cellcolor{yellow!10}&\cellcolor{white!20}\scriptsize$\bar L$&\cellcolor{white!20}\scriptsize {List of identified misbehaving parties}\\ 
%

%%%%%%%%%%%%%
\cellcolor{yellow!10}&\cellcolor{gray!20}\scriptsize&\cellcolor{gray!20}\scriptsize {A portion of a party's deposit into \scf}\\   

\cellcolor{yellow!10}&\multirow{-2}{*}{\cellcolor{gray!20}\scriptsize$\yc$}&\cellcolor{gray!20}\scriptsize{transferred to honest clients if it misbehaves}\\ 
%%%%%%




\cellcolor{yellow!10}&\scriptsize$mk$&\scriptsize{Master key of \prf}\\ 
%
\cellcolor{yellow!10}&\cellcolor{gray!20}\scriptsize$\qinit$&\cellcolor{gray!20}\scriptsize{Initiation predicate}\\ 
%
\cellcolor{yellow!10}&\scriptsize$\qdel$&\scriptsize{Delivery predicate}\\ 
%
\cellcolor{yellow!10}&\cellcolor{gray!20}\scriptsize$\qUnFAbt$&\cellcolor{gray!20}\scriptsize{UnFair-Abort predicate}\\ 

\multirow{-14}{*}{\rotatebox[origin=c]{90}{\cellcolor{yellow!10}\scriptsize{ {\withFai (\fpsi)}}}}
%
\cellcolor{yellow!10}&\scriptsize$\qFAbt$&\scriptsize{Fair-Abort predicate}\\ 
%

\hline 
%%%%%   End of F-PSI  %%%%

%%%%%%%    E-PSI    %%%%%%

\cellcolor{yellow!10}&\cellcolor{gray!20}\scriptsize$\SCe$&\cellcolor{gray!20}\scriptsize {\epsi's smart contract} \\   
 %
\cellcolor{yellow!10}&\cellcolor{white!20}\scriptsize$\dc'$&\cellcolor{white!20}\scriptsize {Extractor's deposit} \\
  %   
\cellcolor{yellow!10}&\cellcolor{gray!20}\scriptsize$\yc'$&\cellcolor{gray!20}\scriptsize {Each client's deposit into \scf}\\   
%
\cellcolor{yellow!10}&\cellcolor{white!20}\scriptsize$\lc$&\cellcolor{white!20}\scriptsize {Reward a client earns for an intersection element}\\   
%
\cellcolor{yellow!10}&\cellcolor{gray!20}\scriptsize$\rc$&\cellcolor{gray!20}\scriptsize {Extractor's cost for extracting an intersection element}\\  
%
\cellcolor{yellow!10}&\cellcolor{white!20}\scriptsize$\fc$&\cellcolor{white!20}\scriptsize {Shorthand for $\lc(m-1)$}\\ 
%
\cellcolor{yellow!10}&\cellcolor{gray!20}&\cellcolor{gray!20}\scriptsize{Price a buyer pays for an intersection element}\\ 
%
\cellcolor{yellow!10}&\multirow{-2}{*}{\cellcolor{gray!20}\scriptsize$\vc$}&\cellcolor{gray!20}\scriptsize{$\vc=m\cdot \lc+2 \rc$}\\ 
%
\cellcolor{yellow!10}&\scriptsize$mk'$&\scriptsize{Another master key of \prf}\\ 
%

\cellcolor{yellow!10}&\cellcolor{gray!20}\scriptsize$ct_{\st mk}$&\cellcolor{gray!20}\scriptsize {Encryption of $mk$ under $pk$}\\   
%            
\cellcolor{yellow!10}&\scriptsize$\qdelwr$&\scriptsize{Delivery-with-Reward predicate}\\ 

\multirow{-12}{*}{\rotatebox[origin=c]{90}{\cellcolor{yellow!10}\scriptsize{ {\withRew (\epsi)}}}}
%
\cellcolor{yellow!10}&\cellcolor{gray!20}\scriptsize$\qUnFAbtwr$&\cellcolor{gray!20}\scriptsize{UnFair-Abort-with-Reward predicate}\\ 



\hline  



%%%%%%%%%%%

\end{tabular}\label{table:notation-table}}}
\end{center}
\end{scriptsize}
%\vspace{-7.5mm}
\end{table}





==> CCS-24/old--Merkle-tree.tex <==
% !TEX root =main.tex


\section{Merkle Tree}\label{sec::merkle-tree}






A Merkle tree is a data structure that supports a compact commitment of a set of values/blocks.  As a result, it includes two parties, prover $\mathcal{P}$ and verifier $\mathcal{V}$. The  Merkle tree scheme includes three algorithms $(\mkgen, \mkprove,$ $\mkver)$, defined as follows: 

\begin{itemize}
%
\item[$\bullet$] The algorithm that constructs a Merkle tree, $\mkgen$, is run by $\mathcal{V}$. It takes  blocks, $u:=u_{\st 1},...,u_{\st n}$, as input. Then, it groups the blocks  in pairs. Next,   a collision-resistant hash function, $\mathtt{H}(.)$, is used to hash each pair. After that, the hash values are grouped in pairs and each pair is further hashed, and this process is repeated until only a single hash value, called ``root'', remains. This yields a  tree with the leaves corresponding to the input blocks and the root corresponding to the last remaining hash value. $\mathcal{V}$ sends the root to $\mathcal{P}$.
%
\item[$\bullet$] The proving algorithm, $\mkprove$, is run by $\mathcal{P}$. It takes a block index, $i$, and a tree as inputs. It outputs a vector proof, of  $\log_{\st 2}(n)$ elements. The proof asserts the membership of $i$-th block in the tree, and consists of all the sibling nodes on a path from the $i$-th block to the root of the Merkle tree (including $i$-th block). The proof is given to $\mathcal{V}$.
%
\item[$\bullet$] The verification algorithm, $\mkver$, is run by $\mathcal{V}$. It takes as an input $i$-th block, a proof, and the tree's root. It checks if the $i$-th block corresponds to the root. If the verification passes, it outputs $1$; otherwise, it outputs $0$.

\end{itemize}

The Merkle tree-based scheme has two properties: \emph{correctness} and \emph{security}. Informally, the correctness requires that if both parties run the algorithms correctly, then a proof is always accepted by  $\mathcal{V}$. The security requires that a computationally bounded malicious $\mathcal{P}$ cannot convince  $\mathcal{V}$ into accepting an incorrect proof, e.g., proof for a non-member block. The security relies on the assumption that it is computationally infeasible to find the hash function's collision. Usually, for the sake of simplicity, it is assumed that the number of blocks, $n$, is a power of $2$. The height of the tree, constructed on $m$ blocks, is $\log_{\st 2}(n)$. 

==> CCS-24/old-Unforgeable-polynomials.tex <==
% !TEX root =main.tex






\vspace{-2mm}

\subsection{Unforgeable Polynomials}

\vspace{-.5mm}

In this section, we introduce the new notion of unforgeable polynomials. Informally, an unforgeable polynomial embeds a secret factor.  To ascertain that an unforgeable polynomial has not been tampered with, a verifier can check if the polynomial is divisible by this secret factor. 

To transform an arbitrary polynomial $\bm\pi$ of degree $d$ into an unforgeable polynomial $\bm\theta$, one can (i) select three secret random polynomials $(\bm\zeta, \bm\omega, \bm \gamma)$ and (ii) compute $\bm\theta=\bm\zeta\cdot \bm\omega\cdot\bm \pi + \bm \gamma \bmod p$, where  $deg(\bm\zeta)= 1, deg(\bm\omega)=d,$ and   $deg(\bm\gamma)= 2d+1$. 

To verify whether $\bm\theta$ has been tampered with, a verifier (given $\bm\theta, \bm \gamma$, and $\bm\zeta$) can check if $\bm\theta-\bm \gamma$ is divisible by $\bm\zeta$. Informally, the security of an unforgeable polynomial states that an adversary (who does not know the three secret random polynomials) cannot tamper with an unforgeable polynomial without being detected, except with a negligible probability. Below, we formally state it. 

\vspace{-1mm}
\begin{theorem}[Unforgeable Polynomial]\label{proof::unforgeable-poly}
%Let polynomials $\zeta$ and $\gamma$ be two secret uniformly random polynomials (i.e., $\zeta, \gamma\stackrel{\st\$}\leftarrow \mathbb F_{\st p}[x]$),   $GCD(\zeta, \gamma)=1$, polynomial $\pi$ be an arbitrary polynomial,   $deg(\zeta)= 1, deg(\gamma)= d+1$,  $deg(\pi)=d$, and $p$ be a $\lambda$-bit prime number. Also, let polynomial $\theta$ be defined as  $\theta=\zeta\cdot \pi+ \gamma \bmod p$. Given $(\theta,\pi)$, the probability that a PPT adversary (which does not know $\zeta$ and $\gamma$) can forge $\theta$ to an arbitrary polynomial $\theta'$ such that  $\theta'\neq \theta$, $deg(\theta')\leq poly(\lambda)$, and $\zeta$ divides $\theta'-\gamma$ is negligible in the security parameter, i.e.,
%
Let polynomials $\bm\zeta$, $\bm\omega$, and $\bm\gamma$ be three secret uniformly random polynomials (i.e., $\bm\zeta,\bm\omega, \bm\gamma\stackrel{\st\$}\leftarrow \mathbb F_{\st p}[x]$), polynomial $\bm\pi$ be an arbitrary polynomial,   $deg(\bm\zeta)= 1,$ $ deg(\bm\omega)=d,  deg(\bm\gamma)= 2d+1$,  $deg(\bm\pi)=d$, and $p$ be a $\lambda$-bit prime number. Also, let polynomial $\bm\theta$ be defined as  $\bm\theta=\bm\zeta\cdot \bm\omega\cdot\bm \pi+\bm \gamma \bmod p$. Given $(\bm\theta,\bm\pi)$, the probability that an adversary (which does not know $\bm\zeta, \bm\omega$, and $\bm\gamma$) can forge $\bm\theta$ to an arbitrary polynomial $\bm\delta$ such that  $\bm\delta\neq \bm\theta$, $deg(\bm\delta)= const(\lambda)$, and $\bm\zeta$ divides $\bm\delta-\bm\gamma$ is negligible in the security parameter $\lambda$, i.e., 
%
$Pr[ \bm\zeta \ | \ (\bm\delta-\bm\gamma) ]\leq \negl(\lambda)$.

\end{theorem}


%\begin{proof}
%
%Let $\bm\tau=\bm\delta-\bm\gamma$ and $\bm\zeta=a\cdot x+b$. Since $\bm\gamma$ is a random polynomial of degree $2d+1$ and unknown to the adversary, given $(\bm\theta, \bm\pi)$,  the adversary cannot learn anything about the factor $\bm\zeta$; as from its point of view every polynomial of degree $1$ in $\mathbb{F}_{\st p}[X]$ is equally likely to be $\bm\zeta$. Moreover,  polynomial $\bm\tau$ has at most $Max\big(deg(\bm\delta), 2d+1\big)$ irreducible non-constant factors.  For $\bm\zeta $ to divide $\bm\tau$,  one of the factors of $\bm\tau$ must be equal to $\bm\zeta$. We  also know that $\bm\zeta$ has been picked uniformly at random (i.e., $a,b
%\stackrel{\st \$}\leftarrow \mathbb F_{\st p}$). Thus, the probability that $\bm\zeta $ divides $\bm\tau$ is negligible in the security parameter, $\lambda$. Specifically,
%
%$$Pr[ \bm\zeta \ | \ (\bm\delta-\bm\gamma)]\leq \frac{Max\big(deg(\bm\delta), 2d+1\big)} {2^{\st \lambda}}=\negl(\lambda)$$
%\end{proof} 

%$Max\big(deg(\theta'), d+1\big)$
 An interesting feature of an unforgeable polynomial is that the verifier can perform the check without needing to know the original polynomial $\bm\pi$. Another appealing feature of the unforgeable polynomial is that it supports \emph{linear combination} and accordingly \emph{batch verification}. Specifically, to turn $n$ arbitrary polynomials $[\bm\pi_{\st 1},..., \bm\pi_{\st n}]$ into unforgeable polynomials, one can construct  $\bm\theta_{\st i}=\bm\zeta\cdot \bm\omega_{\st i}\cdot \bm\pi_{\st i}+ \bm\gamma_{\st i} \bmod p$, where $\forall i, 1\leq i\leq n$.  
 
 

 
To check whether all polynomials $[\bm\theta_{\st 1},..., \bm\theta_{\st n}]$ are intact, a verifier can (i) compute their sum $\bm \chi=\sum\limits_{\st i=1}^{\st n}\bm\theta_{\st i}$ and (ii) check whether $\bm \chi- \sum\limits_{\st i=1}^{\st n}\bm\gamma_{\st i} $ is divisible by $\bm \zeta$.  Informally, the security of unforgeable polynomials states that an adversary (who does not know the three secret random polynomials for each $\bm\theta_{\st i}$) cannot tamper with any subset of the unforgeable polynomials without being detected, except with a negligible probability. We formally state it, below. 
 
 
\vspace{-1mm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{theorem}[Unforgeable Polynomials' Linear Combination]\label{Unforgeable-Polynomials-Linear-Combination}
%
 Let polynomial $\bm\zeta$ be a secret polynomial picked uniformly at random; also, let   $\vv{\bm\omega}=[\bm\omega_{\st 1},..., \bm\omega_{\st n}]$ and $\vv{\bm\gamma}=[\bm\gamma_{\st 1},..., \bm\gamma_{\st n}]$ be two vectors of secret uniformly random polynomials (i.e., ${\bm\zeta}, \bm\omega_{\st i}, \bm\gamma_{\st i} \stackrel{\st\$}\leftarrow \mathbb F_{\st p}[x]$),  $\vv{\bm\pi}=[\bm\pi_{\st 1},..., \bm\pi_{\st n}]$ be a vector of arbitrary polynomials,   $deg(\bm\zeta)= 1, deg(\bm\omega_{\st i})=d,  deg(\bm\gamma_{\st i})= 2d+1$,  $deg(\bm\pi_{\st i})=d$,  $p$ be a $\lambda$-bit prime number and $1\leq i \leq n$. Moreover, let polynomial $\bm\theta_{\st i}$ be defined as  $\bm\theta_{\st i}=\bm\zeta\cdot \bm\omega_{\st i}\cdot \bm\pi_{\st i}+ \bm\gamma_{\st i} \bmod p$, and $\vv{\bm\theta} = [\bm\theta_{\st 1},..., \bm\theta_{\st n}]$.  Given $(\vv{\bm\theta}, \vv{\bm\pi})$, the probability that an adversary (which does not know $\bm\zeta, \vv{\bm\omega}$, and $\vv{\bm\gamma}$) can forge $t$ polynomials, without loss of generality, say $\bm\theta_{\st 1},..., \bm\theta_{\st t} \in \vv{\bm\theta}$ to arbitrary polynomials $\bm\delta_{\st 1},..., \bm\delta_{\st t}$ such that   $\sum\limits_{\st j=1}^{\st t}\bm\delta_{\st j}\neq \sum\limits_{\st j=1}^{\st t}\bm\theta_{\st j}$, $deg(\bm\delta_{\st j})= const(\lambda)$, and $\bm\zeta$ divides $(\sum\limits_{\st j=1}^{\st t}\bm\delta_{\st j} + \sum\limits_{\st j=t+1}^{\st n}\bm\theta_{\st j} - \sum\limits_{\st j=1}^{\st n}\bm\gamma_{\st j} )$ is negligible in the security parameter $\lambda$, i.e.,  
%
$Pr[ \bm\zeta \ | \ (\sum\limits_{\st j=1}^{\st t}\bm\delta_{\st j} + \sum\limits_{\st j=t+1}^{\st n}\bm\theta_{\st j} - \sum\limits_{\st j=1}^{\st n}\bm\gamma_{\st j} ) ]\leq \negl(\lambda)$. 

\end{theorem}



%%%%
%\begin{proof}  
%This proof is a generalisation of that of Theorem \ref{proof::unforgeable-poly}.  
%Let $\bm\tau_{\st j}=\bm\delta_{\st j}-\bm\gamma_{\st j}$ and $\bm\zeta=a\cdot x+b$. Since  every $\bm\gamma_{\st j}$ is a random polynomial of degree $2d+1$ and unknown to the adversary, given $(\vv{\bm\theta}, \vv{\bm\pi})$,  the adversary cannot learn anything about the factor $\bm\zeta$. Each polynomial $\bm\tau_{\st j}$ has at most $Max\big(deg(\bm\delta_{\st j}), 2d+1\big)$ irreducible non-constant factors. 
%%
%%In order for $\bm\zeta$ to divide polynomial $\sum\limits_{\st j=1}^{\st t}\bm\delta_{\st j} + \sum\limits_{\st j=t+1}^{\st n}\bm\theta_{\st j} - \sum\limits_{\st j=1}^{\st n}\bm\gamma_{\st j}$  one of the factors of every $\bm\tau_{\st j}$ needs to equal $\bm\zeta$, where $1 \leq j \leq t$. 
%%
%We  know that $\bm\zeta$ has been picked uniformly at random (i.e., $a,b
%\stackrel{\st \$}\leftarrow \mathbb F_{\st p}$). Therefore, the probability that $\bm\zeta$ divides $\sum\limits_{\st j=1}^{\st t}\bm\delta_{\st j} + \sum\limits_{\st j=t+1}^{\st n}\bm\theta_{\st j} - \sum\limits_{\st j=1}^{\st n}\bm\gamma_{\st j}$ equals the probability that $\bm\zeta$ equals to one of the factors of  every $\bm\tau_{\st j}$, that is negligible in the security parameter. Concretely,
%
%
%$$Pr[ \bm\zeta \ | \ (\sum\limits_{\st j=1}^{\st t}\bm\delta_{\st j} + \sum\limits_{\st j=t+1}^{\st n}\bm\theta_{\st j} - \sum\limits_{\st j=1}^{\st n}\bm\gamma_{\st j} ) ]\leq  \frac{\prod \limits^{\st t}_{\st j=1}Max\big(deg(\bm\delta_{\st j}), 2d+1\big)} {2^{\st \lambda t}}=\negl(\lambda)$$
%%
%\end{proof} 


%It is not hard to see that, Theorem \ref{Unforgeable-Polynomials-Linear-Combination} is a generalisation of Theorem \ref{proof::unforgeable-poly}. 

\vspace{-1mm}

We refer readers to Appendix \ref{sec::proof-of-unforgeable-polys} for the proofs of theorems \ref{proof::unforgeable-poly} and \ref{Unforgeable-Polynomials-Linear-Combination}. In \withFai, we will use unforgeable polynomials (linear combinations) to let a smart contract efficiently check if the polynomials that the clients send to it are intact, i.e.,  are \vopr's outputs.









==> CCS-24/payment.tex <==
% !TEX root =main.tex




\item The parties are paid as follows. 
%
\begin{itemize}
%
\item[$\bullet$]  if all proofs of both extractors are valid, both extractors provided identical elements of the intersections (for each bin), and there is no traitor, then $\mathcal{SC}_{\st\epsi}$:
\begin{enumerate}
%
 \item takes $|S_{\st\cap}|\cdot m\cdot \lc$ amount from the buyer's deposit (in $\mathcal{SC}_{\st\epsi}$) and distributes it among all clients, except the buyer. 
 %
 \item calls \SCpc which returns the extractors' deposit (i.e., $\dc'$ amount each) and pays each extractor $|S_{\st\cap}|\cdot \rc$ amount, for doing their job correctly. 
  %
 \item checks if $|{ { {S}}}_{\scriptscriptstyle\cap}|<\Smin$. If the check passes, then it returns $(\Smin-|S_{\scriptscriptstyle\cap}|)\cdot \vc$ amount  to the buyer.
 %
 \end{enumerate}
% 
\item[$\bullet$] if both extractors failed to deliver any result, then $\mathcal{SC}_{\st\epsi}$:
%
\begin{enumerate}
%
\item refunds the buyer, by sending $\Smin\cdot \vc$ amount (deposited in $\mathcal{SC}_{\st\epsi}$) back to the buyer. 
%
\item retrieves each extractor's deposit (i.e., $\dc$ amount) from the \SCpc and distributes it among the rest of the clients (except the buyer and extractors).  
%
 \end{enumerate}
 %
 \item[$\bullet$]\label{smart-PSI-inconsistency} Otherwise (e.g., if some proofs are invalid, if an extractor's result is inconsistent with the other extractor's result, or there is a traitor), $\mathcal{SC}_{\st\epsi}$ invokes (steps 8.c and 9 of) \SCpc and its auditor to identify the misbehaving extractor, with the help of $ct_{\st mk}$ after decrypting it. $\mathcal{SC}_{\st\epsi}$ asks \SCpc to pay the auditor the total amount of $\chc$ taken from the deposit of the extractor(s) who provided incorrect result to $\mathcal{SC}_{\st\epsi}$. Moreover,
%

\begin{enumerate}
%
\item if \underline{both extractors cheated}:
%
\begin{enumerate}
%
\item\label{both-cheated-no-traitor} if there \underline{is no traitor}, then $\mathcal{SC}_{\st\epsi}$ refunds the buyer, by sending $\Smin\cdot \vc$ amount (deposited in $\mathcal{SC}_{\st\epsi}$) back to the buyer. It also distributes $2\cdot \dc'- \chc$ amount (taken from the extractors' deposit in \SCpc) among the rest of  the clients  (except the buyer and extractors). %The Prisoner's contract pays its dispute resolver $ch$ amount. 
%
%
\item if there \underline{is a traitor}, then:
%%%%%
\begin{enumerate}
%
%
\item\label{both-cheated-honest-traitor} if the traitor delivered a \underline{correct result} in \SCtc, $\mathcal{SC}_{\st\epsi}$ retrieves $\dc'-\dc$ amount from the other dishonest extractor's deposit (in \SCpc) and distributes it among the rest of the clients (except the buyer and dishonest extractor). It asks \SCpc to send $|S_{\st\cap}|\cdot \rc+\dc'+\dc-\chc$ amount to the traitor (via \SCtc). % and $\hat{ch}$ amount to the dispute resolver.
%
\SCtc refunds the traitor's deposit, i.e., $\chc$ amount. It refunds the buyer, by sending $\Smin\cdot \vc-|S_{\st\cap}|\cdot \rc$ amount (deposited in $\mathcal{SC}_{\st\epsi}$) to it.


 %Otherwise (i.e., if it delivered an incorrect result in the Traitor's contract), the Traitor's contract refunds the traitor's deposit (i.e., $ch$ amount).
%
\item if the traitor delivered an \underline{incorrect result} in \SCtc, $\mathcal{SC}_{\st\epsi}$ pays the buyer and rest of the clients in the same way it does in step \ref{both-cheated-no-traitor}. 
%
%distributes $2\cdot \hat d- \hat{ch}$ amount (taken from the extractors deposit in the Prisoner's contract) among the rest of the clients (except the buyer and extractors). 
%
%The Prisoner's contract pays its dispute resolver $\hat{ch}$ amount.
%
\SCtc refunds the traitor,  $\chc$ amount.  %It refunds the buyer, by sending ${\resizeT {\textit {S}}}_{\resizeS {\textit  min}}\cdot v$ amount (deposited in $\mathcal{SC}_{\resizeS {\textit  {EXT}}}$) back to the buyer.


%
\end{enumerate}
%%%%%
\end{enumerate}
%
\item if \underline{one of the extractors cheated}: 
%
\begin{enumerate}
%
\item if there \underline{is no traitor},  $\mathcal{SC}_{\st\epsi}$ calls \SCpc that (a) returns the honest extractor's deposit ($\dc'$ amount), (b) pays this extractor $|S_{\st\cap}|\cdot \rc$ amount, for doing its job honestly, and (c) pays this extractor $ \dc-\chc$ amount taken from the dishonest extractor's deposit. 
%
%and (d) pays its dispute resolver $\hat {ch}$ amount taken from the dishonest extractor's deposit. 
%
%Also, $\mathcal{SC}_{\resizeS {\textit  {EXT}}}$ sends ${\resizeT {\textit {S}}}_{\resizeS {\textit  min}}\cdot v-|S_{\st\cap}|\cdot r$ amount (deposited in $\mathcal{SC}_{\resizeS {\textit  {EXT}}}$) back to the buyer.
%
 $\mathcal{SC}_{\st\epsi}$ pays the buyer and other clients in the same way it does in step \ref{both-cheated-honest-traitor}. 
 
 % $\mathcal{SC}_{\st\epsi}$ compensates the buyer and other clients in a manner consistent with step


% It retreives  $\hat d - \hat c - \hat{ch}$ amount from the dishonest extractor's deposit (in the Prisoner’s contract) and distributes it among the rest of clients (except the buyer and dishonest extractor). %
%
\item if there \underline{is a traitor}
%
%%%%%


\begin{enumerate}[leftmargin=2mm]
%
\item\label{one-cheated-exists-traitor-honest-traitor}  if the traitor delivered a \underline{correct result} in \SCtc (but  cheated in $\mathcal{SC}_{\st\epsi}$),  $\mathcal{SC}_{\st\epsi}$ calls \SCpc that (a) returns the other honest extractor's deposit ($\dc'$ amount), (b) pays the honest extractor $|S_{\st\cap}|\cdot \rc$ amount taken from the buyer's deposit, for doing its job honestly,  (c) pays the honest extractor $\dc- \chc$ amount taken from the traitor's deposit,  
%
%(d) pays its dispute resolver $\hat{ch}$ amount taken from the traitor extractor's deposit (deposited in $\mathcal{SC}_{\resizeS {\textit  {EXT}}}$), 
%
 (d)
 pays to the traitor $|S_{\st\cap}|\cdot \rc$ amount taken from the buyer’s deposit (via the \SCtc), and (e) refunds the traitor $\dc'-\dc$ amount taken from its own deposit.  \SCtc refunds the traitor's deposit (i.e., $\chc$ amount).  $\mathcal{SC}_{\st\epsi}$ takes $|S_{\st\cap}|\cdot m\cdot \lc$ amount from the buyer's deposit (in $\mathcal{SC}_{\st\epsi}$) and distributes it among all clients, except the buyer. If $|{ { {S}}}_{\scriptscriptstyle\cap}|<\Smin$,   $\mathcal{SC}_{\st\epsi}$ returns $(\Smin-|{ { {S}}}_{\scriptscriptstyle\cap}|)\cdot \vc$ amount (deposited in $\mathcal{SC}_{\st\epsi}$)  to the buyer. 
 
 
%
\item  if the traitor delivered an \underline{incorrect result} in \SCtc (and it cheated in $\mathcal{SC}_{\st\epsi}$), then $\mathcal{SC}_{\st\epsi}$ pays the honest extractor in the same way it does in step \ref{one-cheated-exists-traitor-honest-traitor}.  
%
%calls Prisoner's contract that (a) returns the other honest extractor's deposit (i.e., $\hat d$ amount), (b) pays the honest extractor $|S_{\st\cap}|\cdot r$ amount, for doing its job honestly, and (c) pays the honest extractor $\hat c$ amount taken from the traitor extractor's deposit. 
%
%, and  (d) pays its dispute resolver $\hat{ch}$ amount taken from the traitor extractor's deposit (deposited in $\mathcal{SC}_{\resizeS {\textit  {EXT}}}$). 
%
\SCtc refunds the traitor's deposit, i.e., $\chc$ amount. 
%
%$\mathcal{SC}_{\resizeS {\textit  {EXT}}}$ takes ${\resizeT {\textit {S}}}_{\resizeS {\textit  min}} \cdot f$ amount from the traitor's deposit (in $\mathcal{SC}_{\resizeS {\textit  {EXT}}}$) and distributes it among all clients, except the buyer and traitor. 
%
%Also, $\mathcal{SC}_{\resizeS {\textit  {EXT}}}$ sends ${\resizeT {\textit {S}}}_{\resizeS {\textit  min}}\cdot v-|S_{\st\cap}|\cdot r$ amount (deposited in $\mathcal{SC}_{\resizeS {\textit  {EXT}}}$) back to the buyer. 
%
Also, $\mathcal{SC}_{\st\epsi}$ pays the buyer and the rest of the clients in the same way it does in step \ref{both-cheated-honest-traitor}.


%
\end{enumerate}


\end{enumerate}

\end{enumerate}
\end{itemize}



%
%\begin{enumerate}
%
%\item fully refunds the buyer, as before.
%%
%\item calls Prisoner's contract that (a) returns the honest extractor's deposit (i.e., $\hat d$ amount), (b) pays this extractor $|S_{\st\cap}|\cdot r$ amount, for doing its job honestly,  (c) pays this extractor $\hat c$ amount taken from the dishonest extractor's deposit, and (d) pays its dispute resolver $ch$ amount taken from the dishonest extractor's deposit.
%%
%\item retrieves $\hat d-\hat c- ch$ amount from dishonest extractor's deposit (in the Prisoner's contract) and distributes it among the rest of the clients (except the buyer and dishonest extractor). 
%
%\end{enumerate}
%

 
 
 %%%%%%%%%%%. without Traitor
% \item Otherwise (e.g., if some proofs are invalid or if an extractor's result is inconsistent with the other extractor's result), $\mathcal{SC}_{\resizeS {\textit  {EXT}}}$ invokes (steps 8.c and 9 of) the Prisoner's contract to identify the misbehaving extractor. 
%%
%
%\begin{itemize}
%%
%\item[$\bullet$] if both extractors cheated, then $\mathcal{SC}_{\resizeS {\textit  {EXT}}}$:
%%
%\begin{enumerate}
%%
%\item refunds the buyer, by sending ${\resizeT {\textit {S}}}_{\resizeS {\textit  min}}\cdot v$ amount (deposited in $\mathcal{SC}_{\resizeS {\textit  {EXT}}}$) back to the buyer.
%%
%\item retrieves $\hat d-ch$ amount from each extractor's deposit (in the Prisoner's contract) and distributes it among the rest of the clients (except the buyer and extractors). The Prisoner's contract pays its dispute resolver $ch$ amount for each dishonest extractor. 
%%
%\end{enumerate}
%%
%\item[$\bullet$] if one of the extractors cheated, then $\mathcal{SC}_{\resizeS {\textit  {EXT}}}$:
%%
%\begin{enumerate}
%%
%\item fully refunds the buyer, as before.
%%
%\item calls Prisoner's contract that (a) returns the honest extractor's deposit (i.e., $\hat d$ amount), (b) pays this extractor $|S_{\st\cap}|\cdot r$ amount, for doing its job honestly,  (c) pays this extractor $\hat c$ amount taken from the dishonest extractor's deposit, and (d) pays its dispute resolver $ch$ amount taken from the dishonest extractor's deposit.
%%
%\item retrieves $\hat d-\hat c- ch$ amount from dishonest extractor's deposit (in the Prisoner's contract) and distributes it among the rest of the clients (except the buyer and dishonest extractor). 
%%
%\end{enumerate}
%%
%\end{itemize}








==> CCS-24/performance-tables.tex <==
% !TEX root =U-PSI.tex

\section{Performance Evaluation:  Run-time Details}\label{perftables}


%All experiments were conducted on a macOS laptop, with an Intel $i5@2.3$ GHz CPU, and $16$ GB RAM. U-PSI  implementation utilises Cryptopp\footnote{https://www.cryptopp.com/}, NTL\footnote{https://www.shoup.net/ntl/} , and Bloom Filter\footnote{http://www.partow.net/programming/bloomfilter/index.html} libraries  for the cryptographic primitives,  polynomial factorizations and checking elements membership respectively. In the experiments,  the probability of  bins overflow in the hash table, for both U-PSI and \cite{eopsi}, and false positive in the Bloom filters, for U-PSI, is set to $2^{\scriptscriptstyle -40}$. Furthermore, the   error probability in the padding scheme, for \cite{eopsi}, is also set to $2^{\scriptscriptstyle -40}$  that results in padding size in the range $[52,63]$ for the above  set size  range.  To achieve an optimal performance, similar to \cite{eopsi}, we set bin capacity to $d=100$. These choices of the hash table parameters, according to inequality \ref{},   leads to the hash table length in the range $[30,41943]$. 


\vspace{-9mm}



\begin{table*}[!htbp]
\begin{footnotesize}
\begin{center}
\caption{\small Update run-time comparison (in sec.)}\label{tbl::update} 


\renewcommand{\arraystretch}{1.3}

\begin{tabular}{|c|ccccccccccc|c|c} 
\hline 
%{\rowcolors{2}{blue!80!gray!18}{blue!10!gray!18}
\cellcolor{gray!20} \scriptsize \textbf{Protocols} &\cellcolor{gray!20} $2^{\scriptscriptstyle 10}$ &\cellcolor{gray!20}  $2^{\scriptscriptstyle 11}$&  \cellcolor{gray!20}$2^{\scriptscriptstyle 12}$&\cellcolor{gray!20}  $2^{\scriptscriptstyle 13}$&\cellcolor{gray!20} $2^{\scriptscriptstyle 14}$&\cellcolor{gray!20}   $2^{\scriptscriptstyle 15}$&\cellcolor{gray!20}  $2^{\scriptscriptstyle 16}$&\cellcolor{gray!20}   $2^{\scriptscriptstyle 17}$& \cellcolor{gray!20}  $2^{\scriptscriptstyle 18}$& \cellcolor{gray!20} $2^{\scriptscriptstyle 19}$&\cellcolor{gray!20}  $2^{\scriptscriptstyle 20}$ \\
    \hline
    
    \hline



\cellcolor{cyan!20}  \scriptsize \cite{eopsi}:&\cellcolor{cyan!20} 0.1&\cellcolor{cyan!20} 0.12&\cellcolor{cyan!20}  0.17&\cellcolor{cyan!20} 0.26&\cellcolor{cyan!20}  0.46&\cellcolor{cyan!20}  0.79 &\cellcolor{cyan!20}  2.05&\cellcolor{cyan!20}  4.71  &\cellcolor{cyan!20} 10.83 &\cellcolor{cyan!20} 15.49 & \cellcolor{cyan!20} 36.28    \\

\cellcolor{white!20}  \scriptsize U-PSI 40-bit: &\cellcolor{white!20}   &\cellcolor{white!20}   &\cellcolor{white!20} &\cellcolor{white!20}   &\cellcolor{white!20} &\cellcolor{white!20}$\leftarrow$ 0.056 $\rightarrow$ &\cellcolor{white!20} &\cellcolor{white!20} &\cellcolor{white!20}   &\cellcolor{white!20}  &\cellcolor{white!20}  \\ 

   \cellcolor{cyan!20}\scriptsize U-PSI 60-bit:      &\cellcolor{cyan!20} &\cellcolor{cyan!20} &\cellcolor{cyan!20}  &\cellcolor{cyan!20}  &\cellcolor{cyan!20} &\cellcolor{cyan!20} $\leftarrow$ 0.063$\rightarrow$ &\cellcolor{cyan!20} &\cellcolor{cyan!20}&\cellcolor{cyan!20} &\cellcolor{cyan!20} &\cellcolor{cyan!20}  \\ 
       \hline





\end{tabular}
\end{center}
\end{footnotesize}
\end{table*}







%\begin{table*}[!htbp]
%\begin{footnotesize}
%\begin{center}
%\caption{Update run-time comparison (in sec.)}\label{tbl::update} 
%
%
%\renewcommand{\arraystretch}{1.3}
%
%\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c} 
%\hline 
%%{\rowcolors{2}{blue!80!gray!18}{blue!10!gray!18}
%\cellcolor{gray!20} \scriptsize \textbf{Protocols} &\cellcolor{gray!20} $2^{\scriptscriptstyle 10}$ &\cellcolor{gray!20}  $2^{\scriptscriptstyle 11}$&  \cellcolor{gray!20}$2^{\scriptscriptstyle 12}$&\cellcolor{gray!20}  $2^{\scriptscriptstyle 13}$&\cellcolor{gray!20} $2^{\scriptscriptstyle 14}$&\cellcolor{gray!20}   $2^{\scriptscriptstyle 15}$&\cellcolor{gray!20}  $2^{\scriptscriptstyle 16}$&\cellcolor{gray!20}   $2^{\scriptscriptstyle 17}$& \cellcolor{gray!20}  $2^{\scriptscriptstyle 18}$& \cellcolor{gray!20} $2^{\scriptscriptstyle 19}$&\cellcolor{gray!20}  $2^{\scriptscriptstyle 20}$ \\
%    \hline
%    
%    \hline
%
%
%
%\cellcolor{cyan!20}  \scriptsize \cite{eopsi}:&\cellcolor{cyan!20} 0.1&\cellcolor{cyan!20} 0.12&\cellcolor{cyan!20}  0.17&\cellcolor{cyan!20} 0.26&\cellcolor{cyan!20}  0.46&\cellcolor{cyan!20}  0.79 &\cellcolor{cyan!20}  2.05&\cellcolor{cyan!20}  4.71  &\cellcolor{cyan!20} 10.83 &\cellcolor{cyan!20} 15.49 & \cellcolor{cyan!20} 36.28    \\
%
%\cellcolor{white!20}  \scriptsize U-PSI 40-bit: &\cellcolor{white!20} 1.75  &\cellcolor{white!20}  1.75 &\cellcolor{white!20} 1.75&\cellcolor{white!20} 1.75  &\cellcolor{white!20}1.75 &\cellcolor{white!20}1.75&\cellcolor{white!20} 1.75 &\cellcolor{white!20} 1.75&\cellcolor{white!20} 1.75  &\cellcolor{white!20} 1.75 &\cellcolor{white!20} 1.75 \\ 
%
%   \cellcolor{cyan!20}\scriptsize U-PSI 60-bit:      &\cellcolor{cyan!20}1.87 &\cellcolor{cyan!20}1.87 &\cellcolor{cyan!20}1.87  &\cellcolor{cyan!20}1.87  &\cellcolor{cyan!20}1.87 &\cellcolor{cyan!20}1.87  &\cellcolor{cyan!20}1.87 &\cellcolor{cyan!20}1.87 &\cellcolor{cyan!20}1.87 &\cellcolor{cyan!20}1.87 &\cellcolor{cyan!20}1.87  \\ 
%       \hline
%
%
%
%
%
%\end{tabular}
%\end{center}
%\end{footnotesize}
%\end{table*}

\vspace{-15mm}


\begin{table*}[!htbp]
\begin{footnotesize}
\begin{center}
\caption{ \small PSI computation run-time comparison: breakdown by step (in sec.)}\label{tbl::PSI} 


\renewcommand{\arraystretch}{1.3}

\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c} 
\hline 
%{\rowcolors{2}{blue!80!gray!18}{blue!10!gray!18}
\cellcolor{gray!20}\scriptsize \textbf{Phases} &\cellcolor{gray!20} \scriptsize \textbf{Protocols} &\cellcolor{gray!20} $2^{\scriptscriptstyle 10}$ &\cellcolor{gray!20}  $2^{\scriptscriptstyle 11}$&  \cellcolor{gray!20}$2^{\scriptscriptstyle 12}$&\cellcolor{gray!20}  $2^{\scriptscriptstyle 13}$&\cellcolor{gray!20} $2^{\scriptscriptstyle 14}$&\cellcolor{gray!20}   $2^{\scriptscriptstyle 15}$&\cellcolor{gray!20}  $2^{\scriptscriptstyle 16}$&\cellcolor{gray!20}   $2^{\scriptscriptstyle 17}$& \cellcolor{gray!20}  $2^{\scriptscriptstyle 18}$& \cellcolor{gray!20} $2^{\scriptscriptstyle 19}$&\cellcolor{gray!20}  $2^{\scriptscriptstyle 20}$ \\
    \hline
    
    \hline
\NameEntry{\center \scriptsize Data \\ \scriptsize Preparation for \\ \scriptsize   Outsourcing}
 \multirow{4}{*}&\cellcolor{cyan!20}  \scriptsize U-PSI 40-bit: &\cellcolor{cyan!20} 0.17&\cellcolor{cyan!20}  0.3&\cellcolor{cyan!20}  0.6&\cellcolor{cyan!20}  1.4 &\cellcolor{cyan!20}  2.8 &\cellcolor{cyan!20}  5.6  &\cellcolor{cyan!20}  14&\cellcolor{cyan!20}  44  &\cellcolor{cyan!20}  58 &\cellcolor{cyan!20}  121& \cellcolor{cyan!20} 240\\
    \cline{2-13}
 &\cellcolor{white!20}\scriptsize U-PSI 60-bit:&\cellcolor{white!20} 0.18  &\cellcolor{white!20}  0.3 &\cellcolor{white!20}  0.6&\cellcolor{white!20} 1.4  &\cellcolor{white!20} 2.8 &\cellcolor{white!20} 5.7  &\cellcolor{white!20} 14  &\cellcolor{white!20} 46 &\cellcolor{white!20} 60  &\cellcolor{white!20} 128 &\cellcolor{white!20} 253 \\ 
    \cline{2-13}
    &\cellcolor{cyan!20}\scriptsize \cite{eopsi}:&\cellcolor{cyan!20}0.7  &\cellcolor{cyan!20}0.8  &\cellcolor{cyan!20}1  &\cellcolor{cyan!20}1.5  &\cellcolor{cyan!20}3.4 &\cellcolor{cyan!20}8.8  &\cellcolor{cyan!20}15 &\cellcolor{cyan!20}48&\cellcolor{cyan!20}63 &\cellcolor{cyan!20}131 &\cellcolor{cyan!20}256   \\ 
       \hline


    \hline
\NameEntry{\center \scriptsize Client-side \\ \scriptsize Computation \\ \scriptsize  Delegation}
%\makecell{\scriptsize Computation \\ \scriptsize  Delegation}
    \multirow{3}{*}%{\scriptsize Computation Delegation}
    &\cellcolor{white!20} \scriptsize U-PSI 40-bit: &\cellcolor{white!20}  0.2  &\cellcolor{white!20}  0.3 &\cellcolor{white!20}  0.7 &\cellcolor{white!20} 1.5  &\cellcolor{white!20}  3.1 &\cellcolor{white!20}  6.4 &\cellcolor{white!20}  16 &\cellcolor{white!20}  32  &\cellcolor{white!20} 68  &\cellcolor{white!20}  121 &\cellcolor{white!20}  294  \\
    \cline{2-13}
    &\cellcolor{cyan!20}\scriptsize U-PSI 60-bit:&\cellcolor{cyan!20}  0.2&\cellcolor{cyan!20}0.4  &\cellcolor{cyan!20}0.7 &\cellcolor{cyan!20}  1.6  & \cellcolor{cyan!20}  3.3 &\cellcolor{cyan!20} 6.5  &\cellcolor{cyan!20}17 &\cellcolor{cyan!20}35 & \cellcolor{cyan!20}70  &\cellcolor{cyan!20} 141 &\cellcolor{cyan!20} 307  \\ 
    \cline{2-13}
    &\cellcolor{white!20}\scriptsize \cite{eopsi}: &\cellcolor{white!20}  0.4  &\cellcolor{white!20}  0.7 &\cellcolor{white!20} 1.5  &\cellcolor{white!20}   2.9&\cellcolor{white!20} 5.9 &\cellcolor{white!20} 11.9  &\cellcolor{white!20}  32 &\cellcolor{white!20}   63&\cellcolor{white!20} 129&\cellcolor{white!20} 268 &\cellcolor{white!20} 555 \\ 

    \hline


    \hline
\NameEntry{\center \scriptsize Cloud-side \\ \scriptsize  Computation}
%\makecell{\scriptsize Cloud-side \\ \scriptsize  Computation}
    \multirow{3}{*}%{\scriptsize Cloud-side computation}
    &\cellcolor{cyan!20}\scriptsize U-PSI 40-bit:  &\cellcolor{cyan!20} 0.18 &\cellcolor{cyan!20}0.3  &\cellcolor{cyan!20} 0.7  &\cellcolor{cyan!20}1.2  &\cellcolor{cyan!20}2.9  &\cellcolor{cyan!20}6 &\cellcolor{cyan!20}15 &\cellcolor{cyan!20} 30 & \cellcolor{cyan!20}71 &\cellcolor{cyan!20} 162&\cellcolor{cyan!20}473 \\
    \cline{2-13}
    &\cellcolor{white!20} \scriptsize U-PSI 60-bit: &\cellcolor{white!20} 0.19 &\cellcolor{white!20}  0.3  &\cellcolor{white!20} 0.7 &\cellcolor{white!20} 1.4  &\cellcolor{white!20} 3.3 &\cellcolor{white!20}  6.1 &\cellcolor{white!20}  15 &\cellcolor{white!20}  35 &\cellcolor{white!20}  72&\cellcolor{white!20}  164 &\cellcolor{white!20}  489 \\ 
    \cline{2-13}
    &\cellcolor{cyan!20}\scriptsize \cite{eopsi}: &\cellcolor{cyan!20} 0.4  &\cellcolor{cyan!20} 0.6 &\cellcolor{cyan!20} 1.4 &\cellcolor{cyan!20}  2.7&\cellcolor{cyan!20}5.4 & \cellcolor{cyan!20}10  &\cellcolor{cyan!20} 29&\cellcolor{cyan!20}57 &\cellcolor{cyan!20} 116 & \cellcolor{cyan!20}253&\cellcolor{cyan!20} 987  \\ 
       \hline


    \hline
\NameEntry{\center  \scriptsize Client-side \\ \scriptsize Result \\ \scriptsize  Retrieval}
%\makecell{\scriptsize Result \\   \scriptsize Retrieval}
    \multirow{3}{*} %{\scriptsize Result Retrieval}
    &\cellcolor{white!20}\scriptsize U-PSI 40-bit:  &\cellcolor{white!20}  0.59 &\cellcolor{white!20}  1.1 &\cellcolor{white!20}  2.2 &\cellcolor{white!20}  4.6&\cellcolor{white!20}  9.9 &\cellcolor{white!20}  18 &\cellcolor{white!20}   49&\cellcolor{white!20}  95  &\cellcolor{white!20} 195  &\cellcolor{white!20} 417 &\cellcolor{white!20}  1052 \\
    \cline{2-13}
   &\cellcolor{cyan!20} \scriptsize U-PSI 60-bit: &\cellcolor{cyan!20} 0.6  &\cellcolor{cyan!20}1.5   &\cellcolor{cyan!20} 2.8  &\cellcolor{cyan!20} 5.9 &\cellcolor{cyan!20}  12.5 &\cellcolor{cyan!20}24  &\cellcolor{cyan!20} 65 &\cellcolor{cyan!20} 131 &\cellcolor{cyan!20}  244 &\cellcolor{cyan!20} 568  &\cellcolor{cyan!20} 1389  \\ 
   \cline{2-13}
    &\cellcolor{white!20}\scriptsize \cite{eopsi}: &\cellcolor{white!20} 2.4  &\cellcolor{white!20}  5  &\cellcolor{white!20}   10.5 &\cellcolor{white!20}  20.8 &\cellcolor{white!20}    38.4 &\cellcolor{white!20}   81.2 &\cellcolor{white!20}  220   &\cellcolor{white!20}  424  &\cellcolor{white!20}  882  &\cellcolor{white!20}  1781  &\cellcolor{white!20} 3590 \\ 

	    \hline
	    
   \hline

\NameEntry{\center \scriptsize Total}

    \multirow{3}{*} 
    &\cellcolor{cyan!20}\scriptsize U-PSI 40-bit:   &\cellcolor{cyan!20}1.14  &\cellcolor{cyan!20} 2 &\cellcolor{cyan!20}4.2 &\cellcolor{cyan!20}8.7  & \cellcolor{cyan!20}18.7&\cellcolor{cyan!20}36  &\cellcolor{cyan!20}94 &\cellcolor{cyan!20}201  &\cellcolor{cyan!20}392 &\cellcolor{cyan!20} 821&\cellcolor{cyan!20}2059 \\
    \cline{2-13}
   &\cellcolor{white!20}\scriptsize U-PSI 60-bit: &\cellcolor{white!20} 1.17 &\cellcolor{white!20} 2.5 &\cellcolor{white!20} 4.8 &\cellcolor{white!20} 10.3 &\cellcolor{white!20}  21.9&\cellcolor{white!20} 42.3 &\cellcolor{white!20} 111 &\cellcolor{white!20} 247  &\cellcolor{white!20} 446&\cellcolor{white!20} 1001&\cellcolor{white!20} 2438 \\ 
   \cline{2-13}
    &\cellcolor{cyan!20}\scriptsize \cite{eopsi}: &\cellcolor{cyan!20} 3.9  &\cellcolor{cyan!20} 7.1 &\cellcolor{cyan!20} 14.3 &\cellcolor{cyan!20} 27.9  &\cellcolor{cyan!20} 53.1 &\cellcolor{cyan!20}  111.9 &\cellcolor{cyan!20}296&\cellcolor{cyan!20} 592  &\cellcolor{cyan!20}1190&\cellcolor{cyan!20}2433&\cellcolor{cyan!20} 5388 \\ 

    \hline

\end{tabular}
\end{center}
\end{footnotesize}
\end{table*}




%\begin{tikzpicture}
%%\begin{loglogaxis}[
%	xlabel=Cost,
%	ylabel=Error]
%\addplot[color=red,mark=x] coordinates {
%	(5,    8.31160034e-02)
%	(17,   2.54685628e-02)
%	(49,   7.40715288e-03)
%	(129,  2.10192154e-03)
%	(321,  5.87352989e-04)
%	(769,  1.62269942e-04)
%	(1793, 4.44248889e-05)
%	(4097, 1.20714122e-05)
%	(9217, 3.26101452e-06)
%};
%


%\legend{Case 1,Case 2}
%%\end{loglogaxis}
%\end{tikzpicture}







%
%\begin{tikzpicture}
%	\begin{semilogyaxis}[
%		xlabel=Index,ylabel=Value]
%		\addplot[color=black,mark=*] coordinates {
%		(2^10 ,8)
%		(2^11,16)
%		(2^12,88)
%		
%	};
%
%	\addplot[color=blue,mark=*] coordinates {
%		(2^10 ,8)
%		(2^11,16)
%		(2^12,88)
%	};
%	\end{semilogyaxis}%
%\end{tikzpicture}%



==> CCS-24/performance.tex <==
% !TEX root =U-PSI.tex


\section{Performance Evaluation}

We provide an empirical performance evaluation of U-PSI using  a prototype implementation developed in C++\footnote{\scriptsize U-PSI source code is available at  https://github.com/unknown-2018/U-PSI}. The implementation uses the efficient data representation presented in section \ref{BBF}. We compare the performance of U-PSI against  the protocol in \cite{eopsi}, as it is the fastest of the protocols we studied in section \ref{U-PSIEvaluation}. In order to do so, we have developed a prototype implementation of it\footnote{\scriptsize The update simulation for \cite{eopsi}  is available at \scriptsize https://github.com/unknown-2018/Update-Simulation} that allows clients to securely update their outsourced data by downloading and unblinding its entire outsourced data; updating a bin; re-encoding the elements of it; re-blinding the entire dataset; and uploading it to the cloud. More specifically, the implementations utilise  Cryptopp\footnote{\scriptsize https://www.cryptopp.com}, NTL\footnote{\scriptsize https://www.shoup.net/ntl} and Bloom Filter\footnote{\scriptsize http://www.partow.net/programming/bloomfilter/index.html} libraries  for   cryptographic primitives,  polynomial factorization and element membership checks respectively.

All experiments were conducted on a macOS laptop, with an Intel $i5@2.3$ GHz CPU, and $16$ GB RAM. In the experiments, we use randomly generated $40$-bit integers as set elements, and a set size in the range $[2^{\scriptscriptstyle 10},2^{\scriptscriptstyle 20}]$. The probability of bin overflow in the hash table, for both U-PSI and \cite{eopsi}, and false positive in the Bloom filters, for U-PSI, is set to $2^{\scriptscriptstyle -40}$. The error probability in the padding scheme, for \cite{eopsi}, is also set to $2^{\scriptscriptstyle -40}$  that results in padding size in the range $[52,63]$ for the above set size  range. To achieve an optimal performance, similar to \cite{eopsi}, we set bin capacity to $d=100$. These choices of hash table parameters, according to section \ref{PreliminaryHashTable}, lead to a hash table length in the range $[30,41943]$. We also use two different field sizes for U-PSI $40$ and $60$ bits. 

For the update operation in U-PSI, we measure the total run-time of four phases at the client-side: (a) computing an update query, (b) unblinding and decoding a bin, (c) applying the update, and (d) encoding and re-blinding the bin. For the update in \cite{eopsi}, we measure the total time when a client starts unblinding its dataset until it finishes re-blinding it. For the PSI computation in both protocols, we measure the total run-time of four phases: outsourcing, client-side PSI delegation (that includes both clients), cloud-side result computation and client-side result retrieval. Note that we include the run-time of outsourcing in the total time, although this step is performed only once by a client and  next time it delegates the PSI the protocol overall run-time would be lower. 

Fig. \ref{performance} depicts the  performance comparison between the two protocols  for update and PSI computation (see Tables \ref{tbl::update} and \ref{tbl::PSI}  in Appendix \ref{perftables} for a detailed run-time). The x-axes  in the figure are on a \emph{logarithmic scale}. As it is evident in the left-hand side graph in the figure, the update run-time for U-PSI is much lower than for \cite{eopsi}, especially for a larger set size. In particular, the update run-time for \cite{eopsi} grows from  $0.1$ to $36$ seconds when the set size increases from $2^{\scriptscriptstyle 10}$ to $2^{\scriptscriptstyle 20}$; whereas for U-PSI, the update run-time remains $0.056$ and $0.063$ seconds for all set sizes, when the field size is $40$ and $60$ bits, respectively. Therefore, the update in U-PSI is $1.7-642$ times and $1.5-571$ times faster than \cite{eopsi}, for field size $40$ and $60$ bits respectively.  The reason for this huge difference in the performance is that in \cite{eopsi} the client needs to unblind and re-blind all the bins in the hash table; whereas, in U-PSI such operations are carried out only on one bin. 
   
% the update performance of the  protocol in \cite{eopsi} is slightly better than U-PSI when the  set cardinality is smaller than $2^{\scriptscriptstyle 15}$. However, when the  cardinality is  greater than  $2^{\scriptscriptstyle 18}$ the  performance of U-PSI is much better than the other protocol. In particular, when the  size increases from $2^{\scriptscriptstyle 10}$ to $2^{\scriptscriptstyle 20}$,  the update run-time in \cite{eopsi} increases from $0.72$ to $36$ seconds, whereas in U-PSI it remains $1.75$ and $1.87$ seconds when the field size is $40$ and $60$ bits, respectively. Therefore, when the set cardinality is $2^{\scriptscriptstyle 20}$ the update run-time in U-PSI is  a factor of $19-20$ faster than \cite{eopsi}. The reason is that in U-PSI the client and cloud apply the update to only one bin, whereas in \cite{eopsi} the client has to decode and re-encode its entire data.  We expected that for \emph{all set sizes} the update in U-PSI has a lower run-time than in \cite{eopsi}. This can be due to an inefficient prototype implementation of the update  in U-PSI.   

%Here we compare the performance of our protocol against  the protocol proposed in \cite{eopsi}, as it is much faster than the other protocols that we studied in the previous section. Since this protocol  has been designed to  support  only PSI computation, we have also developed a prototype implementation that allows clients to securely update their outsourced date. To do that, a client needs to download and unblind its entire outsourced data,   update a bin, re-encode the elements of it, blind the entire dataset and then upload it to the cloud. We ran PSI and update operations for \cite{eopsi} using the same hash table parameters as those used in the U-PSI.  that results in padding size in the range $[52,63]$ for the above  set size  range. 


% Fig. \ref{performance} depicts the  performance comparison between the two protocols  for the update and PSI computation phases (see Tables \ref{tbl::update} and \ref{tbl::PSI}  in appendix\ref{} for a detailed run-time). The x-axes  in the figure are based on a  logarithmic scale. As it is evident in the left-hand side graph in the figure, the update performance of the  protocol in \cite{eopsi} is slightly better than U-PSI when the  set cardinality is smaller than $2^{\scriptscriptstyle 15}$. However, when the  cardinality is  greater than  $2^{\scriptscriptstyle 18}$ the  performance of U-PSI is much better than the other protocol. In particular, when the  size increases from $2^{\scriptscriptstyle 10}$ to $2^{\scriptscriptstyle 20}$,  the update run-time in \cite{eopsi} increases from $0.72$ to $36$ seconds, whereas in U-PSI it remains $1.75$ and $1.87$ seconds when the field size is $40$ and $60$ bits, respectively. Therefore, when the set cardinality is $2^{\scriptscriptstyle 20}$ the update run-time in U-PSI is  a factor of $19-20$ faster than \cite{eopsi}. The reason is that in U-PSI the client and cloud apply the update to only one bin, whereas in \cite{eopsi} the client has to decode and re-encode its entire data.  We expected that for \emph{all set sizes} the update in U-PSI has a lower run-time than in \cite{eopsi}. This can be due to an inefficient prototype implementation of the update  in U-PSI.   
 
 
Furthermore, as  the right-hand side graph in Fig. \ref{performance} indicates, the run-time for PSI computation in both protocols grows linearly when  the set size increases.  In particular, the PSI run-time  for \cite{eopsi}, grows from $3.9$ to $5388$ seconds when the set cardinality increases from $2^{\scriptscriptstyle 10}$ to $2^{\scriptscriptstyle 20}$.  Nevertheless, the growth for U-PSI is from $1.14$ to $2059$ seconds and from $1.17$ to $2438$ seconds for field size of $40$ and $60$ bits, respectively. Hence, the PSI computation run-time for U-PSI is a factor of $2.2-3.4$ faster than  \cite{eopsi}. The reason for this improvement is that in U-PSI all (arithmetic) operations, especially polynomial factorisations, are performed on a smaller field size. 

\vspace{-4mm}

\begin{figure}
\centering
\includegraphics[width=1 \textwidth]{pics/graphs2.pdf}
\caption{\small Update performance comparison between \cite{eopsi} and U-PSI, left hand side graph. PSI computation performance comparison between \cite{eopsi} and U-PSI, right hand size graph. }\label{performance}
\end{figure}

\vspace{-9mm}



%\begin{tikzpicture}
%%\begin{loglogaxis}[
%	xlabel=Cost,
%	ylabel=Error]
%\addplot[color=red,mark=x] coordinates {
%	(5,    8.31160034e-02)
%	(17,   2.54685628e-02)
%	(49,   7.40715288e-03)
%	(129,  2.10192154e-03)
%	(321,  5.87352989e-04)
%	(769,  1.62269942e-04)
%	(1793, 4.44248889e-05)
%	(4097, 1.20714122e-05)
%	(9217, 3.26101452e-06)
%};
%


%\legend{Case 1,Case 2}
%%\end{loglogaxis}
%\end{tikzpicture}







%
%\begin{tikzpicture}
%	\begin{semilogyaxis}[
%		xlabel=Index,ylabel=Value]
%		\addplot[color=black,mark=*] coordinates {
%		(2^10 ,8)
%		(2^11,16)
%		(2^12,88)
%		
%	};
%
%	\addplot[color=blue,mark=*] coordinates {
%		(2^10 ,8)
%		(2^11,16)
%		(2^12,88)
%	};
%	\end{semilogyaxis}%
%\end{tikzpicture}%



==> CCS-24/proof-of-poly-union.tex <==
% !TEX root =main.tex


\section{Proof of Theorem \ref{theorem:coef-poly-prod}}\label{sec::proof-of-poly-union}

Below, we restate the proof of Theorem \ref{theorem:coef-poly-prod}, taken from \cite{AbadiMZ21}.

\begin{proof}
Let $P=\{p_{\st 1},...,p_{\st t}\}$ and $Q=\{q_{\st 1},...,q_{\st t'}\}$ be the roots of polynomials $\mathbf{p}$ and   $\mathbf{q}$  respectively.  By the Polynomial Remainder Theorem,  polynomials $\mathbf{p}$ and $\mathbf{q}$  can be written as $\mathbf{p}(x)=\mathbf{g}(x)\cdot\prod\limits_{\st i=1}^{\st t}(x-p_{\st i})$ and $\mathbf{q}(x)=\mathbf{g}'(x)\cdot\prod\limits_{\st i=1}^{\st t'}(x-q_{\st i})$ respectively, where $\mathbf{g}(x)$ has degree $d-t$ and $\mathbf{g}'(x)$ has degree $d'-t'$. Let the product of the two polynomials be $\mathbf{r}(x)=\mathbf{p}(x)\cdot \mathbf{q}(x)$. For every $p_{\st i}\in P$, it holds  that $\mathbf{r}(p_{\st i})=0$. Because (a) there exists no non-constant polynomial in $\mathbb{F}_{\st p}[X]$ that has a multiplicative inverse (so it could cancel out factor $(x-p_{\st i})$ of $\mathbf{p}(x)$) and (b) $p_{\st i}$ is a root of $\mathbf{p}(x)$. The same argument  can be used to show for every $q_{\st i}\in Q$, it holds that $\mathbf{r}(q_{\st i})=0$. Thus, $\mathbf{r}(x)$ preserves  roots of  both  $\mathbf{p}$ and $\mathbf{q}$. Moreover, $\mathbf{r}$ does not have any other roots (than $P$ and $Q$). In particular, if $\mathbf{r}(\alpha)=0$, then $\mathbf{p}(\alpha)\cdot \mathbf{q}(\alpha)=0$. Since there is no non-trivial divisors of zero in $\mathbb{F}_{\st p}[X]$  (as it is an integral domain), it must hold that either $\mathbf{p}(\alpha)=0$ or $\mathbf{q}(\alpha)=0$. Hence, $\alpha\in P$ or $\alpha\in Q$.  %\hfill\(\Box\)
%
\end{proof}
\clearpage

%


==> CCS-24/related-work.tex <==
% !TEX root =main.tex


\vspace{-.5mm}
\section{Related Work}\label{sec::related-work}
\vspace{-1mm}

Since their introduction in \cite{DBLP:conf/eurocrypt/FreedmanNP04}, various PSIs have been designed, categorized into \textit{traditional} and \textit{delegated} types.  
%
In traditional PSIs, data owners compute the result interactively using their local data.
%
In this research domain, Raghuraman and Rindal \cite{RaghuramanR22} proposed two two-party PSIs, one secure against semi-honest/passive and the other against malicious/active adversaries. To date, these protocols are the fastest two-party PSIs. They rely on  Oblivious Key-Value Stores (OKVS) data structure and Vector Oblivious Linear Evaluation (VOLE). These PSIs' computation cost is $O(c)$, where $c$ is a set's cardinality.  They also impose $O(c\log c^{\st 2}+\kappa)$ and $O(c\cdot \kappa)$ communication costs in the semi-honest and malicious models respectively, 
where 
%$l$ is a set element's bit-size, and  
$\kappa$ is a security parameter.  
%
Also, researchers designed PSIs that enable multiple (i.e., more than two) parties to compute the intersection. The multi-party PSIs in  \cite{DBLP:conf/scn/InbarOP18,DBLP:conf/ccs/KolesnikovMPRT17} are secure against passive adversaries while those in \cite{Ben-EfraimNOP22,GhoshN19,ZhangLLJL19,DBLP:conf/ccs/KolesnikovMPRT17,NevoTY21} were designed to remain secure against active ones. 
%
%Abadi \et  \cite{AbadiMZ21} showed that the PSIs in  \cite{GhoshN19} are susceptible to several attacks.  
%
To date, the protocols in   \cite{DBLP:conf/ccs/KolesnikovMPRT17} and  \cite{NevoTY21} are the most  efficient multi-party PSIs  designed to be secure against passive and active adversaries respectively. They maintain security even if the majority of parties are corrupt.  The computation and communication complexities of the PSI in  \cite{DBLP:conf/ccs/KolesnikovMPRT17} are  $O(c\cdot m^{\st 2}+c\cdot m )$ and $O(c\cdot m^{\st 2})$. 
%
%Later, to achieve efficiency, Chandran \et \cite{ChandranD0OSS21} proposed a multi-party PSI that remains secure only if the minority of the parties is corrupt by a semi-honest adversary. 
%
The PSI in \cite{NevoTY21} has a parameter $t$ that determines how many parties can collude with each other and must be set before the protocol's execution, where $t\in [2, m)$.  
%
%The protocol divides the parties into three groups, clients: $A_{\st 1},..A_{\st m-t-1}$, leader: $A_{\st m-t}$, and servers: $A_{\st m-t+1},..A_{\st m}$. Each client needs to send a set of messages to every server and the leader which jointly compute the final result. Hence, 
%
Its computation and communication complexities are $O(c\cdot \kappa(m+t^{\st 2}-t(m+1)))$ and $O(c\cdot m\cdot \kappa)$ respectively.


Researchers proposed a ``fair'' two-party PSI in \cite{DBLP:conf/dbsec/DongCCR13},  ensuring that both parties receive the result or neither does if a malicious party aborts during the protocol's execution. It uses asymmetric-key primitives. The protocol's computation and communication complexities are $O(c^{\st 2})$ and $O(c)$  respectively. Since then, various fair two-party PSIs have been proposed, e.g.,  in \cite{DebnathD14,DebnathD16-,DebnathD16}. Currently, the fair PSI presented in \cite{DebnathD16} exhibits superior complexity compared to previous fair PSIs. It uses ElGamal encryption and zero-knowledge proofs. Its overhead is $O(c)$. But, its overall cost is high, due to its reliance on asymmetric key primitives. To date, there exists no fair multi-party PSI. \withFai stands as the inaugural fair multi-party PSI.



%But, its overall overhead is still high, as it relies on asymmetric key primitives, e.g.,  zero-knowledge proofs. So far, there exists no fair \emph{multi-party} PSI in the literature. Our \withFai is the first  fair multi-party PSI.%, which is also efficient.  


Delegated PSIs leverage cloud computing for computation and/or storage. These protocols can be further categorized into those that facilitate \textit{one-off} and \textit{repeated} delegation of PSI computation. The former, such as \cite{kamarascaling,kerschbaum12,c18}, cannot reuse their outsourced encrypted data and require clients to re-encode their data for each computation. The most efficient protocol among them is \cite{kamarascaling}, designed for the two-party setting, with an overhead of $O(c)$.  In contrast, protocols supporting repeated PSI delegation let clients outsource their encrypted data to the cloud just once and subsequently perform an unlimited number of computations on the outsourced data.
 %
 
The protocol in \cite{eopsi} is the first PSI that efficiently supports repeated delegation in the semi-honest model. It uses the polynomial representation of sets and hash tables. Its communication and computation complexities are $O(h\cdot d^{\st 2})$ and $O(h\cdot d)$ respectively, where $h$ is the total number of bins in the hash table, $d$ is a bin's capacity (often $d=100$), and $h\cdot d$ is linear with $c$.  
%
Recently, a multi-party PSI that supports repeated delegation and efficient \emph{updates} has been proposed in \cite{AbadiDMT22}. It is in the semi-honest model. It imposes $O(h\cdot d^{\st 2}\cdot m)$ and $O(h\cdot d\cdot m)$  computation and communication costs respectively, during the PSI computation. %It remains to be seen how a fair delegated PSI can be designed.










 
 
 

==> CCS-24/security-definition.tex <==
% !TEX root =U-PSI.tex


%\section{Security Definition}
%
%In this section, we provide the security definition of our protocol. There are two kinds of party involved in the protocol. Namely, (1) a set of clients $\{\resizeT {\textit A}_{\resizeS {\textit  1}},..., \resizeT {\textit A}_{\resizeS {\textit  m}}\}$ potentially malicious (i.e. active adversaries) and all may collude with each other, and (2) a non-colluding dealer: client $\resizeT {\textit D}$, potentially semi-honest (i.e. a passive adversary). In this work, we consider static adversary,  we assume there is an authenticated private (off-chain) channel between the clients and we consider a standard public blockchain, e.g. Ethereum.

==> CCS-24/securityproof.tex <==
% !TEX root =U-PSI.tex
\section{U-PSI Security Proof}\label{U-PSIProof}

In this section, we  sketch U-PSI's security proof  in the presence of static semi-honest adversaries. We conduct the security analysis for the three cases where one of the parties is corrupted at a time. 
%\begin{theorem-non}
\begin{theorem}
If $\mathtt{PRF}$ and $\mathtt{PRF}'$ are collision-resistant pseudorandom functions, and $\pi$ is a pseudorandom permutation, then U-PSI protocol is secure in the presence of a semi-honest adversary. 
\end{theorem}
%\end{theorem-non}

\vspace{-2mm}

%\newtheorem{prop2}{Proof}
%\begin{prop2} 

\begin{proof}
We will prove the theorem by considering in turn the case where each of the parties has been corrupted. In each case, we invoke the simulator with the corresponding party's input and output.  Our focus is on the case where party $A$ wants to engage in the computation of the intersection, i.e. it authorizes the computation. If party $A$ does not want to proceed with the protocol, the views can be simulated in the same way up to the point where the execution stops.


\
\vspace{-2mm}

\noindent\textbf{Case 1: Corrupted Cloud.} In this case, we show that given the leakage function we can construct a simulator $\textsf {\scriptsize SIM}_{\scriptscriptstyle C}$ that can produce a view computationally indistinguishable from the one in the real model. In the real execution, the cloud's view is:
\begin{equation*}
 \textsf {\scriptsize VIEW}^{\scriptscriptstyle\textsf { U-PSI}}_{\scriptscriptstyle C}(\Lambda, S^{\scriptscriptstyle (A)},S^{\scriptscriptstyle (B)})=\{\Lambda, r_{\scriptscriptstyle C}, \vv{\bm{po}}^{\scriptscriptstyle (A)},\vv{\bm{pl}}^{\scriptscriptstyle (A)}, \vv{\bm{po}}^{\scriptscriptstyle (B)},\vv{\bm{pl}}^{\scriptscriptstyle (B)}, (Q_{\scriptscriptstyle  1}, ..., Q_{\scriptscriptstyle  \Upsilon}),\Lambda \}.
\end{equation*}

In the above view, $r_{\scriptscriptstyle C}$ is the outcome of internal random coins of the cloud,  ($\forall I, I\in \{A, B\}$) $\vv{\bm{po}}^{\scriptscriptstyle (I)}$ are the permuted hash tables  containing the clients' blinded datasets and $\vv{\bm{pl}}^{\scriptscriptstyle (I)}$ are the permuted labels. Moreover, if  the query is for PSI delegation then
\begin{equation*}
 Q_{\scriptscriptstyle  i}=\{tk^{\scriptscriptstyle  (B)}, tk^{\scriptscriptstyle  (A)}, \textsf {\scriptsize \textbf{ID}}^{\scriptscriptstyle (A)},  \textsf {\scriptsize \textbf{ID}}^{\scriptscriptstyle (B)},  \vv{\bm{pm}}_{\scriptscriptstyle \mathtt{ A \rightarrow B}}, \textsf {\scriptsize \textbf{Compute}}\},
\end{equation*}
 otherwise (if the client $I$'s query is for update),  
\begin{equation*}
Q_{\scriptscriptstyle  i}=\{\vv{\bm{o}}^{\scriptscriptstyle (I)}_{\scriptscriptstyle j,c^{ {\text{\tiny (\textit{I})}}}_{\tiny j}}, l^{\scriptscriptstyle (I)}_{\scriptscriptstyle j},\textsf {\scriptsize \textbf{Update}}\}, 
\end{equation*}
for some $j, 1\leq j\leq h$.

%$\textsf {\scriptsize \textbf{ID}}^{\scriptscriptstyle (B)}$
Now we construct the simulator $\textsf {\scriptsize SIM}_{\scriptscriptstyle C}$ in the ideal model which executes as follows. 

\begin{packed_enum}
\item Creates an empty view and appends $\Lambda$ and uniformly random coin $r'_{\scriptscriptstyle C}$ to it. 
%\item Chooses  two random sets $S'^{\scriptscriptstyle (A)}$ and $S'^{\scriptscriptstyle (B)}$, such that $|S'^{\scriptscriptstyle (A)}|, |S'^{\scriptscriptstyle (B)}|<c$.

\item Uses the public parameters and the hash function to construct two hash tables $\mathtt{HT}'^{\scriptscriptstyle (A)}$ and $\mathtt{HT}'^{\scriptscriptstyle (B)}$. It fills each bin of the hash tables with $n$ uniformly random values picked from the field $\mathbb{F}_p$. So, each bin $\mathtt{HT}'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j}$ ($\forall I, I\in \{A,B\}$) contains a vector  $\vv{\bm{o}}'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j}$ of $n$ random values. 



%Then, it maps and insert each  element of the  sets $S'^{\scriptscriptstyle (A)}$ and $S'^{\scriptscriptstyle (B)}$ to the bins of the tables $\mathtt{HT}'^{\scriptscriptstyle (A)}$ and $\mathtt{HT}'^{\scriptscriptstyle (B)}$ respectively. So for every $I\in \{A,B\}$ does as the following. 

%\
%
%\vspace{-2mm}
%
%\begin{center}
%$\forall s'^{\scriptscriptstyle (I)}_{\scriptscriptstyle i}\in S'^{\scriptscriptstyle (I)}: \mathtt{H}( s'^{\scriptscriptstyle (I)}_{\scriptscriptstyle i})=j$, then $s'^{\scriptscriptstyle (I)}_{\scriptscriptstyle i}\rightarrow \mathtt{HT}'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j}$, where $1\leq j \leq h$ and $I\in \{A,B\}$
%\end{center}
%
%\
%
%\vspace{-2mm}


\item \label{labelGen}Assigns a pseudorandom label to each bin $\mathtt{HT}'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j}$ ($\forall I, I\in \{A,B\}$). To do so, it picks fresh label-keys, $lk'^{\scriptscriptstyle(I)}$, and computes the labels as $\forall I, I\in \{A,B\}$ and $\forall j,  1\leq j \leq h$ : $l'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j}=\mathtt{PRF}'(lk'^{\scriptscriptstyle (I)},j)$.




%\item \label{keygen} Assigns a key to each bin in the hash table by picking a master key $mk'^{\scriptscriptstyle (I)}$; and then generating $h$ pseudorandom values.  $\forall j, 1\leq j \leq h$: $k^{\scriptscriptstyle (I)}_{\scriptscriptstyle j}=\mathtt{PRF}(mk'^{\scriptscriptstyle (I)},j)$.



%\item  For every bin $\mathtt{HT}'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j}$ (where $1\leq j\leq h$ and $I\in \{A,B\}$), if it has less than $d$ set elements, pad it with dummy (or random) elements, $r'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j,i}$, to contain $d$ elements. Then, encode the elements as follows.



%\item For every occupied bin $\mathtt{HT}^{\scriptscriptstyle (I)}_{\scriptscriptstyle j}$, containing $d'$ set elements, encode the elements as follows.

%\begin{enumerate}
% \item  Constructs a polynomial representing the elements in the bin.
%
%\
%
%\vspace{-2mm}
%
%\begin{center}
%$\tau'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j}(x)=\prod\limits ^{\scriptscriptstyle d}_{\scriptscriptstyle i=1}(x-e'^{\scriptscriptstyle (I)}_{\scriptscriptstyle i})$, where $e'^{\scriptscriptstyle (I)}_{\scriptscriptstyle i} \in \mathtt{HT}'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j}$, $e'^{\scriptscriptstyle (I)}_{\scriptscriptstyle i}=s'^{\scriptscriptstyle (I)}_{\scriptscriptstyle i} $ or $e'^{\scriptscriptstyle (I)}_{\scriptscriptstyle i}=r'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j,i}$
%\end{center}
%
%\
%
%\vspace{-2mm}
%
%\item Represents $\tau'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j} (x)$ as point-value form, by evaluating it at every element $x_{\scriptscriptstyle i}\in\vv{\bm{x}}$. This yields a vector of  $\tau'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j} (x_{\scriptscriptstyle i})$, $1\leq i \leq n$.


%\item \label{blind} Blinds every value $\tau'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j} (x_{\scriptscriptstyle i})$. To do so, first generate a pseudorandom value $z'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j,c^{ {\text{\tiny (\textit{I})}}}_{\tiny j},i}=\mathtt{PRF}(k^{\scriptscriptstyle (I)}_{\scriptscriptstyle j},i)$, where key $k'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j}$ was generated in step b.\ref{keygen}. Then, computes $o'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j,c^{ {\text{\tiny (\textit{I})}}}_{\tiny j},i}$ as follow. $\forall i, 1\leq i\leq n: o'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j,c^{ {\text{\tiny (\textit{I})}}}_{\tiny j},i}=\tau'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j} (x_{\scriptscriptstyle i})+ z'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j,c^{ {\text{\tiny (\textit{I})}}}_{ j},i}$.



\item Constructs two vectors of the form   $[(\vv{\bm{o}}'^{\scriptscriptstyle (I)}_{\scriptscriptstyle 1},l'^{\scriptscriptstyle (I)}_{\scriptscriptstyle 1}),...,(\vv{\bm{o}}'^{\scriptscriptstyle (I)}_{\scriptscriptstyle h},l'^{\scriptscriptstyle (I)}_{\scriptscriptstyle h})]$ for each $I$, $I\in \{A,B\}$. Then, it randomly permutes each vector. Next,  it inserts each element  $\vv{\bm{o}}'^{\scriptscriptstyle (I)}_{\scriptscriptstyle g}$ ($\forall g, 1\leq g\leq h$) of the permuted vector into $\vv{\bm{po}}'^{\scriptscriptstyle (I)}$. Also, it inserts each element $l'^{\scriptscriptstyle (I)}_{\scriptscriptstyle g}$ of the permuted vector into $\vv{\bm{pl}}'^{\scriptscriptstyle (I)}$. Therefore, it has constructed four vectors: $\vv{\bm{po}}'^{\scriptscriptstyle (A)}$, $\vv{\bm{pl}}'^{\scriptscriptstyle (A)}$, $\vv{\bm{po}}'^{\scriptscriptstyle (B)}$ and   $\vv{\bm{pl}}'^{\scriptscriptstyle (B)}$. It appends the four vectors to the view.





%\item Picks two random keys $pk'^{\scriptscriptstyle (I)}$  ($\forall I, I\in \{A,B\}$), and constructs two permuted vectors, $\vv{\bm{po}}'^{\scriptscriptstyle (I)}=\pi(pk'^{\scriptscriptstyle (I)}, \vv{\bm{o}}'^{\scriptscriptstyle (I)})$ and $\vv{\bm{pl}}'^{\scriptscriptstyle (I)}=\pi(pk'^{\scriptscriptstyle (I)}, \vv{\bm{l}}'^{\scriptscriptstyle (I)})$, where $\vv{\bm{o}}'^{\scriptscriptstyle (I)}=[\vv{\bm{o}}'^{\scriptscriptstyle (I)}_{\scriptscriptstyle 1}, ..., \vv{\bm{o}}'^{\scriptscriptstyle (I)}_{\scriptscriptstyle h}]$ and  vector $\vv{\bm{l}}'^{\scriptscriptstyle (I)}$ contains the labels generated in  step \ref{labelGen}. Then, it inserts $\vv{\bm{po}}'^{\scriptscriptstyle (A)}$, $\vv{\bm{pl}}'^{\scriptscriptstyle (A)}$, $\vv{\bm{po}}'^{\scriptscriptstyle (B)}$ and   $\vv{\bm{pl}}'^{\scriptscriptstyle (B)}$ to its view. 

\item Given the leakage function $[\mathcal{M}^{\scriptscriptstyle (I)},\vv{\bm{T}}]$, it first uses each matrix $\mathcal{M}^{\scriptscriptstyle (I)}$ to construct the corresponding vector $\vv{\bm{v}}^{\scriptscriptstyle (I)}$ that will contain a set of labels $l'^{\scriptscriptstyle (I)}\in \vv{\bm{l}}'^{\scriptscriptstyle (I)}$, and has the same access pattern as the one indicated by the matrix. In order for it to generate this vector, it first constructs  vector $\vv{\bm{v}}^{\scriptscriptstyle (I)}$ of zeros, where $|\vv{\bm{v}}^{\scriptscriptstyle (I)}|=\textbf{p}$. Then, for every row $i$ ($1\leq i\leq \textbf{p}$) of the matrix $\mathcal{M}^{\scriptscriptstyle (I)}$, it performs the following:
\begin{packed_enum}
\item If there exists at least one element set to $1$ in the row and if the $i^{th}$ element in the vector $\vv{\bm{v}}^{\scriptscriptstyle (I)}$ is zero, then it finds a set $G$ such that $\forall g \in G: \mathcal{M}^{\scriptscriptstyle (I)}_{i,g}=1$. Next, it picks a label $l'^{\scriptscriptstyle (I)}\in \vv{\bm{l}}'^{\scriptscriptstyle (I)}$ and inserts it into all $i^{\scriptscriptstyle th}, g^{\scriptscriptstyle th}$ positions of the vector $\vv{\bm{v}}^{\scriptscriptstyle (I)}$. The label must be distinct from the ones used for the previous rows $i'$, where $i'<i$. Otherwise, if the $i^{th}$ element in the vector is non-zero,  it  moves on to the next row. 

\item If all the elements in the row are zero and if the $i^{\scriptscriptstyle th}$ element in the vector $\vv{\bm{v}}^{\scriptscriptstyle (I)}$ is zero, then it picks a label $l'^{\scriptscriptstyle (I)}\in \vv{\bm{l}}'^{\scriptscriptstyle (I)}$ and inserts it at position $i^{\scriptscriptstyle th}$ of the vector, where  the label is distinct from the ones used for the previous rows $i'$, where $i'<i$. Otherwise, if the $i^{\scriptscriptstyle th}$ element in the vector is non-zero,  it  moves on to the next row. 
\end{packed_enum}



\item  Uses $\vv{\bm{T}}$ and checks $T_{\scriptscriptstyle i}$ ( $\forall i, 1\leq i\leq \Upsilon$) as follows:

\begin{packed_enum}
\item if $T_{\scriptscriptstyle i}= \textsf {\scriptsize PSI-Com}$, then sets: 
\begin{equation*}
Q'_{\scriptscriptstyle  i}=\{tk'^{\scriptscriptstyle  (B)}, tk'^{\scriptscriptstyle  (A)},\textsf {\scriptsize \textbf{ID}}^{\scriptscriptstyle  (A)},  \textsf {\scriptsize \textbf{ID}}^{\scriptscriptstyle  (B)},  \vv{\bm{pm}}'_{\scriptscriptstyle \mathtt{ A \rightarrow B}}, \textsf {\scriptsize \textbf{Compute}}\}, 
\end{equation*}
where  $\vv{\bm{pm}}'_{\scriptscriptstyle \mathtt{ A \rightarrow B}}$ contains tuples $(l'^{\scriptscriptstyle  (A)}_{\scriptscriptstyle i},l'^{\scriptscriptstyle  (B)}_{\scriptscriptstyle i})$ randomly permuted. Also, $tk'^{\scriptscriptstyle  (B)}$ and $tk'^{\scriptscriptstyle  (A)}$ are fresh random keys,  and  labels $l'^{\scriptscriptstyle  (I)}_{\scriptscriptstyle i}$ were generated step \ref{labelGen}.  Next, it appends $Q'_{\scriptscriptstyle  i}$ to the view. 
\item if $T_{\scriptscriptstyle i}= \textsf {\scriptsize Upd}^{\scriptscriptstyle (I)}_{\scriptscriptstyle t}$, then sets: 
\begin{equation*}
Q'_{\scriptscriptstyle  i}=\{\vv{\bm{o}}''^{\scriptscriptstyle (I)}, l'^{\scriptscriptstyle (I)}_{\scriptscriptstyle t},\textsf {\scriptsize \textbf{Update}}\},
\end{equation*}
 where $\vv{\bm{o}}''^{\scriptscriptstyle (I)}$ contains $n$  uniformly random values picked from the field $\mathbb{F}_p$ and $l'^{\scriptscriptstyle (I)}_{\scriptscriptstyle t}$ is the $t^{\scriptscriptstyle th}$ element in the vector $\vv{\bm{v}}^{\scriptscriptstyle (I)}$. After that, it appends $Q'_{\scriptscriptstyle  i}$ to the view. 
\end{packed_enum}
\item Appends $\Lambda$ to its view and outputs the view.
\end{packed_enum}

We are ready now to show why the two views are indistinguishable.  In both views, the input and output parts (i.e. $\Lambda$) are identical and the random coins are both uniformly
random, and so they are indistinguishable. Each vector  $\vv{\bm{po}}^{\scriptscriptstyle (I)}_{\scriptscriptstyle i}\in \vv{\bm{po}}^{\scriptscriptstyle (I)}$, ($\forall i, 1\leq i\leq h$ and $\forall I, I\in \{A,B\}$), contains $n$ values blinded with  pseudorandom values (that are the outputs of a pseudorandom function), also each vector  $\vv{\bm{po}}'^{\scriptscriptstyle (I)}_{\scriptscriptstyle i}\in \vv{\bm{po}}'^{\scriptscriptstyle (I)}$ contains $n$ random values sampled uniformly from the same field. Since the blinded values and random values are not distinguishable, the elements of vectors $\vv{\bm{po}}^{\scriptscriptstyle (I)}$ and $\vv{\bm{po}}'^{\scriptscriptstyle (I)}$ are indistinguishable  too. Also,  labels  $l^{\scriptscriptstyle (I)}_{\scriptscriptstyle i} \in \vv{\bm{pl}}^{\scriptscriptstyle (I)}$ and $l'^{\scriptscriptstyle (I)}_{\scriptscriptstyle i} \in \vv{\bm{pl}}'^{\scriptscriptstyle (I)}$, ($\forall i, 1\leq i\leq h$ and $\forall I, I\in \{A,B\}$), are the outputs of a pseudorandom function and they are indistinguishable. Therefore, the elements of vectors $\vv{\bm{pl}}^{\scriptscriptstyle (I)}$ and $\vv{\bm{pl}}'^{\scriptscriptstyle (I)}$ are indistinguishable. Furthermore, since a pseudorandom permutation is indistinguishable from a  random permutation,  permuted vectors $\vv{\bm{po}}^{\scriptscriptstyle (I)}$ and $\vv{\bm{pl}}^{\scriptscriptstyle (I)} $, in the real model, and permuted vectors $\vv{\bm{po}}'^{\scriptscriptstyle (I)}$ and $\vv{\bm{pl}}'^{\scriptscriptstyle (I)} $, in the ideal model, are indistinguishable.


Since  sequence $ Q'_{\scriptscriptstyle 1}, ..., Q'_{\scriptscriptstyle \Upsilon}$ is generated given the leakage function, its access and query patterns are identical to the access and query patterns of $Q_{\scriptscriptstyle 1}, ..., Q_{\scriptscriptstyle \Upsilon}$.  Now we show that $Q_{\scriptscriptstyle i}$ is indistinguishable from $Q'_{\scriptscriptstyle i}$, ($\forall i, 1\leq i\leq \Upsilon$). First we consider the  case where $T_{\scriptscriptstyle i}= \textsf {\scriptsize PSI-Com}$. In this case,  keys $tk^{\scriptscriptstyle (I)}$ and $tk'^{\scriptscriptstyle (I)}$, ($\forall I, I\in \{A,B\}$), are random values, so they are indistinguishable. Also,  messages $\textsf {\scriptsize \textbf{ID}}^{\scriptscriptstyle  (A)}, \textsf {\scriptsize \textbf{ID}}^{\scriptscriptstyle  (B)}$ and $\textsf {\scriptsize \textbf{Compute}}$ are identical in both views.  Moreover, in the real model each pair in randomly permuted vector $\vv{\bm{pm}}_{\scriptscriptstyle \mathtt{ A \rightarrow B}}$ has the form $(l^{\scriptscriptstyle  (A)}_{\scriptscriptstyle g},l^{\scriptscriptstyle  (B)}_{\scriptscriptstyle g})$ where ($\forall g, 1\leq g\leq h $ and $\forall I, I \in \{A,B\}$) $l^{\scriptscriptstyle (I)}_{\scriptscriptstyle g} \in \vv{\bm{l}}^{\scriptscriptstyle (I)}$ and each $l^{\scriptscriptstyle (I)}_{\scriptscriptstyle g}$ is a pseudorandom string. Similarly, in the ideal model each pair in randomly permuted vector  $\vv{\bm{pm}}'_{\scriptscriptstyle \mathtt{ A \rightarrow B}}$ has the form $(l'^{\scriptscriptstyle  (A)}_{\scriptscriptstyle g'},l'^{\scriptscriptstyle  (B)}_{\scriptscriptstyle g'})$ where  $l'^{\scriptscriptstyle (I)}_{\scriptscriptstyle g'} \in \vv{\bm{l}}'^{\scriptscriptstyle (I)}$ and each $l'^{\scriptscriptstyle (I)}_{\scriptscriptstyle g'}$ is a pseudorandom string, so   $\vv{\bm{pm}}_{\scriptscriptstyle \mathtt{ A \rightarrow B}}$  and  $\vv{\bm{pm}}'_{\scriptscriptstyle \mathtt{ A \rightarrow B}}$  are indistinguishable.      Hence,  $Q_{\scriptscriptstyle i}$ is indistinguishable from $Q'_{\scriptscriptstyle i}$.


Now we move on to the case where $T_{\scriptscriptstyle i}= \textsf {\scriptsize Upd}^{\scriptscriptstyle (I)}_{\scriptscriptstyle t}$. In the real model, $\vv{\bm{o}}^{\scriptscriptstyle (I)}_{\scriptscriptstyle j,c^{ {\text{\tiny (\textit{I})}}}_{\tiny j}}$ contains $n$ elements blinded with pseudorandom values, while in the ideal model $\vv{\bm{o}}''^{\scriptscriptstyle (I)}$ comprises  $n$ random values. Since the random values and blinded values are  indistinguishable  vectors $\vv{\bm{o}}^{\scriptscriptstyle (I)}_{\scriptscriptstyle j,c^{ {\text{\tiny (\textit{I})}}}_{\tiny j}}$ and $\vv{\bm{o}}''^{\scriptscriptstyle (I)}$ are indistinguishable. In the real model, $l^{\scriptscriptstyle (I)}_{\scriptscriptstyle j}$ is a pseudorandom string and it belongs to vector $\vv{\bm{l}}^{\scriptscriptstyle (I)}$. In the ideal model, $l'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j}$ is a pseudorandom string and it belongs to vector $\vv{\bm{l}}'^{\scriptscriptstyle (I)}$. Therefore, the labels have the same distribution and are   indistinguishable. Also,  message $\textsf {\scriptsize \textbf{Update}}$ is identical in both models. So, $Q'_{\scriptscriptstyle i}$ and $Q_{\scriptscriptstyle i}$ are indistinguishable in this case too. From the above, we conclude that the views are indistinguishable. 

\
\vspace{-2mm}

\noindent\textbf{Case 2: Corrupted Client $B$.} In the real execution client $B$'s view is defined as:
\begin{equation*}
 \textsf {\scriptsize VIEW}^{\scriptscriptstyle\textsf { D-PSI}}_{\scriptscriptstyle B}(\Lambda, S^{\scriptscriptstyle (A)},S^{\scriptscriptstyle (B)})=\{S^{\scriptscriptstyle (B)}, r_{\scriptscriptstyle B}, \vv{\bm{q}}, \vv{\bm{f}}, f_{\scriptscriptstyle \cap}(S^{\scriptscriptstyle (A)},S^{\scriptscriptstyle (B)})\}. 
\end{equation*}

The simulator $\textsf {\scriptsize SIM}_{\scriptscriptstyle B}$ who receives $pk^{\scriptscriptstyle (B)}, lk^{\scriptscriptstyle (B)}, S^{\scriptscriptstyle (B)}$ and $f_{\scriptscriptstyle \cap}(S^{\scriptscriptstyle (A)},S^{\scriptscriptstyle (B)})$) does the following: 
\begin{packed_enum}
\item Creates an empty view, and appends $S^{\scriptscriptstyle (B)}$ and  uniformly at random chosen coins $r'_{\scriptscriptstyle B}$ to it. Then, it chooses two sets $S'^{\scriptscriptstyle (A)}$ and $S'^{\scriptscriptstyle (B)}$ such that $S'^{\scriptscriptstyle (A)}\cap S'^{\scriptscriptstyle (B)}=f_{\scriptscriptstyle \cap}(S^{\scriptscriptstyle (A)},S^{\scriptscriptstyle (B)})$ and $|S'^{\scriptscriptstyle (A)}|$, $|S'^{\scriptscriptstyle (B)}|\leq c$. 

\item Constructs  $\mathtt{HT}'^{\scriptscriptstyle(A)}$ and $\mathtt{HT}'^{\scriptscriptstyle(B)}$ using the public parameters. Next, it maps the elements in  $S'^{\scriptscriptstyle (A)}$ and $S'^{\scriptscriptstyle (B)}$ to the bins of $\mathtt{HT}'^{\scriptscriptstyle(A)}$ and $\mathtt{HT}'^{\scriptscriptstyle(B)}$, respectively. $\forall I, I\in \{A,B\}$ and $\forall s'^{\scriptscriptstyle (I)}_{\scriptscriptstyle i}\in S'^{\scriptscriptstyle (I)}$: $\mathtt{H}( s'^{\scriptscriptstyle (I)}_{\scriptscriptstyle i})=j$, then $ s'^{\scriptscriptstyle (I)}_{\scriptscriptstyle i}\rightarrow \mathtt{HT}'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j}$, where $1\leq j \leq h$.


\item Constructs  a polynomial representing the $d$ elements of each bin. If a bin contains less than $d$ elements first it is  padded with random values  to $d$ elements. $\forall I, I\in \{A,B\}$ and $\forall j, 1\leq j \leq h$: $\tau'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j}(x)=\prod\limits ^{\scriptscriptstyle d}_{\scriptscriptstyle m=1}(x-e_{\scriptscriptstyle m}^{\scriptscriptstyle (I)})$, where $e^{\scriptscriptstyle (I)}_{\scriptscriptstyle m} \in \mathtt{HT}'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j}$.

% (i.e. $e^{\scriptscriptstyle (I)}_{\scriptscriptstyle i}=s'^{\scriptscriptstyle (I)}_{\scriptscriptstyle i} $ or $e^{\scriptscriptstyle (I)}_{\scriptscriptstyle i}=r'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j,i}$).

\item Assigns a random polynomial $\omega'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j}$ of degree $d$ to each bin $\mathtt{HT}'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j}$ ( $\forall I, I \in \{A,B\}$). Next, it constructs  vectors $\vv{\bm{f}}'_{\scriptscriptstyle j}$ whose elements are computed as $\forall j, 1\leq j\leq h$ and $\forall i, 1\leq i\leq n$: $f'_{\scriptscriptstyle j,i}=\tau'^{\scriptscriptstyle (A)}_{\scriptscriptstyle j}(x_{\scriptscriptstyle i})\cdot  \omega'^{\scriptscriptstyle (A)}_{\scriptscriptstyle j}(x_{\scriptscriptstyle i})+\tau'^{\scriptscriptstyle (B)}_{\scriptscriptstyle j}(x_{\scriptscriptstyle i})\cdot  \omega'^{\scriptscriptstyle (B)}_{\scriptscriptstyle j}(x_{\scriptscriptstyle i})$, where $n=2d+1$.


%where $\tau'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j}(x)$ represents the set elements mapped to that bin. 

%\item Pick a key $mk'$ and derive $h$ keys, $k'_{\scriptscriptstyle j}$, from it. 
%
%\
%
%\vspace{-2mm}
%\begin{center}
%$\forall j, 1\leq j\leq h: k'_{\scriptscriptstyle j}= \mathtt{PRF}(mk', j)$
%\end{center}
%\
%
%\vspace{-2mm}

%\item Use each key $k'_{\scriptscriptstyle j}$ to generate $\vv{\bm{q}}'_{\scriptscriptstyle j}$ whose elements are computed as follows.

\item Generates  vector $\vv{\bm{q}}'=[\vv{\bm{q}}'_{\scriptscriptstyle 1}, ...,  \vv{\bm{q}}'_{\scriptscriptstyle h}]$  where each vector $\vv{\bm{q}}'_{\scriptscriptstyle i}$ contains $n$ random values picked from  field $\mathbb{F}_p$. Then, it appends  $\vv{\bm{q}}''=\pi(pk^{\scriptscriptstyle (B)},\vv{\bm{q}}')$, $\vv{\bm{f}}''=\pi(pk^{\scriptscriptstyle (B)},\vv{\bm{f}}')$ and $f_{\scriptscriptstyle \cap}(S^{\scriptscriptstyle (A)},S^{\scriptscriptstyle (B)})$ to the view and outputs it.



%\
%
%\vspace{-2mm}
%\begin{center}
% $\forall j, 1\leq j\leq h$ and $\forall i, 1\leq i\leq n$: $q'_{\scriptscriptstyle  j,i}= \mathtt{PRF}(k'_{\scriptscriptstyle j}, i)$
%\end{center}
%\
%
%\vspace{-2mm}


\end{packed_enum}






Now we show that the two views are computationally indistinguishable. The entries $S^{\scriptscriptstyle (B)}$ and $\Lambda$ are identical in both views.  In the real model, the elements in $\vv{\bm{q}}_{\scriptscriptstyle j}$ are blinded with pseudorandom values, so the blinded elements are uniformly random  values. On the other hand, in the ideal model the elements in $\vv{\bm{q}}'_{\scriptscriptstyle j}$ are random values drawn from the same field. Moreover, both vectors are permuted in the same way. Hence, the vectors $\vv{\bm{q}}$ and  $\vv{\bm{q}}'$ are computationally indistinguishable. 


Furthermore, in the real model, given each unblinded vector $\vv{\bm{f}}_{\scriptscriptstyle j}$, the adversary interpolates a $2d$-degree polynomial of the form $\phi_{\scriptscriptstyle j}(x)=\omega^{\scriptscriptstyle (A)}_{\scriptscriptstyle j}(x)\cdot \tau^{\scriptscriptstyle (A)}_{\scriptscriptstyle j}(x)+\omega^{\scriptscriptstyle (B)}_{\scriptscriptstyle j}(x)\cdot \tau^{\scriptscriptstyle (B)}_{\scriptscriptstyle j}(x)=\mu_{\scriptscriptstyle j}\cdot gcd(\tau^{\scriptscriptstyle (A)}_{\scriptscriptstyle j}(x),\tau^{\scriptscriptstyle (B)}_{\scriptscriptstyle j}(x))$,   where polynomial $gcd(\tau^{\scriptscriptstyle (A)}_{\scriptscriptstyle j}(x),\tau^{\scriptscriptstyle (B)}_{\scriptscriptstyle j}(x))$ represents intersection of the sets  in the corresponding bin, $\mathtt{HT}_{\scriptscriptstyle j}$. Similarly, in the ideal model, each $2d$-degree polynomial $\phi'_{\scriptscriptstyle j}(x)$ interpolated from vector $\vv{\bm{f}}'_{\scriptscriptstyle j}$ has the form $\phi'_{\scriptscriptstyle j}(x)=\omega'^{\scriptscriptstyle (A)}_{\scriptscriptstyle j}(x)\cdot \tau'^{\scriptscriptstyle (A)}_{\scriptscriptstyle j}(x)+\omega'^{\scriptscriptstyle (B)}_{\scriptscriptstyle j}(x)\cdot \tau'^{\scriptscriptstyle (B)}_{\scriptscriptstyle j}(x)=\mu'_{\scriptscriptstyle j}\cdot gcd(\tau'^{\scriptscriptstyle (A)}_{\scriptscriptstyle j}(x),\tau'^{\scriptscriptstyle (B)}_{\scriptscriptstyle j}(x))$, where $gcd(\tau'^{\scriptscriptstyle (A)}_{\scriptscriptstyle j}(x),\tau'^{\scriptscriptstyle (B)}_{\scriptscriptstyle j}(x))$ represents the sets intersection in the corresponding bin, $\mathtt{HT}'_{\scriptscriptstyle j}$. Also, as we discussed in section \ref{sec::poly}, $\mu_{\scriptscriptstyle j}$ and $\mu'_{\scriptscriptstyle j}$ are  uniformly random polynomials and the probability that their roots represent  set elements is negligible, thus   $\phi_{\scriptscriptstyle j}(x)$ and $\phi'_{\scriptscriptstyle j}(x)$  only contain information about the set intersection and have the same distribution in both models  \cite{DBLP:conf/crypto/KissnerS05,BonehGHWW13}. Moreover, since the same hash table parameters were used, the same elements would reside in the same bins in both models, therefore  polynomials $gcd(\tau^{\scriptscriptstyle (A)}_{\scriptscriptstyle j}(x),\tau^{\scriptscriptstyle (B)}_{\scriptscriptstyle j}(x))$ and $gcd(\tau'^{\scriptscriptstyle (A)}_{\scriptscriptstyle j}(x),\tau'^{\scriptscriptstyle (B)}_{\scriptscriptstyle j}(x))$ represent the set elements of the  intersection for that bin.    Moreover, both vectors $\vv{\bm{f}}$ and $\vv{\bm{f}}'$ are permuted in the same way. So, $\vv{\bm{f}}$ and $\vv{\bm{f}}'$ are indistinguishable as well. Also, the output, $ f_{\scriptscriptstyle \cap}(S^{\scriptscriptstyle (A)},S^{\scriptscriptstyle (B)})$, is identical in both views. Thus,  the two views are computationally indistinguishable. 



\
\vspace{-2mm}

\noindent\textbf{Case 3: Corrupted Client $A$.} In the real execution client $A$'s view is defined as: 
\begin{equation*}
 \textsf {\scriptsize VIEW}^{\scriptscriptstyle\textsf { D-PSI}}_{\scriptscriptstyle A}(\Lambda, S^{\scriptscriptstyle (A)},S^{\scriptscriptstyle (B)})=\{S^{\scriptscriptstyle (A)}, r_{\scriptscriptstyle A}, lk^{\scriptscriptstyle (B)}, pk^{\scriptscriptstyle (B)}, \vv{\bm{r}}^{\scriptscriptstyle (B)},  \textsf {\scriptsize \textbf{ID}}^{\scriptscriptstyle  (B)}, \Lambda \}. 
\end{equation*}


The simulator, $\textsf {\scriptsize SIM}_{\scriptscriptstyle A}$, who receives $S^{\scriptscriptstyle (A)}$ performs as follows. It constructs an empty view, and adds $S^{\scriptscriptstyle (A)}$ and  uniformly at random chosen coins $r'_{\scriptscriptstyle A}$ to the view. It picks two random keys $lk'^{\scriptscriptstyle (B)}$, $pk'^{\scriptscriptstyle (B)}$ and  adds them to the view. Then, it constructs $\vv{\bm{r}}'^{\scriptscriptstyle (B)}=[\vv{\bm{r}}'^{\scriptscriptstyle (B)}_{\scriptscriptstyle 1}, ..., \vv{\bm{r}}'^{\scriptscriptstyle (B)}_{\scriptscriptstyle h}]$, where each vector $\vv{\bm{r}}'^{\scriptscriptstyle (B)}_{\scriptscriptstyle i}$ contains $n$ random values picked from the field. It also appends $\vv{\bm{r}}'^{\scriptscriptstyle (B)}$, $\textsf {\scriptsize \textbf{ID}}^{\scriptscriptstyle  (B)}$ and  $\Lambda$ to the view and outputs the view.

In the following, we will show why the two views are indistinguishable. In both views, $S^{\scriptscriptstyle (A)}, \textsf {\scriptsize \textbf{ID}}^{\scriptscriptstyle  (B)}$ and $\Lambda$ are identical.  Also $r_{\scriptscriptstyle A}$ and $r'_{\scriptscriptstyle A}$ are chosen uniformly at random so they are indistinguishable. Moreover,  values $lk^{\scriptscriptstyle (B)}, pk^{\scriptscriptstyle (B)}, lk'^{\scriptscriptstyle (B)}$ and $pk'^{\scriptscriptstyle (B)}$ are the keys picked uniformly at random, so they are indistinguishable, too. In the real model,  each vector $\vv{\bm{r}}^{\scriptscriptstyle (B)}_{\scriptscriptstyle i}$ contains $n$ values blinded with pseudorandom values. On the other hand, in the ideal model, each vector $\vv{\bm{r}}'^{\scriptscriptstyle (B)}_{\scriptscriptstyle i}$ comprises $n$ random elements of the field. Since the random values and blinded values are indistinguishable,  vectors $\vv{\bm{r}}^{\scriptscriptstyle (B)}$ and $\vv{\bm{r}}'^{\scriptscriptstyle (B)}$ are indistinguishable. Hence, the two views are indistinguishable. 
\end{proof}

\vspace{-3mm}

==> CCS-24/short-coin-tossing.tex <==
% !TEX root =main.tex



\vspace{-2mm}



\subsection{Coin-Tossing Protocol}\label{sec::short-coin-tossing}
\vspace{-.5mm}

A Coin-Tossing protocol, \ct, allows two mutually distrustful parties, say $A$ and $B$, to jointly generate a single random bit. Formally, \ct computes the functionality $\fct(in_{\st A}, in_{\st B})\rightarrow (out_{\st A}, out_{\st B})$, which takes $in_{\st A}$ and  $in_{\st B}$ as inputs of $A$ and $B$ respectively and outputs $out_{\st A}$ to $A$ and $out_{\st B}$ to $B$, where $out_{\st A}=out_{\st B}$. A basic security requirement of a \ct is that the resulting bit is (computationally) indistinguishable from a truly random bit. 
%
Two-party coin-tossing protocols can be generalised to \emph{multi-party} coin-tossing ones to generate a \emph{random string}. 
%
The overheads of multi-party coin-tossing protocols are often linear with the number of participants. In this paper, any secure multi-party \ct that generates a random string can be used. For the sake of simplicity, we allow a multi-party \fct to take $m$ inputs and output a single value, i.e., $\fct(in_{\st 1}, ..., in_{\st m})\rightarrow out$. We refer readers to Appendix \ref{sec::coin-tossing} for further details. 

 




==> CCS-24/short-commitment.tex <==
% !TEX root =main.tex

\vspace{-2mm}

\subsection{Commitment Scheme}\label{subsec:short-commit}
\vspace{-1mm}

A commitment scheme involves a  \emph{sender} and a \emph{receiver}. It includes  two phases, \emph{commit} and  \emph{open}. In the \emph{commit} phase, the sender  commits to a message $x$ as $\mathtt{Com}(x,r)=\mathtt{Com}_{\scriptscriptstyle x}$, that involves a secret value,  $r$. In the \emph{open} phase, the sender sends the opening $\ddot{x}:=(x,r)$ to the receiver which verifies its correctness: $\mathtt{Ver}(\mathtt{Com}_{\scriptscriptstyle x},\ddot{x})\stackrel{\scriptscriptstyle ?}=1$ and accepts if the output is $1$. A commitment scheme must satisfy: (a) \textit{hiding}: it is infeasible for an adversary to learn any information about the committed  message $x$, until the commitment ${com}$ is opened, and (b) \textit{binding}: it is infeasible for a malicious sender to open a commitment ${com}$ to different values than that was  used in the commit phase. We refer readers to Appendix \ref{subsec:commit} for further details. 






==> CCS-24/short-security-model.tex <==
% !TEX root =main.tex


 
  
\vspace{-2.6mm}
\subsection{Security Model}\label{sec::sec-model}
\vspace{-1mm}


The paper employs a simulation-based secure computation model \cite{DBLP:books/cu/Goldreich2004} to define and prove its protocols, addressing both active (malicious) and passive (semi-honest) adversaries. Definitions for both adversary types are outlined, assuming a static adversary and a secure off-chain communication channel between clients. Appendix \ref{sec::sec-model-long} presents a full version of the security model.  


%In this paper, we use the simulation-based model of secure computation \cite{DBLP:books/cu/Goldreich2004} to define and prove our protocols. Since both types of active and passive adversaries are involved in our protocols, we outline definitions for both types.  We consider a static adversary and assume there is a secure (off-chain) channel between the clients.% and we consider a standard public blockchain, e.g., Ethereum.
%
 
  \vspace{-2mm}
  
 \subsubsection{Two-party Computation.} A two-party protocol, $\Gamma$, is characterized by specifying a random process that maps pairs of inputs to pairs of outputs, one for each party. This process is referred to as a functionality  $f:\{0,1\}^{\st *}\times\{0,1\}^{\st *}\rightarrow\{0,1\}^{\st *}\times\{0,1\}^{\st *}$, where $f:=(f_{\st 1},f_{\st 2})$. For every input pair $(x,y)$, the output pair is a random variable $(f_{\st 1} (x,y), f_{\st 2} (x,y))$, such that the party with input $x$ obtains $f_{\st 1} (x,y)$ while the party with input $y$ receives $f_{\st 2} (x,y)$. When $f$ is deterministic, then $f_{\st 1} =f_{\st 2}$. If $f$ is asymmetric and only one party (say the first one) receives the result, $f$ is defined as $f:=(f_{\st 1}(x,y), \bot)$. 
 
  
  \vspace{-1.2mm}
 \subsubsection{Security in the Presence of Passive Adversaries.} 
 
%  In the passive adversarial model, the party corrupted by such an adversary correctly follows the protocol specification. Nonetheless, the adversary obtains the internal state of the corrupted party, including the transcript of all the messages received, and tries to use this to learn information that should remain private. 
  
In this setting, a protocol is secure if whatever can be computed by a party in the protocol can be computed using its input and output only. 
  %
%  In the simulation-based model, it is required that a party’s view in a protocol's 
% execution can be simulated given only its input and output. This implies that the parties learn nothing from the protocol's execution. 
 %
 
 \vspace{-1.5mm}
 
\begin{definition}
Let $f$ represent the deterministic functionality defined above. Protocol $\Gamma$ securely computes $f$ in the presence of a  passive adversary if there exist polynomial time algorithms $(\mathsf {Sim}_{\st 1}, \mathsf {Sim}_{\st 2})$ such that: 
%
%\begin{center}
{\small{
$
  \{\mathsf {Sim}_{\st 1}(x, $ $f_{\st 1}(x,y))\}_{\st x,y}\stackrel{c}{\equiv} \{\mathsf{View}_{\st 1}^{\st \Gamma}(x,y) \}_{\st x,y}$ and 
  %
     $\{\mathsf{Sim}_{\st 2}(y, f_{\st 2}(x,y))\}_{\st x,y}\stackrel{c}{\equiv} \{\mathsf{View}_{\st 2}^{\st \Gamma}(x,y) \}_{\st x,y}
$}}
 % \end{center}
  %
  where party $i$’s view (during the execution of $\Gamma$) on input pair  $(x, y)$ is denoted by $\mathsf{View}_{\st i}^{\st \Gamma}(x,y)$ and equals $(w, r^{\st i}, m_{\st 1}^{\st i}, ..., m_{\st t}^{\st i})$, $w\in\{x,y\}$ is the input of $i^{\st th}$ party, $r_{\st i}$ is the outcome of this party's internal random coin tosses, and $m_{\st j}^{\st i}$ represents the $j^{\st th}$ message this party receives.  %The output of the $i^{\st th}$ party during the execution of $\Gamma$ on $(x, y)$ is denoted by $\mathsf{Output}_{\st 1}^{\st \Gamma}(x,y)$ and can be generated from its own view of the execution.  The joint output of both parties is denoted by $\mathsf{Output}^{\st \Gamma}(x,y):=(\mathsf{Output}_{\st 1}^{\st \Gamma}(x,y), \mathsf{Output}_{\st 2}^{\st \Gamma}(x,y))$.
%
  \vspace{-1mm}
\end{definition}
 

  \vspace{-2.5mm}
  
 \subsubsection{Security in the Presence of Active Adversaries.}  In this setting, correctness is required beyond the possibility that a corrupted party may learn more than it should. To capture the threats,
a protocol's security is analyzed by comparing what an adversary can do in the real protocol to what it can do in an ideal scenario. This is formalized by considering an ideal computation involving an incorruptible Trusted Third Party (TTP) to whom the parties send their inputs and receive the output of the ideal functionality. %Below, we describe the executions in the ideal and real models. 


 
 \vspace{-1.6mm} 
  
  
\begin{definition}\label{def::MPC-active-adv}
Let $f$ be the functionality defined above and $\Gamma$ be a two-party protocol that computes $f$.   Protocol $\Gamma$ securely computes $f$ in the presence of active adversaries if for every PPT adversary $\mathcal{A}$ for the real model, there exists a non-uniform PPT adversary (or simulator) $\mathsf{Sim}$ for the ideal model, such that for every $i\in \{0,1\}$, it holds that: 
%
$
\{\mathsf {Ideal}^{\st f}_{\st \mathsf{Sim}(z), i}(x,y)\}_{\st x,y,z}\stackrel{c}{\equiv} \{\mathsf{Real}_{\st \mathcal{A}(z), i}^{\st \Gamma}(x,y) \}_{\st x,y,z},
$, 
%
 where the ideal execution of $f$ on inputs $(x,$ $ y)$ and $z$ is denoted by $\mathsf{Ideal}^{\st f}_{\st\mathcal{A}(z), i}(x,$ $y)$ and is defined as the output pair of the honest party and $\mathcal{A}$ from the ideal execution. The real execution of $\Gamma$ is denoted by $\mathsf{Real}^{\st \Gamma}_{\st\mathcal{A}(z), i}(x,y)$, it is defined as the joint output of the parties engaging in the real execution of $\Gamma$, in the presence of $\mathcal{A}$. 
 \vspace{-2mm}
 \end{definition}

  

==> CCS-24/smart-PSI-protocol.tex <==
% !TEX root =main.tex


%\section{Sub Protocols}


 \vspace{-2mm}

\section{Definition of Multi-party PSI with Fair Compensation and Reward}


Next, we enhance \p to ``multi-party PSI with Fair Compensation and Reward'' (\ep), which not only provides the functionalities of \p,  but also lets honest clients contributing their set receive a reward from the buyer who initiates the PSI computation.



In \ep, there are (1) a set of clients $\{A_{\st 1},...,A_{\st m}\}$ within which a subset can potentially be active adversaries and engage in collusion, (2) a non-colluding dealer client, $D$, who may be semi-honest, and (3) an auditor $Aud$, who may also be semi-honest.  Every client possesses an input set. 


Moreover,  there are two ``extractor'' clients: $A_{\st 1}$ and $A_{\st 2}$, where $(A_{\st 1},A_{\st 2})\in \{A_{\st 1},...,A_{\st m}\}$.  These extractor clients voluntarily undertake the task of extracting the (encoded) elements of the intersection and transmitting them to a public bulletin board, represented by a smart contract. In exchange for this service, they will receive payment.
%
%We assume these two extractors are corrupted by an active adversary during interacting with other parties (and clients) until they collaborate with the rest of the clients to compute the intersection; 
%
We assume that these two extractors act rationally when they intend to perform the paid task of extracting the intersection and reporting it to the smart contract. This rational behavior allows them to maximize their profit.\footnote{Thus, similar to any $A_{\st i}$ in \p, these extractors might be corrupted by an active adversary and act maliciously during the PSI computation.} For simplicity, we designate client $A_{\st m}$ as the buyer, implying that this party initiates the PSI computation and holds an interest in the outcome.


 The formal definition of \ep is developed based on the definition of \p. Nevertheless, in \ep, we ensure that honest non-buyer clients receive a \emph{reward} for their participation in the protocol and for disclosing a portion of their inputs derived from the outcome. We achieve this through two main upgrades:  (i)  we enhance \qdel to  \qdelwr to ensure that when honest clients receive the result, an honest non-buyer client receives its deposit back along with a reward, while a buyer client receives its deposit back minus the paid reward and (ii) we upgrade  \qUnFAbt to \qUnFAbtwr to ensure that when an adversary aborts in the protocol unfairly, an honest party receives its deposit back along with a predefined amount of compensation and a reward.  
 %
 Predicates  \qinit and \qFAbt remain unchanged. We denote these four predicates as $\bar Q:=(\qinit,  \qdelwr, \qUnFAbtwr, \qFAbt)$. 
 
 For formal definitions of \qdelwr and \qUnFAbtwr, please refer to Appendix \ref{sec::Formal-Definitions-of-E-PSI-Predicates}. 
 %
Next, we present the formal definition of  \ep. 


%%%%%%%%

 \vspace{-1mm}
\begin{definition}[\ep]\label{def::PSI-Q-fair-reward}
Let $f^{\st \text{PSI}}$ be the multi-party PSI functionality defined in Section \ref{sec::F-PSI-model}. Protocol $\Gamma$ realizes $f^{\st \text{PSI}}$ with $\bar Q$-fairness-and-reward in the presence of $m-3$ active-adversary clients  and $two$ rational clients $A_{\st i}s$ or a passive dealer  $D$ or  auditor $Aud$, if for every non-uniform PPT adversary $\mathcal{A}$ for the real model, there is a non-uniform PPT simulator $\mathsf{Sim}$ for the ideal model, such that for every $I\in \{A_{\st 1},...,A_{\st m}, D, Aud\}$, it holds: 
%\begin{equation*}
$\{\mathsf {Ideal}^{\st \mathcal{W}(f^{\st \text{PSI}}, \bar Q)}_{\st \mathsf{Sim}(z), I}(S_{\st 1},$ $ ..., S_{\st m+1})\}_{\st S_{\st 1},..., S_{\st m+1},z}\stackrel{c}{\equiv} \{\mathsf{Real}_{\st \mathcal{A}(z), I}^{\st \Gamma}(S_{\st 1},..., S_{\st m+1}) \}_{\st S_{\st 1},..., S_{\st m+1},z}$, 
%\end{equation*}
where  $z$ is an auxiliary input given to $\mathcal{A}$ and  $\mathcal{W}(f^{\st \text{PSI}}, \bar Q)$ is a functionality that wraps $f^{\st \text{PSI}}$ with predicates $\bar Q:=(\qinit,  \qdelwr, \qUnFAbtwr, \qFAbt)$. 
  \end{definition}



%%%%%%%%

 \vspace{-3.5mm}
\section{Concrete Construction of \ep}


 
 %%%%%%%%%%%


%%%%%%%%%%

%\subsubsection{Preserving the Intersection Privacy.} As stated above, the extractors are required to prove to a smart contract that they know 


 \vspace{-1mm}

\subsection{Description of \withRew (\epsi)}
 \vspace{-.6mm}
 
 
 
 

To construct  \epsi, we mainly use \fpsi, deterministic encryption, ``double-layered'' commitments, the hash-based padding technique, and the counter-collusion smart contracts. % (described in Section \ref{Counter-Collusion-Smart-Contracts}). 
%
Briefly, \epsi works as follows. All clients execute step \ref{gen-FPSI-cont} of \fpsi to reach an agreement on a set of parameters and \fpsi's smart contract.  They also deploy another smart contract, denoted as $\SCe$, and agree on a secret key, $mk'$. 
%
Next, the buyer deposits a certain amount into $\SCe$. This deposit will be distributed among honest clients as a reward. 
%
%All clients check the buyer's deposit and proceed to the next step if they agree with the deposit amount.  

The extractors and $D$ deploy one of the counter-collusion smart contracts, namely \SCpc. These three parties contribute a specific sum to \SCpc.  Each honest extractor will receive a portion of $D$'s deposit for carrying out its task honestly, while each dishonest extractor will incur a penalty, causing a deduction from their deposit. % for engaging in malicious behaviour. 
%
Each client encrypts its set elements (under $mk'$ using deterministic encryption) and represents the encrypted elements as a polynomial. %The reason each client encrypts its set elements is to ensure that the privacy of the plaintext elements in the intersection will be preserved from the public. 



%Then, each client represents the encryption of its set elements as a polynomial. 





%

Following this, the extractors make a commitment to the encryption of their set elements and publicly disclose the outcome. Subsequently, all clients (including $D$) proceed with the remaining steps outlined in \fpsi using their input polynomials. This process results in the creation of a blinded polynomial (for each bin), the correctness of which is verified by \scf. There will be two cases: 

\vspace{-1mm}
\begin{enumerate}[leftmargin=4.5mm]
\item If  \scf confirms the correctness of the result,  all parties receive the deposits they initially placed in \scf. In this case, each extractor finds the set elements in the intersection. Additionally, each extractor provides proof to $\SCe$ that the encryptions of the elements in the intersection match the commitments they previously published. If $\SCe$ accepts both extractors' proofs, it compensates each client with a reward. This reward is funded from the buyer's deposit. The extractors receive refunds of their deposits and are also remunerated for their honest execution of the task. 
%
But, should  $\SCe$ decline to accept one of the extractors' proofs (or if one extractor betrays the other),  $\SCe$ then activates the auditor, specified in the counter-collusion contracts, to identify the misbehaving extractor. Subsequently, $\SCe$ pays a reward to each honest client, with the reward sourced from the misbehaving extractor's deposit. Also, $\SCe$ provides a refund of the buyer's deposit. 

\item If \scf does not approve the result's correctness and \aud identified misbehaving clients, honest clients will receive (a) their deposit back from \fpsi's contract, and (b)  compensation and reward, funded by the misbehaving clients. Also, the buyer and extractors will have their deposits refunded by $\SCe$.  
\end{enumerate}

 Figure \ref{fig:parties-interactions-in-ANE} in Appendix \ref{sec::ANE-workflow}  depicts the parties' interaction.
 
 

 \vspace{-2mm}
\subsection{Detailed Description of \epsi} 
 \vspace{-1mm}



Next, we will provide a more detailed description of the protocol (Table \ref{table:notation-table} on page \pageref{table:notation-table} summarizes the main notations used). 


\vspace{-1mm}
\begin{enumerate}[leftmargin=4mm]

%\item All clients in $\textbf{P}$ sign a smart contract $\mathcal{SC}$ and deploy it to a blockchain. Then, the buyer, $ { A}_{\st {  m}}$, deposits $v$ amounts in the contract.

\item\label{e-psi::call-F-PSI-stepOne}  All clients in $\cl=\{ A_{\st 1},...,   A_{\st m},  D\}$ collectively initiate step \ref{gen-FPSI-cont} of \fpsi (in Section \ref{Fair-PSI-Protocol}) to deploy \fpsi's contract $\mathcal{SC}_{\st\fpsi}$ and agree on a  master key, $mk$. 

\item\label{e-psi::deploy-SC-E-PSI} All clients in $\cl$  deploy a new smart contract, $\SCe$. The address of $\SCe$ is given to all clients. 

\item Buyer $ { A}_{\st {  m}}$, before time $t_{\st 1}$, deposits $\Smin\cdot \vc$  amount to $\SCe$. 
\item\label{e-PSI::buyer-deposit} All clients after  time $t_{\st 2} > t_{\st 1}$ ensure that the buyer has deposited $\Smin\cdot \vc$ amount on $\SCe$. Otherwise, they halt.



\item\label{e-PSI::extractor-deposit} $D$ signs \SCpc with the extractors. $\SCe$ transfers $\Smin\cdot \rc$ amount (from the buyer's deposit) to \SCpc for each extractor. This is the maximum amount to be paid to an honest extractor for honestly declaring the elements of the intersection. %Each honest extractor will be paid $\hat w'= r\cdot |{ { {S}}}_{\st\cap}|$, where 
%
Each extractor  deposits $\dc'=\dc+\Smin\cdot \fc$ amount in \SCpc at time $t_{\st 3}$. At time $t_{\st 4}$ all clients ensure that the extractors deposited a sufficient amount of coins; otherwise, they withdraw their deposit and halt. 

%
\item\label{e-psi::commit-to-mk} $D$ encrypts $mk$ under the public key of the auditor (in \SCpc); let $ct_{\st mk}$ be the resulting ciphertext.  It also generates a commitment of $mk$ as follows: $z'=\mathtt{PRF}(mk, 0),\ com_{\st mk}=\comcom(mk, z')$. It stores $ct_{\st mk}$  and ${com}_{\st mk}$ in $\SCe$. 


\item\label{e-psi::gen-mk-prime} All clients in $\cl$ engage in \ct to agree on another key, $mk'$.
%
\item\label{Smart-PSI:encode-elem} Each client  in $\cl$ encrypts the elements of its set $S:\{ s_{\st 1},..., s_{\st c}\}$ as: $\forall i, 1\leq i\leq c: e_{\st i}=\mathtt{PRP}(mk', s_{\st i})$. 
%
Then, it encodes its encrypted set element as $\bar{e}_{\st i} =e_{\st i} || \mathtt{H}(e_{\st i})$.  
%
Next, it constructs a hash table  $\mathtt{HT}$ and inserts the encoded elements into the table. $\forall i: \mathtt{H}( \bar{e}_{\st i})={ {  {j}}}$, then $\bar{e}_{\st i}\rightarrow \mathtt{HT}_{\st {  {j}}}$. It pads every bin with random dummy elements to $d$ elements (if needed). Then,  for every bin, it builds a polynomial whose roots are the bin's content: $\bm\pi^{\st { {(I)}}}=\prod\limits^{\st d}_{\st i=1} (x-e'_{\st i})$, where $e'_{\st i}$ is either $\bar{e}_{\st i}$, or a dummy value. 




\item\label{merkel-tree-cons} Every extractor in $\{A_{\st 1}, A_{\st 2}\}$: 

\begin{enumerate}
%
%\item for each bin, derives a pseudorandom polynomial: $\gamma'_{\st {  {j}}}$, using key $mk$.
%
%\item for each bin, evaluates $\gamma'_{\st {  {j}}}$ at the encode set elements of that bin: $\gamma'_{\st {  {j,i}}}=\gamma'_{\st {  {j}}}(\bar{e}^{\st { {(I)}}}_{\st i})$.
\item\label{smart-PSI::commit-to-bin} for each $j$-th bin, commits to the bin's elements: $com_{\st{i,j}}=\comcom(e'_{\st i}, q_{\st i})$, where $q_{\st i}$ is a fresh randomness  used for the commitment and $e'_{\st i}$ is either $\bar{e}_{\st i}$, or a dummy value of the bin. %Thus, if the bin contains paddings, it  commits to the paddings too. 




%\item commits to every  encrypted element.  $\forall i, 1\leq i\leq d: \mathtt{a}^{\st { {(I)}}}_{\st i}=\mathtt{Com}(e^{\st { {(I)}}}_{\st i}, q^{\st { {(I)}}}_{\st i})$, where $q^{\st { {(I)}}}_{\st i}$ is a fresh randomness  used for the commitment.
\item  constructs a Merkle tree on top of all committed values: 
\vspace{-1.5mm}
$$\mkgen(com_{\st 1,1},...,com_{\st d,h})\rightarrow g$$ %Let $\mathtt{MT}^{\st g}$ be a Merkel tree with a root node $g^{\st I}$. 
\vspace{-3mm}
\item stores the Merkle tree's root $g$ in $\SCe$.
\end{enumerate}


\item\label{e-psi::invoke-remainer-F-PSI} All clients in $\cl$   run steps \ref{ZSPA}--\ref{compute-res-poly} of \fpsi, where each client now deposits (in the $\mathcal{SC}_{\st\fpsi}$) $\yc'$ amount where $\yc'>\Smin\cdot \vc+{\chc}$. Recall, at the end of step \ref{compute-res-poly}  of \fpsi for each $j$-th bin (i) a random polynomial $\bm\zeta$ is registered in $\mathcal{SC}_{\st\fpsi}$, (ii) a polynomial $\bm\phi$ (blinded by a random polynomial $\bm\gamma'$) is extracted by $\mathcal{SC}_{\st\fpsi}$, and (iii) $\mathcal{SC}_{\st\fpsi}$  checks this polynomial's  correctness. If the latter check:

\begin{itemize}
\item[$\bullet$] passes (i.e., $Flag=True$), then all parties run step \ref{F-PSI::flag-is-true} of \fpsi (with a minor difference, see Appendix \ref{sec::Extracting-Elements-in-Intersection}).  In this case, each party receives $\yc'$ amount it deposited in $\mathcal{SC}_{\st\fpsi}$. They proceed to step \ref{smart-PSI::extractors} below.

\item[$\bullet$]  fails (i.e., $Flag=False$), all parties run step \ref{F-PSI::flag-is-false}  of \fpsi. 
 \aud is paid $\chc$ amount, and each honest party receives back its deposit, i.e., $\yc'$ amount. Also,  from the misbehaving parties' deposit  $\frac{m'\cdot \yc'-\chc}{m-m'}$ amount is sent to each honest client,  to reward and compensate the client $\Smin\cdot \lc$ and $\frac{m'\cdot \yc'-\chc}{m-m'}- \Smin\cdot \lc$ amounts respectively, where $m'$ is the total number of misbehaving parties.  Also, $\SCe$ returns to (a) the buyer its deposit (i.e., $\Smin\cdot \vc$ amount initially paid to $\SCe$), and (b) each extractor its deposit, i.e., $\dc'$ amount initially paid to \SCpc. Then, the protocol halts. 
\end{itemize}

\item\label{smart-PSI::extractors} Every extractor client: 
\begin{enumerate}

\item finds the intersection's elements as follows. It encodes each of its set elements to obtain $\bar e_{\st i}$, as explained in step \ref{Smart-PSI:encode-elem}.  
%i.e.,  it first computes $e^{\st { {(I)}}}_{\st i}=\mathtt{PRP}(mk',s^{\st { {(I)}}}_{\st i})$ and then computes $\bar{e}^{\st { {(I)}}}_{\st i} =e^{\st { {(I)}}}_{\st i} || \mathtt{H}(e^{\st { {(I)}}}_{\st i})$.
%
% and then encodes it:   (i.e. $ {e}^{\st { {(I)}}}_{\st i} =e^{\st { {(I)}}}_{\st i} || \mathtt{H}(e^{\st { {(I)}}}_{\st i})$). 
 %
It determines to which bin the encrypted value belongs, i.e., ${ {  {j}}}=\mathtt{H}( \bar{e}_{\st i})$. It evaluates the resultant polynomial (for that bin) at the encrypted element and considers the element in the intersection if the evaluation is zero: $\bm\phi( \bar{e}_{\st i})-\bm\zeta( \bar{e}_{\st i})\cdot \bm\gamma'( \bar{e}_{\st i})=0$. If the extractor is a traitor, by this step it should have signed the traitor’s contract \SCtc with $ { D}$ and provided related inputs to \SCtc. 

\item \label{extractor-proves} proves that every element in the intersection is among the elements it has committed to. Specifically, for each element in the intersection, for example $\bar{e}_{\st i}$, it sends to $\SCe$: 


\vspace{-1mm}
\begin{enumerate}%[leftmargin=2mm]
%
%\item [$\bullet$]  the opening of commitment $\mathtt{a}'$, i.e., pair $\ddot {x}:=(mk, z')$. This is done only once for all elements in the intersection.  
%
\item [$\bullet$]  commitment $com_{\st i,j}$ (generated in step \ref{smart-PSI::commit-to-bin}, for $\bar{e}_{\st i}$) and its  opening: 
 ${\hat x}':=(\bar{e}_{\st i},  q_{\st i})$.


%
%\item [$\bullet$] the element's commitment: $\mathtt{a}^{\st { {(I)}}}_{\st {  {j,i}}}=\mathtt{Com}(\gamma'_{\st {  {j,i}}}, q^{\st { {(I)}}}_{\st i})$, where $q^{\st { {{(I)}}} }_{\st i}$ was generated in step \ref{merkel-tree-cons}.   
%
%\item[$\bullet$]  $ \bar{e}^{\st { {{(I)}}} }_{\st i}$ and it  commitment's opening:  $\mathtt{m}^{\st { {{(I)}}} }_{\st i}=(\gamma'_{\st {  {j,i}}}, q^{\st { {{(I)}}} }_{\st i})$. 

%
\item[$\bullet$]   proof $h_{\st i}$  asserting $com_{\st i,j}$ is a leaf of  Merkle tree with  root $g$. 

%\item[$\bullet$] the index of the bin to which $ \bar{e}^{\st { {{(I)}}} }_{\st i}$ belongs, i.e., ${ {  {j}}}=\mathtt{H}(\bar {e}^{\st { {{(I)}}} }_{\st i})$. 
 \end{enumerate}
\item sends the opening of $com_{\st mk}$, i.e., pair $\hat {x}:=(mk, z')$, to $\SCe$. This is done only once for all elements in the intersection.  

 \end{enumerate}
\item\label{e-psi::SC-verification} Contract $\SCe$:
%
\begin{enumerate}

\item\label{e-psi::SC-verification--derive-mk}  verifies the opening of the commitment for $mk$, i.e., $\comver(com_{\st mk},$ $\hat{x})=1$. If the verification passes, it generates the index of the bin to which $ \bar{e}_{\st i}$ belongs, i.e., ${ {  {j}}}=\mathtt{H}(\bar {e}_{\st i})$. It  uses $mk$ to derive the pseudorandom polynomial $\bm\gamma'$ for $j$-th bin. 


 \item\label{e-psi::SC-verification--check-three-vals} checks whether (i) the opening of commitment is valid,  (ii) the Merkle tree proof is valid, and (iii) the encrypted element is the resulting polynomial's root. Specifically, it ensures that the following relation holds: 
 \vspace{-2mm}
 $$\big(\comver(com_{\st i,j}, \hat{x}')=1\big)  \wedge \big(\mkver(h_{\st i},g)=1\big) \wedge$$
 %
 %
 $$\big(\bm\phi( \bar{e}_{\st i})-\bm\zeta( \bar{e}_{\st i})\cdot \bm\gamma'( \bar{e}_{\st i})=0\big)$$
 \vspace{-2mm}
%
\end{enumerate}
%
\input{payment}

%\item Contract $\mathcal{SC}_{\st {  {EXT}}}$ after time $t_{\st 3}$ checks if $|{ { {S}}}_{\st\cap}|<{ { {S}}}_{\st {  min}}$. In this case, it returns $({ { {S}}}_{\st {  min}}-|{ { {S}}}_{\st\cap}|)\cdot v$ amount  to the buyer.

\end{enumerate}


 \vspace{-1mm}
 In Appendix \ref{sec::Annesidora-challenges}, we elaborate on the primary challenges we had to confront during the protocol design, which encompassed rewarding clients proportionately to the intersection size and managing collusions among extractors. Also, we refer readers to Appendix \ref{sec::Discussion-Anesidora} for a more discussion of \withRew, where we explain why a naive approach is inadequate, and provide insights into the use of hash-based padding, encryption, and double-layered commitment.
 
 
 

 \vspace{-1mm}
 \begin{theorem}\label{theorem::E-PSI-security}
If  $\mathtt{PRP}$, $\mathtt{PRF}$, the commitment scheme, smart contracts, the Merkle tree scheme, \fpsi and the counter-collusion contracts are secure and the public key encryption is semantically secure,  then  \epsi realizes  $f^{\st \text{PSI}}$ with $\bar Q$-fairness-and-reward (w.r.t. Definition \ref{def::PSI-Q-fair-reward}) in the presence of $m-3$ active-adversary clients $A_{\st j}$s and $two$ rational clients $A_{\st i}s$ or a  passive dealer $D$ or auditor $Aud$, or public which sees the intersection cardinality.
 \end{theorem}

\vspace{-2mm}

We prove Theorem \ref{theorem::E-PSI-security} in Appendix \ref{sec::E-PSI-proof}. 

\vspace{-2mm}




==> CCS-24/smart-PSI.tex <==
% !TEX root =U-PSI.tex

\section{Smart PSI}


In this section we provide smart PSI, a smart contract based private set intersection that charges the result recipients based on the number of set elements it learns. Here we consider stronger adversaries, economically rational semi-honest adversaries, who try to deviates from the protocol if doing so has let them gain some financial benefits. In the protocol, in addition to the roles in the previous protocol,   the is another role called: seller client who charges the result recipient client for the number of elements it learns. We assume that this client does not collude with the result recipient so the result recipient would bribe it and send other clients share to this client. Also, we do not consider fairness here, where either all clients must learn the result or no one. In this protocol, only client $B$ is interested in the intersection result. 

\begin{enumerate}
\item \textbf{Offline Phase} 

\begin{enumerate}
%\item It runs the off line phase in the previous advance protocol

\item\label{smart-contract-agreement} All clients, in $\{\resizeT {\textit A}_{\resizeS {\textit  1}},..., \resizeT {\textit A}_{\resizeS {\textit  m}},\resizeT {\textit  D}_{\resizeS {\textit  1}},\resizeT {\textit  D}_{\resizeS {\textit  2}}, B\}$, agree on a smart contract: $\mathcal{SC}$, provided in Fig. \ref{}. The smart contract is deployed by one of the clients and the address is given to the rest. All clients check the contract, if any client does not agree on the contract, it aborts. Otherwise, it proceeds to the next steps. 


\item\label{randomizing-elements} All clients, agree on  a pseudorandom permutation function, $\mathtt{PRP}$, and fresh secret key, $k_{\scriptscriptstyle o}$, for the function.  Then, each client $I \in \{\resizeT {\textit A}_{\resizeS {\textit  1}},..., \resizeT {\textit A}_{\resizeS {\textit  m}},\resizeT {\textit  D}_{\resizeS {\textit  1}},\resizeT {\textit  D}_{\resizeS {\textit  2}}, B\}$  uses $\mathtt{PRP}$ and the key to map its set elements to random values, as follows. $\forall i, 1\leq i\leq d: v^{\scriptscriptstyle I}_{\scriptscriptstyle i}=\mathtt{PRP}(k_{\scriptscriptstyle o}, s^{\scriptscriptstyle I}_{\scriptscriptstyle i})$. It considers  these encrypted values, $\vv{\bm{v}}^{\scriptscriptstyle I}=\{v^{\scriptscriptstyle I}_{\scriptscriptstyle 1},..,v^{\scriptscriptstyle I}_{\scriptscriptstyle d}\}$, as its set elements. Note that $\mathtt{PRP}$ is deterministic and also the client can always decrypt $v^{\scriptscriptstyle I}_{\scriptscriptstyle i}$ to get its actual set element: $s^{\scriptscriptstyle I}_{\scriptscriptstyle i}=\mathtt{PRP}^{\scriptscriptstyle -1}(k_{\scriptscriptstyle o}, v^{\scriptscriptstyle I}_{\scriptscriptstyle i})$

\item All clients, excluding  $B$, agree on  a \emph{seller} client: $\resizeT {\textit A}_{\resizeS {\textit  s}}$, who  can be any client, e.g. a client with smallest set size;  except  the result recipient, client $B$. 

\item All clients, including the seller,  run the Offline Phase as in previous protocol, where their inputs are the encrypted values computed in step \ref{randomizing-elements}. However, there are two   differences:  (a) the seller in step \ref{offline-autho-param} also picks a fresh key $k_{\scriptscriptstyle s}$ for the $\mathtt{PRF}$, and (b) the seller   in step \ref{offlinedealerrerand}, first picks a random polynomial $\beta(x)$ of degree $2d$ and then then computes: 

$\forall i, 1\leq i \leq n : c^{\resizeS {\textit  A}_{\resizeSS {\textit  s}}}_{\scriptscriptstyle i}     = \omega^{\resizeS {\textit  A}_{\resizeSS {\textit  s}}}_{\scriptscriptstyle i}   \cdot \pi^{\resizeS {\textit  A}_{\resizeSS {\textit  s}}}_{\scriptscriptstyle i}+\sum\limits^{\scriptscriptstyle 2}_{\scriptscriptstyle v=1} r^{\resizeS{\textit A}_{\resizeSS{\textit s}}\resizeS{,}  \resizeS { \textit D}_{\resizeSS {\textit v}}}_{\scriptscriptstyle i} +\sum\limits^{\scriptscriptstyle 2}_{\scriptscriptstyle v=1} q^{\resizeS{\textit A}_{\resizeSS{\textit s}}\resizeS{,}  \resizeS { \textit D}_{\resizeSS {\textit v}}}_{\scriptscriptstyle i}+ \beta_{\scriptscriptstyle i}$

where  $r^{\resizeS{\textit A}_{\resizeSS{\textit s}}\resizeS{,}  \resizeS { \textit D}_{\resizeSS {\textit v}}}_{\scriptscriptstyle i}=\PRF(k^{\resizeS{\textit A}_{\resizeSS{\textit s}}\resizeS{,}  \resizeS { \textit D}_{\resizeSS {\textit v}}},i),\ q^{\resizeS{\textit A}_{\resizeSS{\textit s}}\resizeS{,}  \resizeS { \textit D}_{\resizeSS {\textit v}}}_{\scriptscriptstyle i}=\PRF(l^{\resizeS{\textit A}_{\resizeSS{\textit s}}\resizeS{,}  \resizeS { \textit D}_{\resizeSS {\textit v}}},i)$, $\beta_{i}=\beta(x_{\scriptscriptstyle i})$ and $1\leq v\leq 2$. Note that, if the seller is one of the dealers, e.g. $\resizeT {\textit  D}_{\resizeS {\textit v}}$, it computes the following value instead:  $\forall i, 1\leq i \leq n : c^{\resizeS {\textit  D}_{\resizeSS {\textit  v}}}_{\scriptscriptstyle i}     = \omega^{\resizeS {\textit  D}_{\resizeSS {\textit  v}}}_{\scriptscriptstyle i}   \cdot \pi^{\resizeS {\textit  D}_{\resizeSS {\textit  v}}}_{\scriptscriptstyle i}+\sum\limits^{\scriptscriptstyle 2}_{\scriptscriptstyle p=1} r^{\resizeS{\textit D}_{\resizeSS{\textit v}}\resizeS{,}  \resizeS { \textit A}_{\resizeSS {\textit p}}}_{\scriptscriptstyle i} +\sum\limits^{\scriptscriptstyle 2}_{\scriptscriptstyle p=1} q^{\resizeS{\textit D}_{\resizeSS{\textit v}}\resizeS{,}  \resizeS { \textit A}_{\resizeSS {\textit p}}}_{\scriptscriptstyle i}+ \beta_{\scriptscriptstyle i}$

where  $r^{\resizeS{\textit D}_{\resizeSS{\textit v}}\resizeS{,}  \resizeS { \textit A}_{\resizeSS {\textit p}}}_{\scriptscriptstyle i}=\PRF(k^{\resizeS{\textit D}_{\resizeSS{\textit v}}\resizeS{,}  \resizeS { \textit A}_{\resizeSS {\textit p}}},i),\ q^{\resizeS{\textit D}_{\resizeSS{\textit v}}\resizeS{,}  \resizeS { \textit A}_{\resizeSS {\textit p}}}_{\scriptscriptstyle i}=\PRF(l^{\resizeS{\textit D}_{\resizeSS{\textit v}}\resizeS{,}  \resizeS { \textit A}_{\resizeSS {\textit p}}},i)$,  $\beta_{i}=\beta(x_{\scriptscriptstyle i})$ and $1\leq p\leq 2$ 

\end{enumerate}

\item \textbf{Online Phase} 



\begin{enumerate}
\item All clients, excluding   $B$, agree on parameter $c$: the maximum number of elements in the intersection that will be  sold/revealed to client $B$. Value $c$ is registered on $\mathcal{SC}$. To agree on value $c$, they can either negotiate out-of-the-bound or  use a voting scheme, e.g. by using a combination of commitment scheme and smart contract. See Appendix \ref{} for more detail.

\item Client $B$ deposites $e\cdot c$ coin to the smart contract, $\mathcal{SC}$. The seller client, $\resizeT {\textit A}_{\resizeS {\textit  s}}$,  checks if $e\cdot c$ coin has been deposited to the contract. If not, it aborts and ask other clients to abort too. Otherwise, it commits to: the evaluation of the random polynomial, $\beta(x)$, at every element in $\vv{\bm{v}}^{\resizeS {\textit  A}_{\resizeSS {\textit  s}}}=\{v^{\resizeS {\textit  A}_{\resizeSS {\textit  s}}}_{\scriptscriptstyle 1},..,v^{\resizeS {\textit  A}_{\resizeSS {\textit  s}}}_{\scriptscriptstyle d}\}$.  In particular:  $\forall i, 1\leq i \leq d: t_{\scriptscriptstyle i}=\mathtt{PRF}(k_{\scriptscriptstyle s},v^{\resizeS {\textit  A}_{\resizeSS {\textit  s}}}_{\scriptscriptstyle i}),  h_{\scriptscriptstyle i}= \mathtt{H}(\beta(v^{\resizeS {\textit  A}_{\resizeSS {\textit  s}}}_{\scriptscriptstyle i})\ || \ t_{\scriptscriptstyle i})$.  Next, $\resizeT {\textit A}_{\resizeS {\textit  s}}$ stores the committed values: $h_{\scriptscriptstyle i}$'s, in the contract. 

\item All clients, take the same steps as in steps \ref{clientBkeydist}-\ref{assistant-side-result-computation} in Online Phase in Fig.\ref{}. The only  difference is that the clients  (in steps \ref{authorizer-side-result-computation}, \ref{dealer-side-result-computation}, and \ref{assistant-side-result-computation}) send the messages to  smart contract $\mathcal{SC}$ instead of client $B$. 

\item Contract $\mathcal{SC}$ combines all clients' messages to remove all blinding factors. $\forall i, 1\leq i \leq n :$

$e_{\scriptscriptstyle i}=\sum\limits^{\scriptscriptstyle m}_{\scriptscriptstyle j=1} o^{\resizeS {\textit  A}_{\resizeSS {\textit  j}}}_{\scriptscriptstyle i}+ \sum\limits^{\scriptscriptstyle 2}_{\scriptscriptstyle v=1} o^{\resizeS {\textit  D}_{\resizeSS {\textit  v}}}_{\scriptscriptstyle i}$


\ \  \ \  \ $=\sum\limits^{\scriptscriptstyle m}_{\scriptscriptstyle j=1} (\omega^{\resizeS {\textit  A}_{\resizeSS {\textit  j}}}_{\scriptscriptstyle i}   \cdot \pi^{\resizeS {\textit  A}_{\resizeSS {\textit  j}}}_{\scriptscriptstyle i})+\sum\limits^{\scriptscriptstyle 2}_{\scriptscriptstyle v=1} (\omega^{\resizeS {\textit  D}_{\resizeSS {\textit  v}}}_{\scriptscriptstyle i}   \cdot \pi^{\resizeS {\textit  D}_{\resizeSS {\textit  v}}}_{\scriptscriptstyle i})+  \pi^{\resizeS {\textit B} }_{\scriptscriptstyle i}\cdot(\sum\limits^{\scriptscriptstyle m}_{\scriptscriptstyle j=1} (\zeta^{\resizeS{\textit A}_{\resizeSS{\textit j}}\resizeS{,}  \resizeS { \textit D}_{\resizeSS {\textit 1}}}_{\scriptscriptstyle i}+\zeta^{\resizeS{\textit A}_{\resizeSS{\textit j}}\resizeS{,}  \resizeS { \textit D}_{\resizeSS {\textit 2}}}_{\scriptscriptstyle i})+\sum\limits^{\scriptscriptstyle 2}_{\scriptscriptstyle v=1} (\zeta^{\resizeS{\textit D}_{\resizeSS{\textit v}}\resizeS{,}  \resizeS { \textit A}_{\resizeSS {\textit 1}}}_{\scriptscriptstyle i}+\zeta^{\resizeS{\textit D}_{\resizeSS{\textit v}}\resizeS{,}  \resizeS { \textit A}_{\resizeSS {\textit 2}}}_{\scriptscriptstyle i}))+\beta_{\scriptscriptstyle i}$

\item The contract uses $n$ pairs: $(z_{\scriptscriptstyle i}, e_{\scriptscriptstyle i})$ to interpolate a randomised polynomial: $\xi(x)$. The polynomial is of the form: $\xi(x)=\psi(x)+\beta(x)$, where $\psi(x)$ represents the intersection   and $\beta(x)$ is a uniformly random polynomial picked by the seller. 

\item Client $\resizeT {\textit A}_{\resizeS {\textit  s}}$ \emph{locally}  removes the random polynomial from $\xi(x)$ and  then, evaluates the result polynomial: $\psi(x)$, at every element of its encrypted set: $v^{\resizeS {\textit  A}_{\resizeSS {\textit  s}}}_{\scriptscriptstyle t}\in \vv{\bm{v}}^{\resizeS {\textit  A}_{\resizeSS {\textit s}}}$ ($\forall t, 1\leq t \leq d$). It considers the element in the intersection if the result of the polynomial evaluation is zero, i.e. if $\psi(v^{\resizeS {\textit  A}_{\resizeSS {\textit  s}}}_{\scriptscriptstyle t})=0$.

\item Client $\resizeT {\textit A}_{\resizeS {\textit  s}}$ sends the opening of (at most) $c$ elements in the intersection to the contract. In particular, it sends the following values to $\mathcal{SC}$. $\forall i, 1\leq i\leq c: (t_{\scriptscriptstyle i},v^{\resizeS {\textit  A}_{\resizeSS {\textit  s}}}_{\scriptscriptstyle i})$,  where $\psi(v^{\resizeS {\textit  A}_{\resizeSS {\textit  s}}}_{\scriptscriptstyle i})=0$.

\item Contract $\mathcal{SC}$, given $c$ pairs of $(t_{\scriptscriptstyle i},v^{\resizeS {\textit  A}_{\resizeSS {\textit  s}}}_{\scriptscriptstyle i})$,  performs as follows. $\forall 1\leq i\leq c:$ 
\begin{enumerate}
 \item evaluates  $\xi(x)$ at every element  $\resizeT {\textit A}_{\resizeS {\textit  s}}$ has sent: $\xi(v^{\resizeS {\textit  A}_{\resizeSS {\textit  s}}}_{\scriptscriptstyle i})=\psi(v^{\resizeS {\textit  A}_{\resizeSS {\textit  s}}}_{\scriptscriptstyle i})+\beta(v^{\resizeS {\textit  A}_{\resizeSS {\textit  s}}}_{\scriptscriptstyle i})$
 \item verifies if the polynomial evaluations matches the committed values already stored in the contract. $ \mathtt{H}(\xi(v^{\resizeS {\textit  A}_{\resizeSS {\textit  s}}}_{\scriptscriptstyle i}) \ || \ t_{\scriptscriptstyle i})\stackrel{\scriptscriptstyle ?}=h_{\scriptscriptstyle i}$.  If passed, it sends a share to every client in  $\{\resizeT {\textit A}_{\resizeS {\textit  1}},..., \resizeT {\textit A}_{\resizeS {\textit  m}},\resizeT {\textit  D}_{\resizeS {\textit  1}},\resizeT {\textit  D}_{\resizeS {\textit  2}}\}$. 
 
\end{enumerate}


\end{enumerate}
\end{enumerate}











==> CCS-24/table-cost.tex <==
% !TEX root =main.tex


 \begin{table}[!htb]
 \vspace{-1mm}
\caption{ {\small{Asymptotic costs of different parties in \epsi. In the table, $h$ is the total number of bins, $d$ is a bin's capacity (i.e., $d=100$), $m$ is the total number of clients (excluding $D$), $|S|$ is a set cardinality, and $\bar\xi$ is \ole's security parameter.
%
}}} \label{table::Asymptotic-Cost} 
 \vspace{-3mm}
\begin{center}
%\renewcommand{\arraystretch}{.95}
\scalebox{.93}{
\begin{tabular}{|c|c|c|c|c|} 

   %\hline
        \cline{1-3}  
   %
{\scriptsize {Party}}&{\scriptsize {Computation Cost}}&{\scriptsize {Communication Cost}}\\
     \cline{1-3}  
%&\scriptsize$e=1$&\scriptsize$e>1$\\
\hline

    %SO-PoR 1st row
\scriptsize Client $A_{\st  3},...,    A_{\st   m}$& \cellcolor{gray!50}   \scriptsize$O\Big(h\cdot d(m+d)\Big)$& \cellcolor{gray!50}  \scriptsize$O\Big(h\cdot d^{\st 2}\cdot \bar\xi\Big)$\\
 %  { }
     \cline{1-3}  
     %SO-PoR 2nd row
\scriptsize Dealer $D$&   \cellcolor{gray!20}\scriptsize$O\Big(h\cdot m(d^{\st 2}+d)\Big)$ &  \cellcolor{gray!20}\scriptsize$O\Big(h\cdot d^{\st 2}\cdot \bar\xi\cdot m\Big)$\\
      \cline{1-3}   
      

       %[3] 1st row 
       
   \scriptsize   {Auditor $\aud$ }& \cellcolor{gray!50}\scriptsize$O\Big(h\cdot m\cdot d\Big)$&  \cellcolor{gray!50}\scriptsize$O\Big(h\cdot d\Big)$\\      
            \cline{1-3} 

 % \scriptsize \ \ \ \ \ \ \ \ --------------&&\\
 \scriptsize{Extractor} $A_{\st  1},    A_{\st   2}$& \cellcolor{gray!20}\scriptsize$O\Big(h\cdot d(m+d)\Big)$& \cellcolor{gray!20}\scriptsize$O\Big(|S_{\scriptscriptstyle\cap}|\cdot \log_{\st 2}|S|\Big)$\\
     \cline{2-3}
%{\scriptsize Auditor $\mathcal{D}_{\st n}$}&    \cellcolor{gray!20}\scriptsize$O(\sum\limits_{\st i=e}^{\st n}\frac{n!}{i!(n- i)!})$&    \cellcolor{gray!20}\scriptsize$ O(\sum\limits_{\st i=e}^{\st n}\frac{n!}{i!(n- i)!})$\\
     \cline{1-3}  
     
 \scriptsize Smart contract $\mathcal{SC}_{\epsi}$\ \&\ $\mathcal{SC}_{\fpsi}$& \cellcolor{gray!50}\scriptsize $O\Big( |S_{\st \cap}|(d+ \log_{\st 2} |S|)+h\cdot m\cdot d\Big)$& \cellcolor{gray!50}\scriptsize ---\\
 
   \hline
   
   \hline
   
    
     \scriptsize Overall Complexity & \cellcolor{gray!20}\scriptsize $O\Big(h\cdot d^{2}\cdot m \Big)=O\Big(|S|\cdot d\cdot m\Big)$& \cellcolor{gray!20}\scriptsize {$O\Big(h\cdot d^{\st 2}\cdot \bar\xi\cdot m\Big)$}\\
     
      \cline{1-3}  

\end{tabular} 
} 
\end{center}
 \vspace{-3.5mm}
\end{table}






==> CCS-24/vopr-two-theorems.tex <==
% !TEX root =main.tex
Informally, Lemma \ref{theorem::evaluation-of-random-poly} states that the evaluation of a random polynomial at a fixed value results in a uniformly random value. %It will be used in {\vopr}'s proof to show that during the verification (in {\vopr}) a malicious party cannot learn anything about its counter party's input.
%\noindent\textbf{Remark 3.} In terms of assumption on the collusion between dealers and assistant clients,  parties, the main difference between using OPE in  and  is that if we will have use \cite{} then even if all but one dealers collude with each other, with all but one assistant clients,  with the rest of authorizer clients and client $B$, they cannot learn honest parties' set elements. However, we use the OPE in \cite{} the assumption is that no dealers collude with any assistant clients. 


%\begin{lemma}\label{theorem::evaluation-of-random-poly}
%Let $(x_{\st i}, y_{\st i})$ be arbitrary elements of a finite field $\mathbb{F}_{\st p}$, where $p$ is a security parameter and sufficiently large prime number.  The probability that the evaluation of a random polynomial $\bm\mu(x)$ at $x_{\st i}$ equals $ y_{\st i}$ is negligible in the security parameter. More formally, for $x_{\st i}, y_{\st i} \in \mathbb{F}_{\st p}$ and $\bm\mu(x)\stackrel{\st\$}\leftarrow \mathbb{F}_{\st p}[X]$, $1\leq deg(\mu)\leq d$, we have: $Pr[\bm\mu(x_{\st i})=y_{\st i}]=\epsilon(p)$. 
%\end{lemma}


\begin{lemma}\label{theorem::evaluation-of-random-poly}
Let $x_{\st i}$ be an element of a finite field $\mathbb{F}_{\st p}$, picked uniformly at random and $\bm\mu(x)$ be a random polynomial of constant degree $d$ (where $d=const(p)$) and defined over $\mathbb{F}_{\st p}[X]$. 
%
 Then, the evaluation of $\bm\mu(x)$ at $x_{\st i}$ is distributed uniformly at random over the elements of the  field, i.e., $Pr[\bm\mu(x_{\st i})=y]=\frac{1}{p}$, where $y\in \mathbb{F}_{\st p}$. 


%equals $ y_{\st i}$ is negligible in the security parameter. More formally, for $x_{\st i}, y_{\st i} \in \mathbb{F}_{\st p}$ and $\bm\mu(x)\stackrel{\st\$}\leftarrow \mathbb{F}_{\st p}[X]$, $1\leq deg(\mu)\leq d$, we have: $Pr[\bm\mu(x_{\st i})=y_{\st i}]=\epsilon(p)$. 
\end{lemma}



\begin{proof} Let $\bm\mu(x)=a_{\st 0}+\sum\limits^{\st d}_{\st j=1} a_{\st j}x^{\st j}$, where the  coefficients  are distributed uniformly at random over the field. 



Then, for any choice of $x$ and random coefficients   $a_{\st 1},...,a_{\st d}$, it holds that:
%
$$Pr[\bm\mu(x)=y]=Pr[\sum\limits_{\st i=0}^{\st d} a_{\st j}\cdot x^{\st j} = y] = Pr[a_{\st 0} = y-\sum\limits_{\st j=1}^{\st d} a_{\st j}\cdot x^{\st j}] = \frac{1}{p}$$

  $\forall y\in \mathbb{F}_{\st p}$, as $a_{\st 0}$ has been picked uniformly at random from $\mathbb{F}_{\st p}$. 
%
\end{proof} 



Informally, Theorem \ref{theorem:coef-poly-prod} states that the product of two arbitrary polynomials (in coefficient form) is a polynomial whose roots are the union of the two original polynomials.  Below, we formally state it. The theorem has been taken from \cite{AbadiMZ21}. 


\begin{theorem}\label{theorem:coef-poly-prod}
Let $\mathbf{p}$ and   $\mathbf{q}$ be two arbitrary non-constant polynomials of degree $d$ and $d'$ respectively, such that  $\mathbf{p} , \mathbf{q}   \in \mathbb{F}_{\st p}[X]$ and they are in coefficient form. Then, the product of the two polynomials is a polynomial whose roots include precisely the two polynomials' roots. 
\end{theorem}


%\begin{proof}
%Let $P=\{p_{\st 1},...,p_{\st t}\}$ and $Q=\{q_{\st 1},...,q_{\st t'}\}$ be the roots of polynomials $\mathbf{p}$ and   $\mathbf{q}$  respectively.  By the Polynomial Remainder Theorem,  polynomials $\mathbf{p}$ and $\mathbf{q}$  can be written as $\mathbf{p}(x)=\mathbf{g}(x)\cdot\prod\limits_{\st i=1}^{\st t}(x-p_{\st i})$ and $\mathbf{q}(x)=\mathbf{g}'(x)\cdot\prod\limits_{\st i=1}^{\st t'}(x-q_{\st i})$ respectively, where $\mathbf{g}(x)$ has degree $d-t$ and $\mathbf{g}'(x)$ has degree $d'-t'$. Let the product of the two polynomials be $\mathbf{r}(x)=\mathbf{p}(x)\cdot \mathbf{q}(x)$. For every $p_{\st i}\in P$, it holds  that $\mathbf{r}(p_{\st i})=0$. Because (a) there exists no non-constant polynomial in $\mathbb{F}[X]$ that has a multiplicative inverse (so it could cancel out factor $(x-p_{\st i})$ of $\mathbf{p}(x)$) and (b) $p_{\st i}$ is a root of $\mathbf{p}(x)$. The same argument  can be used to show for every $q_{\st i}\in Q$, it holds  that $\mathbf{r}(q_{\st i})=0$. Thus, $\mathbf{r}(x)$ preserves  roots of  both  $\mathbf{p}$ and $\mathbf{q}$. Moreover, $\mathbf{r}$ does not have any other roots (than $P$ and $Q$). In particular, if $\mathbf{r}(\alpha)=0$, then $\mathbf{p}(\alpha)\cdot \mathbf{q}(\alpha)=0$. Since there is no non-trivial divisors of zero in $\mathbb{F}[X]$  (as it is an integral domain), it must hold that either $\mathbf{p}(\alpha)=0$ or $\mathbf{q}(\alpha)=0$. Hence, $\alpha\in P$ or $\alpha\in Q$.  %\hfill\(\Box\)
%\end{proof}\hfill\(\Box\)




==> CCS-24/workflow-Anesidora.tex <==
% !TEX root =main.tex


\section{\withRew's Workflow}\label{sec::ANE-workflow}
Figure \ref{fig:parties-interactions-in-ANE} outlines the interaction between parties in \withRew.


\begin{figure*}[htp]
    \centering
    \includegraphics[width=13cm]{Diag-2.pdf}
     \vspace{-2mm}
    \caption{Outline of the interactions between parties in \withRew}\label{fig:parties-interactions-in-ANE}
\end{figure*}




==> CCS-24/workflow-Justitia.tex <==
% !TEX root =main.tex


\section{\withFai's Workflow}\label{sec::Justitia-workflow}
Figure \ref{fig:parties-interactions-in-Jus} outlines the interaction between parties in \withFai. 


\begin{figure*}[!h]
    \centering
    \includegraphics[width=13cm]{Diag-1.pdf}
     \vspace{-2mm}
    \caption{Outline of the interactions between parties in \withFai}\label{fig:parties-interactions-in-Jus}
\end{figure*}




==> CCS-24/zeta.tex <==
% !TEX root =main.tex


\subsubsection{Confidentiality of polynomial $\zeta$.} 

 The dealer is the sole entity responsible for selecting and possessing knowledge of the secret polynomial $\zeta$.  This polynomial remains confidential until all parties submit their messages to the smart contract. Subsequently, in step \ref{f-psi::D-gen-switching-poly} on page~\pageref{f-psi::D-gen-switching-poly}, the dealer transmits $\zeta$ to the smart contract. After this juncture, $\zeta$ is no longer a secret. However, malicious parties gain no advantage from knowing $\zeta$, as they have already submitted their inputs to the smart contract.




==> Communication-cost.tex <==
% !TEX root =test.tex


\begin{table*}[!htbp]
\begin{footnotesize}
\begin{center}
\caption{\small Total communication costs in bits for different protocols} \label{tbl::update}


\renewcommand{\arraystretch}{1.3}

\begin{tabular}{|c|c|c} 

\hline 
%{\rowcolors{2}{blue!80!gray!18}{blue!10!gray!18}
\cellcolor{gray!20} \scriptsize \textbf{Protocols} &\cellcolor{gray!20}\scriptsize  Communication cost: total number of bits exchanged \\
    \hline
    
    \hline



\cellcolor{white!20}  \scriptsize Our U-PSI:&\cellcolor{white!20}\scriptsize $ u((\textsl{m}-1)(4hd+4h+3)+h(2d+1)+1)+5771h$& \\

   \cellcolor{cyan!20}\scriptsize Using External Trusted Server in \cite{DBLP:conf/scn/InbarOP18}:    &\cellcolor{cyan!20}\scriptsize  $\textsl{m}^{\scriptscriptstyle 2}  |BF| |s_{\scriptscriptstyle i}|$  &\\ 

\cellcolor{white!20}  \scriptsize Semi-honest PSI in \cite{DBLP:conf/scn/InbarOP18}: &\cellcolor{white!20}\scriptsize   $(\textsl{m}^{\scriptscriptstyle 2}-1)  |BF| (k+2|s_{\scriptscriptstyle i}|)$&\\ 


 
    \cellcolor{cyan!20}\scriptsize Basic Semi-honest PSI in \cite{DBLP:conf/pkc/HazayV17}:      &\cellcolor{cyan!20}\scriptsize$(2  \textsl{m} - 1)  |S|  \Upsilon$&\\ 
    
        \cellcolor{white!20}\scriptsize Table-hashing based PSI in \cite{DBLP:conf/ccs/KolesnikovMPRT17}:      &\cellcolor{white!20}\scriptsize$(\textsl{m} +1)(\textsl{m} -1)( k'  (m_{\scriptscriptstyle 1}  \beta_{\scriptscriptstyle 1} + m_{\scriptscriptstyle 2}  \beta_{\scriptscriptstyle 2}) + 500(m_{\scriptscriptstyle 1}+m_{\scriptscriptstyle 2}) )$&\\ 
        
        \cellcolor{cyan!20}\scriptsize  \cite{DBLP:conf/ccs/ChenLR17}:      &\cellcolor{cyan!20}\scriptsize$1.5 \textsl {C}$ $(\textsl{m}-1) |s_{\scriptscriptstyle i}| |S| \log_{\scriptscriptstyle 2}(|S|)$&\\ 


      \cellcolor{white!20}\scriptsize  \cite{DBLP:conf/uss/Pinkas0SZ15}:      &\cellcolor{white!20}\scriptsize $|S|\theta v+k''(1.2|S|+\theta)$&\\ 
      
      
            \cellcolor{cyan!20}\scriptsize  \cite{kamarascaling}:      &\cellcolor{cyan!20}\scriptsize $3.5 u' (\textsl{m}-1)  |S|$&\\ 


       \hline



 %$ |BF|(\textsl{m}-1)((k+2l)+\textsl{m} (k+2l))$

\end{tabular}
\end{center}
\end{footnotesize}
\end{table*}

 %$ |BF|(\textsl{m}-1)((k+2l)+\textsl{m} (k+2l))$



In the above table, $\textsl{m}$: total number of clients, $u$: finite field size or the output size of pseudorandom function (e.g. $32, 64$ or $128$ bits), $d$: a bin capacity, i.e. $d=100$, also $5771$ is bit-length of a bloom filter that encodes $d$ elements with false positive probability of $2^{\scriptscriptstyle -40}$, and $h$: total number of bins. Also $|s_i|$ refers to bit length of the set element, $k$ is security parameter for OT (for simplicity we set $k=|s_i|$). Moreover, $|BF|$ denotes the bit length of bloom filter, e.g. for $2^{\scriptscriptstyle 20}$ elements and $2^{\scriptscriptstyle -40}$ false positive probability $|BF|=57,707,802$ bits. Also, for \cite{DBLP:conf/scn/InbarOP18}, the communication cost of $|BF|$ times invocation of 1-out-of-2 OT, is calculated according to 2\textsuperscript{nd} row in Table 2 in \cite{DBLP:conf/ccs/AsharovL0Z13}. Moreover, $\Upsilon$ denote the minimla bit-size of ciphertext in additive homomorphic encryption, i.e. $\Upsilon\geq 2048$ and $|S|$ is set cardinality. Furthermore,   $k'$ is the bit-length of oblivious programmable pseudorandom function's (OPRF) output, and $m_{\scriptscriptstyle i}, \beta_{\scriptscriptstyle i}$ are parameters of Cuckoo hashing, defined in Table 2 in \cite{DBLP:conf/ccs/KolesnikovMPRT17}, and $500$ refers to the amortized communication cost of each OPRF instance in bits, and $\textsl{C}$ refers to ciphertext expansion, e.g.  when the sets size are $2^{\scriptscriptstyle 20}$, then $\textsl{C}\geq8.67$, according to Table 5 in \cite{DBLP:conf/ccs/ChenLR17}. Furthermore, $\theta$ denotes the stash size in cuckoo hashing and equals $6$, $v$ is the bit-length of the oblivious pseudorandom function's output, $k''$ is the with of the pseudorandom code, $1.2$ is related to cuckoo hashing utilisation and $u'$ is the output size of pseudorandom permutation.


==> Priliminary.tex <==
% !TEX root =U-PSI.tex

\section{Priliminaries}

\subsection{Notations}
In the following, we  provide a basic and enhanced multiple clients PSI protocols. In the basic protocol, there are three types of parties involved in the protocols: $m>1$ authoriser clients: $\resizeT {\textit A}_{\resizeS {\textit  j}}$ who are not interested in the result, the result recipient client: $B$, and a non-colluding dealer: $D$. All parties are potentially semi-honest. In the first variant of the protocol the dealer does not have any set elements. Then we provide an enhanced protocol   that supports a distributed dealers such that the protocol remains secure even if  all but one dealers collude with client $B$ or  a subset of authoriser clients collude with each other and client $B$. Moreover, in the enhanced protocol, the dealers are actually clients who have  set elements as the computation's inputs.  Note that, in the following protocols, all  values and operations are defined over a finite field of prime order. Let each client $I\in \{\resizeT {\textit A}_{\resizeS {\textit  1}},...,\resizeT {\textit A}_{\resizeS {\textit  m}},B\}$, have a set $S^{\resizeS {\textit I} }=\{s^{\resizeS {\textit I} }_{\scriptscriptstyle 1},..., s^{\resizeS {\textit I} }_{\scriptscriptstyle d}\}$ and   $\vv{\bm{x}}=[x_{\scriptscriptstyle 1},..., x_{\scriptscriptstyle n}]$ be a  public vector of non-zero unique elements, where $n=2d+1$, and $d$ be the set cardinality's upper bound. Let $e$ be a flat price of learning one element of the set.   

\subsection{Shamir Secret Sharing}

\subsection{Oblivious Polynomial Evaluation and Oblivious Linear Function Evaluation} Oblivious polynomial evaluation: OPE, introduced by \cite{Naor:1999:OTP}, is a two-party protocol where a sender  inputs a polynomial, defined over a finite field, and a receiver inputs a single
point of the same finite field. At the end of the protocol, the sender receives nothing while the receiver  receives the polynomial evaluated on the point chosen by the receiver. Informally, the protocol is secure if the sender learns nothing on which point was chosen by the receiver and the receiver evaluates the polynomial on at most one point. OPE protocols can be broadly categorised in two groups: (a) computationally (or conditionally) secure, and (b) information theoretically (or unconditionally) secure. In this paper, we use OPE to evaluate a polynomial of \emph{degree one} and our focus is on the latter category as it best fits our purpose, e.g. due to its computational efficiency, (similar to our protocols) using a finite field over which are arithmetic operations are defined, etc. Information  theoretically OPE protocols can be further divided into three  classes: those that  (a) use an initializer that has an \emph{active role}, e.g. \cite{DBLP:conf/asiacrypt/ChangL01} (b) use an initializer that has a \emph{one-off role} and distributes  random parameters among receiver and sender in the setup phase and does not play any further role, e.g. \cite{DBLP:conf/acisp/HanaokaIMNOW04} and (c) are based on a distributed setting in which a set of servers implement the function of the sender, e.g. in \cite{DBLP:conf/icisc/CianciulloG18}. Our PSI protocol, can use either of these highly efficient OPE protocols, i.e.  \cite{DBLP:conf/acisp/HanaokaIMNOW04} or \cite{DBLP:conf/icisc/CianciulloG18}.  The scheme in \cite{DBLP:conf/acisp/HanaokaIMNOW04} is secure under the assumption that the initializer does not collude with the sender and receiver. Moreover, the scheme in \cite{DBLP:conf/icisc/CianciulloG18} remains secure as long as the sender does not collude with the servers, however if a threshold of the servers  collude with each other they cannot learn anything about the sender's or receiver's input and if a threshold of the servers collude with the receiver they cannot learn the sender's input. We note that the  use of the  OPE proposed in \cite{DBLP:conf/icisc/CianciulloG18}  in our protocol does not introduce any  additional servers, as  their roles are played by a subset of  clients in our protocol, i.e. assistant authorizer clients. For the sake of completeness, we provide both protocols \cite{DBLP:conf/acisp/HanaokaIMNOW04} in this section. 

%\begin{enumerate}
%\item There are three parties involved in this protocol: Sender: $S$, receiver $R$ and initializer $T$, where $S$'s input is $\beta(x)$ and $R$'s input is $b$.
%\item Setup: $T$ picks a random polynomial $\tau(x)$ of degree $d$ and a random value $v$. It sends $\tau(x)$ to $S$. Also, it sends  $v$ and $g=\tau(v)$ to $R$. 
%\item Computation: $R$ sends the value $l=b-v$ to $S$. $S$ then computes and sends to $R$ the polynomial $\delta (x)= \beta(l+x)+\tau(x)$. Then, $R$ computes $\delta(d)-g=\beta(b)=$
%\end{enumerate}





\begin{figure}[ht]
\setlength{\fboxsep}{2pt}
\begin{center}
\begin{boxedminipage}{11cm}
\small{

\

\noindent\textbf {Parties:} Sender: $\mathcal{S}$, receiver: $\mathcal{R}$ and initialiser: $\mathcal{T}$.

\noindent\textbf {Input:} $\mathcal{S}$ has a polynomial: $\beta(x)$  of degree at most $\mathsf{d}$. Also, $\mathcal{R}$ has a value:  $\mathsf{a}$.

\noindent\textbf {Output:} $\mathcal{R}$ obtains $\mathsf{b}=\beta(\mathsf{a})$ and $\mathcal{S}$ gets nothing.

\noindent\textbf {Setup:} 
\begin{enumerate}
\item Initializer $\mathcal{T}$ picks a random polynomial $\tau(x)$ of degree $\mathsf{d}$ and sends it to $\mathcal{S}$. 
\item Also, $\mathcal{T}$ picks a random value $\mathsf{v}$ and sends $\mathsf{v}$ and $\tau(\mathsf{v})$ to $\mathcal{R}$.
\end{enumerate}

\noindent\textbf {Computation:} 
\begin{enumerate}
\item $\mathcal{R}$ sends the value $\mathsf{f}=\mathsf{a}-\mathsf{v}$ to $\mathcal{S}$. 
\item Next, $\mathcal{S}$  computes polynomial $\delta(x)=\beta(\mathsf{f}+x)+\tau(x)$ and sends $\delta(x)$ to $\mathcal{R}$.
\item $\mathcal{R}$ computes $\delta(\mathsf{v})-\tau(\mathsf{v})=\mathsf{b}$
 \end{enumerate}
 \
}


\end{boxedminipage}
\end{center}
\caption{Efficient Information Theoretic OPE \cite{DBLP:conf/acisp/HanaokaIMNOW04}.} 
\label{fig:subroutines}
\end{figure}







\begin{figure}[ht]
\setlength{\fboxsep}{2pt}
\begin{center}
\begin{boxedminipage}{11cm}
\small{

\

\noindent\textbf {Parties:} Sender: $\mathcal{S}$, receiver: $\mathcal{R}$ and $\mathsf{k}$ servers: $\{\mathcal{S}_{\scriptscriptstyle {1}},...,\mathcal{S}_{\scriptscriptstyle \mathsf{k}}\}$.

\noindent\textbf {Input:} $\mathcal{S}$ has a polynomial: $\beta(x)=\mathsf{c}_{\scriptscriptstyle 0}+\mathsf{c}_{\scriptscriptstyle 1}x+...+\mathsf{c}_{\scriptscriptstyle \mathsf{d}}x^{\scriptscriptstyle \mathsf{d}}$  of degree at most $\mathsf{d}$. Also, $\mathcal{R}$ has a value:  $\mathsf{a}$.

\noindent\textbf {Output:} $\mathcal{R}$ obtains $\mathsf{b}=\beta(\mathsf{a})$ and $\mathcal{S}$ gets nothing.

\noindent\textbf {Setup:} 
\begin{enumerate}
\item $\mathcal{S}$ picks $\mathsf{d}$ random values: $\{\mathsf{r}_{\scriptscriptstyle 1},...,\mathsf{r}_{\scriptscriptstyle \mathsf{d}}\}$. Then, it computes the following values. $\forall i,1\leq i \leq \mathsf{d}: \mathsf{z}_{\scriptscriptstyle i}=\mathsf{r}_{\scriptscriptstyle i}\cdot \mathsf{c}_{\scriptscriptstyle i}$


\item $\mathcal{S}$  uses ($\mathsf{k},\mathsf{k}$) Shamir secret sharing scheme to split each coefficient $\mathsf{c}_{\scriptscriptstyle j}$,  into $\mathsf{k}$ shares.  In particular, for each $\mathsf{c}_{\scriptscriptstyle j} \in \{\mathsf{c}_{\scriptscriptstyle 0},...,\mathsf{c}_{\scriptscriptstyle \mathsf{d}}\}$, it:

\begin{enumerate}
\item picks a random polynomial $\tau_{\scriptscriptstyle j}(x)$ of degree at most $\mathsf{k}-1$, such that $\tau_{\scriptscriptstyle j}(0)=\mathsf{c}_{\scriptscriptstyle j}$. 
\item evaluates $\tau_{\scriptscriptstyle j}(x)$ at every elements of  vector $\{1,...,\mathsf{k}\}$.  At the end of this process, each $\mathsf{c}_{\scriptscriptstyle j}$ is split into $\{ \tau_{\scriptscriptstyle j}(1),..., \tau_{\scriptscriptstyle j}(\mathsf{k})\}$ shares. 



%$\forall w,\mathbf{1}\leq w \leq \mathbf{k}: \tau_{\scriptscriptstyle j}(w)= {\tau}_{\scriptscriptstyle j,w}$

\end{enumerate}

\item $\mathcal{S}$  splits each value $\mathsf{z}_{\scriptscriptstyle j}$ into $\mathsf{k}$ shares using ($\mathsf{k},\mathsf{k}$) Shamir secret sharing. At the end of this process, each $\mathsf{z}_{\scriptscriptstyle j}$ is split into $\{ \lambda_{\scriptscriptstyle j}(1),..., \lambda_{\scriptscriptstyle j}(\mathsf{k})\}$ shares, where $\lambda_{\scriptscriptstyle j}(x)$ is a random polynomial of degree at most $\mathsf{k}-1$, such that $\lambda_{\scriptscriptstyle j}(0)=\mathsf{z}_{\scriptscriptstyle j}$.

\item $\mathcal{S}$ privately sends to  $\mathcal{R}$ values: $\{\mathsf{r}_{\scriptscriptstyle 1},..., \mathsf{r}_{\scriptscriptstyle \mathsf{d}}\}$. Moreover, $\mathcal{S}$ sends  to each server: $\mathcal{S}_{\scriptscriptstyle  \mathsf{p}}$, two sets of shares (computed above): $\{\tau_{\scriptscriptstyle 0}( \mathsf{p}),..., \tau_{\scriptscriptstyle \mathsf{d}}( \mathsf{p})\}$ and $\{\lambda_{\scriptscriptstyle 1}( \mathsf{p}),..., \lambda_{\scriptscriptstyle \mathsf{d}}( \mathsf{p})\}$, where $1\leq \mathsf{p}\leq \mathsf{k}$. 



\end{enumerate}

\noindent\textbf {Computation:} 
\begin{enumerate}
\item  $\mathcal{R}$ broadcasts to all servers the following set: $\{\mathsf{e}_{\scriptscriptstyle 1 },...,\mathsf{e}_{\scriptscriptstyle \mathsf{d}}\}$ where $\mathsf{e}_{\scriptscriptstyle i}=\mathsf{a}^{\scriptscriptstyle i}-\mathsf{r}_{\scriptscriptstyle i}$


\item Each server: $\mathcal{S}_{\scriptscriptstyle  \mathsf{p}}$, computes the following value: $  \mathsf{u}_{\scriptscriptstyle \mathsf{p}}=\tau_{\scriptscriptstyle 0}( \mathsf{p})+ \sum\limits^{\scriptscriptstyle \mathsf{d}}_{\scriptscriptstyle i=1}(\tau_{\scriptscriptstyle i}( \mathsf{p})\cdot \mathsf{e}_{\scriptscriptstyle i}+\lambda_{\scriptscriptstyle i}( \mathsf{p}))$

\item $\mathcal{R}$, given pairs ($\mathsf{u}_{\scriptscriptstyle \mathsf{p}}, \mathsf{p}$), interpolates a polynomial $\phi(x)$, e.g.  using Lagrange interpolation, and considers the constant coefficient as the result, i.e. $\phi(0)=\mathsf{b}$.


 \end{enumerate}
 \
}


\end{boxedminipage}
\end{center}
\caption{Efficient Information Theoretic distributed OPE \cite{DBLP:conf/icisc/CianciulloG18}.} 
\label{fig:subroutines}
\end{figure}




\subsection{Pseudorandom Permutation} 


A pseudorandom permutation, $\mathtt{PRP}(,)$,






==> U-PSI-Parties-Communication-cost.tex <==
% !TEX root =test.tex








\begin{table*}[!htbp]
\begin{footnotesize}
\begin{center}
\caption{ \small U-PSI communication: breakdown by step (in MB).}\label{tbl::PSI} 
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|} 
\hline 
%{\rowcolors{2}{blue!80!gray!18}{blue!10!gray!18}
\cellcolor{gray!20}\scriptsize \textbf{Party} &\cellcolor{gray!20} \scriptsize \textbf{Setting}&\cellcolor{gray!20} \scriptsize \textbf{Field-size} &\scriptsize\cellcolor{gray!20} $2^{\scriptscriptstyle 10}$\scriptsize &\scriptsize\cellcolor{gray!20}  $2^{\scriptscriptstyle 11}$&\scriptsize  \cellcolor{gray!20}$2^{\scriptscriptstyle 12}$&\scriptsize\cellcolor{gray!20}  $2^{\scriptscriptstyle 13}$&\scriptsize\cellcolor{gray!20} $2^{\scriptscriptstyle 14}$&\scriptsize\cellcolor{gray!20}   $2^{\scriptscriptstyle 15}$&\scriptsize\cellcolor{gray!20}  $2^{\scriptscriptstyle 16}$&\scriptsize\cellcolor{gray!20}   $2^{\scriptscriptstyle 17}$&\scriptsize \cellcolor{gray!20}  $2^{\scriptscriptstyle 18}$&\scriptsize \cellcolor{gray!20} $2^{\scriptscriptstyle 19}$&\scriptsize\cellcolor{gray!20}  $2^{\scriptscriptstyle 20}$ \\
    \hline
    
     \hline
%\NameEntry{\rotatebox{90}{standards}}
\multirow{20}{*}{\rotatebox[origin=c]{90}{Result Recipient}}
 \multirow{4}{*}&\multirow{5}{*}{\rotatebox[origin=c]{90}{2-Client}}&\cellcolor{cyan!20}\scriptsize 32-bit: &\cellcolor{cyan!20}\scriptsize  0.04&\cellcolor{cyan!20}\scriptsize  0.09&\cellcolor{cyan!20}\scriptsize 0.18   &\cellcolor{cyan!20}\scriptsize   0.37  &\cellcolor{cyan!20}\scriptsize    0.74 &\cellcolor{cyan!20}\scriptsize  1.49   &\cellcolor{cyan!20}\scriptsize 3.99  &\cellcolor{cyan!20} \scriptsize 7.99  &\cellcolor{cyan!20} \scriptsize 15.99  &\cellcolor{cyan!20}\scriptsize 31.98  & \cellcolor{cyan!20} \scriptsize 63.97 \\ 
   \cline{3-13}
  \multirow{4}{*}&&\cellcolor{white!20}\scriptsize  40-bit: &\cellcolor{white!20}\scriptsize 0.05 &\cellcolor{white!20}\scriptsize 0.1  &\cellcolor{white!20}\scriptsize  0.21 &\cellcolor{white!20}\scriptsize   0.42  &\cellcolor{white!20}\scriptsize   0.84  &\cellcolor{white!20}\scriptsize  1.69 &\cellcolor{white!20}\scriptsize 4.52 &\cellcolor{white!20} \scriptsize   9.04&\cellcolor{white!20} \scriptsize 18.1 &\cellcolor{white!20}\scriptsize 36.2  & \cellcolor{white!20} \scriptsize 72.4 \\ 
    \cline{3-13}
      \multirow{4}{*}&&\cellcolor{cyan!20}\scriptsize 60-bit: &\cellcolor{cyan!20}\scriptsize 0.06 &\cellcolor{cyan!20}\scriptsize 0.13&\cellcolor{cyan!20}\scriptsize   0.27&\cellcolor{cyan!20}\scriptsize    0.54 &\cellcolor{cyan!20}\scriptsize 1.09  &\cellcolor{cyan!20}\scriptsize  2.19   &\cellcolor{cyan!20}\scriptsize 5.84 &\cellcolor{cyan!20} \scriptsize   11.68&\cellcolor{cyan!20} \scriptsize  23.36 &\cellcolor{cyan!20}\scriptsize 46.74  & \cellcolor{cyan!20} \scriptsize 93.48 \\ 
    \cline{3-13}
          \multirow{4}{*}&&\cellcolor{white!20}\scriptsize  64-bit: &\cellcolor{white!20}\scriptsize 0.06 &\cellcolor{white!20}\scriptsize 0.14&\cellcolor{white!20}\scriptsize  0.28&\cellcolor{white!20}\scriptsize 0.57   &\cellcolor{white!20}\scriptsize  1.14  &\cellcolor{white!20}\scriptsize 2.28 &\cellcolor{white!20}\scriptsize 6.1 &\cellcolor{white!20} \scriptsize   12.21&\cellcolor{white!20} \scriptsize  24.42 &\cellcolor{white!20}\scriptsize  48.849 & \cellcolor{white!20} \scriptsize 97.7\\ 
    \cline{3-13}
              \multirow{4}{*}&&\cellcolor{cyan!20}\scriptsize  128-bit: &\cellcolor{cyan!20}\scriptsize  0.11&\cellcolor{cyan!20}\scriptsize  0.24&\cellcolor{cyan!20}\scriptsize  0.48  &\cellcolor{cyan!20}\scriptsize    0.96 &\cellcolor{cyan!20}\scriptsize 1.93  &\cellcolor{cyan!20}\scriptsize  3.87   &\cellcolor{cyan!20}\scriptsize   10.31&\cellcolor{cyan!20} \scriptsize  20.63 &\cellcolor{cyan!20} \scriptsize  41.28 &\cellcolor{cyan!20}\scriptsize  82.57 & \cellcolor{cyan!20} \scriptsize 165.14\\ 
    \cline{2-13}

&\multirow{5}{*}{\rotatebox[origin=c]{90}{3-Client}}&\cellcolor{white!20}\scriptsize  32-bit:&\cellcolor{white!20}\scriptsize    0.06&\cellcolor{white!20}  \scriptsize 0.14 &\cellcolor{white!20} \scriptsize 0.28&\cellcolor{white!20}\scriptsize 0.57   &\cellcolor{white!20}  \scriptsize 1.14 &\cellcolor{white!20}  \scriptsize 2.28  &\cellcolor{white!20} \scriptsize  6.1  &\cellcolor{white!20} \scriptsize 12.21 &\cellcolor{white!20} \scriptsize 41.28 &\cellcolor{white!20}\scriptsize 48.84  &\cellcolor{white!20}\scriptsize 97.7  \\ 
    \cline{3-13}
     &&\cellcolor{cyan!20}\scriptsize  40-bit:&\cellcolor{cyan!20}\scriptsize 0.08   &\cellcolor{cyan!20}  \scriptsize 0.16&\cellcolor{cyan!20} \scriptsize 0.33&\cellcolor{cyan!20}\scriptsize  0.66  &\cellcolor{cyan!20}  \scriptsize  1.34&\cellcolor{cyan!20}  \scriptsize 2.68&\cellcolor{cyan!20} \scriptsize 7.15  &\cellcolor{cyan!20} \scriptsize 14.31&\cellcolor{cyan!20} \scriptsize  28.63&\cellcolor{cyan!20}\scriptsize 57.27&\cellcolor{cyan!20}\scriptsize 114.56 \\ 
    \cline{3-13}

     &&\cellcolor{white!20}\scriptsize 60-bit:&\cellcolor{white!20}\scriptsize   0.11&\cellcolor{white!20}  \scriptsize  0.22&\cellcolor{white!20} \scriptsize 0.45&\cellcolor{white!20}\scriptsize  0.91 &\cellcolor{white!20}  \scriptsize  1.83&\cellcolor{white!20}  \scriptsize  3.67 &\cellcolor{white!20} \scriptsize   9.79&\cellcolor{white!20} \scriptsize  19.58&\cellcolor{white!20} \scriptsize 39.17&\cellcolor{white!20}\scriptsize 78.35&\cellcolor{white!20}\scriptsize 156.71 \\ 
    \cline{3-13}
     &&\cellcolor{cyan!20}\scriptsize 64-bit:&\cellcolor{cyan!20}\scriptsize  0.11  &\cellcolor{cyan!20}  \scriptsize 0.24&\cellcolor{cyan!20} \scriptsize 0.48&\cellcolor{cyan!20}\scriptsize 0.96 &\cellcolor{cyan!20}  \scriptsize 1.93&\cellcolor{cyan!20}  \scriptsize 3.87  &\cellcolor{cyan!20} \scriptsize 10.31&\cellcolor{cyan!20} \scriptsize 20.63&\cellcolor{cyan!20} \scriptsize 41.28&\cellcolor{cyan!20}\scriptsize  82.57&\cellcolor{cyan!20}\scriptsize  165.14 \\ 
    \cline{3-13}
         &&\cellcolor{white!20}\scriptsize   128-bit:&\cellcolor{white!20}\scriptsize   0.21&\cellcolor{white!20}  \scriptsize 0.43 &\cellcolor{white!20} \scriptsize  0.87&\cellcolor{white!20}\scriptsize    1.75&\cellcolor{white!20}  \scriptsize  3.51&\cellcolor{white!20}  \scriptsize    7.03&\cellcolor{white!20} \scriptsize 18.74  &\cellcolor{white!20} \scriptsize 37.49 &\cellcolor{white!20} \scriptsize 75&\cellcolor{white!20}\scriptsize  150.01  &\cellcolor{white!20}\scriptsize 300.03  \\ 
    \cline{2-13}

    &\multirow{5}{*}{\rotatebox[origin=c]{90}{5-Client}}&\cellcolor{cyan!20}\scriptsize 32-bit:&\cellcolor{cyan!20}\scriptsize  0.11&\cellcolor{cyan!20}  \scriptsize 0.24 &\cellcolor{cyan!20}\scriptsize   0.48&\cellcolor{cyan!20}\scriptsize   0.96&\cellcolor{cyan!20}\scriptsize 1.93&\cellcolor{cyan!20}  \scriptsize 3.87&\cellcolor{cyan!20}\scriptsize  10.31&\cellcolor{cyan!20}\scriptsize 20.63&\cellcolor{cyan!20}\scriptsize 83.43&\cellcolor{cyan!20}\scriptsize  82.57&\cellcolor{cyan!20}\scriptsize  165.14 \\ 
        \cline{3-13}
          & &\cellcolor{white!20}\scriptsize  40-bit:&\cellcolor{white!20}\scriptsize  0.14&\cellcolor{white!20}  \scriptsize  0.28&\cellcolor{white!20}\scriptsize   0.57 &\cellcolor{white!20}\scriptsize 1.16 &\cellcolor{white!20}\scriptsize 2.32&\cellcolor{white!20}  \scriptsize 4.66&\cellcolor{white!20}\scriptsize 12.42 &\cellcolor{white!20}\scriptsize  24.85&\cellcolor{white!20}\scriptsize  49.71&\cellcolor{white!20}\scriptsize 99.43&\cellcolor{white!20}\scriptsize  198.86\\ 
        \cline{3-13}
           &&\cellcolor{cyan!20}\scriptsize 60-bit:&\cellcolor{cyan!20}\scriptsize  0.2 &\cellcolor{cyan!20}  \scriptsize 0.41 &\cellcolor{cyan!20}\scriptsize 0.82 &\cellcolor{cyan!20}\scriptsize   1.65 &\cellcolor{cyan!20}\scriptsize 3.31&\cellcolor{cyan!20}  \scriptsize 6.63 &\cellcolor{cyan!20}\scriptsize  17.69&\cellcolor{cyan!20}\scriptsize 35.39&\cellcolor{cyan!20}\scriptsize  70.78&\cellcolor{cyan!20}\scriptsize  141.58&\cellcolor{cyan!20}\scriptsize  283.17  \\ 
        \cline{3-13}
          & &\cellcolor{white!20}\scriptsize  64-bit:&\cellcolor{white!20}\scriptsize  0.21&\cellcolor{white!20}  \scriptsize 0.43 &\cellcolor{white!20}\scriptsize   0.87&\cellcolor{white!20}\scriptsize  1.75&\cellcolor{white!20}\scriptsize 3.51&\cellcolor{white!20}  \scriptsize 7.03 &\cellcolor{white!20}\scriptsize  18.74&\cellcolor{white!20}\scriptsize  37.49&\cellcolor{white!20}\scriptsize  75&\cellcolor{white!20}\scriptsize 150&\cellcolor{white!20}\scriptsize  300 \\ 
        \cline{3-13}
          & &\cellcolor{cyan!20}\scriptsize 128-bit:&\cellcolor{cyan!20}\scriptsize  0.4&\cellcolor{cyan!20}  \scriptsize   0.82&\cellcolor{cyan!20}\scriptsize  1.65   &\cellcolor{cyan!20}\scriptsize  3.32&\cellcolor{cyan!20}\scriptsize  6.67&\cellcolor{cyan!20}  \scriptsize 13.35  &\cellcolor{cyan!20}\scriptsize  35.6 &\cellcolor{cyan!20}\scriptsize  71.21&\cellcolor{cyan!20}\scriptsize   142.44&\cellcolor{cyan!20}\scriptsize  284.89&\cellcolor{cyan!20}\scriptsize  569.81  \\ 
        \cline{2-13}
     &\multirow{5}{*}{\rotatebox[origin=c]{90}{10-Client}}&\cellcolor{white!20}\scriptsize  32-bit:&\cellcolor{white!20} \scriptsize  0.23&\cellcolor{white!20}\scriptsize 0.48  &\cellcolor{white!20}\scriptsize  0.97&\cellcolor{white!20}\scriptsize  1.94&\cellcolor{white!20} \scriptsize  3.9&\cellcolor{white!20}\scriptsize 7.82  &\cellcolor{white!20}\scriptsize 20.85  &\cellcolor{white!20}\scriptsize  41.71&\cellcolor{white!20}  \scriptsize 125.58&\cellcolor{white!20}\scriptsize 166.87 &\cellcolor{white!20} \scriptsize 333.75  \\ 
        \cline{3-13}
           &&\cellcolor{cyan!20}\scriptsize  40-bit:&\cellcolor{cyan!20}\scriptsize  0.29  &\cellcolor{cyan!20}  \scriptsize  0.59 &\cellcolor{cyan!20}\scriptsize 1.19    &\cellcolor{cyan!20}\scriptsize  2.39  &\cellcolor{cyan!20}\scriptsize 4.79 &\cellcolor{cyan!20}  \scriptsize 9.6 &\cellcolor{cyan!20}\scriptsize 25.59  &\cellcolor{cyan!20}\scriptsize  51.19 &\cellcolor{cyan!20}\scriptsize  102.4 &\cellcolor{cyan!20}\scriptsize 204.81 &\cellcolor{cyan!20}\scriptsize  409.63 \\ 
        \cline{3-13}
           &&\cellcolor{white!20}\scriptsize  60-bit:&\cellcolor{white!20}\scriptsize    0.42&\cellcolor{white!20}  \scriptsize   0.87&\cellcolor{white!20}\scriptsize   1.74 &\cellcolor{white!20}\scriptsize    3.5 &\cellcolor{white!20}\scriptsize  7.01&\cellcolor{white!20}  \scriptsize  14&\cellcolor{white!20}\scriptsize   37.45&\cellcolor{white!20}\scriptsize  74.9&\cellcolor{white!20}\scriptsize   149.81&\cellcolor{white!20}\scriptsize   299.65&\cellcolor{white!20}\scriptsize   599.31 \\ 
        \cline{3-13}
           &&\cellcolor{cyan!20}\scriptsize  64-bit:&\cellcolor{cyan!20}\scriptsize  0.45 &\cellcolor{cyan!20}  \scriptsize  0.92&\cellcolor{cyan!20}\scriptsize  1.85 &\cellcolor{cyan!20}\scriptsize   3.72 &\cellcolor{cyan!20}\scriptsize  7.46&\cellcolor{cyan!20}  \scriptsize  14.93 &\cellcolor{cyan!20}\scriptsize  39.82 &\cellcolor{cyan!20}\scriptsize  79.64 &\cellcolor{cyan!20}\scriptsize  159.3&\cellcolor{cyan!20}\scriptsize  318.62&\cellcolor{cyan!20}\scriptsize    637.25\\ 
        \cline{3-13}
          & &\cellcolor{white!20}\scriptsize  128-bit:&\cellcolor{white!20}\scriptsize  0.89&\cellcolor{white!20}  \scriptsize   1.8&\cellcolor{white!20}\scriptsize   3.61  &\cellcolor{white!20}\scriptsize 7.26   &\cellcolor{white!20}\scriptsize  14.56&\cellcolor{white!20}  \scriptsize 29.16 &\cellcolor{white!20}\scriptsize   77.75&\cellcolor{white!20}\scriptsize   155.5&\cellcolor{white!20}\scriptsize  311.04&\cellcolor{white!20}\scriptsize   622.11&\cellcolor{white!20}\scriptsize    1244.26 \\ 
        \cline{3-13}
       \hline

%\scriptsize Each  Authoriser 
\multirow{5}{*}{\rotatebox[origin=c]{90}{Each  Authoriser }}

     &\cellcolor{gray!40}&\cellcolor{cyan!20}\scriptsize 32-bit&\cellcolor{cyan!20} \scriptsize  0.02  &\cellcolor{cyan!20}\scriptsize  0.04 &\cellcolor{cyan!20}\scriptsize   0.09 &\cellcolor{cyan!20}\scriptsize   0.19 &\cellcolor{cyan!20}\scriptsize   0.39&\cellcolor{cyan!20} \scriptsize 0.79 &\cellcolor{cyan!20}\scriptsize 2.12   &\cellcolor{cyan!20} \scriptsize  4.25  &\cellcolor{cyan!20} \scriptsize 8.51  &\cellcolor{cyan!20}\scriptsize 17.02   &\cellcolor{cyan!20}\scriptsize  34.05   \\
        \cline{3-13}
           &\cellcolor{gray!40}&\cellcolor{white!20}\scriptsize 40-bit:&\cellcolor{white!20}\scriptsize  0.03  &\cellcolor{white!20}  \scriptsize 0.06  &\cellcolor{white!20}\scriptsize  0.12   &\cellcolor{white!20}\scriptsize 0.24   &\cellcolor{white!20}\scriptsize 0.49 &\cellcolor{white!20}  \scriptsize 0.99 &\cellcolor{white!20}\scriptsize 2.66  &\cellcolor{white!20}\scriptsize  5.32 &\cellcolor{white!20}\scriptsize 10.64  &\cellcolor{white!20}\scriptsize 21.28 &\cellcolor{white!20}\scriptsize 42.57  \\ 
        \cline{3-13}
           &\cellcolor{gray!40}&\cellcolor{cyan!20}\scriptsize 60-bit:&\cellcolor{cyan!20}\scriptsize  0.04  &\cellcolor{cyan!20}  \scriptsize 0.09  &\cellcolor{cyan!20}\scriptsize 0.18    &\cellcolor{cyan!20}\scriptsize   0.37  &\cellcolor{cyan!20}\scriptsize  0.74&\cellcolor{cyan!20}  \scriptsize  1.49&\cellcolor{cyan!20}\scriptsize 3.99  &\cellcolor{cyan!20}\scriptsize  7.98&\cellcolor{cyan!20}\scriptsize 15.96  &\cellcolor{cyan!20}\scriptsize  31.92 &\cellcolor{cyan!20}\scriptsize 63.85   \\ 
        \cline{3-13}
           &\cellcolor{gray!40}&\cellcolor{white!20}\scriptsize 64-bit:&\cellcolor{white!20}\scriptsize  0.04 &\cellcolor{white!20}  \scriptsize  0.09&\cellcolor{white!20}\scriptsize   0.19&\cellcolor{white!20}\scriptsize    0.39&\cellcolor{white!20}\scriptsize  0.79&\cellcolor{white!20}  \scriptsize   1.59&\cellcolor{white!20}\scriptsize  4.25 &\cellcolor{white!20}\scriptsize  8.51 &\cellcolor{white!20}\scriptsize 17.02 &\cellcolor{white!20}\scriptsize  34.05&\cellcolor{white!20}\scriptsize   68.11 \\ 
        \cline{3-13}
           &\cellcolor{gray!40}&\cellcolor{cyan!20}\scriptsize 128-bit:&\cellcolor{cyan!20}\scriptsize  0.09&\cellcolor{cyan!20}  \scriptsize   0.19&\cellcolor{cyan!20}\scriptsize 0.39     &\cellcolor{cyan!20}\scriptsize  0.79  &\cellcolor{cyan!20}\scriptsize  1.59&\cellcolor{cyan!20}  \scriptsize  3.19&\cellcolor{cyan!20}\scriptsize   8.51&\cellcolor{cyan!20}\scriptsize 17.02  &\cellcolor{cyan!20}\scriptsize  34.05&\cellcolor{cyan!20}\scriptsize  68.11 &\cellcolor{cyan!20}\scriptsize   136.23  \\ 
        \cline{3-13}
   
    \hline
%\scriptsize Cloud
\multirow{5}{*}{\rotatebox[origin=c]{90}{Cloud}}
    &\cellcolor{gray!40}&\cellcolor{white!20}\scriptsize  32-bit &\cellcolor{white!20} \scriptsize  0.02&\cellcolor{white!20} \scriptsize 0.04 &\cellcolor{white!20}\scriptsize 0.09   &\cellcolor{white!20} \scriptsize  0.19&\cellcolor{white!20}\scriptsize  0.39&\cellcolor{white!20}\scriptsize 0.79&\cellcolor{white!20}\scriptsize  2.1  &\cellcolor{white!20}\scriptsize  4.21  & \cellcolor{white!20}\scriptsize 8.42  &\cellcolor{white!20}\scriptsize 16.86  &\cellcolor{white!20}\scriptsize 33.72 \\
        \cline{3-13}
           &\cellcolor{gray!40}&\cellcolor{cyan!20}\scriptsize 40-bit:&\cellcolor{cyan!20}\scriptsize   0.03 &\cellcolor{cyan!20}  \scriptsize  0.06 &\cellcolor{cyan!20}\scriptsize   0.12  &\cellcolor{cyan!20}\scriptsize  0.24  &\cellcolor{cyan!20}\scriptsize 0.49 &\cellcolor{cyan!20}  \scriptsize  0.98&\cellcolor{cyan!20}\scriptsize  2.63 &\cellcolor{cyan!20}\scriptsize 5.26  &\cellcolor{cyan!20}\scriptsize 10.53  &\cellcolor{cyan!20}\scriptsize 21.07 &\cellcolor{cyan!20}\scriptsize 42.15   \\ 
        \cline{3-13}
           &\cellcolor{gray!40}&\cellcolor{white!20}\scriptsize 60-bit:&\cellcolor{white!20}\scriptsize  0.04  &\cellcolor{white!20}  \scriptsize   0.09&\cellcolor{white!20}\scriptsize 0.18   &\cellcolor{white!20}\scriptsize  0.36   &\cellcolor{white!20}\scriptsize  0.74&\cellcolor{white!20}  \scriptsize  1.48&\cellcolor{white!20}\scriptsize   3.95&\cellcolor{white!20}\scriptsize  7.9&\cellcolor{white!20}\scriptsize   15.8&\cellcolor{white!20}\scriptsize  31.61 &\cellcolor{white!20}\scriptsize  63.22  \\ 
        \cline{3-13}
           &\cellcolor{gray!40}&\cellcolor{cyan!20}\scriptsize 64-bit:&\cellcolor{cyan!20}\scriptsize  0.04 &\cellcolor{cyan!20}  \scriptsize  0.09&\cellcolor{cyan!20}\scriptsize 0.19   &\cellcolor{cyan!20}\scriptsize   0.39 &\cellcolor{cyan!20}\scriptsize 0.78 &\cellcolor{cyan!20}  \scriptsize  1.58 &\cellcolor{cyan!20}\scriptsize 4.21  &\cellcolor{cyan!20}\scriptsize  8.42 &\cellcolor{cyan!20}\scriptsize 16.85 &\cellcolor{cyan!20}\scriptsize  33.72&\cellcolor{cyan!20}\scriptsize 67.44   \\ 
        \cline{3-13}
           &\cellcolor{gray!40}&\cellcolor{white!20}\scriptsize 128-bit:&\cellcolor{white!20}\scriptsize  0.09&\cellcolor{white!20}  \scriptsize 0.19  &\cellcolor{white!20}\scriptsize 0.39     &\cellcolor{white!20}\scriptsize   0.78 &\cellcolor{white!20}\scriptsize  1.57&\cellcolor{white!20}  \scriptsize  3.16&\cellcolor{white!20}\scriptsize 8.42  &\cellcolor{white!20}\scriptsize   16.85&\cellcolor{white!20}\scriptsize  33.71&\cellcolor{white!20}\scriptsize   67.44&\cellcolor{white!20}\scriptsize 134.88    \\ 
        \cline{3-13}
       \hline
 
\end{tabular}
\end{center}
\end{footnotesize}
\end{table*}





%
%\begin{table*}[!htbp]
%\begin{footnotesize}
%\begin{center}
%\caption{ \small U-PSI communication cost when element and field bit-size is $32$: breakdown by step (in MB).}\label{tbl::PSI} 
%\renewcommand{\arraystretch}{1.3}
%\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|} 
%\hline 
%%{\rowcolors{2}{blue!80!gray!18}{blue!10!gray!18}
%\cellcolor{gray!20}\scriptsize \textbf{Party} &\cellcolor{gray!20} \scriptsize \textbf{Setting} &\scriptsize\cellcolor{gray!20} $2^{\scriptscriptstyle 10}$\scriptsize &\scriptsize\cellcolor{gray!20}  $2^{\scriptscriptstyle 11}$&\scriptsize  \cellcolor{gray!20}$2^{\scriptscriptstyle 12}$&\scriptsize\cellcolor{gray!20}  $2^{\scriptscriptstyle 13}$&\scriptsize\cellcolor{gray!20} $2^{\scriptscriptstyle 14}$&\scriptsize\cellcolor{gray!20}   $2^{\scriptscriptstyle 15}$&\scriptsize\cellcolor{gray!20}  $2^{\scriptscriptstyle 16}$&\scriptsize\cellcolor{gray!20}   $2^{\scriptscriptstyle 17}$&\scriptsize \cellcolor{gray!20}  $2^{\scriptscriptstyle 18}$&\scriptsize \cellcolor{gray!20} $2^{\scriptscriptstyle 19}$&\scriptsize\cellcolor{gray!20}  $2^{\scriptscriptstyle 20}$ \\
%    \hline
%    
%     \hline
%\NameEntry{\center \scriptsize Result \\ \scriptsize Recipient}
% \multirow{4}{*}&\cellcolor{cyan!20}  \scriptsize 2-Client: &\cellcolor{cyan!20}\scriptsize  0.04&\cellcolor{cyan!20}\scriptsize  0.09&\cellcolor{cyan!20}\scriptsize 0.18   &\cellcolor{cyan!20}\scriptsize   0.37  &\cellcolor{cyan!20}\scriptsize    0.74 &\cellcolor{cyan!20}\scriptsize  1.49   &\cellcolor{cyan!20}\scriptsize 3.99  &\cellcolor{cyan!20} \scriptsize 7.99  &\cellcolor{cyan!20} \scriptsize 15.99  &\cellcolor{cyan!20}\scriptsize 31.98  & \cellcolor{cyan!20} \scriptsize 63.97 \\ 
%    \cline{2-13}
% &\cellcolor{white!20}\scriptsize 3-Client:&\cellcolor{white!20}\scriptsize    0.06&\cellcolor{white!20}  \scriptsize 0.14 &\cellcolor{white!20} \scriptsize 0.28&\cellcolor{white!20}\scriptsize 0.57   &\cellcolor{white!20}  \scriptsize 1.14 &\cellcolor{white!20}  \scriptsize 2.28  &\cellcolor{white!20} \scriptsize  6.1  &\cellcolor{white!20} \scriptsize 12.21 &\cellcolor{white!20} \scriptsize 41.28 &\cellcolor{white!20}\scriptsize 48.84  &\cellcolor{white!20}\scriptsize 97.7  \\ 
%    \cline{2-13}
%    &\cellcolor{cyan!20}\scriptsize 5-Client:&\cellcolor{cyan!20}\scriptsize 0.11  &\cellcolor{cyan!20}  \scriptsize  0.24&\cellcolor{cyan!20}\scriptsize 0.48   &\cellcolor{cyan!20}\scriptsize 0.96   &\cellcolor{cyan!20}\scriptsize 1.93&\cellcolor{cyan!20}  \scriptsize 3.87 &\cellcolor{cyan!20}\scriptsize  10.31&\cellcolor{cyan!20}\scriptsize 20.63 &\cellcolor{cyan!20}\scriptsize 83.43 &\cellcolor{cyan!20}\scriptsize 82.57 &\cellcolor{cyan!20}\scriptsize 165.14   \\ 
%        \cline{2-13}
%    &\cellcolor{white!20}\scriptsize 10-Client:&\cellcolor{white!20} \scriptsize  0.23&\cellcolor{white!20}\scriptsize 0.48  &\cellcolor{white!20}\scriptsize  0.97&\cellcolor{white!20}\scriptsize  1.94&\cellcolor{white!20} \scriptsize  3.9&\cellcolor{white!20}\scriptsize 7.82  &\cellcolor{white!20}\scriptsize 20.85  &\cellcolor{white!20}\scriptsize  41.71&\cellcolor{white!20}  \scriptsize 125.58&\cellcolor{white!20}\scriptsize 166.87 &\cellcolor{white!20} \scriptsize 333.75  \\ 
%       \hline
%
%\scriptsize Each  Authoriser 
%
%    \cellcolor{cyan!20} \scriptsize &\cellcolor{cyan!20} &\cellcolor{cyan!20} \scriptsize  0.02  &\cellcolor{cyan!20}\scriptsize  0.04 &\cellcolor{cyan!20}\scriptsize   0.09 &\cellcolor{cyan!20}\scriptsize   0.19 &\cellcolor{cyan!20}\scriptsize   0.39&\cellcolor{cyan!20} \scriptsize 0.79 &\cellcolor{cyan!20}\scriptsize 2.12   &\cellcolor{cyan!20} \scriptsize  4.25  &\cellcolor{cyan!20} \scriptsize 8.51  &\cellcolor{cyan!20}\scriptsize 17.02   &\cellcolor{cyan!20}\scriptsize  34.05   \\
%   
%    \hline
%\scriptsize Cloud
%
%    \multirow{3}{*}%{\scriptsize Cloud-side computation}
%    &\cellcolor{white!20}\scriptsize   &\cellcolor{white!20} \scriptsize  0.02&\cellcolor{white!20} \scriptsize 0.04 &\cellcolor{white!20}\scriptsize 0.09   &\cellcolor{white!20} \scriptsize  0.19&\cellcolor{white!20}\scriptsize  0.39&\cellcolor{white!20}\scriptsize 0.79&\cellcolor{white!20}\scriptsize  2.1  &\cellcolor{white!20}\scriptsize  4.21  & \cellcolor{white!20}\scriptsize 8.42  &\cellcolor{white!20}\scriptsize 16.86  &\cellcolor{white!20}\scriptsize 33.72 \\
%       \hline
% 
%\end{tabular}
%\end{center}
%\end{footnotesize}
%\end{table*}



==> complexity.tex <==
% !TEX root =U-PSI.tex
\section{Complexity Analysis}
\vspace{-2mm}
\subsection{Computation Complexity} \label{compcomp}

We first analyse the computation cost of U-PSI when the clients delegate PSI to the cloud. In our analysis, we do not count the pseudorandom function invocation cost, as it is a fast operation, and dominated by the other operations (e.g. modular arithmetic, shuffling and factorization). In step d.\ref{shuffleB}, client $B$ executes $h$ modular additions, and  shuffles a vector of $h$ elements with a cost of $O(c)$. Also, it performs  $nh$ modular additions in each of steps d.\ref{blindshuffleB} and f.\ref{unblind} to  blind and unblind  the hash table elements,  respectively. In step f.\ref{interpolate} it interpolates $h$ polynomials with each interpolation costing $O(d)$, where $d$ is a constant value. In step f.\ref{factorize}, it factorizes $h$ polynomials with each factorization costing $O(d^{\scriptscriptstyle 2})$. So in total client $B$'s computation cost is $(4+5d+d^{\scriptscriptstyle 2})h$ which is $O(c)$. Client $A$ in step  d.\ref{RegenKeys}  shuffles a vector of $h$ elements that costs $O(h)$ and in  step d.\ref{cleintAshuffles} it does $h$ modular additions, and shuffles a vector of $h$ elements. In step d.\ref{shuffleA}, it performs $2hnd$ modular multiplications and $2hnd$ modular additions to evaluate the pseudorandom polynomials. In the same step, to generate vectors $\vv{\bm{v}}^{\scriptscriptstyle (A)}$ and $\vv{\bm{v}}^{\scriptscriptstyle (B)}$, it performs $2nh$ modular multiplications. In step d.\ref{vectorq}, it permutes two vectors of  $h$ elements and carries out $2nh$ modular additions to generate  vectors $\vv{\bm{q}_{\scriptscriptstyle e}}$. Thus, in total it performs $(9+12d+8d^{\scriptscriptstyle 2})h$ or $O(c)$ modular operations. The cloud in step e.\ref{cloudcomp} performs  $2hnd$ modular multiplications and $2hnd$ modular additions to evaluate the pseudorandom polynomials. In the same step, it performs $2nh$ modular multiplications and $3nh$ modular additions to generate the vectors $\vv{\bm{t}_{\scriptscriptstyle e}}$. Thus, in total the cloud's computation involves $(5+14d+8d^{\scriptscriptstyle 2})h$ or  $O(c)$ modular operations. 
%In our multi-client protocol, the  computation complexity for those clients who authorise the computation,  is similar  to the  two-client protocol's, also the complexity for the cloud and result recipient would be $O(c\textsl{m-2c} )$, where $\textsl{m}$ is the total number of clients. 

In the update phase, each client  carries out $2d+2$ modular additions in step c.\ref{unblindupdate}. It interpolates a polynomial in step c.\ref{interpolateupdate} which costs $O(d)$.  In step c.\ref{InsertionDeletion}, it executes $d$ modular additions and $d$ modular multiplications to evaluate the polynomial at the single value $s$. In the same step, when the update is element insertion, the client extracts a bin's set elements that costs $O(d^{\scriptscriptstyle 2})$, and carries out $nd$ modular multiplications and $nd$ modular additions to evaluate the polynomial. So, the total computation cost for insertion is $5d(1+d)$, or $O(1)$ as $d$ is constant. If the update is element deletion, the client performs $2n$ modular additions to evaluate the two polynomials and $2n$ modular multiplications to generate  pseudorandom values. Finally, in step c.\ref{freshfactors}, the client performs $n+1$ modular additions. Therefore, the client's total computation cost for deletion is $6d+4$ or $O(1)$. 

In \cite{opsi15,DBLP:conf/fc/AbadiTD16,yang2018improved} set elements are represented as a single polynomial whose degree is linear to the set cardinality, $c$. In these protocols, the cost  of computing PSI is dominated by public key encryption operations, with complexity $O(c)$, and  polynomial factorization, with complexity $O(c^{\scriptscriptstyle 2})$. To insert/delete an element in  \cite{opsi15,yang2018improved}, a client needs to encode the element to be inserted/deleted as a polynomial, evaluate the polynomial on $2c+1$ elements and perform $2c+1$ modular multiplications, to blind the evaluated values. Also, the cloud needs to perform the same number of multiplications to apply the update. Therefore, the protocols' update complexity is $O(c)$. However, in \cite{DBLP:conf/fc/AbadiTD16} due to the way each outsourced value is blinded, the client has to download the entire date, remove the blinding factors and apply the change locally that also costs it $O(c)$. The protocol in \cite{eopsi} uses a hash table and encodes  set elements into a set of polynomials of constant degree, and this leads to $O(c)$ for computing PSI. In this protocol, if a client naively updates only one bin, then the cloud would be able to learn which elements have been updated with a non-negligible probability. The reason is that the bins are in their original order, and each bin's address is the hash value of an element in the bin, so if the client retrieves one bin, then the cloud would be able to figure out  what element is being updated  with a non-negligible probability when the set universe is not big. So, for the client to securely update its data, it has to re-encode the entire outsourced data that costs $O(c)$ too. 

Thus, the PSI computation cost in \cite{opsi15,DBLP:conf/fc/AbadiTD16,yang2018improved} is $O(c^{\scriptscriptstyle 2})$ while in our protocol and in \cite{eopsi} it is  $O(c)$. Moreover, update phase has $O(c)$ complexity in  \cite{opsi15,DBLP:conf/fc/AbadiTD16,yang2018improved,eopsi} while it has  much less cost, i.e. $O(1)$, in our protocol. 

\vspace{-3mm}

\subsection{Communication Complexity} \label{commcomp}

In U-PSI for PSI delegation client $B$, in step d.\ref{whatBSends}, sends a single value $tk^{\scriptscriptstyle (B)}$ to the cloud. In this step, it sends two  values, $pk^{\scriptscriptstyle (B)}$ and $lk^{\scriptscriptstyle (B)}$, and vector $\vv{\bm{r}}^{\scriptscriptstyle (B)}$ of $h$ bins to client $A$. Therefore, client $B$'s communication cost is $h(2d+1)+3$ or $O(c)$. In step d.\ref{WhatclientAsends}, client $A$ sends $tk^{\scriptscriptstyle (A)}$ and vector $\pi(pk^{\scriptscriptstyle (A)},\vv{\bm{m}}_{\scriptscriptstyle A \rightarrow B})$ containing $2h$ elements to the cloud. In the same step, it sends vector $\vv{\bm{q}}$ containing $h$ bins to client $B$. So, client $A$'s total communication cost  is $h(3+2d)+1$ or $O(c)$. The cloud's communication cost is $h(2d+1)$ or $O(c)$, as in step e.\ref{EO-cloudRes}, it sends vector $\vv{\bm{t}}$ of $h$ bins to client $B$. 
%Moreover, in our multi-client protocol, the communication cost of the cloud and the clients who authorize the computation remains the same as that of in two-client case, i.e. $O(c)$, but the result recipient' communication cost is $O(c\textsl{m}-c )$. 
To update its outsourced set a client sends to the cloud two labels, one in each of steps c.\ref{firstupdatestep} and c.\ref{lastupdatestep}. Moreover, it sends a vector of $2d+1$ elements in step c.\ref{lastupdatestep}. So, in total its communication cost is $3+2d$ or $O(1)$. Also, the cloud in step c.\ref{firstupdatestep} sends a vector of $2d+1$ elements to the client. Therefore,  the cloud's communication cost is $2d+1$ or $O(1)$. Note that  every message in our protocol is a random element of a finite field.

% Note that in our scheme for a fixed probability of overflow and fixed bin maximum load, the hash table length $h$ is linear to the set cardinality $c=\frac{c'}{m}$ (see section \ref{balls-bins}). 

%The reason is that if we rewrite $d=(1+\sigma)\cdot \frac{c}{h}$ (presented in subsection \ref{balls-bins}) we would have $h=(1+\sigma)\cdot \frac{c}{d}$.  

Both the PSI computation and update phases in the protocols in \cite{opsi15,yang2018improved,DBLP:conf/fc/AbadiTD16} have  $O(c)$ communication complexity.  Note that each message in these protocols for PSI computation is a ciphertext of a public key encryption and its size is  much larger  than the size of a field element, but the messages sent for an update is a field element. The protocol in \cite{eopsi} has $O(c)$ communication complexity for PSI computation, and as a client needs to re-encode the entire dataset to securely update it, it requires sending $h(2d+1)$, or $O(c)$ elements of a finite field.  

%As we stated earlier in section \ref{U-PSIdiscussion}, in O-PSI protocol, in order for a client to  update the data it needs to download them,  update locally, and upload them to the cloud, so its update cost is $O(c)$. Also, in EO-PSI, if  client  simply updates one bin it would leak non-negligible information about  set elements to the cloud (see section \ref{U-PSIdiscussion} for discussion). So,  in EO-PSI, the  secure way for the client to update the outsourced dataset is to retrieve the entire dataset and update it locally and send it back to the cloud.  However, such approach imposes $O(hd)$ communication cost. On the other hand, the protocol in \cite{Lopez-Alt12} that utilizes FHE can support data update  by using the FHE's capabilities. But, the protocol is designed for generic computation and the complexity of update in delegated PSI has not been defined. Note that each message in EO-PSI and U-PSI protocols is a random element of a   field (e.g. $p$ is about $112$ bits), whereas the messages in the other two protocols are ciphertexts of public key encryption that operate in a much larger group/ring. 

Hence,  our protocol and those in \cite{opsi15,DBLP:conf/fc/AbadiTD16,yang2018improved} have $O(c)$ communication complexity for PSI computation, but for updates only in U-PSI the client can securely update its dataset with $O(1)$ communication cost, while this cost is $O(c)$  for the other three protocols.

==> old--Related-work.tex <==
% !TEX root =U-PSI.tex





\section{Related Work and Attacks}\label{attacks}

In this section, we explain a series of attacks that can be carried out on the PSI protocols proposed by Ghosh \textit{et al.} in \cite{GhoshN19}. The main PSI protocols in  \cite{GhoshN19} are (a) two-party, (b) multi-party, and (c) threshold. Our  focus will be on the two-party PSI only for the sake of simplicity; however,  the other two  PSI protocols are susceptible to the same attacks. The protocol mainly utilises polynomial representation of sets and a variant of oblivious linear function evaluation \cite{ghosh2017maliciously} called oblivious polynomial addition (OPA). At a high level, in this protocol, each party generates a polynomial representing their set. Then, they  invoking oblivious polynomial addition (OPA) protocol, presented in Fig. \ref{fig:OPA}, to randomize each other polynomials. After that, they exchange messages that allow them to remove a part of random  polynomials, and find the result. The two-party PSI protocol is presented in detail in Fig. \ref{fig:Two-partyPSI-Ghosh}.

%Then, each party randomises other party's polynomial by invoking a variant of OLE, called $\mathcal{F}_{\scriptscriptstyle OPA}$. To randomise client $B$ polynomial, client $A$ sends two random polynomials: $r_{\scriptscriptstyle A}$ and $u_{\scriptscriptstyle A}$ to $\mathcal{F}_{\scriptscriptstyle OPA}$ while client $B$ sends to $\mathcal{F}_{\scriptscriptstyle OPA}$ its polynomial: $p_{\scriptscriptstyle B}$ (that represents its set). $\mathcal{F}_{\scriptscriptstyle OPA}$ returns a polynomial of the form $s_{\scriptscriptstyle B}=p_{\scriptscriptstyle B}\cdot r_{\scriptscriptstyle A}+u_{\scriptscriptstyle A}$ to client $B$. Then, they invoke  $\mathcal{F}_{\scriptscriptstyle OPA}$ again, this time client $B$ sends two random polynomials while   client $A$ sends its polynomial (representing its set)  $p_{\scriptscriptstyle A}$ to $\mathcal{F}_{\scriptscriptstyle OPA}$. 

% Then, they remove a part of  random values used in the MAC by including the inverse of the random values in another messages exchanged between the clients.  In the end, each client combines the messages and learn a combination of the polynomials randomised by both parties, where the combined protocol represents the intersection of the sets. Now we explain the protocol in more details. Let  $\vv{\bm{x}}= [x_{\scriptscriptstyle 1},...x_{\scriptscriptstyle 2d+1}]$ be a public vector of distinct non-zero elements.  



\begin{figure}[ht]
\setlength{\fboxsep}{1pt}
\begin{center}
\begin{boxedminipage}{12.3cm}

\

Each client $I\in\{A,B\}$ has a set $S^{\scriptscriptstyle (I)}$, where $m=max(|S^{(\scriptscriptstyle A)}|,|S^{(\scriptscriptstyle B)}|)+1$ 

\begin{enumerate}
\item \textbf{PSI Computation}
\begin{enumerate}
\item\label{gen-set-rep} Client $I\in\{A,B\}$: represent its set elements (i.e., all $s^{\scriptscriptstyle (I)}_{\scriptscriptstyle j}\in S^{\scriptscriptstyle (I)}$) as a degree-$m$ polynomial: $p_{\scriptscriptstyle I}=  \omega_{\scriptscriptstyle I}(x)\cdot\prod\limits^{\scriptscriptstyle d}_{\scriptscriptstyle j=1}(x-s^{\scriptscriptstyle (I)}_{\scriptscriptstyle j})$, where  $\omega_{\scriptscriptstyle I}(x)$ is a random polynomial. Each client $I$ picks three random polynomials: $r_{\scriptscriptstyle I}, u_{\scriptscriptstyle I}$ and $r'_{\scriptscriptstyle I}$, where the degree of $u_{\scriptscriptstyle I}$ is $2m$ and the degree of $r_{\scriptscriptstyle I}$ and $r'_{\scriptscriptstyle I}$ is $m$.

%Then each client  picks three random polynomials: $r_{\scriptscriptstyle I}, u_{\scriptscriptstyle I}$ and $r'_{\scriptscriptstyle I}$. %It evaluates  its polynomials at every elements of  $\vv{\bm{x}}$, e.g. $p_{\scriptscriptstyle I,j}=p_{\scriptscriptstyle I}(x_{\scriptscriptstyle j})$. 

\item\label{first-OPA-invocation} The clients   invoke  OPA where  client $A$ inserts $r_{\scriptscriptstyle A}, u_{\scriptscriptstyle A}$ and client $B$ inserts $p_{\scriptscriptstyle B}$ to OPA, which outputs  $s_{\scriptscriptstyle B}=p_{\scriptscriptstyle B}\cdot r_{\scriptscriptstyle A}+u_{\scriptscriptstyle A}$ to client $B$. 

%\item Client B:  uses $m+1$ pairs $(x_{\scriptscriptstyle j}, s_{\scriptscriptstyle B,j})$ to interpolates a polynomial: $s_{\scriptscriptstyle B}=p_{\scriptscriptstyle B}\cdot r_{\scriptscriptstyle A}+u_{\scriptscriptstyle A}$.


\item\label{2nd-OPA-invocation} The clients again invoke OPA, this time client $A$ inserts $p_{\scriptscriptstyle A}$ while client $B$ inserts $r_{\scriptscriptstyle B}, u_{\scriptscriptstyle B}$ to OPA that outputs $s_{\scriptscriptstyle A}=p_{\scriptscriptstyle A}\cdot r_{\scriptscriptstyle B}+u_{\scriptscriptstyle B}$ to client $A$. 
%\item Client $A$ given $m+1$ pairs $(s_{\scriptscriptstyle A,j}, x_{\scriptscriptstyle j})$ interpolates a polynomial: $s_{\scriptscriptstyle A}=p_{\scriptscriptstyle A}\cdot r_{\scriptscriptstyle B}+u_{\scriptscriptstyle B}$. 

\item\label{gen-s-A-prime} Client $A$: sends $s'_{\scriptscriptstyle A}=s_{\scriptscriptstyle A}-u_{\scriptscriptstyle A}+p_{\scriptscriptstyle A}\cdot r'_{\scriptscriptstyle A}$ to client $B$.% where $r'_{\scriptscriptstyle A}$ is a random polynomial. 
\item \label{where-clientB-deviates1}Client $B$: computes: $p_{\scriptscriptstyle \cap}=s'_{\scriptscriptstyle A}+s_{\scriptscriptstyle B}+p_{\scriptscriptstyle B}\cdot r'_{\scriptscriptstyle B}-u_{\scriptscriptstyle B}  =  p_{\scriptscriptstyle A}\cdot r'_{\scriptscriptstyle A}+p_{\scriptscriptstyle A}\cdot r_{\scriptscriptstyle B}+p_{\scriptscriptstyle B}\cdot r_{\scriptscriptstyle A}+p_{\scriptscriptstyle B}\cdot r'_{\scriptscriptstyle B}$. It sends the result polynomial, $p_{\scriptscriptstyle \cap}$, to client $A$.

\item\label{two-party-psi:find-intersect}  To find the intersection, client $I$  evaluates  polynomial $p_{\scriptscriptstyle \cap}$ at every element of its set (i.e., all $s^{\scriptscriptstyle (I)}_{\scriptscriptstyle j}\in S^{\scriptscriptstyle (I)}$), and considers the element in the intersection if  $p_{\scriptscriptstyle \cap}(s^{\scriptscriptstyle (I)}_{\scriptscriptstyle j})=0$.  

\end{enumerate}
\item  \textbf{Output Verification}
\begin{enumerate}
\item\label{two-party-PSI::agree-on-random-vals} The clients agree on two random values: $z$ and $q$, e.g., via a coin tossing protocol. 

\item\label{where-clientB-deviates2} Client $B$ sends $\alpha_{\scriptscriptstyle B}=p_{\scriptscriptstyle B}(z)$, $\beta_{\scriptscriptstyle B}=r_{\scriptscriptstyle B}(z)$, and $\delta_{\scriptscriptstyle B}=r'_{\scriptscriptstyle B}(z)$ to client $A$.

\item\label{checks-on-computingPSI} Client $A$:  checks if:   $p_{\cap}(z)\stackrel{?}=p_{\scriptscriptstyle A}(z)\cdot(\beta_{\scriptscriptstyle B}+r'_{\scriptscriptstyle A}(z))+\alpha_{\scriptscriptstyle B}\cdot(r_{\scriptscriptstyle A}(z)+\delta_{\scriptscriptstyle B})$

\item\label{two-party-PSI::what-A-sends-in-ver}  Client $A$ sends $\alpha_{\scriptscriptstyle A}=p_{\scriptscriptstyle A}(q)$, $\beta_{\scriptscriptstyle A}=r_{\scriptscriptstyle A}(q)$, and $\delta_{\scriptscriptstyle A}=r'_{\scriptscriptstyle A}(q)$ to client $B$.

 \item\label{checks-on-computingPSI-byB} Client $B$:  checks if:   $p_{\cap}(q)\stackrel{?}=p_{\scriptscriptstyle B}(q)\cdot(\beta_{\scriptscriptstyle A}+r'_{\scriptscriptstyle B}(q))+\alpha_{\scriptscriptstyle A}\cdot(r_{\scriptscriptstyle B}(q)+\delta_{\scriptscriptstyle A})$
 
\

\end{enumerate}
%}
\end{enumerate}
\end{boxedminipage}
\end{center}
\caption{Two-party PSI Protocol in \cite{GhoshN19}} 
\label{fig:Two-partyPSI-Ghosh}
\end{figure}


%First, each client $I\in\{A,B\}$ represent its set elements as a degree $m$ polynomial: $p_I= \prod\limits^{c}_{j=1}(x-s^{A}_j)\cdot \omega_I(x)$, where  $\omega_I(x)$ is a random polynomial. Then each client $I$ picks three random polynomials: $r_{I}, u_{I}$ and $r'_{I}$. Each client evaluates  its polynomials at every elements of the vector $\vv{\bm{x}}$, e.g. $p_{\scriptscriptstyle I,j}=p_I(x_{\scriptscriptstyle j})$. Then, clients $A$ and $B$ ($\forall j,1\leq j\leq m+1$) invoke an instance of $\mathcal{F}_{\scriptscriptstyle OPA}$ where  client $A$ (as sender) inserts $r_{\scriptscriptstyle A,j}$ and $u_{\scriptscriptstyle A,j}$ and client $B$ (as receiver) inserts $p_{\scriptscriptstyle B,j}$ to $\mathcal{F}_{\scriptscriptstyle OPA}$, which outputs  $s_{\scriptscriptstyle B,j}=p_{\scriptscriptstyle B,j}\cdot r_{\scriptscriptstyle A,j}+u_{\scriptscriptstyle A,j}$ to client $B$. Client $B$ uses $m+1$ pairs $(s_{B,j}, x_j)$ interpolates a polynomial: $s_B=p_B\cdot r_{A}+u_{A}$. 
%
%
%Then, they change their role and invoke another instance of $\mathcal{F}_{\scriptscriptstyle OPA}$ (for every $1\leq j\leq m+1$), this time client $A$, as receiver, inserts $p_{A,j}$ while client $B$ inserts $r_{\scriptscriptstyle B,j}$ and $u_{\scriptscriptstyle B,j}$ to $\mathcal{F}_{\scriptscriptstyle OPA}$ that outputs $s_{\scriptscriptstyle A,j}=p_{\scriptscriptstyle A,j}\cdot r_{\scriptscriptstyle B,j}+u_{\scriptscriptstyle B,j}$ to client $A$. Client $A$ given $m+1$ pairs $(s_{A,j}, x_j)$ interpolates a polynomial: $s_A=p_A\cdot r_{B}+u_{B}$. Client $A$ sends $s'_{A}=s_{A}-u_{A}+p_{A}\cdot r'_{A}$ to client $B$, where $r'_{A}$ is a random polynomial. Upon receiving client $A$'s message, client $B$ computes:
%\begin{equation}\label{computingPSI}
%\begin{split}
% p_{\cap}&=s'_{\scriptscriptstyle A}+s_{\scriptscriptstyle B}+p_{\scriptscriptstyle B}\cdot r'_{\scriptscriptstyle B}-u_{\scriptscriptstyle B}  \\ &=  p_{A}\cdot r'_{A}+p_{A}\cdot r_{B}+p_{B}\cdot r_{A}+p_{B}\cdot r'_{B}
% \end{split}
% \end{equation}
% 
% It sends the result polynomial: $p_{\cap}$ to client $A$. To find the intersection, client $I \in \{A,B\}$  can (independently) evaluate  polynomial $p_{\cap}$ at every element of its set, $s^{I}_j$, and consider the element in the intersection if  the result is $0$, i.e. $p_{\cap}(s^{I}_j)=0$.  
% 
%
%To allow client $A$ to check the result correctness,  it agrees with $B$ agree on a random value $z$ (e.g. via a coin tossing protocol). Then, client $B$ sends $\alpha_B=p_{B}(z)$, $\beta_{B}=r_{B}(z)$, and $\delta_{B}=r'_B(z)$ to client $A$ who checks if the following equation holds:  
%
%\begin{equation}\label{checks-on-computingPSI}
%p_{\cap}(z)\stackrel{?}=p_{A}(z)\cdot(\beta_{B}+r'_{A}(z))+\alpha_{B}\cdot(r_{A}(z)+\delta_{B})
% \end{equation}

%, for the sake of simplicity, we explain an attack mounted on the two-party PSI, presented in Fig \ref{fig:Two-partyPSI-Ghosh}. 


\subsection{Attack 1: Learning the result without letting other client(s)  do so}  In this section, we explain an attack that allows a malicious party to modify the output of OPA such that it can always learn the actual PSI result while   making its (honest) counter-party believe that there is no element in the intersection.  Briefly, the issue stems from  the insufficient check in step \ref{checks-on-computingPSI}, which allows a  malicious party to mount the attack, and deviate from the protocol without being detected. Now, we explain the attack in detail. Without loss of generality, let client $B$ be a malicious party. Both clients take  steps \ref{gen-set-rep}-\ref{gen-s-A-prime} honestly. Nevertheless, client $B$ in step  \ref{where-clientB-deviates1}, as a part of   computing  polynomial $p_{\scriptscriptstyle \cap}$,  instead of summing $s'_{\scriptscriptstyle A}$ with  the product  $p_{\scriptscriptstyle B}\cdot r'_{\scriptscriptstyle B}$ it sums  $s'_{\scriptscriptstyle A}$ with $r'_{\scriptscriptstyle B}$ and adds the rest of the values honestly. Therefore, now   $p_{\scriptscriptstyle \cap} $ would be: 


\begin{equation}\label{equ:modified-computingPSI}
\begin{split}
 p_{\scriptscriptstyle \cap}&=s'_{\scriptscriptstyle A}+s_{\scriptscriptstyle B}+ r'_{\scriptscriptstyle B}-u_{\scriptscriptstyle B}\\   &=  p_{\scriptscriptstyle A}\cdot r'_{\scriptscriptstyle A}+p_{\scriptscriptstyle A}\cdot r_{\scriptscriptstyle B}+p_{\scriptscriptstyle B}\cdot r_{\scriptscriptstyle A}+ r'_{\scriptscriptstyle B}
 \end{split}
 \end{equation}

 
Client $B$ sends  $p_{\scriptscriptstyle \cap}$, generated in Equation \ref{equ:modified-computingPSI}, to client $A$, in step \ref{where-clientB-deviates1}. In the output verification phase, both clients take step \ref{two-party-PSI::agree-on-random-vals} honestly, to generate $z$ and $q$. Client $B$, in step \ref{where-clientB-deviates2},  computes $\alpha_{\scriptscriptstyle B}=p_{\scriptscriptstyle B}(z)$, $\beta_{\scriptscriptstyle B}=r_{\scriptscriptstyle B}(z)$ honestly, but it sets  $\delta_{\scriptscriptstyle B}=r'_{\scriptscriptstyle B}(z)\cdot (\alpha_{\scriptscriptstyle B})^{\scriptscriptstyle -1}$ (instead of setting $\delta_{\scriptscriptstyle B}=r'_{\scriptscriptstyle B}(z)$). It sends $\alpha_{\scriptscriptstyle B},\beta_{\scriptscriptstyle B}$, and $\delta_{\scriptscriptstyle B}$ to honest client $A$ which in step \ref{checks-on-computingPSI}: 


\begin{enumerate}

\item evaluates the result polynomial, $p_{\scriptscriptstyle \cap}$, at $z$ that yields:


\begin{align*}
\begin{split}
p_{\scriptscriptstyle \cap}(z)&=  p_{\scriptscriptstyle A}(z)\cdot r'_{\scriptscriptstyle A}(z)+p_{\scriptscriptstyle A}(z)\cdot r_{\scriptscriptstyle B}(z)+p_{\scriptscriptstyle B}(z)\cdot r_{\scriptscriptstyle A}(z)+ r'_{\scriptscriptstyle B}(z)\\
\end{split}
\end{align*}

\item  generates $l$ as below (given the three messages, sent by client $B$):


\begin{align*}%\label{iiii}
\begin{split}
l&=p_{\scriptscriptstyle A}(z)\cdot(\beta_{\scriptscriptstyle B}+r'_{\scriptscriptstyle A}(z))+\alpha_{\scriptscriptstyle B}\cdot(r_{\scriptscriptstyle A}(z)+\delta_{\scriptscriptstyle B}) \\
&=p_{\scriptscriptstyle A}(z)\cdot r_{\scriptscriptstyle B}(z)+p_{\scriptscriptstyle A}(z)\cdot r'_{\scriptscriptstyle A}(z)+p_{\scriptscriptstyle B}(z)\cdot r_{\scriptscriptstyle A}(z)+r'_{\scriptscriptstyle B}(z)
 \end{split}
 \end{align*}

\item checks if $p_{\scriptscriptstyle \cap}(z)$ equals  $l$ (i.e., $p_{\scriptscriptstyle \cap}(z)\stackrel{\scriptscriptstyle ?}=l$). It accepts the result, if the check is passes.

\end{enumerate}

%
%\begin{align}\label{xx}
%\begin{split}
%p_{\scriptscriptstyle \cap}(z)&\stackrel{\scriptscriptstyle ?}=p_{\scriptscriptstyle A}(z)\cdot(\beta_{\scriptscriptstyle B}+r'_{\scriptscriptstyle A}(z))+\alpha_{\scriptscriptstyle B}\cdot(r_{\scriptscriptstyle A}(z)+\delta_{\scriptscriptstyle B}) \\
%&\stackrel{\scriptscriptstyle ?}=p_{\scriptscriptstyle A}(z)\cdot(\beta_{\scriptscriptstyle B}+r'_{\scriptscriptstyle A}(z))+\alpha_{\scriptscriptstyle B}\cdot r_{\scriptscriptstyle A}(z)+r'_{\scriptscriptstyle B}(z)
% \end{split}
% \end{align}

\


   As it is evident, the malicious client $B$ by using the above trick can pass the verification in the PSI protocol and convince client $A$ to accept the manipulated result.  Malicious client $B$ can generate the actual result (i.e., sets' intersection) \emph{for itself}, by   honestly computing  $p_{\scriptscriptstyle \cap}$ in step \ref{where-clientB-deviates1} and following the protocol in   step \ref{two-party-psi:find-intersect}. 
   
   
   However, given  manipulated result $p_{\scriptscriptstyle \cap}$, presented in Equation \ref{equ:modified-computingPSI}, honest client $A$ cannot learn  the actual sets' intersection, for the following reason. Let us  rewrite the manipulated result as $p_{\scriptscriptstyle \cap}=  \gamma+ r'_{\scriptscriptstyle B}$, where $\gamma=p_{\scriptscriptstyle A}\cdot r'_{\scriptscriptstyle A}+p_{\scriptscriptstyle A}\cdot r_{\scriptscriptstyle B}+p_{\scriptscriptstyle B}\cdot r_{\scriptscriptstyle A}$. Note that polynomial $\gamma$ encodes the actual result, as its roots contain the intersection of the sets. However, $ r'_{\scriptscriptstyle B}$ is a random polynomial, so the probability that its roots contain all  elements in the intersection is negligible, i.e., is at most $(\frac{m-1}{2^{\scriptscriptstyle {\scriptscriptstyle\lambda}}})^{\scriptscriptstyle\psi}$, where $\lambda$ is the bit-length of the finite field, $m$ is the random polynomial's degree, and $\psi$ is the intersection cardinality. That means the roots of polynomial $p_{\scriptscriptstyle \cap}=  \gamma+ r'_{\scriptscriptstyle B}$ does not contain common roots of both polynomials  $\gamma$ and $r'_{\scriptscriptstyle B}$, except with a negligible probability. Thus, the manipulated polynomial, $p_{\scriptscriptstyle \cap}$, does not represent the intersection of the sets and client $A$, who does not know $r'_{\scriptscriptstyle B}$, cannot learn the correct result.  
   
   
   \
   
   
%   Because, the sum of the polynomial representing  the intersection of the clients set: $p_{\scriptscriptstyle A}\cdot r'_{\scriptscriptstyle A}+p_{\scriptscriptstyle A}\cdot r_{\scriptscriptstyle B}+p_{\scriptscriptstyle B}\cdot r_{\scriptscriptstyle A}$ and  random polynomial $r'_{\scriptscriptstyle B}$ would be a uniformly random polynomial that does have  common roots with the clients' polynomials with a high probability, therefore the intersection would be empty.  
   
   This security issue is inherited by both   the multi-client  and multi-client threshold PSI protocols as well, as they use the same verification mechanism. 
   
   
%However, the above misbehaviour prevents client $A$ from learning the actual intersection. Because, the sum of the polynomial representing  the intersection of the clients set: $p_{\scriptscriptstyle A}\cdot r'_{\scriptscriptstyle A}+p_{\scriptscriptstyle A}\cdot r_{\scriptscriptstyle B}+p_{\scriptscriptstyle B}\cdot r_{\scriptscriptstyle A}$ and  random polynomial $r'_{\scriptscriptstyle B}$ would be a uniformly random polynomial that does have  common roots with the clients' polynomials with a high probability, therefore the intersection would be empty.  This security issue is inherited by both   the multi-client  and multi-client threshold PSI protocols as well, as they utilise the same verification mechanism. 




%\noindent\textbf{Attack 2}: \textit{Learning other client's set element with a non-negligible probability:}

\subsection{Attack 2: Learning Other Client's Set Element}

 A main component of the three PSI protocols is OPA  required  to be secure against malicious adversaries, in the sense that it ensures that the parties insert well-formed inputs and do not learn anything by inserting $0$ as their input.  In particular, OPA uses:  (a) OLE protocol with no checks, whose ideal functionality is, called $\mathcal{F}_{\scriptscriptstyle OLE}$, and (b)  OLE that ensures when an adversary inserts $0$ it learns nothing. The ideal functionality of OLE  is denoted by  $ \mathcal{F}_{\mathtt{OLE}^{\scriptscriptstyle +}}$. 




\begin{figure}[ht]
\setlength{\fboxsep}{0.7pt}
\begin{center}
\begin{boxedminipage}{12.3cm}
\begin{enumerate}
\small{
\item [$\bullet$] \textbf{Public parameters}: a vector of distinct non-zero elements: $\vv{\bm{x}}= [x_{\scriptscriptstyle 1},...x_{\scriptscriptstyle 2d+1}]$
\item \textbf{Computing} $s(x)=p(x)\cdot r(x)+u(x)$, where the sender has  $u(x),r(x)$ and the receiver has  $p(x)$ as inputs, $deg(u)\leq 2d, deg(r)=d, deg(p)\leq d$
\begin{enumerate}
\item \label{sender-evaluate} Sender: $\forall j, 1\leq j\leq 2d+1$, computes $u_{\scriptscriptstyle j}=u(x_{\scriptscriptstyle j})$ and $r_{\scriptscriptstyle j}=r(x_{\scriptscriptstyle j})$. Then, it  inserts $(u_{\scriptscriptstyle j}, r_{\scriptscriptstyle j})$ into  $ \mathcal{F}^{\scriptscriptstyle (j)}_{\mathtt{OLE}^{\scriptscriptstyle +}}$
\item\label{computing-receiver} Receiver:  $\forall j, 1 \leq j\leq 2d+1$, computes $p_{\scriptscriptstyle j}=p(x_{\scriptscriptstyle j})$. Then, it  inserts every $p_{\scriptscriptstyle j}$ into $ \mathcal{F}^{\scriptscriptstyle (j)}_{\mathtt{OLE}^{\scriptscriptstyle +}}$  and receives $s_{\scriptscriptstyle j}=p_{\scriptscriptstyle j}\cdot r_{\scriptscriptstyle j}+u_{\scriptscriptstyle j}$. It interpolates a polynomial $s(x)$ using pairs $(x_{\scriptscriptstyle j},s_{\scriptscriptstyle j})$. Next, it checks if $deg(s)\leq2d$. Otherwise, it aborts.
\end{enumerate}
\item \label{Consistency-check} \textbf{Consistency check}: 
\begin{enumerate}
\item \label{picking-random-x}Sender: picks a random $x_{\scriptscriptstyle s}$, and sends it to the receiver. 
\item\label{receiver-OLE-invocation} Receiver: picks random values $f,v$ and inserts them into an instance of $\mathcal{F}_{\scriptscriptstyle OLE}$, denoted by $\mathcal{F}_{\scriptscriptstyle OLE}^{\scriptscriptstyle 1}$. It inserts $(p(x_{\scriptscriptstyle s}), -s(x_{\scriptscriptstyle s})+f)$ into another instance of $\mathcal{F}_{\scriptscriptstyle OLE}$, say $\mathcal{F}_{\scriptscriptstyle OLE}^{\scriptscriptstyle 2}$. 
\item\label{inserting-to-OLE} Sender: picks a random value $t$, and inserts it to $\mathcal{F}_{\scriptscriptstyle OLE}^{\scriptscriptstyle 1}$ that sends $c=f\cdot t+v$ to  the sender. It also inputs $r(x_{\scriptscriptstyle s})$ into $\mathcal{F}_{\scriptscriptstyle OLE}^{\scriptscriptstyle 2}$ that sends   $\bar{f}=r(x_{\scriptscriptstyle s})\cdot p(x_{\scriptscriptstyle s})-s(x_{\scriptscriptstyle s})+f$ to the sender which sums it with $u(x_{\scriptscriptstyle s})$. This   yields $f'= r(x_{\scriptscriptstyle s})\cdot p(x_{\scriptscriptstyle s})-s(x_{\scriptscriptstyle s})+f+u(x_{\scriptscriptstyle s})$. The sender sends $f'$ to the receiver.
\item\label{receiver-check} Receiver: It aborts if $f'\neq f$; otherwise, it sends $v$ to the sender. 
\item Sender: It aborts if $f'\cdot t+v\neq c$
\end{enumerate}
\item Receiver: picks $x_{\scriptscriptstyle r}$ and runs similar consistency check with the sender. 
}
\end{enumerate}
\end{boxedminipage}
\end{center}
\caption{Oblivious Polynomial Addition (OPA)  in \cite{GhoshN19}} 
\label{fig:OPA}
\end{figure}

%Note that when protocol OPA is used in the PSI protocols, $b(x)$ is a polynomial representing the receiver's set elements. 

In this section, we explain an attack that can be carried out in OPA protocol. We observed that a malicious sender can use OPA as a subroutine to guess one of the receiver's set elements without being caught with a non-negligible probability (i.e.,  probability  independent of the security parameter). In short,  the source of the issue is that the sender is given the ability to independently pick a random value (and send it to the receiver who evaluates its polynomial on the value) that allows a malicious sender to pick a value of its choice, instead of a truly random value.  In particular, both parties take steps \ref{sender-evaluate} and \ref{computing-receiver} honestly. However, in step \ref{picking-random-x}, the malicious sender instead of picking a uniformly random value: $x_{\scriptscriptstyle s}$, it  guesses an element of the receiver's set, e.g. $x'_{\scriptscriptstyle s}$, and sends that value to the  honest receiver who (given  $x'_{\scriptscriptstyle s}$) follows the protocol in step \ref{receiver-OLE-invocation}.   But, in step \ref{inserting-to-OLE}, the malicious sender instead of inserting $r(x'_{\scriptscriptstyle s})$ to $\mathcal{F}_{\scriptscriptstyle OPA}^{\scriptscriptstyle 2}$, it inserts an arbitrary value, $w'$, to $\mathcal{F}_{\scriptscriptstyle OPA}^{\scriptscriptstyle 2}$, where $w'\neq r(x'_{\scriptscriptstyle s})$. In this case, $\mathcal{F}_{\scriptscriptstyle OPA}^{\scriptscriptstyle 2}$ outputs $\bar{f}= w'\cdot p(x'_{\scriptscriptstyle s})-s(x'_{\scriptscriptstyle s})+f$ to the sender which adds the output  with $u(x'_{\scriptscriptstyle s})$ which yields:

\begin{align*}
\begin{split}
  f&'= w'\cdot p(x'_{\scriptscriptstyle s})-s(x'_{\scriptscriptstyle s})+f+u(x'_{\scriptscriptstyle s})\\
  %%
  &=w'\cdot p(x'_{\scriptscriptstyle s})-p(x'_{\scriptscriptstyle s})\cdot r(x'_{\scriptscriptstyle s})+f
  \end{split}
  \end{align*}
  
  Note that, if it correctly guesses the set element, then $p(x'_{\scriptscriptstyle s})=0$, which means $f'=f$; therefore, it can pass the check in step \ref{receiver-check}. The probability that a malicious sender correctly guesses the receiver's set element is at least $Pr=\frac{1}{|\mathcal{U}|}$, where $\mathcal{U}$ is the universe of set elements. This probability is based on the assumption that all set elements have the same distribution, which is not always the case. It is possible that a certain element, $x'_{\scriptscriptstyle s}$, has a higher chance than other elements of the universe to be in a set; in this case, the probability of correctly guessing that element can be even higher, i.e. $Pr\geq \frac{1}{|\mathcal{U}|}$.

To address the issue, one might be tempted to replace $\mathcal{F}_{\scriptscriptstyle OLE}^{\scriptscriptstyle 2}$ by $ \mathcal{F}_{\mathtt{OLE}^{\scriptscriptstyle +}}$ in step \ref{receiver-OLE-invocation} to prevent the honest  receiver from sending  $p(x'_{\scriptscriptstyle s})=0$ to it. However, this would not work, as $ \mathcal{F}_{\mathtt{OLE}^{\scriptscriptstyle +}}$ only ensures that when a party sends $x$ and another one sends $l,g$, the party who sends $x$ cannot learn any extra information when $x=0$. But in OPA, the honest receiver sends $l,g$ and there is no mechanism in place to prevent it from sending zero value(s). The problem can be tackled by at least two  approaches. First, we can assume that the universe of set elements is very big and all elements have the same distribution, so the adversary can guess a set element with only a negligible probability.  But, this is a rare and  strong assumption under which a PSI protocol would have very limited applications and we might be able to design a more   efficient PSI protocol.  Second, the parties can run a coin-tossing protocol  to compute $x_{\scriptscriptstyle s}$, with a small added  cost. 



%\noindent\textbf{Attack 3}: \textit{Deleting Other Client's Set Elements}.

\subsection{Attack 3: Deleting Other Client's Set Elements}

 In this section, we show how a malicious party can manipulate (i.e., delete) its counter-party's set elements without being detected. For the sake of simplicity, we first focus on deleting \emph{a single element}. Later, we will show that the malicious party can  delete \emph{multiple elements}. One of the main sources of the issue is the use of \emph{point-value} (polynomial) representation of sets.



Recall that, in the two-party PSI protocol in step \ref{first-OPA-invocation}, clients $A$ and $B$ invoke an instance of OPA such that client $A$ (as the sender) inserts  two random polynomials: $r_{\scriptscriptstyle A}, u_{\scriptscriptstyle A}$, and client $B$  (as the receiver) inserts polynomial $p_{\scriptscriptstyle B}$ (that represents its set) to OPA. In the end of this step,  OPA returns  $s_{\scriptscriptstyle B}=p_{\scriptscriptstyle B}\cdot r_{\scriptscriptstyle A}+u_{\scriptscriptstyle A}$ to client $B$.  The proposed OPA (as shown in steps \ref{sender-evaluate} and \ref{computing-receiver})  accepts  $y$-coordinates of the polynomials as input.  This means, the parties first evaluate their polynomials at every element of $\vv{\bm{x}}$ to get a set of $y$-coordinates and then send the corresponding $y$-coordinates to  OPA. However, we observed that this leads to a serious security issue; namely, a malicious sender can delete a subset of the receiver's set elements, if it manages to guess the subset. The probability of successfully mounting this attack is independent of the security parameter and only depends on the size of the elements' universe and the ability of the adversary to correctly guess the subset. This means that the probability can be high, e.g., when the set's size is not very large. Before we elaborate on the attack, we provide the following  theorem and proposition that will help to understand the attack. 

\begin{theorem}\label{theorem:Uniqueness-Interp-Poly}(Uniqueness of Interpolating Polynomial \cite{quarteroni2010numerical})
 Let $\vv{\bm{x}}= [x_{\scriptscriptstyle 1},...x_{\scriptscriptstyle h}]$ be a vector of non-zero distinct elements. For $h$ arbitrary values: $y_{\scriptscriptstyle 1},...y_{\scriptscriptstyle h}$ there is a unique polynomial: $\tau$, of degree at most $h-1$ such that: $\forall j, 1\leq j\leq h: \tau(x_{\scriptscriptstyle j})=y_{\scriptscriptstyle j}$,
 where $x_{\scriptscriptstyle j},y_{\scriptscriptstyle j}\in \mathbb{F}_{p}$.
\end{theorem}

\begin{proposition}\label{Attack3}
Let $\vv{\bm{x}}$ be a vector defined  above and $\mu\in \mathbb{F}_{p}[x]$ be a degree $d< h$ polynomial with $d$ distinct roots, i.e. $\mu=\prod\limits^{\scriptscriptstyle d}_{\scriptscriptstyle i=1}(x-e_{\scriptscriptstyle i})$, and let $\mu_{\scriptscriptstyle j}=\mu(x_{\scriptscriptstyle j}),$ where $1\leq j \leq d$. Polynomial $\mu'$ interpolated from pairs $(x_{\scriptscriptstyle 1}, \mu_{\scriptscriptstyle 1}\cdot (x_{\scriptscriptstyle 1}-e_{\scriptscriptstyle c})^{\scriptscriptstyle -1} ),..., (x_{\scriptscriptstyle h}, \mu_{\scriptscriptstyle h}\cdot (x_{\scriptscriptstyle h}-e_{\scriptscriptstyle c})^{\scriptscriptstyle -1} )$ will not have $e_{\scriptscriptstyle c}$ as  root, i.e. $\mu'(e_{\scriptscriptstyle c})\neq0$, where $1\leq c \leq d$. 
\end{proposition}


\begin{proof}
For the sake of simplicity and without loss of generality, let $c=1$. We can rewrite polynomial $\mu$ as $\mu=(x-e_{\scriptscriptstyle 1})\cdot\prod\limits^{\scriptscriptstyle d}_{\scriptscriptstyle i=2}(x-e_{\scriptscriptstyle i})$, then every $\mu_{\scriptscriptstyle j}$ ($1\leq j \leq h$) can be written as: $\mu_{\scriptscriptstyle j}=(x_{\scriptscriptstyle j}-e_{\scriptscriptstyle 1})\cdot\prod\limits^{\scriptscriptstyle d}_{\scriptscriptstyle i=2}(x_{\scriptscriptstyle j}-e_{\scriptscriptstyle i})$. Accordingly,  for every $j$, the product $\alpha_{\scriptscriptstyle j}=\mu_{\scriptscriptstyle j}\cdot (x_{\scriptscriptstyle j}-e_{\scriptscriptstyle 1})^{\scriptscriptstyle -1}$ has the following form: $\alpha_{\scriptscriptstyle j}=\mu_{\scriptscriptstyle j}\cdot (x_{\scriptscriptstyle j}-e_{\scriptscriptstyle 1})^{\scriptscriptstyle -1}=\prod\limits^{\scriptscriptstyle d}_{\scriptscriptstyle i=2}(x_{\scriptscriptstyle j}-e_{\scriptscriptstyle i})$. Let $\mu'$ be another polynomial with  $d-1$ distinct roots identical to the roots of $\mu$ excluding $e_{\scriptscriptstyle 1}$, i.e. $\mu'(e_{\scriptscriptstyle 1})\neq0$. Each $\mu'_{\scriptscriptstyle j}$ can also be written as $\mu'_{\scriptscriptstyle j}=\prod\limits^{\scriptscriptstyle d}_{\scriptscriptstyle i=2}(x_{\scriptscriptstyle j}-e_{\scriptscriptstyle i})$. Due to Theorem \ref{theorem:Uniqueness-Interp-Poly}, given $h$ pairs $(x_{\scriptscriptstyle j},\mu'_{\scriptscriptstyle j})$ there is at most one polynomial of degree at most $h-1$, such that its evaluation on  $x_{\scriptscriptstyle j}$ yields $\mu'_{\scriptscriptstyle j}$,  and that polynomial  is $\mu'$ (defined above). Since, $\mu'_{\scriptscriptstyle j}=\alpha_{\scriptscriptstyle j}$, the polynomial interpolated from $h$ pairs $(x_{\scriptscriptstyle j},\alpha_{\scriptscriptstyle j})$ is  $\mu'$ as well. Since $\mu'$ does not have $e_{\scriptscriptstyle 1}$ as  root, the polynomial interpolated from $d$ pairs $(x_{\scriptscriptstyle 1}, \mu_{\scriptscriptstyle 1}\cdot (x_{\scriptscriptstyle 1}-e_{\scriptscriptstyle 1})^{\scriptscriptstyle -1} ),..., (x_{\scriptscriptstyle h}, \mu_{\scriptscriptstyle h}\cdot (x_{\scriptscriptstyle h}-e_{\scriptscriptstyle 1})^{\scriptscriptstyle -1} )$ would not have $e_{\scriptscriptstyle 1}$ as  root either.   \hfill\(\Box\)
\end{proof}
%on every element $x_{\scriptscriptstyle j}\in \vv{\bm{x}}$; in particular,


First, we will have a closer look at  the first two steps of the original two-party PSI, i.e., Fig. \ref{fig:Two-partyPSI-Ghosh}. Let $\vv{\bm{x}}=[x_{\scriptscriptstyle 1},...,x_{\scriptscriptstyle 2d+1}]$ be a vector of distinct non-zero elements (as defined in Fig \ref{fig:OPA}). In step \ref{gen-set-rep}, each client $I\in\{A,B\}$ represents its set, containing $d$ elements, as a polynomial $p_{\scriptscriptstyle I}=\omega_{\scriptscriptstyle I}(x)\cdot \prod\limits^{\scriptscriptstyle d}_{\scriptscriptstyle j=1}(x-s^{\scriptscriptstyle (I)}_{\scriptscriptstyle j})$, where the roots of polynomial $\prod\limits^{\scriptscriptstyle d}_{\scriptscriptstyle j=1}(x-s^{\scriptscriptstyle (I)}_{\scriptscriptstyle j})$ contain the party's set elements and   $\omega_{\scriptscriptstyle I}(x)$ is a random polynomial. Each client $I$ picks three random polynomials: $r_{\scriptscriptstyle I}, u_{\scriptscriptstyle I}$, and $r'_{\scriptscriptstyle I}$. In  step  \ref{first-OPA-invocation},  client $B$ sends to OPA the polynomial that represents it set elements, i.e., polynomial $p_{\scriptscriptstyle B}(x)=\omega_{\scriptscriptstyle B}(x)\cdot\prod\limits^{\scriptscriptstyle d}_{\scriptscriptstyle i=1}(x-s^{\scriptscriptstyle(B)}_{\scriptscriptstyle i})$. This requires client $B$ to evaluate the polynomial at every element $x_{\scriptscriptstyle j}$, i.e.,   $\forall x_{\scriptscriptstyle j}\in \vv{\bm{x}}:$   $p_{\scriptscriptstyle B}(x_{\scriptscriptstyle j})=\omega_{\scriptscriptstyle B}(x_{\scriptscriptstyle j})\cdot\prod\limits^{\scriptscriptstyle d}_{\scriptscriptstyle i=1}(x_{\scriptscriptstyle j}-s^{\scriptscriptstyle(B)}_{\scriptscriptstyle i})$, and then  sends every $p_{\scriptscriptstyle B}(x_{\scriptscriptstyle j})$ to   OPA. In the same step, client $A$ sends two random polynomials  $r_{\scriptscriptstyle A}$ and $u_{\scriptscriptstyle A}$ to the same (instance of) OPA invoked by client $B$, which requires client $A$ to first evaluate each polynomial at every $x_{\scriptscriptstyle j}\in\vv{\bm{x}}$ and then  send every pair  $(u_{\scriptscriptstyle A}(x_{\scriptscriptstyle j}), r_{\scriptscriptstyle A}(x_{\scriptscriptstyle j}))$ to  OPA. 


\

Now we explain the attack in detail. We split the attack into three phases (a) set  manipulation, (b) passing OPA’s verification, and (c)  passing PSI’s verification. Below we describe each phase. 

\

 \noindent\textit{\textbf{(a) Set  Manipulation.}} In this phase,  our focus will be on the PSI protocol, presented in Fig. \ref{fig:Two-partyPSI-Ghosh}.  Assume that malicious client $A$ knows at least one of  client $B$'s set elements; for instance, element  $s^{\scriptscriptstyle(B)}_{\scriptscriptstyle 1}$. Loosely speaking, the idea is that the malicious client  generates a \emph{multiplicative inverse} of  element $s^{\scriptscriptstyle(B)}_{\scriptscriptstyle 1}$ and inserts it to OPA that  ultimately  cancels out the same element encoded in the polynomial that is  inserted by its counter-party to OPA.   In particular,  malicious client $A$ honestly follows the PSI protocol in step \ref{gen-set-rep}. However, it performs as follows in step \ref{first-OPA-invocation}.

\begin{enumerate}[label=(\roman*)]
\item\label{Set-Manipulation::pick-rand-poly}  picks a random polynomial $\bar{r}_{\scriptscriptstyle A}$, of degree $m-1$. It evaluates the polynomial at every element  $x_{\scriptscriptstyle j}\in \vv{\bm{x}}$. This results in a vector of y-coordinates: $\vv{\bm{q}}_{\scriptscriptstyle 1}=[\bar{r}_{\scriptscriptstyle A}(x_{\scriptscriptstyle 1}),...,$ $ \bar{r}_{\scriptscriptstyle A}(x_{\scriptscriptstyle 2d+1})]$.
%%
\item\label{gen-x-s}  constructs another polynomial of the following form: $x-s^{\scriptscriptstyle(B)}_{\scriptscriptstyle 1}$. It evaluates the polynomial at every element  $x_{\scriptscriptstyle j}$. This results in a vector of y-coordinates: $[(x_{\scriptscriptstyle 1}-s^{\scriptscriptstyle(B)}_{\scriptscriptstyle 1}), ..., (x_{\scriptscriptstyle 2d+1}-s^{\scriptscriptstyle(B)}_{\scriptscriptstyle 1})]$.
%%
\item\label{Set-Manipulation::gen-mul-inverse} generates the multiplicative inverse of each y-coordinate computed in  step \ref{gen-x-s}. This yields  $\vv{\bm{q}}_{\scriptscriptstyle 2}=[(x_{\scriptscriptstyle 1}-s^{\scriptscriptstyle(B)}_{\scriptscriptstyle 1})^{\scriptscriptstyle -1}, ..., (x_{\scriptscriptstyle 2d+1}-s^{\scriptscriptstyle(B)}_{\scriptscriptstyle 1})^{\scriptscriptstyle -1}]$. Note that since all polynomials and values are defined over a finite field, then every element or y-coordinate has a multiplicative inverse. 
%%
\item\label{Set-Manipulation::multipl-vect} multiplies the elements of vectors $\vv{\bm{q}}_{\scriptscriptstyle 1}$ and $\vv{\bm{q}}_{\scriptscriptstyle 2}$, component-wise. This yields $\vv{\bm{q}}_{\scriptscriptstyle 3}=[\bar{r}_{\scriptscriptstyle A}(x_{\scriptscriptstyle 1})\cdot(x_{\scriptscriptstyle 1}-s^{\scriptscriptstyle(B)}_{\scriptscriptstyle 1})^{\scriptscriptstyle -1},..., \bar{r}_{\scriptscriptstyle A}(x_{\scriptscriptstyle 2d+1})\cdot (x_{\scriptscriptstyle 2d+1}-s^{\scriptscriptstyle(B)}_{\scriptscriptstyle 1})^{\scriptscriptstyle -1}]$.
%%
\item\label{Set-Manipulation::eval-u}  evaluates the random polynomial $u_{\scriptscriptstyle A}$, generated honestly in step \ref{gen-set-rep}, at every element $x_{\scriptscriptstyle j}$, which results in $\vv{\bm{q}}_{\scriptscriptstyle 4}=[u_{\scriptscriptstyle A}(x_{\scriptscriptstyle 1}),..., u_{\scriptscriptstyle A}(x_{\scriptscriptstyle 2d+1})]$. 


\item\label{Set-Manipulation::send} sends every pair $(q_{\scriptscriptstyle 4,j}, q_{\scriptscriptstyle 3,j})$ to OPA, where $q_{\scriptscriptstyle 4,j}\in \vv{\bm{q}}_{\scriptscriptstyle 4}$ and  $q_{\scriptscriptstyle 3,j}\in \vv{\bm{q}}_{\scriptscriptstyle 3}$. 
\end{enumerate}

That means  malicious client $A$ instead of sending   $r_{\scriptscriptstyle A}(x_{\scriptscriptstyle j})$, it now  sends $q_{\scriptscriptstyle 3,j}=\bar{r}_{\scriptscriptstyle A}(x_{\scriptscriptstyle j})\cdot (x_{\scriptscriptstyle j}-s^{\scriptscriptstyle(B)}_{\scriptscriptstyle 1})^{\scriptscriptstyle -1}$ to OPA. In this case, OPA, in step \ref{first-OPA-invocation},  returns the following values to honest client $B$. $\forall j, 1\leq j \leq 2d+1:$







%As stated above, client $B$ inserts  polynomial $p_{\scriptscriptstyle B}$ to OPA, where the polynomial has the form $p_{\scriptscriptstyle B}=\omega_{\scriptscriptstyle B}\cdot\prod\limits^{\scriptscriptstyle d}_{\scriptscriptstyle i=1}(x-s^{\scriptscriptstyle(B)}_{\scriptscriptstyle i})$,  values $s^{\scriptscriptstyle(B)}_{\scriptscriptstyle i}$ are client $B$'s set elements and $\omega_{\scriptscriptstyle B}$ is a random polynomial. Client $B$ in
%
%
% step \ref{first-OPA-invocation}, ($\forall j, 1\leq j\leq h$) sends  $p_{\scriptscriptstyle B}(x_{\scriptscriptstyle j})=\omega_{\scriptscriptstyle B}(x_{\scriptscriptstyle j})\cdot\prod\limits^{\scriptscriptstyle d}_{\scriptscriptstyle i=1}(x_{\scriptscriptstyle j}-s^{\scriptscriptstyle(B)}_{\scriptscriptstyle i})$ while client $A$ sends $r_{\scriptscriptstyle A}(x_{\scriptscriptstyle j})$ and $u_{\scriptscriptstyle A}(x_{\scriptscriptstyle j})$ to  OPA.  Assume that malicious client $A$ knows at least one of  client $B$ set elements, e.g. $s^{\scriptscriptstyle(B)}_{\scriptscriptstyle 1}$. In this case, client $A$ replaces $r_{\scriptscriptstyle A}(x_{\scriptscriptstyle j})$ with $r_{\scriptscriptstyle j}=r'_{\scriptscriptstyle A}(x_{\scriptscriptstyle j})\cdot (x_{\scriptscriptstyle j}-s^{\scriptscriptstyle(B)}_{\scriptscriptstyle 1})^{\scriptscriptstyle -1}$, where $r'_{\scriptscriptstyle A}$ is a random polynomial. Next, client $A$ sends $r_{\scriptscriptstyle j}$ and $u_{\scriptscriptstyle A}(x_{\scriptscriptstyle j})$ to OPA that returns:


\begin{align}\label{equation:OPA}
\begin{split}
%%
y_{\scriptscriptstyle j}&=p_{\scriptscriptstyle B}(x_{\scriptscriptstyle j})\cdot q_{\scriptscriptstyle 3,j}+q_{\scriptscriptstyle 4,j}\\
%%
&= \underbrace{\Big(\omega_{\scriptscriptstyle B}(x_{\scriptscriptstyle j})\cdot (x_{\scriptscriptstyle j}-s^{\scriptscriptstyle(B)}_{\scriptscriptstyle 1})\cdot \prod\limits^{\scriptscriptstyle d}_{\scriptscriptstyle i=2}(x_{\scriptscriptstyle j}-s^{\scriptscriptstyle(B)}_{\scriptscriptstyle i})\Big)}_{p_{\scriptscriptstyle B}(x_{\scriptscriptstyle j})}\cdot \underbrace{\Big(\bar{r}_{\scriptscriptstyle A}(x_{\scriptscriptstyle j})\cdot (x_{\scriptscriptstyle j}-s^{\scriptscriptstyle(B)}_{\scriptscriptstyle 1})^{\scriptscriptstyle -1}\Big)}_{ q_{\scriptscriptstyle 3,j}}+\underbrace{u_{\scriptscriptstyle A}(x_{\scriptscriptstyle j})}_{q_{\scriptscriptstyle 4,j}}\\
%%
&= {\Big(\omega_{\scriptscriptstyle B}(x_{\scriptscriptstyle j})\cdot \prod\limits^{\scriptscriptstyle d}_{\scriptscriptstyle i=2}(x_{\scriptscriptstyle j}-s^{\scriptscriptstyle(B)}_{\scriptscriptstyle i})\Big)}\cdot \Big(\bar{r}_{\scriptscriptstyle A}(x_{\scriptscriptstyle j})\Big)+u_{\scriptscriptstyle A}(x_{\scriptscriptstyle j})\\
\end{split}
\end{align}


\


\

%
%&= \Big(\omega_{\scriptscriptstyle B}(x_{\scriptscriptstyle j})\cdot\prod\limits^{\scriptscriptstyle d}_{\scriptscriptstyle i=1}(x_{\scriptscriptstyle j}-s^{\scriptscriptstyle(B)}_{\scriptscriptstyle i})\Big)\cdot \Big(r'_{\scriptscriptstyle A}(x_{\scriptscriptstyle j})\cdot (x_{\scriptscriptstyle j}-s^{\scriptscriptstyle(B)}_{\scriptscriptstyle 1})^{\scriptscriptstyle -1}\Big)+u_{\scriptscriptstyle A}(x_{\scriptscriptstyle j})\\

%\overbrace{\beta\circ \beta\circ... \circ \beta}_{\scriptscriptstyle k \text{\ \ Times}}

%\begin{equation}\label{equation:OPA}
%s'_{\scriptscriptstyle B}(x_{\scriptscriptstyle j})=p_{\scriptscriptstyle B}(x_{\scriptscriptstyle j})\cdot r_{\scriptscriptstyle j}+u_{\scriptscriptstyle A}(x_{\scriptscriptstyle j})= \omega_{\scriptscriptstyle B}(x_{\scriptscriptstyle j})\cdot  r'_{\scriptscriptstyle A}(x_{\scriptscriptstyle j}) \cdot\prod\limits^{\scriptscriptstyle d}_{\scriptscriptstyle i=2}(x_{\scriptscriptstyle j}-s^{\scriptscriptstyle(B)}_{\scriptscriptstyle i})+u_{\scriptscriptstyle A}(x_{\scriptscriptstyle j})
% \end{equation}

Client $B$, in step \ref{first-OPA-invocation}, uses pairs ($x_{\scriptscriptstyle j},y_{\scriptscriptstyle j}$) to interpolate a polynomial, $s'_{\scriptscriptstyle B}$, that has the following form.

\begin{equation}\label{equation:s-prime-B}
s'_{\scriptscriptstyle B}={\Big(\omega_{\scriptscriptstyle B}(x)\cdot \prod\limits^{\scriptscriptstyle d}_{\scriptscriptstyle i=2}(x-s^{\scriptscriptstyle(B)}_{\scriptscriptstyle i})\Big)}\cdot \Big(\bar{r}_{\scriptscriptstyle A}(x)\Big)+u_{\scriptscriptstyle A}(x)
\end{equation}


 According to Equations \ref{equation:OPA} and \ref{equation:s-prime-B}  and  Proposition \ref{Attack3},  malicious client $A$ has managed to remove the set element, $s^{\scriptscriptstyle(B)}_{\scriptscriptstyle 1}$, which ultimately leads to the elimination of the element from the final result, i.e., the sets' intersection. In particular, client $A$ follows the PSI protocol in steps \ref{2nd-OPA-invocation} and \ref{gen-s-A-prime}, it  computes $s'_{\scriptscriptstyle A}=s_{\scriptscriptstyle A}-u_{\scriptscriptstyle A}+p_{\scriptscriptstyle A}\cdot r'_{\scriptscriptstyle A}$ honestly, and sends $s'_{\scriptscriptstyle A}$ to honest client $B$.  Given the interpolated polynomial, $s'_{\scriptscriptstyle B}$, and  polynomial $s'_{\scriptscriptstyle A}$,  client $B$, in step \ref{where-clientB-deviates1}, follows the protocol and computes the result  polynomial (presented below) that is supposed to encode the sets' intersection. 
  
  
  

  \begin{align}\label{equation:result-poly}
  \begin{split}
  p_{\scriptscriptstyle \cap}&=s'_{\scriptscriptstyle A}+s'_{\scriptscriptstyle B}+p_{\scriptscriptstyle B}\cdot r'_{\scriptscriptstyle B}-u_{\scriptscriptstyle B}\\
    %%
  &=p_{\scriptscriptstyle A}\cdot r'_{\scriptscriptstyle A}+p_{\scriptscriptstyle A}\cdot r_{\scriptscriptstyle B}+{\Big(\omega_{\scriptscriptstyle B}\cdot \prod\limits^{\scriptscriptstyle d}_{\scriptscriptstyle i=2}(x-s^{\scriptscriptstyle(B)}_{\scriptscriptstyle i})\Big)}\cdot \bar{r}_{\scriptscriptstyle A}+p_{\scriptscriptstyle B}\cdot r'_{\scriptscriptstyle B}
    \end{split}
  \end{align}

  However, as it is evident in Equation \ref{equation:result-poly}, the result polynomial's roots do not include element $s^{\scriptscriptstyle(B)}_{\scriptscriptstyle 1}$, even if both clients' sets contain it, as roots of polynomial $\Big(\omega_{\scriptscriptstyle B}\cdot \prod\limits^{\scriptscriptstyle d}_{\scriptscriptstyle i=2}(x-s^{\scriptscriptstyle(B)}_{\scriptscriptstyle i})\Big)$ lack that element due to  malicious client $A$'s manipulation described above.  
  
In order for  malicious client $A$ to succeed, it also needs to pass two verifications, one in the OPA and the other in the PSI scheme. Below, we explain how it can do so. 
  
  
  % p_{\scriptscriptstyle A}\cdot r'_{\scriptscriptstyle A}+p_{\scriptscriptstyle A}\cdot r_{\scriptscriptstyle B}+p_{\scriptscriptstyle B}\cdot r_{\scriptscriptstyle A}+p_{\scriptscriptstyle B}\cdot r'_{\scriptscriptstyle B}$. 
  

 \
  
 \noindent\textit{\textbf{(b) Passing OPA's Verification.}} Now, we show how  malicious client $A$ can   pass the verifications in OPA, using the following trick. Therefore, we will focus on the OPA protocol. Since,  we have already covered steps \ref{sender-evaluate} and \ref{computing-receiver} in OPA (when we explained steps \ref{first-OPA-invocation} and \ref{2nd-OPA-invocation} in the two-party PSI)   we will only focus on the ``consistency check'' in this protocol. Briefly, clients $A$ and $B$ honestly follow the OPA protocol in steps \ref{picking-random-x}  and  \ref{receiver-OLE-invocation}. In particular, malicious client $A$ (as sender) in step \ref{picking-random-x} honestly picks a random value $x_{\scriptscriptstyle s}$ and sends it to honest client $B$ (as receiver). Then, client $B$, in step \ref{receiver-OLE-invocation}, picks random values $f,v$ and inserts them into  $\mathcal{F}_{\scriptscriptstyle OLE}^{\scriptscriptstyle 1}$. Client $B$ also inserts $(p_{\scriptscriptstyle B}(x_{\scriptscriptstyle s}), -s'_{\scriptscriptstyle B}(x_{\scriptscriptstyle s})+f)$ into  $\mathcal{F}_{\scriptscriptstyle OLE}^{\scriptscriptstyle 2}$. Recall, $s'_{\scriptscriptstyle B}$ is the polynomial which was defined  in Equation \ref{equation:s-prime-B}. 
  
  
  
  
 
Client $A$ in step \ref{inserting-to-OLE} honestly picks a random value $t$, and inserts it to $\mathcal{F}_{\scriptscriptstyle OLE}^{\scriptscriptstyle 1}$ that sends $c=f\cdot t+v$  back to  the same client. However, client $A$ in the same step,  sends $\bar{r}_{\scriptscriptstyle A}(x_{\scriptscriptstyle s})\cdot (x_{\scriptscriptstyle s}-s^{\scriptscriptstyle(B)}_{\scriptscriptstyle 1})^{\scriptscriptstyle -1}$, instead of $r_{\scriptscriptstyle A}(x_{\scriptscriptstyle s})$,  to $\mathcal{F}_{\scriptscriptstyle OLE}^{\scriptscriptstyle 2}$ that returns the following value to client $A$.


\begin{align}\label{equation:pass-ver-OPA}
\begin{split}
\bar{f}&= \bar{r}_{\scriptscriptstyle A}(x_{\scriptscriptstyle s})\cdot (x_{\scriptscriptstyle s}-s^{\scriptscriptstyle(B)}_{\scriptscriptstyle 1})^{\scriptscriptstyle -1}\cdot p_{\scriptscriptstyle B}(x_{\scriptscriptstyle s})-s'_{\scriptscriptstyle B}(x_{\scriptscriptstyle s})+f\\
%%
&=\bar{r}_{\scriptscriptstyle A}(x_{\scriptscriptstyle s})\cdot (x_{\scriptscriptstyle s}-s^{\scriptscriptstyle(B)}_{\scriptscriptstyle 1})^{\scriptscriptstyle -1}\cdot    \underbrace{\Big(\omega_{\scriptscriptstyle B}(x_{\scriptscriptstyle s})\cdot (x_{\scriptscriptstyle s}-s^{\scriptscriptstyle(B)}_{\scriptscriptstyle 1})\cdot \prod\limits^{\scriptscriptstyle d}_{\scriptscriptstyle i=2}(x_{\scriptscriptstyle s}-s^{\scriptscriptstyle(B)}_{\scriptscriptstyle i})\Big)}_{p_{\scriptscriptstyle B}(x_{s})}-s'_{\scriptscriptstyle B}(x_{\scriptscriptstyle s})+f\\
%%
&=\bar{r}_{\scriptscriptstyle A}(x_{\scriptscriptstyle s})\cdot   \Big(\omega_{\scriptscriptstyle B}(x_{\scriptscriptstyle s})\cdot  \prod\limits^{\scriptscriptstyle d}_{\scriptscriptstyle i=2}(x_{\scriptscriptstyle s}-s^{\scriptscriptstyle(B)}_{\scriptscriptstyle i})\Big)-s'_{\scriptscriptstyle B}(x_{\scriptscriptstyle s})+f\\
%&=\bar{r}_{\scriptscriptstyle A}(x_{\scriptscriptstyle s})\cdot   \Big(\omega_{\scriptscriptstyle B}(x_{\scriptscriptstyle s})\cdot  \prod\limits^{\scriptscriptstyle d}_{\scriptscriptstyle i=2}(x_{\scriptscriptstyle s}-s^{\scriptscriptstyle(B)}_{\scriptscriptstyle i})\Big)-\underbrace{{\Big(\omega_{\scriptscriptstyle B}(x)\cdot \prod\limits^{\scriptscriptstyle d}_{\scriptscriptstyle i=2}(x-s^{\scriptscriptstyle(B)}_{\scriptscriptstyle i})\Big)}\cdot \Big(\bar{r}_{\scriptscriptstyle A}(x)\Big)+u_{\scriptscriptstyle A}(x)}_{s'_{\scriptscriptstyle B}(x_{\scriptscriptstyle s})}+f\\
%%s'_{\scriptscriptstyle B}={\Big(\omega_{\scriptscriptstyle B}(x)\cdot \prod\limits^{\scriptscriptstyle d}_{\scriptscriptstyle i=2}(x-s^{\scriptscriptstyle(B)}_{\scriptscriptstyle i})\Big)}\cdot \Big(\bar{r}_{\scriptscriptstyle A}(x)\Big)+u_{\scriptscriptstyle A}(x)
&=-u_{\scriptscriptstyle A}(x_{\scriptscriptstyle s})+f
 \end{split}
 \end{align}

%   \underbrace{\Big(\omega_{\scriptscriptstyle B}(x_{\scriptscriptstyle j})\cdot (x_{\scriptscriptstyle j}-s^{\scriptscriptstyle(B)}_{\scriptscriptstyle 1})\cdot \prod\limits^{\scriptscriptstyle d}_{\scriptscriptstyle i=2}(x_{\scriptscriptstyle j}-s^{\scriptscriptstyle(B)}_{\scriptscriptstyle i})\Big)}_{p_{\scriptscriptstyle B}}
  
  % \underbrace{\Big(\omega_{\scriptscriptstyle B}(x_{\scriptscriptstyle j})\cdot (x_{\scriptscriptstyle j}-s^{\scriptscriptstyle(B)}_{\scriptscriptstyle 1})\cdot \prod\limits^{\scriptscriptstyle d}_{\scriptscriptstyle i=2}(x_{\scriptscriptstyle j}-s^{\scriptscriptstyle(B)}_{\scriptscriptstyle i})\Big)}_{p_{\scriptscriptstyle B}}
  
 Recall,  polynomial $p_{\scriptscriptstyle B}$, that was inserted by client $B$,  encodes all set elements of client $B$, including $s_{\scriptscriptstyle 1}^{\scriptscriptstyle(B)}$, whereas polynomial $s'_{\scriptscriptstyle B}$ misses that specific element (due to the client $A$'s manipulation in Equation \ref{equation:OPA}). However, as it is indicated in Equation \ref{equation:pass-ver-OPA}, client $A$ has managed  to remove $s_{\scriptscriptstyle 1}^{\scriptscriptstyle(B)}$ from $p_{\scriptscriptstyle B}(x_{\scriptscriptstyle s})$. This will allow client $A$ to escape from being detected, because the result (i.e., $\bar{f}=-u_{\scriptscriptstyle A}(x_{\scriptscriptstyle s})+f$) is what an honest client $A$ would have computed.  Malicious client $A$ completes step \ref{inserting-to-OLE} honestly, by  adding $u(x_{\scriptscriptstyle s})$ to $\bar{f}$, i.e., it computes $f'=\bar{f}+u_{\scriptscriptstyle A}(x_{\scriptscriptstyle s})=f$, and sending $f'$ to client $B$, which checks $f'$ equals the random value it initially picked in step \ref{receiver-OLE-invocation}, i.e., $f$. It is not hard to see that $f'=f$. Hence,  malicious client $A$ has managed to pass this verification. 
   
   
\




  
   \noindent\textit{\textbf{(c) Passing PSI's Verification.}} Next, we show how  malicious client  $A$ can also pass the verification in the PSI protocol (i.e., in step \ref{two-party-PSI::what-A-sends-in-ver} in Fig. \ref{fig:Two-partyPSI-Ghosh}) even though it has manipulated client $B$'s input. Our focus will be on the ``output verification'' in the PSI protocol.   At a high level, to pass this verification, client $A$ uses the same trick it used to pass the verification in OPA. Specifically, in step \ref{two-party-PSI::agree-on-random-vals} both parties honestly agree on two values $z$ and $q$. Then, in step \ref{where-clientB-deviates2}, client $B$ honestly computes $\alpha_{\scriptscriptstyle B}$, $\beta_{\scriptscriptstyle B}$, and $\delta_{\scriptscriptstyle B}$ and sends them to client $A$ which ignores the values and  skips step \ref{checks-on-computingPSI}.  Malicious client $A$, in step \ref{two-party-PSI::what-A-sends-in-ver}, honestly generates $\alpha_{\scriptscriptstyle A}=p_{\scriptscriptstyle A}(q)$ and $\delta_{\scriptscriptstyle A}=r'_{\scriptscriptstyle A}(q)$; however, instead of  setting     $\beta_{\scriptscriptstyle A}=r_{\scriptscriptstyle A}(q)$, it sets     $\beta_{\scriptscriptstyle A}=\bar{r}_{\scriptscriptstyle A}(q)\cdot (q-s^{\scriptscriptstyle(B)}_{\scriptscriptstyle 1})^{\scriptscriptstyle -1}$. It sends $\alpha_{\scriptscriptstyle A}$, $\delta_{\scriptscriptstyle A}$, and $\beta_{\scriptscriptstyle A}$  to client $B$ which acts honestly in step \ref{checks-on-computingPSI-byB}. In particular, it:
   
   \begin{enumerate}
 \item evaluates the result polynomial, $p_{\scriptscriptstyle \cap}$, at $q$ which yields: 
   
   
 $$p_{\scriptscriptstyle \cap}(q)=p_{\scriptscriptstyle A}(q) \cdot r'_{\scriptscriptstyle A}(q)+p_{\scriptscriptstyle A}(q)\cdot r_{\scriptscriptstyle B}(q)+{\Big(\omega_{\scriptscriptstyle B}(q)\cdot \prod\limits^{\scriptscriptstyle d}_{\scriptscriptstyle i=2}(q-s^{\scriptscriptstyle(B)}_{\scriptscriptstyle i})\Big)}\cdot \bar{r}_{\scriptscriptstyle A}(q)+p_{\scriptscriptstyle B}(q)\cdot r'_{\scriptscriptstyle B}(q)$$
 
   \item generates $t$ as below (given the three messages, sent by client $A$):
   


\begin{align*}
\begin{split}
t&=p_{\scriptscriptstyle B}(q)\cdot(\beta_{\scriptscriptstyle A}+r'_{\scriptscriptstyle B}(q))+\alpha_{\scriptscriptstyle A}\cdot(r_{\scriptscriptstyle B}(q)+\delta_{\scriptscriptstyle A})\\
%%
   &=    \Big(\omega_{\scriptscriptstyle B}(q)\cdot \prod\limits^{\scriptscriptstyle d}_{\scriptscriptstyle i=2}(q-s^{\scriptscriptstyle(B)}_{\scriptscriptstyle i})\Big) \cdot \bar{r}_{\scriptscriptstyle A}(q)+ p_{\scriptscriptstyle B}(q)\cdot r'_{\scriptscriptstyle B}(q)+\alpha_{\scriptscriptstyle A}\cdot r_{\scriptscriptstyle B}(q)+ \alpha_{\scriptscriptstyle A}\cdot \delta_{\scriptscriptstyle A}
\end{split}
\end{align*}   
   %
   \item checks if $p_{\scriptscriptstyle \cap}(q)$ equals  $t$ (i.e., $p_{\scriptscriptstyle \cap}(q)\stackrel{\scriptscriptstyle ?}=t$) and accepts the result if the check is passes. 
   \end{enumerate}
   
   As indicated above,  malicious client $A$ (using the above trick) can pass the verification in the PSI protocol and convince client $B$ to accept the manipulated result. 
   
   
   
   \
   
\noindent\textit{\textbf{Deleting Multiple Elements.}} Now we briefly outline how  malicious client $A$ can delete multiple elements from its counter-party's set during the computation of the sets' intersection. Let $S'=\{s^{\scriptscriptstyle (B)}_{\scriptscriptstyle 1},...,s^{\scriptscriptstyle (B)}_{\scriptscriptstyle n}\}$ be a set of elements that malicious client $A$ wants to delete from client $B$'s set, where $n\leq m$. In the ``set manipulation'' phase, in step \ref{Set-Manipulation::pick-rand-poly},  client $A$  picks a random polynomial $\bar{r}_{\scriptscriptstyle A}$ that now has a degree $m-n$. It performs as before in the rest of the same rest. In step \ref{gen-x-s}, it constructs a polynomial that now has the following form: $\prod\limits^{\scriptscriptstyle n}_{\scriptscriptstyle i=1}(x-s^{\scriptscriptstyle (B)}_{\scriptscriptstyle i})$, where $ s^{\scriptscriptstyle (B)}_{\scriptscriptstyle i}\in S'$. In the same step, it evaluates the polynomial at every element $x_{\scriptscriptstyle j}$ which yields $[\prod\limits^{\scriptscriptstyle n}_{\scriptscriptstyle i=1}(x_{\scriptscriptstyle 1}-s^{\scriptscriptstyle (B)}_{\scriptscriptstyle i}),..., \prod\limits^{\scriptscriptstyle n}_{\scriptscriptstyle i=1}(x_{\scriptscriptstyle 2d+1}-s^{\scriptscriptstyle (B)}_{\scriptscriptstyle i})]$. It takes the rest of  steps \ref{Set-Manipulation::gen-mul-inverse}-\ref{Set-Manipulation::send} as previously described in the set manipulation phase. The ``passing OPA’s verification'' phase remains unchanged with the exception that, in step \ref{inserting-to-OLE}, client $A$ now sends $\bar{r}_{\scriptscriptstyle A}(x_{\scriptscriptstyle s})\cdot \prod\limits^{\scriptscriptstyle n}_{\scriptscriptstyle i=1}(x_{\scriptscriptstyle s}-s^{\scriptscriptstyle (B)}_{\scriptscriptstyle i})^{\scriptscriptstyle -1}$  to $\mathcal{F}_{\scriptscriptstyle OLE}^{\scriptscriptstyle 2}$. Similarly,  the ``passing PSI’s verification'' phase remains the same as before, with a difference that, in step \ref{two-party-PSI::what-A-sends-in-ver}, malicious client $A$ now sets     $\beta_{\scriptscriptstyle A}= \bar{r}_{\scriptscriptstyle A}(q)\cdot \prod\limits^{\scriptscriptstyle n}_{\scriptscriptstyle i=1}(q-s^{\scriptscriptstyle (B)}_{\scriptscriptstyle i})^{\scriptscriptstyle -1}$. Thus,  malicious client $A$ can delete multiple elements of client $B$ and pass the verifications.
   
   
   
%  \begin{align}\label{equation:result-poly}
%  \begin{split}
%  p_{\scriptscriptstyle \cap}&=s'_{\scriptscriptstyle A}+s'_{\scriptscriptstyle B}+p_{\scriptscriptstyle B}\cdot r'_{\scriptscriptstyle B}-u_{\scriptscriptstyle B}\\
%    %%
%  &=p_{\scriptscriptstyle A}\cdot r'_{\scriptscriptstyle A}+p_{\scriptscriptstyle A}\cdot r_{\scriptscriptstyle B}+{\Big(\omega_{\scriptscriptstyle B}(x_{\scriptscriptstyle j})\cdot \prod\limits^{\scriptscriptstyle d}_{\scriptscriptstyle i=2}(x_{\scriptscriptstyle j}-s^{\scriptscriptstyle(B)}_{\scriptscriptstyle i})\Big)}\cdot \bar{r}_{\scriptscriptstyle A}+p_{\scriptscriptstyle B}\cdot r'_{\scriptscriptstyle B}
%    \end{split}
%  \end{align}

   
   
   
   
   
   
   
   
   
%   
%   
%Client $A$ sends $\alpha_{\scriptscriptstyle A}=p_{\scriptscriptstyle A}(q)$, $\beta_{\scriptscriptstyle A}=r_{\scriptscriptstyle A}(q)$, and $\delta_{\scriptscriptstyle A}=r'_{\scriptscriptstyle A}(q)$ to client $B$.

% \item\label{checks-on-computingPSI-byB} Client $B$:  checks if:   $p_{\cap}(q)\stackrel{?}=p_{\scriptscriptstyle B}(q)\cdot(\beta_{A}+r'_{\scriptscriptstyle B}(q))+\alpha_{\scriptscriptstyle A}\cdot(r_{\scriptscriptstyle B}(q)+\delta_{\scriptscriptstyle A})$
   
   
   
   
   
   
   
   
   
%   can utilise the  trick  above to pass the verification  in the  PSI protocol (i.e. step \ref{checks-on-computingPSI-byB} in Fig. \ref{fig:Two-partyPSI-Ghosh}) too. In particular, given a fresh random challenge: $x_{\scriptscriptstyle B}$, it sends $r'_{\scriptscriptstyle A}(x_{\scriptscriptstyle B})\cdot (x_{\scriptscriptstyle B}-s^{\scriptscriptstyle(B)}_{\scriptscriptstyle 1})^{\scriptscriptstyle -1}$, instead of $r_{\scriptscriptstyle A}(x_{\scriptscriptstyle B})$,  to client $B$.
%  



\




\subsection{Technical Issue } Another issue in OPA protocol is that the receiver in step \ref{computing-receiver} checks the degree of  polynomial $s(x)$ after it interpolates the polynomial from $m+1$ pairs $(x_{\scriptscriptstyle j},s_{\scriptscriptstyle j} )$ and it aborts if $deg(s)>2d$. The protocol's proof also highly depends on this check. Nonetheless,  according to Theorem \ref{theorem:Uniqueness-Interp-Poly}, there exists a  polynomial that  \emph{always} have a degree at most $2d$. Thus, the check in step \ref{computing-receiver}  does not work and is always passed.



%\noindent\textbf{Technical issue }2: As stated above, in \cite{} $OLE$ is used to combine the sender polynomials:   $a(x)$ and $r(x)$ with the receiver polynomial $b(x)$ where $deg(b)=deg(r)=d$ and $deg(a)=2d$. In particular, parties first agree on a public vector: $\vv{\bm{x}}=[x_{\scriptscriptstyle 1},...x_{\scriptscriptstyle 2d+1}]$ with distinct non-zero values. Then, each party evaluates its polynomial at every element of $\vv{\bm{x}}$. This yields values $a_{\scriptscriptstyle i}, r_{\scriptscriptstyle i}$ and $b_{\scriptscriptstyle i}$. Then (for every $i, 1\leq i\leq 2d+1$), the sender sends $a_{\scriptscriptstyle i}, r_{\scriptscriptstyle i}$ to OLE while the receiver sends $b_{\scriptscriptstyle i}$ to OLE that outputs $b_{\scriptscriptstyle i}, \cdot r_{\scriptscriptstyle i}+a_{\scriptscriptstyle i}$ to the receiver who can use them to interpolate a polynomial $s(x)$. In the case where the receiver sets $b(x)=0$ and sends only zero values to  OLE, the parties can agree on a random value $z$ (via coin tossing). Then, the sender computes $a(z)$ and $r(z)$, commitments to them and  sends the commitments to the receiver who sends $s(z)$ and $r(z)$ to the sender. At this point the sender sends the opening of the  commitments to the sender. The parties do the following checks (a) all the messages they received are non-zero and $s(z)\stackrel{?}=r(z)\cdot b(z)+a(z)$.  The authors (on page  158) argued that the sender may not set its polynomial to zero, instead it sends $d$ zeros among $d+1$ non-zero values to OLE.  This allows the receiver to learn $d$ y-coordinates of $a(x)$. They stated that $d$ y-coordinates plus the one it gets from the check, i.e. $a(z),$ allows the receiver to fully recover $a(x)$. However, we highlight that this is not the case. The reason is that the degree of $a(x)$ is $2d$ therefore at least $2d+1$ y-coordinates are required to interpolate $a(x)$. Moreover, the receiver may insert $n>d$ zeros to OLE. This means that the degree of $r(x)$ is now at least $n$, which leads to a result polynomial of degree at least $d+n>2d$. Nevertheless, the receiver has only $2d+1$ y-coordinates to interpolate a polynomial, so the polynomial it interpolates $s'(x)$ would not be equal to $s(x)=r(x)\cdot b(x)+a(x)$. That means it cannot pass the above check without the knowledge of $r(x)$ and $a(x)$ (or their y-coordinates) (xxxx needs to be proven). Therefore, the only way for the adversary to learn $a(x)$ is to set $r(x)=0$ which can be detected in the above check. We conclude that the $OLE$ would suffice and $OLE^{+}$ is not needed.

%to allow client $A$ perform the check, they agree on a fresh random value, client $A$ computes and sends to client $B$ the following values: $\alpha_A=p_{A}(z)$, $\beta_{A}=r_{A}(z)$, and $\delta_{A}=r'_A(z)$. Now client $B$ checks $\phi(z)\stackrel{?}=p_{B}(z)\cdot(\beta_{A}+r'_{B}(z))+\alpha_{A}\cdot(r_{B}(z)+\delta_{A})$










==> old-evaluation-table.tex <==
%!TEX root = main.tex

\begin{table} 

\begin{center}
\caption{ \small....}  \label{comparisonTable} 
%\renewcommand{\arraystretch}{1}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|} 
\hline

{\cellcolor{gray!40}\scriptsize {Asymptotic Cost \& Features}} &\cellcolor{gray!40}{\scriptsize {E-PSI}}&\cellcolor{gray!40} {\scriptsize{ \cite{AbadiDMT22}}}&\cellcolor{gray!40}{\scriptsize{\cite{DebnathD16}}}&\cellcolor{gray!40}{ \scriptsize {\cite{DBLP:conf/dbsec/DongCCR13}}}&  \cellcolor{gray!40} {\scriptsize{\cite{DBLP:conf/ccs/KolesnikovMPRT17} }}&\cellcolor{gray!40} {\scriptsize{\cite{NevoTY21}}}&\cellcolor{gray!40} {\scriptsize{\cite{RaghuramanR22}}} \\
\hline

{\scriptsize Computation cost}&\cellcolor{gray!20}\scriptsize{$O (h\cdot d^{2}\cdot m  )$}&\cellcolor{gray!20}\scriptsize$O( h\cdot d^{\st 2}\cdot m)$&\cellcolor{gray!20}\scriptsize$O(c)$&\cellcolor{gray!20}\scriptsize $O (c^{\st 2}  )$&\scriptsize$O(c\cdot m^{\st 2}+c\cdot m )$ & &\\


\hline 

%&\scriptsize {Modular expo.}&\cellcolor{gray!20}\scriptsize {$0$}&\cellcolor{gray!20}\scriptsize$5$&\cellcolor{gray!20}\scriptsize$12$\\


\scriptsize  Communication cost&\cellcolor{gray!20}\scriptsize{$O (h\cdot d^{\st 2}\cdot \xi\cdot m )$}&\cellcolor{gray!20}\scriptsize$O(m\cdot h\cdot d)$&\cellcolor{gray!20}\scriptsize$O(c)$&\cellcolor{gray!20}\scriptsize$O (c )$& & &\\


\hline 

\hline

\hline

\scriptsize Supporting fairness&\cellcolor{gray!20}\scriptsize{\textcolor{blue}\checkmark}&\cellcolor{gray!20}\scriptsize\scriptsize{\textcolor{red}{$\times$}}&\cellcolor{gray!20}\scriptsize\textcolor{blue}\checkmark&\scriptsize\textcolor{blue}\checkmark& & &\\ 




\hline

\scriptsize Rewarding participants&\cellcolor{gray!20}\scriptsize{\textcolor{blue}\checkmark}&\cellcolor{gray!20}\scriptsize\textcolor{red}{$\times$}&\cellcolor{gray!20}\scriptsize\textcolor{red}{$\times$}&\scriptsize\textcolor{red}{$\times$} & & &\\ 

\hline
\scriptsize Symmetric-key based  &\cellcolor{gray!20}\scriptsize{\textcolor{blue}\checkmark}&\cellcolor{gray!20}\scriptsize\textcolor{blue}\checkmark&\cellcolor{gray!20}\scriptsize\textcolor{red}{$\times$}&\scriptsize\textcolor{red}{$\times$} & & &\\ 

\hline


\scriptsize Multi-party&\cellcolor{gray!20}\scriptsize{\textcolor{blue}\checkmark}&\cellcolor{gray!20}\scriptsize{\textcolor{blue}\checkmark}&\cellcolor{gray!20}\scriptsize{\textcolor{red}{$\times$}}&\cellcolor{gray!20}\scriptsize\textcolor{red}{$\times$}& & &\\ 

\hline
\end{tabular}
%}
%\renewcommand{\arraystretch}{1}
%\end{footnotesize}
\end{center}
%}
\end{table}






==> performance-tables.tex <==
% !TEX root =U-PSI.tex

\section{Performance Evaluation:  Run-time Details}\label{perftables}


%All experiments were conducted on a macOS laptop, with an Intel $i5@2.3$ GHz CPU, and $16$ GB RAM. U-PSI  implementation utilises Cryptopp\footnote{https://www.cryptopp.com/}, NTL\footnote{https://www.shoup.net/ntl/} , and Bloom Filter\footnote{http://www.partow.net/programming/bloomfilter/index.html} libraries  for the cryptographic primitives,  polynomial factorizations and checking elements membership respectively. In the experiments,  the probability of  bins overflow in the hash table, for both U-PSI and \cite{eopsi}, and false positive in the Bloom filters, for U-PSI, is set to $2^{\scriptscriptstyle -40}$. Furthermore, the   error probability in the padding scheme, for \cite{eopsi}, is also set to $2^{\scriptscriptstyle -40}$  that results in padding size in the range $[52,63]$ for the above  set size  range.  To achieve an optimal performance, similar to \cite{eopsi}, we set bin capacity to $d=100$. These choices of the hash table parameters, according to inequality \ref{},   leads to the hash table length in the range $[30,41943]$. 


\vspace{-9mm}



\begin{table*}[!htbp]
\begin{footnotesize}
\begin{center}
\caption{\small Update run-time comparison (in sec.)}\label{tbl::update} 


\renewcommand{\arraystretch}{1.3}

\begin{tabular}{|c|ccccccccccc|c|c} 
\hline 
%{\rowcolors{2}{blue!80!gray!18}{blue!10!gray!18}
\cellcolor{gray!20} \scriptsize \textbf{Protocols} &\cellcolor{gray!20} $2^{\scriptscriptstyle 10}$ &\cellcolor{gray!20}  $2^{\scriptscriptstyle 11}$&  \cellcolor{gray!20}$2^{\scriptscriptstyle 12}$&\cellcolor{gray!20}  $2^{\scriptscriptstyle 13}$&\cellcolor{gray!20} $2^{\scriptscriptstyle 14}$&\cellcolor{gray!20}   $2^{\scriptscriptstyle 15}$&\cellcolor{gray!20}  $2^{\scriptscriptstyle 16}$&\cellcolor{gray!20}   $2^{\scriptscriptstyle 17}$& \cellcolor{gray!20}  $2^{\scriptscriptstyle 18}$& \cellcolor{gray!20} $2^{\scriptscriptstyle 19}$&\cellcolor{gray!20}  $2^{\scriptscriptstyle 20}$ \\
    \hline
    
    \hline



\cellcolor{cyan!20}  \scriptsize \cite{eopsi}:&\cellcolor{cyan!20} 0.1&\cellcolor{cyan!20} 0.12&\cellcolor{cyan!20}  0.17&\cellcolor{cyan!20} 0.26&\cellcolor{cyan!20}  0.46&\cellcolor{cyan!20}  0.79 &\cellcolor{cyan!20}  2.05&\cellcolor{cyan!20}  4.71  &\cellcolor{cyan!20} 10.83 &\cellcolor{cyan!20} 15.49 & \cellcolor{cyan!20} 36.28    \\

\cellcolor{white!20}  \scriptsize U-PSI 40-bit: &\cellcolor{white!20}   &\cellcolor{white!20}   &\cellcolor{white!20} &\cellcolor{white!20}   &\cellcolor{white!20} &\cellcolor{white!20}$\leftarrow$ 0.056 $\rightarrow$ &\cellcolor{white!20} &\cellcolor{white!20} &\cellcolor{white!20}   &\cellcolor{white!20}  &\cellcolor{white!20}  \\ 

   \cellcolor{cyan!20}\scriptsize U-PSI 60-bit:      &\cellcolor{cyan!20} &\cellcolor{cyan!20} &\cellcolor{cyan!20}  &\cellcolor{cyan!20}  &\cellcolor{cyan!20} &\cellcolor{cyan!20} $\leftarrow$ 0.063$\rightarrow$ &\cellcolor{cyan!20} &\cellcolor{cyan!20}&\cellcolor{cyan!20} &\cellcolor{cyan!20} &\cellcolor{cyan!20}  \\ 
       \hline





\end{tabular}
\end{center}
\end{footnotesize}
\end{table*}







%\begin{table*}[!htbp]
%\begin{footnotesize}
%\begin{center}
%\caption{Update run-time comparison (in sec.)}\label{tbl::update} 
%
%
%\renewcommand{\arraystretch}{1.3}
%
%\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c} 
%\hline 
%%{\rowcolors{2}{blue!80!gray!18}{blue!10!gray!18}
%\cellcolor{gray!20} \scriptsize \textbf{Protocols} &\cellcolor{gray!20} $2^{\scriptscriptstyle 10}$ &\cellcolor{gray!20}  $2^{\scriptscriptstyle 11}$&  \cellcolor{gray!20}$2^{\scriptscriptstyle 12}$&\cellcolor{gray!20}  $2^{\scriptscriptstyle 13}$&\cellcolor{gray!20} $2^{\scriptscriptstyle 14}$&\cellcolor{gray!20}   $2^{\scriptscriptstyle 15}$&\cellcolor{gray!20}  $2^{\scriptscriptstyle 16}$&\cellcolor{gray!20}   $2^{\scriptscriptstyle 17}$& \cellcolor{gray!20}  $2^{\scriptscriptstyle 18}$& \cellcolor{gray!20} $2^{\scriptscriptstyle 19}$&\cellcolor{gray!20}  $2^{\scriptscriptstyle 20}$ \\
%    \hline
%    
%    \hline
%
%
%
%\cellcolor{cyan!20}  \scriptsize \cite{eopsi}:&\cellcolor{cyan!20} 0.1&\cellcolor{cyan!20} 0.12&\cellcolor{cyan!20}  0.17&\cellcolor{cyan!20} 0.26&\cellcolor{cyan!20}  0.46&\cellcolor{cyan!20}  0.79 &\cellcolor{cyan!20}  2.05&\cellcolor{cyan!20}  4.71  &\cellcolor{cyan!20} 10.83 &\cellcolor{cyan!20} 15.49 & \cellcolor{cyan!20} 36.28    \\
%
%\cellcolor{white!20}  \scriptsize U-PSI 40-bit: &\cellcolor{white!20} 1.75  &\cellcolor{white!20}  1.75 &\cellcolor{white!20} 1.75&\cellcolor{white!20} 1.75  &\cellcolor{white!20}1.75 &\cellcolor{white!20}1.75&\cellcolor{white!20} 1.75 &\cellcolor{white!20} 1.75&\cellcolor{white!20} 1.75  &\cellcolor{white!20} 1.75 &\cellcolor{white!20} 1.75 \\ 
%
%   \cellcolor{cyan!20}\scriptsize U-PSI 60-bit:      &\cellcolor{cyan!20}1.87 &\cellcolor{cyan!20}1.87 &\cellcolor{cyan!20}1.87  &\cellcolor{cyan!20}1.87  &\cellcolor{cyan!20}1.87 &\cellcolor{cyan!20}1.87  &\cellcolor{cyan!20}1.87 &\cellcolor{cyan!20}1.87 &\cellcolor{cyan!20}1.87 &\cellcolor{cyan!20}1.87 &\cellcolor{cyan!20}1.87  \\ 
%       \hline
%
%
%
%
%
%\end{tabular}
%\end{center}
%\end{footnotesize}
%\end{table*}

\vspace{-15mm}


\begin{table*}[!htbp]
\begin{footnotesize}
\begin{center}
\caption{ \small PSI computation run-time comparison: breakdown by step (in sec.)}\label{tbl::PSI} 


\renewcommand{\arraystretch}{1.3}

\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c} 
\hline 
%{\rowcolors{2}{blue!80!gray!18}{blue!10!gray!18}
\cellcolor{gray!20}\scriptsize \textbf{Phases} &\cellcolor{gray!20} \scriptsize \textbf{Protocols} &\cellcolor{gray!20} $2^{\scriptscriptstyle 10}$ &\cellcolor{gray!20}  $2^{\scriptscriptstyle 11}$&  \cellcolor{gray!20}$2^{\scriptscriptstyle 12}$&\cellcolor{gray!20}  $2^{\scriptscriptstyle 13}$&\cellcolor{gray!20} $2^{\scriptscriptstyle 14}$&\cellcolor{gray!20}   $2^{\scriptscriptstyle 15}$&\cellcolor{gray!20}  $2^{\scriptscriptstyle 16}$&\cellcolor{gray!20}   $2^{\scriptscriptstyle 17}$& \cellcolor{gray!20}  $2^{\scriptscriptstyle 18}$& \cellcolor{gray!20} $2^{\scriptscriptstyle 19}$&\cellcolor{gray!20}  $2^{\scriptscriptstyle 20}$ \\
    \hline
    
    \hline
\NameEntry{\center \scriptsize Data \\ \scriptsize Preparation for \\ \scriptsize   Outsourcing}
 \multirow{4}{*}&\cellcolor{cyan!20}  \scriptsize U-PSI 40-bit: &\cellcolor{cyan!20} 0.17&\cellcolor{cyan!20}  0.3&\cellcolor{cyan!20}  0.6&\cellcolor{cyan!20}  1.4 &\cellcolor{cyan!20}  2.8 &\cellcolor{cyan!20}  5.6  &\cellcolor{cyan!20}  14&\cellcolor{cyan!20}  44  &\cellcolor{cyan!20}  58 &\cellcolor{cyan!20}  121& \cellcolor{cyan!20} 240\\
    \cline{2-13}
 &\cellcolor{white!20}\scriptsize U-PSI 60-bit:&\cellcolor{white!20} 0.18  &\cellcolor{white!20}  0.3 &\cellcolor{white!20}  0.6&\cellcolor{white!20} 1.4  &\cellcolor{white!20} 2.8 &\cellcolor{white!20} 5.7  &\cellcolor{white!20} 14  &\cellcolor{white!20} 46 &\cellcolor{white!20} 60  &\cellcolor{white!20} 128 &\cellcolor{white!20} 253 \\ 
    \cline{2-13}
    &\cellcolor{cyan!20}\scriptsize \cite{eopsi}:&\cellcolor{cyan!20}0.7  &\cellcolor{cyan!20}0.8  &\cellcolor{cyan!20}1  &\cellcolor{cyan!20}1.5  &\cellcolor{cyan!20}3.4 &\cellcolor{cyan!20}8.8  &\cellcolor{cyan!20}15 &\cellcolor{cyan!20}48&\cellcolor{cyan!20}63 &\cellcolor{cyan!20}131 &\cellcolor{cyan!20}256   \\ 
       \hline


    \hline
\NameEntry{\center \scriptsize Client-side \\ \scriptsize Computation \\ \scriptsize  Delegation}
%\makecell{\scriptsize Computation \\ \scriptsize  Delegation}
    \multirow{3}{*}%{\scriptsize Computation Delegation}
    &\cellcolor{white!20} \scriptsize U-PSI 40-bit: &\cellcolor{white!20}  0.2  &\cellcolor{white!20}  0.3 &\cellcolor{white!20}  0.7 &\cellcolor{white!20} 1.5  &\cellcolor{white!20}  3.1 &\cellcolor{white!20}  6.4 &\cellcolor{white!20}  16 &\cellcolor{white!20}  32  &\cellcolor{white!20} 68  &\cellcolor{white!20}  121 &\cellcolor{white!20}  294  \\
    \cline{2-13}
    &\cellcolor{cyan!20}\scriptsize U-PSI 60-bit:&\cellcolor{cyan!20}  0.2&\cellcolor{cyan!20}0.4  &\cellcolor{cyan!20}0.7 &\cellcolor{cyan!20}  1.6  & \cellcolor{cyan!20}  3.3 &\cellcolor{cyan!20} 6.5  &\cellcolor{cyan!20}17 &\cellcolor{cyan!20}35 & \cellcolor{cyan!20}70  &\cellcolor{cyan!20} 141 &\cellcolor{cyan!20} 307  \\ 
    \cline{2-13}
    &\cellcolor{white!20}\scriptsize \cite{eopsi}: &\cellcolor{white!20}  0.4  &\cellcolor{white!20}  0.7 &\cellcolor{white!20} 1.5  &\cellcolor{white!20}   2.9&\cellcolor{white!20} 5.9 &\cellcolor{white!20} 11.9  &\cellcolor{white!20}  32 &\cellcolor{white!20}   63&\cellcolor{white!20} 129&\cellcolor{white!20} 268 &\cellcolor{white!20} 555 \\ 

    \hline


    \hline
\NameEntry{\center \scriptsize Cloud-side \\ \scriptsize  Computation}
%\makecell{\scriptsize Cloud-side \\ \scriptsize  Computation}
    \multirow{3}{*}%{\scriptsize Cloud-side computation}
    &\cellcolor{cyan!20}\scriptsize U-PSI 40-bit:  &\cellcolor{cyan!20} 0.18 &\cellcolor{cyan!20}0.3  &\cellcolor{cyan!20} 0.7  &\cellcolor{cyan!20}1.2  &\cellcolor{cyan!20}2.9  &\cellcolor{cyan!20}6 &\cellcolor{cyan!20}15 &\cellcolor{cyan!20} 30 & \cellcolor{cyan!20}71 &\cellcolor{cyan!20} 162&\cellcolor{cyan!20}473 \\
    \cline{2-13}
    &\cellcolor{white!20} \scriptsize U-PSI 60-bit: &\cellcolor{white!20} 0.19 &\cellcolor{white!20}  0.3  &\cellcolor{white!20} 0.7 &\cellcolor{white!20} 1.4  &\cellcolor{white!20} 3.3 &\cellcolor{white!20}  6.1 &\cellcolor{white!20}  15 &\cellcolor{white!20}  35 &\cellcolor{white!20}  72&\cellcolor{white!20}  164 &\cellcolor{white!20}  489 \\ 
    \cline{2-13}
    &\cellcolor{cyan!20}\scriptsize \cite{eopsi}: &\cellcolor{cyan!20} 0.4  &\cellcolor{cyan!20} 0.6 &\cellcolor{cyan!20} 1.4 &\cellcolor{cyan!20}  2.7&\cellcolor{cyan!20}5.4 & \cellcolor{cyan!20}10  &\cellcolor{cyan!20} 29&\cellcolor{cyan!20}57 &\cellcolor{cyan!20} 116 & \cellcolor{cyan!20}253&\cellcolor{cyan!20} 987  \\ 
       \hline


    \hline
\NameEntry{\center  \scriptsize Client-side \\ \scriptsize Result \\ \scriptsize  Retrieval}
%\makecell{\scriptsize Result \\   \scriptsize Retrieval}
    \multirow{3}{*} %{\scriptsize Result Retrieval}
    &\cellcolor{white!20}\scriptsize U-PSI 40-bit:  &\cellcolor{white!20}  0.59 &\cellcolor{white!20}  1.1 &\cellcolor{white!20}  2.2 &\cellcolor{white!20}  4.6&\cellcolor{white!20}  9.9 &\cellcolor{white!20}  18 &\cellcolor{white!20}   49&\cellcolor{white!20}  95  &\cellcolor{white!20} 195  &\cellcolor{white!20} 417 &\cellcolor{white!20}  1052 \\
    \cline{2-13}
   &\cellcolor{cyan!20} \scriptsize U-PSI 60-bit: &\cellcolor{cyan!20} 0.6  &\cellcolor{cyan!20}1.5   &\cellcolor{cyan!20} 2.8  &\cellcolor{cyan!20} 5.9 &\cellcolor{cyan!20}  12.5 &\cellcolor{cyan!20}24  &\cellcolor{cyan!20} 65 &\cellcolor{cyan!20} 131 &\cellcolor{cyan!20}  244 &\cellcolor{cyan!20} 568  &\cellcolor{cyan!20} 1389  \\ 
   \cline{2-13}
    &\cellcolor{white!20}\scriptsize \cite{eopsi}: &\cellcolor{white!20} 2.4  &\cellcolor{white!20}  5  &\cellcolor{white!20}   10.5 &\cellcolor{white!20}  20.8 &\cellcolor{white!20}    38.4 &\cellcolor{white!20}   81.2 &\cellcolor{white!20}  220   &\cellcolor{white!20}  424  &\cellcolor{white!20}  882  &\cellcolor{white!20}  1781  &\cellcolor{white!20} 3590 \\ 

	    \hline
	    
   \hline

\NameEntry{\center \scriptsize Total}

    \multirow{3}{*} 
    &\cellcolor{cyan!20}\scriptsize U-PSI 40-bit:   &\cellcolor{cyan!20}1.14  &\cellcolor{cyan!20} 2 &\cellcolor{cyan!20}4.2 &\cellcolor{cyan!20}8.7  & \cellcolor{cyan!20}18.7&\cellcolor{cyan!20}36  &\cellcolor{cyan!20}94 &\cellcolor{cyan!20}201  &\cellcolor{cyan!20}392 &\cellcolor{cyan!20} 821&\cellcolor{cyan!20}2059 \\
    \cline{2-13}
   &\cellcolor{white!20}\scriptsize U-PSI 60-bit: &\cellcolor{white!20} 1.17 &\cellcolor{white!20} 2.5 &\cellcolor{white!20} 4.8 &\cellcolor{white!20} 10.3 &\cellcolor{white!20}  21.9&\cellcolor{white!20} 42.3 &\cellcolor{white!20} 111 &\cellcolor{white!20} 247  &\cellcolor{white!20} 446&\cellcolor{white!20} 1001&\cellcolor{white!20} 2438 \\ 
   \cline{2-13}
    &\cellcolor{cyan!20}\scriptsize \cite{eopsi}: &\cellcolor{cyan!20} 3.9  &\cellcolor{cyan!20} 7.1 &\cellcolor{cyan!20} 14.3 &\cellcolor{cyan!20} 27.9  &\cellcolor{cyan!20} 53.1 &\cellcolor{cyan!20}  111.9 &\cellcolor{cyan!20}296&\cellcolor{cyan!20} 592  &\cellcolor{cyan!20}1190&\cellcolor{cyan!20}2433&\cellcolor{cyan!20} 5388 \\ 

    \hline

\end{tabular}
\end{center}
\end{footnotesize}
\end{table*}




%\begin{tikzpicture}
%%\begin{loglogaxis}[
%	xlabel=Cost,
%	ylabel=Error]
%\addplot[color=red,mark=x] coordinates {
%	(5,    8.31160034e-02)
%	(17,   2.54685628e-02)
%	(49,   7.40715288e-03)
%	(129,  2.10192154e-03)
%	(321,  5.87352989e-04)
%	(769,  1.62269942e-04)
%	(1793, 4.44248889e-05)
%	(4097, 1.20714122e-05)
%	(9217, 3.26101452e-06)
%};
%


%\legend{Case 1,Case 2}
%%\end{loglogaxis}
%\end{tikzpicture}







%
%\begin{tikzpicture}
%	\begin{semilogyaxis}[
%		xlabel=Index,ylabel=Value]
%		\addplot[color=black,mark=*] coordinates {
%		(2^10 ,8)
%		(2^11,16)
%		(2^12,88)
%		
%	};
%
%	\addplot[color=blue,mark=*] coordinates {
%		(2^10 ,8)
%		(2^11,16)
%		(2^12,88)
%	};
%	\end{semilogyaxis}%
%\end{tikzpicture}%



==> performance.tex <==
% !TEX root =U-PSI.tex


\section{Performance Evaluation}

We provide an empirical performance evaluation of U-PSI using  a prototype implementation developed in C++\footnote{\scriptsize U-PSI source code is available at  https://github.com/unknown-2018/U-PSI}. The implementation uses the efficient data representation presented in section \ref{BBF}. We compare the performance of U-PSI against  the protocol in \cite{eopsi}, as it is the fastest of the protocols we studied in section \ref{U-PSIEvaluation}. In order to do so, we have developed a prototype implementation of it\footnote{\scriptsize The update simulation for \cite{eopsi}  is available at \scriptsize https://github.com/unknown-2018/Update-Simulation} that allows clients to securely update their outsourced data by downloading and unblinding its entire outsourced data; updating a bin; re-encoding the elements of it; re-blinding the entire dataset; and uploading it to the cloud. More specifically, the implementations utilise  Cryptopp\footnote{\scriptsize https://www.cryptopp.com}, NTL\footnote{\scriptsize https://www.shoup.net/ntl} and Bloom Filter\footnote{\scriptsize http://www.partow.net/programming/bloomfilter/index.html} libraries  for   cryptographic primitives,  polynomial factorization and element membership checks respectively.

All experiments were conducted on a macOS laptop, with an Intel $i5@2.3$ GHz CPU, and $16$ GB RAM. In the experiments, we use randomly generated $40$-bit integers as set elements, and a set size in the range $[2^{\scriptscriptstyle 10},2^{\scriptscriptstyle 20}]$. The probability of bin overflow in the hash table, for both U-PSI and \cite{eopsi}, and false positive in the Bloom filters, for U-PSI, is set to $2^{\scriptscriptstyle -40}$. The error probability in the padding scheme, for \cite{eopsi}, is also set to $2^{\scriptscriptstyle -40}$  that results in padding size in the range $[52,63]$ for the above set size  range. To achieve an optimal performance, similar to \cite{eopsi}, we set bin capacity to $d=100$. These choices of hash table parameters, according to section \ref{PreliminaryHashTable}, lead to a hash table length in the range $[30,41943]$. We also use two different field sizes for U-PSI $40$ and $60$ bits. 

For the update operation in U-PSI, we measure the total run-time of four phases at the client-side: (a) computing an update query, (b) unblinding and decoding a bin, (c) applying the update, and (d) encoding and re-blinding the bin. For the update in \cite{eopsi}, we measure the total time when a client starts unblinding its dataset until it finishes re-blinding it. For the PSI computation in both protocols, we measure the total run-time of four phases: outsourcing, client-side PSI delegation (that includes both clients), cloud-side result computation and client-side result retrieval. Note that we include the run-time of outsourcing in the total time, although this step is performed only once by a client and  next time it delegates the PSI the protocol overall run-time would be lower. 

Fig. \ref{performance} depicts the  performance comparison between the two protocols  for update and PSI computation (see Tables \ref{tbl::update} and \ref{tbl::PSI}  in Appendix \ref{perftables} for a detailed run-time). The x-axes  in the figure are on a \emph{logarithmic scale}. As it is evident in the left-hand side graph in the figure, the update run-time for U-PSI is much lower than for \cite{eopsi}, especially for a larger set size. In particular, the update run-time for \cite{eopsi} grows from  $0.1$ to $36$ seconds when the set size increases from $2^{\scriptscriptstyle 10}$ to $2^{\scriptscriptstyle 20}$; whereas for U-PSI, the update run-time remains $0.056$ and $0.063$ seconds for all set sizes, when the field size is $40$ and $60$ bits, respectively. Therefore, the update in U-PSI is $1.7-642$ times and $1.5-571$ times faster than \cite{eopsi}, for field size $40$ and $60$ bits respectively.  The reason for this huge difference in the performance is that in \cite{eopsi} the client needs to unblind and re-blind all the bins in the hash table; whereas, in U-PSI such operations are carried out only on one bin. 
   
% the update performance of the  protocol in \cite{eopsi} is slightly better than U-PSI when the  set cardinality is smaller than $2^{\scriptscriptstyle 15}$. However, when the  cardinality is  greater than  $2^{\scriptscriptstyle 18}$ the  performance of U-PSI is much better than the other protocol. In particular, when the  size increases from $2^{\scriptscriptstyle 10}$ to $2^{\scriptscriptstyle 20}$,  the update run-time in \cite{eopsi} increases from $0.72$ to $36$ seconds, whereas in U-PSI it remains $1.75$ and $1.87$ seconds when the field size is $40$ and $60$ bits, respectively. Therefore, when the set cardinality is $2^{\scriptscriptstyle 20}$ the update run-time in U-PSI is  a factor of $19-20$ faster than \cite{eopsi}. The reason is that in U-PSI the client and cloud apply the update to only one bin, whereas in \cite{eopsi} the client has to decode and re-encode its entire data.  We expected that for \emph{all set sizes} the update in U-PSI has a lower run-time than in \cite{eopsi}. This can be due to an inefficient prototype implementation of the update  in U-PSI.   

%Here we compare the performance of our protocol against  the protocol proposed in \cite{eopsi}, as it is much faster than the other protocols that we studied in the previous section. Since this protocol  has been designed to  support  only PSI computation, we have also developed a prototype implementation that allows clients to securely update their outsourced date. To do that, a client needs to download and unblind its entire outsourced data,   update a bin, re-encode the elements of it, blind the entire dataset and then upload it to the cloud. We ran PSI and update operations for \cite{eopsi} using the same hash table parameters as those used in the U-PSI.  that results in padding size in the range $[52,63]$ for the above  set size  range. 


% Fig. \ref{performance} depicts the  performance comparison between the two protocols  for the update and PSI computation phases (see Tables \ref{tbl::update} and \ref{tbl::PSI}  in appendix\ref{} for a detailed run-time). The x-axes  in the figure are based on a  logarithmic scale. As it is evident in the left-hand side graph in the figure, the update performance of the  protocol in \cite{eopsi} is slightly better than U-PSI when the  set cardinality is smaller than $2^{\scriptscriptstyle 15}$. However, when the  cardinality is  greater than  $2^{\scriptscriptstyle 18}$ the  performance of U-PSI is much better than the other protocol. In particular, when the  size increases from $2^{\scriptscriptstyle 10}$ to $2^{\scriptscriptstyle 20}$,  the update run-time in \cite{eopsi} increases from $0.72$ to $36$ seconds, whereas in U-PSI it remains $1.75$ and $1.87$ seconds when the field size is $40$ and $60$ bits, respectively. Therefore, when the set cardinality is $2^{\scriptscriptstyle 20}$ the update run-time in U-PSI is  a factor of $19-20$ faster than \cite{eopsi}. The reason is that in U-PSI the client and cloud apply the update to only one bin, whereas in \cite{eopsi} the client has to decode and re-encode its entire data.  We expected that for \emph{all set sizes} the update in U-PSI has a lower run-time than in \cite{eopsi}. This can be due to an inefficient prototype implementation of the update  in U-PSI.   
 
 
Furthermore, as  the right-hand side graph in Fig. \ref{performance} indicates, the run-time for PSI computation in both protocols grows linearly when  the set size increases.  In particular, the PSI run-time  for \cite{eopsi}, grows from $3.9$ to $5388$ seconds when the set cardinality increases from $2^{\scriptscriptstyle 10}$ to $2^{\scriptscriptstyle 20}$.  Nevertheless, the growth for U-PSI is from $1.14$ to $2059$ seconds and from $1.17$ to $2438$ seconds for field size of $40$ and $60$ bits, respectively. Hence, the PSI computation run-time for U-PSI is a factor of $2.2-3.4$ faster than  \cite{eopsi}. The reason for this improvement is that in U-PSI all (arithmetic) operations, especially polynomial factorisations, are performed on a smaller field size. 

\vspace{-4mm}

\begin{figure}
\centering
\includegraphics[width=1 \textwidth]{pics/graphs2.pdf}
\caption{\small Update performance comparison between \cite{eopsi} and U-PSI, left hand side graph. PSI computation performance comparison between \cite{eopsi} and U-PSI, right hand size graph. }\label{performance}
\end{figure}

\vspace{-9mm}



%\begin{tikzpicture}
%%\begin{loglogaxis}[
%	xlabel=Cost,
%	ylabel=Error]
%\addplot[color=red,mark=x] coordinates {
%	(5,    8.31160034e-02)
%	(17,   2.54685628e-02)
%	(49,   7.40715288e-03)
%	(129,  2.10192154e-03)
%	(321,  5.87352989e-04)
%	(769,  1.62269942e-04)
%	(1793, 4.44248889e-05)
%	(4097, 1.20714122e-05)
%	(9217, 3.26101452e-06)
%};
%


%\legend{Case 1,Case 2}
%%\end{loglogaxis}
%\end{tikzpicture}







%
%\begin{tikzpicture}
%	\begin{semilogyaxis}[
%		xlabel=Index,ylabel=Value]
%		\addplot[color=black,mark=*] coordinates {
%		(2^10 ,8)
%		(2^11,16)
%		(2^12,88)
%		
%	};
%
%	\addplot[color=blue,mark=*] coordinates {
%		(2^10 ,8)
%		(2^11,16)
%		(2^12,88)
%	};
%	\end{semilogyaxis}%
%\end{tikzpicture}%



==> securityproof.tex <==
% !TEX root =U-PSI.tex
\section{U-PSI Security Proof}\label{U-PSIProof}

In this section, we  sketch U-PSI's security proof  in the presence of static semi-honest adversaries. We conduct the security analysis for the three cases where one of the parties is corrupted at a time. 
%\begin{theorem-non}
\begin{theorem}
If $\mathtt{PRF}$ and $\mathtt{PRF}'$ are collision-resistant pseudorandom functions, and $\pi$ is a pseudorandom permutation, then U-PSI protocol is secure in the presence of a semi-honest adversary. 
\end{theorem}
%\end{theorem-non}

\vspace{-2mm}

%\newtheorem{prop2}{Proof}
%\begin{prop2} 

\begin{proof}
We will prove the theorem by considering in turn the case where each of the parties has been corrupted. In each case, we invoke the simulator with the corresponding party's input and output.  Our focus is on the case where party $A$ wants to engage in the computation of the intersection, i.e. it authorizes the computation. If party $A$ does not want to proceed with the protocol, the views can be simulated in the same way up to the point where the execution stops.


\
\vspace{-2mm}

\noindent\textbf{Case 1: Corrupted Cloud.} In this case, we show that given the leakage function we can construct a simulator $\textsf {\scriptsize SIM}_{\scriptscriptstyle C}$ that can produce a view computationally indistinguishable from the one in the real model. In the real execution, the cloud's view is:
\begin{equation*}
 \textsf {\scriptsize VIEW}^{\scriptscriptstyle\textsf { U-PSI}}_{\scriptscriptstyle C}(\Lambda, S^{\scriptscriptstyle (A)},S^{\scriptscriptstyle (B)})=\{\Lambda, r_{\scriptscriptstyle C}, \vv{\bm{po}}^{\scriptscriptstyle (A)},\vv{\bm{pl}}^{\scriptscriptstyle (A)}, \vv{\bm{po}}^{\scriptscriptstyle (B)},\vv{\bm{pl}}^{\scriptscriptstyle (B)}, (Q_{\scriptscriptstyle  1}, ..., Q_{\scriptscriptstyle  \Upsilon}),\Lambda \}.
\end{equation*}

In the above view, $r_{\scriptscriptstyle C}$ is the outcome of internal random coins of the cloud,  ($\forall I, I\in \{A, B\}$) $\vv{\bm{po}}^{\scriptscriptstyle (I)}$ are the permuted hash tables  containing the clients' blinded datasets and $\vv{\bm{pl}}^{\scriptscriptstyle (I)}$ are the permuted labels. Moreover, if  the query is for PSI delegation then
\begin{equation*}
 Q_{\scriptscriptstyle  i}=\{tk^{\scriptscriptstyle  (B)}, tk^{\scriptscriptstyle  (A)}, \textsf {\scriptsize \textbf{ID}}^{\scriptscriptstyle (A)},  \textsf {\scriptsize \textbf{ID}}^{\scriptscriptstyle (B)},  \vv{\bm{pm}}_{\scriptscriptstyle \mathtt{ A \rightarrow B}}, \textsf {\scriptsize \textbf{Compute}}\},
\end{equation*}
 otherwise (if the client $I$'s query is for update),  
\begin{equation*}
Q_{\scriptscriptstyle  i}=\{\vv{\bm{o}}^{\scriptscriptstyle (I)}_{\scriptscriptstyle j,c^{ {\text{\tiny (\textit{I})}}}_{\tiny j}}, l^{\scriptscriptstyle (I)}_{\scriptscriptstyle j},\textsf {\scriptsize \textbf{Update}}\}, 
\end{equation*}
for some $j, 1\leq j\leq h$.

%$\textsf {\scriptsize \textbf{ID}}^{\scriptscriptstyle (B)}$
Now we construct the simulator $\textsf {\scriptsize SIM}_{\scriptscriptstyle C}$ in the ideal model which executes as follows. 

\begin{packed_enum}
\item Creates an empty view and appends $\Lambda$ and uniformly random coin $r'_{\scriptscriptstyle C}$ to it. 
%\item Chooses  two random sets $S'^{\scriptscriptstyle (A)}$ and $S'^{\scriptscriptstyle (B)}$, such that $|S'^{\scriptscriptstyle (A)}|, |S'^{\scriptscriptstyle (B)}|<c$.

\item Uses the public parameters and the hash function to construct two hash tables $\mathtt{HT}'^{\scriptscriptstyle (A)}$ and $\mathtt{HT}'^{\scriptscriptstyle (B)}$. It fills each bin of the hash tables with $n$ uniformly random values picked from the field $\mathbb{F}_p$. So, each bin $\mathtt{HT}'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j}$ ($\forall I, I\in \{A,B\}$) contains a vector  $\vv{\bm{o}}'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j}$ of $n$ random values. 



%Then, it maps and insert each  element of the  sets $S'^{\scriptscriptstyle (A)}$ and $S'^{\scriptscriptstyle (B)}$ to the bins of the tables $\mathtt{HT}'^{\scriptscriptstyle (A)}$ and $\mathtt{HT}'^{\scriptscriptstyle (B)}$ respectively. So for every $I\in \{A,B\}$ does as the following. 

%\
%
%\vspace{-2mm}
%
%\begin{center}
%$\forall s'^{\scriptscriptstyle (I)}_{\scriptscriptstyle i}\in S'^{\scriptscriptstyle (I)}: \mathtt{H}( s'^{\scriptscriptstyle (I)}_{\scriptscriptstyle i})=j$, then $s'^{\scriptscriptstyle (I)}_{\scriptscriptstyle i}\rightarrow \mathtt{HT}'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j}$, where $1\leq j \leq h$ and $I\in \{A,B\}$
%\end{center}
%
%\
%
%\vspace{-2mm}


\item \label{labelGen}Assigns a pseudorandom label to each bin $\mathtt{HT}'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j}$ ($\forall I, I\in \{A,B\}$). To do so, it picks fresh label-keys, $lk'^{\scriptscriptstyle(I)}$, and computes the labels as $\forall I, I\in \{A,B\}$ and $\forall j,  1\leq j \leq h$ : $l'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j}=\mathtt{PRF}'(lk'^{\scriptscriptstyle (I)},j)$.




%\item \label{keygen} Assigns a key to each bin in the hash table by picking a master key $mk'^{\scriptscriptstyle (I)}$; and then generating $h$ pseudorandom values.  $\forall j, 1\leq j \leq h$: $k^{\scriptscriptstyle (I)}_{\scriptscriptstyle j}=\mathtt{PRF}(mk'^{\scriptscriptstyle (I)},j)$.



%\item  For every bin $\mathtt{HT}'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j}$ (where $1\leq j\leq h$ and $I\in \{A,B\}$), if it has less than $d$ set elements, pad it with dummy (or random) elements, $r'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j,i}$, to contain $d$ elements. Then, encode the elements as follows.



%\item For every occupied bin $\mathtt{HT}^{\scriptscriptstyle (I)}_{\scriptscriptstyle j}$, containing $d'$ set elements, encode the elements as follows.

%\begin{enumerate}
% \item  Constructs a polynomial representing the elements in the bin.
%
%\
%
%\vspace{-2mm}
%
%\begin{center}
%$\tau'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j}(x)=\prod\limits ^{\scriptscriptstyle d}_{\scriptscriptstyle i=1}(x-e'^{\scriptscriptstyle (I)}_{\scriptscriptstyle i})$, where $e'^{\scriptscriptstyle (I)}_{\scriptscriptstyle i} \in \mathtt{HT}'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j}$, $e'^{\scriptscriptstyle (I)}_{\scriptscriptstyle i}=s'^{\scriptscriptstyle (I)}_{\scriptscriptstyle i} $ or $e'^{\scriptscriptstyle (I)}_{\scriptscriptstyle i}=r'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j,i}$
%\end{center}
%
%\
%
%\vspace{-2mm}
%
%\item Represents $\tau'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j} (x)$ as point-value form, by evaluating it at every element $x_{\scriptscriptstyle i}\in\vv{\bm{x}}$. This yields a vector of  $\tau'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j} (x_{\scriptscriptstyle i})$, $1\leq i \leq n$.


%\item \label{blind} Blinds every value $\tau'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j} (x_{\scriptscriptstyle i})$. To do so, first generate a pseudorandom value $z'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j,c^{ {\text{\tiny (\textit{I})}}}_{\tiny j},i}=\mathtt{PRF}(k^{\scriptscriptstyle (I)}_{\scriptscriptstyle j},i)$, where key $k'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j}$ was generated in step b.\ref{keygen}. Then, computes $o'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j,c^{ {\text{\tiny (\textit{I})}}}_{\tiny j},i}$ as follow. $\forall i, 1\leq i\leq n: o'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j,c^{ {\text{\tiny (\textit{I})}}}_{\tiny j},i}=\tau'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j} (x_{\scriptscriptstyle i})+ z'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j,c^{ {\text{\tiny (\textit{I})}}}_{ j},i}$.



\item Constructs two vectors of the form   $[(\vv{\bm{o}}'^{\scriptscriptstyle (I)}_{\scriptscriptstyle 1},l'^{\scriptscriptstyle (I)}_{\scriptscriptstyle 1}),...,(\vv{\bm{o}}'^{\scriptscriptstyle (I)}_{\scriptscriptstyle h},l'^{\scriptscriptstyle (I)}_{\scriptscriptstyle h})]$ for each $I$, $I\in \{A,B\}$. Then, it randomly permutes each vector. Next,  it inserts each element  $\vv{\bm{o}}'^{\scriptscriptstyle (I)}_{\scriptscriptstyle g}$ ($\forall g, 1\leq g\leq h$) of the permuted vector into $\vv{\bm{po}}'^{\scriptscriptstyle (I)}$. Also, it inserts each element $l'^{\scriptscriptstyle (I)}_{\scriptscriptstyle g}$ of the permuted vector into $\vv{\bm{pl}}'^{\scriptscriptstyle (I)}$. Therefore, it has constructed four vectors: $\vv{\bm{po}}'^{\scriptscriptstyle (A)}$, $\vv{\bm{pl}}'^{\scriptscriptstyle (A)}$, $\vv{\bm{po}}'^{\scriptscriptstyle (B)}$ and   $\vv{\bm{pl}}'^{\scriptscriptstyle (B)}$. It appends the four vectors to the view.





%\item Picks two random keys $pk'^{\scriptscriptstyle (I)}$  ($\forall I, I\in \{A,B\}$), and constructs two permuted vectors, $\vv{\bm{po}}'^{\scriptscriptstyle (I)}=\pi(pk'^{\scriptscriptstyle (I)}, \vv{\bm{o}}'^{\scriptscriptstyle (I)})$ and $\vv{\bm{pl}}'^{\scriptscriptstyle (I)}=\pi(pk'^{\scriptscriptstyle (I)}, \vv{\bm{l}}'^{\scriptscriptstyle (I)})$, where $\vv{\bm{o}}'^{\scriptscriptstyle (I)}=[\vv{\bm{o}}'^{\scriptscriptstyle (I)}_{\scriptscriptstyle 1}, ..., \vv{\bm{o}}'^{\scriptscriptstyle (I)}_{\scriptscriptstyle h}]$ and  vector $\vv{\bm{l}}'^{\scriptscriptstyle (I)}$ contains the labels generated in  step \ref{labelGen}. Then, it inserts $\vv{\bm{po}}'^{\scriptscriptstyle (A)}$, $\vv{\bm{pl}}'^{\scriptscriptstyle (A)}$, $\vv{\bm{po}}'^{\scriptscriptstyle (B)}$ and   $\vv{\bm{pl}}'^{\scriptscriptstyle (B)}$ to its view. 

\item Given the leakage function $[\mathcal{M}^{\scriptscriptstyle (I)},\vv{\bm{T}}]$, it first uses each matrix $\mathcal{M}^{\scriptscriptstyle (I)}$ to construct the corresponding vector $\vv{\bm{v}}^{\scriptscriptstyle (I)}$ that will contain a set of labels $l'^{\scriptscriptstyle (I)}\in \vv{\bm{l}}'^{\scriptscriptstyle (I)}$, and has the same access pattern as the one indicated by the matrix. In order for it to generate this vector, it first constructs  vector $\vv{\bm{v}}^{\scriptscriptstyle (I)}$ of zeros, where $|\vv{\bm{v}}^{\scriptscriptstyle (I)}|=\textbf{p}$. Then, for every row $i$ ($1\leq i\leq \textbf{p}$) of the matrix $\mathcal{M}^{\scriptscriptstyle (I)}$, it performs the following:
\begin{packed_enum}
\item If there exists at least one element set to $1$ in the row and if the $i^{th}$ element in the vector $\vv{\bm{v}}^{\scriptscriptstyle (I)}$ is zero, then it finds a set $G$ such that $\forall g \in G: \mathcal{M}^{\scriptscriptstyle (I)}_{i,g}=1$. Next, it picks a label $l'^{\scriptscriptstyle (I)}\in \vv{\bm{l}}'^{\scriptscriptstyle (I)}$ and inserts it into all $i^{\scriptscriptstyle th}, g^{\scriptscriptstyle th}$ positions of the vector $\vv{\bm{v}}^{\scriptscriptstyle (I)}$. The label must be distinct from the ones used for the previous rows $i'$, where $i'<i$. Otherwise, if the $i^{th}$ element in the vector is non-zero,  it  moves on to the next row. 

\item If all the elements in the row are zero and if the $i^{\scriptscriptstyle th}$ element in the vector $\vv{\bm{v}}^{\scriptscriptstyle (I)}$ is zero, then it picks a label $l'^{\scriptscriptstyle (I)}\in \vv{\bm{l}}'^{\scriptscriptstyle (I)}$ and inserts it at position $i^{\scriptscriptstyle th}$ of the vector, where  the label is distinct from the ones used for the previous rows $i'$, where $i'<i$. Otherwise, if the $i^{\scriptscriptstyle th}$ element in the vector is non-zero,  it  moves on to the next row. 
\end{packed_enum}



\item  Uses $\vv{\bm{T}}$ and checks $T_{\scriptscriptstyle i}$ ( $\forall i, 1\leq i\leq \Upsilon$) as follows:

\begin{packed_enum}
\item if $T_{\scriptscriptstyle i}= \textsf {\scriptsize PSI-Com}$, then sets: 
\begin{equation*}
Q'_{\scriptscriptstyle  i}=\{tk'^{\scriptscriptstyle  (B)}, tk'^{\scriptscriptstyle  (A)},\textsf {\scriptsize \textbf{ID}}^{\scriptscriptstyle  (A)},  \textsf {\scriptsize \textbf{ID}}^{\scriptscriptstyle  (B)},  \vv{\bm{pm}}'_{\scriptscriptstyle \mathtt{ A \rightarrow B}}, \textsf {\scriptsize \textbf{Compute}}\}, 
\end{equation*}
where  $\vv{\bm{pm}}'_{\scriptscriptstyle \mathtt{ A \rightarrow B}}$ contains tuples $(l'^{\scriptscriptstyle  (A)}_{\scriptscriptstyle i},l'^{\scriptscriptstyle  (B)}_{\scriptscriptstyle i})$ randomly permuted. Also, $tk'^{\scriptscriptstyle  (B)}$ and $tk'^{\scriptscriptstyle  (A)}$ are fresh random keys,  and  labels $l'^{\scriptscriptstyle  (I)}_{\scriptscriptstyle i}$ were generated step \ref{labelGen}.  Next, it appends $Q'_{\scriptscriptstyle  i}$ to the view. 
\item if $T_{\scriptscriptstyle i}= \textsf {\scriptsize Upd}^{\scriptscriptstyle (I)}_{\scriptscriptstyle t}$, then sets: 
\begin{equation*}
Q'_{\scriptscriptstyle  i}=\{\vv{\bm{o}}''^{\scriptscriptstyle (I)}, l'^{\scriptscriptstyle (I)}_{\scriptscriptstyle t},\textsf {\scriptsize \textbf{Update}}\},
\end{equation*}
 where $\vv{\bm{o}}''^{\scriptscriptstyle (I)}$ contains $n$  uniformly random values picked from the field $\mathbb{F}_p$ and $l'^{\scriptscriptstyle (I)}_{\scriptscriptstyle t}$ is the $t^{\scriptscriptstyle th}$ element in the vector $\vv{\bm{v}}^{\scriptscriptstyle (I)}$. After that, it appends $Q'_{\scriptscriptstyle  i}$ to the view. 
\end{packed_enum}
\item Appends $\Lambda$ to its view and outputs the view.
\end{packed_enum}

We are ready now to show why the two views are indistinguishable.  In both views, the input and output parts (i.e. $\Lambda$) are identical and the random coins are both uniformly
random, and so they are indistinguishable. Each vector  $\vv{\bm{po}}^{\scriptscriptstyle (I)}_{\scriptscriptstyle i}\in \vv{\bm{po}}^{\scriptscriptstyle (I)}$, ($\forall i, 1\leq i\leq h$ and $\forall I, I\in \{A,B\}$), contains $n$ values blinded with  pseudorandom values (that are the outputs of a pseudorandom function), also each vector  $\vv{\bm{po}}'^{\scriptscriptstyle (I)}_{\scriptscriptstyle i}\in \vv{\bm{po}}'^{\scriptscriptstyle (I)}$ contains $n$ random values sampled uniformly from the same field. Since the blinded values and random values are not distinguishable, the elements of vectors $\vv{\bm{po}}^{\scriptscriptstyle (I)}$ and $\vv{\bm{po}}'^{\scriptscriptstyle (I)}$ are indistinguishable  too. Also,  labels  $l^{\scriptscriptstyle (I)}_{\scriptscriptstyle i} \in \vv{\bm{pl}}^{\scriptscriptstyle (I)}$ and $l'^{\scriptscriptstyle (I)}_{\scriptscriptstyle i} \in \vv{\bm{pl}}'^{\scriptscriptstyle (I)}$, ($\forall i, 1\leq i\leq h$ and $\forall I, I\in \{A,B\}$), are the outputs of a pseudorandom function and they are indistinguishable. Therefore, the elements of vectors $\vv{\bm{pl}}^{\scriptscriptstyle (I)}$ and $\vv{\bm{pl}}'^{\scriptscriptstyle (I)}$ are indistinguishable. Furthermore, since a pseudorandom permutation is indistinguishable from a  random permutation,  permuted vectors $\vv{\bm{po}}^{\scriptscriptstyle (I)}$ and $\vv{\bm{pl}}^{\scriptscriptstyle (I)} $, in the real model, and permuted vectors $\vv{\bm{po}}'^{\scriptscriptstyle (I)}$ and $\vv{\bm{pl}}'^{\scriptscriptstyle (I)} $, in the ideal model, are indistinguishable.


Since  sequence $ Q'_{\scriptscriptstyle 1}, ..., Q'_{\scriptscriptstyle \Upsilon}$ is generated given the leakage function, its access and query patterns are identical to the access and query patterns of $Q_{\scriptscriptstyle 1}, ..., Q_{\scriptscriptstyle \Upsilon}$.  Now we show that $Q_{\scriptscriptstyle i}$ is indistinguishable from $Q'_{\scriptscriptstyle i}$, ($\forall i, 1\leq i\leq \Upsilon$). First we consider the  case where $T_{\scriptscriptstyle i}= \textsf {\scriptsize PSI-Com}$. In this case,  keys $tk^{\scriptscriptstyle (I)}$ and $tk'^{\scriptscriptstyle (I)}$, ($\forall I, I\in \{A,B\}$), are random values, so they are indistinguishable. Also,  messages $\textsf {\scriptsize \textbf{ID}}^{\scriptscriptstyle  (A)}, \textsf {\scriptsize \textbf{ID}}^{\scriptscriptstyle  (B)}$ and $\textsf {\scriptsize \textbf{Compute}}$ are identical in both views.  Moreover, in the real model each pair in randomly permuted vector $\vv{\bm{pm}}_{\scriptscriptstyle \mathtt{ A \rightarrow B}}$ has the form $(l^{\scriptscriptstyle  (A)}_{\scriptscriptstyle g},l^{\scriptscriptstyle  (B)}_{\scriptscriptstyle g})$ where ($\forall g, 1\leq g\leq h $ and $\forall I, I \in \{A,B\}$) $l^{\scriptscriptstyle (I)}_{\scriptscriptstyle g} \in \vv{\bm{l}}^{\scriptscriptstyle (I)}$ and each $l^{\scriptscriptstyle (I)}_{\scriptscriptstyle g}$ is a pseudorandom string. Similarly, in the ideal model each pair in randomly permuted vector  $\vv{\bm{pm}}'_{\scriptscriptstyle \mathtt{ A \rightarrow B}}$ has the form $(l'^{\scriptscriptstyle  (A)}_{\scriptscriptstyle g'},l'^{\scriptscriptstyle  (B)}_{\scriptscriptstyle g'})$ where  $l'^{\scriptscriptstyle (I)}_{\scriptscriptstyle g'} \in \vv{\bm{l}}'^{\scriptscriptstyle (I)}$ and each $l'^{\scriptscriptstyle (I)}_{\scriptscriptstyle g'}$ is a pseudorandom string, so   $\vv{\bm{pm}}_{\scriptscriptstyle \mathtt{ A \rightarrow B}}$  and  $\vv{\bm{pm}}'_{\scriptscriptstyle \mathtt{ A \rightarrow B}}$  are indistinguishable.      Hence,  $Q_{\scriptscriptstyle i}$ is indistinguishable from $Q'_{\scriptscriptstyle i}$.


Now we move on to the case where $T_{\scriptscriptstyle i}= \textsf {\scriptsize Upd}^{\scriptscriptstyle (I)}_{\scriptscriptstyle t}$. In the real model, $\vv{\bm{o}}^{\scriptscriptstyle (I)}_{\scriptscriptstyle j,c^{ {\text{\tiny (\textit{I})}}}_{\tiny j}}$ contains $n$ elements blinded with pseudorandom values, while in the ideal model $\vv{\bm{o}}''^{\scriptscriptstyle (I)}$ comprises  $n$ random values. Since the random values and blinded values are  indistinguishable  vectors $\vv{\bm{o}}^{\scriptscriptstyle (I)}_{\scriptscriptstyle j,c^{ {\text{\tiny (\textit{I})}}}_{\tiny j}}$ and $\vv{\bm{o}}''^{\scriptscriptstyle (I)}$ are indistinguishable. In the real model, $l^{\scriptscriptstyle (I)}_{\scriptscriptstyle j}$ is a pseudorandom string and it belongs to vector $\vv{\bm{l}}^{\scriptscriptstyle (I)}$. In the ideal model, $l'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j}$ is a pseudorandom string and it belongs to vector $\vv{\bm{l}}'^{\scriptscriptstyle (I)}$. Therefore, the labels have the same distribution and are   indistinguishable. Also,  message $\textsf {\scriptsize \textbf{Update}}$ is identical in both models. So, $Q'_{\scriptscriptstyle i}$ and $Q_{\scriptscriptstyle i}$ are indistinguishable in this case too. From the above, we conclude that the views are indistinguishable. 

\
\vspace{-2mm}

\noindent\textbf{Case 2: Corrupted Client $B$.} In the real execution client $B$'s view is defined as:
\begin{equation*}
 \textsf {\scriptsize VIEW}^{\scriptscriptstyle\textsf { D-PSI}}_{\scriptscriptstyle B}(\Lambda, S^{\scriptscriptstyle (A)},S^{\scriptscriptstyle (B)})=\{S^{\scriptscriptstyle (B)}, r_{\scriptscriptstyle B}, \vv{\bm{q}}, \vv{\bm{f}}, f_{\scriptscriptstyle \cap}(S^{\scriptscriptstyle (A)},S^{\scriptscriptstyle (B)})\}. 
\end{equation*}

The simulator $\textsf {\scriptsize SIM}_{\scriptscriptstyle B}$ who receives $pk^{\scriptscriptstyle (B)}, lk^{\scriptscriptstyle (B)}, S^{\scriptscriptstyle (B)}$ and $f_{\scriptscriptstyle \cap}(S^{\scriptscriptstyle (A)},S^{\scriptscriptstyle (B)})$) does the following: 
\begin{packed_enum}
\item Creates an empty view, and appends $S^{\scriptscriptstyle (B)}$ and  uniformly at random chosen coins $r'_{\scriptscriptstyle B}$ to it. Then, it chooses two sets $S'^{\scriptscriptstyle (A)}$ and $S'^{\scriptscriptstyle (B)}$ such that $S'^{\scriptscriptstyle (A)}\cap S'^{\scriptscriptstyle (B)}=f_{\scriptscriptstyle \cap}(S^{\scriptscriptstyle (A)},S^{\scriptscriptstyle (B)})$ and $|S'^{\scriptscriptstyle (A)}|$, $|S'^{\scriptscriptstyle (B)}|\leq c$. 

\item Constructs  $\mathtt{HT}'^{\scriptscriptstyle(A)}$ and $\mathtt{HT}'^{\scriptscriptstyle(B)}$ using the public parameters. Next, it maps the elements in  $S'^{\scriptscriptstyle (A)}$ and $S'^{\scriptscriptstyle (B)}$ to the bins of $\mathtt{HT}'^{\scriptscriptstyle(A)}$ and $\mathtt{HT}'^{\scriptscriptstyle(B)}$, respectively. $\forall I, I\in \{A,B\}$ and $\forall s'^{\scriptscriptstyle (I)}_{\scriptscriptstyle i}\in S'^{\scriptscriptstyle (I)}$: $\mathtt{H}( s'^{\scriptscriptstyle (I)}_{\scriptscriptstyle i})=j$, then $ s'^{\scriptscriptstyle (I)}_{\scriptscriptstyle i}\rightarrow \mathtt{HT}'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j}$, where $1\leq j \leq h$.


\item Constructs  a polynomial representing the $d$ elements of each bin. If a bin contains less than $d$ elements first it is  padded with random values  to $d$ elements. $\forall I, I\in \{A,B\}$ and $\forall j, 1\leq j \leq h$: $\tau'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j}(x)=\prod\limits ^{\scriptscriptstyle d}_{\scriptscriptstyle m=1}(x-e_{\scriptscriptstyle m}^{\scriptscriptstyle (I)})$, where $e^{\scriptscriptstyle (I)}_{\scriptscriptstyle m} \in \mathtt{HT}'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j}$.

% (i.e. $e^{\scriptscriptstyle (I)}_{\scriptscriptstyle i}=s'^{\scriptscriptstyle (I)}_{\scriptscriptstyle i} $ or $e^{\scriptscriptstyle (I)}_{\scriptscriptstyle i}=r'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j,i}$).

\item Assigns a random polynomial $\omega'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j}$ of degree $d$ to each bin $\mathtt{HT}'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j}$ ( $\forall I, I \in \{A,B\}$). Next, it constructs  vectors $\vv{\bm{f}}'_{\scriptscriptstyle j}$ whose elements are computed as $\forall j, 1\leq j\leq h$ and $\forall i, 1\leq i\leq n$: $f'_{\scriptscriptstyle j,i}=\tau'^{\scriptscriptstyle (A)}_{\scriptscriptstyle j}(x_{\scriptscriptstyle i})\cdot  \omega'^{\scriptscriptstyle (A)}_{\scriptscriptstyle j}(x_{\scriptscriptstyle i})+\tau'^{\scriptscriptstyle (B)}_{\scriptscriptstyle j}(x_{\scriptscriptstyle i})\cdot  \omega'^{\scriptscriptstyle (B)}_{\scriptscriptstyle j}(x_{\scriptscriptstyle i})$, where $n=2d+1$.


%where $\tau'^{\scriptscriptstyle (I)}_{\scriptscriptstyle j}(x)$ represents the set elements mapped to that bin. 

%\item Pick a key $mk'$ and derive $h$ keys, $k'_{\scriptscriptstyle j}$, from it. 
%
%\
%
%\vspace{-2mm}
%\begin{center}
%$\forall j, 1\leq j\leq h: k'_{\scriptscriptstyle j}= \mathtt{PRF}(mk', j)$
%\end{center}
%\
%
%\vspace{-2mm}

%\item Use each key $k'_{\scriptscriptstyle j}$ to generate $\vv{\bm{q}}'_{\scriptscriptstyle j}$ whose elements are computed as follows.

\item Generates  vector $\vv{\bm{q}}'=[\vv{\bm{q}}'_{\scriptscriptstyle 1}, ...,  \vv{\bm{q}}'_{\scriptscriptstyle h}]$  where each vector $\vv{\bm{q}}'_{\scriptscriptstyle i}$ contains $n$ random values picked from  field $\mathbb{F}_p$. Then, it appends  $\vv{\bm{q}}''=\pi(pk^{\scriptscriptstyle (B)},\vv{\bm{q}}')$, $\vv{\bm{f}}''=\pi(pk^{\scriptscriptstyle (B)},\vv{\bm{f}}')$ and $f_{\scriptscriptstyle \cap}(S^{\scriptscriptstyle (A)},S^{\scriptscriptstyle (B)})$ to the view and outputs it.



%\
%
%\vspace{-2mm}
%\begin{center}
% $\forall j, 1\leq j\leq h$ and $\forall i, 1\leq i\leq n$: $q'_{\scriptscriptstyle  j,i}= \mathtt{PRF}(k'_{\scriptscriptstyle j}, i)$
%\end{center}
%\
%
%\vspace{-2mm}


\end{packed_enum}






Now we show that the two views are computationally indistinguishable. The entries $S^{\scriptscriptstyle (B)}$ and $\Lambda$ are identical in both views.  In the real model, the elements in $\vv{\bm{q}}_{\scriptscriptstyle j}$ are blinded with pseudorandom values, so the blinded elements are uniformly random  values. On the other hand, in the ideal model the elements in $\vv{\bm{q}}'_{\scriptscriptstyle j}$ are random values drawn from the same field. Moreover, both vectors are permuted in the same way. Hence, the vectors $\vv{\bm{q}}$ and  $\vv{\bm{q}}'$ are computationally indistinguishable. 


Furthermore, in the real model, given each unblinded vector $\vv{\bm{f}}_{\scriptscriptstyle j}$, the adversary interpolates a $2d$-degree polynomial of the form $\phi_{\scriptscriptstyle j}(x)=\omega^{\scriptscriptstyle (A)}_{\scriptscriptstyle j}(x)\cdot \tau^{\scriptscriptstyle (A)}_{\scriptscriptstyle j}(x)+\omega^{\scriptscriptstyle (B)}_{\scriptscriptstyle j}(x)\cdot \tau^{\scriptscriptstyle (B)}_{\scriptscriptstyle j}(x)=\mu_{\scriptscriptstyle j}\cdot gcd(\tau^{\scriptscriptstyle (A)}_{\scriptscriptstyle j}(x),\tau^{\scriptscriptstyle (B)}_{\scriptscriptstyle j}(x))$,   where polynomial $gcd(\tau^{\scriptscriptstyle (A)}_{\scriptscriptstyle j}(x),\tau^{\scriptscriptstyle (B)}_{\scriptscriptstyle j}(x))$ represents intersection of the sets  in the corresponding bin, $\mathtt{HT}_{\scriptscriptstyle j}$. Similarly, in the ideal model, each $2d$-degree polynomial $\phi'_{\scriptscriptstyle j}(x)$ interpolated from vector $\vv{\bm{f}}'_{\scriptscriptstyle j}$ has the form $\phi'_{\scriptscriptstyle j}(x)=\omega'^{\scriptscriptstyle (A)}_{\scriptscriptstyle j}(x)\cdot \tau'^{\scriptscriptstyle (A)}_{\scriptscriptstyle j}(x)+\omega'^{\scriptscriptstyle (B)}_{\scriptscriptstyle j}(x)\cdot \tau'^{\scriptscriptstyle (B)}_{\scriptscriptstyle j}(x)=\mu'_{\scriptscriptstyle j}\cdot gcd(\tau'^{\scriptscriptstyle (A)}_{\scriptscriptstyle j}(x),\tau'^{\scriptscriptstyle (B)}_{\scriptscriptstyle j}(x))$, where $gcd(\tau'^{\scriptscriptstyle (A)}_{\scriptscriptstyle j}(x),\tau'^{\scriptscriptstyle (B)}_{\scriptscriptstyle j}(x))$ represents the sets intersection in the corresponding bin, $\mathtt{HT}'_{\scriptscriptstyle j}$. Also, as we discussed in section \ref{sec::poly}, $\mu_{\scriptscriptstyle j}$ and $\mu'_{\scriptscriptstyle j}$ are  uniformly random polynomials and the probability that their roots represent  set elements is negligible, thus   $\phi_{\scriptscriptstyle j}(x)$ and $\phi'_{\scriptscriptstyle j}(x)$  only contain information about the set intersection and have the same distribution in both models  \cite{DBLP:conf/crypto/KissnerS05,BonehGHWW13}. Moreover, since the same hash table parameters were used, the same elements would reside in the same bins in both models, therefore  polynomials $gcd(\tau^{\scriptscriptstyle (A)}_{\scriptscriptstyle j}(x),\tau^{\scriptscriptstyle (B)}_{\scriptscriptstyle j}(x))$ and $gcd(\tau'^{\scriptscriptstyle (A)}_{\scriptscriptstyle j}(x),\tau'^{\scriptscriptstyle (B)}_{\scriptscriptstyle j}(x))$ represent the set elements of the  intersection for that bin.    Moreover, both vectors $\vv{\bm{f}}$ and $\vv{\bm{f}}'$ are permuted in the same way. So, $\vv{\bm{f}}$ and $\vv{\bm{f}}'$ are indistinguishable as well. Also, the output, $ f_{\scriptscriptstyle \cap}(S^{\scriptscriptstyle (A)},S^{\scriptscriptstyle (B)})$, is identical in both views. Thus,  the two views are computationally indistinguishable. 



\
\vspace{-2mm}

\noindent\textbf{Case 3: Corrupted Client $A$.} In the real execution client $A$'s view is defined as: 
\begin{equation*}
 \textsf {\scriptsize VIEW}^{\scriptscriptstyle\textsf { D-PSI}}_{\scriptscriptstyle A}(\Lambda, S^{\scriptscriptstyle (A)},S^{\scriptscriptstyle (B)})=\{S^{\scriptscriptstyle (A)}, r_{\scriptscriptstyle A}, lk^{\scriptscriptstyle (B)}, pk^{\scriptscriptstyle (B)}, \vv{\bm{r}}^{\scriptscriptstyle (B)},  \textsf {\scriptsize \textbf{ID}}^{\scriptscriptstyle  (B)}, \Lambda \}. 
\end{equation*}


The simulator, $\textsf {\scriptsize SIM}_{\scriptscriptstyle A}$, who receives $S^{\scriptscriptstyle (A)}$ performs as follows. It constructs an empty view, and adds $S^{\scriptscriptstyle (A)}$ and  uniformly at random chosen coins $r'_{\scriptscriptstyle A}$ to the view. It picks two random keys $lk'^{\scriptscriptstyle (B)}$, $pk'^{\scriptscriptstyle (B)}$ and  adds them to the view. Then, it constructs $\vv{\bm{r}}'^{\scriptscriptstyle (B)}=[\vv{\bm{r}}'^{\scriptscriptstyle (B)}_{\scriptscriptstyle 1}, ..., \vv{\bm{r}}'^{\scriptscriptstyle (B)}_{\scriptscriptstyle h}]$, where each vector $\vv{\bm{r}}'^{\scriptscriptstyle (B)}_{\scriptscriptstyle i}$ contains $n$ random values picked from the field. It also appends $\vv{\bm{r}}'^{\scriptscriptstyle (B)}$, $\textsf {\scriptsize \textbf{ID}}^{\scriptscriptstyle  (B)}$ and  $\Lambda$ to the view and outputs the view.

In the following, we will show why the two views are indistinguishable. In both views, $S^{\scriptscriptstyle (A)}, \textsf {\scriptsize \textbf{ID}}^{\scriptscriptstyle  (B)}$ and $\Lambda$ are identical.  Also $r_{\scriptscriptstyle A}$ and $r'_{\scriptscriptstyle A}$ are chosen uniformly at random so they are indistinguishable. Moreover,  values $lk^{\scriptscriptstyle (B)}, pk^{\scriptscriptstyle (B)}, lk'^{\scriptscriptstyle (B)}$ and $pk'^{\scriptscriptstyle (B)}$ are the keys picked uniformly at random, so they are indistinguishable, too. In the real model,  each vector $\vv{\bm{r}}^{\scriptscriptstyle (B)}_{\scriptscriptstyle i}$ contains $n$ values blinded with pseudorandom values. On the other hand, in the ideal model, each vector $\vv{\bm{r}}'^{\scriptscriptstyle (B)}_{\scriptscriptstyle i}$ comprises $n$ random elements of the field. Since the random values and blinded values are indistinguishable,  vectors $\vv{\bm{r}}^{\scriptscriptstyle (B)}$ and $\vv{\bm{r}}'^{\scriptscriptstyle (B)}$ are indistinguishable. Hence, the two views are indistinguishable. 
\end{proof}

\vspace{-3mm}

==> smart-PSI.tex <==
% !TEX root =U-PSI.tex

\section{Smart PSI}


In this section we provide smart PSI, a smart contract based private set intersection that charges the result recipients based on the number of set elements it learns. Here we consider stronger adversaries, economically rational semi-honest adversaries, who try to deviates from the protocol if doing so has let them gain some financial benefits. In the protocol, in addition to the roles in the previous protocol,   the is another role called: seller client who charges the result recipient client for the number of elements it learns. We assume that this client does not collude with the result recipient so the result recipient would bribe it and send other clients share to this client. Also, we do not consider fairness here, where either all clients must learn the result or no one. In this protocol, only client $B$ is interested in the intersection result. 

\begin{enumerate}
\item \textbf{Offline Phase} 

\begin{enumerate}
%\item It runs the off line phase in the previous advance protocol

\item\label{smart-contract-agreement} All clients, in $\{\resizeT {\textit A}_{\resizeS {\textit  1}},..., \resizeT {\textit A}_{\resizeS {\textit  m}},\resizeT {\textit  D}_{\resizeS {\textit  1}},\resizeT {\textit  D}_{\resizeS {\textit  2}}, B\}$, agree on a smart contract: $\mathcal{SC}$, provided in Fig. \ref{}. The smart contract is deployed by one of the clients and the address is given to the rest. All clients check the contract, if any client does not agree on the contract, it aborts. Otherwise, it proceeds to the next steps. 


\item\label{randomizing-elements} All clients, agree on  a pseudorandom permutation function, $\mathtt{PRP}$, and fresh secret key, $k_{\scriptscriptstyle o}$, for the function.  Then, each client $I \in \{\resizeT {\textit A}_{\resizeS {\textit  1}},..., \resizeT {\textit A}_{\resizeS {\textit  m}},\resizeT {\textit  D}_{\resizeS {\textit  1}},\resizeT {\textit  D}_{\resizeS {\textit  2}}, B\}$  uses $\mathtt{PRP}$ and the key to map its set elements to random values, as follows. $\forall i, 1\leq i\leq d: v^{\scriptscriptstyle I}_{\scriptscriptstyle i}=\mathtt{PRP}(k_{\scriptscriptstyle o}, s^{\scriptscriptstyle I}_{\scriptscriptstyle i})$. It considers  these encrypted values, $\vv{\bm{v}}^{\scriptscriptstyle I}=\{v^{\scriptscriptstyle I}_{\scriptscriptstyle 1},..,v^{\scriptscriptstyle I}_{\scriptscriptstyle d}\}$, as its set elements. Note that $\mathtt{PRP}$ is deterministic and also the client can always decrypt $v^{\scriptscriptstyle I}_{\scriptscriptstyle i}$ to get its actual set element: $s^{\scriptscriptstyle I}_{\scriptscriptstyle i}=\mathtt{PRP}^{\scriptscriptstyle -1}(k_{\scriptscriptstyle o}, v^{\scriptscriptstyle I}_{\scriptscriptstyle i})$

\item All clients, excluding  $B$, agree on  a \emph{seller} client: $\resizeT {\textit A}_{\resizeS {\textit  s}}$, who  can be any client, e.g. a client with smallest set size;  except  the result recipient, client $B$. 

\item All clients, including the seller,  run the Offline Phase as in previous protocol, where their inputs are the encrypted values computed in step \ref{randomizing-elements}. However, there are two   differences:  (a) the seller in step \ref{offline-autho-param} also picks a fresh key $k_{\scriptscriptstyle s}$ for the $\mathtt{PRF}$, and (b) the seller   in step \ref{offlinedealerrerand}, first picks a random polynomial $\beta(x)$ of degree $2d$ and then then computes: 

$\forall i, 1\leq i \leq n : c^{\resizeS {\textit  A}_{\resizeSS {\textit  s}}}_{\scriptscriptstyle i}     = \omega^{\resizeS {\textit  A}_{\resizeSS {\textit  s}}}_{\scriptscriptstyle i}   \cdot \pi^{\resizeS {\textit  A}_{\resizeSS {\textit  s}}}_{\scriptscriptstyle i}+\sum\limits^{\scriptscriptstyle 2}_{\scriptscriptstyle v=1} r^{\resizeS{\textit A}_{\resizeSS{\textit s}}\resizeS{,}  \resizeS { \textit D}_{\resizeSS {\textit v}}}_{\scriptscriptstyle i} +\sum\limits^{\scriptscriptstyle 2}_{\scriptscriptstyle v=1} q^{\resizeS{\textit A}_{\resizeSS{\textit s}}\resizeS{,}  \resizeS { \textit D}_{\resizeSS {\textit v}}}_{\scriptscriptstyle i}+ \beta_{\scriptscriptstyle i}$

where  $r^{\resizeS{\textit A}_{\resizeSS{\textit s}}\resizeS{,}  \resizeS { \textit D}_{\resizeSS {\textit v}}}_{\scriptscriptstyle i}=\PRF(k^{\resizeS{\textit A}_{\resizeSS{\textit s}}\resizeS{,}  \resizeS { \textit D}_{\resizeSS {\textit v}}},i),\ q^{\resizeS{\textit A}_{\resizeSS{\textit s}}\resizeS{,}  \resizeS { \textit D}_{\resizeSS {\textit v}}}_{\scriptscriptstyle i}=\PRF(l^{\resizeS{\textit A}_{\resizeSS{\textit s}}\resizeS{,}  \resizeS { \textit D}_{\resizeSS {\textit v}}},i)$, $\beta_{i}=\beta(x_{\scriptscriptstyle i})$ and $1\leq v\leq 2$. Note that, if the seller is one of the dealers, e.g. $\resizeT {\textit  D}_{\resizeS {\textit v}}$, it computes the following value instead:  $\forall i, 1\leq i \leq n : c^{\resizeS {\textit  D}_{\resizeSS {\textit  v}}}_{\scriptscriptstyle i}     = \omega^{\resizeS {\textit  D}_{\resizeSS {\textit  v}}}_{\scriptscriptstyle i}   \cdot \pi^{\resizeS {\textit  D}_{\resizeSS {\textit  v}}}_{\scriptscriptstyle i}+\sum\limits^{\scriptscriptstyle 2}_{\scriptscriptstyle p=1} r^{\resizeS{\textit D}_{\resizeSS{\textit v}}\resizeS{,}  \resizeS { \textit A}_{\resizeSS {\textit p}}}_{\scriptscriptstyle i} +\sum\limits^{\scriptscriptstyle 2}_{\scriptscriptstyle p=1} q^{\resizeS{\textit D}_{\resizeSS{\textit v}}\resizeS{,}  \resizeS { \textit A}_{\resizeSS {\textit p}}}_{\scriptscriptstyle i}+ \beta_{\scriptscriptstyle i}$

where  $r^{\resizeS{\textit D}_{\resizeSS{\textit v}}\resizeS{,}  \resizeS { \textit A}_{\resizeSS {\textit p}}}_{\scriptscriptstyle i}=\PRF(k^{\resizeS{\textit D}_{\resizeSS{\textit v}}\resizeS{,}  \resizeS { \textit A}_{\resizeSS {\textit p}}},i),\ q^{\resizeS{\textit D}_{\resizeSS{\textit v}}\resizeS{,}  \resizeS { \textit A}_{\resizeSS {\textit p}}}_{\scriptscriptstyle i}=\PRF(l^{\resizeS{\textit D}_{\resizeSS{\textit v}}\resizeS{,}  \resizeS { \textit A}_{\resizeSS {\textit p}}},i)$,  $\beta_{i}=\beta(x_{\scriptscriptstyle i})$ and $1\leq p\leq 2$ 

\end{enumerate}

\item \textbf{Online Phase} 



\begin{enumerate}
\item All clients, excluding   $B$, agree on parameter $c$: the maximum number of elements in the intersection that will be  sold/revealed to client $B$. Value $c$ is registered on $\mathcal{SC}$. To agree on value $c$, they can either negotiate out-of-the-bound or  use a voting scheme, e.g. by using a combination of commitment scheme and smart contract. See Appendix \ref{} for more detail.

\item Client $B$ deposites $e\cdot c$ coin to the smart contract, $\mathcal{SC}$. The seller client, $\resizeT {\textit A}_{\resizeS {\textit  s}}$,  checks if $e\cdot c$ coin has been deposited to the contract. If not, it aborts and ask other clients to abort too. Otherwise, it commits to: the evaluation of the random polynomial, $\beta(x)$, at every element in $\vv{\bm{v}}^{\resizeS {\textit  A}_{\resizeSS {\textit  s}}}=\{v^{\resizeS {\textit  A}_{\resizeSS {\textit  s}}}_{\scriptscriptstyle 1},..,v^{\resizeS {\textit  A}_{\resizeSS {\textit  s}}}_{\scriptscriptstyle d}\}$.  In particular:  $\forall i, 1\leq i \leq d: t_{\scriptscriptstyle i}=\mathtt{PRF}(k_{\scriptscriptstyle s},v^{\resizeS {\textit  A}_{\resizeSS {\textit  s}}}_{\scriptscriptstyle i}),  h_{\scriptscriptstyle i}= \mathtt{H}(\beta(v^{\resizeS {\textit  A}_{\resizeSS {\textit  s}}}_{\scriptscriptstyle i})\ || \ t_{\scriptscriptstyle i})$.  Next, $\resizeT {\textit A}_{\resizeS {\textit  s}}$ stores the committed values: $h_{\scriptscriptstyle i}$'s, in the contract. 

\item All clients, take the same steps as in steps \ref{clientBkeydist}-\ref{assistant-side-result-computation} in Online Phase in Fig.\ref{}. The only  difference is that the clients  (in steps \ref{authorizer-side-result-computation}, \ref{dealer-side-result-computation}, and \ref{assistant-side-result-computation}) send the messages to  smart contract $\mathcal{SC}$ instead of client $B$. 

\item Contract $\mathcal{SC}$ combines all clients' messages to remove all blinding factors. $\forall i, 1\leq i \leq n :$

$e_{\scriptscriptstyle i}=\sum\limits^{\scriptscriptstyle m}_{\scriptscriptstyle j=1} o^{\resizeS {\textit  A}_{\resizeSS {\textit  j}}}_{\scriptscriptstyle i}+ \sum\limits^{\scriptscriptstyle 2}_{\scriptscriptstyle v=1} o^{\resizeS {\textit  D}_{\resizeSS {\textit  v}}}_{\scriptscriptstyle i}$


\ \  \ \  \ $=\sum\limits^{\scriptscriptstyle m}_{\scriptscriptstyle j=1} (\omega^{\resizeS {\textit  A}_{\resizeSS {\textit  j}}}_{\scriptscriptstyle i}   \cdot \pi^{\resizeS {\textit  A}_{\resizeSS {\textit  j}}}_{\scriptscriptstyle i})+\sum\limits^{\scriptscriptstyle 2}_{\scriptscriptstyle v=1} (\omega^{\resizeS {\textit  D}_{\resizeSS {\textit  v}}}_{\scriptscriptstyle i}   \cdot \pi^{\resizeS {\textit  D}_{\resizeSS {\textit  v}}}_{\scriptscriptstyle i})+  \pi^{\resizeS {\textit B} }_{\scriptscriptstyle i}\cdot(\sum\limits^{\scriptscriptstyle m}_{\scriptscriptstyle j=1} (\zeta^{\resizeS{\textit A}_{\resizeSS{\textit j}}\resizeS{,}  \resizeS { \textit D}_{\resizeSS {\textit 1}}}_{\scriptscriptstyle i}+\zeta^{\resizeS{\textit A}_{\resizeSS{\textit j}}\resizeS{,}  \resizeS { \textit D}_{\resizeSS {\textit 2}}}_{\scriptscriptstyle i})+\sum\limits^{\scriptscriptstyle 2}_{\scriptscriptstyle v=1} (\zeta^{\resizeS{\textit D}_{\resizeSS{\textit v}}\resizeS{,}  \resizeS { \textit A}_{\resizeSS {\textit 1}}}_{\scriptscriptstyle i}+\zeta^{\resizeS{\textit D}_{\resizeSS{\textit v}}\resizeS{,}  \resizeS { \textit A}_{\resizeSS {\textit 2}}}_{\scriptscriptstyle i}))+\beta_{\scriptscriptstyle i}$

\item The contract uses $n$ pairs: $(z_{\scriptscriptstyle i}, e_{\scriptscriptstyle i})$ to interpolate a randomised polynomial: $\xi(x)$. The polynomial is of the form: $\xi(x)=\psi(x)+\beta(x)$, where $\psi(x)$ represents the intersection   and $\beta(x)$ is a uniformly random polynomial picked by the seller. 

\item Client $\resizeT {\textit A}_{\resizeS {\textit  s}}$ \emph{locally}  removes the random polynomial from $\xi(x)$ and  then, evaluates the result polynomial: $\psi(x)$, at every element of its encrypted set: $v^{\resizeS {\textit  A}_{\resizeSS {\textit  s}}}_{\scriptscriptstyle t}\in \vv{\bm{v}}^{\resizeS {\textit  A}_{\resizeSS {\textit s}}}$ ($\forall t, 1\leq t \leq d$). It considers the element in the intersection if the result of the polynomial evaluation is zero, i.e. if $\psi(v^{\resizeS {\textit  A}_{\resizeSS {\textit  s}}}_{\scriptscriptstyle t})=0$.

\item Client $\resizeT {\textit A}_{\resizeS {\textit  s}}$ sends the opening of (at most) $c$ elements in the intersection to the contract. In particular, it sends the following values to $\mathcal{SC}$. $\forall i, 1\leq i\leq c: (t_{\scriptscriptstyle i},v^{\resizeS {\textit  A}_{\resizeSS {\textit  s}}}_{\scriptscriptstyle i})$,  where $\psi(v^{\resizeS {\textit  A}_{\resizeSS {\textit  s}}}_{\scriptscriptstyle i})=0$.

\item Contract $\mathcal{SC}$, given $c$ pairs of $(t_{\scriptscriptstyle i},v^{\resizeS {\textit  A}_{\resizeSS {\textit  s}}}_{\scriptscriptstyle i})$,  performs as follows. $\forall 1\leq i\leq c:$ 
\begin{enumerate}
 \item evaluates  $\xi(x)$ at every element  $\resizeT {\textit A}_{\resizeS {\textit  s}}$ has sent: $\xi(v^{\resizeS {\textit  A}_{\resizeSS {\textit  s}}}_{\scriptscriptstyle i})=\psi(v^{\resizeS {\textit  A}_{\resizeSS {\textit  s}}}_{\scriptscriptstyle i})+\beta(v^{\resizeS {\textit  A}_{\resizeSS {\textit  s}}}_{\scriptscriptstyle i})$
 \item verifies if the polynomial evaluations matches the committed values already stored in the contract. $ \mathtt{H}(\xi(v^{\resizeS {\textit  A}_{\resizeSS {\textit  s}}}_{\scriptscriptstyle i}) \ || \ t_{\scriptscriptstyle i})\stackrel{\scriptscriptstyle ?}=h_{\scriptscriptstyle i}$.  If passed, it sends a share to every client in  $\{\resizeT {\textit A}_{\resizeS {\textit  1}},..., \resizeT {\textit A}_{\resizeS {\textit  m}},\resizeT {\textit  D}_{\resizeS {\textit  1}},\resizeT {\textit  D}_{\resizeS {\textit  2}}\}$. 
 
\end{enumerate}


\end{enumerate}
\end{enumerate}










